GRACE: Loss-Resilient Real-Time Video through Neural Codecs

In real-time video communication, retransmitting lost packets over high-latency networks is not viable due to strict latency requirements. To counter packet losses without retransmission, two primary strategies are employed -- encoder-based forward error correction (FEC) and decoder-based error concealment. The former encodes data with redundancy before transmission, yet determining the optimal redundancy level in advance proves challenging. The latter reconstructs video from partially received frames, but dividing a frame into independently coded partitions inherently compromises compression efficiency, and the lost information cannot be effectively recovered by the decoder without adapting the encoder. We present a loss-resilient real-time video system called GRACE, which preserves the user's quality of experience (QoE) across a wide range of packet losses through a new neural video codec. Central to GRACE's enhanced loss resilience is its joint training of the neural encoder and decoder under a spectrum of simulated packet losses. In lossless scenarios, GRACE achieves video quality on par with conventional codecs (e.g., H.265). As the loss rate escalates, GRACE exhibits a more graceful, less pronounced decline in quality, consistently outperforming other loss-resilient schemes. Through extensive evaluation on various videos and real network traces, we demonstrate that GRACE reduces undecodable frames by 95% and stall duration by 90% compared with FEC, while markedly boosting video quality over error concealment methods. In a user study with 240 crowdsourced participants and 960 subjective ratings, GRACE registers a 38% higher mean opinion score (MOS) than other baselines.

==> latexrun <==
#!/usr/bin/env python3

# Copyright (c) 2013, 2014 Austin Clements

# Permission is hereby granted, free of charge, to any person obtaining a copy
# of this software and associated documentation files (the "Software"), to deal
# in the Software without restriction, including without limitation the rights
# to use, copy, modify, merge, publish, distribute, sublicense, and/or sell
# copies of the Software, and to permit persons to whom the Software is
# furnished to do so, subject to the following conditions:

# The above copyright notice and this permission notice shall be included in
# all copies or substantial portions of the Software.

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
# IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
# FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN NO EVENT SHALL THE
# AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER
# LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM,
# OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN
# THE SOFTWARE.

import sys
import os
import errno
import argparse
import shlex
import json
import subprocess
import re
import collections
import hashlib
import shutil
import curses
import filecmp
import io
import traceback
import time

try:
    import fcntl
except ImportError:
    # Non-UNIX platform
    fcntl = None

def debug(string, *args):
    if debug.enabled:
        print(string.format(*args), file=sys.stderr)
debug.enabled = False

def debug_exc():
    if debug.enabled:
        traceback.print_exc()

def main():
    # Parse command-line
    arg_parser = argparse.ArgumentParser(
        description='''A 21st century LaTeX wrapper,
        %(prog)s runs latex (and bibtex) the right number of times so you
        don't have to,
        strips the log spew to make errors visible,
        and plays well with standard build tools.''')
    arg_parser.add_argument(
        '-o', metavar='FILE', dest='output', default=None,
        help='Output file name (default: derived from input file)')
    arg_parser.add_argument(
        '--latex-cmd', metavar='CMD', default='pdflatex',
        help='Latex command (default: %(default)s)')
    arg_parser.add_argument(
        '--latex-args', metavar='ARGS', type=arg_parser_shlex,
        help='Additional command-line arguments for latex.'
        ' This will be parsed and split using POSIX shell rules.')
    arg_parser.add_argument(
        '--bibtex-cmd', metavar='CMD', default='bibtex',
        help='Bibtex command (default: %(default)s)')
    arg_parser.add_argument(
        '--bibtex-args', metavar='ARGS', type=arg_parser_shlex,
        help='Additional command-line arguments for bibtex')
    arg_parser.add_argument(
        '--max-iterations', metavar='N', type=int, default=10,
        help='Max number of times to run latex before giving up'
        ' (default: %(default)s)')
    arg_parser.add_argument(
        '-W', metavar='(no-)CLASS',
        action=ArgParserWarnAction, dest='nowarns', default=set(['underfull']),
        help='Enable/disable warning from CLASS, which can be any package name, '
        'LaTeX warning class (e.g., font), bad box type '
        '(underfull, overfull, loose, tight), or "all"')
    arg_parser.add_argument(
        '-O', metavar='DIR', dest='obj_dir', default='latex.out',
        help='Directory for intermediate files and control database '
        '(default: %(default)s)')
    arg_parser.add_argument(
        '--color', choices=('auto', 'always', 'never'), default='auto',
        help='When to colorize messages')
    arg_parser.add_argument(
        '--verbose-cmds', action='store_true', default=False,
        help='Print commands as they are executed')
    arg_parser.add_argument(
        '--debug', action='store_true',
        help='Enable detailed debug output')
    actions = arg_parser.add_argument_group('actions')
    actions.add_argument(
        '--clean-all', action='store_true', help='Delete output files')
    actions.add_argument(
        'file', nargs='?', help='.tex file to compile')
    args = arg_parser.parse_args()
    if not any([args.clean_all, args.file]):
        arg_parser.error('at least one action is required')
    args.latex_args = args.latex_args or []
    args.bibtex_args = args.bibtex_args or []

    verbose_cmd.enabled = args.verbose_cmds
    debug.enabled = args.debug

    # A note about encodings: POSIX encoding is a mess; TeX encoding
    # is a disaster.  Our goal is to make things no worse, so we want
    # byte-accurate round-tripping of TeX messages.  Since TeX
    # messages are *basically* text, we use strings and
    # surrogateescape'ing for both input and output.  I'm not fond of
    # setting surrogateescape globally, but it's far easier than
    # dealing with every place we pass TeX output through.
    # Conveniently, JSON can round-trip surrogateescape'd strings, so
    # our control database doesn't need special handling.
    sys.stdout = io.TextIOWrapper(
        sys.stdout.buffer, encoding=sys.stdout.encoding,
        errors='surrogateescape', line_buffering=sys.stdout.line_buffering)
    sys.stderr = io.TextIOWrapper(
        sys.stderr.buffer, encoding=sys.stderr.encoding,
        errors='surrogateescape', line_buffering=sys.stderr.line_buffering)

    Message.setup_color(args.color)

    # Open control database.
    dbpath = os.path.join(args.obj_dir, '.latexrun.db')
    if not os.path.exists(dbpath) and os.path.exists('.latexrun.db'):
        # The control database used to live in the source directory.
        # Support this for backwards compatibility.
        dbpath = '.latexrun.db'
    try:
        db = DB(dbpath)
    except (ValueError, OSError) as e:
        print('error opening {}: {}'.format(e.filename if hasattr(e, 'filename')
                                            else dbpath, e),
              file=sys.stderr)
        debug_exc()
        sys.exit(1)

    # Clean
    if args.clean_all:
        try:
            db.do_clean(args.obj_dir)
        except OSError as e:
            print(e, file=sys.stderr)
            debug_exc()
            sys.exit(1)

    # Build
    if not args.file:
        return
    task_commit = None
    try:
        task_latex = LaTeX(db, args.file, args.latex_cmd, args.latex_args,
                           args.obj_dir, args.nowarns)
        task_commit = LaTeXCommit(db, task_latex, args.output)
        task_bibtex = BibTeX(db, task_latex, args.bibtex_cmd, args.bibtex_args,
                             args.nowarns, args.obj_dir)
        tasks = [task_latex, task_commit, task_bibtex]
        stable = run_tasks(tasks, args.max_iterations)

        # Print final task output and gather exit status
        status = 0
        for task in tasks:
            status = max(task.report(), status)

        if not stable:
            print('error: files are still changing after {} iterations; giving up'
                  .format(args.max_iterations), file=sys.stderr)
            status = max(status, 1)
    except TaskError as e:
        print(str(e), file=sys.stderr)
        debug_exc()
        status = 1

    # Report final status, if interesting
    fstatus = 'There were errors' if task_commit is None else task_commit.status
    if fstatus:
        output = args.output
        if output is None:
            if task_latex.get_outname() is not None:
                output = os.path.basename(task_latex.get_outname())
            else:
                output = 'output'
        if Message._color:
            terminfo.send('bold', ('setaf', 1))
        print('{}; {} not updated'.format(fstatus, output))
        if Message._color:
            terminfo.send('sgr0')
    sys.exit(status)

def arg_parser_shlex(string):
    """Argument parser for shell token lists."""
    try:
        return shlex.split(string)
    except ValueError as e:
        raise argparse.ArgumentTypeError(str(e)) from None

class ArgParserWarnAction(argparse.Action):
    def __call__(self, parser, namespace, value, option_string=None):
        nowarn = getattr(namespace, self.dest)
        if value == 'all':
            nowarn.clear()
        elif value.startswith('no-'):
            nowarn.add(value[3:])
        else:
            nowarn.discard(value)
        setattr(namespace, self.dest, nowarn)

def verbose_cmd(args, cwd=None, env=None):
    if verbose_cmd.enabled:
        cmd = ' '.join(map(shlex.quote, args))
        if cwd is not None:
            cmd = '(cd {} && {})'.format(shlex.quote(cwd), cmd)
        if env is not None:
            for k, v in env.items():
                if os.environ.get(k) != v:
                    cmd = '{}={} {}'.format(k, shlex.quote(v), cmd)
        print(cmd, file=sys.stderr)
verbose_cmd.enabled = False

def mkdir_p(path):
    try:
        os.makedirs(path)
    except OSError as exc:
        if exc.errno == errno.EEXIST and os.path.isdir(path):
            pass
        else: raise

class DB:
    """A latexrun control database."""

    _VERSION = 'latexrun-db-v2'

    def __init__(self, filename):
        self.__filename = filename

        # Make sure database directory exists
        if os.path.dirname(self.__filename):
            os.makedirs(os.path.dirname(self.__filename), exist_ok=True)

        # Lock the database if possible. We don't release this lock
        # until the process exits.
        lockpath = self.__filename + '.lock'
        if fcntl is not None:
            lockfd = os.open(lockpath, os.O_CREAT|os.O_WRONLY, 0o666)
            # Note that this is actually an fcntl lock, not a lockf
            # lock. Don't be fooled.
            fcntl.lockf(lockfd, fcntl.LOCK_EX, 1)

        try:
            fp = open(filename, 'r')
        except FileNotFoundError:
            debug('creating new database')
            self.__val = {'version': DB._VERSION}
        else:
            debug('loading database')
            self.__val = json.load(fp)
            if 'version' not in self.__val:
                raise ValueError('file exists, but does not appear to be a latexrun database'.format(filename))
            if self.__val['version'] != DB._VERSION:
                raise ValueError('unknown database version {!r}'
                                 .format(self.__val['version']))

    def commit(self):
        debug('committing database')
        # Atomically commit database
        tmp_filename = self.__filename + '.tmp'
        with open(tmp_filename, 'w') as fp:
            json.dump(self.__val, fp, indent=2, separators=(',', ': '))
            fp.flush()
            os.fsync(fp.fileno())
        os.rename(tmp_filename, self.__filename)

    def get_summary(self, task_id):
        """Return the recorded summary for the given task or None."""
        return self.__val.get('tasks', {}).get(task_id)

    def set_summary(self, task_id, summary):
        """Set the summary for the given task."""
        self.__val.setdefault('tasks', {})[task_id] = summary

    def add_clean(self, filename):
        """Add an output file to be cleaned.

        Unlike the output files recorded in the task summaries,
        cleanable files strictly accumulate until a clean is
        performed.
        """
        self.__val.setdefault('clean', {})[filename] = hash_cache.get(filename)

    def do_clean(self, obj_dir=None):
        """Remove output files and delete database.

        If obj_dir is not None and it is empty after all files are
        removed, it will also be removed.
        """

        for f, want_hash in self.__val.get('clean', {}).items():
            have_hash = hash_cache.get(f)
            if have_hash is not None:
                if want_hash == have_hash:
                    debug('unlinking {}', f)
                    hash_cache.invalidate(f)
                    os.unlink(f)
                else:
                    print('warning: {} has changed; not removing'.format(f),
                          file=sys.stderr)
        self.__val = {'version': DB._VERSION}
        try:
            os.unlink(self.__filename)
        except FileNotFoundError:
            pass
        if obj_dir is not None:
            try:
                os.rmdir(obj_dir)
            except OSError:
                pass

class HashCache:
    """Cache of file hashes.

    As latexrun reaches fixed-point, it hashes the same files over and
    over, many of which never change.  Since hashing is somewhat
    expensive, we keep a simple cache of these hashes.
    """

    def __init__(self):
        self.__cache = {}

    def get(self, filename):
        """Return the hash of filename, or * if it was clobbered."""
        try:
            with open(filename, 'rb') as fp:
                st = os.fstat(fp.fileno())
                key = (st.st_dev, st.st_ino)
                if key in self.__cache:
                    return self.__cache[key]

                debug('hashing {}', filename)
                h = hashlib.sha256()
                while True:
                    block = fp.read(256*1024)
                    if not len(block):
                        break
                    h.update(block)
                self.__cache[key] = h.hexdigest()
                return self.__cache[key]
        except (FileNotFoundError, IsADirectoryError):
            return None

    def clobber(self, filename):
        """If filename's hash is not known, record an invalid hash.

        This can be used when filename was overwritten before we were
        necessarily able to obtain its hash.  filename must exist.
        """
        st = os.stat(filename)
        key = (st.st_dev, st.st_ino)
        if key not in self.__cache:
            self.__cache[key] = '*'

    def invalidate(self, filename):
        try:
            st = os.stat(filename)
        except OSError as e:
            # Pessimistically wipe the whole cache
            debug('wiping hash cache ({})', e)
            self.__cache.clear()
        else:
            key = (st.st_dev, st.st_ino)
            if key in self.__cache:
                del self.__cache[key]
hash_cache = HashCache()

class _Terminfo:
    def __init__(self):
        self.__tty = os.isatty(sys.stdout.fileno())
        if self.__tty:
            curses.setupterm()
        self.__ti = {}

    def __ensure(self, cap):
        if cap not in self.__ti:
            if not self.__tty:
                string = None
            else:
                string = curses.tigetstr(cap)
                if string is None or b'$<' in string:
                    # Don't have this capability or it has a pause
                    string = None
            self.__ti[cap] = string
        return self.__ti[cap]

    def has(self, *caps):
        return all(self.__ensure(cap) is not None for cap in caps)

    def send(self, *caps):
        # Flush TextIOWrapper to the binary IO buffer
        sys.stdout.flush()
        for cap in caps:
            # We should use curses.putp here, but it's broken in
            # Python3 because it writes directly to C's buffered
            # stdout and there's no way to flush that.
            if isinstance(cap, tuple):
                s = curses.tparm(self.__ensure(cap[0]), *cap[1:])
            else:
                s = self.__ensure(cap)
            sys.stdout.buffer.write(s)
terminfo = _Terminfo()

class Progress:
    _enabled = None

    def __init__(self, prefix):
        self.__prefix = prefix
        if Progress._enabled is None:
            Progress._enabled = (not debug.enabled) and \
                                terminfo.has('cr', 'el', 'rmam', 'smam')

    def __enter__(self):
        self.last = ''
        self.update('')
        return self

    def __exit__(self, typ, value, traceback):
        if Progress._enabled:
            # Beginning of line and clear
            terminfo.send('cr', 'el')
            sys.stdout.flush()

    def update(self, msg):
        if not Progress._enabled:
            return
        out = '[' + self.__prefix + ']'
        if msg:
            out += ' ' + msg
        if out != self.last:
            # Beginning of line, clear line, disable wrap
            terminfo.send('cr', 'el', 'rmam')
            sys.stdout.write(out)
            # Enable wrap
            terminfo.send('smam')
            self.last = out
            sys.stdout.flush()

class Message(collections.namedtuple(
        'Message', 'typ filename lineno msg')):
    def emit(self):
        if self.filename:
            if self.filename.startswith('./'):
                finfo = self.filename[2:]
            else:
                finfo = self.filename
        else:
            finfo = '<no file>'
        if self.lineno is not None:
            finfo += ':' + str(self.lineno)
        finfo += ': '
        if self._color:
            terminfo.send('bold')
        sys.stdout.write(finfo)

        if self.typ != 'info':
            if self._color:
                terminfo.send(('setaf', 5 if self.typ == 'warning' else 1))
            sys.stdout.write(self.typ + ': ')
        if self._color:
            terminfo.send('sgr0')
        sys.stdout.write(self.msg + '\n')

    @classmethod
    def setup_color(cls, state):
        if state == 'never':
            cls._color = False
        elif state == 'always':
            cls._color = True
        elif state == 'auto':
            cls._color = terminfo.has('setaf', 'bold', 'sgr0')
        else:
            raise ValueError('Illegal color state {:r}'.format(state))


##################################################################
# Task framework
#

terminate_task_loop = False
start_time = time.time()

def run_tasks(tasks, max_iterations):
    """Execute tasks in round-robin order until all are stable.

    This will also exit if terminate_task_loop is true.  Tasks may use
    this to terminate after a fatal error (even if that fatal error
    doesn't necessarily indicate stability; as long as re-running the
    task will never eliminate the fatal error).

    Return True if fixed-point is reached or terminate_task_loop is
    set within max_iterations iterations.
    """

    global terminate_task_loop
    terminate_task_loop = False

    nstable = 0
    for iteration in range(max_iterations):
        for task in tasks:
            if task.stable():
                nstable += 1
                if nstable == len(tasks):
                    debug('fixed-point reached')
                    return True
            else:
                task.run()
                nstable = 0
                if terminate_task_loop:
                    debug('terminate_task_loop set')
                    return True
    debug('fixed-point not reached')
    return False

class TaskError(Exception):
    pass

class Task:
    """A deterministic computation whose inputs and outputs can be captured."""

    def __init__(self, db, task_id):
        self.__db = db
        self.__task_id = task_id

    def __debug(self, string, *args):
        if debug.enabled:
            debug('task {}: {}', self.__task_id, string.format(*args))

    def stable(self):
        """Return True if running this task will not affect system state.

        Functionally, let f be the task, and s be the system state.
        Then s' = f(s).  If it must be that s' == s (that is, f has
        reached a fixed point), then this function must return True.
        """
        last_summary = self.__db.get_summary(self.__task_id)
        if last_summary is None:
            # Task has never run, so running it will modify system
            # state
            changed = 'never run'
        else:
            # If any of the inputs have changed since the last run of
            # this task, the result may change, so re-run the task.
            # Also, it's possible something else changed an output
            # file, in which case we also want to re-run the task, so
            # check the outputs, too.
            changed = self.__summary_changed(last_summary)

        if changed:
            self.__debug('unstable (changed: {})', changed)
            return False
        else:
            self.__debug('stable')
            return True

    def __summary_changed(self, summary):
        """Test if any inputs changed from summary.

        Returns a string describing the changed input, or None.
        """
        for dep in summary['deps']:
            fn, args, val = dep
            method = getattr(self, '_input_' + fn, None)
            if method is None:
                return 'unknown dependency method {}'.format(fn)
            if method == self._input_unstable or method(*args) != val:
                return '{}{}'.format(fn, tuple(args))
        return None

    def _input(self, name, *args):
        """Register an input for this run.

        This calls self._input_<name>(*args) to get the value of this
        input.  This function should run quickly and return some
        projection of system state that affects the result of this
        computation.

        Both args and the return value must be JSON serializable.
        """
        method = getattr(self, '_input_' + name)
        val = method(*args)
        if [name, args, val] not in self.__deps:
            self.__deps.append([name, args, val])
        return val

    def run(self):
        # Before we run the task, pre-hash any files that were output
        # files in the last run.  These may be input by this run and
        # then clobbered, at which point it will be too late to get an
        # input hash.  Ideally we would only hash files that were
        # *both* input and output files, but latex doesn't tell us
        # about input files that didn't exist, so if we start from a
        # clean slate, we often require an extra run because we don't
        # know a file is input/output until after the second run.
        last_summary = self.__db.get_summary(self.__task_id)
        if last_summary is not None:
            for io_filename in last_summary['output_files']:
                self.__debug('pre-hashing {}', io_filename)
                hash_cache.get(io_filename)

        # Run the task
        self.__debug('running')
        self.__deps = []
        result = self._execute()

        # Clear cached output file hashes
        for filename in result.output_filenames:
            hash_cache.invalidate(filename)

        # If the output files change, then the computation needs to be
        # re-run, so record them as inputs
        for filename in result.output_filenames:
            self._input('file', filename)

        # Update task summary in database
        self.__db.set_summary(self.__task_id,
                              self.__make_summary(self.__deps, result))
        del self.__deps

        # Add output files to be cleaned
        for f in result.output_filenames:
            self.__db.add_clean(f)

        try:
            self.__db.commit()
        except OSError as e:
            raise TaskError('error committing control database {}: {}'.format(
                getattr(e, 'filename', '<unknown path>'), e)) from e

    def __make_summary(self, deps, run_result):
        """Construct a new task summary."""
        return {
            'deps': deps,
            'output_files': {f: hash_cache.get(f)
                             for f in run_result.output_filenames},
            'extra': run_result.extra,
        }

    def _execute(self):
        """Abstract: Execute this task.

        Subclasses should implement this method to execute this task.
        This method must return a RunResult giving the inputs that
        were used by the task and the outputs it produced.
        """
        raise NotImplementedError('Task._execute is abstract')

    def _get_result_extra(self):
        """Return the 'extra' result from the previous run, or None."""
        summary = self.__db.get_summary(self.__task_id)
        if summary is None:
            return None
        return summary['extra']

    def report(self):
        """Report the task's results to stdout and return exit status.

        This may be called when the task has never executed.
        Subclasses should override this.  The default implementation
        reports nothing and returns 0.
        """
        return 0

    # Standard input functions

    def _input_env(self, var):
        return os.environ.get(var)

    def _input_file(self, path):
        return hash_cache.get(path)

    def _input_unstable(self):
        """Mark this run as unstable, regardless of other inputs."""
        return None

    def _input_unknown_input(self):
        """An unknown input that may change after latexrun exits.

        This conservatively marks some unknown input that definitely
        won't change while latexrun is running, but may change before
        the user next runs latexrun.  This allows the task to
        stabilize during this invocation, but will cause the task to
        re-run on the next invocation.
        """
        return start_time

class RunResult(collections.namedtuple(
        'RunResult', 'output_filenames extra')):
    """The result of a single task execution.

    This captures all files written by the task, and task-specific
    results that need to be persisted between runs (for example, to
    enable reporting of a task's results).
    """
    pass

##################################################################
# LaTeX task
#

def normalize_input_path(path):
    # Resolve the directory of the input path, but leave the file
    # component alone because it affects TeX's behavior.
    head, tail = os.path.split(path)
    npath = os.path.join(os.path.realpath(head), tail)
    return os.path.relpath(path)

class LaTeX(Task):
    def __init__(self, db, tex_filename, cmd, cmd_args, obj_dir, nowarns):
        super().__init__(db, 'latex::' + normalize_input_path(tex_filename))
        self.__tex_filename = tex_filename
        self.__cmd = cmd
        self.__cmd_args = cmd_args
        self.__obj_dir = obj_dir
        self.__nowarns = nowarns

        self.__pass = 0

    def _input_args(self):
        # If filename starts with a character the tex command-line
        # treats specially, then tweak it so it doesn't.
        filename = self.__tex_filename
        if filename.startswith(('-', '&', '\\')):
            filename = './' + filename
        # XXX Put these at the beginning in case the provided
        # arguments are malformed.  Might want to do a best-effort
        # check for incompatible user-provided arguments (note:
        # arguments can be given with one or two dashes and those with
        # values can use an equals or a space).
        return [self.__cmd] + self.__cmd_args + \
            ['-interaction', 'nonstopmode', '-recorder',
             '-output-directory', self.__obj_dir, filename]

    def _execute(self):
        # Run latex
        self.__pass += 1
        args = self._input('args')
        debug('running {}', args)
        try:
            os.makedirs(self.__obj_dir, exist_ok=True)
        except OSError as e:
            raise TaskError('failed to create %s: ' % self.__obj_dir + str(e)) \
                from e
        try:
            verbose_cmd(args)
            p = subprocess.Popen(args,
                                 stdin=subprocess.DEVNULL,
                                 stdout=subprocess.PIPE,
                                 stderr=subprocess.STDOUT)
            stdout, has_errors, missing_includes = self.__feed_terminal(p.stdout)
            status = p.wait()
        except OSError as e:
            raise TaskError('failed to execute latex task: ' + str(e)) from e

        # Register environment variable inputs
        for env_var in ['TEXMFOUTPUT', 'TEXINPUTS', 'TEXFORMATS', 'TEXPOOL',
                        'TFMFONTS', 'PATH']:
            self._input('env', env_var)

        jobname, outname = self.__parse_jobname(stdout)
        inputs, outputs = self.__parse_recorder(jobname)

        # LaTeX overwrites its own inputs.  Mark its output files as
        # clobbered before we hash its input files.
        for path in outputs:
            # In some abort cases (e.g., >=100 errors), LaTeX claims
            # output files that don't actually exist.
            if os.path.exists(path):
                hash_cache.clobber(path)
        # Depend on input files.  Task.run pre-hashed outputs from the
        # previous run, so if this isn't the first run and as long as
        # the set of outputs didn't change, we'll be able to get the
        # input hashes, even if they were clobbered.
        for path in inputs:
            self._input('file', path)

        if missing_includes:
            # Missing \includes are tricky.  Ideally we'd depend on
            # the absence of some file, but in fact we'd have to
            # depend on the failure of a whole kpathsea lookup.
            # Rather than try to be clever, just mark this as an
            # unknown input so we'll run at least once on the next
            # invocation.
            self._input('unknown_input')

        if not self.__create_outdirs(stdout) and has_errors:
            # LaTeX reported unrecoverable errors (other than output
            # directory errors, which we just fixed).  We could
            # continue to stabilize the document, which may change
            # some of the other problems reported (but not the
            # unrecoverable errors), or we can just abort now and get
            # back to the user quickly with the major errors.  We opt
            # for the latter.
            global terminate_task_loop
            terminate_task_loop = True
            # This error could depend on something we failed to track.
            # It would be really confusing if we continued to report
            # the error after the user fixed it, so be conservative
            # and force a re-run next time.
            self._input('unknown_input')

        return RunResult(outputs,
                         {'jobname': jobname, 'outname': outname,
                          'status': status})

    def __feed_terminal(self, stdout):
        prefix = 'latex'
        if self.__pass > 1:
            prefix += ' ({})'.format(self.__pass)
        with Progress(prefix) as progress:
            buf = []
            filt = LaTeXFilter()
            while True:
                # Use os.read to read only what's available on the pipe,
                # without waiting to fill a buffer
                data = os.read(stdout.fileno(), 4096)
                if not data:
                    break
                # See "A note about encoding" above
                data = data.decode('ascii', errors='surrogateescape')
                buf.append(data)
                filt.feed(data)
                file_stack = filt.get_file_stack()
                if file_stack:
                    tos = file_stack[-1]
                    if tos.startswith('./'):
                        tos = tos[2:]
                    progress.update('>' * len(file_stack) + ' ' + tos)
                else:
                    progress.update('')

            # Were there unrecoverable errors?
            has_errors = any(msg.typ == 'error' for msg in filt.get_messages())

            return ''.join(buf), has_errors, filt.has_missing_includes()

    def __parse_jobname(self, stdout):
        """Extract the job name and output name from latex's output.

        We get these from latex because they depend on complicated
        file name parsing rules, are affected by arguments like
        -output-directory, and may be just "texput" if things fail
        really early.  The output name may be None if there were no
        pages of output.
        """
        jobname = outname = None
        for m in re.finditer(r'^Transcript written on "?(.*)\.log"?\.$', stdout,
                             re.MULTILINE | re.DOTALL):
            jobname = m.group(1).replace('\n', '')
        if jobname is None:
            print(stdout, file=sys.stderr)
            raise TaskError('failed to extract job name from latex log')
        for m in re.finditer(r'^Output written on "?(.*\.[^ ."]+)"? \([0-9]+ page',
                             stdout, re.MULTILINE | re.DOTALL):
            outname = m.group(1).replace('\n', '')
        if outname is None and not \
           re.search(r'^No pages of output\.$|^! Emergency stop\.$'
                     r'|^!  ==> Fatal error occurred, no output PDF file produced!$',
                     stdout, re.MULTILINE):
            print(stdout, file=sys.stderr)
            raise TaskError('failed to extract output name from latex log')

        # LuaTeX (0.76.0) doesn't include the output directory in the
        # logged transcript or output file name.
        if os.path.basename(jobname) == jobname and \
           os.path.exists(os.path.join(self.__obj_dir, jobname + '.log')):
            jobname = os.path.join(self.__obj_dir, jobname)
            if outname is not None:
                outname = os.path.join(self.__obj_dir, outname)

        return jobname, outname

    def __parse_recorder(self, jobname):
        """Parse file recorder output."""
        # XXX If latex fails because a file isn't found, that doesn't
        # go into the .fls file, but creating that file will affect
        # the computation, so it should be included as an input.
        # Though it's generally true that files can be added earlier
        # in search paths and will affect the output without us knowing.
        #
        # XXX This is a serious problem for bibtex, since the first
        # run won't depend on the .bbl file!  But maybe the .aux file
        # will always cause a re-run, at which point the .bbl will
        # exist?
        filename = jobname + '.fls'
        try:
            recorder = open(filename)
        except OSError as e:
            raise TaskError('failed to open file recorder output: ' + str(e)) \
                from e
        pwd, inputs, outputs = '', set(), set()
        for linenum, line in enumerate(recorder):
            parts = line.rstrip('\n').split(' ', 1)
            if parts[0] == 'PWD':
                pwd = parts[1]
            elif parts[0] in ('INPUT', 'OUTPUT'):
                if parts[1].startswith('/'):
                    path = parts[1]
                else:
                    # Try to make "nice" paths, especially for clean
                    path = os.path.relpath(os.path.join(pwd, parts[1]))
                if parts[0] == 'INPUT':
                    inputs.add(path)
                else:
                    outputs.add(path)
            else:
                raise TaskError('syntax error on line {} of {}'
                                .format(linenum, filename))
        # Ironically, latex omits the .fls file itself
        outputs.add(filename)
        return inputs, outputs

    def __create_outdirs(self, stdout):
        # In some cases, such as \include'ing a file from a
        # subdirectory, TeX will attempt to create files in
        # subdirectories of the output directory that don't exist.
        # Detect this, create the output directory, and re-run.
        m = re.search('^! I can\'t write on file `(.*)\'\\.$', stdout, re.M)
        if m and m.group(1).find('/') > 0 and '../' not in m.group(1):
            debug('considering creating output sub-directory for {}'.
                  format(m.group(1)))
            subdir = os.path.dirname(m.group(1))
            newdir = os.path.join(self.__obj_dir, subdir)
            if os.path.isdir(subdir) and not os.path.isdir(newdir):
                debug('creating output subdirectory {}'.format(newdir))
                try:
                    mkdir_p(newdir)
                except OSError as e:
                    raise TaskError('failed to create output subdirectory: ' +
                                    str(e)) from e
                self._input('unstable')
                return True

    def report(self):
        extra = self._get_result_extra()
        if extra is None:
            return 0

        # Parse the log
        logfile = open(extra['jobname'] + '.log', 'rt', errors='surrogateescape')
        for msg in self.__clean_messages(
                LaTeXFilter(self.__nowarns).feed(
                    logfile.read(), True).get_messages()):
            msg.emit()

        # Return LaTeX's exit status
        return extra['status']

    def __clean_messages(self, msgs):
        """Make some standard log messages more user-friendly."""
        have_undefined_reference = False
        for msg in msgs:
            if msg.msg == '==> Fatal error occurred, no output PDF file produced!':
                msg = msg._replace(typ='info',
                                   msg='Fatal error (no output file produced)')
            if msg.msg.startswith('[LaTeX] '):
                # Strip unnecessary package name
                msg = msg._replace(msg=msg.msg.split(' ', 1)[1])
            if re.match(r'Reference .* undefined', msg.msg):
                have_undefined_reference = True
            if have_undefined_reference and \
               re.match(r'There were undefined references', msg.msg):
                # LaTeX prints this at the end so the user knows it's
                # worthwhile looking back at the log.  Since latexrun
                # makes the earlier messages obvious, this is
                # redundant.
                continue
            yield msg

    def get_tex_filename(self):
        return self.__tex_filename

    def get_jobname(self):
        extra = self._get_result_extra()
        if extra is None:
            return None
        return extra['jobname']

    def get_outname(self):
        extra = self._get_result_extra()
        if extra is None:
            return None
        return extra['outname']

    def get_status(self):
        extra = self._get_result_extra()
        if extra is None:
            return None
        return extra['status']

class LaTeXCommit(Task):
    def __init__(self, db, latex_task, output_path):
        super().__init__(db, 'latex_commit::' +
                         normalize_input_path(latex_task.get_tex_filename()))
        self.__latex_task = latex_task
        self.__output_path = output_path
        self.status = 'There were errors'

    def _input_latex(self):
        return self.__latex_task.get_status(), self.__latex_task.get_outname()

    def _execute(self):
        self.status = 'There were errors'

        # If latex succeeded with output, atomically commit the output
        status, outname = self._input('latex')
        if status != 0 or outname is None:
            debug('not committing (status {}, outname {})', status, outname)
            if outname is None:
                self.status = 'No pages of output'
            return RunResult([], None)

        commit = self.__output_path or os.path.basename(outname)
        if os.path.abspath(commit) == os.path.abspath(outname):
            debug('skipping commit (outname is commit name)')
            self.status = None
            return RunResult([], None)

        try:
            if os.path.exists(commit) and filecmp.cmp(outname, commit):
                debug('skipping commit ({} and {} are identical)',
                      outname, commit)
                # To avoid confusion, touch the output file
                open(outname, 'r+b').close()
            else:
                debug('commiting {} to {}', outname, commit)
                shutil.copy(outname, outname + '~')
                os.rename(outname + '~', commit)
        except OSError as e:
            raise TaskError('error committing latex output: {}'.format(e)) from e
        self._input('file', outname)
        self.status = None
        return RunResult([commit], None)

class LaTeXFilter:
    TRACE = False               # Set to enable detailed parse tracing

    def __init__(self, nowarns=[]):
        self.__data = ''
        self.__restart_pos = 0
        self.__restart_file_stack = []
        self.__restart_messages_len = 0
        self.__messages = []
        self.__first_file = None
        self.__fatal_error = False
        self.__missing_includes = False
        self.__pageno = 1
        self.__restart_pageno = 1

        self.__suppress = {cls: 0 for cls in nowarns}

    def feed(self, data, eof=False):
        """Feed LaTeX log data to the parser.

        The log data can be from LaTeX's standard output, or from the
        log file.  If there will be no more data, set eof to True.
        """

        self.__data += data
        self.__data_complete = eof

        # Reset to last known-good restart point
        self.__pos = self.__restart_pos
        self.__file_stack = self.__restart_file_stack.copy()
        self.__messages = self.__messages[:self.__restart_messages_len]
        self.__lstart = self.__lend = -1
        self.__pageno = self.__restart_pageno

        # Parse forward
        while self.__pos < len(self.__data):
            self.__noise()

        # Handle suppressed warnings
        if eof:
            msgs = ['%d %s warning%s' % (count, cls, "s" if count > 1 else "")
                    for cls, count in self.__suppress.items() if count]
            if msgs:
                self.__message('info', None,
                               '%s not shown (use -Wall to show them)' %
                               ', '.join(msgs), filename=self.__first_file)

        if eof and len(self.__file_stack) and not self.__fatal_error:
            # Fatal errors generally cause TeX to "succumb" without
            # closing the file stack, so don't complain in that case.
            self.__message('warning', None,
                           "unbalanced `(' in log; file names may be wrong")
        return self

    def get_messages(self):
        """Return a list of warning and error Messages."""
        return self.__messages

    def get_file_stack(self):
        """Return the file stack for the data that has been parsed.

        This results a list from outermost file to innermost file.
        The list may be empty.
        """

        return self.__file_stack

    def has_missing_includes(self):
        """Return True if the log reported missing \\include files."""
        return self.__missing_includes

    def __save_restart_point(self):
        """Save the current state as a known-good restart point.

        On the next call to feed, the parser will reset to this point.
        """
        self.__restart_pos = self.__pos
        self.__restart_file_stack = self.__file_stack.copy()
        self.__restart_messages_len = len(self.__messages)
        self.__restart_pageno = self.__pageno

    def __message(self, typ, lineno, msg, cls=None, filename=None):
        if cls is not None and cls in self.__suppress:
            self.__suppress[cls] += 1
            return
        filename = filename or (self.__file_stack[-1] if self.__file_stack
                                else self.__first_file)
        self.__messages.append(Message(typ, filename, lineno, msg))

    def __ensure_line(self):
        """Update lstart and lend."""
        if self.__lstart <= self.__pos < self.__lend:
            return
        self.__lstart = self.__data.rfind('\n', 0, self.__pos) + 1
        self.__lend = self.__data.find('\n', self.__pos) + 1
        if self.__lend == 0:
            self.__lend = len(self.__data)

    @property
    def __col(self):
        """The 0-based column number of __pos."""
        self.__ensure_line()
        return self.__pos - self.__lstart

    @property
    def __avail(self):
        return self.__pos < len(self.__data)

    def __lookingat(self, needle):
        return self.__data.startswith(needle, self.__pos)

    def __lookingatre(self, regexp, flags=0):
        return re.compile(regexp, flags=flags).match(self.__data, self.__pos)

    def __skip_line(self):
        self.__ensure_line()
        self.__pos = self.__lend

    def __consume_line(self, unwrap=False):
        self.__ensure_line()
        data = self.__data[self.__pos:self.__lend]
        self.__pos = self.__lend
        if unwrap:
            # TeX helpfully wraps all terminal output at 79 columns
            # (max_print_line).  If requested, unwrap it.  There's
            # simply no way to do this perfectly, since there could be
            # a line that happens to be 79 columns.
            #
            # We check for >=80 because a bug in LuaTeX causes it to
            # wrap at 80 columns instead of 79 (LuaTeX #900).
            while self.__lend - self.__lstart >= 80:
                if self.TRACE: print('<{}> wrapping'.format(self.__pos))
                self.__ensure_line()
                data = data[:-1] + self.__data[self.__pos:self.__lend]
                self.__pos = self.__lend
        return data

    # Parser productions

    def __noise(self):
        # Most of TeX's output is line noise that combines error
        # messages, warnings, file names, user errors and warnings,
        # and echos of token lists and other input.  This attempts to
        # tease these apart, paying particular attention to all of the
        # places where TeX echos input so that parens in the input do
        # not confuse the file name scanner.  There are three
        # functions in TeX that echo input: show_token_list (used by
        # runaway and show_context, which is used by print_err),
        # short_display (used by overfull/etc h/vbox), and show_print
        # (used in issue_message and the same places as
        # show_token_list).
        lookingat, lookingatre = self.__lookingat, self.__lookingatre
        if self.__col == 0:
            # The following messages are always preceded by a newline
            if lookingat('! '):
                return self.__errmessage()
            if lookingat('!pdfTeX error: '):
                return self.__pdftex_fail()
            if lookingat('Runaway '):
                return self.__runaway()
            if lookingatre(r'(Overfull|Underfull|Loose|Tight) \\[hv]box \('):
                return self.__bad_box()
            if lookingatre('(Package |Class |LaTeX |pdfTeX )?(\w+ )?warning: ', re.I):
                return self.__generic_warning()
            if lookingatre('No file .*\\.tex\\.$', re.M):
                # This happens with \includes of missing files.  For
                # whatever reason, LaTeX doesn't consider this even
                # worth a warning, but I do!
                self.__message('warning', None,
                               self.__simplify_message(
                                   self.__consume_line(unwrap=True).strip()))
                self.__missing_includes = True
                return
            # Other things that are common and irrelevant
            if lookingatre(r'(Package|Class|LaTeX) (\w+ )?info: ', re.I):
                return self.__generic_info()
            if lookingatre(r'(Document Class|File|Package): '):
                # Output from "\ProvidesX"
                return self.__consume_line(unwrap=True)
            if lookingatre(r'\\\w+=\\[a-z]+\d+\n'):
                # Output from "\new{count,dimen,skip,...}"
                return self.__consume_line(unwrap=True)

        # print(self.__data[self.__lstart:self.__lend].rstrip())
        # self.__pos = self.__lend
        # return

        # Now that we've substantially reduced the spew and hopefully
        # eliminated all input echoing, we're left with the file name
        # stack, page outs, and random other messages from both TeX
        # and various packages.  We'll assume at this point that all
        # parentheses belong to the file name stack or, if they're in
        # random other messages, they're at least balanced and nothing
        # interesting happens between them.  For page outs, ship_out
        # prints a space if not at the beginning of a line, then a
        # "[", then the page number being shipped out (this is
        # usually, but not always, followed by "]").
        m = re.compile(r'[(){}\n]|(?<=[\n ])\[\d+', re.M).\
            search(self.__data, self.__pos)
        if m is None:
            self.__pos = len(self.__data)
            return
        self.__pos = m.start() + 1
        ch = self.__data[m.start()]
        if ch == '\n':
            # Save this as a known-good restart point for incremental
            # parsing, since we definitely didn't match any of the
            # known message types above.
            self.__save_restart_point()
        elif ch == '[':
            # This is printed at the end of a page, so we're beginning
            # page n+1.
            self.__pageno = int(self.__lookingatre(r'\d+').group(0)) + 1
        elif ((self.__data.startswith('`', m.start() - 1) or
               self.__data.startswith('`\\', m.start() - 2)) and
               self.__data.startswith('\'', m.start() + 1)):
            # (, ), {, and } sometimes appear in TeX's error
            # descriptions, but they're always in `'s (and sometimes
            # backslashed)
            return
        elif ch == '(':
            # XXX Check that the stack doesn't drop to empty and then re-grow
            first = self.__first_file is None and self.__col == 1
            filename = self.__filename()
            self.__file_stack.append(filename)
            if first:
                self.__first_file = filename
            if self.TRACE:
                print('<{}>{}enter {}'.format(
                    m.start(), ' '*len(self.__file_stack), filename))
        elif ch == ')':
            if len(self.__file_stack):
                if self.TRACE:
                    print('<{}>{}exit {}'.format(
                        m.start(), ' '*len(self.__file_stack),
                        self.__file_stack[-1]))
                self.__file_stack.pop()
            else:
                self.__message('warning', None,
                               "extra `)' in log; file names may be wrong ")
        elif ch == '{':
            # TeX uses this for various things we want to ignore, like
            # file names and print_mark.  Consume up to the '}'
            epos = self.__data.find('}', self.__pos)
            if epos != -1:
                self.__pos = epos + 1
            else:
                self.__message('warning', None,
                               "unbalanced `{' in log; file names may be wrong")
        elif ch == '}':
            self.__message('warning', None,
                           "extra `}' in log; file names may be wrong")

    def __filename(self):
        initcol = self.__col
        first = True
        name = ''
        # File names may wrap, but if they do, TeX will always print a
        # newline before the open paren
        while first or (initcol == 1 and self.__lookingat('\n')
                        and self.__col >= 79):
            if not first:
                self.__pos += 1
            m = self.__lookingatre(r'[^(){} \n]*')
            name += m.group()
            self.__pos = m.end()
            first = False
        return name

    def __simplify_message(self, msg):
        msg = re.sub(r'^(?:Package |Class |LaTeX |pdfTeX )?([^ ]+) (?:Error|Warning): ',
                     r'[\1] ', msg, flags=re.I)
        msg = re.sub(r'\.$', '', msg)
        msg = re.sub(r'has occurred (while \\output is active)', r'\1', msg)
        return msg

    def __errmessage(self):
        # Procedure print_err (including \errmessage, itself used by
        # LaTeX's \GenericError and all of its callers), as well as
        # fatal_error.  Prints "\n!  " followed by error text
        # ("Emergency stop" in the case of fatal_error).  print_err is
        # always followed by a call to error, which prints a period,
        # and a newline...
        msg = self.__consume_line(unwrap=True)[1:].strip()
        is_fatal_error = (msg == 'Emergency stop.')
        msg = self.__simplify_message(msg)
        # ... and then calls show_context, which prints the input
        # stack as pairs of lines giving the context.  These context
        # lines are truncated so they never wrap.  Each pair of lines
        # will start with either "<something> " if the context is a
        # token list, "<*> " for terminal input (or command line),
        # "<read ...>" for stream reads, something like "\macroname
        # #1->" for macros (though everything after \macroname is
        # subject to being elided as "..."), or "l.[0-9]+ " if it's a
        # file.  This is followed by the errant input with a line
        # break where the error occurred.
        lineno = None
        found_context = False
        stack = []
        while self.__avail:
            m1 = self.__lookingatre(r'<([a-z ]+|\*|read [^ >]*)> |\\.*(->|...)')
            m2 = self.__lookingatre('l\.[0-9]+ ')
            if m1:
                found_context = True
                pre = self.__consume_line().rstrip('\n')
                stack.append(pre)
            elif m2:
                found_context = True
                pre = self.__consume_line().rstrip('\n')
                info, rest = pre.split(' ', 1)
                lineno = int(info[2:])
                stack.append(rest)
            elif found_context:
                # Done with context
                break
            if found_context:
                # Consume the second context line
                post = self.__consume_line().rstrip('\n')
                # Clean up goofy trailing ^^M TeX sometimes includes
                post = re.sub(r'\^\^M$', '', post)
                if post[:len(pre)].isspace() and not post.isspace():
                    stack.append(len(stack[-1]))
                    stack[-2] += post[len(pre):]
            else:
                # If we haven't found the context, skip the line.
                self.__skip_line()
        stack_msg = ''
        for i, trace in enumerate(stack):
            stack_msg += ('\n         ' + (' ' * trace) + '^'
                          if isinstance(trace, int) else
                          '\n      at ' + trace.rstrip() if i == 0 else
                          '\n    from ' + trace.rstrip())

        if is_fatal_error:
            # fatal_error always prints one additional line of message
            info = self.__consume_line().strip()
            if info.startswith('*** '):
                info = info[4:]
            msg += ': '  + info.lstrip('(').rstrip(')')

        self.__message('error', lineno, msg + stack_msg)
        self.__fatal_error = True

    def __pdftex_fail(self):
        # Procedure pdftex_fail.  Prints "\n!pdfTeX error: ", the
        # message, and a newline.  Unlike print_err, there's never
        # context.
        msg = self.__consume_line(unwrap=True)[1:].strip()
        msg = self.__simplify_message(msg)
        self.__message('error', None, msg)

    def __runaway(self):
        # Procedure runaway.  Prints "\nRunaway ...\n" possibly
        # followed by token list (user text).  Always followed by a
        # call to print_err, so skip lines until we see the print_err.
        self.__skip_line()      # Skip "Runaway ...\n"
        if not self.__lookingat('! ') and self.__avail:
            # Skip token list, which is limited to one line
            self.__skip_line()

    def __bad_box(self):
        # Function hpack and vpack.  hpack prints a warning, a
        # newline, then a short_display of the offending text.
        # Unfortunately, there's nothing indicating the end of the
        # offending text, but it should be on one (possible wrapped)
        # line.  vpack prints a warning and then, *unless output is
        # active*, a newline.  The missing newline is probably a bug,
        # but it sure makes our lives harder.
        origpos = self.__pos
        msg = self.__consume_line()
        m = re.search(r' in (?:paragraph|alignment) at lines ([0-9]+)--([0-9]+)', msg) or \
            re.search(r' detected at line ([0-9]+)', msg)
        if m:
            # Sometimes TeX prints crazy line ranges like "at lines
            # 8500--250".  The lower number seems roughly sane, so use
            # that.  I'm not sure what causes this, but it may be
            # related to shipout routines messing up line registers.
            lineno = min(int(m.group(1)), int(m.groups()[-1]))
            msg = msg[:m.start()]
        else:
            m = re.search(r' while \\output is active', msg)
            if m:
                lineno = None
                msg = msg[:m.end()]
            else:
                self.__message('warning', None,
                               'malformed bad box message in log')
                return
        # Back up to the end of the known message text
        self.__pos = origpos + m.end()
        if self.__lookingat('\n'):
            # We have a newline, so consume it and look for the
            # offending text.
            self.__pos += 1
            # If there is offending text, it will start with a font
            # name, which will start with a \.
            if 'hbox' in msg and self.__lookingat('\\'):
                self.__consume_line(unwrap=True)
        msg = self.__simplify_message(msg) + ' (page {})'.format(self.__pageno)
        cls = msg.split(None, 1)[0].lower()
        self.__message('warning', lineno, msg, cls=cls)

    def __generic_warning(self):
        # Warnings produced by LaTeX's \GenericWarning (which is
        # called by \{Package,Class}Warning and \@latex@warning),
        # warnings produced by pdftex_warn, and other random warnings.
        msg, cls = self.__generic_info()
        # Most warnings include an input line emitted by \on@line
        m = re.search(' on input line ([0-9]+)', msg)
        if m:
            lineno = int(m.group(1))
            msg = msg[:m.start()]
        else:
            lineno = None
        msg = self.__simplify_message(msg)
        self.__message('warning', lineno, msg, cls=cls)

    def __generic_info(self):
        # Messages produced by LaTeX's \Generic{Error,Warning,Info}
        # and things that look like them
        msg = self.__consume_line(unwrap=True).strip()
        # Package and class messages are continued with lines
        # containing '(package name)            '
        pkg_name = msg.split(' ', 2)[1]
        prefix = '(' + pkg_name + ')            '
        while self.__lookingat(prefix):
            # Collect extra lines.  It's important that we keep these
            # because they may contain context information like line
            # numbers.
            extra = self.__consume_line(unwrap=True)
            msg += ' ' + extra[len(prefix):].strip()
        return msg, pkg_name.lower()

##################################################################
# BibTeX task
#

class BibTeX(Task):
    def __init__(self, db, latex_task, cmd, cmd_args, nowarns, obj_dir):
        super().__init__(db, 'bibtex::' + normalize_input_path(
            latex_task.get_tex_filename()))
        self.__latex_task = latex_task
        self.__cmd = cmd
        self.__cmd_args = cmd_args
        self.__obj_dir = obj_dir

    def stable(self):
        # If bibtex doesn't have its inputs, then it's stable because
        # it has no effect on system state.
        jobname = self.__latex_task.get_jobname()
        if jobname is None:
            # We don't know where the .aux file is until latex has run
            return True
        if not os.path.exists(jobname + '.aux'):
            # Input isn't ready, so bibtex will simply fail without
            # affecting system state.  Hence, this task is trivially
            # stable.
            return True
        if not self.__find_bib_cmds(os.path.dirname(jobname), jobname + '.aux'):
            # The tex file doesn't refer to any bibliographic data, so
            # don't run bibtex.
            return True

        return super().stable()

    def __find_bib_cmds(self, basedir, auxname, stack=()):
        debug('scanning for bib commands in {}'.format(auxname))
        if auxname in stack:
            raise TaskError('.aux file loop')
        stack = stack + (auxname,)

        try:
            aux_data = open(auxname, errors='surrogateescape').read()
        except FileNotFoundError:
            # The aux file may not exist if latex aborted
            return False
        if re.search(r'^\\bibstyle\{', aux_data, flags=re.M) or \
           re.search(r'^\\bibdata\{',  aux_data, flags=re.M):
            return True

        if re.search(r'^\\abx@aux@cite\{', aux_data, flags=re.M):
            # biber citation
            return True

        # Recurse into included aux files (see aux_input_command), in
        # case \bibliography appears in an \included file.
        for m in re.finditer(r'^\\@input\{([^}]*)\}', aux_data, flags=re.M):
            if self.__find_bib_cmds(basedir, os.path.join(basedir, m.group(1)),
                                    stack):
                return True

        return False

    def _input_args(self):
        if self.__is_biber():
            aux_name = os.path.basename(self.__latex_task.get_jobname())
        else:
            aux_name = os.path.basename(self.__latex_task.get_jobname()) + '.aux'
        return [self.__cmd] + self.__cmd_args + [aux_name]

    def _input_cwd(self):
        return os.path.dirname(self.__latex_task.get_jobname())

    def _input_auxfile(self, auxname):
        # We don't consider the .aux files regular inputs.
        # Instead, we extract just the bit that BibTeX cares about
        # and depend on that.  See get_aux_command_and_process in
        # bibtex.web.
        debug('hashing filtered aux file {}', auxname)
        try:
            with open(auxname, 'rb') as aux:
                h = hashlib.sha256()
                for line in aux:
                    if line.startswith((b'\\citation{', b'\\bibdata{',
                                        b'\\bibstyle{', b'\\@input{',
                                        b'\\abx@aux@cite{')):
                        h.update(line)
                return h.hexdigest()
        except FileNotFoundError:
            debug('{} does not exist', auxname)
            return None

    def __path_join(self, first, rest):
        if rest is None:
            # Append ':' to keep the default search path
            return first + ':'
        return first + ':' + rest

    def __is_biber(self):
        return "biber" in self.__cmd

    def _execute(self):
        # This gets complicated when \include is involved.  \include
        # switches to a different aux file and records its path in the
        # main aux file.  However, BibTeX does not consider this path
        # to be relative to the location of the main aux file, so we
        # have to run BibTeX *in the output directory* for it to
        # follow these includes (there's no way to tell BibTeX other
        # locations to search).  Unfortunately, this means BibTeX will
        # no longer be able to find local bib or bst files, but so we
        # tell it where to look by setting BIBINPUTS and BSTINPUTS
        # (luckily we can control this search).  We have to pass this
        # same environment down to Kpathsea when we resolve the paths
        # in BibTeX's log.
        args, cwd = self._input('args'), self._input('cwd')
        debug('running {} in {}', args, cwd)

        env = os.environ.copy()
        env['BIBINPUTS'] = self.__path_join(os.getcwd(), env.get('BIBINPUTS'))
        env['BSTINPUTS'] = self.__path_join(os.getcwd(), env.get('BSTINPUTS'))

        try:
            verbose_cmd(args, cwd, env)
            p = subprocess.Popen(args, cwd=cwd, env=env,
                                 stdin=subprocess.DEVNULL,
                                 stdout=subprocess.PIPE,
                                 stderr=subprocess.STDOUT)
            stdout = self.__feed_terminal(p.stdout)
            status = p.wait()
        except OSError as e:
            raise TaskError('failed to execute bibtex task: ' + str(e)) from e

        inputs, auxnames, outbase = self.__parse_inputs(stdout, cwd, env)
        if not inputs and not auxnames:
            # BibTeX failed catastrophically.
            print(stdout, file=sys.stderr)
            raise TaskError('failed to execute bibtex task')

        # Register environment variable inputs
        for env_var in ['TEXMFOUTPUT', 'BSTINPUTS', 'BIBINPUTS', 'PATH']:
            self._input('env', env_var)

        # Register file inputs
        for path in auxnames:
            self._input('auxfile', path)
        for path in inputs:
            self._input('file', path)

        if self.__is_biber():
            outbase = os.path.join(cwd, outbase)
        outputs = [outbase + '.bbl', outbase + '.blg']
        return RunResult(outputs, {'outbase': outbase, 'status': status,
                                   'inputs': inputs})

    def __feed_terminal(self, stdout):
        with Progress('bibtex') as progress:
            buf, linebuf = [], ''
            while True:
                data = os.read(stdout.fileno(), 4096)
                if not data:
                    break
                # See "A note about encoding" above
                data = data.decode('ascii', errors='surrogateescape')
                buf.append(data)
                linebuf += data
                while '\n' in linebuf:
                    line, _, linebuf = linebuf.partition('\n')
                    if line.startswith('Database file'):
                        progress.update(line.split(': ', 1)[1])
        return ''.join(buf)

    def __parse_inputs(self, log, cwd, env):
        # BibTeX conveniently logs every file that it opens, and its
        # log is actually sensible (see calls to a_open_in in
        # bibtex.web.)  The only trick is that these file names are
        # pre-kpathsea lookup and may be relative to the directory we
        # ran BibTeX in.
        #
        # Because BibTeX actually depends on very little in the .aux
        # file (and it's likely other things will change in the .aux
        # file), we don't count the whole .aux file as an input, but
        # instead depend only on the lines that matter to BibTeX.
        kpathsea = Kpathsea('bibtex')
        inputs = []
        auxnames = []
        outbase = None
        for line in log.splitlines():
            m = re.match('(?:The top-level auxiliary file:'
                         '|A level-[0-9]+ auxiliary file:) (.*)', line)
            if m:
                auxnames.append(os.path.join(cwd, m.group(1)))
                continue
            m = re.match('(?:(The style file:)|(Database file #[0-9]+:)) (.*)',
                         line)
            if m:
                filename = m.group(3)
                if m.group(1):
                    filename = kpathsea.find_file(filename, 'bst', cwd, env)
                elif m.group(2):
                    filename = kpathsea.find_file(filename, 'bib', cwd, env)

                # If this path is relative to the source directory,
                # clean it up for error reporting and portability of
                # the dependency DB
                if filename.startswith('/'):
                    relname = os.path.relpath(filename)
                    if '../' not in relname:
                        filename = relname

                inputs.append(filename)

            # biber output
            m = re.search("Found BibTeX data source '(.*?)'",
                         line)
            if m:
                filename = m.group(1)
                inputs.append(filename)

            m = re.search("Logfile is '(.*?)'", line)
            if m:
                outbase = m.group(1)[:-4]

        if outbase is None:
            outbase = auxnames[0][:-4]

        return inputs, auxnames, outbase

    def report(self):
        extra = self._get_result_extra()
        if extra is None:
            return 0

        # Parse and pretty-print the log
        log = open(extra['outbase'] + '.blg', 'rt').read()
        inputs = extra['inputs']
        for msg in BibTeXFilter(log, inputs).get_messages():
            msg.emit()

        # BibTeX exits with 1 if there are warnings, 2 if there are
        # errors, and 3 if there are fatal errors (sysdep.h).
        # Translate to a normal UNIX exit status.
        if extra['status'] >= 2:
            return 1
        return 0

class BibTeXFilter:
    def __init__(self, data, inputs):
        self.__inputs = inputs
        self.__key_locs = None

        self.__messages = []

        prev_line = ''
        for line in data.splitlines():
            msg = self.__process_line(prev_line, line)
            if msg is not None:
                self.__messages.append(Message(*msg))
            prev_line = line

    def get_messages(self):
        """Return a list of warning and error Messages."""
        # BibTeX reports most errors in no particular order.  Sort by
        # file and line.
        return sorted(self.__messages,
                      key=lambda msg: (msg.filename or '', msg.lineno or 0))

    def __process_line(self, prev_line, line):
        m = None
        def match(regexp):
            nonlocal m
            m = re.match(regexp, line)
            return m

        # BibTeX has many error paths, but luckily the set is closed,
        # so we can find all of them.  This first case is the
        # workhorse format.
        #
        # AUX errors: aux_err/aux_err_return/aux_err_print
        #
        # BST errors: bst_ln_num_print/bst_err/
        # bst_err_print_and_look_for_blank_line_return/
        # bst_warn_print/bst_warn/
        # skip_token/skip_token_print/
        # bst_ext_warn/bst_ext_warn_print/
        # bst_ex_warn/bst_ex_warn_print/
        # bst_mild_ex_warn/bst_mild_ex_warn_print/
        # bst_string_size_exceeded
        #
        # BIB errors: bib_ln_num_print/
        # bib_err_print/bib_err/
        # bib_warn_print/bib_warn/
        # bib_one_of_two_expected_err/macro_name_warning/
        if match('(.*?)---?line ([0-9]+) of file (.*)'):
            # Sometimes the real error is printed on the previous line
            if m.group(1) == 'while executing':
                # bst_ex_warn.  The real message is on the previous line
                text = prev_line
            else:
                text = m.group(1) or prev_line
            typ, msg = self.__canonicalize(text)
            return (typ, m.group(3), int(m.group(2)), msg)

        # overflow/print_overflow
        if match('Sorry---you\'ve exceeded BibTeX\'s (.*)'):
            return ('error', None, None, 'capacity exceeded: ' + m.group(1))
        # confusion/print_confusion
        if match('(.*)---this can\'t happen$'):
            return ('error', None, None, 'internal error: ' + m.group(1))
        # aux_end_err
        if match('I found (no .*)---while reading file (.*)'):
            return ('error', m.group(2), None, m.group(1))
        # bad_cross_reference_print/
        # nonexistent_cross_reference_error/
        # @<Complain about a nested cross reference@>
        #
        # This is split across two lines.  Match the second.
        if match('^refers to entry "'):
            typ, msg = self.__canonicalize(prev_line + ' ' + line)
            msg = re.sub('^a (bad cross reference)', '\\1', msg)
            # Try to give this key a location
            filename = lineno = None
            m2 = re.search(r'--entry "[^"]"', prev_line)
            if m2:
                filename, lineno = self.__find_key(m2.group(1))
            return (typ, filename, lineno, msg)
        # print_missing_entry
        if match('Warning--I didn\'t find a database entry for (".*")'):
            return ('warning', None, None,
                    'no database entry for ' + m.group(1))
        # x_warning
        if match('Warning--(.*)'):
            # Most formats give warnings about "something in <key>".
            # Try to match it up.
            filename = lineno = None
            for m2 in reversed(list(re.finditer(r' in ([^, \t\n]+)\b', line))):
                if m2:
                    filename, lineno = self.__find_key(m2.group(1))
                    if filename:
                        break
            return ('warning', filename, lineno, m.group(1))
        # @<Clean up and leave@>
        if match('Aborted at line ([0-9]+) of file (.*)'):
            return ('info', m.group(2), int(m.group(1)), 'aborted')

        # biber type errors
        if match('^.*> WARN - (.*)$'):
            print ('warning', None, None, m.group(1))
            m2 = re.match("(.*) in file '(.*?)', skipping ...", m.group(1))
            if m2:
                return ('warning', m2.group(2), "0", m2.group(1))
            return ('warning', None, None, m.group(1))

        if match('^.*> ERROR - (.*)$'):
            m2 = re.match("BibTeX subsystem: (.*?), line (\d+), (.*)$", m.group(1))
            if m2:
                return ('error', m2.group(1), m2.group(2), m2.group(3))
            return ('error', None, None, m.group(1))


    def __canonicalize(self, msg):
        if msg.startswith('Warning'):
            msg = re.sub('^Warning-*', '', msg)
            typ = 'warning'
        else:
            typ = 'error'
        msg = re.sub('^I(\'m| was)? ', '', msg)
        msg = msg[:1].lower() + msg[1:]
        return typ, msg

    def __find_key(self, key):
        if self.__key_locs is None:
            p = BibTeXKeyParser()
            self.__key_locs = {}
            for filename in self.__inputs:
                data = open(filename, 'rt', errors='surrogateescape').read()
                for pkey, lineno in p.parse(data):
                    self.__key_locs.setdefault(pkey, (filename, lineno))
        return self.__key_locs.get(key, (None, None))

class BibTeXKeyParser:
    """Just enough of a BibTeX parser to find keys."""

    def parse(self, data):
        IDENT_RE = '(?![0-9])([^\x00-\x20\x80-\xff \t"#%\'(),={}]+)'
        self.__pos, self.__data = 0, data
        # Find the next entry
        while self.__consume('[^@]*@[ \t\n]*'):
            # What type of entry?
            if not self.__consume(IDENT_RE + '[ \t\n]*'):
                continue
            typ = self.__m.group(1)
            if typ == 'comment':
                continue
            start = self.__pos
            if not self.__consume('([{(])[ \t\n]*'):
                continue
            closing, key_re = {'{' : ('}', '([^, \t\n}]*)'),
                               '(' : (')', '([^, \t\n]*)')}[self.__m.group(1)]
            if typ not in ('preamble', 'string'):
                # Regular entry; get key
                if self.__consume(key_re):
                    yield self.__m.group(1), self.__lineno()
            # Consume body of entry
            self.__pos = start
            self.__balanced(closing)

    def __consume(self, regexp):
        self.__m = re.compile(regexp).match(self.__data, self.__pos)
        if self.__m:
            self.__pos = self.__m.end()
        return self.__m

    def __lineno(self):
        return self.__data.count('\n', 0, self.__pos) + 1

    def __balanced(self, closing):
        self.__pos += 1
        level = 0
        skip = re.compile('[{}' + closing + ']')
        while True:
            m = skip.search(self.__data, self.__pos)
            if not m:
                break
            self.__pos = m.end()
            ch = m.group(0)
            if level == 0 and ch == closing:
                break
            elif ch == '{':
                level += 1
            elif ch == '}':
                level -= 1

class Kpathsea:
    def __init__(self, program_name):
        self.__progname = program_name

    def find_file(self, name, format, cwd=None, env=None):
        """Return the resolved path of 'name' or None."""

        args = ['kpsewhich', '-progname', self.__progname, '-format', format,
                name]
        try:
            verbose_cmd(args, cwd, env)
            path = subprocess.check_output(
                args, cwd=cwd, env=env, universal_newlines=True).strip()
        except subprocess.CalledProcessError as e:
            if e.returncode != 1:
                raise
            return None
        if cwd is None:
            return path
        return os.path.join(cwd, path)

if __name__ == "__main__":
    main()


==> sections/old/abstract.tex <==
\begin{abstract}
Your abstract text goes here. Just a few facts. Whet our appetites.
Not more than 200 words, if possible, and preferably closer to 150.
\end{abstract}


==> sections/old/abstract_v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\begin{abstract}
%Your abstract text goes here. Just a few facts. Whet our appetites.
%Not more than 200 words, if possible, and preferably closer to 150.


Across many real-time video applications, we observe an emerging need for a new primitive which allows clients to decode the next frame at a decent quality as soon as {\em any} non-empty subset of its packets is received. 
Unfortunately, today's real-time video systems fall short of this criterion, because they must reliably deliver at least certain number of packets for a frame to be decodable, and they pad video data with non-trivial redundancy in anticipation of certain packet loss rate, which sacrifices video quality if no packets turn out lost. 
This paper articulate a new abstraction of {\em data-scalable} real-time video delivery: the {\em same} video encoding, under no packet loss, has decent quality close to traditional coding without redundancy, and {\em with each missed packet, quality naturally degrades gracefully.} 
While traditional video codecs, this paper presents the first implementation {\em autoencoder-based} data-scalable video codec and a practical real-time video system, called \name, that is built on the new video codec.
We describe the design and implementation of our custom autoencoder (NN coder and NN decoder) and a suite of frame delivering optimizations that embrace the benefit of the data-scalable primitive and can be incrementally integrated in WebRTC framework. 
\jc{a few words on result highlight}

% A growing list of applications depend on real-time video, but they face a lasting challenge---the network may delay or drop {\em any} packets, forcing the video decoder to render a frame when only a subset of its packets have arrived.
% Traditional loss-resilient approaches (FEC, fountain codes) can recover encoded data from {\em arbitrary} subset of packets, but only if the arrived data are more than the encoded data.
% So they must know, {\em before} encoding and sending a frame to the network, how many of its packets will arrive on time.
% As bursts of packet losses and delays are inevitable in wide-area networks, we argue that a more desirable solution should be {\em data-scalable}---without knowing the arrived data rate in advance, should naturally achieve a higher quality if more packets arrive by the time the receiver renders the frame, and the quality should degrade gracefully if fewer packets arrive on time. 
% In this paper, we present the design and implementation of a true data-scalable real-time video system. 
% The key technique is a {\em new custom autoencoder} (a pair of NN encoder and NN decoder).
% Though traditional autoencoders are not naturally data-scalable, we can make it data-scalable by training the autoencoder to learn a smooth relationship between frame reconstruction (decoded video quality) and the amount of perturbation (packet losses) on the coded data.
% \jc{a few words on result highlight}


%Thus, it is crucial to render each frame at a high video quality without needing to wait for all packets to arrive. 
%A desirable codec, therefore, should naturally achieve a higher quality if more packets arrive by the time the receiver renders the frame. 
%We refer to this seemingly simple property as {\em data-scalable} coding and argue that {\em none} of existing solutions are truly rate-scalable.
%Existing loss-resilient schemes, such as FEC and fountain codes, must know, {\em before} encoding a frame, how many packets will arrive in time. 


\end{abstract}


==> sections/old/abstract_v3.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\begin{abstract}
%Your abstract text goes here. Just a few facts. Whet our appetites.
%Not more than 200 words, if possible, and preferably closer to 150.


Across many real-time video applications, we observe a growing need to allow clients to decode each frame once {\em any} (non-empty) subset of its packets is received and still obtain a high quality given the amount of data received. 
This calls for an abstraction, we refer to as {\em data-scalable} video delivery: the {\em same} video encoding, under no packet loss, has decent quality close to traditional coding without redundancy, and {\em with each missed packet, quality naturally degrades gracefully.} 
Unfortunately, existing techniques fall short of this ideal---they either must deliver at least certain number of packets for a frame to be decodable, and/or they pad video data with non-trivial redundancy in anticipation of certain packet loss rate, which hurts video quality if no packets turn out lost. 
We explore an alternative approach to data-scalable video delivery, using neural-network video autoencoders.
This paper presents \name, which trains a custom video autoencoder to optimizes compression efficiency {\em and} resilience to loss and transmits individually decodable packets to realize data-scalable video delivery, thus allowing clients to flexibly trade frame delay with video quality in real-time video.
\name addresses two high-level challenges: (1) how to encode and delivery real-time frames efficiently over autoencoders, and (2) how to train autoencoders to obtain decent quality under a range of packet loss rates. 
We test \name (and other traditional codecs and loss-resilient schemes) on real network traces and video datasets, and show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it achieves can significantly reduce video frame delay (by 2-3$\times$ at 95th percentile) with marginally lowered video quality.

%\jc{a few words on result highlight}

%a concrete real-time video system, called \name, that is built on the new video codec.
%We describe the design and implementation of our custom autoencoder (NN coder and NN decoder) and a suite of frame delivering optimizations that embrace the benefit of the data-scalable primitive and can be incrementally integrated in WebRTC framework. 
%\jc{a few words on result highlight}

% A growing list of applications depend on real-time video, but they face a lasting challenge---the network may delay or drop {\em any} packets, forcing the video decoder to render a frame when only a subset of its packets have arrived.
% Traditional loss-resilient approaches (FEC, fountain codes) can recover encoded data from {\em arbitrary} subset of packets, but only if the arrived data are more than the encoded data.
% So they must know, {\em before} encoding and sending a frame to the network, how many of its packets will arrive on time.
% As bursts of packet losses and delays are inevitable in wide-area networks, we argue that a more desirable solution should be {\em data-scalable}---without knowing the arrived data rate in advance, should naturally achieve a higher quality if more packets arrive by the time the receiver renders the frame, and the quality should degrade gracefully if fewer packets arrive on time. 
% In this paper, we present the design and implementation of a true data-scalable real-time video system. 
% The key technique is a {\em new custom autoencoder} (a pair of NN encoder and NN decoder).
% Though traditional autoencoders are not naturally data-scalable, we can make it data-scalable by training the autoencoder to learn a smooth relationship between frame reconstruction (decoded video quality) and the amount of perturbation (packet losses) on the coded data.
% \jc{a few words on result highlight}


%Thus, it is crucial to render each frame at a high video quality without needing to wait for all packets to arrive. 
%A desirable codec, therefore, should naturally achieve a higher quality if more packets arrive by the time the receiver renders the frame. 
%We refer to this seemingly simple property as {\em data-scalable} coding and argue that {\em none} of existing solutions are truly rate-scalable.
%Existing loss-resilient schemes, such as FEC and fountain codes, must know, {\em before} encoding a frame, how many packets will arrive in time. 


\end{abstract}


==> sections/old/abstract_v4.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\begin{abstract}
%Your abstract text goes here. Just a few facts. Whet our appetites.
%Not more than 200 words, if possible, and preferably closer to 150.


Across many real-time video applications, we see a growing need (especially in networks with long RTTs and dynamic bandwidth) for clients to  decode each frame once {\em any} (non-empty) subset of packets is received and achieve quality with each new packet.
We call it {\em data-scalable} delivery. 
%This is pressingly needed .
Unfortunately, existing techniques (\eg FEC, RS and Fountain Codes) fall short---they require either delivery of a minimum number of packets to decode frames, and/or pad video data with redundancy in anticipation of packet losses, which hurts video quality if no packets get lost. 
This work explores a new approach, inspired by recent advances of neural-network autoencoders, which make data-scalable delivery possible. 
We present \name, a concrete data-scalable real-time video system.
With the {\em same} video encoding, \name's quality is slightly lower than traditional codec without redundancy when no packet is lost, but {\em with each missed packet, its quality degrades much more gracefully} than existing solutions, allowing clients to flexibly trade between frame delay and video quality.
\name makes following contributions.
It trains new custom autoencoders to balance compression efficiency {\em and} resilience against a wide range of packet losses; and 
it uses a new transmission scheme to deliver autoencoder-coded frames as individually decodable packets.
We test \name (and traditional loss-resilient schemes and codecs) on real network traces and videos, and show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces tail video frame delay (by 2$\times$ at the 95th percentile) with the marginally lowered video quality.



%\name trains a custom video autoencoder to optimize compression efficiency {\em and} resilience to packet losses, and transmits individually decodable packets.
%\name addresses two high-level challenges: (1) how to encode and delivery real-time frames efficiently over autoencoders, and (2) how to train autoencoders to obtain decent quality under a range of packet loss rates. 
%We test \name (and other traditional codecs and loss-resilient schemes) on real network traces and video datasets, and show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it achieves can significantly reduce video frame delay (by 2-3$\times$ at 95th percentile) with marginally lowered video quality.








\begin{comment}

Across many real-time video applications, we observe a growing need to allow clients to decode each frame once {\em any} (non-empty) subset of its packets is received and still obtain a high quality given the amount of data received. 
This calls for an abstraction, we refer to as {\em data-scalable} video delivery: the {\em same} video encoding, under no packet loss, has decent quality close to traditional coding without redundancy, and {\em with each missed packet, quality naturally degrades gracefully.} 
Unfortunately, existing techniques fall short of this ideal---they either must deliver at least certain number of packets for a frame to be decodable, and/or they pad video data with non-trivial redundancy in anticipation of certain packet loss rate, which hurts video quality if no packets turn out lost. 
We explore an alternative approach to data-scalable video delivery, using neural-network video autoencoders.
This paper presents \name, which trains a custom video autoencoder to optimizes compression efficiency {\em and} resilience to loss and transmits individually decodable packets to realize data-scalable video delivery, thus allowing clients to flexibly trade frame delay with video quality in real-time video.
\name addresses two high-level challenges: (1) how to encode and delivery real-time frames efficiently over autoencoders, and (2) how to train autoencoders to obtain decent quality under a range of packet loss rates. 
We test \name (and other traditional codecs and loss-resilient schemes) on real network traces and video datasets, and show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it achieves can significantly reduce video frame delay (by 2-3$\times$ at 95th percentile) with marginally lowered video quality.

\end{comment}

%\jc{a few words on result highlight}

%a concrete real-time video system, called \name, that is built on the new video codec.
%We describe the design and implementation of our custom autoencoder (NN coder and NN decoder) and a suite of frame delivering optimizations that embrace the benefit of the data-scalable primitive and can be incrementally integrated in WebRTC framework. 
%\jc{a few words on result highlight}

% A growing list of applications depend on real-time video, but they face a lasting challenge---the network may delay or drop {\em any} packets, forcing the video decoder to render a frame when only a subset of its packets have arrived.
% Traditional loss-resilient approaches (FEC, fountain codes) can recover encoded data from {\em arbitrary} subset of packets, but only if the arrived data are more than the encoded data.
% So they must know, {\em before} encoding and sending a frame to the network, how many of its packets will arrive on time.
% As bursts of packet losses and delays are inevitable in wide-area networks, we argue that a more desirable solution should be {\em data-scalable}---without knowing the arrived data rate in advance, should naturally achieve a higher quality if more packets arrive by the time the receiver renders the frame, and the quality should degrade gracefully if fewer packets arrive on time. 
% In this paper, we present the design and implementation of a true data-scalable real-time video system. 
% The key technique is a {\em new custom autoencoder} (a pair of NN encoder and NN decoder).
% Though traditional autoencoders are not naturally data-scalable, we can make it data-scalable by training the autoencoder to learn a smooth relationship between frame reconstruction (decoded video quality) and the amount of perturbation (packet losses) on the coded data.
% \jc{a few words on result highlight}


%Thus, it is crucial to render each frame at a high video quality without needing to wait for all packets to arrive. 
%A desirable codec, therefore, should naturally achieve a higher quality if more packets arrive by the time the receiver renders the frame. 
%We refer to this seemingly simple property as {\em data-scalable} coding and argue that {\em none} of existing solutions are truly rate-scalable.
%Existing loss-resilient schemes, such as FEC and fountain codes, must know, {\em before} encoding a frame, how many packets will arrive in time. 


\end{abstract}


==> sections/old/abstract_v5.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\begin{abstract}

Many real-time video applications today operate under high latency and/or dynamic bandwidth, causing bursts of packet losses that are hard to predict and avoid. 
To handle packet losses, an ideal loss-resilient video coding scheme should, {\em without retransmission}, be able to decode each frame if {\em any subset} (non-empty) of packets is received, achieve better quality with more received packets, and if all packets are received, reach similar quality as if the video is coded with minimum redundancy (\eg H.264).
We call it {\em data-scalable} coding (DSC).
%This is pressingly needed .
Unfortunately, existing techniques (\eg FEC, RS and Fountain Codes) fall short---they must reliably receive a minimum number of packets to decode a frame, and/or pad video data with a pre-determined rate of redundancy, which degrades video quality if all packets are received.
This work explores the possibility of an alternative approach to DSC, based on recent advances of neural-network video autoencoders.
Our insight is that while existing autoencoders are not data-scalable, {\em they could be made so by novel training and packetization schemes}. 
To show its promise, we present \name, a concrete DSC-based real-time video system.
\name trains a new autoencoder by injecting random data erasures in its training.
The output of the autoencoder is then packetized and individually entropy-encoded such that with when all packets arrive, \name's quality is only slightly lower than the traditional non-loss-tolerant coding (H.264/265), and that {\em with each missed packet, its quality degrades much more gracefully} than existing solutions.
\name is complementary to the underlying congestion control logic and reaches better tradeoffs between frame delay and video quality than traditional loss-resilient video codecs. 
% \name makes following contributions.
% It trains new custom autoencoders to balance compression efficiency {\em and} resilience against a wide range of packet losses; and 
% it uses a new transmission scheme to deliver autoencoder-coded frames as individually decodable packets.
We test \name on real network traces and videos and show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces tail video frame delay (by 2$\times$ at the 95th percentile) with the marginally lowered video quality.

\end{abstract}

==> sections/old/abstract_v6.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\begin{abstract}



%Despite many prior efforts, most Internet video systems achieve decent video quality in presence of packet loss at the expense of lower quality in absence of packet loss.
%%achieve decent quality under packet losses---loss resilience---at the expense of lower quality under no packet loss.
%%Despite many prior efforts, existing loss-resilient video systems fundamentally trade compression efficiency (quality under no packet loss) for loss resilience (quality under packet losses).
%As a result, they often raise loss resilience 
%%(\eg adding more error-correction redundancy) 
%only {\em after} packet loss occurs, so some lost packets always have to be resent.

In real-time videos, resending {\em any} packets, especially in networks with high latency, can lead to stuttering, poor video quality, and user frustration.
Despite extensive research, current real-time video systems still use redundancy to handle packet loss, thus compromising on quality in the the absence of packet loss.
Since predicting packet loss is challenging, these systems only enhance their resilience to packet loss after it occurs, leaving some frames insufficiently protected against burst packet losses.
They may also add too much redundancy even after the packet loss has subsided. 

We present \name, a new real-time video communication system.
With \name, {\em(i)} a video frame can be decoded, as long as {\em any} non-empty subset of its packets are received, and {\em(ii)} the quality gracefully degrades as more packets are lost, and {\em(iii)} approximates that of a standard codec (like H.265) in absence of packet loss.
%but {\em(iii)} without sacrificing the quality in absence of packet loss. 
%We refer to it as data-scalable (DS) coding.
To achieve this, \name encodes and decodes frames by using neural networks (NNs). 
It uses a new packetization scheme that makes packet loss appear to have the same effect as randomly masking (zeroing) a subset of elements in the NN-encoded output, and the NN encoder and decoder are specially trained to achieve decent quality if a random subset of elements in the NN-encoded output are masked. %set to zeros.
%, and uses a new packetization and entropy-coding scheme that makes packet loss appear to have the same impact of random zeroing on the NN-encoded output. 
%under different rates of random data erasure.
Using various test videos and real network traces, we show that 
%when combined with the same rate adaptation logic, 
the quality of \name is slightly lower than H.265 when no packets are lost, but significantly reduces the 95th percentile of frame delay (between encoding a frame and its decoding) by 2$\times$ when packet loss occurs compared to other loss-resilient schemes while achieving comparable quality. 
This is because \name does not require retransmission of packets (unless all packets are lost) or skipping of frames.




%We have also developed new schemes for packetization, packet queuing, and speeding up NN-based coding, to reduce frame delay and ensure graceful degradation of quality in presence of packet loss. 
%Using real network traces and a variety of test videos, we show that when combined with the same rate adaptation logic, \name has slightly lower quality than H.265 when no packets are lost, but significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to other loss-resilient schemes. 
%This is because \name does not require retransmission of packets (unless all packets are lost) or skipping of frames.


%a frame can be decoded with any non-empty subset of its packets, with the quality being close to that of H.265 if all packets are received, and degrading gracefully with fewer received packets.
%That is, no need to retransmit any packet or skip any frame, unless all packets of a frame are lost.
%More importantly, the sender does not explicitly decide how much error protection to add before sending a frame.
%This means that the sender does not explicitly decide how much error protection to add before sending a frame, 

%That is, there is no need to resend any packet or skip any frame unless all packets are lost.
%This means that using the same video coding, the video quality naturally degrades gracefully in the presence of packet loss, without compromising quality in the absence of packet loss.


%Our insight is that while existing autoencoders are not data-scalable, {\em they could be made so by novel training and packetization schemes}. 
%\name trains a new autoencoder by injecting random data erasures in its training.
%The output of the autoencoder is then packetized and individually entropy-encoded such that with when all packets arrive, \name's quality is only slightly lower than the traditional non-loss-tolerant coding (H.264/265), and that {\em with each missed packet, its quality degrades much more gracefully} than existing solutions.
%\name is complementary to the underlying congestion control logic and reaches better tradeoffs between frame delay and video quality than traditional loss-resilient video codecs. 
%% \name makes following contributions.
%% It trains new custom autoencoders to balance compression efficiency {\em and} resilience against a wide range of packet losses; and 
%% it uses a new transmission scheme to deliver autoencoder-coded frames as individually decodable packets.
%We test \name on real network traces and videos and show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces tail video frame delay (by 2$\times$ at the 95th percentile) with the marginally lowered video quality.

\end{abstract}


\begin{comment}

In real-time videos, resending {\em any} lost packets, particularly in long-latency networks, can cause low quality, video stuttering, and ultimately user frustration. 
Despite intense research, state-of-the-art real-time video systems have to sacrifice quality in absence of packet loss (\eg by adding redundancy) in order to achieve decent quality in presence of packet loss. 
Since packet loss is difficult to predict, they increase loss resilience only after packet loss occurs, leaving some frames insufficiently protected against packet loss after a burst of packet loss, and they may add too much redundancy even after packet loss disappears. 

%As a result of this tradeoff between compression efficiency and loss resilience, 

%have to trade lower video quality for resilience to more packet loss.
%As a result, they often increase loss resilience only after packet loss occurs.






We present \name, a new real-time video communication system. 
When {\em any} non-empty subset of a frame's packets are received, \name can decode the frame at a quality close to that of H.265 in absence of packet loss, and the quality degrades gracefully with more lost packets.
We refer to this as data-scalable (DS) coding.
To achieve it, \name first replaces the traditional video encoder and decoder with new loss-resilient neural networks (NNs) that are specially trained to gain decent quality under a range of erasure rates of coded data.
With these NN encoder and decoder, we develop new schemes for packetization and frame scheduling, such that frame delay is low and quality
%such that without resending packets (unless all packets are lost), \name's video quality 
degrades gracefully in the presence of packet loss, without compromising quality in the absence of packet loss.
%under various rate of data erasures on the encoded data, such that the decoded quality degrades gracefully under more data erasures. 
Using real network traces and a wide range of test videos, we show that when using the same rate adaptation logic, \name has marginally worse quality than H.265 when no packet is lost, but significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to other loss-resilient schemes, since \name does not need to retransmit packets (unless all packets are lost) or skip frames.
%because it retransmits fewer packets without explicitly adding loss-protection redundancy.


\end{comment}

\begin{comment}


Despite many prior efforts, most real-time Internet video systems increase loss resilience only {\em after} packet loss occurs.
This is because protecting against any packet loss will likely incur  redundancy in coded data and lower video quality when no packet is lost. 
As a result, frames are unlikely protected right after a burst of packet losses. 
Yet, in real-time video applications, resending {\em any} lost packets, particularly in long-latency networks, can 
%where
%%In online video calls and cloud gaming, 
%ideally each frame should be decoded soon after some of its packets are received. 
%{\em Any} lost or delayed packet can block a video frame and its subsequent frames, 
cause low quality, video stuttering, and ultimately user frustration. 
%The alternative is not desirable either: to keep a high loss resilience all the time means lower quality in absence of packet loss.
%if all packets arrive on time.
%Since it is hard to predict when, which or how many packets will be lost, 
%The result is that the sender has to either risk video stuttering or raise loss resilience (\eg by adding much error-correction redundancy) and lower quality even if all packets arrive.

%%which maintains high quality when no packet is lost while only retransmitting a few lost packets. 
%Yet, they fail to protect real-time video applications (\eg online conferencing and cloud gaming) against packet losses, because {\em any} lost or delayed packet may {\em directly} delay a real-time video frame and its subsequent frames, causing low quality, stuttering, and ultimately user frustration. 
%Since it is hard to predict when, which or how many packets will be lost, the sender has to either risk video stuttering or add much error-correction redundancy in coded data which lowers quality even if all packets arrive.


\end{comment}

\begin{comment}
\newpage 

However, real-time video applications, such as online conferencing and cloud gaming, are plagued with random bursts of packet losses or latency jitters. 
As a result, it is hard to predict when, which or how many packets will be missing when a frame is supposed to be decoded, causing video stutters, low quality, and ultimately user frustration.

Real-time video, such as online conferencing and cloud gaming, is plagued with random bursts of packet losses or latency jitters. 



%There has been intense research on real-time video communication, but they are either {\em reactive}---such as lowering bitrate or increasing FEC redundancy after losses occur---or too slow to 


In real-time videos, {\em any} packet can be lost or delayed at {\em any} time, making it difficult to maintain high quality against packet losses by bitrate adaptation or redundant coding.
Thus, a desirable coding and streaming system should be able to decode each frame if {\em any subset} (non-empty) of packets is received, achieve better quality with more received packets, and if all packets are received, reach similar quality as if the video is coded with minimum redundancy (\eg H.264).

Many real-time video applications today operate under high latency and/or dynamic bandwidth, causing bursts of packet losses that are hard to predict and avoid. 
To handle packet losses, an ideal loss-resilient video coding scheme should, {\em without retransmission}, be able to decode each frame if {\em any subset} (non-empty) of packets is received, achieve better quality with more received packets, and if all packets are received, reach similar quality as if the video is coded with minimum redundancy (\eg H.264).
We call it {\em data-scalable} coding (DSC).
%This is pressingly needed .
Unfortunately, existing techniques (\eg FEC, RS and Fountain Codes) fall short---they must reliably receive a minimum number of packets to decode a frame, and/or pad video data with a pre-determined rate of redundancy, which degrades video quality if all packets are received.
This work explores the possibility of an alternative approach to DSC, based on recent advances of neural-network video autoencoders.
Our insight is that while existing autoencoders are not data-scalable, {\em they could be made so by novel training and packetization schemes}. 
To show its promise, we present \name, a concrete DSC-based real-time video system.
\name trains a new autoencoder by injecting random data erasures in its training.
The output of the autoencoder is then packetized and individually entropy-encoded such that with when all packets arrive, \name's quality is only slightly lower than the traditional non-loss-tolerant coding (H.264/265), and that {\em with each missed packet, its quality degrades much more gracefully} than existing solutions.
\name is complementary to the underlying congestion control logic and reaches better tradeoffs between frame delay and video quality than traditional loss-resilient video codecs. 
% \name makes following contributions.
% It trains new custom autoencoders to balance compression efficiency {\em and} resilience against a wide range of packet losses; and 
% it uses a new transmission scheme to deliver autoencoder-coded frames as individually decodable packets.
We test \name on real network traces and videos and show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces tail video frame delay (by 2$\times$ at the 95th percentile) with the marginally lowered video quality.
\end{comment}



==> sections/old/abstract_v7.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\begin{abstract}



%Despite many prior efforts, most Internet video systems achieve decent video quality in presence of packet loss at the expense of lower quality in absence of packet loss.
%%achieve decent quality under packet losses---loss resilience---at the expense of lower quality under no packet loss.
%%Despite many prior efforts, existing loss-resilient video systems fundamentally trade compression efficiency (quality under no packet loss) for loss resilience (quality under packet losses).
%As a result, they often raise loss resilience 
%%(\eg adding more error-correction redundancy) 
%only {\em after} packet loss occurs, so some lost packets always have to be resent.

In real-time video communication, such as video conferencing and cloud gaming, retransmitting any packets over long-latency networks can cause video stalls and user frustration.
To tolerate packet loss, existing solutions either rely on encoder-side forward error coding or decoder-side postprocessing error concealment. 
Neither is ideal: the former adds redundancy by the encoder {\em before} packet loss occurs, so it is difficult to decide the amount of redundancy, and the latter must sacrifice compression efficiency in order for partially received packets to be decodable and interpolate missing data which often hurts quality.
% sacrifices compression efficiency in order for partially received packets to be decodable. \yc{and the latter must guess the missing data and has error-prone reconstruction, since the sender does not add any redundancy}

\passed{\fyy{I wouldn't use Anon as the system name. It's better to come up with a different catchy name.}}
This paper presents \name\footnote{Anonymized for submission.}, a new real-time video system which {\em jointly trains} a pair of neural-net (NN) encoder and NN decoder that optimize video quality under {\em both} low and high packet loss rates.
To simulate packet loss, \name splits each encoded frame into $n$ packets such that losing one packet has the same effect as randomly zeroing $1/n$ values in the encoder's output. 
Our insight is that by training the NN encoder and NN decoder under different rates of simulated packet loss, the resulting NN encoder and NN decoder form a {\em generative autoencoder} with the following property: 
with the same frame encoding, \name obtains quality similar to the classic codec used in WebRTC without FEC when there is no packet loss; and with higher packet loss rates, the quality gradually degrades but is still better than state-of-the-art loss-resilient schemes.
%On a variety of test video content, we show that 
%%even though \name's encoder does not know the actual packet loss rate, 
%when no packet is lost, \name obtains quality similar to the codec used in WebRTC without FEC, and the quality gradually degrades but still better than state-of-the-art loss-resilient schemes under different packet loss rate. 
Using real network traces, we show that \name reduces the number of non-renderable frames and  stall duration by \review{95}\% and  \review{90}\% respectively, when compared with state-of-the-art loss-resilient schemes, such as Tambur (streaming FEC) and neural-net error concealment schemes. 
\passed{\yc{will 20x and 10x sounds too good? maybe we can use tail latency here, which is 3x}}


%In real-time video communication, such as video conferencing and cloud gaming, packet loss is hard to avoid, but retransmitting any packets can cause video stalls and user frustration, especially in long-latency networks.
%Many loss-resilient schemes exist, such as forward error correction (FEC) and receiver-side error recovery. 
%However, to tolerate packet loss, the sender must add redundancy or lower quality {\em before} packet loss occurs, which makes it difficult to decide when to prepare for packet loss and how much redundancy is appropriate.
\passed{\fyy{I understand the high-level message this passage is trying to deliver, but it's not very clear.
Consider 1) laying out the background more clearly by saying retransmission is infeasible on high-RTT networks due to the stringent latency requirement of RTC; 2) the remaining 
(non-interactive) approaches to achieving loss resilience primarily comprise: a) \textit{forward} error correction at the encoder, and b) \textit{post-processing} error concealment at the decoder (according to \url{https://ieeexplore.ieee.org/document/664283}). The former faces the challenge of determining the redundancy rate prior to uncertain losses, whereas the latter requires sacrificing compression efficiency so as to enable reconstruction from partially received video. (Details can also be cut in the abstract and postponed to the intro.)}}

%This paper presents \name, a new real-time video communication system that uses a pair of neural encoder and neural decoder. 
\passed{\fyy{This sentence does not summary the strengths of \name very well.}}
%The sender splits each encoded frame into packets such that any $x\%$ packet loss appear to be randomly masking $x\%$ of values in the encoder output. 
\passed{\fyy{This sentence is very confusing since it is not immediately clear what is ``masking'' (a word not widely understood outside of the ML community) and more importantly, why doing so is beneficial. Instead of providing technical details, ideally a high-level intuition about how \name works should be given here.}}
%\name~{\em jointly trains} the neural encoder and decoder to optimize video quality when various fractions of values in the encoder output are masked at random.
\passed{\fyy{I think this is the right level of details to put first. It can also be used to contrast with the encoder-heavy/forward approaches and decoder-heavy/post-processing approaches.}}
% that consists of a pair of neural encoder and neural decoder and a novel scheme to transform encoder output to packets. 
%In other words, with the same encoding output, \name optimizes video quality under various packet loss rates. 
%On a variety of test video content, we show that 
%%even though \name's encoder does not know the actual packet loss rate, 
%when no packet is lost, \name obtains quality similar to the codec used in WebRTC without FEC, and the quality gradually degrades but still better than state-of-the-art loss-resilient schemes under different packet loss rate. 
%Using real network traces, we show that \name reduces the number of non-recoverable frames and the stall duration by \fillme\% and  \fillme\% respectively, when compared with state-of-the-art loss-resilient schemes, such as Tambur (streaming FEC) and neural-net error concealment schemes.

%\name~{\em jointly trains} a pair of neural encoder and neural decoder to optimize video quality when various fractions of values in the encoder output are masked at random.
%In runtime, \name splits each encoded frame into packets such that any $x\%$ packet loss appear to be randomly masking $x\%$ of values in the encoder output. 


% significantly reduces the 95th percentile of frame delay (between encoding a frame and its decoding) by 2$\times$ when packet loss occurs compared to state-of-the-art loss-resilient schemes while achieving comparable quality. 
% This is because \name does not require retransmission of packets (unless all packets are lost) or skipping of frames.

\tempstrike{
With \name, {\em(i)} a video frame can be decoded, as long as {\em any} non-empty subset of its packets are received, and {\em(ii)} the quality gracefully degrades as more packets are lost, and {\em(iii)} approximates that of a standard codec (like H.265) in absence of packet loss.
%but {\em(iii)} without sacrificing the quality in absence of packet loss. 
%We refer to it as data-scalable (DS) coding.
To achieve this, \name encodes and decodes frames by using neural networks (NNs). 
It uses a new packetization scheme that makes packet loss appear to have the same effect as randomly masking (zeroing) a subset of elements in the NN-encoded output, and the NN encoder and decoder are specially trained to achieve decent quality if a random subset of elements in the NN-encoded output are masked. %set to zeros.
%, and uses a new packetization and entropy-coding scheme that makes packet loss appear to have the same impact of random zeroing on the NN-encoded output. 
%under different rates of random data erasure.
Using various test videos and real network traces, we show that 
%when combined with the same rate adaptation logic, 
the quality of \name is slightly lower than H.265 when no packets are lost, but significantly reduces the 95th percentile of frame delay (between encoding a frame and its decoding) by 2$\times$ when packet loss occurs compared to other loss-resilient schemes while achieving comparable quality. 
This is because \name does not require retransmission of packets (unless all packets are lost) or skipping of frames.
}



%We have also developed new schemes for packetization, packet queuing, and speeding up NN-based coding, to reduce frame delay and ensure graceful degradation of quality in presence of packet loss. 
%Using real network traces and a variety of test videos, we show that when combined with the same rate adaptation logic, \name has slightly lower quality than H.265 when no packets are lost, but significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to other loss-resilient schemes. 
%This is because \name does not require retransmission of packets (unless all packets are lost) or skipping of frames.


%a frame can be decoded with any non-empty subset of its packets, with the quality being close to that of H.265 if all packets are received, and degrading gracefully with fewer received packets.
%That is, no need to retransmit any packet or skip any frame, unless all packets of a frame are lost.
%More importantly, the sender does not explicitly decide how much error protection to add before sending a frame.
%This means that the sender does not explicitly decide how much error protection to add before sending a frame, 

%That is, there is no need to resend any packet or skip any frame unless all packets are lost.
%This means that using the same video coding, the video quality naturally degrades gracefully in the presence of packet loss, without compromising quality in the absence of packet loss.


%Our insight is that while existing autoencoders are not data-scalable, {\em they could be made so by novel training and packetization schemes}. 
%\name trains a new autoencoder by injecting random data erasures in its training.
%The output of the autoencoder is then packetized and individually entropy-encoded such that with when all packets arrive, \name's quality is only slightly lower than the traditional non-loss-tolerant coding (H.264/265), and that {\em with each missed packet, its quality degrades much more gracefully} than existing solutions.
%\name is complementary to the underlying congestion control logic and reaches better tradeoffs between frame delay and video quality than traditional loss-resilient video codecs. 
%% \name makes following contributions.
%% It trains new custom autoencoders to balance compression efficiency {\em and} resilience against a wide range of packet losses; and 
%% it uses a new transmission scheme to deliver autoencoder-coded frames as individually decodable packets.
%We test \name on real network traces and videos and show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces tail video frame delay (by 2$\times$ at the 95th percentile) with the marginally lowered video quality.

\end{abstract}


\begin{comment}

In real-time videos, resending {\em any} lost packets, particularly in long-latency networks, can cause low quality, video stuttering, and ultimately user frustration. 
Despite intense research, state-of-the-art real-time video systems have to sacrifice quality in absence of packet loss (\eg by adding redundancy) in order to achieve decent quality in presence of packet loss. 
Since packet loss is difficult to predict, they increase loss resilience only after packet loss occurs, leaving some frames insufficiently protected against packet loss after a burst of packet loss, and they may add too much redundancy even after packet loss disappears. 

%As a result of this tradeoff between compression efficiency and loss resilience, 

%have to trade lower video quality for resilience to more packet loss.
%As a result, they often increase loss resilience only after packet loss occurs.






We present \name, a new real-time video communication system. 
When {\em any} non-empty subset of a frame's packets are received, \name can decode the frame at a quality close to that of H.265 in absence of packet loss, and the quality degrades gracefully with more lost packets.
We refer to this as data-scalable (DS) coding.
To achieve it, \name first replaces the traditional video encoder and decoder with new loss-resilient neural networks (NNs) that are specially trained to gain decent quality under a range of erasure rates of coded data.
With these NN encoder and decoder, we develop new schemes for packetization and frame scheduling, such that frame delay is low and quality
%such that without resending packets (unless all packets are lost), \name's video quality 
degrades gracefully in the presence of packet loss, without compromising quality in the absence of packet loss.
%under various rate of data erasures on the encoded data, such that the decoded quality degrades gracefully under more data erasures. 
Using real network traces and a wide range of test videos, we show that when using the same rate adaptation logic, \name has marginally worse quality than H.265 when no packet is lost, but significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to other loss-resilient schemes, since \name does not need to retransmit packets (unless all packets are lost) or skip frames.
%because it retransmits fewer packets without explicitly adding loss-protection redundancy.


\end{comment}

\begin{comment}


Despite many prior efforts, most real-time Internet video systems increase loss resilience only {\em after} packet loss occurs.
This is because protecting against any packet loss will likely incur  redundancy in coded data and lower video quality when no packet is lost. 
As a result, frames are unlikely protected right after a burst of packet losses. 
Yet, in real-time video applications, resending {\em any} lost packets, particularly in long-latency networks, can 
%where
%%In online video calls and cloud gaming, 
%ideally each frame should be decoded soon after some of its packets are received. 
%{\em Any} lost or delayed packet can block a video frame and its subsequent frames, 
cause low quality, video stuttering, and ultimately user frustration. 
%The alternative is not desirable either: to keep a high loss resilience all the time means lower quality in absence of packet loss.
%if all packets arrive on time.
%Since it is hard to predict when, which or how many packets will be lost, 
%The result is that the sender has to either risk video stuttering or raise loss resilience (\eg by adding much error-correction redundancy) and lower quality even if all packets arrive.

%%which maintains high quality when no packet is lost while only retransmitting a few lost packets. 
%Yet, they fail to protect real-time video applications (\eg online conferencing and cloud gaming) against packet losses, because {\em any} lost or delayed packet may {\em directly} delay a real-time video frame and its subsequent frames, causing low quality, stuttering, and ultimately user frustration. 
%Since it is hard to predict when, which or how many packets will be lost, the sender has to either risk video stuttering or add much error-correction redundancy in coded data which lowers quality even if all packets arrive.


\end{comment}

\begin{comment}
\newpage 

However, real-time video applications, such as online conferencing and cloud gaming, are plagued with random bursts of packet losses or latency jitters. 
As a result, it is hard to predict when, which or how many packets will be missing when a frame is supposed to be decoded, causing video stutters, low quality, and ultimately user frustration.

Real-time video, such as online conferencing and cloud gaming, is plagued with random bursts of packet losses or latency jitters. 



%There has been intense research on real-time video communication, but they are either {\em reactive}---such as lowering bitrate or increasing FEC redundancy after losses occur---or too slow to 


In real-time videos, {\em any} packet can be lost or delayed at {\em any} time, making it difficult to maintain high quality against packet losses by bitrate adaptation or redundant coding.
Thus, a desirable coding and streaming system should be able to decode each frame if {\em any subset} (non-empty) of packets is received, achieve better quality with more received packets, and if all packets are received, reach similar quality as if the video is coded with minimum redundancy (\eg H.264).

Many real-time video applications today operate under high latency and/or dynamic bandwidth, causing bursts of packet losses that are hard to predict and avoid. 
To handle packet losses, an ideal loss-resilient video coding scheme should, {\em without retransmission}, be able to decode each frame if {\em any subset} (non-empty) of packets is received, achieve better quality with more received packets, and if all packets are received, reach similar quality as if the video is coded with minimum redundancy (\eg H.264).
We call it {\em data-scalable} coding (DSC).
%This is pressingly needed .
Unfortunately, existing techniques (\eg FEC, RS and Fountain Codes) fall short---they must reliably receive a minimum number of packets to decode a frame, and/or pad video data with a pre-determined rate of redundancy, which degrades video quality if all packets are received.
This work explores the possibility of an alternative approach to DSC, based on recent advances of neural-network video autoencoders.
Our insight is that while existing autoencoders are not data-scalable, {\em they could be made so by novel training and packetization schemes}. 
To show its promise, we present \name, a concrete DSC-based real-time video system.
\name trains a new autoencoder by injecting random data erasures in its training.
The output of the autoencoder is then packetized and individually entropy-encoded such that with when all packets arrive, \name's quality is only slightly lower than the traditional non-loss-tolerant coding (H.264/265), and that {\em with each missed packet, its quality degrades much more gracefully} than existing solutions.
\name is complementary to the underlying congestion control logic and reaches better tradeoffs between frame delay and video quality than traditional loss-resilient video codecs. 
% \name makes following contributions.
% It trains new custom autoencoders to balance compression efficiency {\em and} resilience against a wide range of packet losses; and 
% it uses a new transmission scheme to deliver autoencoder-coded frames as individually decodable packets.
We test \name on real network traces and videos and show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces tail video frame delay (by 2$\times$ at the 95th percentile) with the marginally lowered video quality.
\end{comment}



==> sections/old/abstract_v8.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\begin{abstract}



%Despite many prior efforts, most Internet video systems achieve decent video quality in presence of packet loss at the expense of lower quality in absence of packet loss.
%%achieve decent quality under packet losses---loss resilience---at the expense of lower quality under no packet loss.
%%Despite many prior efforts, existing loss-resilient video systems fundamentally trade compression efficiency (quality under no packet loss) for loss resilience (quality under packet losses).
%As a result, they often raise loss resilience 
%%(\eg adding more error-correction redundancy) 
%only {\em after} packet loss occurs, so some lost packets always have to be resent.

In real-time video communication, such as video conferencing and cloud gaming, retransmitting any packets over long-latency networks can cause video stalls and user frustration.
To avoid retransmission, existing solutions either rely on either encoder-based forward error coding or decoder-based postprocessing for error concealment. 
Neither is ideal: the former must add redundancy {\em before} packet loss occurs, so it is difficult to decide the right amount of redundancy, and the latter must sacrifice compression efficiency in order for partially received packets to be decodable and the limited redundancy in encoding often results in substantial quality degradation, even when missing parts are reconstructed.
% sacrifices compression efficiency in order for partially received packets to be decodable. \yc{and the latter must guess the missing data and has error-prone reconstruction, since the sender does not add any redundancy}


This paper presents \name, a new real-time video system using a pair of {\em jointly-trained} neural-net (NN) encoder and NN decoder to optimize video quality under {\em both} low and high packet loss rates.
To simulate packet loss, \name splits the encoder's output into $n$ packets such that losing one packet has the same effect on the decoder as randomly zeroing $1/n$ values in the encoder's output. 
Our insight is that by training the NN encoder and NN decoder under different rates of simulated packet loss, the resulting NN encoder and NN decoder will jointly form a {\em generative autoencoder} with the following property: 
with the same frame encoding, \name obtains quality similar to the classic codecs (without FEC) when there is no packet loss; and with higher packet loss rates, the quality gradually degrades but is still better than state-of-the-art loss-resilient schemes.
%On a variety of test video content, we show that 
%%even though \name's encoder does not know the actual packet loss rate, 
%when no packet is lost, \name obtains quality similar to the codec used in WebRTC without FEC, and the quality gradually degrades but still better than state-of-the-art loss-resilient schemes under different packet loss rate. 
Using real network traces, we show that \name reduces the number of non-renderable frames and  stall duration by \review{95}\% and  \review{90}\% respectively without sacrificing video quality (in SSIM), when compared with state-of-the-art loss-resilient schemes, such as Tambur (streaming FEC) and neural-net error concealment schemes. 
Moreover, real user evaluations highlight Grace++ can achieve a 38\% higher mean opinion score compared to competitive loss-resilient schemes, largely attributed to its ability to minimize video stalls and reduce skipped frames.
\yc{potential improvement: make the settings more realistic: e.g., getting some real-world video conference/video gaming network traces or video content}
%\passed{\yc{will 20x and 10x sounds too good? maybe we can use tail latency here, which is 3x}}


%In real-time video communication, such as video conferencing and cloud gaming, packet loss is hard to avoid, but retransmitting any packets can cause video stalls and user frustration, especially in long-latency networks.
%Many loss-resilient schemes exist, such as forward error correction (FEC) and receiver-side error recovery. 
%However, to tolerate packet loss, the sender must add redundancy or lower quality {\em before} packet loss occurs, which makes it difficult to decide when to prepare for packet loss and how much redundancy is appropriate.
%\passed{\fyy{I understand the high-level message this passage is trying to deliver, but it's not very clear.
%Consider 1) laying out the background more clearly by saying retransmission is infeasible on high-RTT networks due to the stringent latency requirement of RTC; 2) the remaining 
%(non-interactive) approaches to achieving loss resilience primarily comprise: a) \textit{forward} error correction at the encoder, and b) \textit{post-processing} error concealment at the decoder (according to \url{https://ieeexplore.ieee.org/document/664283}). The former faces the challenge of determining the redundancy rate prior to uncertain losses, whereas the latter requires sacrificing compression efficiency so as to enable reconstruction from partially received video. (Details can also be cut in the abstract and postponed to the intro.)}}

%This paper presents \name, a new real-time video communication system that uses a pair of neural encoder and neural decoder. 
%\passed{\fyy{This sentence does not summary the strengths of \name very well.}}
%The sender splits each encoded frame into packets such that any $x\%$ packet loss appear to be randomly masking $x\%$ of values in the encoder output. 
%\passed{\fyy{This sentence is very confusing since it is not immediately clear what is ``masking'' (a word not widely understood outside of the ML community) and more importantly, why doing so is beneficial. Instead of providing technical details, ideally a high-level intuition about how \name works should be given here.}}
%\name~{\em jointly trains} the neural encoder and decoder to optimize video quality when various fractions of values in the encoder output are masked at random.
%\passed{\fyy{I think this is the right level of details to put first. It can also be used to contrast with the encoder-heavy/forward approaches and decoder-heavy/post-processing approaches.}}
% that consists of a pair of neural encoder and neural decoder and a novel scheme to transform encoder output to packets. 
%In other words, with the same encoding output, \name optimizes video quality under various packet loss rates. 
%On a variety of test video content, we show that 
%%even though \name's encoder does not know the actual packet loss rate, 
%when no packet is lost, \name obtains quality similar to the codec used in WebRTC without FEC, and the quality gradually degrades but still better than state-of-the-art loss-resilient schemes under different packet loss rate. 
%Using real network traces, we show that \name reduces the number of non-recoverable frames and the stall duration by \fillme\% and  \fillme\% respectively, when compared with state-of-the-art loss-resilient schemes, such as Tambur (streaming FEC) and neural-net error concealment schemes.

%\name~{\em jointly trains} a pair of neural encoder and neural decoder to optimize video quality when various fractions of values in the encoder output are masked at random.
%In runtime, \name splits each encoded frame into packets such that any $x\%$ packet loss appear to be randomly masking $x\%$ of values in the encoder output. 


% significantly reduces the 95th percentile of frame delay (between encoding a frame and its decoding) by 2$\times$ when packet loss occurs compared to state-of-the-art loss-resilient schemes while achieving comparable quality. 
% This is because \name does not require retransmission of packets (unless all packets are lost) or skipping of frames.

\tempstrike{
With \name, {\em(i)} a video frame can be decoded, as long as {\em any} non-empty subset of its packets are received, and {\em(ii)} the quality gracefully degrades as more packets are lost, and {\em(iii)} approximates that of a standard codec (like H.265) in absence of packet loss.
%but {\em(iii)} without sacrificing the quality in absence of packet loss. 
%We refer to it as data-scalable (DS) coding.
To achieve this, \name encodes and decodes frames by using neural networks (NNs). 
It uses a new packetization scheme that makes packet loss appear to have the same effect as randomly masking (zeroing) a subset of elements in the NN-encoded output, and the NN encoder and decoder are specially trained to achieve decent quality if a random subset of elements in the NN-encoded output are masked. %set to zeros.
%, and uses a new packetization and entropy-coding scheme that makes packet loss appear to have the same impact of random zeroing on the NN-encoded output. 
%under different rates of random data erasure.
Using various test videos and real network traces, we show that 
%when combined with the same rate adaptation logic, 
the quality of \name is slightly lower than H.265 when no packets are lost, but significantly reduces the 95th percentile of frame delay (between encoding a frame and its decoding) by 2$\times$ when packet loss occurs compared to other loss-resilient schemes while achieving comparable quality. 
This is because \name does not require retransmission of packets (unless all packets are lost) or skipping of frames.
}



%We have also developed new schemes for packetization, packet queuing, and speeding up NN-based coding, to reduce frame delay and ensure graceful degradation of quality in presence of packet loss. 
%Using real network traces and a variety of test videos, we show that when combined with the same rate adaptation logic, \name has slightly lower quality than H.265 when no packets are lost, but significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to other loss-resilient schemes. 
%This is because \name does not require retransmission of packets (unless all packets are lost) or skipping of frames.


%a frame can be decoded with any non-empty subset of its packets, with the quality being close to that of H.265 if all packets are received, and degrading gracefully with fewer received packets.
%That is, no need to retransmit any packet or skip any frame, unless all packets of a frame are lost.
%More importantly, the sender does not explicitly decide how much error protection to add before sending a frame.
%This means that the sender does not explicitly decide how much error protection to add before sending a frame, 

%That is, there is no need to resend any packet or skip any frame unless all packets are lost.
%This means that using the same video coding, the video quality naturally degrades gracefully in the presence of packet loss, without compromising quality in the absence of packet loss.


%Our insight is that while existing autoencoders are not data-scalable, {\em they could be made so by novel training and packetization schemes}. 
%\name trains a new autoencoder by injecting random data erasures in its training.
%The output of the autoencoder is then packetized and individually entropy-encoded such that with when all packets arrive, \name's quality is only slightly lower than the traditional non-loss-tolerant coding (H.264/265), and that {\em with each missed packet, its quality degrades much more gracefully} than existing solutions.
%\name is complementary to the underlying congestion control logic and reaches better tradeoffs between frame delay and video quality than traditional loss-resilient video codecs. 
%% \name makes following contributions.
%% It trains new custom autoencoders to balance compression efficiency {\em and} resilience against a wide range of packet losses; and 
%% it uses a new transmission scheme to deliver autoencoder-coded frames as individually decodable packets.
%We test \name on real network traces and videos and show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces tail video frame delay (by 2$\times$ at the 95th percentile) with the marginally lowered video quality.

\end{abstract}


\begin{comment}

In real-time videos, resending {\em any} lost packets, particularly in long-latency networks, can cause low quality, video stuttering, and ultimately user frustration. 
Despite intense research, state-of-the-art real-time video systems have to sacrifice quality in absence of packet loss (\eg by adding redundancy) in order to achieve decent quality in presence of packet loss. 
Since packet loss is difficult to predict, they increase loss resilience only after packet loss occurs, leaving some frames insufficiently protected against packet loss after a burst of packet loss, and they may add too much redundancy even after packet loss disappears. 

%As a result of this tradeoff between compression efficiency and loss resilience, 

%have to trade lower video quality for resilience to more packet loss.
%As a result, they often increase loss resilience only after packet loss occurs.






We present \name, a new real-time video communication system. 
When {\em any} non-empty subset of a frame's packets are received, \name can decode the frame at a quality close to that of H.265 in absence of packet loss, and the quality degrades gracefully with more lost packets.
We refer to this as data-scalable (DS) coding.
To achieve it, \name first replaces the traditional video encoder and decoder with new loss-resilient neural networks (NNs) that are specially trained to gain decent quality under a range of erasure rates of coded data.
With these NN encoder and decoder, we develop new schemes for packetization and frame scheduling, such that frame delay is low and quality
%such that without resending packets (unless all packets are lost), \name's video quality 
degrades gracefully in the presence of packet loss, without compromising quality in the absence of packet loss.
%under various rate of data erasures on the encoded data, such that the decoded quality degrades gracefully under more data erasures. 
Using real network traces and a wide range of test videos, we show that when using the same rate adaptation logic, \name has marginally worse quality than H.265 when no packet is lost, but significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to other loss-resilient schemes, since \name does not need to retransmit packets (unless all packets are lost) or skip frames.
%because it retransmits fewer packets without explicitly adding loss-protection redundancy.


\end{comment}

\begin{comment}


Despite many prior efforts, most real-time Internet video systems increase loss resilience only {\em after} packet loss occurs.
This is because protecting against any packet loss will likely incur  redundancy in coded data and lower video quality when no packet is lost. 
As a result, frames are unlikely protected right after a burst of packet losses. 
Yet, in real-time video applications, resending {\em any} lost packets, particularly in long-latency networks, can 
%where
%%In online video calls and cloud gaming, 
%ideally each frame should be decoded soon after some of its packets are received. 
%{\em Any} lost or delayed packet can block a video frame and its subsequent frames, 
cause low quality, video stuttering, and ultimately user frustration. 
%The alternative is not desirable either: to keep a high loss resilience all the time means lower quality in absence of packet loss.
%if all packets arrive on time.
%Since it is hard to predict when, which or how many packets will be lost, 
%The result is that the sender has to either risk video stuttering or raise loss resilience (\eg by adding much error-correction redundancy) and lower quality even if all packets arrive.

%%which maintains high quality when no packet is lost while only retransmitting a few lost packets. 
%Yet, they fail to protect real-time video applications (\eg online conferencing and cloud gaming) against packet losses, because {\em any} lost or delayed packet may {\em directly} delay a real-time video frame and its subsequent frames, causing low quality, stuttering, and ultimately user frustration. 
%Since it is hard to predict when, which or how many packets will be lost, the sender has to either risk video stuttering or add much error-correction redundancy in coded data which lowers quality even if all packets arrive.


\end{comment}

\begin{comment}
\newpage 

However, real-time video applications, such as online conferencing and cloud gaming, are plagued with random bursts of packet losses or latency jitters. 
As a result, it is hard to predict when, which or how many packets will be missing when a frame is supposed to be decoded, causing video stutters, low quality, and ultimately user frustration.

Real-time video, such as online conferencing and cloud gaming, is plagued with random bursts of packet losses or latency jitters. 



%There has been intense research on real-time video communication, but they are either {\em reactive}---such as lowering bitrate or increasing FEC redundancy after losses occur---or too slow to 


In real-time videos, {\em any} packet can be lost or delayed at {\em any} time, making it difficult to maintain high quality against packet losses by bitrate adaptation or redundant coding.
Thus, a desirable coding and streaming system should be able to decode each frame if {\em any subset} (non-empty) of packets is received, achieve better quality with more received packets, and if all packets are received, reach similar quality as if the video is coded with minimum redundancy (\eg H.264).

Many real-time video applications today operate under high latency and/or dynamic bandwidth, causing bursts of packet losses that are hard to predict and avoid. 
To handle packet losses, an ideal loss-resilient video coding scheme should, {\em without retransmission}, be able to decode each frame if {\em any subset} (non-empty) of packets is received, achieve better quality with more received packets, and if all packets are received, reach similar quality as if the video is coded with minimum redundancy (\eg H.264).
We call it {\em data-scalable} coding (DSC).
%This is pressingly needed .
Unfortunately, existing techniques (\eg FEC, RS and Fountain Codes) fall short---they must reliably receive a minimum number of packets to decode a frame, and/or pad video data with a pre-determined rate of redundancy, which degrades video quality if all packets are received.
This work explores the possibility of an alternative approach to DSC, based on recent advances of neural-network video autoencoders.
Our insight is that while existing autoencoders are not data-scalable, {\em they could be made so by novel training and packetization schemes}. 
To show its promise, we present \name, a concrete DSC-based real-time video system.
\name trains a new autoencoder by injecting random data erasures in its training.
The output of the autoencoder is then packetized and individually entropy-encoded such that with when all packets arrive, \name's quality is only slightly lower than the traditional non-loss-tolerant coding (H.264/265), and that {\em with each missed packet, its quality degrades much more gracefully} than existing solutions.
\name is complementary to the underlying congestion control logic and reaches better tradeoffs between frame delay and video quality than traditional loss-resilient video codecs. 
% \name makes following contributions.
% It trains new custom autoencoders to balance compression efficiency {\em and} resilience against a wide range of packet losses; and 
% it uses a new transmission scheme to deliver autoencoder-coded frames as individually decodable packets.
We test \name on real network traces and videos and show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces tail video frame delay (by 2$\times$ at the 95th percentile) with the marginally lowered video quality.
\end{comment}



==> sections/old/eval.tex <==
\tightsection{Evaluation}

\tightsubsection{Experiment setup}
\begin{itemize}
    \item Testbed (simulation & emulation)
    \item Traces we used
    \item Baselines
\end{itemize}

\tightsubsection{Simulation (frame level)}
Frame level quality improvement compared with baselines
\begin{itemize}
    \item PSNR under different losses
    \item PSNR CDF for different frames (we have a better tail)
\end{itemize}

\tightsubsection{Trace-driven experiments (packet level)}
\begin{itemize}
    \item tail PSNR v.s. avg delay
    \item avg PSNR v.s. tail delay
\end{itemize}

\tightsubsection{Microbenchmark}
\begin{itemize}
    \item Improvement on different video type
    \item Improvement breakdown
\end{itemize}

==> sections/old/eval_sep20_4.24.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Evaluation}
\label{sec:eval}

Our key findings can be summarized as follows:
\begin{packeditemize}
\item {\bf Loss resilience:} \name's quality under no packet loss is on par with H.264 and H.265 and gracefully degrades with higher loss rates. 
Under 20-80\% packet loss, \name improves the SSIM by 1.4-4 dB at \fillme~Mbps compared to various loss-resilient baselines across diverse videos.
%\jc{this should be backed up with some concrete numbers, such as improve SSIM by xxx-xxx dB at \fillme packet loss rate}

\item {\bf Better video smoothness:} 
Under bandwidth fluctuations in real network traces, \name reduces the the number of video freezes over 200~ms by up-to 90\%, tail frame delay by up-to 2-4$\times$, and the non-rendered frames by up-to 95\%.
%has almost {\em zero} video stalls for over 200ms, which is up-to 90\% lower than loss-resilient baselines.
%Also, \name reduces the tail frame delay by 2-4$\times$ and the ratio of non-rendered frames by 95\%.
Our user study has also confirmed that \name's rated score is 38\% higher than the baselines. %\jc{please update this with new results.}

\item {\bf Speed:} Our implementation of \name can encode/decode 480p video at 87~fps/122~fps and 720p HD video at 31.2~fps/44.1~fps using Nvidia A40 GPU, 1.5-5$\times$ faster than recent autoencoder-based video codecs~\cite{swift, yang2020learning,shi2022alphavc, dvc}. 
% off-the-shelf autoencoders~\cite{swift, dvc}. 
With the optimization described in \S\ref{subsec:fast-coding}), \name can encode/decode 720p HD video at 41~fps/66~fps on CPU with marginal quality degradation on an iPhone 14 Pro. 
%\yc{this number is inaccurate since it does not consider h264 mv}
\end{packeditemize}


\tightsubsection{Setup}
\label{subsec:eval:setup}




% We build \name's autoencoder based on DVC~\cite{dvc}, a state-of-the-art video autoencoder. 
% We fine-tuned \name on the vimeo-90K~\cite{vimeo-dataset} dataset from the pretrained model of DVC. The fine-tuning takes two steps: we first fine-tuned a base model with packet losses applied during training.  
% Then, we employed 11 distinct $\alpha$s (in Eq.~\ref{eq:2}), ranging from $1/64$ to $1/32768$ to fine-tune the residual encoder and decoder. This enables \name to support various bitrates (\S\ref{subsec:fast-coding}). 
% We set the learning rate at $10^{-4}$, and each step of fine-tuning typically takes 1-2 hours on an Nvidia A40 GPU.
%\fyy{Besides fine-tuning DVC's pretrained model, are there other differences?} 

%Figure~\ref{fig:dvc-arch} shows the architecture of the encoder and decoder. On the sender side, the encoder neural network takes the current frame and its reference frame as the input, and outputs the encoded motion vectors and residuals (\S\ref{subsec:background}). On the receiver side, the decoder neural network decodes the received motion vector and residuals, then reconstructs the new frame based on the reference frame.
%\fyy{Why repeat Grace's design in the experimental setup? It's better to treat this paragraph as "implementation" and explain how DVC is adapted for this purpose.}


\mypara{Baselines}
We use H.265 (in \texttt{ffmpeg}, v4.2.7), a latest video codec that achieve better or comparable compression efficiency as VP8/9 and H.264~\cite{x265vp9compare, grois2013performance} (which we confirm in \S\ref{app:h26xvpx}), as the base codec of all baselines (except NVC-based ones).
We compare \name with a range of loss-resilient baseline that cover various approaches described in \S\ref{subsec:related}.
For space limits, more details are given in \S\ref{app:baseline}.
%\yihua{update text: rewrite baseline implementation}
%We implemented loss-resilient baselines using H.265 from \texttt{ffmpeg} (version 4.2.7), one of the most advanced video codecs, boasting comparable or superior compression efficiency to other widely-used codecs such as H.264, VP8, and VP9~\cite{x265vp9compare, grois2013performance} (We also confirmed this on our own testing videos in Appendix~\ref{app:h26xvpx}). 
%These baselines embody different design alternatives (\S\ref{subsec:related}) for loss-resilient video coding. 
%\ref{app:baseline} provides more details of the baseline implementation.
%\jc{did you forget to add the baseline that trains \name decoder only?}
%\jc{\name (ours) can be dropped from this list. move its details to the new implementation subsection please. maybe add more details to FEC and error concealment so that people can reimplement your baseline just based on the text here. (please note that important details CANNOT be put in appendix.)}
% We implemented the following loss-resilient baselines using H.265 of \texttt{ffmpeg} (version 4.2.7). It is worth noting that H.265 is one of the most advanced video codecs, having on-par or better compression efficiency compared to other widely-used codecs such as H.264, VP8 and VP9~\cite{x265vp9compare, grois2013performance}. The baselines are covering different design choices (\S\ref{subsec:related}) for loss-resilient video coding. Due to space limitations, we put the detailed baseline implementation (except \name) to Appendix~\ref{app:baseline}. %\yc{should I also bold the name of each baseline? Now the bolded texts are design choices.}
\begin{packeditemize}  
  \item {\bf Forward error correction}: 
  We use Tambur~\cite{rudow2023tambur}, a state-of-the-art FEC solution based on streaming codes~\cite{badr2017fec}.
%   with H.265.
The redundancy rate of Tambur, defined as $\frac{p}{n}$ (with $p$ as the number of parity packets and $n$ the total packets, including parity packets~\cite{xiao2012dynamic, lee2022r}), dynamically adapts based on the packet loss measured in the preceding 2 seconds. 
Compared to regular FEC, streaming codes reduce the number of non-decodable frames while transmitting an equivalent amount of parity packets.
We have also confirmed that Tambur outperforms the default FEC scheme of WebRTC,
%using the same logic as WebRTC\cite{WEBRTCSRC}. 
%\edit{We use the same logic as WebRTC to determine the redundancy rate, and confirms that Tambur outperforms the default FEC scheme used by WebRTC, because the use of streaming codes~\cite{rudow2023tambur, badr2017fec} reduces the number of non-decodable frames while transmitting an equivalent amount of parity packets as the default FEC scheme.}
   %This solution outperforms WebRTC's default FEC scheme, reducing the number of non-decodable frames while transmitting an equivalent amount of parity packets.
   %\jc{this sounds contradicting: it's using the same logic as webrtc to determine the redundancy rate, then why is it better? (i know the answer, but the text doesn't say it..)}
  %This approach, utilized in WebRTC\cite{WEBRTCSRC}, assures superior quality compared to a constant redundancy.
  %We implement Tambur~\cite{rudow2023tambur}, a state-of-the-art forward error correction solution using streaming code, with H.265\footnote{Following recent work in real-time video coding~\cite{ZEROLAT1,ffmpegstreaming}, we use the \texttt{zerolatency} option (no B-frames) and the \texttt{fast} preset of H.265. The command line we used to encode a video is \texttt{ffmpeg -y -i Video.y4m -c:v libx265 -preset fast -tune zerolatency -x265-params "crf=Q:keyint=3000" output.mp4} where {\em Q} controls the quality of the frame.}. It performs better than the default FEC scheme used in WebRTC since it decreases the number of non-decodable frames when sending the same amount of parity packets. According to the prior work~\cite{xiao2012dynamic}, we define the redundancy rate of Tambur as $\frac{p}{n}$ where $p$ is the number of parity packets $n$ is the total number of packets (including parity packets). The redundancy rate is dynamically set based on the packet loss measured in the previous 2 seconds, which is also used in WebRTC~\cite{WEBRTCSRC} and has better quality compared with adding a constant redundancy.
  
  % We implement Tambur~\cite{rudow2023tambur} with H.265\footnote{Following recent work in real-time video coding~\cite{ZEROLAT1,ffmpegstreaming}, we use the \texttt{zerolatency} option (no B-frames) and the \texttt{fast} preset of H.265. The command line we used to encode a video is \texttt{ffmpeg -y -i Video.y4m -c:v libx265 -preset fast -tune zerolatency -x265-params "crf=Q:keyint=3000" output.mp4} where {\em Q} controls the quality of the frame.}, and we do not restrict their GoP (I-frame interval), a state-of-the-art forward error correction solution using streaming code. \fyy{We only had one key frame at the very beginning of a video session and did not have any GoP. Putting that aside, this detail is still unnecessary if you don't/can't justify why a state-of-the-art approach is not adopted.} Tambur performs better than the default FEC scheme used in WebRTC since it can decrease the number of non-decodable frames when sending the same amount of parity packets. According to the prior work~\cite{xiao2012dynamic}, we define the redundancy rate of Tambur as $\frac{p}{n}$ where $p$ is the number of parity packets $n$ is the total number of packets (including parity packets). According to WebRTC~\cite{WEBRTCSRC}, the redundancy rate is dynamically set based on the packet loss measured in the previous 2 seconds, which has better quality compared with adding a constant redundancy.
  %\yc{mention the redundancy rate is determined by webrtc logic, either here or in the simulation section}
  
    
  \item {\bf Neural error concealment}: 
  We use ECFVI~\cite{kang2022error}, one of the state-of-the-art NN-based error concealment methods, which surpasses the prior works that recover motion estimation~\cite{sankisa2018video} or use inpainting~\cite{chang2019free}.\footnote{A parallel work, Reparo~\cite{reparo}, claims decent error concealment on a specific type of video (talking head), but it does not compare with any NN-based baselines and there is no public codebase to test it.} 
  \edit{To make each packet independently decodable, we apply the flexible macroblock ordering (FMO~\cite{dhondt2004flexible}) technique, splitting the frame into $64\times64$-pixel\footnote{A smaller block size such as $16\times16$ pixels greatly inflates the frame size~\cite{kumar2006error, wenger2002scattered, 4494082}, while a larger block size such as $256\times256$ will loss too much information upon packet loss, making it difficult for the model to conceal errors. We empirically select the block size to be $64\times64$ pixels to balance the tradeoff between the frame size and the quality.}
  blocks and mapping them randomly to packets.
  The use of FMO increases the size of the encoded frame by 10\%, which corroborates with the previous works~\cite{kumar2006error, wenger2002scattered, 4494082}.
  After decoding the incomplete frame, }ECFVI uses neural networks to both estimate the missing motion vector and enhance the reconstructed frame by inpainting. 
  %According to the prior works~\cite{kumar2006error, wenger2002scattered, 4494082}, we assume an extra 10\% size overhead to make sure each packet is individually decodable. \jc{should mention FMO and the block sizes, and justify the choices.}
  %Details about how we implement this baseline can be found in Appendix~\ref{app:baseline}. 
  %\jc{need more details here, how to packetize, what's exactly the impact of loss on a frame? why is it representative? is it fair to Grace? if it's too long, you can put it in appendix and refer to it here} %as the per-packet entropy coding technique.
  %Error concealment recovers quality from the packet loss by predicting the missing content using hand-tune heuristics~\cite{zhou2010efficient, varsa2001non} or neural networks~\cite{kang2022error, sankisa2018video, mathieu2015deep}. Error concealment methods need to work with per-packet entropy coding techniques such as flexible macroblock ordering~\cite{KUMAR2006425} because it requires an incomplete frame to be decodable. 

  %The baseline encodes/decodes the video using H.265. When there is an incomplete frame, the baseline takes 3 steps to conceal the errors. It will first use a neural network to estimate the motion vector of the missing part based on previous frames. Then, it will propagate the missing pixel values from the reference frame with the estimated motion vector. Finally, it will use an inpainting neural network to improve the frame quality and reduce error propagation. It is better than motion-prediction-only or inpainting-only error concealment methods (\cite{sankisa2018video, mathieu2015deep}). We also assume a \fillme\% size overhead caused by the per-packet entropy coding, which matches the overhead mentioned in~\cite{??}.
  
  \item {\bf Scalable video coding (SVC)}: %SVC encodes a video at multiple quality layers and sends data layer by layer. 
  We implement an idealized SVC, such that when the first $x$ layers arrive, it will reach a quality the same as that of H.265 at receiving the same amount of bytes. 
  This idealized implementation is better than the state-of-the-art NN-based SVC~\cite{swift}. 
  We also add 50\% FEC to protect the base layer for SVC, following a common practice in real-time videos~\cite{khalek2012cross}.


  
  \item {\bf Selective frame skipping}: 
  % One potential design choice of selective frame skipping is optimizing the frame delay by only retransmitting the important frames that will cause huge damage to the video quality when missing. 
  We implement two recent baselines. 
  % for this design choice based on Voxel~\cite{voxel} and Salsify~\cite{salsify}.
  Salsify~\cite{salsify} can skip the loss-affected frames at the decoder side after the encoder receives the packet loss indication and resends a new p-frame using the last fully received frame as a reference.
  Voxel~\cite{voxel} uses selective frame skipping to reduce the video rebuffering ratio and improve the user's QoE.
%  We provide more details about their implementation in Appendix~\ref{app:baseline}.


%\jc{seems too much space spent on a minor baseline. shrink it please?}
  
  %Unlike traditional codecs (\eg, H.265 or VP9), functional codecs are able to skip incomplete frames when packet loss happens and decode the first complete frame without a significant quality drop. Salsify~\cite{salsify} is a recent work implementing the functional codec. 
  %We implement the Salsify baseline based on H.265 with the following features: {\em (i)} the encoded frame size of the codec will never overshoot the target bitrate calculated by the underlying congestion control algorithm, and {\em (ii)} when packet loss happens, the encoder can dynamically choose a reference frame to make later frames decodable without retransmitting any packets.

%  \edit{We show more details about how to integrate \name and SR in Appendix~\ref{app:sr}.}
  %We use a state-of-the-art SR model, SwinIR~\cite{swinir}, as the tool to improve the video quality for both \name and other baselines after the receiver successfully decodes the frame. \yc{consider move it to 5.5}

\end{packeditemize}
% For the baselines of functional codec (Salsify), SVC, and selective frame skipping (Voxel), we make an idealized assumption that on each frame, the output bitrate of the codec perfectly matches the target bitrate chosen by the congestion control algorithm (explained in \S\ref{subsec:eval:e2e}), \ie never overshooting or undershooting, but the actual quality matches that of the highest \texttt{qp} that leads to a frame greater than the target bitrate. 
% We used an idealized version of functional codec (Salsify), SVC, and selective frame skipping (Voxel) baselines. 
We also made an idealized assumption in favor of SVC, Salsify, and Voxel that 
the codec's output bitrate on every frame flawlessly aligns with the target bitrate determined by the congestion control algorithm (\S\ref{subsec:eval:e2e}), \ie no overshoots or undershoots in a real codec.
This assumption makes these baselines perform slightly better than they should.

\mypara{Variants of \name} 
\edit{
To highlight the impact of different ideas, we also test \textbf{\namepretrain} and \textbf{\namedecoder}, which are trained the same way as \name except that \namepretrain does not use simulated loss, whereas \namedecoder freezes the encoder NN weights (\ie fine-tuning only the decoder NN with simulated loss).
They serve as a reference for alternative ways of simulating packet loss in training. 
In addition, we also test \textbf{\namelite}, which uses the optimizations described in \S\ref{subsec:fast-coding}.}
% We also implement and test the following variants of \name proposed in \S\ref{sec:core} and \S\ref{subsec:fast-coding}. \textbf{\namepretrain}: \name trained without seeing any packet loss. \textbf{\namedecoder}: \name trained with packet loss solely on the decoder side. \textbf{\namelite}: \name with the speedup optimizations in \S\ref{subsec:fast-coding}.



We also test the quality improvement of the state-of-the-art super-resolution (SR) model~\cite{liang2021swinir} on \name and its baselines.
Since SR can be applied to any decoded frames, it is {\em orthogonal} to \name's design space. 
For space limits, we elaborate the details of this experiment in \S\ref{app:sr}.


% However, the actual quality corresponds to the highest \texttt{qp} resulting in a frame size exceeding the target bitrate.
% These optimizations make the baselines' performance slightly better.
% In other words, their performance is higher than it would actually be in the real world.

\mypara{Testbed implementation}
Our testbed has 2 Nvidia A40 GPUs to run the video encoding and decoding with \name's NVC (each using one GPU).
We use a packet-level network simulator to compare \name with baselines under various network conditions. The simulator uses a configurable drop tail queue to mimic congestion-induced packet losses and uses a token bucket scheme to simulate bandwidth variation every 0.1 seconds. Google Congestion Control (GCC)~\cite{carlucci2016analysis}, a standard WebRTC algorithm, is used to determine the target bitrate of video codecs at each frame.
\jc{Yihua, can we bring back the result with Salsify CC? given there are many recent papers on improving cc for conferencing, people may wonder if GCC is too outdated..}
\yc{claim the following things to protect ourself: GCC is SOTA and widely used, GCC is very responsive to bandwidth drop and loss, (maybe we can also mention network have random loss)}
The simulator includes 
%emulates a complete real-time video communication application, including 
encoding, packetization, rate adaptation, and decoding.
We set the default frame rate at 25fps (on par with typical RTC frame rates~\cite{macmillan2021measuring}), though \name can encode at a higher frame rate (\S\ref{subsec:eval:micro}).
% (matching state-of-the-art real-time video measurements~\cite{macmillan2021measuring}). 
% The packets are transmitted over a network simulated by the simulator. 
It records each decoded frame and its delay, including encoding, transmission, and decoding. We confirmed our simulator's accuracy regarding frame delay via a real-world validation experiment in the appendix (\S\ref{subsec:eval:e2e}).


% To compare \name and the baselines under different network scenarios, we implemented a packet-level network simulator. 
% The simulator uses a drop tail queue with a configurable queue length to simulate packet losses caused by the congestion. It implements the token bucket algorithm to simulate the bandwidth variation at a frequency of 0.1 seconds.
% To determine the target bitrate of the video codecs used during simulation, we implemented Google congestion control~\cite{carlucci2016analysis} (\textit{GCC}), the standard congestion control algorithm used in WebRTC. %and the congestion control from~\cite{salsify} (\textit{Sal-CC}). 

% During the runtime, the simulator takes as input a bandwidth trace and a video. It {\em emulates} the {\em end-to-end} real-time video communication application, including encoding, packetization, sending rate adaptation, and decoding. The encoder is running at 25fps, matching the measurements from the state-of-the-art real-time video measurement~\cite{macmillan2021measuring}. The encoded packets are sent over a simulated network controlled by the simulator. 
% The output of the simulator includes a decoded video and the end-to-end delay of each decoded frame (including the time used for encoding and decoding). We also validated that the frame delay produced by our simulator is accurate by running a real-world validation experiment (in \S\ref{subsec:eval:e2e}).



% \begin{table*}
% \begin{centering}
% \small
% \begin{tabular}{ccccc}
% \toprule
% Dataset & \#videos & Duration (s) & Resolution & Characteristics \\
% \midrule
% Kinetics~\cite{Kinetics} & 49 & 490 & 1280$\times$720 and 640$\times$360 & Human actions and interaction of objects \\
% GamingVideoSet~\cite{barman2018gamingvideoset} & 6 & 180 & 1920$\times$1080 & High quality PC game recordings \\
% UVG~\cite{mercat2020uvg} & 5 & 120 & 1920$\times$1280 & HD videos (human, nature, sports, etc.) \\
% FVC~\cite{FVCDATASET} & 6 & 135 & 1920$\times$1080 & Video calls (indoor and outdoor) \\
% \midrule
% Total & 66 & 925 & & \\
% \bottomrule
% \end{tabular}
% \vspace{0.3cm}
% \tightcaption{Dataset description 
% % \jc{YIHUA: 3. add citation, 4. in text, add a link to the data repo (github). ask zhengxu (anonymized)}
%  }
% % \vspace{-0.8cm}
% \label{tab:dataset}
% \end{centering}
% \end{table*}

\begin{table}[]
\begin{centering}
\begin{tabular}{ccccc}
\toprule
Dataset                                           & \begin{tabular}[c]{@{}c@{}}\# of\\ videos\end{tabular} & Length (s) & Size                                                & Description                                                                             \\ \hline
\midrule
{\color[HTML]{000000} Kinetics}                   & 45                                                     & 450 & \begin{tabular}[c]{@{}c@{}}720p\\ 360p\end{tabular} & \begin{tabular}[c]{@{}c@{}}Human actions \\ and interaction\\ with objects\end{tabular} \\ \hline
\multicolumn{1}{l}{{\color[HTML]{000000} Gaming}} & 5                                                      & 100 & 1080p                                               & \begin{tabular}[c]{@{}c@{}}PC game\\ recordings\end{tabular}                            \\ \hline
{\color[HTML]{000000} UVG}                        & 5                                                      & 100 & 1080p                                               & \begin{tabular}[c]{@{}c@{}}HD Videos \\ (human, nature, \\ sports, etc.)\end{tabular}   \\ \hline
{\color[HTML]{000000} FVC}                        & 5                                                      & 100 & 1080p                                               & \begin{tabular}[c]{@{}c@{}}Video calls\\ (indoor/outdoor)\end{tabular}                  \\ 
\midrule
Total                                             & 60                                                     & 750 &                                                     &   \\                                                                                     
\bottomrule
\end{tabular}
\tightcaption{Dataset description}
\label{tab:dataset}                               
\end{centering}
\end{table}

\mypara{Test videos}
Our evaluation uses 60 videos randomly sampled from four public datasets, summarized in Table~\ref{tab:dataset}.\footnote{We share the videos in an anonymous link\jc{Yihua please add it here}.}
The total content length is 750 seconds where each video is 10-30 seconds long, matching the setup of similar works~\cite{salsify, rudow2023tambur, conti2021not}.%\jc{Yihua, please fix}
%The video content includes human actions in different environments, video game recordings, nature scenes, sports, as well as indoor and outdoor video calls. 
%The detailed description of the datasets is in Table~\ref{tab:dataset}.
Importantly, these videos are obtained from entirely different sources than the training set, and they span a range of spatial complexity and temporal complexity (detailed in \S\ref{app:siti}), as well as multiple resolutions.
This diversity allows us to assess \name's average performance across different contents and study how content affects its performance.

%allow us to thoroughly assess the generalization capabilities of autoencoders. They encompass various spatial and temporal dynamics (discussed in \S\ref{app:siti}), across multiple resolutions, ensuring a minimum of 5 videos per resolution. The reported performance constitutes an average across all video frames.


\mypara{Network traces}
We test \name and the baselines on 16 real bandwidth traces, eight of which are LTE traces from the Mahimahi network-emulation tool~\cite{netravali2015mahimahi},
and the rest are broadband traces from FCC~\cite{fcc-dataset}.
The bandwidth fluctuates between 0.2~Mbps to 8~Mbps in the traces.
By default, we set the one-way propagation delay to 100ms and the queue size to 25 packets. We will also vary these values to show their impact in \S\ref{subsec:eval:e2e}.


\mypara{Metrics}
Following the prior studies about real-time video communication~\cite{rudow2023tambur, salsify} and user QoE~\cite{garcia2019understanding, garcia2020assessment, ammar2016video}, we measure the performance of a video session in the following three aspects.
\begin{packeditemize}
    \item {\em Quality}: is measured by frame-level SSIM, reported as the average across received frames. Conforming to recent related work~\cite{salsify}, we express SSIM values in dB (obtained by $-10\log(1 - \text{SSIM})$).
    %{\em Quality} of a video is measured by frame-level SSIM, and we report the average value across received frames. Following the recent related work~\cite{salsify}, we report the SSIM values in dB\footnote{We use $-10 * log(1 - SSIM)$ to calculate the corresponding dB values.}. 
    \item {\em Realtimeness} is measured via the tail of frame delay and the ratio of non-rendered frames. Frame delay represents the time from encoding commencement to decoding completion. Non-rendered frames are either undecodable (\eg insufficient FEC protection) or arriving too late (\ie over 400ms after the frame is encoded).
%    , and thus not displayed by the receiver.
    %is measured by the tail of end-to-end frame delay and the ratio of non-rendered frames. End-to-end frame delay means the time lapse between the beginning of encoding and the end of decoding. Non-rendered frames refer to frames that are not played by the receiver due to not being decodable or arriving too late (more than 200ms after the previous frame).
    \item {\em Smoothness} of the video is measured by video stalls.
%    where a video stall is defined as the fraction of inter-frame gaps that exceed a threshold. 
    Following the previous work~\cite{macmillan2021measuring} and the convention of WebRTC, we define a video stall as an inter-frame gap over 200ms. 
    We report the average count of video stalls per second, and the ratio of video stalls is defined as the percentage of time that the video is spent in the stalls.
    %We choose this threshold as it matches the definition in WebRTC. 
\end{packeditemize}


%Table~\ref{sec:??} summarizes the datasets.
% Importantly, we choose these videos because they are different from the training set, allowing us to stress-test the generalization of autoencoders.
% These videos cover a range of spatial and temporal dynamics (details are shown in \S\ref{app:siti}), 
% and also cover multiple resolutions, with at least 5 videos in each resolution. 
% The performance is reported as an average across all the frames in the videos.
% \fyy{The video dataset can be justified briefly, leaving details to the appendix.}


% \begin{figure}[t!]
%      \centering
%      \includegraphics[width=1\linewidth]{figs/ssim-loss-v4.pdf}
%      \vspace{-0.2cm}
%      \tightcaption{\name's loss resilience for different bitrates and different number of lossy frames.
%      \fyy{Figures shouldn't be too dense: 1) font size should be readable; 2) information should be easy to parse,
%      e.g., avoid including too many subfigures. This figure is the primary results, but think about how long it would 
%      take a reader to understand the takeaway. Some secondary results should simply moved to the appendix.}}
%      \label{fig:loss_by_bitrate}
%      \vspace{-0.1cm}
% \end{figure}

\begin{figure*}[t!]
     \centering
     \includegraphics[width=\linewidth]{figs/ssim-loss-dataset.pdf}
     \vspace{-0.3cm}
     \tightcaption{Comparing \name's loss resilience to baselines on different datasets, bitrate is 6~Mbps.}
     \label{fig:loss_by_dataset}
\end{figure*}

\begin{figure}[t!]
     \centering
     \includegraphics[width=\linewidth]{figs/ssim-loss-bitrate.pdf}
     \vspace{-0.3cm}
     \tightcaption{Comparing \name's loss resilience to baselines on different bitrates.}
     \label{fig:loss_by_bitrate}
\end{figure}

% \begin{figure}[t!]
%      \centering
%      \includegraphics[width=\linewidth]{figs/ssim-loss-v6.pdf}
%      \tightcaption{\name has a better loss resilience than other baselines on different bitrates.\jc{no need to emphasize "1 frame"}\yc{no markers, no grid, bolder lines, Y-axis closer to Y-label}}
%      \label{fig:loss_by_bitrate}
%      \vspace{-0.1cm}
% \end{figure}

% \begin{figure*}[t!]
%      \centering
%      \includegraphics[width=\linewidth]{figs/test1.pdf}
%      \vspace{-0.3cm}
%      \tightcaption{test ssim vs size}
%      \label{fig:test1}
% \end{figure*}

% \begin{figure*}[t!]
%      \centering
%      \includegraphics[width=\linewidth]{figs/test2.pdf}
%      \vspace{-0.3cm}
%      \tightcaption{test ssim vs loss}
%      \label{fig:test2}
% \end{figure*}

% \begin{figure*}[t!]
%      \centering
%      \includegraphics[width=\linewidth]{figs/test2.pdf}
%      \vspace{-0.3cm}
%      \tightcaption{test ssim vs loss}
%      \label{fig:test3}
% \end{figure*}



\begin{figure}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/stress-test.pdf}
    \tightcaption{\name can maintain the frame quality when packet losses happen consecutively on more than 10 frames without encoder/decoder synchronization. \yc{this is really weird}}
    %\jc{The axis should be "\# of consecutive frames with xxx\% packet loss. it should start from where they diverge"}}
    \label{fig:stress-test}
\end{figure}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/loss-visualization-example-early.pdf}
    \tightcaption{Example decoded images using \name and error concealment when there are 50\% packet loss on 3 consecutive frames. \name has less image distortion and maintains a higher SSIM compared to the baseline.}
    \label{fig:early-visual-example}
\end{figure}

\tightsubsection{Compression efficiency and loss resilience}
\label{subsec:eval:resilience}

\mypara{Loss resilience of \name}
We first compare \name with the baselines under different packet loss rates and different bitrates. 
We align the encoding bitrate of all the baselines with differences controlled within 5\%.
We ensure that \name's encoded bitrate is {\em never} higher than the baselines, so even if the actually encoded bitrate is different, it does not favor \name. 

The most salient feature of \name is the graceful quality degradation with more packet losses. 
As shown in Figure~\ref{fig:loss_by_bitrate}a and~\ref{fig:loss_by_bitrate}b, The average SSIM drop is only 0.5 dB to 2 dB when packet loss changes from 20\% to 50\% and the packet loss only impacts a single frame.
Even when the loss ratio is as high as 80\%, \name can still have an average SSIM of 12~dB across different bitrates, which is much better than H.265 with various FEC redundancy rates. 
It also significantly outperforms SVC, because if a packet from the lower layer is lost, all the higher layers will not be decodable when using SVC. 

We further contrast \name with the machine-learning-based error concealment solution (\S\ref{subsec:eval:setup}). \name consistently surpasses these baselines by 0.8-2.4 dB higher SSIM, a result attributable to the joint encoder-decoder training process that makes it able to reconstruct pixels more accurately. 

\edit{
In real-world scenarios, packet loss sometimes can affect multiple consecutive frames~\cite{rudow2023tambur}.
Therefore, we subjected \name to a rigorous test, simulating an extreme scenario where consecutive frames experience persistent packet loss, and the encoder and decoder remain unsynchronized. 
As depicted in Figure~\ref{fig:stress-test}, \name markedly surpasses the NN-based error concealment baseline in such conditions. 
At persistent packet loss rates of both 30\% and 50\%, \name achieves an SSIM that is 2-3~dB higher than the baseline. 
While the quality for both \name and the error concealment method deteriorates as more frames are affected by packet loss, \name's decline is considerably more gradual. 
Remarkably, it maintains satisfactory quality for over 10-15 frames.
Figure~\ref{fig:early-visual-example} gives a visualization example of the decoded image when there is 50\% packet loss on 3 consecutive frames. 
Compared to the NN-based error concealment baseline, \name achieves both higher SSIM and less visual distortion.
}

% Figure~\ref{fig:loss_by_bitrate}c and~\ref{fig:loss_by_bitrate}d compares \name and the baselines when x\% packet loss occurs across all 3 (or 5) consecutive frames.
% \name also outperforms the baselines, achieving a higher SSIM up to 2~.5dB over different loss rates between 10\% and 80\%.


% We subjected \name to a rigorous test, simulating an extreme scenario where consecutive frames experience persistent packet loss, and the encoder and decoder remain unsynchronized. 
% As depicted in Figure~\ref{fig:stress-test}, \name markedly surpasses the NN-based error concealment baseline in such conditions. 
% At persistent packet loss rates of both 30\% and 50\%, \name achieves an SSIM that is 2-3~dB higher than the baseline. 
% While the quality for both \name and the error concealment method deteriorates as more frames are affected by packet loss, \name's decline is considerably more gradual. 
% Remarkably, it maintains satisfactory quality for over 10-15 frames.

% We also evaluated \name's loss resilience on different bitrates. The detailed results are put in Appendix~\ref{app:??} due to space constraints.


% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[t]{0.48\linewidth}
%         \includegraphics[width=\linewidth]{figs/ssim-bpp-kall.pdf}
%         \tightcaption{SSIM vs. bitrate for Kinetics dataset}
%         \label{fig:}
%         % \vspace*{3mm}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.48\linewidth}
%         \includegraphics[width=1.05\linewidth]{figs/ssim-bpp-game.pdf}
%         \tightcaption{SSIM vs. bitrate for gaming dataset}
%         \label{fig:}
%         % \vspace*{3mm}
%     \end{subfigure}
    
%     \begin{subfigure}[b]{0.48\linewidth}
%         \vspace*{3mm}

%         \includegraphics[width=1.05\linewidth]{figs/ssim-bpp-fvc.pdf}
%         \tightcaption{SSIM vs. bitrate for FVC dataset}
%         \label{fig:}
%     \end{subfigure}
%     % \begin{subfigure}[b]{0.48\linewidth}
%     %     \includegraphics[width=\linewidth]{figs/psnr-bpp-fvc.pdf}
%     %     \tightcaption{PSNR vs. bit per pixel for FVC dataset}
%     %     \label{fig:}
%     % \end{subfigure}
%     \begin{subfigure}[b]{0.48\linewidth}
%         \includegraphics[width=1.05\linewidth]{figs/ssim-bpp-uvg.pdf}
%         \tightcaption{SSIM vs. bitrate for UVG dataset}
%         \label{fig:}
%     \end{subfigure}
%     \vspace*{4mm}

%     \tightcaption{Quality-size tradeoff of \name.}
%     \vspace{-0.1cm}
%     \label{fig:psnr-vs-bpp}
% \end{figure}




\mypara{Compression efficiency of \name} 
% For any loss-resilient schemes, 
There is always a tradeoff between compression and loss resilience, and \name is no exception. 
We assessed \name's quality under zero packet loss, juxtaposed with H.264 and H.265, using the test videos from Table~\ref{tab:dataset}. 
As indicated in Figure~\ref{fig:psnr-bpp}, \name aligns closely with H.264 and marginally underperforms H.265. 
In comparison with the baseline using Tambur that applies a constant 50\% redundancy to tolerate up to 50\% packet losses, \name offers a superior quality-bitrate trade-off, implying improved video quality at identical bitrates. 
Furthermore, \name spans a broad bitrate range across all datasets, from 0.25Mbps to over 10Mbps.

\edit{
To delve deeper into the nuances of \name's compression efficiency, we evaluated the quality difference between \name and H.264 on video frames grouped by their spatial index (SI) and temporal index (TI)\cite{itu1999subjective}. 
SI and TI are well-established metrics assessing the spatiotemporal complexity of videos, with higher SI/TI values indicating greater spatial/temporal complexities. 
While \name's overall compression efficiency marginally surpasses H.264, Figure\ref{fig:generalization-study} reveals a notable trend: \name significantly outperforms H.264 for low-SI videos but lags behind for high-SI videos. 
This trend can be attributed to two factors. 
Firstly, using convolutional neural networks, \name's NN encoder excels when motion and residuals are smooth, \eg neighboring values are close to each other. 
Low SI videos typically exhibit this smoother motion and residual pattern compared to their high SI counterparts. 
Secondly, in order to achieve loss resilience in high SI videos, \name's encoder introduces additional redundancy, which inadvertently compromises compression efficiency.
}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/ssim-bpp-short.pdf}
    \tightcaption{Quality-size tradeoff of \name on videos with different resolution. \name is better than H.264 and slightly worse than H.265 in terms of compression efficiency.}
    \label{fig:psnr-bpp}
\end{figure}

% \begin{figure*}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{figs/ssim-bpp-all-long.pdf}
%     \tightcaption{Quality-size tradeoff of \name on different datasets. \name is better than H.264 and slightly worse than H.265 in terms of compression efficiency. \yc{show 1080P and 720P}}
%     \label{fig:psnr-bpp}
% \end{figure*}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.75\linewidth]{figs/siti-heatmap.pdf}
    \tightcaption{Average quality difference on SSIM (dB) between \name and H.264 on videos grouped by SI and TI when the bitrate is 5~Mbps. At the same bitrate, \name has a better quality than H.264 on low-SI videos, but lags behind H.264 on high-SI videos.\yc{try 265}}
    \label{fig:generalization-study}
\end{figure}


\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/e2e-sim-short.pdf}
    \vspace{-0.2cm}
    \tightcaption{End-to-end simulation result on covering different network trace datasets, one-way-delay and network queue length. (a) and (b) shows the impact of the network trace dataset. (a) and (c) shows the impact of one-way-delay. (a) and (d) shows the impact of network queue length. On different setups, \name outperforms baselines in terms of the tradeoff between video stall ratio and video quality \yc{fix italic and FCC}}
     \label{fig:gcc-delay-simulation}
\end{figure}

\begin{comment}
\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
         \centering
         \includegraphics[width=2\linewidth]{figs/gccstall-queue25-delay50-long.pdf}
         \tightcaption{One-way delay = 50ms}
         \label{fig:gcc-50-25}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.49\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay100.pdf}
         \tightcaption{One-way delay = 100ms}
         \label{fig:gcc-100-25}
     \end{subfigure}
     \hfill
     \vspace{0.5cm}
     \tightcaption{End-to-end simulation result under different one-way delay. Network queue length = 25 packets \yc{show (100, 25, LTE), (100, 25, FCC), (100, 35, LTE), (50, 25, LTE) and explicitly say comparing (a) and (b) we can get xxx}}
     \label{fig:gcc-delay-simulation}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
         \centering
         \includegraphics[width=2\linewidth]{figs/gccstall-queue15-delay100-long.pdf}
         \tightcaption{Queue = 15 packets}
         \label{fig:gcc-100-15}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.49\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue35-delay100.pdf}
         \tightcaption{Queue = 35 packets}
         \label{fig:gcc-100-35}
     \end{subfigure}
     \hfill
     \vspace{0.5cm}
     \tightcaption{End-to-end simulation result under different network queue lengths. One-way delay = 100ms }
     \label{fig:gcc-queue-simulation}
\end{figure}


\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=4\linewidth]{figs/gccstall-queue25-delay50-long.pdf}
         \tightcaption{One-way delay = 50ms}
         \label{fig:gcc-50-25}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay75.pdf}
         \tightcaption{One-way delay = 75ms}
         \label{fig:gcc-75-25}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay100.pdf}
         \tightcaption{One-way delay = 100ms}
         \label{fig:gcc-100-25}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.24\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay100.pdf}
         \tightcaption{One-way delay = 150ms}
         \label{fig:gcc-150-25}
     \end{subfigure}
     \hfill
     \vspace{0.5cm}
     \tightcaption{End-to-end simulation result under different one-way delay. Network queue length = 25 packets
     \fyy{Again, there are too many subfigures to parse. Use the fewest figures to convey the takeaway.}}
     \label{fig:gcc-delay-simulation}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=4\linewidth]{figs/gccstall-queue15-delay100-long.pdf}
         \tightcaption{Queue = 15 packets}
         \label{fig:gcc-100-15}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay100.pdf}
         \tightcaption{Queue = 25 packets}
         \label{fig:gcc-100-25}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue35-delay100.pdf}
         \tightcaption{Queue = 35 packets}
         \label{fig:gcc-100-35}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.24\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue45-delay100.pdf}
         \tightcaption{Queue = 45 packets}
         \label{fig:gcc-100-45}
     \end{subfigure}
     \hfill
     \vspace{0.5cm}
     \tightcaption{End-to-end simulation result under different network queue lengths. One-way delay = 100ms}
     \label{fig:gcc-queue-simulation}
\end{figure*}
\end{comment}






%\jc{
%\begin{itemize}
%    \item by bitrate
%    \item by video set
%    \item psnr vs. bitrate
%\end{itemize}
%}

% \jc{need a footnote to explain why intra-mb insertion is so bad}








\tightsubsection{Video quality vs. realtimeness/smoothness}
\label{subsec:eval:e2e}

% To determine the target bitrate of the video codecs used during simulation, we implemented two different congestion control algorithms: Google congestion control~\cite{carlucci2016analysis} (\textit{GCC}, the standard congestion control used in WebRTC) and the congestion control from~\cite{salsify} (\textit{Sal-CC}). 
%We also implemented FEC-protected H.265 and Salsify codec as the baseline codecs (\S\ref{subsec:eval:setup}).

% Figure~\ref{fig:gcc-delay-simulation} and Figure~\ref{fig:gcc-queue-simulation} 
\name's loss resilience and the ability to decode incomplete frames make it achieve a better quality vs realtimeness or smoothness tradeoff than the baselines, as it does not require any retransmission. 

We evaluated \name against baselines in terms of average quality (SSIM) and video stall ratio using LTE traces under different network delays (50ms and 100ms) and queue lengths (spanning 15 to 35 packets). 
As depicted in Figures~\ref{fig:gcc-delay-simulation} and~\ref{fig:gcc-queue-simulation}, \name significantly reduces the video stall ratio compared to the baselines. Under all network conditions, \name maintained a video stall ratio below 0.5\%, while the baselines ranged from 2\% to 16\%. 

The primary cause of video stalls is congestion-induced packet loss. When packets are lost, Salsify must skip frames, resulting in increased delay, while H.265 awaits retransmission of lost packets, increasing delay and competing with regular video traffic. 
Although Tambur has a much smaller video freeze ratio, matching the results in their paper, it does not solve the fundamental limitation of FEC-based solution: when unpredictable congestion losses are higher than the protection rate, it still causes significant video stalls.
SVC and Voxel also wait for retransmission if the base layer is damaged or a crucial frame is lost. \name, however, can decode a frame as long as any packet from that frame is received.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.325\linewidth}
         \centering
         \includegraphics[width=3\linewidth]{figs/tail-latency-long.pdf}
         \tightcaption{Tail frame latency}
         \label{fig:tail-latency}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.325\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/non-rendered-frames.pdf}
         \tightcaption{\% of non-rendered frames}
         \label{fig:non-rendered-frames}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.325\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/frequency-of-stalls.pdf}
         \tightcaption{Average stalls/sec (\name <0.001)}
         \label{fig:frequency-of-stalls}
     \end{subfigure}
     \hfill
     \vspace{0.3cm}
     \tightcaption{End-to-end simulation result shows \name outperforms other baselines on various metrics of realtimeness and smoothness.}
     \label{fig:other-metrics}
\end{figure}

% \begin{figure}[t!]
%      \begin{subfigure}[b]{0.48\linewidth}
%          \centering
%          \includegraphics[width=2\linewidth]{figs/fcc-gccdelay-queue25-delay100-long.pdf}
%          \tightcaption{SSIM vs. non-rendered frame ratio, using FCC dataset}
%          \label{fig:queue15-psnr-stall}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.48\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/fcc-gccstall-queue25-delay100.pdf}
%          \tightcaption{SSIM vs. video stall ratio using FCC dataset}
%          \label{fig:queue15-ssim-delay}
%      \end{subfigure}
%      \hfill
%      \vspace{0.4cm}
%      \tightcaption{\name also outperforms the baselines when using network traces from FCC dataset }
%      \vspace{-0.1cm}
%      \label{fig:fcc-simulation}
% \end{figure}


\name also attains an average SSIM comparable to the Salsify or H.265 codecs (with or without Tambur), ranging between 15.5~dB and 16~dB across varied network conditions. 
SVC and Voxel exhibit a marginally lower SSIM, as packet losses inflict greater damage on them compared to \name.
Although error concealment techniques mitigate the stall ratio, they fall short in quality when compared to \name, which also corroborates the results in \S\ref{subsec:eval:resilience}. 
It is noteworthy that the machine-learning-based error concealment approach we employ already surpasses traditional methods, such as those implemented in H.264, in terms of reconstruction quality~\cite{zhou2010efficient, varsa2001non}. 
%However, most machine-learning-based error concealment solutions, to the best of our knowledge, necessitate a minimum of hundreds of milliseconds for error concealment, which is a duration incompatible with the latency requirements of real-time video streaming.

Though \name's SSIM is on par or slightly lower than some baselines, we believe that the reduction in frame delay and stall ratio is worth the minor drop in quality. This is confirmed by our user study later.


Figure~\ref{fig:other-metrics} compares \name with the baselines on other realtimeness and smoothness metrics with the one-way delay set to 100~ms and the queue length set to 25 packets.
For clarity, we only put the baselines with comparable average SSIM in this figure (without Voxel and error concealment).
Despite maintaining similar video quality, \name surpasses these baselines by reducing the 98 percentile frame delay by a factor of 2-5$\times$.
As evidenced in Figure~\ref{fig:non-rendered-frames}, \name only fails to render 0.2\% of frames, far superior to the 4-10\% non-rendered frames exhibited by the baselines.
Additionally, Figure~\ref{fig:frequency-of-stalls} demonstrates that \name experiences few video stalls, thereby markedly outperforming all baselines.
We also evaluated \name with a different congestion control algorithm, Salsify CC~\cite{salsify}. More details can be found in  \S\ref{app:salcc}.
%\yc{Can we say anything interesting about Salsify CC results?}
    


% \mypara{Impact of bandwidth distributions}
We also run the simulation based on the broadband traces from FCC dataset~\cite{fcc-dataset}. Compared to the LTE traces, broadband traces have similar average bandwidth but fewer bandwidth drops. We run the simulation with a propagation delay of 100ms and a droptail queue of 25 packets. %and use GCC as the congestion control algorithm. 
Figure~\ref{fig:fcc-simulation} shows that \name still has a better trade-off between video quality and the ratio of delayed frames and video freezes than the baselines. 

% \mypara{Ablation study of key components} 
% We then conduct an ablation study by removing per-packet entropy coding (\S\ref{??}) and loss-resilience training (\S\ref{??}). 
% We run the experiment using Sal-CC with the same one-way delay and queue length as in Figure~\ref{fig:normal-simulation}. 



Finally, Figure~\ref{fig:timeseries-ours} shows a concrete example of \name's behavior.
% compare \name and the baselines in a concrete bandwidth trace sample to illustrate why it can achieve a better tradeoff (Figure~\ref{fig:timeseries-ours}).
The bandwidth drops from 8~Mbps to 2~Mbps at 1.5sec and last for 800ms, before bouncing back to 8Mbps (another bandwidth drop occurs at 3.5sec).
During each bandwidth drop, \name's delay does not increase as sharply as the baselines (notably Salsify is the second best since it could skip frames while H.265 needs to wait for the retransmission).
\name and Salsify use the same CC, so their quality roughly matches on frames not skipped by Salsify.
That said, \name's quality degrades marginally with no frame skipping during congestion, limiting the drop of SSIM to less than 4 dB when there are more than 10 consecutive frames experiencing packet loss over 60\%. 
With the help of the resync logic (\S\ref{sec:delivery}), \name's quality bounces back soon (within 1 RTT) after packet losses disappear. 


% When we run \name with the models trained without any packet losses, the average SSIM will be decreased from \fillme dB to \fillme dB. This is because the frame quality will be significantly decreased when packet loss happens.


\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    %\includegraphics[width=1.05\linewidth]{figs/timeseries-new.pdf}
    \includegraphics[width=0.8\linewidth]{figs/timeseries-vertical-new.pdf}
    \tightcaption{\name achieves lower delay and decent quality during sudden bandwidth drops: the delay is lower compared to both baselines, and it can render more frames than Salsify without skipping or retransmission. \yc{align font, use larger linewidth}}
    \label{fig:timeseries-ours}
\end{figure}

\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    \includegraphics[width=1.0\linewidth]{figs/user-study-new.pdf}
    \tightcaption{User study experiment shows that videos streamed by \name are more favored by users.}
    \label{fig:user-study}
\end{figure}


\mypara{User study of video quality} 
% To show decreasing the ratio of delayed frames and video freezes is worth the minor drop in quality for real users, 
To validate \name's improvement on real-world users, we set up a user study website and gathered 960 user video ratings with Amazon MTurk~\cite{mturk} (IRB approved) from 240 crowdsource workers.
We sampled 8 video clips (spanning cloud gaming, real-time sports events, daily human activities, and video conferencing) rendered by \name, Salsify codec, WebRTC with default FEC, and H.265 with Tambur with the same setup as the simulation. 
(Appendix~\ref{fig:user-study-screenshot} shows a screenshot of each video.)
The sampled videos have the same distribution of quality, realtimeness, and smoothness as Figure~\ref{fig:gcc-delay-simulation}. 
% , and the user study is properly randomized following the steps described in \cite{sensei}.
When an MTurk user signs up for the user study, the user will be randomly assigned to rate their user experience (with a Likert scale of 1-5) on the videos rendered by different methods. 
Figure~\ref{fig:user-study} shows the mean opinion score (MOS) of each video. 
The result confirms that the videos rendered by \name are more favored by real users.

% with the average MOS across videos from 2.6 to 3.6 compared to the baselines.



 

%In Figure~???????????????????????????\ref{??}, we use three metrics for video quality, even though our autoencoders are trained to optimize L2-norm between the reconstructed and original images, which is similar to RGB-PSNR, their quality compared to baselines is similar under different metrics.

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_traceset_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_rtt_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_queue_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}


%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=1.pdf}
%    \caption{Aggressiveness = 1}
%    \label{fig:}
%\end{figure*}
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=0.75.pdf}
%    \caption{Aggressiveness = 5}
%    \label{fig:}
%\end{figure*}








% \jc{YIHUA, please fill in some detailed reading}

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/encoding-lat-gpu.pdf}
%          \caption{Encoding latency on A100 GPU}
%          \label{fig:gpu-encoding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/encoding-lat-cpu.pdf}
%          \caption{Encoding latency on CPU}
%          \label{fig:gpu-decoding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/decoding-lat-gpu.pdf}
%          \caption{Decoding latency on A100 GPU}
%          \label{fig:cpu-encoding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/decoding-lat-cpu.pdf}
%          \caption{Decoding latency on CPU}
%          \label{fig:cpu-decoding}
%      \end{subfigure}
%      \hfill
%      \tightcaption{Compute overhead of \name.}
%      \label{fig:computing-overhead}
% \end{figure} 

% \begin{figure*}[t!]
%     \centering
%     \begin{subfigure}[t]{0.37\linewidth}
%          \centering         
%          \includegraphics[width=\linewidth]{figs/encoding-decoding-lat-gpu.pdf}
%          \tightcaption{Encoding/decoding latency on GPU}
%          \label{fig:gpu-coding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.37\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/encoding-decoding-lat-cpu.pdf}
%          \tightcaption{Encoding/decoding latency on CPU}
%          \label{fig:cpu-coding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.24\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/encoding-lat-multi-copy.pdf}
%          \tightcaption{Encoding latency of multiple bitrates}
%          \label{fig:gpu-multi-coding}
%      \end{subfigure}
%      \hfill
%      \vspace{0.4cm}
%      \tightcaption{Compute overhead of \name. \jc{convert this to a single column table?}}
%      \label{fig:computing-overhead} 
% \end{figure*} 

% \begin{table}[t!]
% \begin{centering}
% \begin{tabular}{ccc}
%                   & Enc. time (ms) & Dec. time (ms) \\ 
% \toprule
% Motion estimation & 9              & N/A            \\ \hline
% MV encoding        & 2.1            & N/A            \\ \hline
% MV decoding        & 3.6            & 3.6            \\ \hline
% Frame smoothing   & 13.5           & 13.5           \\ \hline
% Residual encoding & 1.5            & N/A            \\ \hline
% Residual decoding & 2.4            & 2.4            \\ 
% \bottomrule
% Total time        & 32.1           & 19.5          
% \end{tabular}
% \end{centering}
% \tightcaption{Encoding/decoding time breakdown when running \name on Nvidia A40 GPU\jc{can we make it a bar chart? and compare it with h265? doesn't make sense to have "N/A"}}
% \label{tab:coding-time-gpu}
% \end{table}

\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    \includegraphics[width=1\linewidth]{figs/coding-latency-gpu.pdf}
    \tightcaption{Latency breakdown of encoding/decoding a 720p frame by \name. \yc{lower priority: add some labels to show "30 fps" and "25 fps"}}
    \label{fig:coding-time-gpu}
\end{figure}

    
\begin{table}[t!]
\begin{centering}
\begin{tabular}{c|cc|cc}
                      & \multicolumn{2}{c|}{Encoding (ms)} & \multicolumn{2}{c}{Decoding (ms)} \\ \cline{2-5} 
                      & 720p             & 480p             & 720p             & 480p            \\ \hline
\name, unoptimized        & 314.2            & 126.3            & 239.8            & 96.0            \\ \hline
\namelite   & 38.1             & 15.5             & 14.4             & 5.8            
\end{tabular}
\end{centering}
\tightcaption{Encoding/decoding time per frame for \name and \namelite on an iPhone 14 Pro}
\label{tab:coding-time-cpu}
\end{table}


\tightsubsection{Microbenchmarking}
\label{subsec:eval:micro}


\edit{
\mypara{Encoding/decoding latency breakdown}
We test the encoding/decoding latency of \name an Nvidia A40 GPU and break down the latency to each component.
Table~\ref{tab:coding-time-gpu} shows that \name is capable of encoding and decoding a 720P frame in 32.0~ms and 19.5 ms, respectively. 
This equates to frame rates of 31.2~fps and 51.2~fps for encoding and decoding 720P frames, respectively. 
The latency breakdown shows that motion estimation and frame smoothing are the most time-consuming steps, taking 70\% of the encoding time.

The resynchronization proposed in \S\ref{subsec:protocol} requires the encoder to run the MV decoder and residual decoder upon receiving the packet loss feedback. 
As listed in Table~\ref{tab:coding-time-gpu}, the two steps only take $3.6 + 2.4 = 6$~ms, which means an encoder running at 25~fps is able to encode a frame and finish such resynchronization without breaking the time constraint.

To encode an extra copy under a different bitrate for a 720p video frame, \name only needs 1.5~ms by running residual encoding again, as the most time-intensive portion of encoding is shared across models (\S\ref{subsec:fast-coding}).
% Given that the most time-intensive portion of encoding is shared across models in \name, the additional time required to encode multiple versions is minimal with the bitrate control optimizations in \S\ref{subsec:fast-coding}, averaging merely 1.5ms per extra copy for 720p video (0.5ms for 480p). 
Consequently, \name can encode three distinct copies within 35~ms, enabling the bitrate control as described in \S\ref{subsec:fast-coding}. 
Empirically, we found that over 65\% of frames require a single encoding pass, while 34\% need a second pass to adjust to the target bitrate. 
A marginal subset, less than 1\%, is subjected to a third encoding pass.



\mypara{Impact of speed optimizations in \namelite}
We compare the encoding/decoding time of \name (without speed optimization in \S\ref{subsec:fast-coding}) and \namelite on an iPhone 14 Pro.
As illustrated in Table~\ref{tab:coding-time-cpu}, the optimizations in \namelite significantly curtail encoding and decoding times. 
For 720P videos, \name necessitated 314.2 and 239.8ms to encode and decode a frame, respectively; however, these times were dramatically reduced to 38.1ms and 14.4ms when using \namelite.
This result also demonstrates \namelite is capable of streaming 720P real-time video on resource-constrained devices like iPhones. 

Figure~\ref{fig:ssim-loss-cpu} and~\ref{fig:ssim-bpp-cpu} compares the loss resilience and the compression efficiency between \name and \namelite.
Despite the \namelite exhibiting a marginally lower SSIM of 0.5 dB compared to \name, the optimizations do not compromise its loss resilience features.
When 10\% to 60\% packet is applied to a frame, \namelite only has a small SSIM drop between 0.5 to 2.5~dB, outperforming H.264 with FEC and SVC.

We conduct the end-to-end simulation on LTE traces with 100~ms network delay and a 25-packet network queue to compare the video quality and realtimeness/smoothness tradeoff between \name and \namelite. 
Table~\ref{tab:cpu-simulation} shows that the average SSIM only decreased from 15.5 dB to 15.0 dB after applying the speed optimizations in \namelite, and the optimizations do not affect the realtimeness and smoothness of the decoded video much.
}

% \mypara{\name's fast bitrate adaptation}





% \begin{figure}[t!]
%      \begin{subfigure}[t]{0.48\linewidth}
%          \centering
%          \includegraphics[width=1.05\linewidth]{figs/ssim-loss-cpu.pdf}
%          \tightcaption{\namelite still have good loss resilience.}
%          \label{fig:ssim-loss-cpu}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.48\linewidth}
%          \centering
%          \includegraphics[width=1.05\linewidth]{figs/ssim-bpp-cpu.pdf}
%          \tightcaption{\namelite has on-par compression efficiency with H.264 }
%          \label{fig:ssim-bpp-cpu}
%      \end{subfigure}
%      \hfill
%      \vspace{0.5cm}
%      \tightcaption{Loss resilience and compression efficiency of \name when running on mobile devices with the optimization in \S\ref{subsec:fast-coding}.}
%      \label{fig:cpu-performance}
% \end{figure}

\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    \includegraphics[width=1\linewidth]{figs/cpu-study-single.pdf}
    \tightcaption{\namelite has similar loss resilience compared to \name and outperforms other baselines.}
    \label{fig:cpu-performance}
\end{figure}


\begin{figure}[t!]
     \centering
     \includegraphics[width=\linewidth]{figs/abl-study-single.pdf}
     \tightcaption{Although \namedecoder and \namepretrain have slightly better quality than \name when there is no packet loss, they are much less loss resilient than \name \yc{use green for grace-d and grace-p}}
     \label{fig:ssim-loss-abl}
     \vspace{-0.1cm}
\end{figure}

\begin{comment}

\begin{table}[t!]
\begin{centering}
\begin{tabular}{c|c|c|c}
           & \begin{tabular}[c]{@{}c@{}}SSIM\\ (dB)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\% of non \\ rendered frames\end{tabular} & \begin{tabular}[c]{@{}c@{}}Video stall\\ ratio\end{tabular} \\ \hline
\name      & 15.53                                               & 0.21                                                                 & 0.0011                                                      \\ \hline
\namelite & 15.01                                               & 0.22                                                                 & 0.0012                                                     
\end{tabular}
\tightcaption{End-to-end simulation shows \namelite has the same benefits in video realtimeness/smoothness compared to \name.\jc{please don't introduce a new table format, unless really necessary. see my slack message?}}
\label{tab:cpu-simulation}
\end{centering}
\end{table}


\begin{table}[t!]
\begin{centering}
\begin{tabular}{c|c|c|c}
           & \begin{tabular}[c]{@{}c@{}}SSIM\\ (dB)\end{tabular} & \begin{tabular}[c]{@{}c@{}}\% of non \\ rendered frames\end{tabular} & \begin{tabular}[c]{@{}c@{}}Video stall\\ ratio\end{tabular} \\ \hline
\name      & 15.53                                               & 0.21                                                                 & 0.0011                                                      \\ \hline
\namedecoder & 13.91                                               & 0.24                                                                 & 0.0014    \\ \hline                                    
\namepretrain & 12.53                                               & 0.33                                                                 & 0.0023                                                  
\end{tabular}
\tightcaption{End-to-end simulation shows although \namedecoder and \namepretrain has similar video realtimeness/smoothness as \name, they suffer from low video quality. \jc{please don't introduce a new table format, unless really necessary. see my slack message?}}
\label{tab:abl-simulation}
\end{centering}
\end{table}

\end{comment}


% \begin{figure}[t!]
%     \centering
%          \centering
%         \includegraphics[width=0.99\linewidth]{figs/loss-visualization-example-late.pdf}
%     \tightcaption{Example decoded images when there are 50\% packet loss on 3 consecutive frames, comparing \name and \name w/o training encoder. }
%     \label{fig:late-visual-example}
% \end{figure}
% \begin{figure}[t!]
%      \begin{subfigure}[t]{0.48\linewidth}
%          \centering
%          \includegraphics[width=2\linewidth]{figs/abl-gccdelay-queue25-delay100-long.pdf}
%          \tightcaption{SSIM vs. non-rendered frame ratio, using different versions of \name}
%          \label{fig:queue15-psnr-stall}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.48\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/abl-gccstall-queue25-delay100.pdf}
%          \tightcaption{SSIM vs. video stall ratio, using different versions of \name}
%          \label{fig:queue15-ssim-delay}
%      \end{subfigure}
%      \hfill
%      \vspace{0.5cm}
%      \tightcaption{Simulation results comparing \name to its variants}
%      \label{fig:simulation-ablation}
% \end{figure}




% Figure~\ref{fig:cpu-encoding} and Figure~\ref{fig:cpu-decoding} shows our optimizations on CPU can significantly reduce the encoding and decoding time. For 720P videos, the original model takes 5217ms and 3996ms to encode and decode a frame, while the time decreases to 35.1ms and 40.9ms after applying our optimizations. This shows that with our optimization, \name is able to stream the 720P video purely using CPU.
% Compared with the GPU version of \name, the optimized CPU version has a lower SSIM of 0.8 dB. However, it does not impact the improvement in the ratio of delayed frames. %, and the quality is not bad compared to the error concealment baseline.

% \begin{figure}[t!]
%     \centering
%          \centering
%         %\includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
%         \includegraphics[width=0.7\linewidth]{figs/encoding-multiple-version.png}
%          \label{fig:system-encoding-versions}
%          \vspace{.05cm}
%     \tightcaption{Encoding latency of encoding multiple versions \textcolor{red}{TODO: Yihua}}
%     \label{fig:multiple-encoding}
% \end{figure}




\edit{
% \mypara{Ablation study for \name's training methodology}
\mypara{Impact of joint training}
Figure~\ref{fig:ssim-loss-abl} compares the loss resilience of \name to its two variants: \namepretrain (which is trained without packet loss) and \namedecoder (which only trains the decoder with packed loss).
When there are multiple consecutive frames impacted by packet loss, \name outperforms both variants by 0.5-2~dB in SSIM as the loss rate changes from 0.1 to 0.8. 
% Figure~\ref{fig:late-visual-example} shows the visual example comparing the decoded image of \name and its two variants when 50\% loss happens on 3 consecutive frames.
% \namepretrain, having never encountered packet loss during training, struggles to faithfully reconstruct the frame when faced with packet loss. 
% \namedecoder does yield a marginal improvement in frame quality, but visible artifacts still exist.
% In contrast, the joint training of both the encoder and decoder under packet loss conditions enables \name to deliver the most superior reconstruction quality, devoid of any prominent artifacts, and also achieves a high SSIM during loss.

We also conducted the end-to-end simulation to test the realtimeness/smoothness trade-off of \namepretrain, \namedecoder, and \namelite, using LTE traces with 100ms network delay and a 25-packet network queue.
As shown in Table~\ref{tab:abl-simulation}, without loss-resilience training, \namepretrain experiences significant quality degradation due to packet loss, with the SSIM dropping from 15.5 dB to 12.4 dB in comparison to \name. 
Moreover, solely fine-tuning the decoder with loss is insufficient, resulting in a quality drop from 15.5dB to 13.9dB. 


\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/loss-visualization-example-late.pdf}
    \tightcaption{Comparing reconstructed image when the same packet loss is applied to the pre-trained NVC (\namepretrain), a variant with only decoder fine-tuned with loss (\namedecoder), and \name (both encoder and decoder jointly fine-tuned).
%    Example decoded images when there are 50\% packet loss on 3 consecutive frames, comparing \name and \name w/o training encoder. 
    }
    \label{fig:late-visual-example}
\end{figure}

% To highlight the benefit of joint training, we train a new \name variant by fine-tuning \namepretrain in the same way as \name except for freezing the encoder NN weights, \ie fine-tuning only the decoder with simulated loss.
% We refer to this variant as \namedecoder.
Figure~\ref{fig:late-visual-example} compares the reconstructed frame of \name, \namepretrain, and \namedecoder when the same 50\% packet loss is applied to the encoded tensor of the same image. 
\namepretrain, having never encountered packet loss during training, struggles to faithfully reconstruct the frame when faced with packet loss. 
\namedecoder does yield a marginal improvement in frame quality, but visible artifacts still exist.
In contrast, by joint training both the encoder and decoder under packet loss, \name delivers the best reconstruction quality, without any prominent artifacts, achieving a high SSIM.
% \S\ref{subsec:eval:micro} will provide more comprehensive evaluation of the advantages of jointly training NVC under various packet loss.

% 

% We also test \name without the per-packet entropy coding technique described in \S\ref{subsec:packetization}.
% Figure~\ref{fig:simulation-ablation} shows that both the delayed frame ratio and the stall ratio will increase if \name does not have the per-packet entropy coding.
% This is because, without it, the size of the encoded frame will have an increase of 1.5$\times$, and this size increase may overload the network when bandwidth suddenly drops. 
}

% \yc{note for myself: need to check the consistency of "CPU version \name". The text used a lot of different ways to describe it and it's very confusing. Need to align with section 4.3}


%It also shows without training with loss, the pretrained autoencoder models will suffer from quality drops caused by packet loss. The SSIM will drop from 15.8dB to 12.4dB compared to \name.




% As discussed in \S\ref{subsec:related}, SR can be used as a complementary tool to enhance the video quality at the receiver side. 
% We use SwinIR~\cite{liang2021swinir}, a state-of-the-art SR model in our simulation to validate \name can also benefit from SR the same as baselines.
% Our experiments shows that SR can improve the quality for any codecs at the receiver side, agnostic to what codec is being used.
% Due to size constrain, we put more details into Appendix~\ref{app:sr}.





% Figure~\ref{fig:gpu-encoding} shows the encoding latency for \name to encode multiple different copies of frames with different bitrates (\S\ref{subsec:fast-coding}). Since the models share the most time-consuming part of the encoding, the overhead of encoding multiple versions is negligible: only 2.6ms for every extra copy. Therefore, \name can encode 3 different copies in 40.9ms, allowing the encoder to do bitrate adaptation in real-time.
% Empirically in our study, over 65\% frames will only be encoded once and 34\% frames will be encoded twice to adapt to the target bitrate. Less than 1\% frames will be encoded 3 times. 
% Figure~\ref{??} shows the effectiveness of our bitrate controlling algorithm (\S\ref{??}). Over \fillme\% of frames will falls in the range of $[0.8, 1]\times$ target bitrate and it will never produce a frame that overshoots the target bitrate.

% \mypara{Model training decisions}
% To validate the design choices of loss distribution we used during model training, we conduct an ablation study of different loss distributions. We test two different setups: (i) the probability of using 0 loss is the same as other loss rates, and (ii) loss rates as high as 80\% and 90\% are added during training. As shown in Figure~???\ref{fig:training-loss-study}, both setups can cause the SSIM under 0 loss decrease around \fillme dB. 
% When the probability of 0 loss is low, the model will learn to deprioritize the quality under 0 loss, which will impact the average video quality. We also observe that seeing a loss as high as 80\% or 90\% will also damage the quality under 0 loss.


% Our implementation of \name optimizes both memory footprint and encoding/decoding delay (described in \S???\ref{subsec:optimize}), and we test its effectiveness on a Nvidia GeForce RTX 3080 GPU. 
% Figure~???\ref{fig:system-encoding} and Figure~???\ref{fig:system-decoding} show that compared to the original (unoptimized) implementation of pre-trained autoencoder (which takes 100ms to encode a 480p frame), our implementation can encode a 480p frame in less than 25ms (a 4×4\times speedup).\footnote{The only autoencoder that achieves comparable encoding/decoding speed is~\cite{elf}, and it achieves such speed on a 5x more expensive Titan V GPU. We hope to compare it with \name, but it is not open-source.}
% This translates to almost 40fps. 
% Even for 720p HD videos, our optimized codec can achieve 18fps (55ms encoding per frame). 
% % \fillme~fps/\fillme~fps, \name encodes/decodes 480p frames at \fillme~fps/\fillme~fps, a \fillme×\times speedup.
% This acceleration comes from downsampling frames in motion-vector estimation. 
% Moreover, when adapting to a target bitrate, \name encodes the next frame multiple times {\em without} needing to run the entire encoder multiple times, because it re-uses the motion-compensated prediction, so only the residuals need to be encoded at multiple bitrates. Figure~??????\ref{fig:system-encoding-versions} shows that the delay of encoding a frame at three different bitrates only increases marginally compared to encoding one frame. 







% In terms of memory usage, our optimized implementation saves the memory footprint of loading 9 models by over 60\% since most NN layers are shared. 
% % Figure~??????\ref{??} shows that compared to loading the multiple autoencoders (I-frame encoder/decoder and a P-frame encoder/decoder of each bitrate) in GPU memory, the memory usage \name's autoencoders (not including the memory usage of intermediate features) is \fillme\% smaller, because they share most of the layers (only the last \fillme layers of the encoder and the first \fillme layers of the decoders are different). 
% Note that \name does not change the NN architecture of the autoencoders---only the weights are retrained and the way they are used is optimized. We speculate that they could be made more efficient with appropriate modification to its NN architecture.

% Figure~??????\ref{??} validate that \name's compression efficiency is comparable to (even slightly better than) without the optimizations (\ie without sharing the NN backbone or downsampling and sharing the motion-vectors.)
% This is because, though quality does drop with these optimizations, the encoded size also drops (due largely to the downsampled motion vectors), which result in a similar bitrate-quality trade-off frontier.

% \jc{The only autoencoder that achieves comparable encoding/decoding speed is Elf~\cite{??}. 
% We hope to compare it with \name, but it is not open-source. }


% \jc{remember to highlight that the speed is comparable to elf, which runs on the 5x more expensive titan v gpu.}

% \begin{figure}[t!]
%     \centering
%          \centering
%         \includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
% %        \includegraphics[width=0.7\linewidth]{figs/a.pdf}
%          \label{fig:}
%          \vspace{.05cm}
%     \tightcaption{Training curve study \textcolor{red}{put into appendix}}
%     \label{fig:training-loss-study}
% \end{figure}
%!TEX root = ../main.tex
%!TEX spellcheck = en_US



==> sections/old/eval_v0.tex <==
\tightsection{Evaluation}

\tightsubsection{Experiment setup}
\begin{itemize}
    \item Testbed (simulation & emulation)
    \item Traces we used
    \item Baselines
\end{itemize}

\tightsubsection{Simulation (frame level)}
Frame level quality improvement compared with baselines
\begin{itemize}
    \item PSNR under different losses
    \item PSNR CDF for different frames (we have a better tail)
\end{itemize}

\tightsubsection{Trace-driven experiments (packet level)}
\begin{itemize}
    \item tail PSNR v.s. avg delay
    \item avg PSNR v.s. tail delay
\end{itemize}

\tightsubsection{Microbenchmark}
\begin{itemize}
    \item Improvement on different video type
    \item Improvement breakdown
\end{itemize}

==> sections/old/eval_v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\section{Evaluation}
\label{sec:eval}

The findings from our evaluation of \name can be summarized as follows:
\begin{packeditemize}
\item Though in terms of quality under no packet loss, \newae is on par with H.264 and slightly worse than H.265, it is data-scalable---graceful quality degradation with higher loss rate---under various video content and bitrate. 
\jc{a few example numbers}
\item Under dynamic network conditions, \name strikes a better trade-off between average video quality and tail delay than a wide range of baselines.
\jc{a few example numbers}
\end{packeditemize}

\subsection{Setup}

We test \name's implementation (described in \S\ref{??}) at two levels.
First, we test \newae's loss resilience when encoding/decoding real videos under controlled packet losses, and compare it with other loss-resilient schemes.
Second, we test \name (including its codec and delivery framework) over real bandwidth traces, and compare it with other real-time baseline solutions (baselines explained shortly).



\mypara{Network and compute conditions}
We test \name on \fillme real bandwidth traces from FCC.
We filter traces \fillme.\jc{ziyi and hanchen, please describe the filter here.}

We conduct all experiments on a machine with two Nvidia \fillme GPUs as the sender and receiver (each using one GPU). 
\jc{more details, such as cuda version, linux version, cpu, memory, etc}
To make the results more convincing, we measure \name's encoding and decoding delays on the GPU (see results in \S\ref{??}) and we include these delays in \name's frame delay. 

Our evaluation uses videos from three datasets (\fillme, \fillme and \fillme), each video is of \fillme minutes. 
The videos cover three resolutions (360p at 25fps, 720p at 25fps, and 1080p at 20fps), with at least \fillme videos in each resolution. 
The performance is reported as an average across all the frames in the videos.


\mypara{Baselines}
We compare the performance of \name with multiple state-of-the-art real-time video techniques that use different combinations of video coding and congestion control algorithms: 
\begin{packeditemize}
\item {\em Reference:} H.26x with adaptive FEC and GCC
\item {\em Salsify:}
\item {\em Idealized SVC:}
\end{packeditemize}


\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/psnr-bpp-example.pdf}
         \label{fig:}
    \caption{an example. need more of it in different datasets}
    \label{fig:}
\end{figure}


\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-loss-kin.pdf}
         \caption{Kinetics dataset}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-loss-uvg.pdf}
         \caption{UVG dataset}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-loss-fvc.pdf}
         \caption{FVC dataset}
         \label{fig:}
     \end{subfigure}
     \hfill
     \caption{PSNR vs LOSS different dataset (bpp = 0.08)}
    \label{fig:}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-loss-lowbr.pdf}
         \caption{Small bitrate (bpp = 0.08)}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-loss-medbr.pdf}
         \caption{Med bitrate (bpp = 0.16)}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-loss-highbr.pdf}
         \caption{High bitrates (bpp = 0.24)}
         \label{fig:}
     \end{subfigure}
    \caption{PSNR vs LOSS of different bitrate, using multiple datasets}
    \label{fig:}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-bpp-kin.pdf}
         \caption{Kinetics dataset}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-bpp-uvg.pdf}
         \caption{UVG dataset }
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/psnr-vs-bpp-fvc.pdf}
         \caption{FVC dataset}
         \label{fig:}
     \end{subfigure}
    \caption{PSNR vs BPP different dataset}
    \label{fig:}
\end{figure*}

\subsection{Loss resilience}

\jc{
\begin{itemize}
    \item by bitrate
    \item by video set
    \item psnr vs. bitrate
\end{itemize}
}



\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_traceset_placeholder.pdf}
    \caption{}
    \label{fig:}
\end{figure*}


\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_rtt_placeholder.pdf}
    \caption{}
    \label{fig:}
\end{figure*}


\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_queue_placeholder.pdf}
    \caption{}
    \label{fig:}
\end{figure*}


\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
    \caption{}
    \label{fig:}
\end{figure*}

\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
    \caption{}
    \label{fig:}
\end{figure*}


\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=1.pdf}
    \caption{Aggressiveness = 1}
    \label{fig:}
\end{figure*}

\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=0.75.pdf}
    \caption{Aggressiveness = 5}
    \label{fig:}
\end{figure*}


\begin{figure}[t!]
    \centering
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/loss-distribution.pdf}
         \caption{Impact of different data loss distribution used during training}
         \label{fig:training_loss_distribution}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/loss-pattern.pdf}
         \caption{Impact of different data loss pattern used during training}
         \label{fig:training_loss_pattern}
     \end{subfigure}
    \label{fig:training_loss_simulation}
\end{figure}

\subsection{Video quality vs. tail delay}

\jc{
\begin{itemize}
    \item by trace set
    \item by rtt
    \item by queue length
    \item a concrete example
\end{itemize}
}

\subsection{Memory and compute overhead}

\jc{remember to highlight that the speed is comparable to elf, which runs on the 5x more expensive titan v gpu.}


\subsection{Design choices in \name}

\jc{
\begin{itemize}
    \item different training loss patterns
    \item different training \rate distributions
    \item saliency-based redunancy
    \item packet prioritization
    \item computing overhead in delay and in memory
\end{itemize}
}



==> sections/old/eval_v3.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Evaluation}
\label{sec:eval}

The findings of our evaluation can be summarized as follows:
\begin{packeditemize}
\item {\bf Loss resilience:} Though \newae's quality under no packet loss is on par with H.264 and slightly worse than H.265, it is data-scalable---graceful quality degradation with higher loss rate---under various videos and bitrates. 
%\jc{a few example numbers}
\item {\bf Quality-delay tradeoff:} On real and synthetic network traces with bandwidth fluctuation, \name reduces tail delay by 2$\times$, compared to other loss-resilient schemes (FEC, Salsify) while still obtaining decent quality.
%strikes a better trade-off between average video quality and tail delay than a wide range of baselines.
%\jc{a few example numbers}
\item {\bf Overhead:} Our implementation of \name can encode/decode 480p video at 40~~fps/50~fps and 720p HD video at 18~fps/30~fps, a 1.5$\times$ speedup compared to off-the-shelf autoencoders.
\end{packeditemize}


\tightsubsection{Setup}
\label{subsec:eval:setup}

\mypara{Baseline implementations}
Our baseline codecs include H.265 and H.264. 
We use their implementations in \texttt{ffmpeg} (version 4.2.7). 
Importantly, we do not restrict their GoP (I-frame interval) and the number of history frames to search for reference macroblocks. 
Following recent work in real-time video coding~\cite{ZEROLAT1,ZEROLAT2}, we use the \texttt{zerolatency} option (no B-frames) and the \texttt{fast} preset of H.265\footnote{The command line we used to encode a video is \texttt{ffmpeg -y -i Video.y4m -c:v libx265 -preset fast -tune zerolatency -x265-params "crf=Q:keyint=3000" output.mp4} where {\em Q} controls the quality and size of the output video}.

We use implementations for SVC, Salsify, and FEC, based on H.265.
We simplify the implementation in a way that makes their quality slightly better than they would actually do. 
Our implementation of SVC assumes that each quality level exactly {\em matches} the quality and size of the non-SVC coding of H.265, whereas even the state-of-the-art SVC (based also on autoencoders~\cite{swift}) achieves lower quality than H.265 at a quality level of the same frame size. (This effectively is an idealized version of Swift~\cite{swift}.)
We follow Salsify's logic for congestion control, frame skipping, and packet pacing, but instead of using Salsify's multi-trial encoding to approximate the target bitrate of each frame, we assume that the encoded frame size exactly {\em matches} each frame's target bitrate but the quality matches the {\em qp} value whose bitrate is barely {\em higher} than the target bitrate.
For FEC-protected H.26x, we use the same loss-rate prediction logic implemented in the public release of WebRTC~\cite{WEBRTCSRC} but remove the upper-bound of 50\% redundancy rate that is used in WebRTC \eg if the predicted packet loss rate is 60\%, we assume FEC will tolerate any packet loss ratio under 60\%.) %but instead of mapping it to the coarse-grained FEC redundancy rates, we assume an idealized FEC that can reconstruct a frame if the actual loss rate matches the predicted loss rate (\eg if the predicted packet loss rate is 50\%, we assume FEC will exactly tolerate 50\% packet loss.)
%This effectively approximates the situation where data can be packetized infinitesimally.
While these simplifying assumptions lead to a slightly optimistic estimate of the baselines' performance, we hope they make our results more relevant in the long run, as the implementations of SVC, and bitrate control, and FEC might evolve and improve in the future.

\mypara{Network and compute conditions}
We test \name on 8 real bandwidth traces distributed with the Mahimahi network-emulation tool~\cite{netravali2015mahimahi}\footnote{The data set has 16 traces. We filtered out the traces having an average bandwidth lower than 1Mbps as they do not fit the bandwidth requirement of video traffic.}. 
%and we filter traces .
By default, we set the one-way network propagation delay to be 100ms and the queue size to be 25 packets.
We also show the impact of different propagation delays and queue sizes in \S\ref{subsec:eval:e2e}.
We conduct all experiments on a machine with two Nvidia GeForce RTX 2080 GPUs as the sender and receiver (each using one GPU). The server runs Ubuntu 18.04 with 2 Intel Xeon Silver 4110 CPU and 64GB memory.
%\jc{more details, such as cuda version, linux version, cpu, memory, etc}
We measure \name's encoding and decoding delays on the GPU (see results in \S\ref{subsec:eval:system}) and we include these delays in \name's frame delay. 


\mypara{Metrics}
We measure the performance of a video session in three aspects.
Quality of a frame is measured by SSIM and PSNR (RGB and YUV), and we report the average value across received frames. 
Delay of a frame is measured by the time lapse between the beginning of encoding to the end of decoding. 
For skipped frames (by Salsify), their decoding time equals the next decoding time of the next received frame. 
We report the tail (95th\% percentile) of the delays across frames in a session.
%\jc{describe frame rate metric}


\mypara{Test videos}
Our evaluation uses 60 videos from three public datasets (Kinetics~\cite{Kinetics}, UVG~\cite{mercat2020uvg} and FVC~\cite{FVCDATASET}), each video is of at least 10 seconds. 
%Table~\ref{sec:??} summarizes the datasets.
Importantly, we choose these videos because they are different from the training set, allowing us to stress-test the generalization of autoencoders.
The FVC dataset includes 5 videos captured from video conferencing, one of \name's main target use-cases.
These videos cover a range of spatial and temporal dynamics (\S\ref{app:siti})
and cover three resolutions (640$\times$360, 1280$\times$720 and 1920$\times$1280), with at least 5 videos in each resolution. 
The performance is reported as an average across all the frames in the videos.



%\mypara{Baselines}
%We compare the performance of \name with multiple state-of-the-art real-time video techniques that use different combinations of video coding and congestion control algorithms: 
%\begin{packeditemize}
%\item {\em Reference:} H.26x with adaptive FEC and GCC
%\item {\em Salsify:}
%\item {\em Idealized SVC:}
%\end{packeditemize}


% \begin{figure}[t!]
%     \centering
%          \centering
%         \includegraphics[width=0.99\linewidth]{figs/psnr-bpp-example.pdf}
%          \label{fig:}
%     \caption{an example. need more of it in different datasets}
%     \label{fig:}
% \end{figure}



% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/psnr-vs-loss-360p.pdf}
%          \caption{360P videos (bitrate = 1.4Mbps)}
%          \label{fig:}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/psnr-vs-loss-HD.pdf}
%          \caption{1080P videos (bitrate = 6.2Mbps)}
%          \label{fig:}
%      \end{subfigure}
%      \hfill
%      \caption{\newae's loss resilience on videos with different resolutions}
%     \label{fig:loss_by_resolution}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/eval-psnr-loss-together2.pdf}
    \tightcaption{\newae's loss resilience by bitrate and resolution}
    \label{fig:loss_by_resolution_bitrate}
\end{figure}

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/psnr-vs-loss-lowbr.pdf}
%          \caption{720P videos (bitrate = 2.4Mbps)}
%          \label{fig:}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/psnr-vs-loss-720p.pdf}
%          \caption{720P videos (bitrate = 3.2Mbps)}
%          \label{fig:}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/psnr-vs-loss-medbr.pdf}
%          \caption{720P videos (bitrate = 3.6Mbps)}
%          \label{fig:}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/psnr-vs-loss-highbr.pdf}
%          \caption{720P videos (bitrate = 4.8Mbps)}
%          \label{fig:}
%      \end{subfigure}
%      \hfill
%     \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/psnr-vs-loss-360p.pdf}
%          \caption{360P videos (bitrate = 1.4Mbps)}
%          \label{fig:}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/psnr-vs-loss-HD.pdf}
%          \caption{1080P videos (bitrate = 6.2Mbps)}
%          \label{fig:}
%      \end{subfigure}
%     \caption{\newae's loss resilience on different encoding bitrates}
%     \label{fig:loss_by_resolution_bitrate}
% \end{figure}


% \begin{figure*}[t!]
%     \centering
%     \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/psnr-vs-bpp-kin.pdf}
%          \caption{Kinetics dataset}
%          \label{fig:}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/psnr-vs-bpp-uvg.pdf}
%          \caption{UVG dataset }
%          \label{fig:}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figs/psnr-vs-bpp-fvc.pdf}
%          \caption{FVC dataset}
%          \label{fig:}
%      \end{subfigure}
%     \caption{PSNR vs BPP different dataset\jc{YIHUA, can we change x-axis to Bitrate? i guess that's more commen?}}
%     \label{fig:}
% \end{figure*}



\tightsubsection{Coding efficiency and loss resilience}

% \name's gains stem from the performance of the autoencoder \newae.
Figure~\ref{fig:loss_by_resolution_bitrate} compares \newae with the baselines codecs\footnote{We do not put Intra-MB insertion baseline here, since it's quality will quick drop below x-axis when loss ratio is between 5\% to 10\%.} under different packet loss rates when encoding videos of the same resolution and same target bitrate. 
In each figure, all lines have almost the same encoding bitrate with difference controlled within 5\%.
We ensure that \newae's encoded bitrate is {\em never} higher than the baselines, so even if the actual encoded bitrate is different, it does not favor \newae.
% Similarly, Figure~\ref{fig:loss_by_bitrate} compares the same set of solution when they have the same encoding bitrate.

% For each figure, the encoded bitrates of different solutions are controlled within 10\% difference (and to make it less favorable to \newae, we make sure that \newae's encoded bitrate is never higher than the baselines).
% Figure~\ref{fig:loss_by_resolution} shows the results by video resolution and Figure~\ref{fig:loss_by_bitrate} shows the results by encoding bitrate on 720P videos\footnote{We do not put Intra-MB insertion baseline here, since it's quality will quick drop below x-axis when loss ratio is between 5\% to 10\%}. 
The most salient feature of \newae is the graceful quality degradation with more packet losses. 
The average PSNR drop is only 2.1 to 3.9 under 30\% and 50\% packet losses. Even when the loss ratio is as high as 80\%, it has an average PSNR of 36.4, which is much better than the baselines except H.264 with 80\% FEC.
Compared with H.264 with fixed FEC protection, \newae can have a higher PSNR of 1.1 to 2.0 among different resolutions and different bitrates when there is no loss. This is because any arrived bytes in \newae contribute to the quality while in FEC, the redundant data is useless even if they do arrive at the decoder. On the other hand, FEC-based loss resiliency is also in a dilemma that a low FEC rate cannot protect against the high loss, but a high FEC rate leads to poor quality when the packet loss ratio is small. Our \newae solve's such dilemma by the graceful quality degradation.
\newae is also better than SVC with unequal FEC protection (\S\ref{subsec:abstractions}). 
The quality of SVC decreases quickly when the loss rate is small, as the high-quality layers are unlikely to be decodable in such cases. 
% As shown in Figure~\ref{fig:loss_by_resolution_bitrate}, \newae has a average PSNR gain of 3.9 over SVC when the loss ratio is 30\%.
We also note that the pretrained autoencoder models, which have not seen any losses in training, degrade poorly with higher loss rates. 
% It has an average PSNR decrease of 4.3 when loss ratio is 30\%, which is 2$\times$ higher than \newae.
% to h264 + fec baseline
% comparing to SVC


%\jc{
%\begin{itemize}
%    \item by bitrate
%    \item by video set
%    \item psnr vs. bitrate
%\end{itemize}
%}

% \jc{need a footnote to explain why intra-mb insertion is so bad}


\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
         \label{fig:}
         \vspace{.05cm}
    \tightcaption{Quality-size tradeoff of \newae. \vspace{.05cm}}
    \label{fig:psnr-vs-bpp}
\end{figure}

For any loss-resilient schemes, the ability to tolerate packet losses often comes with a drop of quality in absence of packet losses, and \newae is no exception. 
Figure~\ref{fig:psnr-vs-bpp} compares the \newae's quality under no packet losses with that of H.264 and H.265 across the test videos (all of which are randomly sampled from three datasets that are different from the training set, \S\ref{subsec:eval:setup}).
% evaluates the price \newae pays to get its loss resilience. It shows the average PSNR of \newae, H.264 and H.265 on different bitrate across all test videos.
Fortunately, at the same encoded bitrate, \newae is similar to H.264 and is only slightly worse than H.265. 
When bitrate varies from 2Mbps to 8Mbps, the average PSNR is 44.29, 44.31, and 44.84 for \newae, H.264 and H.265 respectively.

Remember that H.26x uses the zerolatency option and fast preset (which is typical to real-time videos, including WebRTC\footnote{Google's WebRTC~\cite{WEBRTCSRC} uses OpenH264~\cite{OPENH264}. They set the runtime parameter "usageType" to CAMERA\_VIDEO\_REAL\_TIME  (similar to zerolatency) and "complexityMode" to LOW\_COMPLEXITY (similar to fast)}. %\jc{Yihua, please add a footnote about the following: one is usageType = CAMERA\_VIDEO\_REAL\_TIME  (similar to zerolatency) and another is complexityMode = LOW\_COMPLEXITY (similar to fast)})
We confirm that without these settings, H.265's coding efficiency is better than \newae in the absence of packet losses.
However, our goal is a data-scalable autoencoder for real-time videos (shown shortly), rather than an autoencoder that outperforms heavily engineered H.26x codecs. 
Moreover, the coding efficiency of autoencoder could still be improved (\eg our autoencoder estimates motion vectors based only on one reference frame). 

%In Figure~\ref{??}, we use three metrics for video quality, even though our autoencoders are trained to optimize L2-norm between the reconstructed and original images, which is similar to RGB-PSNR, their quality compared to baselines is similar under different metrics.

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_traceset_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_rtt_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_queue_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}


%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=1.pdf}
%    \caption{Aggressiveness = 1}
%    \label{fig:}
%\end{figure*}
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=0.75.pdf}
%    \caption{Aggressiveness = 5}
%    \label{fig:}
%\end{figure*}



\begin{figure}[t!]
    \centering
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         %\includegraphics[width=1.0\linewidth]{figs/e2e-yuvpsnr.pdf}
         \includegraphics[width=2.0\linewidth]{figs/e2e-yuvpsnr-long.pdf}
         \caption{PSNR}
         \label{fig:}
     \end{subfigure}
     %\hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         %\includegraphics[width=1.0\linewidth]{figs/e2e-ssim.pdf}
         \includegraphics[width=1.0\linewidth]{figs/e2e-ssim-long.pdf}
         \caption{SSIM}
         \label{fig:}
     \end{subfigure}
     \vspace{.05cm}
    \tightcaption{Video quality vs. tail delay (by quality metrics) \vspace{.1cm}}
    \label{fig:e2e-quality}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=2.0\linewidth]{figs/e2e-lowrtt-long.pdf}

         \caption{Propagation delay = 100ms)}
         \label{fig:}
     \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.32\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figs/e2e-medrtt.pdf}
    %      \caption{Medium RTT (200ms)}
    %      \label{fig:}
    %  \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=1.0\linewidth]{figs/e2e-highrtt-long.pdf}
         \caption{Propagation delay = 300ms)}
         \label{fig:}
     \end{subfigure}
     \vspace{.05cm}
    \tightcaption{Video quality vs. tail delay under different RTT\vspace{.1cm}}
    \label{fig:e2e-rtt}
\end{figure}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=2.0\linewidth]{figs/e2e-lowqueue-long.pdf}
         \caption{Droptail queue = 15 packets}
         \label{fig:}
     \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.32\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figs/e2e-medqueue.pdf}
    %      \caption{Medium queue (25 packets)}
    %      \label{fig:}
    %  \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=1.0\linewidth]{figs/e2e-highqueue-long.pdf}
         \caption{Droptail queue = 35 packets}
         \label{fig:}
     \end{subfigure}\vspace{.05cm}
    \tightcaption{Video quality vs. tail delay under different queues \vspace{.1cm}}
    \label{fig:e2e-queue}
\end{figure}

\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    \includegraphics[width=0.75\linewidth]{figs/timeseries-jc.pdf}
    \tightcaption{\name achieves lower delay and decent quality during sudden bandwidth drops.}
    \label{fig:timeseries-ours}
\end{figure}



\tightsubsection{Video quality vs. tail frame delay}
\label{subsec:eval:e2e}

Next, we run \name and the baseline codecs on real bandwidth traces from Verizon and T-Mobile LTE (\S\ref{subsec:eval:setup}). 
We set RTT at default values (200ms) and droptail queue length of 25 packets.
We implemented two different congestion control algorithms: Google congestion control~\cite{carlucci2016analysis} (\textit{GCC}) and the congestion control from the previous work (\textit{Sal-CC})~\cite{salsify}. 
We also implemented FEC-protected H.265 and Salsify codec as the baseline codecs (\S\ref{subsec:eval:setup}).

Figure~\ref{fig:e2e-quality} compares \name and the baselines, in average quality (both PSNR and SSIM) and the 95-th percentile of frame-level delay across frames in a session. 
We see that \name significantly decreases the tail frame delay: \name is 251ms and 267ms when using GCC and Sal-CC respectively, compared to 401ms and 412ms for Salsify codec, and 4066ms and 1652ms for H.265 codec. When there is a packet loss, Salsify codec needs to skip frames, causing a delay increase. For H.265 codec, it needs to wait for those lost packets being retrasmitted, and such retransmission traffic will compete with the normal video traffic, causing a higher delay on H.265.

When under the same congestion control (Sal-CC or GCC), the average PSNR of \name, Salsify codec and H.265 are 46.2, 47.8, 47.9, respectively. 
Though \name's PSNR is on par or slightly lower, we believe the reduction in tail frame delay is worth the minor drop in quality.
We make a similar observation when measuring quality in SSIM (dB): \name's quality is similar or slightly lower than the quality of baseline using the same CC. 


% \yihua{check if we already mentioned congestion control before}
%We play a \fillme-second long video on \fillme cellular network traces~\cite{??} and set the propagation delay at \fillme ms and queue length at \fillme. 
%\jc{YIHUA, please fill in some detailed reading}

%\jc{
%\begin{itemize}
%    \item by trace set
%    \item by rtt
%    \item by queue length
%    \item a concrete example
%\end{itemize}
%}

We then test \name's performance on the same traces but under different queue lengths and different propagation delays.
Figure~\ref{fig:e2e-rtt} and Figure~\ref{fig:e2e-queue} show that \name consistently reduces tail delay under different network delays or under different droptail queue lengths. 
In particular, \name has more delay reduction when the queue is shorter. 
This is because during congestion, shorter queues tend to drop previous frames packets more aggressively, and might still delivery {\em some} packets (though not all) of the latest frame to the receiver. 
In such cases, \name lets the client decode the frame early based on any subset of packets it has received. 

% we use synthetic bandwidth traces, where the bandwidth is 5Mbps but scattered with episodes of low bandwidth 1Mbps for 500ms (see Figure~\ref{??} for an example) and these low bandwidth episodes come at a Poisson distribution. 
% Such patterns are typically used in prior work (\eg~\cite{??,??) } to emulate impact of bursty competing flows.

% As shown in Figure~\ref{??}, \name has higher tail delay reduction under higher propagation delays or shorter queues. \jc{YIHUA, please fill in some detailed reading}
% These results highlight that \name reduces delay when packet retransmission or redundancy-based schemes do not suffice. 
% Likewise, our gain will be negligible if the RTT is very low to allow instant packet retransmission (in which case, we speculate SVC will be more fitting), or if the packet losses are largely constant (in which case, FEC will be an ideal choice).

Finally, we show how \name and the baselines behavior in a concrete bandwidth trace sample (Figure~\ref{fig:timeseries-ours}).
The bandwidth drops from 5Mbps to 1Mbps at 1.9sec and last for 200ms, before bouncing back to 5Mbps (another bandwidth drop occurs at 3.9sec).
We can see that during each bandwidth drop, \name's delay does not increase as sharp as the baselines (notably Salsify is the second best since it could skip frames).
\name and Salsify use the same CC, so their quality roughly matches on frames not skipped by Salsify.
That said, \name's quality degrades marginally with no frame skipping during congestion, and it bounces back once packet losses disappear. 



% \jc{YIHUA, please fill in some detailed reading}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/encoding-lat.pdf}
         \caption{Encoding latency}
         \label{fig:system-encoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/decode.pdf}
         \caption{Decoding latency}
         \label{fig:system-decoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/multicode.pdf}
         \caption{Latency of encoding multiple versions}
         \label{fig:system-encoding-versions}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/mem-usage.pdf}
         \caption{Memory usage of loading multiple models}
         \label{fig:system-memeory}
     \end{subfigure}
     \hfill
     \tightcaption{Memory and compute overhead of \newae}
     \label{fig:}
\end{figure}

\tightsubsection{Memory and computing overhead}
\label{subsec:eval:system}

% \zy{There is a typo ("decodeing latency") on the y-axis label on Figure 16 (b). (figs/decode.pdf)}

% Remember that \newae needs a P-frame encoder and a I-frame encoder to encode each frame as a P-frame and an I-patch (a small spatial region without reference).
Our implementation of \newae optimizes both memory footprint and encoding/decoding delay (described in \S\ref{subsec:optimize}), and we test its effectiveness on a Nvidia GeForce RTX 3080 GPU. 
Figure~\ref{fig:system-encoding} and Figure~\ref{fig:system-decoding} show that compared to the original (unoptimized) implementation of pre-trained autoencoder (which takes 100ms to encode a 480p frame), our implementation can encode a 480p frame in less than 25ms (a $4\times$ speedup).\footnote{The only autoencoder that achieves comparable encoding/decoding speed is~\cite{elf}, and it achieves such speed on a 5x more expensive Titan V GPU. We hope to compare it with \newae, but it is not open-source.}
This translates to almost 40fps. 
Even for 720p HD videos, our optimized codec can achieve 18fps (55ms encoding per frame). 
% \fillme~fps/\fillme~fps, \newae encodes/decodes 480p frames at \fillme~fps/\fillme~fps, a \fillme$\times$ speedup.
This acceleration comes from downsampling frames in motion-vector estimation. 
Moreover, when adapting to a target bitrate, \name encodes the next frame multiple times {\em without} needing to run the entire encoder multiple times, because it re-uses the motion-compensated prediction, so only the residuals need to be encoded at multiple bitrates.
Figure~\ref{fig:system-encoding-versions} shows that the delay of encoding a frame at three different bitrates only increases marginally compared to encoding one frame. 

In terms of memory usage, our optimized implementation saves the memory footprint of loading 9 models by over 60\% since most NN layers are shared. 
% Figure~\ref{??} shows that compared to loading the multiple autoencoders (I-frame encoder/decoder and a P-frame encoder/decoder of each bitrate) in GPU memory, the memory usage \name's autoencoders (not including the memory usage of intermediate features) is \fillme\% smaller, because they share most of the layers (only the last \fillme layers of the encoder and the first \fillme layers of the decoders are different). 
Note that \newae does not change the NN architecture of the autoencoders---only the weights are retrained and the way they are used is optimized. We speculate that they could be made more efficient with appropriate modification to its NN architecture.

% Figure~\ref{??} validate that \newae's coding efficiency is comparable to (even slightly better than) without the optimizations (\ie without sharing the NN backbone or downsampling and sharing the motion-vectors.)
% This is because, though quality does drop with these optimizations, the encoded size also drops (due largely to the downsampled motion vectors), which result in a similar bitrate-quality trade-off frontier.

% \jc{The only autoencoder that achieves comparable encoding/decoding speed is Elf~\cite{??}. 
% We hope to compare it with \newae, but it is not open-source. }


% \jc{remember to highlight that the speed is comparable to elf, which runs on the 5x more expensive titan v gpu.}

\begin{comment}

\subsection{Design choices in \name}

\jc{
\begin{itemize}
    \item different training loss patterns
    \item different training \rate distributions
    \item saliency-based redunancy
    \item packet prioritization
    \item computing overhead in delay and in memory
\end{itemize}
}

\end{comment}

==> sections/old/eval_v4.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Evaluation}
\label{sec:eval}

The findings of our evaluation can be summarized as follows:
\begin{packeditemize}
\item {\bf Quality-delay tradeoff:} On real and synthetic network traces with bandwidth fluctuation, \name reduces tail delay by 2$\times$, compared to other loss-resilient schemes (FEC, Salsify, error concealment~\cite{??}) while still obtaining decent quality. \name can also eliminate all the video freezes longer than 500ms. Our real user study also shows \name delivers better user experience compared to the baselines.
\item {\bf Loss resilience:} Though \newae's quality under no packet loss is on par with H.264 and slightly worse than H.265, it is data-scalable---graceful quality degradation with higher loss rate---under various videos and bitrates. 
\item {\bf User experience}: Our user study shows the video rendered by \name can achieve higher average subjective ratings by users than the baselines.
%\jc{a few example numbers}
%strikes a better trade-off between average video quality and tail delay than a wide range of baselines.
%\jc{a few example numbers}
\item {\bf Overhead:} Our implementation of \name can encode/decode 480p video at \fillme~fps/\fillme~fps and 720p HD video at \fillme~fps/\fillme~fps, a \fillme$\times$ speedup compared to off-the-shelf autoencoders. With the optimization for CPU (\S\ref{??}), \name can also encode/decode 720p HD video at \fillme~fps/\fillme~fps on CPU without causing huge quality degredation.
\end{packeditemize}


\tightsubsection{Setup}
\label{subsec:eval:setup}

\mypara{Baseline implementations}
\yihua{update text: rewrite baseline implementation}
Our baseline codecs include H.265 and H.264. 
We use their implementations in \texttt{ffmpeg} (version 4.2.7). 
Importantly, we do not restrict their GoP (I-frame interval) and the number of history frames to search for reference macroblocks. 
Following recent work in real-time video coding~\cite{ZEROLAT1,ZEROLAT2}, we use the \texttt{zerolatency} option (no B-frames) and the \texttt{fast} preset of H.265\footnote{The command line we used to encode a video is \texttt{ffmpeg -y -i Video.y4m -c:v libx265 -preset fast -tune zerolatency -x265-params "crf=Q:keyint=3000" output.mp4} where {\em Q} controls the quality and size of the output video}.

We use implementations for SVC, Salsify, and FEC, based on H.265.
We simplify the implementation in a way that makes their quality slightly better than they would actually do. 
Our implementation of SVC assumes that each quality level exactly {\em matches} the quality and size of the non-SVC coding of H.265, whereas even the state-of-the-art SVC (based also on autoencoders~\cite{swift}) achieves lower quality than H.265 at a quality level of the same frame size. (This effectively is an idealized version of Swift~\cite{swift}.)
We follow Salsify's logic for congestion control, frame skipping, and packet pacing, but instead of using Salsify's multi-trial encoding to approximate the target bitrate of each frame, we assume that the encoded frame size exactly {\em matches} each frame's target bitrate but the quality matches the {\em qp} value whose bitrate is barely {\em higher} than the target bitrate.
For FEC-protected H.26x, we use the same loss-rate prediction logic implemented in the public release of WebRTC~\cite{WEBRTCSRC} but remove the upper-bound of 50\% redundancy rate that is used in WebRTC \eg if the predicted packet loss rate is 60\%, we assume FEC will tolerate any packet loss ratio under 60\%.) %but instead of mapping it to the coarse-grained FEC redundancy rates, we assume an idealized FEC that can reconstruct a frame if the actual loss rate matches the predicted loss rate (\eg if the predicted packet loss rate is 50\%, we assume FEC will exactly tolerate 50\% packet loss.)
%This effectively approximates the situation where data can be packetized infinitesimally.
While these simplifying assumptions lead to a slightly optimistic estimate of the baselines' performance, we hope they make our results more relevant in the long run, as the implementations of SVC, and bitrate control, and FEC might evolve and improve in the future.

\mypara{Testbed setup and network traces}
%\mypara{Network and compute conditions}
\yihua{update simulator implementation here, with a visualization (network trace, link configuration, sender receiver, GPU)}
To evaluate \name and the baselines, we built an end-to-end packet level simulator as shown in Figure~\ref{??}.
The simulator runs on a linux machine with two Nvidia GeForce RTX 3080 GPUs that is used for video encoding and decoding (each using one GPU). 
The server runs Ubuntu 18.04 with 2 Inten Xeon 4210R CPU and 256GB memory.

We test \name on 8 real bandwidth traces distributed with the Mahimahi network-emulation tool~\cite{netravali2015mahimahi}\footnote{The data set has 16 traces. We filtered out the traces having an average bandwidth lower than 1Mbps as they do not fit the bandwidth requirement of video traffic.}.
We also evaluate the system on broadband traces from FCC dataset in \S\ref{??}


By default, we set the one-way network propagation delay to be 100ms and the queue size to be 25 packets (equals to \fillme BDP).
We also show the impact of different propagation delays and queue sizes in \S\ref{subsec:eval:e2e}.
% We conduct all experiments on a machine with two Nvidia GeForce RTX 2080 GPUs as the sender and receiver (each using one GPU). The server runs Ubuntu 18.04 with 2 Intel Xeon Silver 4110 CPU and 64GB memory.
% %\jc{more details, such as cuda version, linux version, cpu, memory, etc}
% We measure \name's encoding and decoding delays on the GPU (see results in \S\ref{subsec:eval:system}) and we include these delays in \name's frame delay. 


\mypara{Metrics}
We measure the performance of a video session in three aspects.
{\em Quality} of a frame is measured by SSIM and PSNR (RGB and YUV), and we report the average value across received frames. 
{\em Delay} of a frame is measured by the time lapse between the beginning of encoding to the end of decoding. 
For skipped frames (by Salsify), their decoding time equals the next decoding time of the next received frame. 
We report the tail (95th\% percentile) of the delays across frames in a session.
\textcolor{blue}{
We also measure the {\em smoothness} of the video by calculating the average video stalls per minute, where a video stall is defined as a frame freezing for more than 0.5 second.}
\jc{why AVERAGE quality vs TAIL delay?}
%\jc{describe frame rate metric}


\mypara{Test videos}
Our evaluation uses 60 videos from three public datasets (Kinetics~\cite{Kinetics}, UVG~\cite{mercat2020uvg} and FVC~\cite{FVCDATASET}), each video is of at least 10 seconds. 
%Table~\ref{sec:??} summarizes the datasets.
Importantly, we choose these videos because they are different from the training set, allowing us to stress-test the generalization of autoencoders.
The FVC dataset includes 5 videos captured from video conferencing, one of \name's main target use-cases.
These videos cover a range of spatial and temporal dynamics (\S\ref{app:siti})
and cover three resolutions (640$\times$360, 1280$\times$720 and 1920$\times$1280), with at least 5 videos in each resolution. 
The performance is reported as an average across all the frames in the videos.



%\mypara{Baselines}
%We compare the performance of \name with multiple state-of-the-art real-time video techniques that use different combinations of video coding and congestion control algorithms: 
%\begin{packeditemize}
%\item {\em Reference:} H.26x with adaptive FEC and GCC
%\item {\em Salsify:}
%\item {\em Idealized SVC:}
%\end{packeditemize}



\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, using GCC}
         \label{fig:normal-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/gcc-default-stall.pdf}
         \caption{SSIM V.S. average stall ratio, using GCC}
         \label{fig:normal-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/sal-default-delay.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, using Salsify-CC}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/sal-default-stall.pdf}
         \caption{SSIM V.S. average stall ratio, using Salsify-CC}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
     \vspace{-0.2cm}
     \tightcaption{Overall simulation result using default setup \textcolor{red}{more smart baselines)}}
     \label{fig:normal-simulation}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-queue15.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, when queue = 15}
         \label{fig:queue15-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-queue15.pdf}
         \caption{SSIM V.S. avg stall ratio, when queue = 15}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-queue35.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, when queue = 35}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-queue35.pdf}
         \caption{SSIM V.S. avg stall ratio, when queue = 35}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \vspace{-0.2cm}
     \tightcaption{Impact of different queue length \textcolor{red}{TODO: Hanchen!}}
     \label{fig:simulation-queue15}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-delay50.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, when delay = 50}
         \label{fig:queue15-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-delay50.pdf}
         \caption{SSIM V.S. avg stall ratio, when delay = 50}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-delay150.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, when delay = 150}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-delay150.pdf}
         \caption{SSIM V.S. avg stall ratio, when delay = 150}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \vspace{-0.2cm}
     \tightcaption{Impact of different propagation delay \textcolor{red}{TODO: Hanchen!}}
     \label{fig:simulation-queue15}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/e2e-part-delay.png}
         \caption{SSIM V.S. 95\% tail frame delay, using AQM}
         \label{fig:queue15-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/e2e-part-stall.png}
         \caption{SSIM V.S. avg stall ratio, using AQM}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/e2e-part-delay.png}
         \caption{SSIM V.S. 95\% tail frame delay, when 1\% random loss}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/e2e-part-stall.png}
         \caption{SSIM V.S. avg stall ratio, when 1\% random loss}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \vspace{-0.2cm}
     \tightcaption{Impact of other factors (AQM, random loss) \textcolor{red}{TODO: Hanchen!}}
     \label{fig:simulation-queue15}
\end{figure*}




\begin{figure}[t!]
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/e2e-part-delay.png}
         \caption{SSIM V.S. 95\% tail frame delay, using FCC dataset}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/e2e-part-stall.png}
         \caption{SSIM V.S. 95\% avg stall ratio, using FCC dataset}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \vspace{-0.1cm}
     \tightcaption{Results using FCC dataset \textcolor{red}{TODO: Hanchen!}}
     \label{fig:simulation-ablation}
\end{figure}


\begin{figure}[t!]
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/e2e-part-delay.png}
         \caption{SSIM V.S. 95\% tail frame delay, if we remove xxx features}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/e2e-part-stall.png}
         \caption{SSIM V.S. 95\% avg stall ratio, if we remove xxx features}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \vspace{-0.1cm}
     \tightcaption{Ablation study (per packet EC, loss resilience) \textcolor{red}{TODO: Hanchen!}}
     \label{fig:simulation-ablation}
\end{figure}


\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    \includegraphics[width=0.75\linewidth]{figs/timeseries-jc.pdf}
    \tightcaption{\name achieves lower delay and decent quality during sudden bandwidth drops. \textcolor{red}{TODO: Hanchen!}}
    \label{fig:timeseries-ours}
\end{figure}


\tightsubsection{Video quality vs. tail frame delay}
\label{subsec:eval:e2e}

We run \name and the baseline codecs on real bandwidth traces from Verizon and T-Mobile LTE (\S\ref{subsec:eval:setup}). 
We set propagation delay at default values (100ms) and a droptail queue length of 25 packets.
We implemented two different congestion control algorithms: Google congestion control~\cite{carlucci2016analysis} (\textit{GCC}) and the congestion control from the previous work (\textit{Sal-CC})~\cite{salsify}. 
We also implemented FEC-protected H.265 and Salsify codec as the baseline codecs (\S\ref{subsec:eval:setup}).

\yihua{change the text to include new graphs here}

Figure~\ref{fig:normal-psnr-delay} and~\ref{fig:normal-ssim-delay} compares \name and the baselines, in average quality (both PSNR and SSIM) and the 95-th percentile of frame-level delay across frames in a session. 
We see that \name significantly decreases the tail frame delay: \name is 251ms and 267ms when using GCC and Sal-CC respectively, compared to 401ms and 412ms for Salsify codec, and 4066ms and 1652ms for H.265 codec. When there is a packet loss, Salsify codec needs to skip frames, causing a delay increase. For H.265 codec, it needs to wait for those lost packets being retrasmitted, and such retransmission traffic will compete with the normal video traffic, causing a higher delay on H.265.

When under the same congestion control (Sal-CC or GCC), the average PSNR of \name, Salsify codec and H.265 are 46.2, 47.8, 47.9, respectively. 
Though \name's PSNR is on par or slightly lower, we believe the reduction in tail frame delay is worth the minor drop in quality\textcolor{blue}{, which is also confirmed by our user study (will show later)}.
We make a similar observation when measuring quality in SSIM (dB): \name's quality is similar or slightly lower than the quality of baseline using the same CC. 

\textcolor{blue}{Although \name has a slightly lower frame quality, Figure~\ref{fig:normal-psnr-stall} shows that it does not have any video stalls longer than 500ms on the network traces we used, while the baselines cannot avoid stalls. More importantly, the figure also shows that \name can eliminate the video stalls no matter which underlying congestion control it is using. This is because the data-scalibility of \newae make the frame still decodable under packet losses while the baseline methods need to wait for at least one round trip time when the received frame is not decodable. }

% \yihua{check if we already mentioned congestion control before}
%We play a \fillme-second long video on \fillme cellular network traces~\cite{??} and set the propagation delay at \fillme ms and queue length at \fillme. 
%\jc{YIHUA, please fill in some detailed reading}

%\jc{
%\begin{itemize}
%    \item by trace set
%    \item by rtt
%    \item by queue length
%    \item a concrete example
%\end{itemize}
%}

We then test \name's performance on the same traces but under different queue lengths and different propagation delays.
Figure~\ref{fig:simulation-queue15},~\ref{fig:simulation-queue35},~\ref{fig:simulation-rtt100} and~\ref{fig:simulation-rtt300} show that \name consistently reduces tail delay \textcolor{blue}{and eliminates the video stalls} under different network delays or under different droptail queue lengths.
In particular, \name has more delay reduction when the queue is shorter. 
This is because during congestion, shorter queues tend to drop previous frames packets more aggressively, and might still delivery {\em some} packets (though not all) of the latest frame to the receiver. 
In such cases, \name lets the client decode the frame early based on any subset of packets it has received. 

\textcolor{blue}{To show decreasing tail delay and increasing smoothness is worth the minor drop in quality for real users, we also setup a real user study on Amazon MTurk~\cite{??}. We sampled 8 video clips rendered by \name, Salsify codec and H.265 using {\em Sal-CC} as congestion control while using the same setup as Figure~\ref{fig:normal-simulation}. We confirm the sampled video clips have the same distribution of quality, tail delay and smoothness as Figure~\ref{fig:normal-simulation}. The video clips covers different genres including cloud gaming, real time sports events and indoor activities. When an MTurk user is signed up for the user study, the user will be randomly assigned to rate their user experience (with a Likert scale of 1-5) on the videos rendered by different methods. Figure~\ref{fig:user-study} shows the average rating (\ie, mean opinion score or MOS) among 750 users on the videos from each methods. It shows that \name can improve the MOS from 2-2.5 to 3.8-4.7.} 

% we use synthetic bandwidth traces, where the bandwidth is 5Mbps but scattered with episodes of low bandwidth 1Mbps for 500ms (see Figure~\ref{??} for an example) and these low bandwidth episodes come at a Poisson distribution. 
% Such patterns are typically used in prior work (\eg~\cite{??,??) } to emulate impact of bursty competing flows.

% As shown in Figure~\ref{??}, \name has higher tail delay reduction under higher propagation delays or shorter queues. \jc{YIHUA, please fill in some detailed reading}
% These results highlight that \name reduces delay when packet retransmission or redundancy-based schemes do not suffice. 
% Likewise, our gain will be negligible if the RTT is very low to allow instant packet retransmission (in which case, we speculate SVC will be more fitting), or if the packet losses are largely constant (in which case, FEC will be an ideal choice).

Finally, we show how \name and the baselines behavior in a concrete bandwidth trace sample (Figure~\ref{fig:timeseries-ours}).
The bandwidth drops from 5Mbps to 1Mbps at 1.9sec and last for 200ms, before bouncing back to 5Mbps (another bandwidth drop occurs at 3.9sec).
We can see that during each bandwidth drop, \name's delay does not increase as sharp as the baselines (notably Salsify is the second best since it could skip frames).
\name and Salsify use the same CC, so their quality roughly matches on frames not skipped by Salsify.
That said, \name's quality degrades marginally with no frame skipping during congestion, and it bounces back once packet losses disappear. 


\begin{figure}[t!]
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/ssim_loss_1200.pdf}
         \caption{Bitrate = 0.05}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/psnrloss.pdf}
         \caption{BPP = 0.10}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
        \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/psnrloss.pdf}
         \caption{BPP = 0.20}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/psnrloss.pdf}
         \caption{BPP = 0.40}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \vspace{-0.1cm}
     \tightcaption{\newae's loss resilience by bitrate and resolution \textcolor{red}{TODO: Yuhan, this figure is outdated, please add new bar-chart figures, grouped by different bitrates (bpps)}}
     \label{fig:loss_by_resolution_bitrate}
\end{figure}


\tightsubsection{Coding efficiency and loss resilience}

% \name's gains stem from the performance of the autoencoder \newae.
Figure~\ref{fig:loss_by_resolution_bitrate} compares \newae with the baselines codecs\footnote{We do not put Intra-MB insertion baseline here, since it's quality will quick drop below x-axis when loss ratio is between 5\% to 10\%.} under different packet loss rates when encoding videos of the same resolution and same target bitrate. 
In each figure, all lines have almost the same encoding bitrate with difference controlled within 5\%.
We ensure that \newae's encoded bitrate is {\em never} higher than the baselines, so even if the actual encoded bitrate is different, it does not favor \newae.
% Similarly, Figure~\ref{fig:loss_by_bitrate} compares the same set of solution when they have the same encoding bitrate.

% For each figure, the encoded bitrates of different solutions are controlled within 10\% difference (and to make it less favorable to \newae, we make sure that \newae's encoded bitrate is never higher than the baselines).
% Figure~\ref{fig:loss_by_resolution} shows the results by video resolution and Figure~\ref{fig:loss_by_bitrate} shows the results by encoding bitrate on 720P videos\footnote{We do not put Intra-MB insertion baseline here, since it's quality will quick drop below x-axis when loss ratio is between 5\% to 10\%}. 
The most salient feature of \newae is the graceful quality degradation with more packet losses. 
The average PSNR drop is only 2.1 to 3.9 under 30\% and 50\% packet losses. Even when the loss ratio is as high as 80\%, it has an average PSNR of 36.4, which is much better than the baselines except H.264 with 80\% FEC.
Compared with H.264 with fixed FEC protection, \newae can have a higher PSNR of 1.1 to 2.0 among different resolutions and different bitrates when there is no loss. This is because any arrived bytes in \newae contribute to the quality while in FEC, the redundant data is useless even if they do arrive at the decoder. On the other hand, FEC-based loss resiliency is also in a dilemma that a low FEC rate cannot protect against the high loss, but a high FEC rate leads to poor quality when the packet loss ratio is small. Our \newae solve's such dilemma by the graceful quality degradation.
\newae is also better than SVC with unequal FEC protection (\S\ref{subsec:abstractions}). 
The quality of SVC decreases quickly when the loss rate is small, as the high-quality layers are unlikely to be decodable in such cases. 
% As shown in Figure~\ref{fig:loss_by_resolution_bitrate}, \newae has a average PSNR gain of 3.9 over SVC when the loss ratio is 30\%.
We also note that the pretrained autoencoder models, which have not seen any losses in training, degrade poorly with higher loss rates. 
% It has an average PSNR decrease of 4.3 when loss ratio is 30\%, which is 2$\times$ higher than \newae.
% to h264 + fec baseline
% comparing to SVC


%\jc{
%\begin{itemize}
%    \item by bitrate
%    \item by video set
%    \item psnr vs. bitrate
%\end{itemize}
%}

% \jc{need a footnote to explain why intra-mb insertion is so bad}


\begin{figure}[t!]
    \centering
         \centering
        %\includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
        \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/psnr_v1.pdf}
         \label{fig:}
         \end{subfigure}
             \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/ssim_v1.pdf}
         \label{fig:}
         \end{subfigure}
         \vspace{.05cm}
    \tightcaption{Quality-size tradeoff of \newae. \textcolor{red}{TODO: Yuhan, here we need 2 figures with Y-axis of PSNR and SSIM}}
    \label{fig:psnr-vs-bpp}
\end{figure}



\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    \includegraphics[width=0.75\linewidth]{figs/decoded examples.pdf}
    \tightcaption{Example of decoded images under loss \textcolor{red}{TODO: Yihua, consistent plotting scripts and text}}
    \label{fig:decoded-example}
\end{figure}



\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    \includegraphics[width=0.75\linewidth]{figs/user-study-placeholder.pdf}
    \tightcaption{User study result \textcolor{red}{TODO: Yihua, consistent plotting scripts and text}}
    \label{fig:user-study}
\end{figure}



For any loss-resilient schemes, the ability to tolerate packet losses often comes with a drop of quality in absence of packet losses, and \newae is no exception. 
Figure~\ref{fig:psnr-vs-bpp} compares the \newae's quality under no packet losses with that of H.264 and H.265 across the test videos (all of which are randomly sampled from three datasets that are different from the training set, \S\ref{subsec:eval:setup}).
% evaluates the price \newae pays to get its loss resilience. It shows the average PSNR of \newae, H.264 and H.265 on different bitrate across all test videos.
Fortunately, at the same encoded bitrate, \newae is similar to H.264 and is only slightly worse than H.265. 
When bitrate varies from 2Mbps to 8Mbps, the average PSNR is 44.29, 44.31, and 44.84 for \newae, H.264 and H.265 respectively.

Remember that H.26x uses the zerolatency option and fast preset (which is typical to real-time videos, including WebRTC\footnote{Google's WebRTC~\cite{WEBRTCSRC} uses OpenH264~\cite{OPENH264}. They set the runtime parameter "usageType" to CAMERA\_VIDEO\_REAL\_TIME  (similar to zerolatency) and "complexityMode" to LOW\_COMPLEXITY (similar to fast)}. %\jc{Yihua, please add a footnote about the following: one is usageType = CAMERA\_VIDEO\_REAL\_TIME  (similar to zerolatency) and another is complexityMode = LOW\_COMPLEXITY (similar to fast)})
We confirm that without these settings, H.265's coding efficiency is better than \newae in the absence of packet losses.
However, our goal is a data-scalable autoencoder for real-time videos (shown shortly), rather than an autoencoder that outperforms heavily engineered H.26x codecs. 
Moreover, the coding efficiency of autoencoder could still be improved (\eg our autoencoder estimates motion vectors based only on one reference frame). 

%In Figure~\ref{??}, we use three metrics for video quality, even though our autoencoders are trained to optimize L2-norm between the reconstructed and original images, which is similar to RGB-PSNR, their quality compared to baselines is similar under different metrics.

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_traceset_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_rtt_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_queue_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}


%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=1.pdf}
%    \caption{Aggressiveness = 1}
%    \label{fig:}
%\end{figure*}
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=0.75.pdf}
%    \caption{Aggressiveness = 5}
%    \label{fig:}
%\end{figure*}








% \jc{YIHUA, please fill in some detailed reading}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/encoding speed example.pdf}
         \caption{Encoding latency}
         \label{fig:system-encoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/decding speed example.pdf}
         \caption{Decoding latency}
         \label{fig:system-decoding}
     \end{subfigure}
     \hfill
     % \begin{subfigure}[b]{0.49\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figs/multicode.pdf}
     %     \caption{Latency of encoding multiple versions}
     %     \label{fig:system-encoding-versions}
     % \end{subfigure}
     % \hfill
     % \begin{subfigure}[b]{0.49\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figs/mem-usage.pdf}
     %     \caption{Memory usage of loading multiple models}
     %     \label{fig:system-memeory}
     % \end{subfigure}
     % \hfill
     \tightcaption{Compute overhead of \newae \textcolor{red}{TODO: ziyi: update this graph}}
     \label{fig:}
\end{figure}

\begin{figure}[t!]
    \centering
         \centering
        %\includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
        \includegraphics[width=0.7\linewidth]{figs/cpu e2e.pdf}
         \label{fig:}
         \vspace{.05cm}
    \tightcaption{CPU end to end result. \textcolor{red}{TODO: Ziyi and Hanchen}}
    \label{fig:psnr-vs-bpp}
\end{figure}

\tightsubsection{Memory and computing overhead}
\label{subsec:eval:system}

% \zy{There is a typo ("decodeing latency") on the y-axis label on Figure 16 (b). (figs/decode.pdf)}

% Remember that \newae needs a P-frame encoder and a I-frame encoder to encode each frame as a P-frame and an I-patch (a small spatial region without reference).
Our implementation of \newae optimizes both memory footprint and encoding/decoding delay (described in \S\ref{subsec:optimize}), and we test its effectiveness on a Nvidia GeForce RTX 3080 GPU. 
Figure~\ref{fig:system-encoding} and Figure~\ref{fig:system-decoding} show that compared to the original (unoptimized) implementation of pre-trained autoencoder (which takes 100ms to encode a 480p frame), our implementation can encode a 480p frame in less than 25ms (a $4\times$ speedup).\footnote{The only autoencoder that achieves comparable encoding/decoding speed is~\cite{elf}, and it achieves such speed on a 5x more expensive Titan V GPU. We hope to compare it with \newae, but it is not open-source.}
This translates to almost 40fps. 
Even for 720p HD videos, our optimized codec can achieve 18fps (55ms encoding per frame). 
% \fillme~fps/\fillme~fps, \newae encodes/decodes 480p frames at \fillme~fps/\fillme~fps, a \fillme$\times$ speedup.
This acceleration comes from downsampling frames in motion-vector estimation. 
Moreover, when adapting to a target bitrate, \name encodes the next frame multiple times {\em without} needing to run the entire encoder multiple times, because it re-uses the motion-compensated prediction, so only the residuals need to be encoded at multiple bitrates.
Figure~\ref{fig:system-encoding-versions} shows that the delay of encoding a frame at three different bitrates only increases marginally compared to encoding one frame. 

In terms of memory usage, our optimized implementation saves the memory footprint of loading 9 models by over 60\% since most NN layers are shared. 
% Figure~\ref{??} shows that compared to loading the multiple autoencoders (I-frame encoder/decoder and a P-frame encoder/decoder of each bitrate) in GPU memory, the memory usage \name's autoencoders (not including the memory usage of intermediate features) is \fillme\% smaller, because they share most of the layers (only the last \fillme layers of the encoder and the first \fillme layers of the decoders are different). 
Note that \newae does not change the NN architecture of the autoencoders---only the weights are retrained and the way they are used is optimized. We speculate that they could be made more efficient with appropriate modification to its NN architecture.

% Figure~\ref{??} validate that \newae's coding efficiency is comparable to (even slightly better than) without the optimizations (\ie without sharing the NN backbone or downsampling and sharing the motion-vectors.)
% This is because, though quality does drop with these optimizations, the encoded size also drops (due largely to the downsampled motion vectors), which result in a similar bitrate-quality trade-off frontier.

% \jc{The only autoencoder that achieves comparable encoding/decoding speed is Elf~\cite{??}. 
% We hope to compare it with \newae, but it is not open-source. }


% \jc{remember to highlight that the speed is comparable to elf, which runs on the 5x more expensive titan v gpu.}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
%        \includegraphics[width=0.7\linewidth]{figs/a.pdf}
         \label{fig:}
         \vspace{.05cm}
    \tightcaption{Training curve study \textcolor{red}{Yihua and Anton}}
    \label{fig:psnr-vs-bpp}
\end{figure}


==> sections/old/eval_v5.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Evaluation}
\label{sec:eval}

The findings of our evaluation can be summarized as follows:
\begin{packeditemize}
\item {\bf Quality-delay tradeoff:} Under bandwidth fluctuations in real network traces, \name reduces the ratio of frames whose delay exceeds 400~ms by 4-8$\times$ compared to other loss-resilient schemes. %(FEC, Salsify, SVC, error concealment and frame skipping)
% (FEC, Salsify, SVC, error concealment~\cite{itu1999subjective} and Voxel~\cite{voxel}) 
while still obtaining decent quality.
Also, \name has significantly fewer stutterings (video freezes for over 200ms). Our user study has also confirmed that \name is rated more favorably than baselines.
% can also eliminate all the video freezes longer than 200ms. Our real user study also shows \name delivers better user experience compared to the baselines.
% \item {\bf User experience}: Our subjective IRB-approved user study shows the video rendered by \name are rated much more favorably by users than baseline loss resilient schemes.
% can achieve higher average subjective ratings by users than the baselines.
\item {\bf Loss resilience:} Though \name's quality under no packet loss is on par with H.264 and H.265, it is data-scalable---graceful quality degradation with higher loss rate---under various videos and bitrates. 
%\jc{a few example numbers}
%strikes a better trade-off between average video quality and tail delay than a wide range of baselines.
%\jc{a few example numbers}
\item {\bf Overhead:} Our implementation of \name can encode/decode 480p video at 40~fps/65~fps and 720p HD video at 28~fps/35~fps, a 1.5-2$\times$ speedup compared to off-the-shelf autoencoders. With the optimization for CPU (\S\ref{subsec:fast-coding}), \name can also encode/decode 720p HD video at 27~fps/25~fps on CPU without causing huge quality degredation.
\end{packeditemize}


\tightsubsection{Setup}
\label{subsec:eval:setup}

\mypara{Training of \name}
We trained \name's autoencoder by fine-tuning the DVC model from~\cite{dvc} on vimeo-90K~\cite{vimeo-dataset} dataset.
We set learning rate to $10^{-4}$ and the fine-tuning usually takes 1-2 hours with an Nvidia RTX 3080 GPU.

\mypara{Baselines}
%\yihua{update text: rewrite baseline implementation}
We implemented the following loss-resilient baselines using H.265 and H.264 of \texttt{ffmpeg} (version 4.2.7).
\begin{packeditemize}
  \item {\em H.265 (or H.264) with FEC (Tambur)}~\cite{rudow2023tambur}: We use the implementation from \texttt{ffmpeg} and do not restrict their GoP (I-frame interval) and the number of history frames to search for reference macroblocks. Following recent work in real-time video coding~\cite{ZEROLAT1,ffmpegstreaming}, we use the \texttt{zerolatency} option (no B-frames) and the \texttt{fast} preset of H.265\footnote{The command line we used to encode a video is \texttt{ffmpeg -y -i Video.y4m -c:v libx265 -preset fast -tune zerolatency -x265-params "crf=Q:keyint=3000" output.mp4} where {\em Q} controls the quality of the frame.} 
  \edit{For FEC-protected H.26x, we implemented Tambur~\cite{rudow2023tambur}, which is the latest smart FEC-protection algorithm using streaming codes~\cite{badr2017fec}. To estimate the loss rates, we use the same logic as WebRTC described in~\cite{holmer2013handling, carlucci2016analysis}.}
  %For FEC-protected H.26x, we use the same FEC logic of WebRTC described in~\cite{holmer2013handling, carlucci2016analysis}.
  % we use the same loss-rate prediction logic implemented in the public release of WebRTC~\cite{WEBRTCSRC}\jc{cite the paper}.
  \item {\em SVC}: We used an idealized SVC implementation such that when the first $\times$ packets arrive, it will reach a quality same as that of H.265 at the same size.
  This slightly outperforms the state-of-the-art SVC~\cite{swift}.
  % achieves quality slightly better than it would actually be. The implementation assumes that each quality level will has {\em exactly} the same quality and size of the non-SVC coding of H.265, whereas even the state-of-the-art SVC~\cite{swift} achieves lower quality than H.265 at a quality level of the same frame size. 
  By default, we also add 50\% FEC to protect the base layer for SVC.
  \item {\em Salsify-codec}~\cite{salsify}: We use implementation of Salsify from their official github repo~\cite{salsify-impl} The encoded frame size of Salsify-codec will never overshoot the target bitrate calculated by the underlying congestion control algorithm. When packet loss happens, the encoder can dynamically choose a reference frame to make later frames decodable without retransmitting any packets.%\jc{yihua: substantiate}
  \item {\em H.264 with error concealment}~\cite{kang2022error}: \edit{We implemented the error concealment technique for H.264-coded video using a recent machine-learning-based error concealment solution~\cite{kang2022error}. It uses neural networks to estimate the missing motion vectors and inpaint the missing areas. We assign 128$\times$128-pixel blocks randomly to packets and assume each packet is individually decodable. Note that this may substantially increase the frame size~\cite{KUMAR2006425}, but to err on the side of caution, we ignore this overhead.}
  %\footnote{Some early papers tried to apply error concealment on H.265, which might perform better though still limited by the issues outlined in \S\ref{subsec:prior}.} using motion vector reconstruction~\cite{zhou2010efficient}. We also trained an inpainting model for improving the quality of the reconstructed image. 
  %We randomly assign MBs to packets and assume each packet is individually decodable. Note that this may substantially increase the frame size~\cite{KUMAR2006425}, but to err on the side of caution, we ignore this overhead.
  % are any lost packet will not affect the decoding of macroblocks in the arrived packets (\ie packets are independently decodable). 
  \item {\em Voxel}~\cite{voxel}: We adapt the idea in~\cite{voxel} and sort the video frames by the PSNR drop caused by skipping the frame. For 25\% frames with the lowest PSNR drop, we use error concealment without any packet retransmission, and for the remaining frames (which cause more PSNR drops when skipped), we retransmit all the lost packets. Following~\cite{voxel}, we use a GoP (chunk length) of 4 seconds.
  \yihua{add a paragraph about what SR baseline we are using here}
  % \item {\em Grace-naive}~\cite{cheng2022grace}: Our previous work on \name delved into the potential applications of autoencoders for data scalable video codecs, yet it harbored several shortcomings. It employed a simplistic per-packet entropy encoding approach, which incurred a significantly higher overhead than the method outlined in \S\ref{subsec:packetization}. It also lacked the optimizations proposed in \S\ref{sec:delivery}. A comprehensive comparison between \name and {\em Grace-naive} is provided in \S\ref{sec:related}.





  % We also assume the segment length of the video is 4 seconds (\ie a new I-frame will be sent every 4 seconds) for this baseline. 
\end{packeditemize}

For the baselines of Salsify, SVC, and Voxel, we make an idealized assumption that on each frame, the output bitrate of the codec perfectly matches the target bitrate chosen by the congestion control algorithm (explained in \S\ref{subsec:eval:e2e}), \ie never overshooting or undershooting, but the actual quality matches that of the highest \texttt{qp} that leads to a frame greater than the target bitrate. 
To err on the side of caution, these optimizations make the baselines' performance slightly better.
% In other words, their performance is higher than it would actually be in the real world.

% \yihua{need to emphasis that we are cheating for error concealment and Voxel. 1. assume perfectly match the target bitrate, 2. idealized per packet ec for h264 }

% Our baseline codecs include H.265 and H.264. 
% We use their implementations in \texttt{ffmpeg} (version 4.2.7). 
% Importantly, we do not restrict their GoP (I-frame interval) and the number of history frames to search for reference macroblocks. 
% Following recent work in real-time video coding~\cite{ZEROLAT1,ZEROLAT2}, we use the \texttt{zerolatency} option (no B-frames) and the \texttt{fast} preset of H.265\footnote{The command line we used to encode a video is \texttt{ffmpeg -y -i Video.y4m -c:v libx265 -preset fast -tune zerolatency -x265-params "crf=Q:keyint=3000" output.mp4} where {\em Q} controls the quality and size of the output video}.

% We use implementations for SVC, Salsify, and FEC, based on H.265.
% We simplify the implementation in a way that makes their quality slightly better than they would actually do. 
% Our implementation of SVC assumes that each quality level exactly {\em matches} the quality and size of the non-SVC coding of H.265, whereas even the state-of-the-art SVC (based also on autoencoders~\cite{swift}) achieves lower quality than H.265 at a quality level of the same frame size. (This effectively is an idealized version of Swift~\cite{swift}.)
% We follow Salsify's logic for congestion control, frame skipping, and packet pacing, but instead of using Salsify's multi-trial encoding to approximate the target bitrate of each frame, we assume that the encoded frame size exactly {\em matches} each frame's target bitrate but the quality matches the {\em qp} value whose bitrate is barely {\em higher} than the target bitrate.
% For FEC-protected H.26x, we use the same loss-rate prediction logic implemented in the public release of WebRTC~\cite{WEBRTCSRC} but remove the upper-bound of 50\% redundancy rate that is used in WebRTC \eg if the predicted packet loss rate is 60\%, we assume FEC will tolerate any packet loss ratio under 60\%.) %but instead of mapping it to the coarse-grained FEC redundancy rates, we assume an idealized FEC that can reconstruct a frame if the actual loss rate matches the predicted loss rate (\eg if the predicted packet loss rate is 50\%, we assume FEC will exactly tolerate 50\% packet loss.)
%This effectively approximates the situation where data can be packetized infinitesimally.
% While these simplifying assumptions lead to a slightly optimistic estimate of the baselines' performance, we hope they make our results more relevant in the long run, as the implementations of SVC, and bitrate control, and FEC might evolve and improve in the future.

\mypara{Testbed setup and network traces}
%\mypara{Network and compute conditions}
% \yihua{update a visualization for the simulator (network trace, link configuration, sender receiver, GPU)}
To evaluate \name and the baselines, we built a packet-level simulator that includes the encoder and decoder.
The simulator takes as input a bandwidth trace and a video and simulates the {\em end-to-end} video streaming process, including encoding, packetization, packet transmission, and decoding. The output of the simulator includes a decoded video and end-to-end delay of each decoded frame. 
The simulator uses a drop tail queue with a configurable queue length to simulate packet losses caused by the congestion.
% The simulator runs on a Linux machine with two Nvidia GeForce RTX 3080 GPUs\jc{is this different from the real benchmark?} that are used for video encoding and decoding (each using one GPU). 
The server runs Ubuntu 18.04 with 2 Intel Xeon 4210R CPU and 256GB memory.
We test \name on eight real bandwidth traces from the LTE traces in the Mahimahi network-emulation tool~\cite{netravali2015mahimahi} (we filtered out the traces having an average bandwidth lower than 1Mbps).
The simulator updates bandwidth every 0.5 seconds.

\begin{comment}
    

We test \name on 16 real bandwidth traces, eight of which are LTE traces from the Mahimahi network-emulation tool~\cite{netravali2015mahimahi} (we filtered out the traces having an average bandwidth lower than 1Mbps),
% \footnote{The data set has 16 traces. We filtered out the traces having an average bandwidth lower than 1Mbps as they do not fit the bandwidth requirement of video traffic.}, 
and the remaining ones are broadband traces from FCC dataset~\cite{fcc-dataset}.
% These bandwidth traces fluctuate between 0.2Mbps to 8Mbps, and 
The simulator updates bandwidth every 0.5 seconds.
% Within each trace, the bandwidth is ranging from 0.2Mbps to 8Mbps, and will change every 0.5 seconds.

\end{comment}

By default, we set the one-way network propagation delay to be 100ms and the queue size to be 25 packets.
% (equals to 0.75×\times BDP).
We will also vary these values to show their impact in \S\ref{subsec:eval:e2e}.
% also show the impact of different propagation delays and queue sizes 
% We conduct all experiments on a machine with two Nvidia GeForce RTX 2080 GPUs as the sender and receiver (each using one GPU). The server runs Ubuntu 18.04 with 2 Intel Xeon Silver 4110 CPU and 64GB memory.
% %\jc{more details, such as cuda version, linux version, cpu, memory, etc}
% We measure \name's encoding and decoding delays on the GPU (see results in \S????????????????????????????????????\ref{subsec:eval:system}) and we include these delays in \name's frame delay. 


\mypara{Metrics}
We measure the performance of a video session in the following three aspects.
\begin{packeditemize}
    \item {\em Quality} of a video is measured by frame-level SSIM, and we report the average value across received frames. 
    \item {\em Realtimeness} reports the ratio of the frames that has a {\em frame-level delay} over 400ms~\cite{zoom-latency-setting}.
    Frame delay means the time lapse between the beginning of encoding and the end of decoding.
    For skipped frames, we follow Salsify~\cite{salsify} and set their decoding time to the decoding time of the next received frame.
    % is measured by the {\em frame-level delay}, \ie time lapse between the beginning of encoding to the end of decoding. 
    % For skipped frames (by Salsify), their decoding time equals the next decoding time of the next received frame. 
    % We report the ratio of the frames that has a delay over 400ms. %tail (98th^{th}\% percentile) of the delays across frames in a session.
    \item {\em Smoothness} of the video is measured by the video stall ratio, where a stall is defined as the fraction of inter-frame gaps that exceed a threshold. Following the previous work~\cite{macmillan2021measuring} and the logic in WebRTC, we set the threshold to 200ms. %We choose this threshold as it matches the definition in WebRTC. 
\end{packeditemize}



% \textcolor{blue}{
% We also measure the {\em smoothness} of the video by calculating the average video stalls per minute, where a video stall is defined as a frame freezing for more than 0.5 second.}
% \jc{why AVERAGE quality vs TAIL delay?}
%\jc{describe frame rate metric}

% \begin{table}
% \begin{center}
% \footnotesize
% \begin{tabular}{ ccccc } 
%  \hline
%   & \textbf{\# of videos} & \textbf{Duration} & \textbf{Resolution} & \textbf{Characteristics} \\ \hline
%  \textbf{Kinetics 360P} & 49 & 490 secs  & 640×\times3 & \\ \hline 
%  \textbf{UVG} & 5 & 120 secs & 1920$\times$1080 & \\ \hline 
%  \textbf{FVC} & 6 & 135 secs & 1920$\times$1080 & \\ \hline 
%  \hline
% \end{tabular}
% \end{center}
% \label{tab:dataset}
% \vspace{0.3cm}
% \tightcaption{Dataset description.\jc{
% YIHUA: 1. add description. 2. add 360p, 3. add citation, 4. in text, add a link to the data repo (github). ask zhengxu (anonymized)}}
% \end{table}

\begin{table}[]
\footnotesize
\begin{tabular}{ccccc}
\hline
Dataset                                                  & \# of videos & Duration & Resolution       & Characteristics                                                                     \\ \hline
\begin{tabular}[c]{@{}c@{}}Kinetics \\ 360P\end{tabular} & 8            & 80 sec   & 640$\times$360   & \begin{tabular}[c]{@{}c@{}}Human actions and\\ interaction of objects\end{tabular}  \\ \hline
\begin{tabular}[c]{@{}c@{}}Kinetics \\ 720P\end{tabular} & 41           & 410 sec  & 1280$\times$720  & \begin{tabular}[c]{@{}c@{}}Human actions and \\ interaction of objects\end{tabular} \\ \hline
UVG                                                      & 5            & 120 sec  & 1920$\times$1280 & \begin{tabular}[c]{@{}c@{}}HD videos (human, \\ nature, sports, etc)\end{tabular}   \\ \hline
FVC                                                      & 6            & 135 sec  & 1920$\times$1080 & \begin{tabular}[c]{@{}c@{}}Video calls \\ (indoor and outdoor)\end{tabular}         \\ \hline
Total                                                    & 60           & 745 sec  &                  &                                                                                     \\ \hline
\end{tabular}
\vspace{0.3cm}
\tightcaption{Dataset description 
% \jc{YIHUA: 3. add citation, 4. in text, add a link to the data repo (github). ask zhengxu (anonymized)}
 }
\label{tab:dataset}
\end{table}

\mypara{Test videos}
Our evaluation uses 60 videos randomly sampled from three public datasets (Kinetics~\cite{Kinetics}, UVG~\cite{mercat2020uvg} and FVC~\cite{FVCDATASET}), each video is at least 10 seconds. The detailed description is in Table~\ref{tab:dataset}.
%Table~\ref{sec:??} summarizes the datasets.
Importantly, we choose these videos because they are different from the training set, allowing us to stress-test the generalization of autoencoders.
The FVC dataset includes 5 videos captured from video conferencing, one of \name's main target use cases.
These videos cover a range of spatial and temporal dynamics (\S\ref{app:siti})
and cover multiple resolutions, %(640$\times$360, 1280$\times$720 and 1920$\times$1280)
with at least 5 videos in each resolution. 
The performance is reported as an average across all the frames in the videos.



%\mypara{Baselines}
%We compare the performance of \name with multiple state-of-the-art real-time video techniques that use different combinations of video coding and congestion control algorithms: 
%\begin{packeditemize}
%\item {\em Reference:} H.26x with adaptive FEC and GCC
%\item {\em Salsify:}
%\item {\em Idealized SVC:}
%\end{packeditemize}



\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.245\linewidth}
         \centering
         %\includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
         %\includegraphics[width=\linewidth]{figs/placeholders/gcc-delay-results-queue25delay100.pdf}
         \includegraphics[width=4\linewidth]{figs/gccdelay-queue25-delay100-long.pdf}
         \caption{SSIM vs. delayed frame ratio, using GCC}
         \label{fig:normal-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/gcc-stall-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay100.pdf}
         \caption{SSIM vs. video stall ratio, using GCC}
         \label{fig:normal-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/saldelay-queue25-delay100.pdf}
         \caption{SSIM vs. delayed frame ratio, using Salsify-CC}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/salstall-queue25-delay100.pdf}
         \caption{SSIM vs. video stall ratio, using Salsify-CC}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
     % \vspace{-0.2cm}
     \tightcaption{End-to-end simulation result using one-way delay = 100ms and queue = 25 packets}
     \label{fig:normal-simulation}
\end{figure*}


\begin{comment}
% THIS IS FOR SIGCOMM SUBMISSION, JUST ONE FIGURE TO SHOW MULTIPLE DELAY AND QUEUE LENGTHS
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.245\linewidth}
         \centering
         %\includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
         % \includegraphics[width=\linewidth]{figs/placeholders/gcc-delay-results-queue15delay100.pdf}
         \includegraphics[width=4\linewidth]{figs/gccdelay-queue15-delay100-long.pdf}
         \caption{Queue = 15 packets}
         \label{fig:normal-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/gcc-stall-results-queue15delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccdelay-queue35-delay100.pdf}
         \caption{Queue = 35 packets}
         \label{fig:normal-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue15delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccdelay-queue25-delay50.pdf}
         \caption{One-way delay = 50 ms}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue15delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccdelay-queue25-delay150.pdf}
         \caption{One-way delay = 150 ms}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
     \vspace{-0.2cm}
     \tightcaption{End-to-end simulation result, varying queue length and one-way delay}
     \label{fig:queue15-simulation}
\end{figure*}
\end{comment}


\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.245\linewidth}
         \centering
         %\includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
         % \includegraphics[width=\linewidth]{figs/placeholders/gcc-delay-results-queue15delay100.pdf}
         \includegraphics[width=4\linewidth]{figs/gccdelay-queue15-delay100-long.pdf}
         \caption{SSIM vs. delayed frame ratio, using GCC}
         \label{fig:normal-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/gcc-stall-results-queue15delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue15-delay100.pdf}
         \caption{SSIM vs. video stall ratio, using GCC}
         \label{fig:normal-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue15delay100.pdf}
         \includegraphics[width=\linewidth]{figs/saldelay-queue15-delay100.pdf}
         \caption{SSIM vs. delayed frame ratio, using Salsify-CC}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue15delay100.pdf}
         \includegraphics[width=\linewidth]{figs/salstall-queue15-delay100.pdf}
         \caption{SSIM vs. video stall ratio, using Salsify-CC}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
     % \vspace{-0.2cm}
     \tightcaption{End-to-end simulation result using one-way delay = 100ms and queue = 15 packets}
     \label{fig:queue15-simulation}
\end{figure*}


\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.245\linewidth}
         \centering
         %\includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
         % \includegraphics[width=\linewidth]{figs/placeholders/gcc-delay-results-queue35delay100.pdf}
         \includegraphics[width=4\linewidth]{figs/gccdelay-queue35-delay100-long.pdf}
         \caption{SSIM vs. delayed frame ratio, using GCC}
         \label{fig:normal-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/gcc-stall-results-queue35delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue35-delay100.pdf}
         \caption{SSIM vs. video stall ratio, using GCC}
         \label{fig:normal-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue35delay100.pdf}
         \includegraphics[width=\linewidth]{figs/saldelay-queue35-delay100.pdf}
         \caption{SSIM vs. delayed frame ratio, using Salsify-CC}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue35delay100.pdf}
         \includegraphics[width=\linewidth]{figs/salstall-queue25-delay100.pdf}
         \caption{SSIM vs. video stall ratio, using Salsify-CC}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
     % \vspace{-0.2cm}
     \tightcaption{End-to-end simulation result using one-way delay = 100ms and queue = 35 packets}
     \label{fig:queue35-simulation}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.245\linewidth}
         \centering
         %\includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
         % \includegraphics[width=\linewidth]{figs/placeholders/gcc-delay-results-queue25delay50.pdf}
         \includegraphics[width=4\linewidth]{figs/gccdelay-queue25-delay50-long.pdf}
         \caption{SSIM vs. delayed frame ratio, using GCC}
         \label{fig:normal-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/gcc-stall-results-queue25delay50.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay50.pdf}
         \caption{SSIM vs. video stall ratio, using GCC}
         \label{fig:normal-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/saldelay-queue25-delay50.pdf}
         \caption{SSIM vs. delayed frame ratio, using Salsify-CC}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay50.pdf}
         \includegraphics[width=\linewidth]{figs/salstall-queue25-delay50.pdf}
         \caption{SSIM vs. video stall ratio, using Salsify-CC}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
     % \vspace{-0.2cm}
     \tightcaption{End-to-end simulation result using one-way delay = 50ms and queue = 25 packets}
     \label{fig:delay50-simulation}
\end{figure*}


% \begin{figure*}[t!]
%     \centering
%     \begin{subfigure}[t]{0.245\linewidth}
%          \centering
%          %\includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
%          % \includegraphics[width=\linewidth]{figs/placeholders/gcc-delay-results-queue25delay150.pdf}
%          \includegraphics[width=4\linewidth]{figs/gccdelay-queue25-delay50-long.pdf}
%          \caption{SSIM vs. delayed frame ratio, using GCC}
%          \label{fig:normal-psnr-delay}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.245\linewidth}
%          \centering
%          % \includegraphics[width=\linewidth]{figs/placeholders/gcc-stall-results-queue25delay150.pdf}
%          \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay50.pdf}
%          \caption{SSIM vs. video stall ratio, using GCC}
%          \label{fig:normal-ssim-delay}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.245\linewidth}
%          \centering
%          % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay150.pdf}
%          \includegraphics[width=\linewidth]{figs/saldelay-queue25-delay50.pdf}
%          \caption{SSIM vs. delayed frame ratio, using Salsify-CC}
%          \label{fig:normal-psnr-stall}
%      \end{subfigure}
%      \hfill
%       \begin{subfigure}[t]{0.245\linewidth}
%          \centering
%          % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay150.pdf}
%          \includegraphics[width=\linewidth]{figs/salstall-queue25-delay50.pdf}
%          \caption{SSIM vs. video stall ratio, using Salsify-CC}
%          \label{fig:normal-psnr-stall}
%      \end{subfigure}
%      \hfill
%      \vspace{-0.2cm}
%      \tightcaption{End-to-end simulation result using one-way delay = 150ms and queue = 25 packets \yihua{update the text (now the delay is 50 not 150)}}
%      \label{fig:delay150-simulation}
% \end{figure*}




\begin{figure}[t!]
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=2\linewidth]{figs/fcc-gccdelay-queue25-delay100-long.pdf}
         \caption{SSIM vs. delayed frame ratio, using FCC dataset}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/fcc-gccstall-queue25-delay100.pdf}
         \caption{SSIM vs. video stall ratio using FCC dataset}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \vspace{-0.1cm}
     \tightcaption{Results using FCC dataset}
     \label{fig:fcc-simulation}
\end{figure}


\begin{figure}[t!]
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=2\linewidth]{figs/abl-gccdelay-queue25-delay100-long.pdf}
         \caption{SSIM vs. delayed frame ratio, using different versions of \name}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/abl-gccstall-queue25-delay100.pdf}
         \caption{SSIM vs. video stall ratio, using different versions of \name}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     % \vspace{-0.1cm}
     \tightcaption{Ablation study (per packet EC, loss resilience) }
     \label{fig:simulation-ablation}
\end{figure}



\tightsubsection{Video quality vs. realtimeness and smoothness}
\label{subsec:eval:e2e}

We run \name and the baselines on real bandwidth traces from Verizon and T-Mobile LTE (\S\ref{subsec:eval:setup}). 
%We set propagation delay at default values (100ms) and a droptail queue length of 25 packets.
We implemented two different congestion control algorithms: Google congestion control~\cite{carlucci2016analysis} (\textit{GCC}, the standard congestion control used in WebRTC) and the congestion control from~\cite{salsify} (\textit{Sal-CC}). 
%We also implemented FEC-protected H.265 and Salsify codec as the baseline codecs (\S????????????????????????????????????????????????????????????\ref{subsec:eval:setup}).

Figure~\ref{fig:normal-simulation} compares \name with the baselines in average quality (SSIM) and the ratio of delayed frames and video stalls.
We see that \name significantly decreases both video delay and stall ratio. The ratio of delayed frames for \name is 0.8\% and 1.1\% when using GCC and Sal-CC respectively, while most of the baselines are ranging from 3.8\%-8.2\% and 4.2\%-8.8\%, respectively. 
% \name can also avoid all the video freezes under 200ms, while most of the baselines have a stall ratio ranged from 5\% to 18\%.
The major cause of frame delay and video stalls is congestion-induced packet loss. 
For instance, when there is a packet loss, the Salsify codec needs to skip frames, causing a delay increase, and H.265 needs to wait for those lost packets to be retransmitted, which competes with normal video traffic. 
SVC and Voxel must wait for retransmission if the base layer is damaged or it is an important frame. 
In contrast, \name can decode a frame if any packet of that frame arrived at the receiver side.
% , thus will not be impacted much by packet losses.


When under the same congestion control (Sal-CC or GCC), the average SSIM of \name, Salsify codec and H.265 are 13.8 dB, 14.3 dB and 14.5 dB respectively. SVC and Voxel have slightly lower SSIM, as packet losses will impose higher damage to them than \name. 
\edit{Despite error concealment techniques such as \name reducing frame delay and stall ratio, they fall short in quality when compared to \name. It's noteworthy that the machine-learning-based error concealment approach we employ already surpasses traditional methods, such as those implemented in H.264, in terms of reconstruction quality~\cite{zhou2010efficient, varsa2001non}. However, most machine-learning-based error concealment solutions, to the best of our knowledge, necessitate a minimum of several hundred milliseconds for error concealment, which is a duration incompatible with the latency requirements of real-time video streaming.}
%Although the error concealment technique can reduce frame delay and stall ratio as \name, its quality is much worse than \name. We also note that we are using a machine-learning-based error concealment technique that can already deliver better reconstruction quality than traditional error concealment implemented in H.264~\cite{zhou2010efficient, varsa2001non}. To our best knowledge, most machine-learning-based error concealment solutions require at least hundreds of milliseconds to conceal errors, which does not meet the latency requirement of real-time video streaming.
% : the SSIM is only 10.2 dB and 7.3 dB when using GCC and Sal-CC respectively.
Though \name's SSIM is on par or slightly lower than some baselines, we believe that the reduction in frame delay and stall ratio is worth the minor drop in quality, which is also confirmed by our user study (as we will show later).

\name also outperforms our prior work ({\em Grace-naive}) by having a higher SSIM. This improvement is due to \name's efficient per-packet entropy coding approach, which results in significantly less size overhead compared to prior methods. Moreover, \name's state re-sync protocol (\S\ref{subsec:protocol}) effectively curbs error propagation caused by packet losses.


% \yihua{check if we already mentioned congestion control before}
%We play a \fillme-second long video on \fillme cellular network traces~\cite{??} and set the propagation delay at \fillme ms and queue length at \fillme. 
%\jc{YIHUA, please fill in some detailed reading}

%\jc{
%\begin{itemize}
%    \item by trace set
%    \item by rtt
%    \item by queue length
%    \item a concrete example
%\end{itemize}
%}

% \mypara{Impact of queue and delay} 
% We then test \name's performance on the same traces but under different queue lengths and different propagation delays.
Figure~\ref{fig:queue15-simulation} to Figure~\ref{fig:delay50-simulation} shows that \name consistently reduces the ratio of delayed frames in different network delays or drop-tail queue lengths. 
\name has more delay reduction when the queue is shorter or the network delay is larger. 
This is because, during congestion, shorter queues tend to drop previous frames packets more aggressively, and might still delivery {\em some} packets (though not all) of the latest frame to the receiver. 
\name lets the client decode the frame early based on any subset of packets it has received. 
% And longer delay will increase the latency of packet loss feedback, causing a longer delay for baselines to recover from packet losses.


    


% \mypara{Impact of bandwidth distributions}
We also run the simulation based on the broadband traces from FCC dataset~\cite{fcc-dataset}. Compared to the LTE traces, broadband traces have similar average bandwidth but fewer bandwidth drops. We run the simulation with the default setting (a propagation delay of 100ms and a droptail queue of 25 packets) and use GCC as the congestion control algorithm. 
Figure~\ref{fig:fcc-simulation} shows that \name still has a better trade-off between video quality and the ratio of delayed frames and video freezes than the baselines. 

% \mypara{Ablation study of key components} 
% We then conduct an ablation study by removing per-packet entropy coding (\S\ref{??}) and loss-resilience training (\S\ref{??}). 
% We run the experiment using Sal-CC with the same one-way delay and queue length as in Figure~\ref{fig:normal-simulation}. 

Moreover, Figure~\ref{fig:simulation-ablation} shows that both the delayed frame ratio and the stall ratio will increase if \name does not use per-packet entropy coding described in \S\ref{subsec:packetization} (the red cross). 
This is because, without it, the size of the encoded frame will have an increase of 1.5$\times$, and this size increase may overload the network when bandwidth suddenly drops. 

We also evaluate the impact of the optimizations proposed in~\S\ref{subsec:fast-coding} for speeding up CPU encoding/decoding. As shown in Figure~\ref{fig:simulation-ablation}, the average SSIM decreased from 13.8 to 13.4 after applying the CPU-related optimizations, and the optimizations do not affect the realtimeness and smoothness of the decoded video.

Finally, we compare \name and the baselines in a concrete bandwidth trace sample (Figure~\ref{fig:timeseries-ours}).
The bandwidth drops from 8Mbps to 2Mbps at 1.5sec and last for 800ms, before bouncing back to 8Mbps (another bandwidth drop occurs at 3.5sec).
We can see that during each bandwidth drop, \name's delay does not increase as sharply as the baselines (notably Salsify is the second best since it could skip frames).
\name and Salsify use the same CC, so their quality roughly matches on frames not skipped by Salsify.
That said, \name's quality degrades marginally with no frame skipping during congestion, and it bounces back once packet losses disappear. 




% When we run \name with the models trained without any packet losses, the average SSIM will be decreased from \fillme dB to \fillme dB. This is because the frame quality will be significantly decreased when packet loss happens.


\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    \includegraphics[width=1.05\linewidth]{figs/timeseries-new.pdf}
    \tightcaption{\name achieves lower delay and decent quality during sudden bandwidth drops.}
    \label{fig:timeseries-ours}
\end{figure}

\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    \includegraphics[width=0.8\linewidth]{figs/user-study.pdf}
    \tightcaption{Comparing \name with Salsify and H.265 by user study}
    \label{fig:user-study}
\end{figure}


\mypara{User study of video quality} 
% To show decreasing the ratio of delayed frames and video freezes is worth the minor drop in quality for real users, 
To validate \name's improvement, we set up a real user study on Amazon MTurk~\cite{mturk} (IRB approved). 
We sampled 8 video clips (spanning cloud gaming, real-time sports events, and indoor activities) rendered by \name, Salsify codec and H.265 using {\em GCC} as congestion control while using the same setup as Figure~\ref{fig:normal-simulation}. 
We confirm the sampled video clips have the same distribution of quality, the ratio of delayed frames and video freezes as Figure~\ref{fig:normal-simulation}. 
% , and the user study is properly randomized following the steps described in \cite{sensei}.
When an MTurk user is signed up for the user study, the user will be randomly assigned to rate their user experience (with a Likert scale of 1-5) on the videos rendered by different methods. 
Figure~\ref{fig:user-study} shows the average rating (\ie, mean opinion score or MOS) among 750 users on the videos from each method. It shows that \name can improve the MOS from 2-2.5 to 3.8-4.7. 



\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/ssim-bpp-k360.pdf}
        \tightcaption{SSIM vs. bit per pixel for Kinetics dataset, 360P videos}
        \label{fig:}
        % \vspace*{3mm}

    \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/psnr-bpp-k360.pdf}
    %     \tightcaption{PSNR vs. bit per pixel for Kinetics dataset 360P videos}
    %     \label{fig:}
    % \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/ssim-bpp-k720.pdf}
        \tightcaption{SSIM vs. bit per pixel for Kinetics dataset 720P videos}
        \label{fig:}

    \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/psnr-bpp-k720.pdf}
    %     \tightcaption{PSNR vs. bit per pixel for Kinetics dataset 720P videos}
    %     \label{fig:}
    % \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
        \vspace*{3mm}

        \includegraphics[width=\linewidth]{figs/ssim-bpp-fvc.pdf}
        \tightcaption{SSIM vs. bit per pixel for FVC dataset}
        \label{fig:}
    \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/psnr-bpp-fvc.pdf}
    %     \tightcaption{PSNR vs. bit per pixel for FVC dataset}
    %     \label{fig:}
    % \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/ssim-bpp-uvg.pdf}
        \tightcaption{SSIM vs. bit per pixel for UVG dataset}
        \label{fig:}
    \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/psnr-bpp-uvg.pdf}
    %     \tightcaption{PSNR vs. bit per pixel for UVG dataset}
    %     \label{fig:}
    % \end{subfigure}
    \vspace*{4mm}

    \tightcaption{Quality-size tradeoff of \name.}
    \label{fig:psnr-vs-bpp}
\end{figure}


\begin{figure}[t!]
     % \begin{subfigure}[b]{0.48\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figs/ssim-loss-0.05.pdf}
     %     \caption{Bpp = 0.05}
     %     \label{fig:queue15-psnr-stall}
     % \end{subfigure}
     % \hfill
     % \begin{subfigure}[b]{0.48\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figs/ssim-loss-0.1.pdf}
     %     \caption{Bpp = 0.1}
     %     \label{fig:queue15-ssim-delay}
     % \end{subfigure}
     % \hfill
     %    \begin{subfigure}[b]{0.48\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figs/ssim-loss-0.2.pdf}
     %     \caption{Bpp = 0.2}
     %     \label{fig:queue15-psnr-stall}
     % \end{subfigure}
     % \hfill
     % \begin{subfigure}[b]{0.48\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figs/ssim-loss-0.3.pdf}
     %     \caption{Bpp = 0.3}
     %     \label{fig:queue15-ssim-delay}
     % \end{subfigure}
     % \hfill
     % \vspace{-0.1cm}
     \centering
     \includegraphics[width=1.07\linewidth]{figs/ssim-loss-v2.pdf}
     \tightcaption{\name's loss resilience for different BPPs and different number of lossy frames}
     \label{fig:loss_by_bitrate}
\end{figure}


\tightsubsection{Coding efficiency and loss resilience}
\label{subsec:eval:resilience}

\mypara{Coding efficiency of \name} 
% For any loss-resilient schemes, 
There is always a tradeoff between compression and loss resilience, and \name is no exception.
% The ability to tolerate packet losses often comes with a drop in quality in absence of packet losses, and \name is no exception. 
Figure~\ref{fig:psnr-vs-bpp} compares the \name's quality under no packet loss with that of H.264 and H.265 across the test videos from Table~\ref{tab:dataset} (all of which are different from the training set).
Following the previous works, we use {\em bit per pixel} (BPP) to measure size.
Figure~\ref{fig:psnr-vs-bpp} shows that \name is similar to H.264 and is only slightly worse than H.265.
It also shows that \name can cover a wide range of BPPs among all datasets, from 0.03 to 0.5. 
% This enables more flexible bitrate adaptation when running \name.

\begin{comment}

Remember that H.26x uses the zerolatency option and fast preset (which is typical to real-time videos, including WebRTC\footnote{Google's WebRTC~\cite{WEBRTCSRC} uses OpenH264~\cite{OPENH264}. They set the runtime parameter "usageType" to CAMERA\_VIDEO\_REAL\_TIME  (similar to zerolatency) and "complexityMode" to LOW\_COMPLEXITY (similar to fast)}. 
We confirm that without these settings, H.265's coding efficiency is better than \name in the absence of packet losses.
However, our goal is a data-scalable autoencoder for real-time videos (shown shortly) rather than an autoencoder that outperforms heavily engineered H.26x codecs. 
Moreover, the coding efficiency of the autoencoder could still be improved (\eg our autoencoder estimates motion vectors based only on one reference frame).

\end{comment}

\mypara{Loss resilience of \name}
Figure~\ref{fig:loss_by_bitrate} compares \name with the baseline codecs under different packet loss rates. \edit{We apply packet losses for $N$ consecutive frames and calculated the decoded quality of the lossy frames. Figure~\ref{fig:loss_by_bitrate} shows the result when $N=1,3,5$.}
% when encoding videos from Table~???\ref{tab:dataset}.
In each figure, all lines have almost the same encoding BPP with differences controlled within 5\%.
We ensure that \name's encoded BPP is {\em never} higher than the baselines, so even if the actual encoded BPP is different, it does not favor \name. Figure~\ref{fig:decoded-example} in Appendix~\ref{app:visualization} shows an example to visualize the behavior of \name under packet loss.

The most salient feature of \name is the graceful quality degradation with more packet losses. 
The average SSIM drop is only 1 dB to 3 dB under 20\% and 50\% packet losses among all the BPPs. 
Even when the loss ratio is as high as 80\%, \name can still have an average SSIM of 12 dB across different BPPs, which is much better than H.264 with various FEC redundancy rates, and SVC for the reasons elaborated in \S\ref{subsec:eval:e2e}.

We further contrast \name with alternative decoder-side error concealment baselines, encompassing a pretrained autoencoder~\cite{dvc}, \name with an untrained encoder neural network, and a machine-learning-based error concealment solution (\S\ref{subsec:eval:setup}). \name consistently surpasses these baselines, a result attributable to its joint encoder-decoder training process that facilitates the introduction of redundancy into the encoded byte stream. Conversely, other decoder-side error concealment baselines lack this redundancy in the encoder's output.

\edit{In real-world scenarios, packet loss typically affects not merely a single frame, but a series of consecutive frames~\cite{rudow2023tambur}. Figure~\ref{fig:loss_by_bitrate}c and~\ref{fig:loss_by_bitrate}d shows the performance of \name and the baselines when packet losses occur across 3 and 5 consecutive frames. When compared to other baselines, \name is capable of achieving a higher SSIM, up to 2, covering different loss rates between 10\% and 80\%. We have excluded FEC and SVC from Figure~\ref{fig:loss_by_bitrate}c and~\ref{fig:loss_by_bitrate}d, as it becomes inconsequential to compute the quality of subsequent frames if preceding ones are undecodable.}



\begin{comment}
    
Compared with H.264 with fixed FEC protection, \name can have a higher SSIM of 1.1 dB to 1.9 dB among different resolutions and different BPPs when there is no loss. 
This is because any arrived bytes in \name contribute to the quality while in FEC, the redundant data is useless even if they do arrive at the decoder. 
On the other hand, FEC-based loss resiliency is also in a dilemma that a low FEC rate cannot protect against the high loss, but a high FEC rate leads to poor quality when the packet loss ratio is small. 
Our \name solves this dilemma by graceful quality degradation.

Compared to the error concealment baseline, \name's quality decreases more gracefully when the loss rate increases. This is because when the loss rate is high (\eg larger than 50\%), the error concealment baseline can hardly recover the motion vectors, which causes a fast quality degradation. However, \name's encoder learns to encode the frame with some redundancy, such that it can still recover some of the lost data from the received packets.

\name is also better than SVC with unequal FEC protection (\S??????????????????????????????????????????\ref{subsec:prior}). 
The quality of SVC decreases quickly when the loss rate is small, as the high-quality layers are unlikely to be decodable in such cases. 
We also note that the pre-trained autoencoder models, which have not seen any losses in training, degrade poorly with higher loss rates. 


\end{comment}


\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/burst-loss.pdf}
         \caption{50\% of packet loss is applied to frame 6, 7, 8}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/long-loss.pdf}
         \caption{10\%, 30\%, 50\% packet loss is applied on {\em every} frame after 6-th frame}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
    \tightcaption{The detailed behavior of \name under different kind of losses.}
    \label{fig:loss-behavior}
\end{figure}

% We conduct a detailed analysis of \name under different kinds of packet losses
Figure~\ref{fig:loss-behavior} shows that if there is a transient packet loss, the quality of the following frames will not keep degrading. When the packet losses are persistent, \name can still deliver good quality for more than 10 frames, without needing any synchronization between the encoder and the receiver.

%\jc{
%\begin{itemize}
%    \item by bitrate
%    \item by video set
%    \item psnr vs. bitrate
%\end{itemize}
%}

% \jc{need a footnote to explain why intra-mb insertion is so bad}



 

%In Figure~???????????????????????????\ref{??}, we use three metrics for video quality, even though our autoencoders are trained to optimize L2-norm between the reconstructed and original images, which is similar to RGB-PSNR, their quality compared to baselines is similar under different metrics.

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_traceset_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_rtt_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_queue_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}


%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=1.pdf}
%    \caption{Aggressiveness = 1}
%    \label{fig:}
%\end{figure*}
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=0.75.pdf}
%    \caption{Aggressiveness = 5}
%    \label{fig:}
%\end{figure*}








% \jc{YIHUA, please fill in some detailed reading}

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/encoding-lat-gpu.pdf}
%          \caption{Encoding latency on A100 GPU}
%          \label{fig:gpu-encoding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/encoding-lat-cpu.pdf}
%          \caption{Encoding latency on CPU}
%          \label{fig:gpu-decoding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/decoding-lat-gpu.pdf}
%          \caption{Decoding latency on A100 GPU}
%          \label{fig:cpu-encoding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/decoding-lat-cpu.pdf}
%          \caption{Decoding latency on CPU}
%          \label{fig:cpu-decoding}
%      \end{subfigure}
%      \hfill
%      \tightcaption{Compute overhead of \name.}
%      \label{fig:computing-overhead}
% \end{figure} 

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/encoding-lat-gpu-new.pdf}
         \caption{Encoding latency on A100 GPU}
         \label{fig:gpu-encoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/encoding-lat-copies-gpu-new.pdf}
         \caption{Total latency to encode multiple copies of different bitrates}
         \label{fig:gpu-multi-encoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/encoding-lat-cpu-new.pdf}
         \caption{Encoding latency on CPU}
         \label{fig:gpu-decoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/decoding-lat-gpu-new.pdf}
         \caption{Decoding latency on A100 GPU}
         \label{fig:cpu-encoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/decoding-lat-cpu-new.pdf}
         \caption{Decoding latency on CPU}
         \label{fig:cpu-decoding}
     \end{subfigure}
     \hfill
     \tightcaption{Compute overhead of \name.}
     \label{fig:computing-overhead}
\end{figure*} 

% \begin{figure}[t!]
%      \begin{subfigure}[b]{0.48\linewidth}
%          \centering
%          \includegraphics[width=2\linewidth]{figs/cpu-gccdelay-queue25-delay100-long.pdf}
%          \caption{SSIM vs. delayed frame ratio}
%          \label{fig:queue15-psnr-stall}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.48\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/cpu-gccstall-queue25-delay100.pdf}
%          \caption{SSIM vs. video stall ratio}s
%          \label{fig:queue15-ssim-delay}
%      \end{subfigure}
%      \hfill
%      \vspace{-0.1cm}
%      \tightcaption{End-to-end simulation results for CPU version \name \zy{missing legend for the black dot}}
%      \label{fig:simulation-ablation}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%          \centering
%         %\includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
%         \includegraphics[width=0.7\linewidth]{figs/cpu e2e.pdf}
%          \label{fig:}
%          \vspace{.05cm}
%     \tightcaption{CPU end to end result. \textcolor{red}{TODO: Ziyi and Hanchen}}
%     \label{fig:cpu-simulation}
% \end{figure}

\tightsubsection{Microbenchmarking results}
\label{subsec:eval:system}

% \zy{There is a typo ("decodeing latency") on the y-axis label on Figure 16 (b). (figs/decode.pdf)}

% Remember that \name needs a P-frame encoder and a I-frame encoder to encode each frame as a P-frame and an I-patch (a small spatial region without reference).
\mypara{Computational overhead}
% We test the encoding/decoding speed of un-optimized \name, optimized \name (\S\ref{subsec:fast-coding}) and H.264 from \texttt{ffmpeg} on a Linux server with an A100 GPU and Intel Xeon Silver 4210R CPU (32 threads).
% Figure~\ref{fig:gpu-encoding} and Figure~\ref{fig:gpu-decoding} show the encoding and decoding speed on GPU. With the optimizations, \name can encode and decode a 720P frame in 34.9ms and 15.5ms respectively, which is 1.5$\times$ and 2$\times$ faster than the unoptimized version. This translates to 28fps and 35fps for encoding and decoding 720P frames. 
% For 480P videos, optimized \name can encode/decode in 25.3 and 15.4ms, which equals to 40fps and 65fps for encoding and decoding.
We conducted encoding/decoding speed tests on {\em Grace-naive},  \name (\S\ref{subsec:fast-coding}), and H.264 from \texttt{ffmpeg} on a Linux server equipped with an A100 GPU and Intel Xeon Silver 4210R CPU (32 threads). The results, presented in Figure~\ref{fig:gpu-encoding} and 
Figure~\ref{fig:gpu-decoding}, illustrate the GPU encoding and decoding speed. Following optimizations, \name was capable of encoding and decoding a 720P frame in 34.9ms and 15.5ms, respectively, marking an improvement of 1.5$\times$ and 2$\times$ over our prior work. This equates to frame rates of 28fps and 35fps for encoding and decoding 720P frames, respectively. Also, the overhead for \name to encode a new copy for bitrate adaptation is negligible. As shown in Figure~\ref{fig:gpu-multi-encoding}, it only takes 2.1ms for \name to encode a new copy of a different bitrate, while Grace-naive needs more than 10ms to do the same thing.

% Figure~\ref{fig:cpu-encoding} and Figure~\ref{fig:cpu-decoding} shows our optimizations on CPU can significantly reduce the encoding and decoding time. For 720P videos, the original model takes 5217ms and 3996ms to encode and decode a frame, while the time decreases to 35.1ms and 40.9ms after applying our optimizations. This shows that with our optimization, \name is able to stream the 720P video purely using CPU.
% Compared with the GPU version of \name, the optimized CPU version has a lower SSIM of 0.8 dB. However, it does not impact the improvement in the ratio of delayed frames. %, and the quality is not bad compared to the error concealment baseline.

As illustrated in Figure~\ref{fig:cpu-encoding} and Figure~\ref{fig:cpu-decoding}, our CPU optimizations significantly curtail encoding and decoding times. For 720P videos, the initial model necessitated 5217ms and 3996ms to encode and decode a frame, respectively; however, these times were dramatically reduced to 35.1ms and 40.9ms following our optimization. This demonstrates that \name, with our optimization, is capable of streaming 720P video using the CPU alone. Despite the optimized CPU version of \name exhibiting a marginally lower SSIM of 0.8 dB compared to its GPU counterpart, this discrepancy does not compromise the improvement in the ratio of delayed frames.

% \begin{figure}[t!]
%     \centering
%          \centering
%         %\includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
%         \includegraphics[width=0.7\linewidth]{figs/encoding-multiple-version.png}
%          \label{fig:system-encoding-versions}
%          \vspace{.05cm}
%     \tightcaption{Encoding latency of encoding multiple versions \textcolor{red}{TODO: Yihua}}
%     \label{fig:multiple-encoding}
% \end{figure}

\mypara{Bitrate adaptation}
Figure~\ref{fig:gpu-encoding} also depicts the latency incurred by \name while encoding multiple frame copies at varying bitrates (\S\ref{subsec:fast-coding}). Given that the most time-intensive portion of encoding is shared across models, the additional time required to encode multiple versions is minimal, averaging merely 2.6ms per extra copy. Consequently, \name is capable of encoding three distinct copies within 40.9ms, thus facilitating real-time bitrate adaptation by the encoder. Our empirical observations reveal that over 65\% of frames require a single encoding pass, while 34\% necessitate a second pass to adjust to the target bitrate. A marginal subset, less than 1\%, is subjected to a third encoding pass.

% Figure~\ref{fig:gpu-encoding} shows the encoding latency for \name to encode multiple different copies of frames with different bitrates (\S\ref{subsec:fast-coding}). Since the models share the most time-consuming part of the encoding, the overhead of encoding multiple versions is negligible: only 2.6ms for every extra copy. Therefore, \name can encode 3 different copies in 40.9ms, allowing the encoder to do bitrate adaptation in real-time.
% Empirically in our study, over 65\% frames will only be encoded once and 34\% frames will be encoded twice to adapt to the target bitrate. Less than 1\% frames will be encoded 3 times. 
% Figure~\ref{??} shows the effectiveness of our bitrate controlling algorithm (\S\ref{??}). Over \fillme\% of frames will falls in the range of $[0.8, 1]\times$ target bitrate and it will never produce a frame that overshoots the target bitrate.

% \mypara{Model training decisions}
% To validate the design choices of loss distribution we used during model training, we conduct an ablation study of different loss distributions. We test two different setups: (i) the probability of using 0 loss is the same as other loss rates, and (ii) loss rates as high as 80\% and 90\% are added during training. As shown in Figure~???\ref{fig:training-loss-study}, both setups can cause the SSIM under 0 loss decrease around \fillme dB. 
% When the probability of 0 loss is low, the model will learn to deprioritize the quality under 0 loss, which will impact the average video quality. We also observe that seeing a loss as high as 80\% or 90\% will also damage the quality under 0 loss.


% Our implementation of \name optimizes both memory footprint and encoding/decoding delay (described in \S???\ref{subsec:optimize}), and we test its effectiveness on a Nvidia GeForce RTX 3080 GPU. 
% Figure~???\ref{fig:system-encoding} and Figure~???\ref{fig:system-decoding} show that compared to the original (unoptimized) implementation of pre-trained autoencoder (which takes 100ms to encode a 480p frame), our implementation can encode a 480p frame in less than 25ms (a 4×4\times speedup).\footnote{The only autoencoder that achieves comparable encoding/decoding speed is~\cite{elf}, and it achieves such speed on a 5x more expensive Titan V GPU. We hope to compare it with \name, but it is not open-source.}
% This translates to almost 40fps. 
% Even for 720p HD videos, our optimized codec can achieve 18fps (55ms encoding per frame). 
% % \fillme~fps/\fillme~fps, \name encodes/decodes 480p frames at \fillme~fps/\fillme~fps, a \fillme×\times speedup.
% This acceleration comes from downsampling frames in motion-vector estimation. 
% Moreover, when adapting to a target bitrate, \name encodes the next frame multiple times {\em without} needing to run the entire encoder multiple times, because it re-uses the motion-compensated prediction, so only the residuals need to be encoded at multiple bitrates. Figure~??????\ref{fig:system-encoding-versions} shows that the delay of encoding a frame at three different bitrates only increases marginally compared to encoding one frame. 







% In terms of memory usage, our optimized implementation saves the memory footprint of loading 9 models by over 60\% since most NN layers are shared. 
% % Figure~??????\ref{??} shows that compared to loading the multiple autoencoders (I-frame encoder/decoder and a P-frame encoder/decoder of each bitrate) in GPU memory, the memory usage \name's autoencoders (not including the memory usage of intermediate features) is \fillme\% smaller, because they share most of the layers (only the last \fillme layers of the encoder and the first \fillme layers of the decoders are different). 
% Note that \name does not change the NN architecture of the autoencoders---only the weights are retrained and the way they are used is optimized. We speculate that they could be made more efficient with appropriate modification to its NN architecture.

% Figure~??????\ref{??} validate that \name's coding efficiency is comparable to (even slightly better than) without the optimizations (\ie without sharing the NN backbone or downsampling and sharing the motion-vectors.)
% This is because, though quality does drop with these optimizations, the encoded size also drops (due largely to the downsampled motion vectors), which result in a similar bitrate-quality trade-off frontier.

% \jc{The only autoencoder that achieves comparable encoding/decoding speed is Elf~\cite{??}. 
% We hope to compare it with \name, but it is not open-source. }


% \jc{remember to highlight that the speed is comparable to elf, which runs on the 5x more expensive titan v gpu.}

% \begin{figure}[t!]
%     \centering
%          \centering
%         \includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
% %        \includegraphics[width=0.7\linewidth]{figs/a.pdf}
%          \label{fig:}
%          \vspace{.05cm}
%     \tightcaption{Training curve study \textcolor{red}{put into appendix}}
%     \label{fig:training-loss-study}
% \end{figure}
%!TEX root = ../main.tex
%!TEX spellcheck = en_US



==> sections/old/eval_v6.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Evaluation}
\label{sec:eval}

The findings of our evaluation can be summarized as follows:
\begin{packeditemize}
\item {\bf Quality-delay tradeoff:} Under bandwidth fluctuations in real network traces, \name has significantly fewer video stalls (video freezes for over 200ms) compared to other loss-resilient schemes, in terms of both frequency of stalls and total stall duration.
Also, \name reduces the tail frame delay and ratio of non-rendered frames.
Our user study has also confirmed that \name is rated more favorably than baselines.

\item {\bf Loss resilience:} Though \name's quality under no packet loss is on par with H.264 and H.265, it is data-scalable---graceful quality degradation with higher loss rate---under various videos and bitrates. 

\item {\bf Overhead:} Our implementation of \name can encode/decode 480p video at 40~fps/65~fps and 720p HD video at 28~fps/35~fps using \fillme GPU, a 1.5-2$\times$ speedup compared to off-the-shelf autoencoders. With the optimization for CPU (\S\ref{subsec:fast-coding}), \name can also encode/decode 720p HD video at 27~fps/25~fps on CPU without causing huge quality degredation.
\end{packeditemize}


\tightsubsection{Setup}
\label{subsec:eval:setup}

\mypara{Training of \name}
We build \name's autoencoder based on DVC~\cite{dvc}, a state-of-the-art video autoencoder. Figure~\ref{fig:dvc-arch} shows the architecture of the encoder and decoder. On the sender side, the encoder neural network takes the current frame and its reference frame as the input, and outputs the encoded motion vectors and residuals (\S\ref{subsec:background}). On the receiver side, the decoder neural network decodes the received motion vector and residuals, then reconstructs the new frame based on the reference frame.

We fine-tuned the \name autoencoder using the DVC model from~\cite{dvc} and trained it on the vimeo-90K~\cite{vimeo-dataset} dataset. We employed 11 distinct $\alpha$s (in Eq.~\ref{eq:2}), ranging from $1/64$ to $1/32768$. This enables the model to support various bitrates (\S\ref{subsec:fast-coding}). 
We set the learning rate at $10^{-4}$, and fine-tuning typically takes 1-2 hours on an Nvidia A40 GPU.
\jc{need to add more training details and model arch}

\mypara{Baselines}
%\yihua{update text: rewrite baseline implementation}
We implemented the following loss-resilient baselines using H.265 and H.264 of \texttt{ffmpeg} (version 4.2.7). The baselines are covering the following design choices (\S\ref{subsec:prior}) for loss-resilient video coding:
\begin{packeditemize}
  \item {\bf Error correction coding}: The most common loss resilient design choice in real-time video is to add forward error correction (FEC), including rateless coding~\cite{castura2006rateless} and streaming code~\cite{badr2017fec}. We implement Tambur~\cite{rudow2023tambur} with H.265, a state-of-the-art forward error correction solution using streaming code. Tambur performs better than the default FEC scheme used in WebRTC since it can decrease the number of non-decodable frames when sending the same amount of parity packets. 
  
  Following recent work in real-time video coding~\cite{ZEROLAT1,ffmpegstreaming}, we use the \texttt{zerolatency} option (no B-frames) and the \texttt{fast} preset of H.265\footnote{The command line we used to encode a video is \texttt{ffmpeg -y -i Video.y4m -c:v libx265 -preset fast -tune zerolatency -x265-params "crf=Q:keyint=3000" output.mp4} where {\em Q} controls the quality of the frame.} , and we do not restrict their GoP (I-frame interval). 
  We set Tambur's latency deadline $\tau$ to 3 frames, and the number of parity packets is determined dynamically by the packet loss rate in last 2 seconds, following the logic in Google's WebRTC implementation~\cite{WEBRTCSRC}.

    
  \item {\bf Error concealment}: Error concealment recovers quality from the packet loss by predicting the missing content using hand-tune heuristics~\cite{zhou2010efficient, varsa2001non} or neural networks~\cite{kang2022error, sankisa2018video, mathieu2015deep}. Error concealment methods need to work with per-packet entropy coding techniques such as flexible macroblock ordering~\cite{KUMAR2006425} because it requires an incomplete frame to be decodable. We use a state-of-the-art machine-learning-based error concealment method~\cite{kang2022error} with \fillme as the per-packet entropy coding technique.

  The baseline encodes/decodes the video using H.265. When there is an incomplete frame, the baseline takes 3 steps to conceal the errors. It will first use a neural network to estimate the motion vector of the missing part based on previous frames. Then, it will propagate the missing pixel values from the reference frame with the estimated motion vector. Finally, it will use an inpainting neural network to improve the frame quality and reduce error propagation. It is better than motion-prediction-only or inpainting-only error concealment methods (\cite{sankisa2018video, mathieu2015deep}). We also assume a \fillme\% size overhead caused by the per-packet entropy coding, which matches the overhead mentioned in~\cite{??}.
  
  \item {\bf Scalable video coding (SVC)}: SVC encodes a video at multiple quality layers and sends data layer by layer. We implement an idealized SVC, such that when the first $\times$ layers arrive, it will reach a quality the same as that of H.265 at receiving the same amount of bytes. This idealized SVC implementation is already better than the state-of-the-art SVC~\cite{swift}.
  By default, we also add 50\% FEC to protect the base layer for SVC, as it is also a common practice in real-time videos~\cite{???}.
  


  
  \item {\bf Selective frame skipping}: Another design choice for loss-resilient real-time video is to only retransmit the important missing packet that will cause huge damage to the video quality. We implement a baseline for this design choice based on Voxel~\cite{voxel}, a prior work using selective frame skipping to reduce the video rebuffering ratio and improve the user's QoE.

  We sort the video frames by the SSIM drop caused by skipping the frame\footnote{In real-time video communication, we usually cannot get the quality drop caused by skipping frames in advance. We are making an idealized assumption that cheating for our baseline.}. For 25\% frames with the lowest SSIM drop, we use the default error concealment method in H.264/AVC~\cite{zhou2010efficient} without any packet retransmission, and for the remaining frames (which cause more SSIM drops when skipped), we retransmit all the lost packets. 
  We use a GoP (chunk length) of 4 seconds, which is also used by Voxel.
  
  \item {\bf Functional codec}: Unlike traditional codecs (\eg, H.265 or VP9), functional codecs are able to skip incomplete frames when packet loss happens and decode the first complete frame without a significant quality drop. Salsify~\cite{salsify} is a recent work implementing the functional codec. 
  
  We implement the Salsify baseline based on H.265 with the following functional codec features: {\em (i)} the encoded frame size of the codec will never overshoot the target bitrate calculated by the underlying congestion control algorithm, and {\em (ii)} when packet loss happens, the encoder can dynamically choose a reference frame to make later frames decodable without retransmitting any packets.

  \item {\bf Super-resolution (SR)}: SR technique is widely employed to enhance the video quality at the receiver side~\cite{livenas, swinir}. It is worth noting that since SR should work for any video codec, it is {\em orthogonal} to \name's design space. We use a state-of-the-art SR model, SwinIR~\cite{swinir}, as the tool to improve the video quality for both \name and other baselines after the receiver successfully decodes the frame. 

\end{packeditemize}

For the baselines of Salsify (functional codec), SVC, and Voxel (selective frame skipping), we make an idealized assumption that on each frame, the output bitrate of the codec perfectly matches the target bitrate chosen by the congestion control algorithm (explained in \S\ref{subsec:eval:e2e}), \ie never overshooting or undershooting, but the actual quality matches that of the highest \texttt{qp} that leads to a frame greater than the target bitrate. 
To err on the side of caution, these optimizations make the baselines' performance slightly better.
% In other words, their performance is higher than it would actually be in the real world.

% \yihua{need to emphasis that we are cheating for error concealment and Voxel. 1. assume perfectly match the target bitrate, 2. idealized per packet ec for h264 }

% Our baseline codecs include H.265 and H.264. 
% We use their implementations in \texttt{ffmpeg} (version 4.2.7). 
% Importantly, we do not restrict their GoP (I-frame interval) and the number of history frames to search for reference macroblocks. 
% Following recent work in real-time video coding~\cite{ZEROLAT1,ZEROLAT2}, we use the \texttt{zerolatency} option (no B-frames) and the \texttt{fast} preset of H.265\footnote{The command line we used to encode a video is \texttt{ffmpeg -y -i Video.y4m -c:v libx265 -preset fast -tune zerolatency -x265-params "crf=Q:keyint=3000" output.mp4} where {\em Q} controls the quality and size of the output video}.

% We use implementations for SVC, Salsify, and FEC, based on H.265.
% We simplify the implementation in a way that makes their quality slightly better than they would actually do. 
% Our implementation of SVC assumes that each quality level exactly {\em matches} the quality and size of the non-SVC coding of H.265, whereas even the state-of-the-art SVC (based also on autoencoders~\cite{swift}) achieves lower quality than H.265 at a quality level of the same frame size. (This effectively is an idealized version of Swift~\cite{swift}.)
% We follow Salsify's logic for congestion control, frame skipping, and packet pacing, but instead of using Salsify's multi-trial encoding to approximate the target bitrate of each frame, we assume that the encoded frame size exactly {\em matches} each frame's target bitrate but the quality matches the {\em qp} value whose bitrate is barely {\em higher} than the target bitrate.
% For FEC-protected H.26x, we use the same loss-rate prediction logic implemented in the public release of WebRTC~\cite{WEBRTCSRC} but remove the upper-bound of 50\% redundancy rate that is used in WebRTC \eg if the predicted packet loss rate is 60\%, we assume FEC will tolerate any packet loss ratio under 60\%.) %but instead of mapping it to the coarse-grained FEC redundancy rates, we assume an idealized FEC that can reconstruct a frame if the actual loss rate matches the predicted loss rate (\eg if the predicted packet loss rate is 50\%, we assume FEC will exactly tolerate 50\% packet loss.)
%This effectively approximates the situation where data can be packetized infinitesimally.
% While these simplifying assumptions lead to a slightly optimistic estimate of the baselines' performance, we hope they make our results more relevant in the long run, as the implementations of SVC, and bitrate control, and FEC might evolve and improve in the future.

\mypara{Testbed setup}
To compare \name and the baselines, we run them on a packet-level network simulator. 
The simulator uses a drop tail queue with a configurable queue length to simulate packet losses caused by the congestion. It implements the token bucket algorithm to simulate the bandwidth variation at a frequency of 0.1 seconds.
To determine the target bitrate of the video codecs used during simulation, we implemented two different congestion control algorithms: Google congestion control~\cite{carlucci2016analysis} (\textit{GCC}, the standard congestion control used in WebRTC) and the congestion control from~\cite{salsify} (\textit{Sal-CC}). 
During the runtime, the simulator takes as input a bandwidth trace and a video and simulates the {\em end-to-end} real-time video communication process, including encoding, packetization, sending rate adaptation, packet transmission, and decoding. The output of the simulator includes a decoded video and the end-to-end delay of each decoded frame (including the time used for encoding and decoding). We also validated that the frame delay produced by our simulator is accurate by running a real-world validation experiment (in \S\ref{subsec:eval:e2e}).

The simulator runs on an Ubuntu 18.04 server with 2 Intel Xeon 4210R CPU, and 256GB memory. The server also has 2 Nvidia A40 GPUs to run the video encoding and decoding with \name's autoencoder (each using one GPU).

\mypara{Network traces and test videos}
We test \name and the baselines on 16 real bandwidth traces, eight of which are LTE traces from the Mahimahi network-emulation tool~\cite{netravali2015mahimahi} (we filtered out the traces having an average bandwidth lower than 1Mbps),
and the remaining ones are broadband traces from FCC dataset~\cite{fcc-dataset}.
By default, we set the one-way network propagation delay to be 100ms and the queue size to 25 packets. We will also vary these values to show their impact in \S\ref{subsec:eval:e2e}.

Our evaluation uses 60 videos randomly sampled from three public datasets (Kinetics~\cite{Kinetics}, UVG~\cite{mercat2020uvg} and FVC~\cite{FVCDATASET}), each video is at least 10 seconds. 
The video content includes human actions in different environments, nature scenes, sports, as well as indoor and outdoor video calls. The detailed description is in Table~\ref{tab:dataset}.
%Table~\ref{sec:??} summarizes the datasets.
Importantly, we choose these videos because they are different from the training set, allowing us to stress-test the generalization of autoencoders.
These videos cover a range of spatial and temporal dynamics (details are shown in \S\ref{app:siti}), 
and also cover multiple resolutions, with at least 5 videos in each resolution. 
The performance is reported as an average across all the frames in the videos.


% % (equals to 0.75×\times BDP).
% 
% also show the impact of different propagation delays and queue sizes 
% We conduct all experiments on a machine with two Nvidia GeForce RTX 2080 GPUs as the sender and receiver (each using one GPU). The server runs Ubuntu 18.04 with 2 Intel Xeon Silver 4110 CPU and 64GB memory.
% %\jc{more details, such as cuda version, linux version, cpu, memory, etc}
% We measure \name's encoding and decoding delays on the GPU (see results in \S????????????????????????????????????\ref{subsec:eval:system}) and we include these delays in \name's frame delay. 


\mypara{Metrics}
We measure the performance of a video session in the following three aspects.
\begin{packeditemize}
    \item {\em Quality} of a video is measured by frame-level SSIM, and we report the average value across received frames. 
    \item {\em Realtimeness} is measured by the tail of end-to-end frame delay and the ratio of non-rendered frames. End-to-end frame delay means the time lapse between the beginning of encoding and the end of decoding. Non-rendered frames refer to frames that are not played by the receiver due to not being decodable or arriving too late (more than 200ms after the previous frame).
    %reports the ratio of the frames that has a {\em frame-level delay} over 400ms~\cite{zoom-latency-setting}.
    %Frame delay means the time lapse between the beginning of encoding and the end of decoding.
    %For skipped frames, we follow Salsify~\cite{salsify} and set their decoding time to the decoding time of the next received frame.
    % is measured by the {\em frame-level delay}, \ie time lapse between the beginning of encoding to the end of decoding. 
    % For skipped frames (by Salsify), their decoding time equals the next decoding time of the next received frame. 
    % We report the ratio of the frames that has a delay over 400ms. %tail (98th^{th}\% percentile) of the delays across frames in a session.
    \item {\em Smoothness} of the video is measured by the frequency and the ratio of video stalls, where a video stall is defined as the fraction of inter-frame gaps that exceed a threshold. Following the previous work~\cite{macmillan2021measuring} and the logic in WebRTC, we set the threshold to 200ms. The frequency of video stalls means the number of video stalls per second, and the ratio of video stalls is defined as the percentage of time that the video is spent in the stalls.
    %We choose this threshold as it matches the definition in WebRTC. 
\end{packeditemize}



% \textcolor{blue}{
% We also measure the {\em smoothness} of the video by calculating the average video stalls per minute, where a video stall is defined as a frame freezing for more than 0.5 second.}
% \jc{why AVERAGE quality vs TAIL delay?}
%\jc{describe frame rate metric}

% \begin{table}
% \begin{center}
% \footnotesize
% \begin{tabular}{ ccccc } 
%  \hline
%   & \textbf{\# of videos} & \textbf{Duration} & \textbf{Resolution} & \textbf{Characteristics} \\ \hline
%  \textbf{Kinetics 360P} & 49 & 490 secs  & 640×\times3 & \\ \hline 
%  \textbf{UVG} & 5 & 120 secs & 1920$\times$1080 & \\ \hline 
%  \textbf{FVC} & 6 & 135 secs & 1920$\times$1080 & \\ \hline 
%  \hline
% \end{tabular}
% \end{center}
% \label{tab:dataset}
% \vspace{0.3cm}
% \tightcaption{Dataset description.\jc{
% YIHUA: 1. add description. 2. add 360p, 3. add citation, 4. in text, add a link to the data repo (github). ask zhengxu (anonymized)}}
% \end{table}

\begin{table}[]
\footnotesize
\begin{tabular}{ccccc}
\hline
Dataset                                                  & \# of videos & Duration & Resolution       & Characteristics                                                                     \\ \hline
\begin{tabular}[c]{@{}c@{}}Kinetics \\ 360P\end{tabular} & 8            & 80 sec   & 640$\times$360   & \begin{tabular}[c]{@{}c@{}}Human actions and\\ interaction of objects\end{tabular}  \\ \hline
\begin{tabular}[c]{@{}c@{}}Kinetics \\ 720P\end{tabular} & 41           & 410 sec  & 1280$\times$720  & \begin{tabular}[c]{@{}c@{}}Human actions and \\ interaction of objects\end{tabular} \\ \hline
UVG                                                      & 5            & 120 sec  & 1920$\times$1280 & \begin{tabular}[c]{@{}c@{}}HD videos (human, \\ nature, sports, etc)\end{tabular}   \\ \hline
FVC                                                      & 6            & 135 sec  & 1920$\times$1080 & \begin{tabular}[c]{@{}c@{}}Video calls \\ (indoor and outdoor)\end{tabular}         \\ \hline
Total                                                    & 60           & 745 sec  &                  &                                                                                     \\ \hline
\end{tabular}
\vspace{0.3cm}
\tightcaption{Dataset description 
% \jc{YIHUA: 3. add citation, 4. in text, add a link to the data repo (github). ask zhengxu (anonymized)}
 }
\label{tab:dataset}
\end{table}

% \mypara{Test videos}
% Our evaluation uses 60 videos randomly sampled from three public datasets (Kinetics~\cite{Kinetics}, UVG~\cite{mercat2020uvg} and FVC~\cite{FVCDATASET}), each video is at least 10 seconds. The detailed description is in Table~\ref{tab:dataset}.
% %Table~\ref{sec:??} summarizes the datasets.
% Importantly, we choose these videos because they are different from the training set, allowing us to stress-test the generalization of autoencoders.
% The FVC dataset includes 5 videos captured from video conferencing, one of \name's main target use cases.
% These videos cover a range of spatial and temporal dynamics (\S\ref{app:siti})
% and cover multiple resolutions, %(640$\times$360, 1280$\times$720 and 1920$\times$1280)
% with at least 5 videos in each resolution. 
% The performance is reported as an average across all the frames in the videos.



%\mypara{Baselines}
%We compare the performance of \name with multiple state-of-the-art real-time video techniques that use different combinations of video coding and congestion control algorithms: 
%\begin{packeditemize}
%\item {\em Reference:} H.26x with adaptive FEC and GCC
%\item {\em Salsify:}
%\item {\em Idealized SVC:}
%\end{packeditemize}



\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.245\linewidth}
         \centering
         \includegraphics[width=4\linewidth]{figs/gccstall-queue25-delay50-long.pdf}
         \tightcaption{One-way delay = 50ms}
         \label{fig:gcc-50-25}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay75.pdf}
         \tightcaption{One-way delay = 75ms}
         \label{fig:gcc-75-25}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay100.pdf}
         \tightcaption{One-way delay = 100ms}
         \label{fig:gcc-100-25}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay100.pdf}
         \tightcaption{One-way delay = 150ms}
         \label{fig:gcc-150-25}
     \end{subfigure}
     \hfill
     \vspace{0.3cm}
     \tightcaption{End-to-end simulation result under different one-way delay. Network queue length = 25 packets}
     \label{fig:gcc-delay-simulation}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.245\linewidth}
         \centering
         \includegraphics[width=4\linewidth]{figs/gccstall-queue15-delay100-long.pdf}
         \tightcaption{Queue = 15 packets}
         \label{fig:gcc-100-15}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/gccstall-queue15-delay100.pdf}
         \tightcaption{Queue = 25 packets}
         \label{fig:gcc-100-25}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue35-delay100.pdf}
         \tightcaption{Queue = 35 packets}
         \label{fig:gcc-100-35}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.245\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue45-delay100.pdf}
         \tightcaption{Queue = 45 packets}
         \label{fig:gcc-100-45}
     \end{subfigure}
     \hfill
     \vspace{0.3cm}
     \tightcaption{End-to-end simulation result under different network queue lengths. One-way delay = 100ms}
     \label{fig:gcc-queue-simulation}
\end{figure*}


\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.325\linewidth}
         \centering
         \includegraphics[width=3\linewidth]{figs/tail-latency-long.pdf}
         \tightcaption{Tail latency}
         \label{fig:tail-latency}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.325\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/non-rendered-frames.pdf}
         \tightcaption{non rendered frames}
         \label{fig:non-rendered-frames}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.325\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/frequency-of-stalls.pdf}
         \tightcaption{frequency of stalls}
         \label{fig:frequency-of-stalls}
     \end{subfigure}
     \hfill
     \vspace{0.3cm}
     \tightcaption{End-to-end simulation result, comparing \name with other baselines on different metrics}
     \label{fig:other-metrics}
\end{figure}

\begin{figure}[t!]
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=2\linewidth]{figs/fcc-gccdelay-queue25-delay100-long.pdf}
         \caption{SSIM vs. non-rendered frame ratio, using FCC dataset}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/fcc-gccstall-queue25-delay100.pdf}
         \caption{SSIM vs. video stall ratio using FCC dataset}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \vspace{-0.1cm}
     \tightcaption{Results using FCC dataset}
     \label{fig:fcc-simulation}
\end{figure}




\tightsubsection{Video quality vs. realtimeness and smoothness}
\label{subsec:eval:e2e}

% To determine the target bitrate of the video codecs used during simulation, we implemented two different congestion control algorithms: Google congestion control~\cite{carlucci2016analysis} (\textit{GCC}, the standard congestion control used in WebRTC) and the congestion control from~\cite{salsify} (\textit{Sal-CC}). 
%We also implemented FEC-protected H.265 and Salsify codec as the baseline codecs (\S????????????????????????????????????????????????????????????\ref{subsec:eval:setup}).

% Figure~\ref{fig:gcc-delay-simulation} and Figure~\ref{fig:gcc-queue-simulation} 
We evaluated \name against baseline models in terms of average quality (SSIM) and video stall ratio using LTE traces under various network delays (ranging from 50ms to 150ms) and queue lengths (spanning 15 to 45 packets). 
As depicted in Figures~\ref{fig:gcc-delay-simulation} and ~\ref{fig:gcc-queue-simulation}, \name significantly reduces the video stall ratio compared to the baselines. Under all network conditions and congestion control algorithms, \name maintained a video stall ratio below 0.5\%, while the baselines ranged from 2\% to 16\%. 
The primary cause of video stalls is congestion-induced packet loss. When packets are lost, Salsify must skip frames, resulting in increased delay, while H.265 awaits retransmission of lost packets, competing with regular video traffic. 
Tambur has lower video stall ratios than H.265 and Salsify. However, unpredictable congestion losses will still cause video stalls if Tambur is not adding redundancy.
SVC and Voxel also wait for retransmission if the base layer is damaged or a crucial frame is lost. \name, however, can decode a frame as long as any packet from that frame is received.



Using GCC for congestion control, \name attains an average SSIM comparable to the Salsify or H.265 codecs (with or without Tambur), ranging between 15.5dB and 16dB across varied network conditions. 
SVC and Voxel exhibit a marginally lower SSIM, as packet losses inflict greater damage on them compared to \name.
Despite the error concealment techniques mitigates the stall ratio, it fall short in quality when compared to \name. 
It is noteworthy that the machine-learning-based error concealment approach we employ already surpasses traditional methods, such as those implemented in H.264, in terms of reconstruction quality~\cite{zhou2010efficient, varsa2001non}. 
However, most machine-learning-based error concealment solutions, to the best of our knowledge, necessitate a minimum of several hundred milliseconds for error concealment, which is a duration incompatible with the latency requirements of real-time video streaming.

\name can also work with the congestion control algorithm proposed in Salsify (Sal-CC)~\cite{salsify}, which is more aggressive than GCC. Sal-CC has a higher average sending rate, while paying the cost of potentially having more packet losses. 
Figure~\ref{fig:gcc-delay-simulation} and Figure~\ref{fig:gcc-queue-simulation} show that changing from GCC to Sal-CC increases the average SSIM of 0.7-1.1dB for \name with a negligible increase in video stall ratio. 
In contrast, the video stall ratio for Salsify codec will increase a lot when using Sal-CC, because Salsify codec needs to keep skipping frames for more than one RTT when packet loss happens, which leads to frequent video stalls.

Though \name's SSIM is on par or slightly lower than some baselines, we believe that the reduction in frame delay and stall ratio is worth the minor drop in quality, which is also confirmed by our user study (as we will show later).


Figure~\ref{fig:other-metrics} compares \name with the baselines on other metrics when the one-way delay is 100ms and the queue length is 25 packets.
We only put the baselines with comparable average SSIM in this figure (so Voxel and error concealment is not here).
Despite maintaining similar video quality, \name surpasses these baselines by reducing the 98\% frame delay by a factor of 2-5$\times$.
As evidenced in Figure~\ref{fig:non-rendered-frames}, \name only fails to render 0.2\% of frames, far superior to the 4-10\% non-rendered frames exhibited by the baselines.
Additionally, Figure~\ref{fig:frequency-of-stalls} demonstrates that \name experiences few video stalls, thereby markedly outperforming all baselines.

    


% \mypara{Impact of bandwidth distributions}
We also run the simulation based on the broadband traces from FCC dataset~\cite{fcc-dataset}. Compared to the LTE traces, broadband traces have similar average bandwidth but fewer bandwidth drops. We run the simulation with a propagation delay of 100ms and a droptail queue of 25 packets and use GCC as the congestion control algorithm. 
Figure~\ref{fig:fcc-simulation} shows that \name still has a better trade-off between video quality and the ratio of delayed frames and video freezes than the baselines. 

% \mypara{Ablation study of key components} 
% We then conduct an ablation study by removing per-packet entropy coding (\S\ref{??}) and loss-resilience training (\S\ref{??}). 
% We run the experiment using Sal-CC with the same one-way delay and queue length as in Figure~\ref{fig:normal-simulation}. 



Finally, we compare \name and the baselines in a concrete bandwidth trace sample (Figure~\ref{fig:timeseries-ours}).
The bandwidth drops from 8Mbps to 2Mbps at 1.5sec and last for 800ms, before bouncing back to 8Mbps (another bandwidth drop occurs at 3.5sec).
We can see that during each bandwidth drop, \name's delay does not increase as sharply as the baselines (notably Salsify is the second best since it could skip frames).
\name and Salsify use the same CC, so their quality roughly matches on frames not skipped by Salsify.
That said, \name's quality degrades marginally with no frame skipping during congestion, and it bounces back once packet losses disappear. 


% When we run \name with the models trained without any packet losses, the average SSIM will be decreased from \fillme dB to \fillme dB. This is because the frame quality will be significantly decreased when packet loss happens.


\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    \includegraphics[width=1.05\linewidth]{figs/timeseries-new.pdf}
    \tightcaption{\name achieves lower delay and decent quality during sudden bandwidth drops.}
    \label{fig:timeseries-ours}
\end{figure}

\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    \includegraphics[width=0.8\linewidth]{figs/user-study.pdf}
    \tightcaption{Comparing \name with Salsify and H.265 by user study}
    \label{fig:user-study}
\end{figure}


\mypara{User study of video quality} 
% To show decreasing the ratio of delayed frames and video freezes is worth the minor drop in quality for real users, 
To validate \name's improvement, we set up a user study website and gathered 960 user video ratings with Amazon MTurk~\cite{mturk} (IRB approved) in 240 sessions. 
We sampled 8 video clips (spanning cloud gaming, real-time sports events, daily human activities, and talking heads) rendered by \name, Salsify codec and H.265 using {\em GCC} as congestion control while using the same setup as Figure~\ref{fig:normal-simulation}. Appendix~\ref{???} shows the sampled content of the videos.
The sampled video clips have the same distribution of quality, the ratio of delayed frames and video freezes as Figure~\ref{fig:gcc-delay-simulation}. 
% , and the user study is properly randomized following the steps described in \cite{sensei}.
When an MTurk user signed up for the user study, the user will be randomly assigned to rate their user experience (with a Likert scale of 1-5) on the videos rendered by different methods. 
Figure~\ref{fig:user-study} shows the average rating (\ie, mean opinion score or MOS) for each videos from each method. It shows that \name can improve the MOS from 2-2.5 to 3.8-4.7. 

% \yihua{add the real-world validation here: encoding/decoding pipeline running in real-time and measure the latency to show that our system is actually runnable.}


\begin{figure}[t!]
    \centering
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/ssim-bpp-k360.pdf}
    %     \tightcaption{SSIM vs. bit per pixel for Kinetics dataset, 360P videos}
    %     \label{fig:}
    %     % \vspace*{3mm}

    % \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/psnr-bpp-k360.pdf}
    %     \tightcaption{PSNR vs. bit per pixel for Kinetics dataset 360P videos}
    %     \label{fig:}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/ssim-bpp-k720.pdf}
    %     \tightcaption{SSIM vs. bit per pixel for Kinetics dataset 720P videos}
    %     \label{fig:}

    % \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/psnr-bpp-k720.pdf}
    %     \tightcaption{PSNR vs. bit per pixel for Kinetics dataset 720P videos}
    %     \label{fig:}
    % \end{subfigure}
    \begin{subfigure}[t]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/ssim-bpp-kall.pdf}
        \tightcaption{SSIM vs. bit per pixel for Kinetics dataset}
        \label{fig:}
        % \vspace*{3mm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/ssim-bpp-game.pdf}
        \tightcaption{SSIM vs. bit per pixel for gaming dataset}
        \label{fig:}
        % \vspace*{3mm}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.48\linewidth}
        \vspace*{3mm}

        \includegraphics[width=\linewidth]{figs/ssim-bpp-fvc.pdf}
        \tightcaption{SSIM vs. bit per pixel for FVC dataset}
        \label{fig:}
    \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/psnr-bpp-fvc.pdf}
    %     \tightcaption{PSNR vs. bit per pixel for FVC dataset}
    %     \label{fig:}
    % \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/ssim-bpp-uvg.pdf}
        \tightcaption{SSIM vs. bit per pixel for UVG dataset}
        \label{fig:}
    \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/psnr-bpp-uvg.pdf}
    %     \tightcaption{PSNR vs. bit per pixel for UVG dataset}
    %     \label{fig:}
    % \end{subfigure}
    \vspace*{4mm}

    \tightcaption{Quality-size tradeoff of \name.\yc{fix legends!}}
    \label{fig:psnr-vs-bpp}
\end{figure}


\begin{figure}[t!]
     % \begin{subfigure}[b]{0.48\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figs/ssim-loss-0.05.pdf}
     %     \caption{Bpp = 0.05}
     %     \label{fig:queue15-psnr-stall}
     % \end{subfigure}
     % \hfill
     % \begin{subfigure}[b]{0.48\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figs/ssim-loss-0.1.pdf}
     %     \caption{Bpp = 0.1}
     %     \label{fig:queue15-ssim-delay}
     % \end{subfigure}
     % \hfill
     %    \begin{subfigure}[b]{0.48\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figs/ssim-loss-0.2.pdf}
     %     \caption{Bpp = 0.2}
     %     \label{fig:queue15-psnr-stall}
     % \end{subfigure}
     % \hfill
     % \begin{subfigure}[b]{0.48\linewidth}
     %     \centering
     %     \includegraphics[width=\linewidth]{figs/ssim-loss-0.3.pdf}
     %     \caption{Bpp = 0.3}
     %     \label{fig:queue15-ssim-delay}
     % \end{subfigure}
     % \hfill
     % \vspace{-0.1cm}
     \centering
     \includegraphics[width=1.07\linewidth]{figs/ssim-loss-v2.pdf}
     \tightcaption{\name's loss resilience for different BPPs and different number of lossy frames}
     \label{fig:loss_by_bitrate}
\end{figure}


\tightsubsection{Coding efficiency and loss resilience}
\label{subsec:eval:resilience}

\mypara{Coding efficiency of \name} 
% For any loss-resilient schemes, 
There is always a tradeoff between compression and loss resilience, and \name is no exception.
% The ability to tolerate packet losses often comes with a drop in quality in absence of packet losses, and \name is no exception. 
Figure~\ref{fig:psnr-vs-bpp} compares the \name's quality under no packet loss with that of H.264 and H.265 across the test videos from Table~\ref{tab:dataset} (all of which are different from the training set).
Following the previous works, we use {\em bit per pixel} (BPP) to measure size.
Figure~\ref{fig:psnr-vs-bpp} shows that \name is similar to H.264 and is only slightly worse than H.265.
It also shows that \name can cover a wide range of BPPs among all datasets, from 0.03 to 0.5. 
% This enables more flexible bitrate adaptation when running \name.

\begin{comment}

Remember that H.26x uses the zerolatency option and fast preset (which is typical to real-time videos, including WebRTC\footnote{Google's WebRTC~\cite{WEBRTCSRC} uses OpenH264~\cite{OPENH264}. They set the runtime parameter "usageType" to CAMERA\_VIDEO\_REAL\_TIME  (similar to zerolatency) and "complexityMode" to LOW\_COMPLEXITY (similar to fast)}. 
We confirm that without these settings, H.265's coding efficiency is better than \name in the absence of packet losses.
However, our goal is a data-scalable autoencoder for real-time videos (shown shortly) rather than an autoencoder that outperforms heavily engineered H.26x codecs. 
Moreover, the coding efficiency of the autoencoder could still be improved (\eg our autoencoder estimates motion vectors based only on one reference frame).

\end{comment}

\mypara{Loss resilience of \name}
Figure~\ref{fig:loss_by_bitrate} compares \name with the baseline codecs under different packet loss rates. \edit{We apply packet losses for $N$ consecutive frames and calculated the decoded quality of the lossy frames. Figure~\ref{fig:loss_by_bitrate} shows the result when $N=1,3,5$.}
% when encoding videos from Table~???\ref{tab:dataset}.
In each figure, all lines have almost the same encoding BPP with differences controlled within 5\%.
We ensure that \name's encoded BPP is {\em never} higher than the baselines, so even if the actual encoded BPP is different, it does not favor \name. Figure~\ref{fig:decoded-example} in Appendix~\ref{app:visualization} shows an example to visualize the behavior of \name under packet loss.

The most salient feature of \name is the graceful quality degradation with more packet losses. 
The average SSIM drop is only 1 dB to 3 dB under 20\% and 50\% packet losses among all the BPPs. 
Even when the loss ratio is as high as 80\%, \name can still have an average SSIM of 12 dB across different BPPs, which is much better than H.264 with various FEC redundancy rates, and SVC for the reasons elaborated in \S\ref{subsec:eval:e2e}.

We further contrast \name with alternative decoder-side error concealment baselines, encompassing a pretrained autoencoder~\cite{dvc}, \name with an untrained encoder neural network, and a machine-learning-based error concealment solution (\S\ref{subsec:eval:setup}). \name consistently surpasses these baselines, a result attributable to its joint encoder-decoder training process that facilitates the introduction of redundancy into the encoded byte stream. Conversely, other decoder-side error concealment baselines lack this redundancy in the encoder's output.

\edit{In real-world scenarios, packet loss typically affects not merely a single frame, but a series of consecutive frames~\cite{rudow2023tambur}. Figure~\ref{fig:loss_by_bitrate}c and~\ref{fig:loss_by_bitrate}d shows the performance of \name and the baselines when packet losses occur across 3 and 5 consecutive frames. When compared to other baselines, \name is capable of achieving a higher SSIM, up to 2, covering different loss rates between 10\% and 80\%. We have excluded FEC and SVC from Figure~\ref{fig:loss_by_bitrate}c and~\ref{fig:loss_by_bitrate}d, as it becomes inconsequential to compute the quality of subsequent frames if preceding ones are undecodable.}



\begin{comment}
    
Compared with H.264 with fixed FEC protection, \name can have a higher SSIM of 1.1 dB to 1.9 dB among different resolutions and different BPPs when there is no loss. 
This is because any arrived bytes in \name contribute to the quality while in FEC, the redundant data is useless even if they do arrive at the decoder. 
On the other hand, FEC-based loss resiliency is also in a dilemma that a low FEC rate cannot protect against the high loss, but a high FEC rate leads to poor quality when the packet loss ratio is small. 
Our \name solves this dilemma by graceful quality degradation.

Compared to the error concealment baseline, \name's quality decreases more gracefully when the loss rate increases. This is because when the loss rate is high (\eg larger than 50\%), the error concealment baseline can hardly recover the motion vectors, which causes a fast quality degradation. However, \name's encoder learns to encode the frame with some redundancy, such that it can still recover some of the lost data from the received packets.

\name is also better than SVC with unequal FEC protection (\S??????????????????????????????????????????\ref{subsec:prior}). 
The quality of SVC decreases quickly when the loss rate is small, as the high-quality layers are unlikely to be decodable in such cases. 
We also note that the pre-trained autoencoder models, which have not seen any losses in training, degrade poorly with higher loss rates. 


\end{comment}


\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/burst-loss.pdf}
         \caption{50\% of packet loss is applied to frame 6, 7, 8}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/long-loss.pdf}
         \caption{10\%, 30\%, 50\% packet loss is applied on {\em every} frame after 6-th frame}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
    \tightcaption{The detailed behavior of \name under different kind of losses.}
    \label{fig:loss-behavior}
\end{figure}

% We conduct a detailed analysis of \name under different kinds of packet losses
Figure~\ref{fig:loss-behavior} shows that if there is a transient packet loss, the quality of the following frames will not keep degrading. When the packet losses are persistent, \name can still deliver good quality for more than 10 frames, without needing any synchronization between the encoder and the receiver.

%\jc{
%\begin{itemize}
%    \item by bitrate
%    \item by video set
%    \item psnr vs. bitrate
%\end{itemize}
%}

% \jc{need a footnote to explain why intra-mb insertion is so bad}



 

%In Figure~???????????????????????????\ref{??}, we use three metrics for video quality, even though our autoencoders are trained to optimize L2-norm between the reconstructed and original images, which is similar to RGB-PSNR, their quality compared to baselines is similar under different metrics.

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_traceset_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_rtt_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_queue_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}


%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=1.pdf}
%    \caption{Aggressiveness = 1}
%    \label{fig:}
%\end{figure*}
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=0.75.pdf}
%    \caption{Aggressiveness = 5}
%    \label{fig:}
%\end{figure*}








% \jc{YIHUA, please fill in some detailed reading}

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/encoding-lat-gpu.pdf}
%          \caption{Encoding latency on A100 GPU}
%          \label{fig:gpu-encoding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/encoding-lat-cpu.pdf}
%          \caption{Encoding latency on CPU}
%          \label{fig:gpu-decoding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/decoding-lat-gpu.pdf}
%          \caption{Decoding latency on A100 GPU}
%          \label{fig:cpu-encoding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/decoding-lat-cpu.pdf}
%          \caption{Decoding latency on CPU}
%          \label{fig:cpu-decoding}
%      \end{subfigure}
%      \hfill
%      \tightcaption{Compute overhead of \name.}
%      \label{fig:computing-overhead}
% \end{figure} 

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/encoding-lat-gpu-new.pdf}
         \caption{Encoding latency on A100 GPU}
         \label{fig:gpu-encoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/encoding-lat-copies-gpu-new.pdf}
         \caption{Total latency to encode multiple copies of different bitrates}
         \label{fig:gpu-multi-encoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/encoding-lat-cpu-new.pdf}
         \caption{Encoding latency on CPU}
         \label{fig:gpu-decoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/decoding-lat-gpu-new.pdf}
         \caption{Decoding latency on A100 GPU}
         \label{fig:cpu-encoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/decoding-lat-cpu-new.pdf}
         \caption{Decoding latency on CPU}
         \label{fig:cpu-decoding}
     \end{subfigure}
     \hfill
     \tightcaption{Compute overhead of \name.}
     \label{fig:computing-overhead}
\end{figure*} 

% \begin{figure}[t!]
%      \begin{subfigure}[b]{0.48\linewidth}
%          \centering
%          \includegraphics[width=2\linewidth]{figs/cpu-gccdelay-queue25-delay100-long.pdf}
%          \caption{SSIM vs. delayed frame ratio}
%          \label{fig:queue15-psnr-stall}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.48\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/cpu-gccstall-queue25-delay100.pdf}
%          \caption{SSIM vs. video stall ratio}s
%          \label{fig:queue15-ssim-delay}
%      \end{subfigure}
%      \hfill
%      \vspace{-0.1cm}
%      \tightcaption{End-to-end simulation results for CPU version \name \zy{missing legend for the black dot}}
%      \label{fig:simulation-ablation}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%          \centering
%         %\includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
%         \includegraphics[width=0.7\linewidth]{figs/cpu e2e.pdf}
%          \label{fig:}
%          \vspace{.05cm}
%     \tightcaption{CPU end to end result. \textcolor{red}{TODO: Ziyi and Hanchen}}
%     \label{fig:cpu-simulation}
% \end{figure}

\tightsubsection{Computational overhead}
\label{subsec:eval:system}

% \zy{There is a typo ("decodeing latency") on the y-axis label on Figure 16 (b). (figs/decode.pdf)}

% Remember that \name needs a P-frame encoder and a I-frame encoder to encode each frame as a P-frame and an I-patch (a small spatial region without reference).
%\mypara{Computational overhead}
% We test the encoding/decoding speed of un-optimized \name, optimized \name (\S\ref{subsec:fast-coding}) and H.264 from \texttt{ffmpeg} on a Linux server with an A100 GPU and Intel Xeon Silver 4210R CPU (32 threads).
% Figure~\ref{fig:gpu-encoding} and Figure~\ref{fig:gpu-decoding} show the encoding and decoding speed on GPU. With the optimizations, \name can encode and decode a 720P frame in 34.9ms and 15.5ms respectively, which is 1.5$\times$ and 2$\times$ faster than the unoptimized version. This translates to 28fps and 35fps for encoding and decoding 720P frames. 
% For 480P videos, optimized \name can encode/decode in 25.3 and 15.4ms, which equals to 40fps and 65fps for encoding and decoding.
\yihua{discussion about the setup here}
We conducted encoding/decoding speed tests on {\em \name-naive},  \name (\S\ref{subsec:fast-coding}), and H.264 from \texttt{ffmpeg} on our testbed (equipped with Nvidia A40 GPU and Intel Xeon 4210R CPU 2.40GHz). The results, presented in Figure~\ref{fig:gpu-encoding} and 
Figure~\ref{fig:gpu-decoding}, illustrate the GPU encoding and decoding speed. Following optimizations, \name was capable of encoding and decoding a 720P frame in 34.9ms and 15.5ms, respectively, marking an improvement of 1.5$\times$ and 2$\times$ over our prior work. This equates to frame rates of 28fps and 35fps for encoding and decoding 720P frames, respectively. Also, the overhead for \name to encode a new copy for bitrate adaptation is negligible. As shown in Figure~\ref{fig:gpu-multi-encoding}, it only takes 2.1ms for \name to encode a new copy of a different bitrate, while \name-naive needs more than 10ms to do the same thing.

% Figure~\ref{fig:cpu-encoding} and Figure~\ref{fig:cpu-decoding} shows our optimizations on CPU can significantly reduce the encoding and decoding time. For 720P videos, the original model takes 5217ms and 3996ms to encode and decode a frame, while the time decreases to 35.1ms and 40.9ms after applying our optimizations. This shows that with our optimization, \name is able to stream the 720P video purely using CPU.
% Compared with the GPU version of \name, the optimized CPU version has a lower SSIM of 0.8 dB. However, it does not impact the improvement in the ratio of delayed frames. %, and the quality is not bad compared to the error concealment baseline.

As illustrated in Figure~\ref{fig:cpu-encoding} and Figure~\ref{fig:cpu-decoding}, our CPU optimizations significantly curtail encoding and decoding times. For 720P videos, the initial model necessitated 5217ms and 3996ms to encode and decode a frame, respectively; however, these times were dramatically reduced to 35.1ms and 40.9ms following our optimization. This demonstrates that \name, with our optimization, is capable of streaming 720P video using the CPU alone. Despite the optimized CPU version of \name exhibiting a marginally lower SSIM of 0.8 dB compared to its GPU counterpart, this discrepancy does not compromise the improvement in the ratio of delayed frames.

% \begin{figure}[t!]
%     \centering
%          \centering
%         %\includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
%         \includegraphics[width=0.7\linewidth]{figs/encoding-multiple-version.png}
%          \label{fig:system-encoding-versions}
%          \vspace{.05cm}
%     \tightcaption{Encoding latency of encoding multiple versions \textcolor{red}{TODO: Yihua}}
%     \label{fig:multiple-encoding}
% \end{figure}

\mypara{\name's fast bitrate adaptation}
Figure~\ref{fig:gpu-encoding} also depicts the latency incurred by \name while encoding multiple frame copies at varying bitrates (\S\ref{subsec:fast-coding}). Given that the most time-intensive portion of encoding is shared across models, the additional time required to encode multiple versions is minimal, averaging merely 2.6ms per extra copy. Consequently, \name is capable of encoding three distinct copies within 40.9ms, thus facilitating real-time bitrate adaptation by the encoder. Our empirical observations reveal that over 65\% of frames require a single encoding pass, while 34\% necessitate a second pass to adjust to the target bitrate. A marginal subset, less than 1\%, is subjected to a third encoding pass.

\tightsubsection{Microbenchmarking}
\begin{figure}[t!]
     \begin{subfigure}[t]{0.48\linewidth}
         \centering
         \includegraphics[width=2\linewidth]{figs/abl-gccdelay-queue25-delay100-long.pdf}
         \caption{SSIM vs. non-rendered frame ratio, using different versions of \name}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/abl-gccstall-queue25-delay100.pdf}
         \caption{SSIM vs. video stall ratio, using different versions of \name}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     % \vspace{-0.1cm}
     \tightcaption{Ablation study (per packet EC, loss resilience) }
     \label{fig:simulation-ablation}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.45\linewidth}
        \includegraphics[width=\linewidth]{figs/sr-expr.pdf}
        \tightcaption{The quality of \name and baselines after super-resolution}
        \label{fig:sr-experiment}
    \end{minipage}
    \hfill % or \hspace{5mm} if you want to specify a certain amount of space
    \begin{minipage}[t]{0.45\linewidth}
        \includegraphics[width=\linewidth]{figs/validation.pdf}
        \tightcaption{The simulated frame delay of \name is close to the real world measured frame delay}
        \label{fig:validation}
    \end{minipage}
\end{figure}


\mypara{Ablation study}
Moreover, Figure~\ref{fig:simulation-ablation} shows that both the delayed frame ratio and the stall ratio will increase if \name does not use per-packet entropy coding described in \S\ref{subsec:packetization} (the red cross). 
This is because, without it, the size of the encoded frame will have an increase of 1.5$\times$, and this size increase may overload the network when bandwidth suddenly drops. 
It also shows without training with loss, the pretrained autoencoder models will suffer from quality drops caused by packet loss. The SSIM will drop from 15.7 to 12.4 compared to \name.

We also evaluate the impact of the optimizations proposed in~\S\ref{subsec:fast-coding} for speeding up CPU encoding/decoding. As shown in Figure~\ref{fig:simulation-ablation}, the average SSIM decreased from 15.8 to 15.4 after applying the CPU-related optimizations, and the optimizations do not affect the realtimeness and smoothness of the decoded video much.

\mypara{Working with super-resolution}
Figure~\ref{fig:sr-experiment} shows the tradeoff between quality and video stall ratio when using SR to enhance the quality at the receiver side. 
We run the simulation using LTE traces with a 100ms one-way delay and a 25-packet queue, and the congestion control algorithm is GCC. 
When using SR, \name can still have on-par SSIM with Salsify codec, H.265 w/ Tambur: 15.8 dB, 16.4 dB, and 16.0 dB respectively.
The quality of SVC is still lower than \name even with super-resolution. This is because packet loss can make higher layers of SVC undecodable, resulting in lower quality.
This shows SR technique is complementary to our work, as it can improve the quality for any codecs at the receiver side.

\mypara{Simulator validation}
To validate that the frame delay measured in simulation matches the real-world numbers, we run a real-world emulation using \name. Being the same as simulation, we use 2 Nvidia A40 GPUs, one for encoding and one for decoding. 
The encoder process encodes the video using \name's encoder and send the encoded packets through an emulated network.
The decoder process decodes the frame using the same logic as mentioned in \S\ref{sec:delivery}.
We compute the real-world frame delay by calculating the difference between the encoding time and the decoding time of a frame.
Figure~\ref{fig:validation} compares the simulated frame delay and real-world measured frame. We use the bandwidth trace same as Figure~\ref{fig:timeseries-ours}. The result validates that our simulated frame delay is accurate.
It is worth noting that we are running real encoding and decoding process in the simulation, hence the calculated frame quality should also be the same as using \name in real-world.




% Figure~\ref{fig:gpu-encoding} shows the encoding latency for \name to encode multiple different copies of frames with different bitrates (\S\ref{subsec:fast-coding}). Since the models share the most time-consuming part of the encoding, the overhead of encoding multiple versions is negligible: only 2.6ms for every extra copy. Therefore, \name can encode 3 different copies in 40.9ms, allowing the encoder to do bitrate adaptation in real-time.
% Empirically in our study, over 65\% frames will only be encoded once and 34\% frames will be encoded twice to adapt to the target bitrate. Less than 1\% frames will be encoded 3 times. 
% Figure~\ref{??} shows the effectiveness of our bitrate controlling algorithm (\S\ref{??}). Over \fillme\% of frames will falls in the range of $[0.8, 1]\times$ target bitrate and it will never produce a frame that overshoots the target bitrate.

% \mypara{Model training decisions}
% To validate the design choices of loss distribution we used during model training, we conduct an ablation study of different loss distributions. We test two different setups: (i) the probability of using 0 loss is the same as other loss rates, and (ii) loss rates as high as 80\% and 90\% are added during training. As shown in Figure~???\ref{fig:training-loss-study}, both setups can cause the SSIM under 0 loss decrease around \fillme dB. 
% When the probability of 0 loss is low, the model will learn to deprioritize the quality under 0 loss, which will impact the average video quality. We also observe that seeing a loss as high as 80\% or 90\% will also damage the quality under 0 loss.


% Our implementation of \name optimizes both memory footprint and encoding/decoding delay (described in \S???\ref{subsec:optimize}), and we test its effectiveness on a Nvidia GeForce RTX 3080 GPU. 
% Figure~???\ref{fig:system-encoding} and Figure~???\ref{fig:system-decoding} show that compared to the original (unoptimized) implementation of pre-trained autoencoder (which takes 100ms to encode a 480p frame), our implementation can encode a 480p frame in less than 25ms (a 4×4\times speedup).\footnote{The only autoencoder that achieves comparable encoding/decoding speed is~\cite{elf}, and it achieves such speed on a 5x more expensive Titan V GPU. We hope to compare it with \name, but it is not open-source.}
% This translates to almost 40fps. 
% Even for 720p HD videos, our optimized codec can achieve 18fps (55ms encoding per frame). 
% % \fillme~fps/\fillme~fps, \name encodes/decodes 480p frames at \fillme~fps/\fillme~fps, a \fillme×\times speedup.
% This acceleration comes from downsampling frames in motion-vector estimation. 
% Moreover, when adapting to a target bitrate, \name encodes the next frame multiple times {\em without} needing to run the entire encoder multiple times, because it re-uses the motion-compensated prediction, so only the residuals need to be encoded at multiple bitrates. Figure~??????\ref{fig:system-encoding-versions} shows that the delay of encoding a frame at three different bitrates only increases marginally compared to encoding one frame. 







% In terms of memory usage, our optimized implementation saves the memory footprint of loading 9 models by over 60\% since most NN layers are shared. 
% % Figure~??????\ref{??} shows that compared to loading the multiple autoencoders (I-frame encoder/decoder and a P-frame encoder/decoder of each bitrate) in GPU memory, the memory usage \name's autoencoders (not including the memory usage of intermediate features) is \fillme\% smaller, because they share most of the layers (only the last \fillme layers of the encoder and the first \fillme layers of the decoders are different). 
% Note that \name does not change the NN architecture of the autoencoders---only the weights are retrained and the way they are used is optimized. We speculate that they could be made more efficient with appropriate modification to its NN architecture.

% Figure~??????\ref{??} validate that \name's coding efficiency is comparable to (even slightly better than) without the optimizations (\ie without sharing the NN backbone or downsampling and sharing the motion-vectors.)
% This is because, though quality does drop with these optimizations, the encoded size also drops (due largely to the downsampled motion vectors), which result in a similar bitrate-quality trade-off frontier.

% \jc{The only autoencoder that achieves comparable encoding/decoding speed is Elf~\cite{??}. 
% We hope to compare it with \name, but it is not open-source. }


% \jc{remember to highlight that the speed is comparable to elf, which runs on the 5x more expensive titan v gpu.}

% \begin{figure}[t!]
%     \centering
%          \centering
%         \includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
% %        \includegraphics[width=0.7\linewidth]{figs/a.pdf}
%          \label{fig:}
%          \vspace{.05cm}
%     \tightcaption{Training curve study \textcolor{red}{put into appendix}}
%     \label{fig:training-loss-study}
% \end{figure}
%!TEX root = ../main.tex
%!TEX spellcheck = en_US



==> sections/old/eval_v7.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Evaluation}
\label{sec:eval}

The findings of our evaluation can be summarized as follows:
\begin{packeditemize}
\item {\bf Loss resilience:} \name's quality under no packet loss is on par with H.264 and H.265 and its quality gracefully degrades with higher loss rates.  Notably, when loss rates fluctuate between 20\% and 80\%, \name can enhance the SSIM by 1.4-4 dB compared to baseline measures across diverse videos and bitrates.
%\jc{this should be backed up with some concrete numbers, such as improve SSIM by xxx-xxx dB at \fillme packet loss rate}

\item {\bf Quality-delay tradeoff:} Under bandwidth fluctuations in real network traces, \name has almost {\em zero} video stalls (video freezes for over 200ms), achieving a reduction of 90\% compared to other loss-resilient schemes.
Also, \name reduces the tail frame delay by 2-4$\times$ and the ratio of non-rendered frames by 95\%.
Our user study has also confirmed that \name's rated score is 38\% higher than the baselines. %\jc{please update this with new results.}

\item {\bf Overhead:} Our implementation of \name can encode/decode 480p video at 87~fps/122~fps and 720p HD video at 31.2~fps/44.1~fps using Nvidia A40 GPU, a 1.5-5$\times$ faster compared to recent autoencoder-based video codecs~\cite{swift, yang2020learning,shi2022alphavc, dvc}. 
% off-the-shelf autoencoders~\cite{swift, dvc}. 
With the optimization for CPU (\S\ref{subsec:fast-coding}), \name can also encode/decode 720p HD video at 27~fps/25~fps on CPU with marginal quality degradation.
\end{packeditemize}


\tightsubsection{Setup}
\label{subsec:eval:setup}



\mypara{Training of \name}
\name's autoencoder, based on the cutting-edge video autoencoder DVC~\cite{dvc}, is fine-tuned using the vimeo-90K~\cite{vimeo-dataset} dataset. This fine-tuning involved two steps: initial fine-tuning of a base model with packet losses (\S\ref{sec:core}), followed by employing 11 discrete $\alpha$s (Eq.~\ref{eq:2}), from $1/64$ to $1/32768$, to refine the residual encoder and decoder for bitrate adaptation (\S\ref{subsec:fast-coding}). 
With a learning rate of $10^{-4}$, each fine-tuning step typically took 1-2 hours on an Nvidia A40 GPU.
% We build \name's autoencoder based on DVC~\cite{dvc}, a state-of-the-art video autoencoder. 
% We fine-tuned \name on the vimeo-90K~\cite{vimeo-dataset} dataset from the pretrained model of DVC. The fine-tuning takes two steps: we first fine-tuned a base model with packet losses applied during training.  
% Then, we employed 11 distinct $\alpha$s (in Eq.~\ref{eq:2}), ranging from $1/64$ to $1/32768$ to fine-tune the residual encoder and decoder. This enables \name to support various bitrates (\S\ref{subsec:fast-coding}). 
% We set the learning rate at $10^{-4}$, and each step of fine-tuning typically takes 1-2 hours on an Nvidia A40 GPU.
%\fyy{Besides fine-tuning DVC's pretrained model, are there other differences?} 

%Figure~\ref{fig:dvc-arch} shows the architecture of the encoder and decoder. On the sender side, the encoder neural network takes the current frame and its reference frame as the input, and outputs the encoded motion vectors and residuals (\S\ref{subsec:background}). On the receiver side, the decoder neural network decodes the received motion vector and residuals, then reconstructs the new frame based on the reference frame.
%\fyy{Why repeat Grace's design in the experimental setup? It's better to treat this paragraph as "implementation" and explain how DVC is adapted for this purpose.}


\mypara{Baselines}
%\yihua{update text: rewrite baseline implementation}
We implemented loss-resilient baselines using H.265 from \texttt{ffmpeg} (version 4.2.7), one of the most advanced video codecs, boasting comparable or superior compression efficiency to other widely-used codecs such as H.264, VP8, and VP9~\cite{x265vp9compare, grois2013performance} (We also confirmed this on our own testing videos in Appendix~\ref{app:h26xvpx}). 
These baselines embody different design alternatives (\S\ref{subsec:related}) for loss-resilient video coding. Given space constraints, detailed baseline implementation, excluding \name, is relegated to Appendix~\ref{app:baseline}.
% We implemented the following loss-resilient baselines using H.265 of \texttt{ffmpeg} (version 4.2.7). It is worth noting that H.265 is one of the most advanced video codecs, having on-par or better compression efficiency compared to other widely-used codecs such as H.264, VP8 and VP9~\cite{x265vp9compare, grois2013performance}. The baselines are covering different design choices (\S\ref{subsec:related}) for loss-resilient video coding. Due to space limitations, we put the detailed baseline implementation (except \name) to Appendix~\ref{app:baseline}. %\yc{should I also bold the name of each baseline? Now the bolded texts are design choices.}
\begin{packeditemize}
  \item {\bf \name (ours)}: We implement \name's autoencoder with 1100 lines of Python code, including encoding, decoding, packetization, and bitrate adaptation. 
  We use \textit{torchac}~\cite{torchac} for entropy coding and % \fyy{Has ``per-packet entropy coding'' been described and justified in previous sesions (compared with the standard approach of entropy-encoding DCT coefficients?} 
  %Since \name's autoencoder is focusing on compressing inter frames (P-frames), we use BPG~\cite{bpg} to encode the first I-frame and the I-patches (\S\ref{sec:delivery}).
  BPG~\cite{bpg} for the first I-frame and the I-patches (\S\ref{sec:delivery}).
  
  \item {\bf Forward error correction}: 
  We implement Tambur~\cite{rudow2023tambur}, a state-of-the-art FEC solution with H.265.
  This solution outperforms WebRTC's default FEC scheme, reducing the number of non-decodable frames while transmitting an equivalent amount of parity packets. The redundancy rate of Tambur, defined as $\frac{p}{n}$ (with $p$ as the number of parity packets and $n$ the total packets, including parity packets~\cite{xiao2012dynamic, lee2022r}), dynamically adapts based on the packet loss measured in the preceding 2 seconds using the same logic as WebRTC\cite{WEBRTCSRC}. %This approach, utilized in WebRTC\cite{WEBRTCSRC}, assures superior quality compared to a constant redundancy.
  %We implement Tambur~\cite{rudow2023tambur}, a state-of-the-art forward error correction solution using streaming code, with H.265\footnote{Following recent work in real-time video coding~\cite{ZEROLAT1,ffmpegstreaming}, we use the \texttt{zerolatency} option (no B-frames) and the \texttt{fast} preset of H.265. The command line we used to encode a video is \texttt{ffmpeg -y -i Video.y4m -c:v libx265 -preset fast -tune zerolatency -x265-params "crf=Q:keyint=3000" output.mp4} where {\em Q} controls the quality of the frame.}. It performs better than the default FEC scheme used in WebRTC since it decreases the number of non-decodable frames when sending the same amount of parity packets. According to the prior work~\cite{xiao2012dynamic}, we define the redundancy rate of Tambur as $\frac{p}{n}$ where $p$ is the number of parity packets $n$ is the total number of packets (including parity packets). The redundancy rate is dynamically set based on the packet loss measured in the previous 2 seconds, which is also used in WebRTC~\cite{WEBRTCSRC} and has better quality compared with adding a constant redundancy.
  
  % We implement Tambur~\cite{rudow2023tambur} with H.265\footnote{Following recent work in real-time video coding~\cite{ZEROLAT1,ffmpegstreaming}, we use the \texttt{zerolatency} option (no B-frames) and the \texttt{fast} preset of H.265. The command line we used to encode a video is \texttt{ffmpeg -y -i Video.y4m -c:v libx265 -preset fast -tune zerolatency -x265-params "crf=Q:keyint=3000" output.mp4} where {\em Q} controls the quality of the frame.}, and we do not restrict their GoP (I-frame interval), a state-of-the-art forward error correction solution using streaming code. \fyy{We only had one key frame at the very beginning of a video session and did not have any GoP. Putting that aside, this detail is still unnecessary if you don't/can't justify why a state-of-the-art approach is not adopted.} Tambur performs better than the default FEC scheme used in WebRTC since it can decrease the number of non-decodable frames when sending the same amount of parity packets. According to the prior work~\cite{xiao2012dynamic}, we define the redundancy rate of Tambur as $\frac{p}{n}$ where $p$ is the number of parity packets $n$ is the total number of packets (including parity packets). According to WebRTC~\cite{WEBRTCSRC}, the redundancy rate is dynamically set based on the packet loss measured in the previous 2 seconds, which has better quality compared with adding a constant redundancy.
  %\yc{mention the redundancy rate is determined by webrtc logic, either here or in the simulation section}
  
    
  \item {\bf Postprocessing error concealment}: 
  We use a state-of-the-art machine-learning-based error concealment method~\cite{kang2022error} as the error concealment baseline. 
  The baseline uses neural networks to both estimate the missing motion vector and enhance the reconstructed frame by inpainting. It surpasses the related works that only do motion estimation~\cite{sankisa2018video} or inpainting~\cite{chang2019free}. 
  According to the prior works~\cite{kumar2006error, wenger2002scattered, 4494082}, we assume an extra 10\% size overhead to make sure each packet is individually decodable. %as the per-packet entropy coding technique.
  %Error concealment recovers quality from the packet loss by predicting the missing content using hand-tune heuristics~\cite{zhou2010efficient, varsa2001non} or neural networks~\cite{kang2022error, sankisa2018video, mathieu2015deep}. Error concealment methods need to work with per-packet entropy coding techniques such as flexible macroblock ordering~\cite{KUMAR2006425} because it requires an incomplete frame to be decodable. 

  %The baseline encodes/decodes the video using H.265. When there is an incomplete frame, the baseline takes 3 steps to conceal the errors. It will first use a neural network to estimate the motion vector of the missing part based on previous frames. Then, it will propagate the missing pixel values from the reference frame with the estimated motion vector. Finally, it will use an inpainting neural network to improve the frame quality and reduce error propagation. It is better than motion-prediction-only or inpainting-only error concealment methods (\cite{sankisa2018video, mathieu2015deep}). We also assume a \fillme\% size overhead caused by the per-packet entropy coding, which matches the overhead mentioned in~\cite{??}.
  
  \item {\bf Scalable video coding (SVC)}: %SVC encodes a video at multiple quality layers and sends data layer by layer. 
  We implement an idealized SVC, such that when the first $x$ layers arrive, it will reach a quality the same as that of H.265 at receiving the same amount of bytes. 
  This idealized implementation is already better than the state-of-the-art SVC~\cite{swift}.
  We also add 50\% FEC to protect the base layer for SVC, as it is also a common practice in real-time videos~\cite{khalek2012cross}.


  
  \item {\bf Selective frame skipping}: One potential design choice of selective frame skipping is optimizing the frame delay by only retransmitting the important frames that will cause huge damage to the video quality when missing. We implement a baseline for this design choice based on Voxel~\cite{voxel}, a recent work using selective frame skipping to reduce the video rebuffering ratio and improve the user's QoE. 

  Functional codecs also support frame skipping. We implemented the recent functional codec, Salsify~\cite{salsify}, based on H.265 with two features: firstly, the encoded frame size never surpasses the target bitrate determined by the underlying congestion control algorithm; secondly, upon packet loss, the encoder can dynamically select a reference frame, enabling subsequent frames to be decoded without resending any packets.
  %Unlike traditional codecs (\eg, H.265 or VP9), functional codecs are able to skip incomplete frames when packet loss happens and decode the first complete frame without a significant quality drop. Salsify~\cite{salsify} is a recent work implementing the functional codec. 
  %We implement the Salsify baseline based on H.265 with the following features: {\em (i)} the encoded frame size of the codec will never overshoot the target bitrate calculated by the underlying congestion control algorithm, and {\em (ii)} when packet loss happens, the encoder can dynamically choose a reference frame to make later frames decodable without retransmitting any packets.

  \item {\bf Super-resolution (SR)}: We tests the quality improvement of the state-of-the-art SR model~\cite{liang2021swinir} on our baselines. It is worth noting that since SR should work for any video codec, it is {\em orthogonal} to \name's design space. 
  %We use a state-of-the-art SR model, SwinIR~\cite{swinir}, as the tool to improve the video quality for both \name and other baselines after the receiver successfully decodes the frame. \yc{consider move it to 5.5}

\end{packeditemize}

% For the baselines of functional codec (Salsify), SVC, and selective frame skipping (Voxel), we make an idealized assumption that on each frame, the output bitrate of the codec perfectly matches the target bitrate chosen by the congestion control algorithm (explained in \S\ref{subsec:eval:e2e}), \ie never overshooting or undershooting, but the actual quality matches that of the highest \texttt{qp} that leads to a frame greater than the target bitrate. 
We used an idealized version of functional codec (Salsify), SVC, and selective frame skipping (Voxel) baselines. For each frame, we assume that the codec's output bitrate flawlessly aligns with the target bitrate determined by the congestion control algorithm (\S\ref{subsec:eval:e2e}), i.e., there are no overshoots or undershoots. However, the actual quality corresponds to the highest \texttt{qp} resulting in a frame size exceeding the target bitrate.
These optimizations make the baselines' performance slightly better.
% In other words, their performance is higher than it would actually be in the real world.

\mypara{Testbed implementation}
Our testbed has 2 Nvidia A40 GPUs to run the video encoding and decoding with \name's autoencoder (each using one GPU).
We developed a packet-level network simulator to compare \name with baselines across various network conditions. The simulator employs a configurable drop tail queue to mimic packet losses induced by congestion and implements a token bucket algorithm for simulating bandwidth variation every 0.1 seconds. Google congestion control~\cite{carlucci2016analysis}, a standard WebRTC algorithm, was utilized to establish the target bitrate of video codecs during simulations.
The simulator emulates a complete real-time video communication application, including encoding, packetization, rate adaptation, and decoding, operating at a 25fps encoding rate (matching state-of-the-art real-time video measurements~\cite{macmillan2021measuring}). 
% The packets are transmitted over a network simulated by the simulator. 
It outputs a decoded video and the end-to-end delay of each frame, incorporating encoding and decoding time. We confirmed our simulator's accuracy regarding frame delay via a real-world validation experiment in the appendix (\S\ref{subsec:eval:e2e}).


% To compare \name and the baselines under different network scenarios, we implemented a packet-level network simulator. 
% The simulator uses a drop tail queue with a configurable queue length to simulate packet losses caused by the congestion. It implements the token bucket algorithm to simulate the bandwidth variation at a frequency of 0.1 seconds.
% To determine the target bitrate of the video codecs used during simulation, we implemented Google congestion control~\cite{carlucci2016analysis} (\textit{GCC}), the standard congestion control algorithm used in WebRTC. %and the congestion control from~\cite{salsify} (\textit{Sal-CC}). 

% During the runtime, the simulator takes as input a bandwidth trace and a video. It {\em emulates} the {\em end-to-end} real-time video communication application, including encoding, packetization, sending rate adaptation, and decoding. The encoder is running at 25fps, matching the measurements from the state-of-the-art real-time video measurement~\cite{macmillan2021measuring}. The encoded packets are sent over a simulated network controlled by the simulator. 
% The output of the simulator includes a decoded video and the end-to-end delay of each decoded frame (including the time used for encoding and decoding). We also validated that the frame delay produced by our simulator is accurate by running a real-world validation experiment (in \S\ref{subsec:eval:e2e}).



\begin{table}[]
\footnotesize
\begin{tabular}{ccccc}
\hline
Dataset                                                  & \# of videos & Duration & Resolution       & Characteristics                                                                     \\ \hline
\begin{tabular}[c]{@{}c@{}}Kinetics~\cite{Kinetics}\end{tabular}         & 49            & 490 sec & \begin{tabular}[c]{@{}c@{}}1280$\times$720\\ 640$\times$360\end{tabular}   & \begin{tabular}[c]{@{}c@{}}Human actions and\\ interaction of objects\end{tabular}  \\ \hline
\begin{tabular}[c]{@{}c@{}}GamingVideoSet\\~\cite{barman2018gamingvideoset}\end{tabular}   & 6            & 180 sec  & 1920$\times$1080  & \begin{tabular}[c]{@{}c@{}}High quality PC \\ game recordings\end{tabular} \\ \hline
UVG~\cite{mercat2020uvg}                                                      & 5            & 120 sec  & 1920$\times$1280 & \begin{tabular}[c]{@{}c@{}}HD videos (human, \\ nature, sports, etc)\end{tabular}   \\ \hline
FVC~\cite{FVCDATASET}                                                      & 6            & 135 sec  & 1920$\times$1080 & \begin{tabular}[c]{@{}c@{}}Video calls \\ (indoor and outdoor)\end{tabular}         \\ \hline
Total                                                    & 66           & 925 sec  &                  &                                                                                     \\ \hline
\end{tabular}
\vspace{0.3cm}
\tightcaption{Dataset description 
% \jc{YIHUA: 3. add citation, 4. in text, add a link to the data repo (github). ask zhengxu (anonymized)}
 }
 \vspace{-0.8cm}
\label{tab:dataset}
\end{table}

\mypara{Network traces and test videos}
We test \name and the baselines on 16 real bandwidth traces, eight of which are LTE traces from the Mahimahi network-emulation tool~\cite{netravali2015mahimahi} (we filtered out the traces having an average bandwidth lower than 1Mbps),
and the rest are broadband traces from FCC~\cite{fcc-dataset}.
By default, we set the one-way propagation delay to 100ms and the queue size to 25 packets. We will also vary these values to show their impact in \S\ref{subsec:eval:e2e}.

Our evaluation uses 66 videos randomly sampled from three public datasets, and each video is at least 10 seconds. 
%The video content includes human actions in different environments, video game recordings, nature scenes, sports, as well as indoor and outdoor video calls. 
The detailed description of the datasets is in Table~\ref{tab:dataset}.
These videos, distinct from the training set, allow us to thoroughly assess the generalization capabilities of autoencoders. They encompass various spatial and temporal dynamics (discussed in \S\ref{app:siti}), across multiple resolutions, ensuring a minimum of 5 videos per resolution. The reported performance constitutes an average across all video frames.
%Table~\ref{sec:??} summarizes the datasets.
% Importantly, we choose these videos because they are different from the training set, allowing us to stress-test the generalization of autoencoders.
% These videos cover a range of spatial and temporal dynamics (details are shown in \S\ref{app:siti}), 
% and also cover multiple resolutions, with at least 5 videos in each resolution. 
% The performance is reported as an average across all the frames in the videos.
% \fyy{The video dataset can be justified briefly, leaving details to the appendix.}


\begin{figure}[t!]
     \centering
     \includegraphics[width=1\linewidth]{figs/ssim-loss-v4.pdf}
     \vspace{-0.2cm}
     \tightcaption{\name's loss resilience for different bitrates and different number of lossy frames.}
     \label{fig:loss_by_bitrate}
     \vspace{-0.1cm}
\end{figure}

\begin{figure}[t!]
    \centering
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/ssim-bpp-k360.pdf}
    %     \tightcaption{SSIM vs. bit per pixel for Kinetics dataset, 360P videos}
    %     \label{fig:}
    %     % \vspace*{3mm}

    % \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/psnr-bpp-k360.pdf}
    %     \tightcaption{PSNR vs. bit per pixel for Kinetics dataset 360P videos}
    %     \label{fig:}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/ssim-bpp-k720.pdf}
    %     \tightcaption{SSIM vs. bit per pixel for Kinetics dataset 720P videos}
    %     \label{fig:}

    % \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/psnr-bpp-k720.pdf}
    %     \tightcaption{PSNR vs. bit per pixel for Kinetics dataset 720P videos}
    %     \label{fig:}
    % \end{subfigure}
    \begin{subfigure}[t]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/ssim-bpp-kall.pdf}
        \tightcaption{SSIM vs. bitrate for Kinetics dataset}
        \label{fig:}
        % \vspace*{3mm}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/ssim-bpp-game.pdf}
        \tightcaption{SSIM vs. bitrate for gaming dataset}
        \label{fig:}
        % \vspace*{3mm}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.48\linewidth}
        \vspace*{3mm}

        \includegraphics[width=\linewidth]{figs/ssim-bpp-fvc.pdf}
        \tightcaption{SSIM vs. bitrate for FVC dataset}
        \label{fig:}
    \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/psnr-bpp-fvc.pdf}
    %     \tightcaption{PSNR vs. bit per pixel for FVC dataset}
    %     \label{fig:}
    % \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{figs/ssim-bpp-uvg.pdf}
        \tightcaption{SSIM vs. bitrate for UVG dataset}
        \label{fig:}
    \end{subfigure}
    % \begin{subfigure}[b]{0.48\linewidth}
    %     \includegraphics[width=\linewidth]{figs/psnr-bpp-uvg.pdf}
    %     \tightcaption{PSNR vs. bit per pixel for UVG dataset}
    %     \label{fig:}
    % \end{subfigure}
    \vspace*{4mm}

    \tightcaption{Quality-size tradeoff of \name.}
    \vspace{-0.1cm}
    \label{fig:psnr-vs-bpp}
\end{figure}


\mypara{Metrics}
Following the prior studies about real-time video communication~\cite{rudow2023tambur, salsify} and user QoE~\cite{garcia2019understanding, garcia2020assessment, ammar2016video}, we measure the performance of a video session in the following three aspects.
\begin{packeditemize}
    \item {\em Quality}: is measured by frame-level SSIM, reported as the average across received frames. Conforming to recent related work~\cite{salsify}, we express SSIM values in dB (obtained by $-10log(1 - SSIM)$.)
    %{\em Quality} of a video is measured by frame-level SSIM, and we report the average value across received frames. Following the recent related work~\cite{salsify}, we report the SSIM values in dB\footnote{We use $-10 * log(1 - SSIM)$ to calculate the corresponding dB values.}. 
    \item {\em Realtimeness} is measured via the tail of end-to-end frame delay and the ratio of non-rendered frames. End-to-end frame delay represents the time from encoding commencement to decoding completion. Non-rendered frames are those undecoded or late-arriving (over 200ms after the previous frame), and thus not displayed by the receiver.
    %is measured by the tail of end-to-end frame delay and the ratio of non-rendered frames. End-to-end frame delay means the time lapse between the beginning of encoding and the end of decoding. Non-rendered frames refer to frames that are not played by the receiver due to not being decodable or arriving too late (more than 200ms after the previous frame).
    \item {\em Smoothness} of the video is measured by the count and the ratio of video stalls, where a video stall is defined as the fraction of inter-frame gaps that exceed a threshold. Following the previous work~\cite{macmillan2021measuring} and the logic in WebRTC, we set the threshold to 200ms. We report the average count of video stalls per second, and the ratio of video stalls is defined as the percentage of time that the video is spent in the stalls.
    %We choose this threshold as it matches the definition in WebRTC. 
\end{packeditemize}





% \mypara{Test videos}
% Our evaluation uses 60 videos randomly sampled from three public datasets (Kinetics~\cite{Kinetics}, UVG~\cite{mercat2020uvg} and FVC~\cite{FVCDATASET}), each video is at least 10 seconds. The detailed description is in Table~\ref{tab:dataset}.
% %Table~\ref{sec:??} summarizes the datasets.
% Importantly, we choose these videos because they are different from the training set, allowing us to stress-test the generalization of autoencoders.
% The FVC dataset includes 5 videos captured from video conferencing, one of \name's main target use cases.
% These videos cover a range of spatial and temporal dynamics (\S\ref{app:siti})
% and cover multiple resolutions, %(640$\times$360, 1280$\times$720 and 1920$\times$1280)
% with at least 5 videos in each resolution. 
% The performance is reported as an average across all the frames in the videos.



%\mypara{Baselines}
%We compare the performance of \name with multiple state-of-the-art real-time video techniques that use different combinations of video coding and congestion control algorithms: 
%\begin{packeditemize}
%\item {\em Reference:} H.26x with adaptive FEC and GCC
%\item {\em Salsify:}
%\item {\em Idealized SVC:}
%\end{packeditemize}



% \yihua{add the real-world validation here: encoding/decoding pipeline running in real-time and measure the latency to show that our system is actually runnable.}



\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=4\linewidth]{figs/gccstall-queue25-delay50-long.pdf}
         \tightcaption{One-way delay = 50ms}
         \label{fig:gcc-50-25}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay75.pdf}
         \tightcaption{One-way delay = 75ms}
         \label{fig:gcc-75-25}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay100.pdf}
         \tightcaption{One-way delay = 100ms}
         \label{fig:gcc-100-25}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.24\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay100.pdf}
         \tightcaption{One-way delay = 150ms}
         \label{fig:gcc-150-25}
     \end{subfigure}
     \hfill
     \vspace{0.5cm}
     \tightcaption{End-to-end simulation result under different one-way delay. Network queue length = 25 packets}
     \label{fig:gcc-delay-simulation}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=4\linewidth]{figs/gccstall-queue15-delay100-long.pdf}
         \tightcaption{Queue = 15 packets}
         \label{fig:gcc-100-15}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/gccstall-queue25-delay100.pdf}
         \tightcaption{Queue = 25 packets}
         \label{fig:gcc-100-25}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.24\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue35-delay100.pdf}
         \tightcaption{Queue = 35 packets}
         \label{fig:gcc-100-35}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.24\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/gccstall-queue45-delay100.pdf}
         \tightcaption{Queue = 45 packets}
         \label{fig:gcc-100-45}
     \end{subfigure}
     \hfill
     \vspace{0.5cm}
     \tightcaption{End-to-end simulation result under different network queue lengths. One-way delay = 100ms}
     \label{fig:gcc-queue-simulation}
\end{figure*}


\tightsubsection{Coding efficiency and loss resilience}
\label{subsec:eval:resilience}

\mypara{Loss resilience of \name}
%Figure~\ref{fig:loss_by_bitrate} compares \name with the baseline codecs under different packet loss rates. \edit{We apply packet losses for $N$ consecutive frames and calculated the decoded quality of the lossy frames. Figure~\ref{fig:loss_by_bitrate} shows the result when $N=1,3,5$.}
We first compare \name with the baseline codecs under different packet loss rates. \edit{We apply packet losses for $N$ consecutive frames and calculated the decoded quality of the lossy frames. Figure~\ref{fig:loss_by_bitrate} shows the result when $N=1,3,5$.}
% when encoding videos from Table~???\ref{tab:dataset}.
In each figure, all lines have almost the same encoding bitrate with differences controlled within 5\%.
We ensure that \name's encoded bitrate is {\em never} higher than the baselines, so even if the actually encoded bitrate is different, it does not favor \name. Figure~\ref{fig:decoded-example} shows an example to visualize the behavior of \name under packet loss.

The most salient feature of \name is the graceful quality degradation with more packet losses. 
The average SSIM drop is only 1 dB to 3 dB under 20\% and 50\% packet losses among all the bitrates. 
Even when the loss ratio is as high as 80\%, \name can still have an average SSIM of 12 dB across different bitrates, which is much better than H.264 with various FEC redundancy rates. It also significantly outperforms SVC, because if a packet from the lower layer is lost, all the higher layers will not be decodable. %for the reasons elaborated in \S\ref{subsec:eval:e2e}.

We further contrast \name with alternative decoder-side error concealment baselines, encompassing a pretrained autoencoder~\cite{dvc}, \name with an untrained encoder neural network, and the machine-learning-based error concealment solution (\S\ref{subsec:eval:setup}). \name consistently surpasses these baselines by 0.8-2.4 dB higher SSIM, a result attributable to the joint encoder-decoder training process that makes it able to reconstruct pixels more accurately. Conversely, other decoder-side error concealment baselines lack this ability as their encoder is agnostic to packet losses.

In real-world scenarios, packet loss sometimes can affect multiple consecutive frames~\cite{rudow2023tambur}. Figure~\ref{fig:loss_by_bitrate}e and~\ref{fig:loss_by_bitrate}f shows the performance of \name and the baselines when $x\%$ packet losses occur across all 3 and 5 consecutive frames. When compared to other baselines, \name is capable of achieving a higher SSIM, up to 2 dB, covering different loss rates between 10\% and 80\%. %We have excluded FEC and SVC from Figure~\ref{fig:loss_by_bitrate}c and~\ref{fig:loss_by_bitrate}d, as it becomes inconsequential to compute the quality of subsequent frames if preceding ones are undecodable.

\mypara{Coding efficiency of \name} 
% For any loss-resilient schemes, 
There is always a tradeoff between compression and loss resilience, and \name is no exception. 
We assessed \name's quality under zero packet loss, juxtaposed with H.264 and H.265, utilizing test videos from Table~\ref{tab:dataset}. 
As indicated in Figure~\ref{fig:psnr-vs-bpp}, \name aligns closely with H.264 and marginally underperforms H.265. 
In comparison with the baseline (Tambur applying a constant 50\% redundancy to tolerate up to 50\% packet losses), \name offers a superior quality-bitrate trade-off, implying improved video quality at identical bitrates. Furthermore, \name spans a broad bitrate range across all datasets, from 0.25Mbps to over 10Mbps.
% We compare the \name's quality under no packet loss with that of H.264 and H.265 across the test videos from Table~\ref{tab:dataset} (all of which are different from the training set).
% Figure~\ref{fig:psnr-vs-bpp} shows that \name is similar to H.264 and is only slightly worse than H.265. 
% Compared to the baseline that always adds a 50\% rate FEC (tolerates up to 50\% packet losses), \name has a better tradeoff between quality and bitrate, which means it can deliver better-quality video when sending at the same bitrate compared to the baseline.
% It also shows that \name can cover a wide range of bitrates among all datasets, from 0.25Mbps to more than 10Mbps. 
% This enables more flexible bitrate adaptation when running \name.





%\jc{
%\begin{itemize}
%    \item by bitrate
%    \item by video set
%    \item psnr vs. bitrate
%\end{itemize}
%}

% \jc{need a footnote to explain why intra-mb insertion is so bad}








\tightsubsection{Video quality vs. realtimeness/smoothness}
\label{subsec:eval:e2e}

% To determine the target bitrate of the video codecs used during simulation, we implemented two different congestion control algorithms: Google congestion control~\cite{carlucci2016analysis} (\textit{GCC}, the standard congestion control used in WebRTC) and the congestion control from~\cite{salsify} (\textit{Sal-CC}). 
%We also implemented FEC-protected H.265 and Salsify codec as the baseline codecs (\S\ref{subsec:eval:setup}).

% Figure~\ref{fig:gcc-delay-simulation} and Figure~\ref{fig:gcc-queue-simulation} 
\name's loss resilience and the ability to decode incomplete frames make it achieve a better quality vs realtimeness or smoothness tradeoff than the baselines, as it does not require any retransmission. 

We evaluated \name against baselines in terms of average quality (SSIM) and video stall ratio using LTE traces under various network delays (ranging from 50ms to 150ms) and queue lengths (spanning 15 to 45 packets). 
As depicted in Figures~\ref{fig:gcc-delay-simulation} and~\ref{fig:gcc-queue-simulation}, \name significantly reduces the video stall ratio compared to the baselines. Under all network conditions, \name maintained a video stall ratio below 0.5\%, while the baselines ranged from 2\% to 16\%. 

The primary cause of video stalls is congestion-induced packet loss. When packets are lost, Salsify must skip frames, resulting in increased delay, while H.265 awaits retransmission of lost packets, increasing delay and competing with regular video traffic. 
Although Tambur has a much smaller video freeze ratio, matching the results in their paper, it does not solve the fundamental limitation of FEC-based solution: when unpredictable congestion losses are higher than the protection rate, it still causes significant video stalls.
SVC and Voxel also wait for retransmission if the base layer is damaged or a crucial frame is lost. \name, however, can decode a frame as long as any packet from that frame is received.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.325\linewidth}
         \centering
         \includegraphics[width=3\linewidth]{figs/tail-latency-long.pdf}
         \tightcaption{Tail frame latency}
         \label{fig:tail-latency}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.325\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/non-rendered-frames.pdf}
         \tightcaption{non rendered frames}
         \label{fig:non-rendered-frames}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.325\linewidth}
         \centering
         % \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay100.pdf}
         \includegraphics[width=\linewidth]{figs/frequency-of-stalls.pdf}
         \tightcaption{Average stalls per second (\name is less than 0.001)}
         \label{fig:frequency-of-stalls}
     \end{subfigure}
     \hfill
     \vspace{0.3cm}
     \tightcaption{End-to-end simulation result, comparing \name with other baselines on various metrics of realtimeness and smoothness.}
     \label{fig:other-metrics}
\end{figure}

\begin{figure}[t!]
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=2\linewidth]{figs/fcc-gccdelay-queue25-delay100-long.pdf}
         \tightcaption{SSIM vs. non-rendered frame ratio, using FCC dataset}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/fcc-gccstall-queue25-delay100.pdf}
         \tightcaption{SSIM vs. video stall ratio using FCC dataset}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \vspace{0.4cm}
     \tightcaption{\name also outperforms the baselines when using network traces from FCC dataset}
     \vspace{-0.1cm}
     \label{fig:fcc-simulation}
\end{figure}


\name also attains an average SSIM comparable to the Salsify or H.265 codecs (with or without Tambur), ranging between 15.5dB and 16dB across varied network conditions. 
SVC and Voxel exhibit a marginally lower SSIM, as packet losses inflict greater damage on them compared to \name.
Although error concealment techniques mitigate the stall ratio, they fall short in quality when compared to \name, which also corroborates the results in \S\ref{subsec:eval:resilience}. 
It is noteworthy that the machine-learning-based error concealment approach we employ already surpasses traditional methods, such as those implemented in H.264, in terms of reconstruction quality~\cite{zhou2010efficient, varsa2001non}. 
%However, most machine-learning-based error concealment solutions, to the best of our knowledge, necessitate a minimum of hundreds of milliseconds for error concealment, which is a duration incompatible with the latency requirements of real-time video streaming.

Though \name's SSIM is on par or slightly lower than some baselines, we believe that the reduction in frame delay and stall ratio is worth the minor drop in quality. This is confirmed by our user study later.


Figure~\ref{fig:other-metrics} compares \name with the baselines on other realtimeness and smoothness metrics with the one-way delay set to 100ms and the queue length set to 25 packets.
For clarity, we only put the baselines with comparable average SSIM in this figure (without Voxel and error concealment).
Despite maintaining similar video quality, \name surpasses these baselines by reducing the 98 percentile frame delay by a factor of 2-5$\times$.
As evidenced in Figure~\ref{fig:non-rendered-frames}, \name only fails to render 0.2\% of frames, far superior to the 4-10\% non-rendered frames exhibited by the baselines.
Additionally, Figure~\ref{fig:frequency-of-stalls} demonstrates that \name experiences few video stalls, thereby markedly outperforming all baselines.

    


% \mypara{Impact of bandwidth distributions}
We also run the simulation based on the broadband traces from FCC dataset~\cite{fcc-dataset}. Compared to the LTE traces, broadband traces have similar average bandwidth but fewer bandwidth drops. We run the simulation with a propagation delay of 100ms and a droptail queue of 25 packets. %and use GCC as the congestion control algorithm. 
Figure~\ref{fig:fcc-simulation} shows that \name still has a better trade-off between video quality and the ratio of delayed frames and video freezes than the baselines. 

% \mypara{Ablation study of key components} 
% We then conduct an ablation study by removing per-packet entropy coding (\S\ref{??}) and loss-resilience training (\S\ref{??}). 
% We run the experiment using Sal-CC with the same one-way delay and queue length as in Figure~\ref{fig:normal-simulation}. 



Finally, Figure~\ref{fig:timeseries-ours} shows a concrete example of \name's behavior.
% compare \name and the baselines in a concrete bandwidth trace sample to illustrate why it can achieve a better tradeoff (Figure~\ref{fig:timeseries-ours}).
The bandwidth drops from 8Mbps to 2Mbps at 1.5sec and last for 800ms, before bouncing back to 8Mbps (another bandwidth drop occurs at 3.5sec).
During each bandwidth drop, \name's delay does not increase as sharply as the baselines (notably Salsify is the second best since it could skip frames while H.265 needs to wait for the retransmission).
\name and Salsify use the same CC, so their quality roughly matches on frames not skipped by Salsify.
That said, \name's quality degrades marginally with no frame skipping during congestion, limiting the drop of SSIM to less than 4 dB when there are more than 10 consecutive frames experiencing packet loss over 60\%. 
With the help of the resync logic (\S\ref{sec:delivery}), \name's quality bounces back soon (within 1 RTT) after packet losses disappear. 


% When we run \name with the models trained without any packet losses, the average SSIM will be decreased from \fillme dB to \fillme dB. This is because the frame quality will be significantly decreased when packet loss happens.


\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    %\includegraphics[width=1.05\linewidth]{figs/timeseries-new.pdf}
    \includegraphics[width=0.68\linewidth]{figs/timeseries-vertical.pdf}
    \tightcaption{\name achieves lower delay and decent quality during sudden bandwidth drops: the delay is lower compared to both baselines, and it can render more frames than Salsify without skipping or retransmission.}
    \label{fig:timeseries-ours}
\end{figure}

\begin{figure}[t!]
    \centering
    % \includegraphics[width=0.8\linewidth]{figs/timeseries-placeholder.png}
    \includegraphics[width=0.8\linewidth]{figs/user-study-new.pdf}
    \tightcaption{Comparing \name with Salsify and H.265 (with FEC or Tambur) by user study}
    \label{fig:user-study}
\end{figure}


\mypara{User study of video quality} 
% To show decreasing the ratio of delayed frames and video freezes is worth the minor drop in quality for real users, 
To validate \name's improvement on real-world users, we set up a user study website and gathered 960 user video ratings with Amazon MTurk~\cite{mturk} (IRB approved) in 240 sessions. 
We sampled 8 video clips (spanning cloud gaming, real-time sports events, daily human activities, and video conferencing) rendered by \name, Salsify codec, and H.265 using basic FEC or Tambur with the same setup as the simulation. 
(Appendix~\ref{fig:user-study-screenshot} shows a screenshot of each video.)
The sampled videos have the same distribution of quality, realtimeness, and smoothness as Figure~\ref{fig:gcc-delay-simulation}. 
% , and the user study is properly randomized following the steps described in \cite{sensei}.
When an MTurk user signs up for the user study, the user will be randomly assigned to rate their user experience (with a Likert scale of 1-5) on the videos rendered by different methods. 
Figure~\ref{fig:user-study} shows the mean opinion score (MOS) of each video. 
The result confirms that the videos rendered by \name are more favored by real users.

% with the average MOS across videos from 2.6 to 3.6 compared to the baselines.



 

%In Figure~???????????????????????????\ref{??}, we use three metrics for video quality, even though our autoencoders are trained to optimize L2-norm between the reconstructed and original images, which is similar to RGB-PSNR, their quality compared to baselines is similar under different metrics.

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_traceset_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_rtt_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_queue_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/eval_e2e_by_cc_placeholder.pdf}
%    \caption{}
%    \label{fig:}
%\end{figure*}


%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=1.pdf}
%    \caption{Aggressiveness = 1}
%    \label{fig:}
%\end{figure*}
%
%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.85\linewidth]{figs/psnr_vs_delay_ag=0.75.pdf}
%    \caption{Aggressiveness = 5}
%    \label{fig:}
%\end{figure*}








% \jc{YIHUA, please fill in some detailed reading}

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/encoding-lat-gpu.pdf}
%          \caption{Encoding latency on A100 GPU}
%          \label{fig:gpu-encoding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/encoding-lat-cpu.pdf}
%          \caption{Encoding latency on CPU}
%          \label{fig:gpu-decoding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/decoding-lat-gpu.pdf}
%          \caption{Decoding latency on A100 GPU}
%          \label{fig:cpu-encoding}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/decoding-lat-cpu.pdf}
%          \caption{Decoding latency on CPU}
%          \label{fig:cpu-decoding}
%      \end{subfigure}
%      \hfill
%      \tightcaption{Compute overhead of \name.}
%      \label{fig:computing-overhead}
% \end{figure} 

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.195\linewidth}
         \centering         \includegraphics[width=\linewidth]{figs/encoding-lat-gpu-new.pdf}
         \tightcaption{Encoding latency on A40 GPU}
         \label{fig:gpu-encoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/encoding-lat-copies-gpu-new.pdf}
         \tightcaption{Total latency to encode multiple copies of different bitrates}
         \label{fig:gpu-multi-encoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/decoding-lat-gpu-new.pdf}
         \tightcaption{Decoding latency on A40 GPU}
         \label{fig:gpu-decoding}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/encoding-lat-cpu-new.pdf}
         \tightcaption{Encoding latency on CPU}
         \label{fig:cpu-encoding}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.195\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/decoding-lat-cpu-new.pdf}
         \tightcaption{Decoding latency on CPU}
         \label{fig:cpu-decoding}
     \end{subfigure}
     \hfill
     \vspace{0.4cm}
     \tightcaption{Compute overhead of \name. \passed{\zy{in figure b, Graco should be 32.1ms, 33.1ms, 34.1ms; in figure d, Grace for 720p should be 22.7ms}}}
     \label{fig:computing-overhead} 
\end{figure*} 

% \begin{figure}[t!]
%      \begin{subfigure}[b]{0.48\linewidth}
%          \centering
%          \includegraphics[width=2\linewidth]{figs/cpu-gccdelay-queue25-delay100-long.pdf}
%          \caption{SSIM vs. delayed frame ratio}
%          \label{fig:queue15-psnr-stall}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.48\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/cpu-gccstall-queue25-delay100.pdf}
%          \caption{SSIM vs. video stall ratio}s
%          \label{fig:queue15-ssim-delay}
%      \end{subfigure}
%      \hfill
%      \vspace{-0.1cm}
%      \tightcaption{End-to-end simulation results for CPU version \name \zy{missing legend for the black dot}}
%      \label{fig:simulation-ablation}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%          \centering
%         %\includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
%         \includegraphics[width=0.7\linewidth]{figs/cpu e2e.pdf}
%          \label{fig:}
%          \vspace{.05cm}
%     \tightcaption{CPU end to end result. \textcolor{red}{TODO: Ziyi and Hanchen}}
%     \label{fig:cpu-simulation}
% \end{figure}

\tightsubsection{Computational overhead}
\label{subsec:eval:system}

% \zy{There is a typo ("decodeing latency") on the y-axis label on Figure 16 (b). (figs/decode.pdf)}

% Remember that \name needs a P-frame encoder and a I-frame encoder to encode each frame as a P-frame and an I-patch (a small spatial region without reference).
%\mypara{Computational overhead}
% We test the encoding/decoding speed of un-optimized \name, optimized \name (\S\ref{subsec:fast-coding}) and H.264 from \texttt{ffmpeg} on a Linux server with an A100 GPU and Intel Xeon Silver 4210R CPU (32 threads).
% Figure~\ref{fig:gpu-encoding} and Figure~\ref{fig:gpu-decoding} show the encoding and decoding speed on GPU. With the optimizations, \name can encode and decode a 720P frame in 34.9ms and 15.5ms respectively, which is 1.5$\times$ and 2$\times$ faster than the unoptimized version. This translates to 28fps and 35fps for encoding and decoding 720P frames. 
% For 480P videos, optimized \name can encode/decode in 25.3 and 15.4ms, which equals to 40fps and 65fps for encoding and decoding.
We test \name's encoding/decoding speed with and without the optimizations in \S\ref{subsec:fast-coding}, and H.265 from \texttt{ffmpeg} on our testbed (equipped with Nvidia A40 GPU and Intel Xeon 4216 CPU with \review{32} threads). 
From Figure~\ref{fig:gpu-encoding} to 
Figure~\ref{fig:gpu-decoding}, we can see that with the optimization, \name is capable of encoding and decoding a 720P frame in 32.1ms and 22.7 ms, respectively. This equates to frame rates of 31.2~fps and 44.1~fps for encoding and decoding 720P frames, respectively. 

% Figure~\ref{fig:cpu-encoding} and Figure~\ref{fig:cpu-decoding} shows our optimizations on CPU can significantly reduce the encoding and decoding time. For 720P videos, the original model takes 5217ms and 3996ms to encode and decode a frame, while the time decreases to 35.1ms and 40.9ms after applying our optimizations. This shows that with our optimization, \name is able to stream the 720P video purely using CPU.
% Compared with the GPU version of \name, the optimized CPU version has a lower SSIM of 0.8 dB. However, it does not impact the improvement in the ratio of delayed frames. %, and the quality is not bad compared to the error concealment baseline.

As illustrated in Figure~\ref{fig:cpu-encoding} and Figure~\ref{fig:cpu-decoding}, our CPU optimizations significantly curtail encoding and decoding times. For 720P videos, the initial model necessitated 5217ms and 3996ms to encode and decode a frame, respectively; however, these times were dramatically reduced to 35.1ms and 40.9ms following our optimization. This demonstrates that \name, with our optimization, is capable of streaming 720P video using the CPU alone. Despite the optimized CPU version of \name exhibiting a marginally lower SSIM of 0.5 dB compared to its GPU counterpart (Figure~\ref{fig:simulation-ablation}), this discrepancy does not compromise the improvement in the ratio of delayed frames.

It is worth noting that \name is 1.5-5$\times$ faster than the recent autoencoder-based video codec: Swift~\cite{swift} requires more than 100ms to encode a frame. RLVC~\cite{yang2020learning} has a comparable encoding speed with DVC~\cite{dvc}, but still 1.5$\times$ slower than ours. AlphaVC~\cite{shi2022alphavc} needs several hundred milliseconds to encode a single frame, which is more than 5$\times$ slower than \name.

% \begin{figure}[t!]
%     \centering
%          \centering
%         %\includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
%         \includegraphics[width=0.7\linewidth]{figs/encoding-multiple-version.png}
%          \label{fig:system-encoding-versions}
%          \vspace{.05cm}
%     \tightcaption{Encoding latency of encoding multiple versions \textcolor{red}{TODO: Yihua}}
%     \label{fig:multiple-encoding}
% \end{figure}

\mypara{\name's fast bitrate adaptation}
Figure~\ref{fig:gpu-multi-encoding} shows \name's latency while encoding multiple frame copies at varying bitrates (\S\ref{subsec:fast-coding}). Given that the most time-intensive portion of encoding is shared across models, the additional time required to encode multiple versions is minimal, averaging merely 1.05ms per extra copy for 720p video (0.5ms for 480p). Consequently, \name can encode three distinct copies within 34.1ms, enabling the bitrate control as described in \S\ref{subsec:fast-coding}. Empirically, we found that over 65\% of frames require a single encoding pass, while 34\% need a second pass to adjust to the target bitrate. A marginal subset, less than 1\%, is subjected to a third encoding pass.

\tightsubsection{Microbenchmarking}
\label{subsec:eval:micro}

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[t]{0.48\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/burst-loss.pdf}
%          \caption{50\% of packet loss is applied to frame 6, 7, 8}
%          \label{fig:queue15-psnr-stall}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.48\linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figs/long-loss.pdf}
%          \caption{10\%, 30\%, 50\% packet loss is applied on {\em every} frame after 6-th frame}
%          \label{fig:queue15-psnr-stall}
%      \end{subfigure}
%     \tightcaption{The detailed behavior of \name under different kind of losses.}
%     \label{fig:loss-behavior}
% \end{figure}

\begin{figure}[t!]
     \begin{subfigure}[t]{0.48\linewidth}
         \centering
         \includegraphics[width=2\linewidth]{figs/abl-gccdelay-queue25-delay100-long.pdf}
         \tightcaption{SSIM vs. non-rendered frame ratio, using different versions of \name}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/abl-gccstall-queue25-delay100.pdf}
         \tightcaption{SSIM vs. video stall ratio, using different versions of \name}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \vspace{0.5cm}
     \tightcaption{Ablation study (per packet EC, loss resilience) }
     \label{fig:simulation-ablation}
\end{figure}




% \mypara{Detailed behavior of \name under loss}
% Figure~\ref{fig:loss-behavior} shows that if there is a transient packet loss, the quality of the following frames will not keep degrading. When the packet losses are persistent, \name can still deliver good quality for more than 10 frames, without needing any synchronization between the encoder and the receiver.



\mypara{Ablation study}
We also conducted an ablation test using the following variants of \name: CPU version of \name (\S\ref{subsec:fast-coding}), \name without per-packet entropy coding (\S\ref{subsec:packetization}), \name without jointly training encoder and decoder (only trained decoder), and \name without training with packet loss.

Figure~\ref{fig:simulation-ablation} shows the impact of the optimizations proposed in~\S\ref{subsec:fast-coding} for speeding up CPU encoding/decoding (the yellow circle). 
The average SSIM decreased from 15.8 dB to 15.3 dB after applying the CPU-related optimizations, and the optimizations do not affect the realtimeness and smoothness of the decoded video much.
We can also see that both the delayed frame ratio and the stall ratio will increase if \name does not use per-packet entropy coding described in \S\ref{subsec:packetization} (the red cross). 
This is because, without it, the size of the encoded frame will have an increase of 1.5$\times$, and this size increase may overload the network when bandwidth suddenly drops. 
%It also shows without training with loss, the pretrained autoencoder models will suffer from quality drops caused by packet loss. The SSIM will drop from 15.8dB to 12.4dB compared to \name.

Without loss-resilience training, pretrained autoencoder models experience significant quality degradation due to packet loss, with the SSIM dropping from 15.8 dB to 12.4 dB in comparison to \name. 
Moreover, solely fine-tuning the decoder with loss is insufficient, resulting in a quality drop from 15.8dB to 13.9dB. 
This can be attributed to the decoder's difficulty in recovering accurate content without redundancy in the encoded frame when there is no redundancy in it. 
By training the encoder and decoder jointly, the encoder learns to incorporate redundancy, aiding the decoder in correctly restoring lost information.

\mypara{Working with super-resolution}
In line with the discussion in \S\ref{subsec:related}, Super-Resolution (SR) can supplement the receiver-side video quality. We employed SwinIR~\cite{liang2021swinir}, a leading SR model, in our simulation to confirm that \name, like baselines, can also leverage SR benefits. Our experiments demonstrated that SR boosts receiver-side quality for all codecs, irrespective of the specific codec employed. For more details, refer to Appendix~\ref{app:sr}.
% As discussed in \S\ref{subsec:related}, SR can be used as a complementary tool to enhance the video quality at the receiver side. 
% We use SwinIR~\cite{liang2021swinir}, a state-of-the-art SR model in our simulation to validate \name can also benefit from SR the same as baselines.
% Our experiments shows that SR can improve the quality for any codecs at the receiver side, agnostic to what codec is being used.
% Due to size constrain, we put more details into Appendix~\ref{app:sr}.





% Figure~\ref{fig:gpu-encoding} shows the encoding latency for \name to encode multiple different copies of frames with different bitrates (\S\ref{subsec:fast-coding}). Since the models share the most time-consuming part of the encoding, the overhead of encoding multiple versions is negligible: only 2.6ms for every extra copy. Therefore, \name can encode 3 different copies in 40.9ms, allowing the encoder to do bitrate adaptation in real-time.
% Empirically in our study, over 65\% frames will only be encoded once and 34\% frames will be encoded twice to adapt to the target bitrate. Less than 1\% frames will be encoded 3 times. 
% Figure~\ref{??} shows the effectiveness of our bitrate controlling algorithm (\S\ref{??}). Over \fillme\% of frames will falls in the range of $[0.8, 1]\times$ target bitrate and it will never produce a frame that overshoots the target bitrate.

% \mypara{Model training decisions}
% To validate the design choices of loss distribution we used during model training, we conduct an ablation study of different loss distributions. We test two different setups: (i) the probability of using 0 loss is the same as other loss rates, and (ii) loss rates as high as 80\% and 90\% are added during training. As shown in Figure~???\ref{fig:training-loss-study}, both setups can cause the SSIM under 0 loss decrease around \fillme dB. 
% When the probability of 0 loss is low, the model will learn to deprioritize the quality under 0 loss, which will impact the average video quality. We also observe that seeing a loss as high as 80\% or 90\% will also damage the quality under 0 loss.


% Our implementation of \name optimizes both memory footprint and encoding/decoding delay (described in \S???\ref{subsec:optimize}), and we test its effectiveness on a Nvidia GeForce RTX 3080 GPU. 
% Figure~???\ref{fig:system-encoding} and Figure~???\ref{fig:system-decoding} show that compared to the original (unoptimized) implementation of pre-trained autoencoder (which takes 100ms to encode a 480p frame), our implementation can encode a 480p frame in less than 25ms (a 4×4\times speedup).\footnote{The only autoencoder that achieves comparable encoding/decoding speed is~\cite{elf}, and it achieves such speed on a 5x more expensive Titan V GPU. We hope to compare it with \name, but it is not open-source.}
% This translates to almost 40fps. 
% Even for 720p HD videos, our optimized codec can achieve 18fps (55ms encoding per frame). 
% % \fillme~fps/\fillme~fps, \name encodes/decodes 480p frames at \fillme~fps/\fillme~fps, a \fillme×\times speedup.
% This acceleration comes from downsampling frames in motion-vector estimation. 
% Moreover, when adapting to a target bitrate, \name encodes the next frame multiple times {\em without} needing to run the entire encoder multiple times, because it re-uses the motion-compensated prediction, so only the residuals need to be encoded at multiple bitrates. Figure~??????\ref{fig:system-encoding-versions} shows that the delay of encoding a frame at three different bitrates only increases marginally compared to encoding one frame. 







% In terms of memory usage, our optimized implementation saves the memory footprint of loading 9 models by over 60\% since most NN layers are shared. 
% % Figure~??????\ref{??} shows that compared to loading the multiple autoencoders (I-frame encoder/decoder and a P-frame encoder/decoder of each bitrate) in GPU memory, the memory usage \name's autoencoders (not including the memory usage of intermediate features) is \fillme\% smaller, because they share most of the layers (only the last \fillme layers of the encoder and the first \fillme layers of the decoders are different). 
% Note that \name does not change the NN architecture of the autoencoders---only the weights are retrained and the way they are used is optimized. We speculate that they could be made more efficient with appropriate modification to its NN architecture.

% Figure~??????\ref{??} validate that \name's coding efficiency is comparable to (even slightly better than) without the optimizations (\ie without sharing the NN backbone or downsampling and sharing the motion-vectors.)
% This is because, though quality does drop with these optimizations, the encoded size also drops (due largely to the downsampled motion vectors), which result in a similar bitrate-quality trade-off frontier.

% \jc{The only autoencoder that achieves comparable encoding/decoding speed is Elf~\cite{??}. 
% We hope to compare it with \name, but it is not open-source. }


% \jc{remember to highlight that the speed is comparable to elf, which runs on the 5x more expensive titan v gpu.}

% \begin{figure}[t!]
%     \centering
%          \centering
%         \includegraphics[width=0.7\linewidth]{figs/psnr-vs-bpp-all.pdf}
% %        \includegraphics[width=0.7\linewidth]{figs/a.pdf}
%          \label{fig:}
%          \vspace{.05cm}
%     \tightcaption{Training curve study \textcolor{red}{put into appendix}}
%     \label{fig:training-loss-study}
% \end{figure}
%!TEX root = ../main.tex
%!TEX spellcheck = en_US



==> sections/old/intro-nsdi-v1.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\section{Introduction}

Real-time video communication has become an integral part of our daily
lives~\cite{blum2021webrtc}, spanning online
conferences~\cite{webrtc-vc-1,webrtc-vc-2},
cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2},
interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2},
and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
To ensure a high quality of experience (QoE) for users,
real-time video applications must protect against
packet losses\footnote{Our notion of packet losses refers to both packets
dropped in transit and those not received by the decoding deadline.}.
However, retransmitting lost packets across high-latency networks
is not feasible due to stringent real-time latency requirements~\cite{itu-g114}.

To recover packet losses without retransmission,
existing solutions broadly adopt two strategies~\cite{wang2000error,wang1998error}.
First, encoder-side forward error correction (FEC) schemes~\cite{wicker1999reed}
incorporate redundancy in data before transmission.
A redundancy rate of $R\%$, the percentage of redundant packets relative to
the total data size, can recover up to $R\%$ of lost data.
Nevertheless, determining the optimal $R$ value involves forecasting the packet
loss rate, posing a practical challenge.
%Under the same bandwidth, a larger $R$ is more resilient
%to packet losses but also entails lower video quality.
%Furthermore, video is no longer decodable when the loss rate exceeds $R$.
Second, decoder-side error concealment reconstructs
portions of a video frame compromised by packet losses.
%In recent years, error concealment has largely evolved from traditional 
%image processing techniques (e.g., interpolation) into 
%learning-based generative methods (e.g., inpainting~\cite{kang2022error}).
Implementing error concealment, however, requires partitioning a video frame 
into independently decodable units (e.g., slices~\cite{XXX} or tiles~\cite{XXX}),
resulting in reduced compression efficiency.
In \S\ref{subsec:related}, we discuss other strategies that are not specifically
designed for loss resilience but can be repurposed to tolerate packet loss,
such as scalable video coding (SVC) and super resolution.
% We show that they either sacrifice coding efficiency when there are no
% packet losses, or fail to decode video or retain video quality under high packet losses.
% \yc{This section is clear, but it didn't explain what are the problems of the existing solutions.}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.6\columnwidth]{intro-illustration.pdf}
  \caption{Illustration of the video quality achieved by
  different loss-resilient schemes, operating under the same bandwidth budget,
  across varying packet loss rates.}
  \label{fig:intro-example}
  \vspace{-10pt}
\end{figure}

In this paper, we present \name, a learning-based video system designed for
loss resilience, preserving video quality across a wide range of packet losses.
Our key insight is that jointly optimizing the encoder and decoder
under a spectrum of simulated packet losses considerably strengthens loss resilience.
\fyy{Alternate flow: here seems to be a natural place to compare with
the existing encoder-only and decoder-only approaches, referencing to Figure 1.
Then start a new paragraph to talk about how Grace works at a high level.}
To facilitate the joint optimization, \name leverages the latest advances in neural
video codecs~\cite{dvc} and integrates neural networks into the core components
of a conventional encoder and decoder (rather than replacing them entirely).
\edit{To add packet loss in the training of the neural video codec, 
\name randomly partitions the encoder's output into different packets so that a lost packet will render the values in its partition to zeros in the decoder's input.
During training, \name sees a wide spectrum of packet losses, ranging from 0\% to 60\%.}
\fyy{There is a missing link between using neural codec (above) to the amazing
performance of Grace (below). Think about how to transition.}
\fyy{This paragraph is central to intro, but 1) the motivation
for using neural video codecs is still weak (I used "To facilitate the joint optimization" for lack
of a better reason, but hopefully there is a better reason);
2) I don't think I appreciate how packet loss is introduced exactly in this place. It sounds a little
too detailed. Instead of saying that, it would be better to describe how Grace works at a high level
(such as its workflow).}

As a result, it achieves video quality on par with traditional codecs,
such as H.265 (without FEC), in the absence of packet losses.
As the packet loss intensifies,
\name retains higher quality than state-of-the-art loss-resilient schemes,
exhibiting a more graceful degradation in quality. \S\ref{sec:core} shows more details of the training process of \name and explains why it can be loss-tolerant. 
In Figure~\ref{fig:intro-example}, we illustrate the superiority of \name over
other loss-resilient schemes within the same bandwidth budget.
Unlike encoder-based FEC, \name neither requires predicting the
packet loss rate prior to transmission, nor suffers from a sharp collapse
in decodability as the loss rate escalates.
A video frame produced by \name remains decodable at \textit{any} loss rate
(unless all packets are lost), with its quality progressively improving as
more packets are received.
When compared with decoder-based error concealment,
\name avoids sacrificing compression efficiency upfront for error resilience
and consistently yields higher video quality under varying losses. 
%\fyy{After reading the following paragraphs, I think the above two paragraphs
%(paraphrased from the previous version) are too eager to introduce all the benefits
%of Grace, without letting the reader taste how it works, or appreciate how
%challenging it is to get there.}
\fyy{I merged the design goals and benefits of Grace into this single paragraph,
but the text needs to be shortened.}

\edit{
Jointly optimizing the encoder and decoder under a spectrum of packet losses enables \name's neural video codec to have a more graceful quality degradation under packet losses.
However, in order to make the end-to-end video system fully embrace such capability from the \name's codec, there are still three main system challenges.
{\em (i)} The packetizer of \name should allow packets to be individually decodable and guarantee the effect of losing one packet is equivalent to randomly zeroing values in the encoder's output. 
{\em (ii)} The video system should efficiently synchronize the encoder and decoder states to avoid video stream corruption after packet loss ends.
{\em (iii)} \name should be efficient enough to encode/decode videos in real time on resource-constrained devices like laptops and mobile phones.
}

\edit{
\name addresses the above challenges with the following designs.
\begin{packeditemize}
    \item (\S\ref{subsec:packetization}) \name uses a new packetization scheme that {\em randomly} partitions the encoder's output before entropy encoding each partition into a separate packet. 
    Therefore, each packet is individually decodable, and the impact of a lost packet is mapped to the random erasure of values in the encoder's output.
    \name also regularizes the neural network encoder during training so that the random partition scheme does not have the compression efficiency reduction problem like the error concealment solutions.
    \item (\S\ref{subsec:protocol}) We design a new protocol for \name to re-synchronize the encoder and decoder states without retransmission. 
    When getting the packet loss feedback from the decoder, the encoder quickly re-decodes the recent frames as seen by the decoder to align its state with the decoder and such re-decoding only requires 7\% of the encoding time.
    \item (\S\ref{subsec:fast-coding}) \name embraces the latest hardware acceleration techniques including OpenVINO~\cite{openvino} and CoreML~\cite{coreml} to speed up the neural network inference on CPUs and mobile devices. 
    \name also trains multiple encoders that produce different encoded bitrates but share most computation, making it possible to encode a frame at multiple bitrates with negligible overhead.
\end{packeditemize}
}

% \name's neural video codec provides the basis for the loss tolerance. 
% \fyy{What basis? Avoid vague language. Here is probably the place to set the stage
% first for neural video codec: I would describe why choose
% neural video codec in Grace and what it can already do.
% Then go on to say what it cannot do.}
% However, there are still two challenges in order to make the whole video system loss-resilient. 
% First, each packet should be independently decodable, regardless of the loss of any other packets.
% Most of the traditional codecs such as H.265 and VP9 do not meet this requirement.
% This is because they use entropy coding to compress the encoded video before splitting the data into packets,
% resulting in entropy decoding failure when packet loss happens.
% \yc{think about how to phrase this more like a challenge instead of a requirement. The complexity is from doing per-packet entropy encode without size inflation.}
% Second, the video system needs to efficiently synchronize the encoder and decoder states after packet loss to prevent error propagation.
% \fyy{It is unclear why synchronization of states is required. "Error" is not defined.}
% Reconstruction errors will accumulate when using decoder-side error concealment techniques
% \fyy{Why mention "error concealment" here? Confusing.}, 
% and such errors will keep affecting the frame quality after the packet loss ends (it is also known as error propagation~\cite{??}).
% In order to mitigate the errors, existing solutions either need to retransmit the lost packets or send a new keyframe to refresh the video stream, 
% both incurring a significant overhead in bandwidth. \fyy{Retransmitting lost packets
% should not incur a high bandwidth overhead. This is confusing.}

% \name addresses the above challenges. 
% It uses a new packetization scheme that partitions the encoder's output tensor
% \fyy{pay attention to newly introduced concepts as "tensor" has not been introduced
% earlier.} before entropy encoding each partition into a separate packet (\S\ref{subsec:packetization}).
% It also regularizes the neural network encoder during training so that such a scheme does not cause significant size inflation.
% We also design a new protocol for \name to re-synchronize the encoder and decoder states without the need for retransmission or a new keyframe (\S\ref{subsec:protocol}).
% \fyy{Overall, the descriptions of both two challenges seem too long, with details unsuitable
% for the intro. In contrast, the solutions are too short. I don't understand it without
% more details.}


% To use neural video codecs for real-time video applications, another important concern is 
% that neural networks are usually too heavy to run on client devices efficiently.
% \fyy{Is this simply the third challenge?.}
% \name uses two optimizations to improve the efficiency of video encoding and decoding (\S\ref{subsec:fast-coding}). 
% First, \name trains multiple pre-trained encoders that produce different encoded bitrates but share most computation.
% Therefore, \name can encode a frame at multiple bitrates with negligible overhead and pick the encoded bitrate most similar to the target bitrate at runtime. 
% \yc{maybe consider saying neural video codecs are not good at bitrate adaptation since it may require multiple-pass inference? Otherwise, it sounds like coming from nowhere.}
% Second, \name embraces the latest hardware acceleration techniques including OpenVINO~\cite{openvino} and CoreML~\cite{coreml} to speed up the neural network inference on CPUs and mobile devices.


\fyy{Think about if the reader needs to know all these details and key results. Usually not in the intro. Just bring the last paragraph here and use a few sentences to describe results highlights. Similar to what I did in the abstract.} 
We have implemented \name and evaluated it by transmitting videos covering a range of content genres (all different from the training set) over real network traces (\S\ref{sec:eval}).
\edit{
Comparison between \name and a spectrum of state-of-the-art loss-resilient schemes shows that 
it reduces undecodable frames by 95\% and stall duration by 90\% compared with FEC, 
and boosts video quality over error concealment by 3~dB of SSIM. 
Our IRB-approved user study shows \name has a 38\% higher mean opinion score (MOS), further attesting to its effectiveness.
\name can also encode and decode efficiently on resource-constrained devices: \fillme and \fillme fps for 720{p} video on an iPhone 14 Pro at drop of only \fillme dB in SSIM.
}

% {\em (i)} forward error concealment (Tambur~\cite{rudow2023tambur}), 
% {\em (ii)} postprocessing error concealment by neural-net in-painting~\cite{xiang2019generative}, 
% {\em (iii)} scalable video coding (Swift~\cite{swift}), and
% {\em (iv)} selective frame skipping (Voxel~\cite{voxel} and Salsify~\cite{salsify}).
% Our key results are: 
% \begin{packeditemize}
%   \item \name achieves better quality, by 1.4-4 dB of SSIM\footnote{The definition of SSIM dB is in \S\ref{subsec:eval:setup}}, than other loss-resilient schemes at the same packet loss (between 20\% and 80\%) and bitrate (between 0.8Mbps and 4.8Mbps). 
  
%   \item \name achieves a similar average quality (in SSIM) with the codec used in WebRTC at the same bitrate. In other words, \name does not sacrifice quality when there is no packet loss. 
  
%   \item When different loss-resilient schemes are run on real network traces
%   \footnote{To be fair, we run \name and the baselines over the same congestion control (CC) algorithm, GCC~\cite{carlucci2016analysis}, which is the standard CC used in WebRTC.}
%   , \name reduces undecodable frames by 95\% and stall duration by 90\% compared with FEC; 
%   it also significantly boosts video quality over error concealment---without notably affecting other metrics in both comparisons.
  
%   \item With much less video stuttering and fewer skipped frames, our IRB-approved user study confirms that \name has \review{38}\% higher mean opinion score (MOS) than the most competitive loss-resilient schemes.
  
%   \item On a single Nvidia A40 GPU, \name can decode 480p and 720p at 120~fps and 44.1~fps, respectively and encode 480p and 720p at 87.7~fps and 31.2~fps, respectively, which is 1.5-5$\times$ faster than recent video autoencoders. 
%   On an iPhone 14 Pro, it can encode 720{p} videos at 41~fps (on par with GPU-based implementation) at only a drop of 0.5 dB in SSIM. \yc{the fps is higher than it should be, because we didn't consider the time to get h264 mv on iphone}
  
% \end{packeditemize}

To put \name's contribution in perspective, neural video codecs have long been used in multimedia, but \name is, to our best knowledge, the first to jointly train generative NN encoder and decoder to improve loss resilience in real-time video.
\name is closely related to using NNs to generatively reconstruct the missing data in lost packets, but they do not jointly train the encoder for loss resilience (\eg~\cite{sankisa2018video,reparo}) or handle only special content type at low resolution~\cite{reparo}.
\name is also related to but different from an emergent technique~\cite{kurka2020deepjscc,bourtsoulatze2019deep,gunduz2019machine} which trains autoencoders to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss).
\fyy{After the intro, the reader should know how Grace works at a high level.
I definitely don't feel like knowing its workflow after reading the intro,
e.g., what happens during training and inference, respectively?}
\fyy{The last paragraph is fine but breaks the flow in my opinion. I usually prefer to state the contributions first, including "Grace is the first work to ...", before providing the results highlights.}


% \begin{itemize}
%     \item A loss-tolerant video system should deal with the following challenges: 
%     \begin{itemize}
%         \item Each packet of a frame should be independently decodable regardless of other frames -- we have per-packet entropy coding for this
%         \item Should be able to sync the states between sender and receiver to prevent error propagation -- we have state synchronization protocol
%     \end{itemize}
%     \textit{(emphasize \name is not just a NN, but a video system)}

%     \item Challenges to make NN being practical for realtime video applications
%     \begin{itemize}
%         \item too heavy for edge devices to run -- our CPU optimization for edge devices
%         \item bitrate adaptation (need to find some citations) -- backbone sharing for faster bitrate adaptation
%     \end{itemize}
%     \textit{(we are not too heavy)}

%     \item We have implemented and evaluated \name on XXX and compared it against YYY baselines. Here are the key results
%     \begin{itemize}
%         \item similar average quality (not sacrificing quality)
%         \item better quality than EC, lower stall/delay than FEC
%         \item Higher user score
%         \item Fast inference speed to match real time requirement
%     \end{itemize}

%     \item Key contribution: {\em jointly} train encoder and decoder  {\em with loss}.
% \end{itemize}
%This enhanced resilience can be attributed to \name's exposure to packet
%losses during training, which steers it to transform video into a loss-resistant
%space.

==> sections/old/intro-nsdi-v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\section{Introduction}

Real-time video communication has become an integral part of our daily
lives~\cite{blum2021webrtc}, spanning online
conferences~\cite{webrtc-vc-1,webrtc-vc-2},
cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2},
interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2},
and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
To ensure a high quality of experience (QoE) for users,
real-time video applications must protect against
packet losses\footnote{Our notion of packet losses refers to both packets
dropped in transit and those not received by the decoding deadline.}.
However, retransmitting lost packets across high-latency networks
is not feasible due to stringent real-time latency requirements~\cite{itu-g114}.

To recover packet losses without retransmission,
existing solutions broadly adopt two strategies~\cite{wang2000error,wang1998error}.
First, encoder-side forward error correction (FEC) schemes~\cite{wicker1999reed}
incorporate redundancy in data before transmission.
A redundancy rate of $R\%$, the percentage of redundant packets relative to
the total data size, can recover up to $R\%$ of lost data.
Nevertheless, determining the optimal $R$ value involves forecasting the packet
loss rate, posing a practical challenge.
%Under the same bandwidth, a larger $R$ is more resilient
%to packet losses but also entails lower video quality.
%Furthermore, video is no longer decodable when the loss rate exceeds $R$.
Second, decoder-side error concealment reconstructs
portions of a video frame compromised by packet losses.
%In recent years, error concealment has largely evolved from traditional 
%image processing techniques (e.g., interpolation) into 
%learning-based generative methods (e.g., inpainting~\cite{kang2022error}).
\edit{However, error concealment techniques may fail to accurately reconstruct the missing information, especially when objects have unpredictable motions or a new object appears.}
Moreover, implementing error concealment requires partitioning a video frame 
into independently decodable units (e.g., slices~\cite{XXX} or tiles~\cite{XXX}),
resulting in reduced compression efficiency.
In \S\ref{subsec:related}, we discuss other strategies that are not specifically
designed for loss resilience but can be repurposed to tolerate packet loss,
such as scalable video coding (SVC) and super resolution.
% We show that they either sacrifice coding efficiency when there are no
% packet losses, or fail to decode video or retain video quality under high packet losses.
% \yc{This section is clear, but it didn't explain what are the problems of the existing solutions.}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.6\columnwidth]{intro-illustration.pdf}
  \caption{Illustration of the video quality achieved by
  different loss-resilient schemes, operating under the same bandwidth budget,
  across varying packet loss rates.}
  \label{fig:intro-example}
  \vspace{-10pt}
\end{figure}

In this paper, we present \name, a learning-based video system designed for
loss resilience, preserving video quality across a wide range of packet losses.
In Figure~\ref{fig:intro-example}, we illustrate the superiority of \name over
other loss-resilient schemes within the same bandwidth budget.
Unlike encoder-based FEC, \name neither requires predicting the
packet loss rate prior to transmission, nor suffers from a sharp collapse
in decodability as the loss rate escalates.
A video frame produced by \name remains decodable at \textit{any} loss rate
(unless all packets are lost), with its quality progressively improving as
more packets are received.
When compared with decoder-based error concealment,
\name avoids sacrificing compression efficiency upfront for error resilience
and consistently yields higher video quality under varying losses. 
% \fyy{I merged the design goals and benefits of Grace into this single paragraph,
% but the text needs to be shortened.}

% \fyy{Alternate flow: here seems to be a natural place to compare with
% the existing encoder-only and decoder-only approaches, referencing to Figure 1.
% Then start a new paragraph to talk about how Grace works at a high level.}

\fyy{The next paragraph is central to intro, but 1) the motivation
for using neural video codecs is still weak (I used "To facilitate the joint optimization" for lack
of a better reason, but hopefully there is a better reason);
2) I don't think I appreciate how packet loss is introduced exactly in this place. It sounds a little
too detailed. Instead of saying that, it would be better to describe how Grace works at a high level
(such as its workflow).}

Our key insight is that {\em jointly optimizing the encoder and decoder
under a spectrum of simulated packet losses} considerably strengthens loss resilience.
To facilitate the joint optimization, \name leverages the latest advances in neural
video codecs~\cite{dvc} and integrates neural networks into the core components
of a conventional encoder and decoder (rather than replacing them entirely).
By jointly optimizing the encoder and decoder, rather than only the decoder, \name's encoder learns to add redundancy to the information that is critical to the frame quality, enabling a better reconstruction than error concealment when packet loss happens.
Optimizing under a spectrum of packet losses, rather than a fixed loss rate, prevents \name from having the sharp quality collapse like the encoder-based FEC.

To simulate packet loss in the training of the neural video codec, values in the encoder's output are randomly zeroed before feeding to the decoder.  
During the inference, \name randomly partitions the encoder's output into different packets so that packet loss has the same effect on the encoder's output as during training.
\S\ref{sec:core} shows more details of the training process of \name and explains why it can be loss-tolerant. 
% \name is trained with a wide spectrum of packet loss, ranging from 0\% to 60\%. 
% As a result, it achieves video quality on par with traditional codecs,
% such as H.265 (without FEC), in the absence of packet losses.
% As the packet loss intensifies,
% \name retains higher quality than state-of-the-art loss-resilient schemes,
% exhibiting a more graceful degradation in quality. 

% \edit{To add packet loss in the training of the neural video codec, 
% \name randomly partitions the encoder's output into different packets so that a lost packet will render the values in its partition to zeros in the decoder's input.
% During training, \name sees a wide spectrum of packet losses, ranging from 0\% to 60\%.}
% \fyy{There is a missing link between using neural codec (above) to the amazing
% performance of Grace (below). Think about how to transition.}




Jointly optimizing the encoder and decoder under a spectrum of packet losses enables \name's neural video codec to have a more graceful quality degradation under packet losses.
However, in order to make the end-to-end video system fully embrace such capability from the \name's codec, there are still three main system challenges.
{\em (i)} The packetizer of \name should allow packets to be individually decodable and guarantee the effect of losing one packet is equivalent to randomly zeroing values in the encoder's output. 
{\em (ii)} The video system should efficiently synchronize the encoder and decoder states to avoid video stream corruption after packet loss ends.
{\em (iii)} \name should be efficient enough to encode/decode videos in real time on resource-constrained devices like laptops and mobile phones.


\name addresses the above challenges with the following designs.
\begin{packeditemize}
    \item (\S\ref{subsec:packetization}) \name uses a new packetization scheme that {\em randomly} partitions the encoder's output before entropy encoding each partition into a separate packet. 
    Therefore, each packet is individually decodable, and the impact of a lost packet is mapped to the random erasure of values in the encoder's output.
    \name also regularizes the neural network encoder during training so that the random partition scheme does not have the compression efficiency reduction problem like the error concealment solutions.
    \item (\S\ref{subsec:protocol}) We design a new protocol for \name to re-synchronize the encoder and decoder states without retransmission. 
    When getting the packet loss feedback from the decoder, the encoder quickly re-decodes the recent frames as seen by the decoder to align its state with the decoder and such re-decoding only requires 7\% of the encoding time.
    \item (\S\ref{subsec:fast-coding}) Contrary to existing neural video codecs that rely on complex neural networks for motion prediction, \name leverages the motion prediction capabilities of conventional codecs such as H.264, thereby substantially reducing encoding overhead.
    \name also trains multiple encoders that produce different encoded bitrates but share most computation, making it possible to encode a frame at multiple bitrates with negligible overhead.
    %\name embraces the latest hardware acceleration techniques including OpenVINO~\cite{openvino} and CoreML~\cite{coreml} to speed up the neural network inference on CPUs and mobile devices. 
\end{packeditemize}

% \name's neural video codec provides the basis for the loss tolerance. 
% \fyy{What basis? Avoid vague language. Here is probably the place to set the stage
% first for neural video codec: I would describe why choose
% neural video codec in Grace and what it can already do.
% Then go on to say what it cannot do.}
% However, there are still two challenges in order to make the whole video system loss-resilient. 
% First, each packet should be independently decodable, regardless of the loss of any other packets.
% Most of the traditional codecs such as H.265 and VP9 do not meet this requirement.
% This is because they use entropy coding to compress the encoded video before splitting the data into packets,
% resulting in entropy decoding failure when packet loss happens.
% \yc{think about how to phrase this more like a challenge instead of a requirement. The complexity is from doing per-packet entropy encode without size inflation.}
% Second, the video system needs to efficiently synchronize the encoder and decoder states after packet loss to prevent error propagation.
% \fyy{It is unclear why synchronization of states is required. "Error" is not defined.}
% Reconstruction errors will accumulate when using decoder-side error concealment techniques
% \fyy{Why mention "error concealment" here? Confusing.}, 
% and such errors will keep affecting the frame quality after the packet loss ends (it is also known as error propagation~\cite{??}).
% In order to mitigate the errors, existing solutions either need to retransmit the lost packets or send a new keyframe to refresh the video stream, 
% both incurring a significant overhead in bandwidth. \fyy{Retransmitting lost packets
% should not incur a high bandwidth overhead. This is confusing.}

% \name addresses the above challenges. 
% It uses a new packetization scheme that partitions the encoder's output tensor
% \fyy{pay attention to newly introduced concepts as "tensor" has not been introduced
% earlier.} before entropy encoding each partition into a separate packet (\S\ref{subsec:packetization}).
% It also regularizes the neural network encoder during training so that such a scheme does not cause significant size inflation.
% We also design a new protocol for \name to re-synchronize the encoder and decoder states without the need for retransmission or a new keyframe (\S\ref{subsec:protocol}).
% \fyy{Overall, the descriptions of both two challenges seem too long, with details unsuitable
% for the intro. In contrast, the solutions are too short. I don't understand it without
% more details.}


% To use neural video codecs for real-time video applications, another important concern is 
% that neural networks are usually too heavy to run on client devices efficiently.
% \fyy{Is this simply the third challenge?.}
% \name uses two optimizations to improve the efficiency of video encoding and decoding (\S\ref{subsec:fast-coding}). 
% First, \name trains multiple pre-trained encoders that produce different encoded bitrates but share most computation.
% Therefore, \name can encode a frame at multiple bitrates with negligible overhead and pick the encoded bitrate most similar to the target bitrate at runtime. 
% \yc{maybe consider saying neural video codecs are not good at bitrate adaptation since it may require multiple-pass inference? Otherwise, it sounds like coming from nowhere.}
% Second, \name embraces the latest hardware acceleration techniques including OpenVINO~\cite{openvino} and CoreML~\cite{coreml} to speed up the neural network inference on CPUs and mobile devices.


% \fyy{Think about if the reader needs to know all these details and key results. Usually not in the intro. Just bring the last paragraph here and use a few sentences to describe results highlights. Similar to what I did in the abstract.} 
% We have implemented \name and evaluated it by transmitting videos covering a range of content genres (all different from the training set) over real network traces (\S\ref{sec:eval}).

\name is closely related to using NNs to generatively reconstruct the missing data in lost packets, but they do not jointly train the encoder for loss resilience (\eg~\cite{sankisa2018video,reparo}) or handle only special content type at low resolution~\cite{reparo}.
\name is also related to but different from an emergent technique~\cite{kurka2020deepjscc,bourtsoulatze2019deep,gunduz2019machine} which trains autoencoders to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss).

This paper makes following key contributions:
\begin{packeditemize}
    \item We present \name, which is, to our best knowledge, the first to jointly train generative NN encoder and decoder under a spectrum of packet losses to improve loss resilience in real-time video (\S\ref{sec:core}).
    \item We propose technical optimizations to enable the use of neural video codec in the real-time video system, addressing practical challenges including packetization, encoder/decoder state synchronization, and runtime efficiency (\S\ref{sec:delivery}).
    \item Comprehensive experiments (\S\ref{sec:eval}) on real network traces and a diverse set of videos show that \name reduces undecodable frames by 95\% and stall duration by 90\% compared to baselines using FEC,  and boosts video quality over baselines using error concealment by 3~dB of SSIM. 
Our IRB-approved user study attests to \name's effectiveness by showing it has a 38\% higher mean opinion score (MOS).
\name also achieves more than 40~fps on resource-constrained devices such as iPhone 14 Pro, matching the requirement of real time videos.
\end{packeditemize}


% To put \name's contribution in perspective, neural video codecs have long been used in multimedia, but \name is, to our best knowledge, the first to jointly train generative NN encoder and decoder to improve loss resilience in real-time video.
% Our evaluation results (\S\ref{sec:eval}) show that \name reduces undecodable frames by 95\% and stall duration by 90\% compared with FEC, 
% and boosts video quality over error concealment by 3~dB of SSIM. 
% Our IRB-approved user study attests to \name's effectiveness by showing it has a 38\% higher mean opinion score (MOS).
% \name also achieves more than 40~fps on resource-constrained devices such as iPhone 14 Pro, matching the requirement of real time videos.

\fyy{After the intro, the reader should know how Grace works at a high level.
I definitely don't feel like knowing its workflow after reading the intro,
e.g., what happens during training and inference, respectively?}
\fyy{The last paragraph is fine but breaks the flow in my opinion. I usually prefer to state the contributions first, including "Grace is the first work to ...", before providing the results highlights.
}
% Comparison between \name and a spectrum of state-of-the-art loss-resilient schemes shows that 
% it reduces undecodable frames by 95\% and stall duration by 90\% compared with FEC, 
% and boosts video quality over error concealment by 3~dB of SSIM. 
% Our IRB-approved user study shows \name has a 38\% higher mean opinion score (MOS), further attesting to its effectiveness.
% \name can also encode and decode efficiently on resource-constrained devices: \fillme and \fillme fps for 720{p} video on an iPhone 14 Pro at drop of only \fillme dB in SSIM.

% {\em (i)} forward error concealment (Tambur~\cite{rudow2023tambur}), 
% {\em (ii)} postprocessing error concealment by neural-net in-painting~\cite{xiang2019generative}, 
% {\em (iii)} scalable video coding (Swift~\cite{swift}), and
% {\em (iv)} selective frame skipping (Voxel~\cite{voxel} and Salsify~\cite{salsify}).
% Our key results are: 
% \begin{packeditemize}
%   \item \name achieves better quality, by 1.4-4 dB of SSIM\footnote{The definition of SSIM dB is in \S\ref{subsec:eval:setup}}, than other loss-resilient schemes at the same packet loss (between 20\% and 80\%) and bitrate (between 0.8Mbps and 4.8Mbps). 
  
%   \item \name achieves a similar average quality (in SSIM) with the codec used in WebRTC at the same bitrate. In other words, \name does not sacrifice quality when there is no packet loss. 
  
%   \item When different loss-resilient schemes are run on real network traces
%   \footnote{To be fair, we run \name and the baselines over the same congestion control (CC) algorithm, GCC~\cite{carlucci2016analysis}, which is the standard CC used in WebRTC.}
%   , \name reduces undecodable frames by 95\% and stall duration by 90\% compared with FEC; 
%   it also significantly boosts video quality over error concealment---without notably affecting other metrics in both comparisons.
  
%   \item With much less video stuttering and fewer skipped frames, our IRB-approved user study confirms that \name has \review{38}\% higher mean opinion score (MOS) than the most competitive loss-resilient schemes.
  
%   \item On a single Nvidia A40 GPU, \name can decode 480p and 720p at 120~fps and 44.1~fps, respectively and encode 480p and 720p at 87.7~fps and 31.2~fps, respectively, which is 1.5-5$\times$ faster than recent video autoencoders. 
%   On an iPhone 14 Pro, it can encode 720{p} videos at 41~fps (on par with GPU-based implementation) at only a drop of 0.5 dB in SSIM. \yc{the fps is higher than it should be, because we didn't consider the time to get h264 mv on iphone}
  
% \end{packeditemize}

% To put \name's contribution in perspective, neural video codecs have long been used in multimedia, but \name is, to our best knowledge, the first to jointly train generative NN encoder and decoder to improve loss resilience in real-time video.
% \name is closely related to using NNs to generatively reconstruct the missing data in lost packets, but they do not jointly train the encoder for loss resilience (\eg~\cite{sankisa2018video,reparo}) or handle only special content type at low resolution~\cite{reparo}.
% \name is also related to but different from an emergent technique~\cite{kurka2020deepjscc,bourtsoulatze2019deep,gunduz2019machine} which trains autoencoders to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss).
% \fyy{After the intro, the reader should know how Grace works at a high level.
% I definitely don't feel like knowing its workflow after reading the intro,
% e.g., what happens during training and inference, respectively?}
% \fyy{The last paragraph is fine but breaks the flow in my opinion. I usually prefer to state the contributions first, including "Grace is the first work to ...", before providing the results highlights.}


% \begin{itemize}
%     \item A loss-tolerant video system should deal with the following challenges: 
%     \begin{itemize}
%         \item Each packet of a frame should be independently decodable regardless of other frames -- we have per-packet entropy coding for this
%         \item Should be able to sync the states between sender and receiver to prevent error propagation -- we have state synchronization protocol
%     \end{itemize}
%     \textit{(emphasize \name is not just a NN, but a video system)}

%     \item Challenges to make NN being practical for realtime video applications
%     \begin{itemize}
%         \item too heavy for edge devices to run -- our CPU optimization for edge devices
%         \item bitrate adaptation (need to find some citations) -- backbone sharing for faster bitrate adaptation
%     \end{itemize}
%     \textit{(we are not too heavy)}

%     \item We have implemented and evaluated \name on XXX and compared it against YYY baselines. Here are the key results
%     \begin{itemize}
%         \item similar average quality (not sacrificing quality)
%         \item better quality than EC, lower stall/delay than FEC
%         \item Higher user score
%         \item Fast inference speed to match real time requirement
%     \end{itemize}

%     \item Key contribution: {\em jointly} train encoder and decoder  {\em with loss}.
% \end{itemize}
%This enhanced resilience can be attributed to \name's exposure to packet
%losses during training, which steers it to transform video into a loss-resistant
%space.

==> sections/old/intro-nsdi24.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}

Real-time video communication has a long history in research, yet only recently has it become truly widespread in our daily lives~\cite{blum2021webrtc}.
RTC (and WebRTC clients) has become the de-facto platform for real-time videos, just like HTTP and DASH is for streaming videos, enabling more and more new applications~\cite{webrtc-trend-1,webrtc-trend-2}, from online meetings~\cite{webrtc-vc-1,webrtc-vc-2}, cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2}, to interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2} and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
%The amount of time people spend on real-time videos grow faster than the time spent on watching streaming videos~\cite{webrtc-trend-1,webrtc-trend-2}.





%Compared to streaming videos (over HTTP), such as video-on-demand, users are at least as susceptible to video stuttering and poor quality when using real-time video applications (\eg video conferencing and online gaming). 
%However, real-time video clients use a very short buffer in order to render each frame as soon as they are received.
%For instance, the buffer in WebRTC is merely 10s of ms~\cite{10.1145/3410449}; in contrast, HTTP-based streaming videos, even live sports event, have a buffer of at least 10 seconds. 
%To make it worse, long latencies and bandwidth fluctuations remain across wide-area networks and cellular networks, causing occasional packet loss and latency jitter. 
%Waiting/retransmitting a single packet can take 100s ms or longer and block multiple frames, causing video stuttering.
%Thus, loss-resilient video coding, which can tolerate any packet loss rate\footnote{To avoid ambiguity, we define {\em the packet loss rate on a frame} as the fraction of its packets not received before the receiver decodes the frame, \eg every 50ms at 20 frames per second (fps).
%A packet can be lost due to packet drops, queuing delay or out-of-order delivery, and the missing packets can be consecutive or random.}, is crucial for real-time videos.

Yet, users of real-time video applications still has poor experience due to video stalls, low visual quality or frequent quality switches~\cite{10.1145/3487552.3487842, webrtc-performance}. 
This is because the nature of real-time applications requires the clients to have a very short buffer, \eg tens of milliseconds in WebRTC~\cite{10.1145/3410449}\footnote{In contrast, HTTP-based streaming videos, even live sports events, have a buffer of at least 10 seconds, allowing streaming video players to retransmit packets without causing video stalls. 
%However, this is not possible for RTC-based real-time video clients.
}. 
%\passed{\amz{This should read as "tens of milliseconds" not "ten seconds of milliseconds", right?}}
This means that resending {\em any} packet, especially in long-latency networks, will block the decoding of multiple frames and cause video stalls.
Hence, it is crucial to tolerate packet loss, especially since packet drops and high latency jitters remain common across wide-area and cellular networks.
% Unfortunately, packet drops and high latency jitter remain common across wide-area networks and cellular networks.
% Therefore, it is crucial for real-time video coding to tolerate packet loss.
Here, we define {\em packet loss} on a given frame as any packets not received before the receiver decodes the frame.
%, \eg every 50ms at 20 frames per second (fps).
Packet loss can be consecutive or random and can result from packet drops or latency jitter.\footnote{It is important to clarify that our notion of packet loss rate is {\bf\em not} the traditional network-level loss rate. Even if a packet is not dropped, it can still be counted as a packet loss, if it arrives too late. It is not rare for real-time video clients to have a high (over 50\%) packet loss rate on some frames, even if the network has a very low packet drop rate. Our definition of packet loss rate is consistent with recent papers~\cite{rudow2023tambur,google-doc-fec}.}
%queuing delay or out-of-order delivery.
% \passed{\jc{rewrote to tune down the contrast with vod. see if it's better}}
% \passed{\fyy{I wouldn't contrast RTC with video-on-demand streaming. Their differences are well understood, and the comparison wastes the precious space in the first page.}}

%Yet, users are at least as susceptible to video stuttering and poor quality when using real-time video applications (\eg video calls and online gaming) as when watching on-demand videos (\eg Netflix). 
%% Despite intensive research on congestion control and bitrate adaptation~\cite{salsify,sprout} for Internet videos, 
%Long latencies and bandwidth fluctuations remain across wide-area networks and cellular networks.
%% , such as long-distance video calls. 
%To make it more challenging, real-time video clients use a very short buffer (\eg merely 10 ms in WebRTC~\cite{10.1145/3410449}) to render each frame as soon as they are received. 
%Consequently, waiting/retransmitting a single packet, which could take 100s ms or longer, will block multiple frames and cause a visual stuttering.

% These packet retransmits may not be concealed by the short buffer---merely 10 ms in WebRTC~\cite{10.1145/3410449}, which allows frames to be played as soon as they are decoded.
% As a result, the extra delay to wait or resend a single packet frame, which could take 100s ms or longer in long-latency links, can block the decoding of multiple frames and cause a visual stuttering. 


\begin{comment}
might be conceal by the playback buffer in on-demand streaming videos, 
%In on-demand video streaming, the extra delay of packet retransmits (which could be 100s ms or higher in long-latency links) is easy to conceal by the video buffer, but 
this may not be true for 
real-time videos use a very short buffer (\eg merely \fillme ms in WebRTC)~\cite{??}  in order to play each frame as soon as it is decoded.
As a result, the additional delay to wait or resend a single packet frame might block the decoding of multiple frames and cause a visual stuttering. 
\end{comment}




%Despite of many loss-resilience coding schemes, they fall short in different ways. 
%% fall short at realizing DS coding. 
%First, state-of-the-art scheme based on forward error correction (FEC), such as Tambur~\cite{tambur}, can tolerate packet loss but it is difficult to set an appropriate rate of FEC redundancy. 
%To tolerate $x$\% packet loss, it must add at least $x$\% redundancy {\em before} transmission~\cite{holmer2013handling, uberti2015webrtc}, and quality will be lowered to make space for the redundancy, even if all packets turn out to be successfully received (Figure~\ref{fig:intro-example}(a)). 
%Therefore, most systems, such as WebRTC, do not add FEC redundancy by default, and increase FEC redundancy only {\em reactively}, after packet loss has affected some frames~\cite{holmer2013handling}.
%%, which requires packets to be resent until enough packets are received.
%%For these frames whose \rate is underestimated, 
%%the receiver must still request the sender to resend some packets until at least 70\% of packets have arrived.
%%Even after the packet loss has subsided, FEC may still add too much redundancy, thereby reducing  video quality.  
%%Secondly, DS may seem similar to the concepts of 
%Second, scalable video coding (SVC)~\cite{SVCFEC1} and fine granularity scalability (FGS)~\cite{ma2022deepfgs,li2001overview} in theory can improve quality as more packets are received. 
%However, these schemes split a video into a hierarchy of layers, and packet loss at a lower layer can block the decoding of higher layers (Figure~\ref{fig:intro-example}(b)).
%%and their quality increases only if packets of a higher layer received in a specific hierarchy.
%%However, there is a key difference: quality in DS coding depends on how many packets are received {\em regardless} of which packets, but SVC and FGS split video into layers and their quality increases only if more layers are received in a specific hierarchy.
%Third, receiver-side error concealment may seem promising, but in order to decode any subset of packets, it must either use FEC or split a frame into independently encoded partitions.
%As a result, it has a lower quality than traditional codec like H.265 at the same bitrate~\cite{KUMAR2006425} (Figure~\ref{fig:intro-example}(c)).



% Existing loss-resilient video coding schemes generally fall in two categories, and they each fall short in different ways. 
Two general categories of loss-resilient video coding exist, but they each fall short in different ways ~\cite{wang2000error,wang1998error}.
% https://ivpl.northwestern.edu/wp-content/uploads/2019/02/Error_resilient_video_coding_techniques.pdf, https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=664283
First, in {\em encoder-based forward} error correction, the sender adds redundancy to each frame {\em before} sending it out.
For instance, forward-error correction (FEC), which is well-studied and used in WebRTC~\cite{holmer2013handling, xiao2012dynamic}, can tolerate any $x$\% loss of packets by adding $x$\% redundancy.
However, since the redundancy must be added by the sender before knowing the packet loss rate, it is difficult to pick an appropriate amount of FEC redundancy. 
It still requires retransmission and causes video delay/stall if the redundancy is smaller than the actual packet loss, yet adding too much FEC redundancy lowers the video quality regardless of how many packets are lost. 
Because of the negative impact of FEC redundancy on quality, WebRTC and other systems do not add FEC redundancy by default and add FEC redundancy only until some frames are already affected by packet loss~\cite{holmer2013handling}. 
Second, in {\em decoder-based post-processing} error concealment, the decoder uses received data to reconstruct the regions or frames affected by packet loss.
However, the sender must sacrifice compression efficiency in order for each received packet to be independently decodable~\cite{KUMAR2006425}.
%its quality at zero packet loss is worse than traditional codec like H.265 at the same bitrate~\cite{KUMAR2006425}, because it must add redundancy bits to allow each packet to be independently decodable (Figure~\ref{fig:intro-example}(c)).
Moreover, the decoder cannot reconstruct all lost information, since the encoder is trying to include as little redundancy as possible to achieve a better compression ratio.
%As a result, its quality is lower than traditional codec like H.265 at the same bitrate~\cite{KUMAR2006425}, even when all packets are received (Figure~\ref{fig:intro-example}(c)).
\S\ref{subsec:related} will discuss more schemes that might help tolerate loss but are not designed specifically for loss resilience, such as scalable video coding, and super-resolution.
In short, these solutions either sacrifice the quality when there is no packet loss or fail to get decent quality under high packet loss rates.

% \passed{\jc{good point. SVC doesn't have to be here; it should be used to contrast DS coding later. the text is updated.}}
% \passed{\fyy{SVC is never designed to be an error-resilient scheme, and thus can be pushed back to Section 2 and related work. It is still important to mention SVC after ``we will discuss more schemes'' or explicitly explain why (e.g., it does not tolerate lost packets in its base layers), in case reviewers have it in mind and get confused. Later in Section 2/related work, is it also fair to say when evaluated from the perspective of error resilience, SVC is inferior to state-of-the-art post-processing error concealment approaches? It also needs to sacrifice compression efficiency to produce enhancement layers
% (so the starting point of Figure 1(b) is inaccurate).
% Anyway, removing SVC will make this paragraph logically easier to understand: there are ``forward'' approaches and ``post-processing'' approaches, but Grace jointly optimizes both or you can say Grace takes an unprecedented approach.}}


\begin{figure}[t!]
    \centering
        \includegraphics[width=0.83\linewidth]{figs/intro-example-illustrative-threelines.pdf}
         \tightcaption{Illustration existing loss-resilient schemes vs. this work at the same bitrate but under different packet loss rates. 
%         \name's data-scalable coding under packet loss of different \rates when compared with existing loss-resilient schemes. 
         (actual figures from our evaluation appear
later (e.g., Figures~\ref{fig:loss_by_bitrate}). 
        % \yc{just put a note here, should we add SVC in this graph? I like it but we may need to change some text?}
        \passed{\fyy{Similarly, SVC should be removed from Figure 1; otherwise, there's too much to parse. Then, one figure with three curves would suffice. Besides, DMR is not defined yet. Can you actually get rid of that and just say packet loss rate?}}
        } 
    \label{fig:intro-example}
    \vspace{-0.2cm}
    % \vspace{-0.5cm}
\end{figure}

%\begin{figure}[t!]
%    \centering
%%        \includegraphics[width=0.9\linewidth]{figs/intro-example-illustrative-short.pdf}
%        \includegraphics[width=0.99\linewidth]{figs/intro-example-illustrative-separate.pdf}
%         \tightcaption{Illustration existing loss-resilient schemes vs. this work at the same bitrate but under different packet loss rates. 
%%         \name's data-scalable coding under packet loss of different \rates when compared with existing loss-resilient schemes. 
%         (actual figures from our evaluation appear
%later (e.g., Figures~\ref{fig:loss_by_bitrate}). 
%\fyy{Similarly, SVC should be removed from Figure 1; otherwise, there's too much to parse.
%Then, one figure with three curves would suffice.
%Besides, DMR is not defined yet. Can you actually get rid of
%that and just say packet loss rate?}}
%    \label{fig:intro-example}
%    % \vspace{-0.5cm}
%\end{figure}

%\begin{figure}[t!]
%    \centering
%        \includegraphics[width=0.99\linewidth]{figs/intro-example-illustrative-old.pdf}
%         \tightcaption{(a) An example of \name's loss resilience under packet loss of different \rates, and (b) the potential quality/delay improvement by \name. These figures are illustrative; actual figures from our evaluation and trace analysis appear
%later (e.g., Figures~\ref{fig:normal-simulation}, \ref{fig:queue15-simulation}, \ref{fig:loss_by_bitrate}). }
%    \label{fig:intro-example}
%    % \vspace{-0.5cm}
%\end{figure}

% for high-quality, smooth real-time videos.

In this paper, we present \name, a new approach that {\em jointly trains a pair of neural-net (NN) encoder and NN decoder to optimize quality under a variety of packet loss rates}. 
Our insight is that by training the NN encoder and decoder under different rates of simulated packet loss (explained shortly), the resulting NN encoder and decoder forms a {\em generative autoencoder} with the following property: %that tolerates the packet loss while only marginally sacrificing the quality when there is no packet loss.
{\em (i)} With the same encoding (regardless of the packet loss rate), \name obtains quality similar to the classic codec (H.265) used in WebRTC without FEC when there is no packet loss, and {\em (ii)} as the packet loss rate raises, the quality gradually degrades but is still better than state-of-the-art loss-resilient schemes.
%In other words, \name's video quality degrade gracefully with more packet loss while only marginally sacrificing the quality when there is no packet loss. 
%training the autoencoder under various packet loss rates, the decoded video quality can {\em degrade gracefully with more packet loss while only marginally sacrificing the quality in absence of packet loss}. 
\passed{\amz{I find the phrase "in absence of packet loss" difficult to parse, and it's used often in the intro. Can you replace at least a few instances with "when there is no packet loss"?}}
We refer to it as {\em Data-Scalable} (DS) coding. 
Figure~\ref{fig:intro-example} illustrates the contrast between DS coding, encoder-based forward error correction, and decoder-based post-processing error concealment.
% \yc{should we put svc here if it's in figure 1?}
More specifically, DS coding has four practical benefits:
{\em (i)} it does not need to know the loss rate before encoding each frame, 
{\em (ii)} a frame is decodable under {\em any} packet loss rate, unless all packets are lost, 
{\em (iii)} quality gradually improves if more packets are received\footnote{Scalable video coding (SVC)~\cite{SVCFEC1} and fine granularity scalability (FGS)~\cite{ma2022deepfgs,li2001overview} in theory could also improve quality with more packets. 
However, they split a video into a hierarchy of layers, 
%and packet loss at a lower layer can block the decoding of higher layers. Thus, 
so unlike DS coding, a new packet may not always improve quality, if the lower layers are not fully received.}, and
{\em (iv)} when all packets are received, it reaches a quality similar to the traditional codec like H.265 used in WebRTC.
\passed{\amz{Item (iii) is confusingly written -- if I understood correctly after reading the footnote, "quality gradually improves as more packets are received" or "quality scales gradually as more packets are received" will be more clear.}}

%More specifically, \name encodes and decode each frame 
%%We present \name, a concrete example of this approach that encodes and decodes video frames 
%using a {\em novel antoencoder} whose encoder and decoder are neural nets (NNs).
To add packet loss in the training of its generative autoencoder, \name simulates packet loss as follows.
%jointly train the NN encoder and NN decoder under various loss rates, 
%\name simulates packet loss as follows. 
Different from traditional video codec that splits the entropy-encoded byte stream into multiple packets, \name uses a new packetization scheme that first {\em partitions} the encoder's output tensor and then {\em entropy encodes} each partition as a {\em separate} packet. 
If all packets are received, the decoder's input will be identical to the encoder's output.
If a packet is lost, the values in its partition are set to zeros (\ie {\em masked}) in the decoder's input.
During training, given a packet loss rate, \name simulates such process to zeroing out elements corresponding to the lost packets.
%By training under different rates of simulated packet loss, 
%By simulating the effect of packet loss on decoder's input, \name jointly trains the encoder and decoder NNs to optimize the decoded video quality under various rates of packet loss. 
\S\ref{sec:core} shows more details of our training process and packetization process. 
\yc{revisit this paragraph, it's not really talking about how to "simulate" the packet loss. Maybe change the first sentence?}


Once its generative autoencoder is trained, \name entails several optimizations to stream video online efficiently (\S\ref{sec:delivery}).
%entails several optimizations to stream video efficiently online (\S\ref{sec:delivery}).
%For instance, \name minimizes the size inflation caused by the design choice of entropy encoding each packet separately (rather than entropy encode the entire encoder's output). 
For instance, in order to encode each frame at a given target bitrate, \name trains multiple pre-trained 
% \yc{the word "pre-trained" is a bit confusing here, are we saying we are not doing online training?} 
encoders that produce different encoded bitrates but share most computation, so with minimum compute overhead, \name can encode a frame at multiple bitrates and then pick a encoded bitrate similar to the target bitrate. 
\name's decoder can decode a partially received frame without any retransmission, and to avoid out-of-sync coding states, \name uses a protocol to re-synchronize the encoder and decoder states. 
%When the receiver decodes a frame of partially received packets, \name uses a protocol to re-synchronize the encoder and decoder states without packet retransmission.
\name also entails optimizations to run the NN encoder and decoder on CPUs and reduce the size inflation due to per-packet entropy encoding. 

%\name's per-packet entropy encoding
\passed{\amz{This sentence is confusing, since the entropy encoding scheme is not mentioned before, so I had no context for the size inflation. Flipping the sentence ("\name entropy encodes each packet separately, so we optimized the design to minimize potential size inflation" would read easier.}}
%\name also uses a customized protocol to re-synchronize the states on the sender when the receiver decodes a frame without waiting for all packets to arrive.
%\S\ref{sec:delivery} details other optimizations, such as a way to drastically reduce autoencoder overhead (on GPUs and CPUs) and efficient bitrate control to fit the encoding bitrate to target sending rate set by congestion control.
%To make \name practical, \name also includes schemes to 
%speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{subsec:fast-coding}).








\tempstrike{
\mypara{Data-scalable (DS) coding}
We define the {\em Data Missing Rate} (\rate) of a frame as the fraction of packets not received before the  receiver decodes the frame\footnote{\rate is similar to packet loss rate defined on a single frame.}, \eg every 50ms at 20 frames per second (fps).
A packet can be missing due to packet drops, queuing delay or out-of-order delivery, and the missing packets can be consecutive or random.
{\em Without} knowing the actual \rate, an ideal loss-resilient coding scheme should encode a frame  such that
%Then {\em without} knowing the actual \rate, an ideal loss-resilient scheme should meet three criteria: 
\begin{packeditemize}
\item {\em (i)} the frame is decodable under any \rate below 100\% (\ie at least one packet is received), 
\item {\em (ii)} the quality is close to a non-loss-resilient codec (\eg H.265) when all packets are received, and
%as long as {\em any} (non-empty) subset of packets of the frame is received, 
%(\ie no need for retransmission unless all data is lost);  
\item {\em (iii)} quality degrades gracefully with higher \rate, \ie quality gradually improves if {\em any} more packets are received.
\end{packeditemize}
We call such a coding scheme {\em data-scalable} (DS).
DS coding is ideal for real-time video, because without retransmission, its quality degrades gracefully with more packet loss (higher \rate) while not sacrificing quality in absence of packet loss. 
}





\tempstrike{
Some loss-resilient scheme uses an older but reliably received frame as the reference frame, allowing the decoder to safely skip a loss-affected frame (\eg~\cite{salsify}).
%without hurting future frames, 
However, using an old reference frame means more bits to achieve the same quality as using the last frame as reference, which lowers compression efficiency.
}


%achieve high {\em compression efficiency}, which means high quality with fewer bits, and {\em loss resilience} under various data missing rate or {\em \rate} defined by
%the fraction of data that is not received, due to packet drops or queuing, before a frame is decoded.

\tempstrike{
Unfortunately, current real-time video systems achieve loss resilience by adding various forms of redundancies, thus sacrificing compression efficiency (as elaborated in \S\ref{subsec:prior}).\footnote{
Scalable video coding (SVC~\cite{SVCFEC1}, FGS~\cite{ma2022deepfgs,li2001overview}, Swift~\cite{swift}), which works well for on-demand streaming videos, will be much less effective in real-time videos which send packets of a frame together, instead of layer by layer (see \S\ref{subsec:prior}).
For this reason, scalable video coding is not commonly used to improve unicast real-time videos~\cite{salsify}. 
Similarly, selective frame skipping (\eg~\cite{voxel}) might work for on-demand videos, but in real-time videos, most frames are P-frames which cause poor quality once dropped, unless I-frames are frequently inserted.
Nonetheless, we will still evaluate them against \name.}
%\jc{add old reference frame}
}



\tempstrike{
In contrast, an ideal loss-resilient coding should be {\em Data-Scalable} (DS)---{\em its quality should degrade gracefully with higher packet loss rate but without sacrificing the quality in absence of packet loss} (illustrated in Figure~\ref{fig:intro-example}(d)). 
DS coding has several benefits: 
{\em (i)} it does not need to predict loss rate before sending the packets (unlike FEC), 
{\em (ii)} a frame can be decodable under {\em any} loss rate, unless all packets are lost, 
{\em (iii)} quality gradually improves if {\em any} more packets are received (unlike SVC), and
{\em (iv)} when all packets are received, it reaches a quality similar to the traditional codec like H.265 used in WebRTC (unlike error concealment).

This paper presents \name, a new loss-resilient scheme for real-time video, which better approximates DS coding by using an autoencoder (neural encoder and neural decoder) to optimize quality under various packet loss rates.
The key idea is two-fold.
\begin{packeditemize} 
\item \name's {\em a loss-resilient autoencoder} (\S\ref{subsec:training}) consists of a pair of neural encoder and neural decoder {\em jointly trained} to optimize video quality when $x$\% of values in the encoder output of a frame are randomly selected and masked (\ie set to zeros), with $x$\% between 0 to 100\%, before the masked data is fed to the decoder. 
This simulates the effect of random data masking between the encoder and the decoder.
\item \name uses a {\em novel packetization scheme} (\S\ref{subsec:packetization}) to partition the encoder output of a frame and entropy encodes each partition as an independently decodable packet, so that losing any $x$\% packets (which can be consecutive or random) has the same effect on the input of the decoder as masking $x$\% of randomly selected values.
In short, packet loss will appear to have same effect as random data masking between the encoder and the decoder.
\end{packeditemize} 
}

%When put together, the two ideas help \name to optimize quality under various packet loss rates, so it better approximates DS coding than prior schemes.
%
%When no packet is lost, \name's quality is similar to H.265 at the same bitrate, but as loss rate increases, \name's quality degrades much more gracefully than state-of-the-art loss-resilient coding schemes.
%%(Figure~\ref{fig:intro-example}). 
%In short, \name better approximates DS coding than prior schemes when packet loss affects one frame. 
%%when tested under different \rates.



%presents a way to smooth frame size across different frame types (I-frames and P-frames)


%To leverage the new data-scalable (DS) autoencoders, \name also includes a customized video streaming framework to delivery a sequence of frames to synchronize the states on the sender and the receiver when the receiver decodes a frame without waiting for 
%%in a slightly lazy fashion.
%It also includes optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).
%to deliver autoencoder-generated data.
%It uses a new packetization scheme on randomly shuffled \aecode with per-packet entropy encoding, which makes packet loss of $n\%$ \rate appear to have the same effect as $n\%$ random making on the \aecode (\S\ref{subsec:packetization}). 
%\name also uses techniques for DS coding over a sequence of frames, as well as optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).







We have implemented \name and evaluated \name using real network traces and a range of video content genres (all from different data sources than the training set of the autoencoder) and compare it against a range of state-of-the-art variants of different loss resilient schemes, including 
{\em (i)} forward error concealment (Tambur~\cite{rudow2023tambur}), 
{\em (ii)} postprocessing error concealment by neural-net in-painting~\cite{xiang2019generative}, 
{\em (iii)} scalable video coding (Swift~\cite{swift}), and
{\em (iv)} selective frame skipping (Voxel~\cite{voxel} and Salsify~\cite{salsify}).
%å, and {\em (v)} functional codecs (Salsify~\cite{salsify}).
%{\em (i)} FEC (Tambur~\cite{rudow2023tambur}), {\em (ii)} error concealment (neural-net generative in-painting~\cite{xiang2019generative} and selective skipping~\cite{voxel}), {\em (iii)} Scalable Video Coding~\cite{swift}, and {\em (iv)} Salsify's functional codec~\cite{salsify}
% including GCC~\cite{carlucci2016analysis} and Salsify~\cite{salsify} (except that packet retransmission is turned off for loss-resilient decoders).
Our key results are: 
\begin{packeditemize}
  \item \name achieves better quality, by 1.4-4 dB of SSIM\footnote{The definition of SSIM dB is in \S\ref{subsec:eval:setup}}, than other loss-resilient schemes at the same packet loss (between 20\% and 80\%) and bitrate (between 0.8Mbps and 4.8Mbps). 
  \item \name achieves a similar average quality (in SSIM) with the codec used in WebRTC at the same bitrate. In other words, \name does not sacrifice quality when there is no packet loss. %in absence of packet loss.
  \item When different loss-resilient schemes are run on real network traces
  \footnote{To be fair, we run \name and the baselines over the same congestion control (CC) algorithm, GCC~\cite{carlucci2016analysis}, which is the standard CC used in WebRTC.}
  , \name's superior loss resilience leads to 90\% reduced duration of video stalls, 95\% reduced number of non-rendered frames, and 66\% reduced tail frame delay (98$^{th}$ percentile). 
  %\name  reduces the duration of video stalls, number of non-rendered frames, and 98$^{th}$ percentile frame delay by \review{90}\%, \review{95}\%, and \review{66}\% respectively, when compared to the most competitive baselines
  \item With much less video stuttering and fewer skipped frames, our IRB-approved user study confirms that \name has \review{38}\% higher mean opinion score (MOS) than the most competitive loss-resilient schemes.
  \item On a single Nvidia A40 GPU, \name can decode 480p and 720p at 120~fps and 44.1~fps, respectively and encode 480p and 720p at 87.7~fps and 31.2~fps, which is 1.5-5$\times$ faster than recent video autoencoders. On CPUs, it can encode 720{p} videos at 28.5~fps (on par with GPU-based implementation) at only a drop of 0.5 dB in SSIM. \yc{update the numbers to reflect Ziyi's latest results}
\end{packeditemize}
%ratio of delayed frames (defined as the frames whose delay between encoding and decoding is larger than 400~ms) by up-to 4$\times$ and the stall rate (defined as the fraction of inter-frame gaps that exceed 200~ms) by 10$\times$. 
%compared to the most competitive baselines which still have to retransmit packets or skip frames.


To put \name's contribution in perspective, neural video codecs have long been used in multimedia, but \name is, to our best knowledge, the first to jointly train generative NN encoder and decoder to improve loss resilience in real-time video.
\name is closely related to using NNs to generatively reconstruct the missing data in lost packets, but they do not jointly train the encoder for loss resilience (\eg~\cite{sankisa2018video,reparo}) or handle only special content type at low resolution~\cite{reparo}.
\name is also related to but different from an emergent technique~\cite{kurka2020deepjscc,bourtsoulatze2019deep,gunduz2019machine} which trains autoencoders to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss).
%Most work on autoencoders has focused on improving {\em compression efficiency} rather than loss resilience, such as scalable video coding (Swift~\cite{swift} and DeepFGS~\cite{ma2022deepfgs}), super resolution~\cite{gemino,neuroscaler,livenas}.
%Neural networks have been used to reconstruct missing spatial blocks in lost packets (\eg~\cite{sankisa2018video,reparo}, which uses NNs on the decoder side and handles only specific video content (\eg talking head~\cite{reparo}). 
%In contrast, \name jointly trains the encoder and decoder to handle packet loss.
%\name is related to but different from an emergent techniques~\cite{kurka2020deepjscc,bourtsoulatze2019deep,gunduz2019machine} which train autoencoders to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss).

% \passed{\jc{agreed that this is a bit too long. tried to shrink it.}}
% \passed{\amz{I understand including so much comparison to related work to hedge the "first to our knowledge" claim, but it is quite long considering the related work comes so soon after. I would remove everything after the first sentence and put it above the limitations paragraph, or just wrap up all the citations in a "other approaches address compression efficiency, post-processing, or signal noise". }}

While \name improves real-time video quality under packet loss, it has limitations (\S\ref{sec:limit}). 
%\amz{This sentence is awkward, I think you can more generously say "While \name improves quality under packet loss, the approach has limitations."}
First, though our implementation of \name can run much faster than traditional autoencoders,
% and achieves lower delay than alternative solutions 
\name cannot run in real-time on resource-constraint devices yet. 
%\amz{Fast enough for what, real-time? }
Second, we focus on unicast video communication, rather than problems in multi-party conferencing (\eg stream forwarding). 
% Third, \name cannot improve the video quality when all packets are lost. 
%\amz{Cannot improve what? }
%\jc{mention that packet loss is often not 100\% given audio still continues}
%While \name decides {\em what} each packet contains, 
Our main goal is to show the potential of training generative autoencoders under different loss rates, and we expect it will spark more efforts to tackle these limitations.


\tempstrike{
% \ie no data loss between the encoder and the decoder, so they need to combined with a loss-resilient scheme.
For instance, Swift~\cite{swift} and DeepFGS~\cite{ma2022deepfgs} use NN codecs to improve scalable video coding (rather than loss tolerance) for on-demand (rather than real-time) videos. 
Super-resolution (SR)~\cite{gemino,neuralscaler} enhances the decoded video quality at the receiver when the available bandwidth is low
DeepJSCC uses an autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss)~\cite{kurka2020deepjscc}.
\name also differs from neural super-resolution models~\cite{neuroscaler,livenas} and generative neural error concealment~\cite{sankisa2018video, reparo} which only trains NNs on the receiver and handles only specific video content (\eg talking head~\cite{reparo}), whereas \name jointly trains the encoder and decoder to handle packet loss.


, and {\em (v)} super resolution (SR)~\cite{??}.\footnote{\editSOCC{The main use case of SR is to enhance the decoded video quality at the receiver when the available bandwidth is low. Such technique should work for any kind of video codecs. Therefore, SR is orthogonal to \name.}} %\jc{explain SR is orthogonal}

}

%There are two key findings (an example of which is given in Figure~\ref{fig:intro-example}). 
%First, when no packets are lost, \name's quality does not exceed H.265 at the same bitrate, but in presence of more packet loss, \name's quality degrades much more gracefully than other loss-resilient coding schemes.
%Second, we use packet-level simulation driven by real-world bandwidth traces and run \name and the baseline loss-resilient coding schemes. % on the same CC logic (retransmits disabled).
%We show that compared to the baselines, \name reduces the ratio of delayed frames (defined as the frames whose delay between encoding and decoding is larger than 400~ms) by up-to 4$\times$ and the stall rate (defined as the fraction of inter-frame gaps that exceed 200~ms) by 10$\times$. 
%%compared to the most competitive baselines which still have to retransmit packets or skip frames.
%With much less video stuttering and fewer skipped frames, our user study confirms that \name has higher average subjective ratings by users than the baselines.
%
%Second, \name borrows existing congestion control (CC) logics {\em without} packet retransmits unless all packets of a frame are lost), such as GCC~\cite{carlucci2016analysis}, which decides the target frame size and how fast to send the \name-encoded packets.


%\textbf{This work does not raise any ethical issues.}



%Though autoencoders have a long history in multimedia, standard autoencoders have focused on better compression efficiency (achieving higher quality in fewer bits) and are not inherently loss-resilient.
%This is because, in traditional autoencoder training, the decoder always receives the {\em same} \aecode produced by the encoder, which does not prepare the autoencoders to handle any data loss during transmission. 
%
%To put it in context, neural encoders and decoders have long been used in multimedia (see \S\ref{sec:related}) but \name is, to our best knowledge, the first to demonstrate the potential of autoencoders to improve loss resilience in real-time video.
%Swift and DeepFGS, for instance, use autoencoders to improve scalable video coding (rather than loss tolerance) for on-demand (rather than real-time) videos~\cite{swift, ma2022deepfgs}. 
%DeepJSCC uses an autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss)~\cite{kurka2020deepjscc}.
%\name also differs from neural error concealment~\cite{sankisa2018video} which only uses NNs on the receiver, whereas \name jointly trains the encoder and decoder to handle packet loss.


\tempstrike{


Autoencoders work like a standard video codec but replace part of the encoder and decoder with neural networks (NNs). 
Though autoencoders have a long history in multimedia, standard autoencoders have focused on better compression efficiency (achieving higher quality in fewer bits) and are not inherently loss-resilient.
This is because, in traditional autoencoder training, the decoder always receives the {\em same} \aecode produced by the encoder, which does not prepare the autoencoders to handle any data loss during transmission. 



This paper presents \name, a new approach to loss-resilient real-time video, by customizing {\em  autoencoders}. 
%This paper presents \name, a new end-to-end loss-resilient real-time video streaming system, by customizing {\em  autoencoders} following the idea proposed in~\cite{cheng2022grace}. 

In \name, we show that autoencoder-based video streaming can be loss-resilient by customizing the autoencoder training process (\S\ref{sec:core}) and video streaming framework (\S\ref{sec:delivery}).

In \name's autoencoder training process (\S\ref{subsec:training}), when the NN encoder returns a \aecode, we randomly mask n\% of its elements to zeros before feeding it to the NN decoder, a process we call {\em random masking}. We vary the rate of random masking ($n\%$) between [0\%, 100\%), which as explained shortly, simulates the effect of packet loss under different \rates.
% As explained shortly, varying the rate of random masking (n%n\%) between [0\%, 100\%) simulates the effect of packet loss under different \rates.
Consequently, our trained autoencoder, {\em without} knowing the actual \rate, can encode a frame such that it can: {\em (i)} decode a frame as long as {\em any} (non-empty) subset of packets of the frame is received;
%(\ie no need for retransmission unless all data is lost);  
{\em (ii)} achieve better quality with the addition of each new packet (\ie graceful degradation with higher \rate); and
{\em (iii)} reach a quality close to a non-loss-resilient coding algorithm (such as H.265) when all packets are received.
We refer to it as {\em Data-Scalable} ({\em DS}) video coding.
In contrast, FEC is not DS coding, since its quality does not improve with more data if the \rate is below a threshold but the quality drops abruptly (due to retransmits) once the \rate exceeds the threshold.

}

% Our prior work of data-scalable (DS) autoencoders~\cite{cheng2022grace} suffers from multiple problems: {\em (i)} naive entropy encoding lowers compression efficiency, {\em (ii)} encoding speed insufficiently fast (<20fps) for real-time video streaming requirements, and {\em (iii)} additional quality degradation due to error propagation from packet losses.
% %To leverage the new data-scalable (DS) autoencoders, 
% To address the above challenges, \name uses a customized video streaming framework to deliver autoencoder-generated data.
% It uses a new packetization scheme with per-packet entropy encoding, which makes packet loss of $n\%$ \rate appear to have the same effect as $n\%$ random making on the \aecode (\S\ref{subsec:packetization}) with negligible size overhead. 
% \name also uses techniques for DS coding over a sequence of frames to minimize the propagation of error, as well as optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).


\begin{comment}

It uses a novel packetization scheme that makes packet loss of n%n\% appear to have the same effect as n%n\% random making on the \aecode (see \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{subsec:packetization} for details). 
%Standard autoencoders entropy encode the NN encoder output (\aecode) and packetize the resulting bitstream, so any packet loss will render it undecodable by the receiver.
The basic idea is to randomly split the \aecode's elements to partitions, each separately entropy-encoded as an independently decodable packet, and if n%n\% packets are lost, we set their elements in the \aecode to zeros, which mimics random masking.
However, this naive scheme greatly increases the size of the compressed data, due to the additional space needed to store the symbol distribution (used by entropy-decoding) in each packet.
\name addresses this challenge by carefully coarsening the granularity of symbol distributions, which significantly reduces size increase while maintaining the compression efficiency of entropy coding. 

\end{comment}





\begin{comment}

Ideally, the quality should degrade gracefully with more packet loss (higher \rate), without compromising the quality in absence of packet loss.
Specifically, it should be able to 
{\em (i)} decode a frame as long as {\em any} (non-empty) subset of packets of the frame is received;
%(\ie no need for retransmission unless all data is lost);  
{\em (ii)} achieve better quality with the addition of each new packet (\ie lower \rate); and
{\em (iii)}  reach a quality close to a non-loss-resilient coding algorithm (such as H.265), when all packets are received.
We refer to it as {\em Data-Scalable} ({\em DS}) video coding.
FEC is not DS coding, since its quality does not improve with more data if the packet loss rate is below a threshold but the quality drops abruptly once loss rate exceeds the threshold.


\mypara{Data-scalable autoencoder}
This paper introduces {\em \name}, a real-time video system that, for the first time, uses {\em  autoencoders (AEs)} to realize data-scalable (DS) video delivery.
%which explores a new approach to DS video delivery by using {\em neural-net (NN) autoencoders}.
At a high level, autoencoders work like a standard video codec but replace some coding logic with neural networks (NNs). 
It uses an NN encoder to encode a frame to a {\em \aecode} (without entropy encoding), and an NN decoder to decode to a reconstructed frame that is similar to the original frame. 


We choose autoencoders, not because the off-the-shelf models are inherently data-scalable (DS), but due to their unique properties that {\em could} enable DS coding. 
%\name is a particular design that harnesses these properties to enable DS coding.
Specifically, the NN decoder can reconstruct a decent-quality frame, even if we {\em randomly erase} (\ie set to zeroes) a subset of $n\%$ elements in the \aecode (the output of the NN encoder).
In other words, {\em random data erasure} on the \aecode has a limited impact on the decoding quality of autoencoders. 
This can be attributed to the lack of stringent dependencies among the elements in a \aecode\footnote{
%Mathematically, this smoothness is a result of NN encoders and decoders having continuous derivatives everywhere. Moreover, 
This can also be intuitively understood that NN decoders share the architecture of {\em generative} NNs, such as variational autoencoder (VAE), which can create realistic-looking images from random inputs.}, unlike SVC where the decoding of a layer depends on the lower layers.


Despite the promise of autoencoders, several practical challenges remain.
%\name addresses several practical challenges.
Two of them will be highlighted here.

%Despite the promise of autoencoders, \name must address several practical challenges, such as improving quality under various \rates, making entropy encoding of \aecodes loss-resilient, controlling bitrate, and speeding up autoencoder coding. 
%Two of them will be highlighted here.


%\mypara{Adding packet loss in autoencoder training}
\mypara{Training autoencoder with packet loss}
First, the quality of standard autoencoders drops quite significantly if more data is erased from the \aecode. 
This is because the standard autoencoder training, in which  the decoder always sees the same \aecode returned by the encoder, never prepares the autoencoder to handle any data loss between the encoder and the decoder. 
\name trains autoencoders different (see \S\ref{??} for details).
It applies random data erasures to the \aecode (which could simulate the effect of packet loss as explained shortly), and by varying the rate of data erasure between [0\%, 100\%), 
%In other words, by training the NN encoder and NN decoder jointly, 
the new autoencoders not only learn how to compress high-quality frames efficiently but also to be robust to different rates of random data erasures. 

%, which simulates the effects of packet loss under different \rates (which will be explained shortly).






\mypara{Per-packet entropy coding for autoencoder}
Standard autoencoders use entropy encoding to losslessly compress a \aecode to a single bitstream and then packetize it, so any packet loss will render it undecodable.
%entropy coding used in current autoencoders cannot tolerate any packet loss. 
A naive idea is to randomly 
split the \aecode's elements to partitions,
%split a \aecode to sub-tensors, 
each separately entropy-encoded as an independently decodable packet, and if $n\%$ packets are lost, we set their elements in the \aecode to zeros, which resembles random erasure.
%effectively erases a random subset of $n\%$ elements.
%is the same as 
%random data erasure.
However, this naive per-packet entropy coding greatly increases the size of the compressed data, due to the additional space needed to store the symbol distribution (used by entropy-decoding) in each packet.
%To mitigate the size increase, 
\name carefully coarsens the granularity of symbol distributions, which significantly reduces size increase while maintaining the compression efficiency of entropy coding (see \S\ref{??} for details). 




Besides achieving loss resilience on a single frame, \name uses a novel frame delivery system to approximate DS coding over a sequence of frames, speed up autoencoder coding (on GPUs and CPUs), and enable efficient bitrate control (\S\ref{??}).




\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/fig1-example.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/fig1-example-osdi.pdf}
        \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/fig1.png}
         \caption{graceful degradation}
         \label{fig:normal-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
         \caption{delay quality tradeoff}
         \label{fig:normal-ssim-delay}
     \end{subfigure}
         \label{fig:}
         \tightcaption{Example results of \name's (a) more graceful degradation in presence of packet loss than prior solutions, and (b) better tradeoffs between video quality and tail frame delay, which corroborates the subjective rating of users.
         More results can be found in \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{sec:eval}. 
%         \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
    \jc{TODO: add a horizontal line to indicate the quality of H.265}
    \textcolor{red}{Yihua: TODO: update real values (fig1data.xlsx)}
         }
    \label{fig:intro-example}
\end{figure}

\end{comment}






%including a custom streaming protocol
%controlling bitrate, and speeding up autoencoder coding. 


%, so that even if the selected bitrate overshoots the bandwidth, we can still obtain decent quality.


%Being a coding system, \name can work with existing congestion control (CC) logics---CC decides how fast to send packets, and \name decides {\em what} each packet contains.




%Much remains unknown about the limits of autoencoders as a loss-resilient coding layer.

%To our best knowledge, \name is the first end-to-end autoencoder-based video system for loss-resilient real-time videos.
%that achieves stream real-time videos in a data-scalable fashion. 



%arising from training and using autoencoders in real-time video communication.

%Many aspects of \name are also inspired by prior work. 
%That said, \name, to our best knowledge, is the first to develop custom autoencoders that realize data-scalable video delivery.

%\name aims at unicast video sessions, rather than multi-party conferences. 
%It is also important that \name's autoencoders do {\em not} achieve better compression efficiency than recent heavily engineered video codecs, such as H.265. 
%Indeed, \name's video quality is still slightly lower than H.265 at the same bitrate. 








==> sections/old/intro.tex <==
%-------------------------------------------------------------------------------
\tightsection{Introduction}
%-------------------------------------------------------------------------------

Usage of real-time video conferencing applications are increasing rapidly.

The goal of real time video conferencing is high visual quality and low latency. However, achieving such goal is challenging because of unavoidable and unpredictable packet losses.

Towards this problem, state-of-art solutions can be divided into 2 categories: retransmission-based method and hand-crafted loss tolerant mechanisms. However, all of those methods are not optimal...

Our goal and our design...

==> sections/old/intro_sep20_5.10.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

%%%%%%%%%%%%%%%%%%
% Trying to split the description of figure 1
%%%%%%%%%%%%%%%%%%

\section{Introduction}

Real-time video communication has become an integral part of our daily
lives~\cite{blum2021webrtc}, spanning online
conferences~\cite{webrtc-vc-1,webrtc-vc-2},
cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2},
interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2},
and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
To ensure a high quality of experience (QoE) for users,
real-time video applications must protect against
packet losses\footnote{In this study, we use the term
``packet loss'' to refer to both packets
dropped in transit and those not received by the decoding deadline.
Under this definition, a video frame could experience a high packet
loss rate (e.g., 50\%) even if the actual network loss
rate is low~\cite{rudow2023tambur}.}.
%Thus, many real-time video frames can have a high (over 50\%) packet loss rate, even if the network has a low average packet drop rate, which corroborates with other studies~\cite{??,??}.}.
However, retransmitting lost packets across high-latency networks
is not feasible due to stringent real-time latency requirements~\cite{itu-g114}.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.6\columnwidth]{intro-illustration.pdf}
  \caption{Illustration of the video quality achieved by
  different loss-resilient schemes, operating under the same bandwidth budget,
  across varying packet loss rates.
  Actual experimental results are shown in Figure~\ref{fig:loss_by_dataset}.}
  %(Actual figures from our evaluation appear later, \eg Figure~\ref{??}.)}
  \label{fig:intro-example}
  \vspace{-10pt}
\end{figure}

Loss-resilient techniques generally fall into two categories.
First is encoder-side forward error correction (FEC), such as Reed-Solomn codes~\cite{wicker1999reed}, fountain codes~\cite{mackay1997near, mackay2005fountain}, and more recently, streaming codes~\cite{rudow2023tambur, badr2017fec}.
%, are widely used.
% to recover packet losses without retransmission.
FEC incorporates redundancy into data prior to transmission.
With a redundancy rate of $R\%$---the percentage of redundant data relative to the total data size---up to $R\%$ of lost data can be recovered.
Beyond that, video becomes undecodable,
rendering a sharp collapse in video quality (Figure~\ref{fig:intro-example}).
Increasing $R$ protects against higher losses but also entails a higher bandwidth overhead, which in turn reduces video quality.
Thus, determining the optimal $R$ in advance poses a practical challenge.
%As illustrated in Figure~\ref{fig:intro-example}, a larger $R$ can tolerate more packet losses at the expense of lower video quality, and the video is no longer decodable when the loss rate exceeds $R\%$, causing a sharp collapse in video quality.
%\passed{\fyy{This is not a good place to insert parentheses as they break the flow and sound informal. Generally refrain from overuse of parentheses.}} 
%Nevertheless, determining the optimal $R$ value involves forecasting the packet loss rate, posing a practical challenge.
%Under the same bandwidth, a larger $R$ is more resilient to packet losses but also entails lower video quality.

%Another popular solution to recover from packet loss is decoder-side error concealment,
The second category is decoder-side error concealment,
which reconstructs portions of a video frame affected by packet losses, through handcrafted heuristics~\cite{kolkeri2009error, zhou2010efficient,wang2013novel} or neural networks~\cite{xiang2019generative,kang2022error,sankisa2018video, mathieu2015deep,reparo}.
Nevertheless, implementing error concealment requires partitioning a video frame into independently decodable units (\eg slices~\cite{XXX} or tiles~\cite{XXX}) first, thus reducing compression efficiency.
Moreover, since the encoder is not optimized for loss resilience, the lost information cannot be effectively retrieved by the decoder alone.
%it aggressively compresses each frame, resulting in each packet containing little redundancy to help reconstruct the missing information.
As a result, the video quality tends to deteriorate rapidly with increasing packet loss, as illustrated in Figure~\ref{fig:intro-example}.
% More importantly, since the encoding of each frame has minimum redundancy \fyy{What does "minimum" redundancy mean? This is not clear. And why can't it have more redundancy?}, error concealment techniques may not always accurately reconstruct the information in lost packets, especially when objects have unpredictable motions or a new object appears
% \fyy{I don't think people will understand why this is the case after reading this sentence. The example after "especially"
% does not help with the understanding.}.
% Therefore, the quality can degrade quickly as the packet loss rate escalates as depicted in Figure~\ref{fig:intro-example}.

% In \S\ref{subsec:related}, we discuss other strategies that are not specifically
% designed for loss resilience but can be repurposed to tolerate packet loss,
% such as scalable video coding (SVC) and super resolution.
% We show that they either sacrifice coding efficiency when there are no
% packet losses, or fail to decode video or retain video quality under high packet losses.
% \yc{This section is clear, but it didn't explain what are the problems of the existing solutions.}



% In Figure~\ref{fig:intro-example}, we illustrate the superiority of \name over
% other loss-resilient schemes within the same bandwidth budget.
% Unlike encoder-based FEC, \name neither requires predicting the
% packet loss rate prior to transmission, nor suffers from a sharp collapse
% in decodability as the loss rate escalates.
% A video frame produced by \name remains decodable at \textit{any} loss rate
% (unless all packets are lost), with its quality progressively improving as
% more packets are received.
% When compared with decoder-based error concealment,
% \name avoids sacrificing compression efficiency upfront for error resilience
% and consistently yields higher video quality under varying losses. 
% % \fyy{I merged the design goals and benefits of Grace into this single paragraph,
% but the text needs to be shortened.}

% \fyy{Alternate flow: here seems to be a natural place to compare with
% the existing encoder-only and decoder-only approaches, referencing to Figure 1.
% Then start a new paragraph to talk about how Grace works at a high level.}

% \fyy{The next paragraph is central to intro, but 1) the motivation
% for using neural video codecs is still weak (I used "To facilitate the joint optimization" for lack
% of a better reason, but hopefully there is a better reason);}

In this paper, we present \name, a loss-resilient real-time video system designed to maintain the user's quality of experience (QoE) across a wide range of packet losses.
Our key insight is that {\em jointly optimizing the encoder and decoder under a spectrum of simulated packet losses} considerably strengthens loss resilience.
To facilitate this joint optimization, \name strategically employs a neural video codec (NVC)~\cite{dvc}, integrating neural networks into the core components of a conventional video encoder and decoder.
%which architecture also holds promise for robustness against data perturbation (such as packet loss)~\cite{??}.
%\edit{to make the encoder and decoder trainable.}\hc{"to train encoder and decoder for this specific purpose"}
%\yc{maybe we can say NVC is inherently more robust to XXX (think about the term here) + citation}
%\fyy{This sentence sounds incomplete}.
%\jc{i removed the text about replacing core components of conventional codecs, since it's not critical and it's already implicit in the term neural video codecs. feel free to revert if you want}
% and integrates neural networks into the core components 
%of a conventional encoder and decoder (rather than replacing them entirely).
In contrast to FEC, \name's NVC is trained to handle \textit{diverse} packet losses, eliminating the need to predict a loss rate beforehand and preventing the undecodable video under exceedingly high losses.
Unlike decoder-side error concealment, \name \textit{jointly} trains the encoder and decoder, so that the encoder 
learns to properly distribute each pixel's information across multiple output elements in anticipation of losses, facilitating the decoder's frame reconstruction when packets are actually lost.
%thereby  enhancing its output's resilience to packet loss and allowing the decoder to better reconstruct the original frame when packet loss happens.
% making the encoder's output more robust to packet loss. 
%As a result, the decoder can better reconstruct the original frame when packet loss happens.
%learns to add some redundancy \fyy{what do you mean?} to enable a better reconstruction of information critical to frame quality when packet loss happens.
%to the information critical to the frame quality, enabling a better reconstruction when packet loss happens.
%By jointly optimizing the encoder and decoder, rather than only the decoder, \name's encoder learns to add redundancy to the information that is critical to the frame quality, enabling a better reconstruction than error concealment methods when packet loss happens.
Consequently, \name displays a more graceful quality degradation amid varying losses, while consistently delivering higher video quality than previous solutions (Figure~\ref{fig:intro-example}).
% Optimizing under a spectrum of packet losses, rather than a fixed loss rate, prevents \name from having the sharp quality collapse like the encoder-based FEC.

% \jc{This paragraph seems a bit out of blue. maybe we should say to joint training encoder/decoder under loss, it is important to simulate the impact of packet loss during training the same way as the inference. This will be a natural place to introduce random zeroing and packetization, etc
% Maybe list THIS as the first non-NN challenge?}
% During the training of the neural video codec in \name, packet losses are simulated by zeroing values in the encoder's output before feeding to the decoder.  
% During the inference, \name randomly partitions the encoder's output into different packets so that packet loss has the same effect on the encoder's output as during training. 
% \S\ref{sec:core} shows more details of the training process of \name and explains why it can be loss-tolerant. 
% \name is trained with a wide spectrum of packet loss, ranging from 0\% to 60\%. 
% As a result, it achieves video quality on par with traditional codecs,
% such as H.265 (without FEC), in the absence of packet losses.
% As the packet loss intensifies,
% \name retains higher quality than state-of-the-art loss-resilient schemes,
% exhibiting a more graceful degradation in quality. 

% \edit{To add packet loss in the training of the neural video codec, 
% \name randomly partitions the encoder's output into different packets so that a lost packet will render the values in its partition to zeros in the decoder's input.
% During training, \name sees a wide spectrum of packet losses, ranging from 0\% to 60\%.}
% \fyy{There is a missing link between using neural codec (above) to the amazing
% performance of Grace (below). Think about how to transition.}




%Jointly optimizing the encoder and decoder under a spectrum of packet losses enables \name's NVC to have a graceful quality degradation under packet losses.
%However, to unleash such capability from the \name's codec, the end-to-end video system needs to address three new challenges.
%However, in order to make the end-to-end video system fully embrace such capability from the \name's codec, there are still three main system challenges.
To materialize the above benefits of \name's codec, however,
three system challenges remain to be addressed.

First, packet loss simulation during training must be carefully designed to ensure that simulated losses mirror real-world effects.
%the same effect as the real ones.
%the effect of real packet losses is the same as during training.
To this end, we randomly zero (``mask'') values in the encoder's output during training to simulate packet loss (\S\ref{sec:core}).
%values in the encoder's output are randomly zeroed (masked) 
%before feeding into the decoder (\S\ref{sec:core}).
At runtime, \name employs a novel packetization scheme that partitions the encoder's output using a reversible random function~\cite{lcg} before entropy-encoding each partition into a separate packet.
If a packet goes missing, its corresponding values in the encoded output are zeroed. 
As a result, each packet is individually decodable, and the impact of a lost packet matches that of simulated packet loss (\S\ref{subsec:packetization}).
%is mapped to the random erasure of values in the encoder's output.
%Section~\S\ref{sec:core} and \S\ref{subsec:packetization} provides more details about the training and packetization process of \name. 

Second, to prevent video stream corruption after packet loss ends, \name designs a new protocol to efficiently re-synchronize the encoder and decoder states without blocking video decoding.
%the video system should efficiently synchronize the encoder and decoder states to avoid video stream corruption after packet loss ends.
%To this end, we design a new protocol for \name to re-synchronize the encoder and decoder states without blocking the decoder.
%retransmission.
When packet loss occurs, the decoder can still decode the partially received packets by leveraging the NVC's inherent loss resilience. Moreover, it also informs the encoder of the loss information. This allows encoder to quickly update the recent reference frames to align with those on the decoder side.
%When the decoder decodes a frame based on partially received packets, 
%When getting the packet loss feedback from the decoder, the encoder quickly re-decodes the recent frames as seen by the decoder to align its state with the decoder.
Such re-decoding only increases the encoding time by 7\% whenever it happens (\S\ref{subsec:protocol}).
%Such re-decoding only requires 7\% of the encoding time (\S\ref{subsec:protocol}).

Third, \name must be efficient to encode and decode video in real time across various devices, from laptops to mobile phones.
Existing NVCs, however, often employ expensive neural networks, particularly for motion estimation and prediction.
%Among the performance optimizations,
We show that by downscaling the image input for motion estimation and simplifying motion prediction, \name accelerates the encoding and decoding by $4\times$ on GPUs without a noticeable impact on loss resilience. 
Moreover, with hardware-specific runtimes such as OpenVINO and CoreML, \name attains over 30~fps on CPUs and iPhones (\S\ref{subsec:fast-coding}).

\begin{comment}
%resource-constrained devices like laptops and mobile phones.
Existing neural video codecs usually use heavy neural networks for motion prediction~\cite{dvc}.
Our insight using the motion predicted from the down-scaled image only has negligible impact on frame quality compared to using a full-size image for motion prediction.
By downscaling the width and height of the image by $2\times$, the motion prediction network can be sped up by $4\times$. 
\name also applies the latest hardware acceleration techniques including OpenVINO~\cite{openvino} and CoreML~\cite{coreml} to speed up the neural network inference on CPUs and mobile devices (\S\ref{subsec:fast-coding}). 
% \name also trains multiple encoders that produce different encoded bitrates but share most computation, making it possible to encode a frame at multiple bitrates with negligible overhead.
\end{comment}


% \name addresses the above challenges with the following designs.
% \begin{packeditemize}
%     \item (\S\ref{subsec:packetization}) \name uses a new packetization scheme that {\em randomly} partitions the encoder's output before entropy encoding each partition into a separate packet. 
%     Therefore, each packet is individually decodable, and the impact of a lost packet is mapped to the random erasure of values in the encoder's output.
%     \name also regularizes the neural network encoder during training so that the random partition scheme does not have the compression efficiency reduction problem like the error concealment solutions.
%     \item (\S\ref{subsec:protocol}) We design a new protocol for \name to re-synchronize the encoder and decoder states without retransmission. 
%     When getting the packet loss feedback from the decoder, the encoder quickly re-decodes the recent frames as seen by the decoder to align its state with the decoder and such re-decoding only requires 7\% of the encoding time.
%     \item (\S\ref{subsec:fast-coding}) Contrary to existing neural video codecs that rely on complex neural networks for motion prediction, \name leverages the motion prediction capabilities of conventional codecs such as H.264, thereby substantially reducing encoding overhead.
%     \name also trains multiple encoders that produce different encoded bitrates but share most computation, making it possible to encode a frame at multiple bitrates with negligible overhead.
%     %\name embraces the latest hardware acceleration techniques including OpenVINO~\cite{openvino} and CoreML~\cite{coreml} to speed up the neural network inference on CPUs and mobile devices. 
% \end{packeditemize}

% {\em (i)} The packetizer of \name should allow packets to be individually decodable and guarantee the effect of losing one packet is equivalent to randomly zeroing values in the encoder's output. 
% {\em (ii)} The video system should efficiently synchronize the encoder and decoder states to avoid video stream corruption after packet loss ends.
% {\em (iii)} \name should be efficient enough to encode/decode videos in real time on resource-constrained devices like laptops and mobile phones.

% \name's neural video codec provides the basis for the loss tolerance. 
% \fyy{What basis? Avoid vague language. Here is probably the place to set the stage
% first for neural video codec: I would describe why choose
% neural video codec in Grace and what it can already do.
% Then go on to say what it cannot do.}
% However, there are still two challenges in order to make the whole video system loss-resilient. 
% First, each packet should be independently decodable, regardless of the loss of any other packets.
% Most of the traditional codecs such as H.265 and VP9 do not meet this requirement.
% This is because they use entropy coding to compress the encoded video before splitting the data into packets,
% resulting in entropy decoding failure when packet loss happens.
% \yc{think about how to phrase this more like a challenge instead of a requirement. The complexity is from doing per-packet entropy encode without size inflation.}
% Second, the video system needs to efficiently synchronize the encoder and decoder states after packet loss to prevent error propagation.
% \fyy{It is unclear why synchronization of states is required. "Error" is not defined.}
% Reconstruction errors will accumulate when using decoder-side error concealment techniques
% \fyy{Why mention "error concealment" here? Confusing.}, 
% and such errors will keep affecting the frame quality after the packet loss ends (it is also known as error propagation~\cite{??}).
% In order to mitigate the errors, existing solutions either need to retransmit the lost packets or send a new keyframe to refresh the video stream, 
% both incurring a significant overhead in bandwidth. \fyy{Retransmitting lost packets
% should not incur a high bandwidth overhead. This is confusing.}

% \name addresses the above challenges. 
% It uses a new packetization scheme that partitions the encoder's output tensor
% \fyy{pay attention to newly introduced concepts as "tensor" has not been introduced
% earlier.} before entropy encoding each partition into a separate packet (\S\ref{subsec:packetization}).
% It also regularizes the neural network encoder during training so that such a scheme does not cause significant size inflation.
% We also design a new protocol for \name to re-synchronize the encoder and decoder states without the need for retransmission or a new keyframe (\S\ref{subsec:protocol}).
% \fyy{Overall, the descriptions of both two challenges seem too long, with details unsuitable
% for the intro. In contrast, the solutions are too short. I don't understand it without
% more details.}


% To use neural video codecs for real-time video applications, another important concern is 
% that neural networks are usually too heavy to run on client devices efficiently.
% \fyy{Is this simply the third challenge?.}
% \name uses two optimizations to improve the efficiency of video encoding and decoding (\S\ref{subsec:fast-coding}). 
% First, \name trains multiple pre-trained encoders that produce different encoded bitrates but share most computation.
% Therefore, \name can encode a frame at multiple bitrates with negligible overhead and pick the encoded bitrate most similar to the target bitrate at runtime. 
% \yc{maybe consider saying neural video codecs are not good at bitrate adaptation since it may require multiple-pass inference? Otherwise, it sounds like coming from nowhere.}
% Second, \name embraces the latest hardware acceleration techniques including OpenVINO~\cite{openvino} and CoreML~\cite{coreml} to speed up the neural network inference on CPUs and mobile devices.


% \fyy{Think about if the reader needs to know all these details and key results. Usually not in the intro. Just bring the last paragraph here and use a few sentences to describe results highlights. Similar to what I did in the abstract.} 
% We have implemented \name and evaluated it by transmitting videos covering a range of content genres (all different from the training set) over real network traces (\S\ref{sec:eval}).

% \name is closely related to using NNs to generatively reconstruct the missing data in lost packets, but they do not jointly train the encoder for loss resilience (\eg~\cite{sankisa2018video,reparo}) or handle only special content type at low resolution~\cite{reparo}.
% \name is also related to but different from an emergent technique~\cite{kurka2020deepjscc,bourtsoulatze2019deep,gunduz2019machine} which trains autoencoders to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss).
% \fyy{I would suggest moving this paragraph to related work. This doesn't need to be mentioned in the intro.}


Comprehensive experiments (\S\ref{sec:eval}) on a diverse set of videos and real network traces show that 
with the same congestion control logic, 
\name reduces undecodable frames by 95\% and stall duration by 90\% compared with state-of-the-art FEC baselines. It also boosts 
the visual quality metric of SSIM by 3~dB
%video quality by 3~dB of SSIM (a visual quality metric)
over a recent neural error concealment scheme (\S\ref{subsec:eval:setup}).
%defined in \S\ref{subsec:eval:setup}. 
%(We run \name and baselines on the same congestion control logic.)
Our IRB-approved user study with 240 crowdsourced participants and
a total of 96 subjective ratings demonstrates 
a 38\% higher mean opinion score (MOS) for \name,
further attesting to its effectiveness.
Regarding computational efficiency, \name achieves more than 40~fps on popular mobile devices (e.g., iPhone 14 Pro), meeting the real-time requirement.
%resource-constrained devices such as , matching the requirement of real time videos.

Our contributions are summarized as follows. 
{\em (i)} We present \name, which, to the best of our knowledge, represents the first effort to jointly train a neural video encoder and decoder under a spectrum of packet losses, aiming to improve loss resilience in real-time video (\S\ref{sec:core}).
{\em (ii)} We build the end-to-end video system to address the practical challenges associated with integrating a new NVC, developing optimization techniques related to packetization, encoder/decoder state synchronization, and runtime efficiency (\S\ref{sec:delivery}).
%develop optimization techniques to better utilize the new NVC in an end-to-end video system, addressing challenges including packetization, encoder/decoder state synchronization, and runtime efficiency (\S\ref{sec:delivery}).
%\jc{it may sound like we develop a whole new NVC from scratch. if so, people may wonder if the contribution is too vision-centric.}

\begin{comment}

Our contributions can be summarized as follows:
%This paper makes following key contributions:
\begin{packeditemize}
    \item We present \name, which is, to our best knowledge, the first to jointly train neural video encoder and decoder under a spectrum of packet losses to improve loss resilience in real-time video (\S\ref{sec:core}).
    \item We present optimizations to best utilize the new NVC in an end-to-end video system, addressing challenges including packetization, encoder/decoder state synchronization, and runtime efficiency (\S\ref{sec:delivery}).
    \item Comprehensive experiments (\S\ref{sec:eval}) on real network traces and a diverse set of videos show that \name reduces undecodable frames by 95\% and stall duration by 90\% compared to baselines using FEC,  and boosts video quality over baselines using error concealment by 3~dB of SSIM. 
Our IRB-approved user study attests to \name's effectiveness by showing it has a 38\% higher mean opinion score (MOS).
\name also achieves more than 40~fps on resource-constrained devices such as iPhone 14 Pro, matching the requirement of real time videos.
\end{packeditemize}

\end{comment}

% To put \name's contribution in perspective, neural video codecs have long been used in multimedia, but \name is, to our best knowledge, the first to jointly train generative NN encoder and decoder to improve loss resilience in real-time video.
% Our evaluation results (\S\ref{sec:eval}) show that \name reduces undecodable frames by 95\% and stall duration by 90\% compared with FEC, 
% and boosts video quality over error concealment by 3~dB of SSIM. 
% Our IRB-approved user study attests to \name's effectiveness by showing it has a 38\% higher mean opinion score (MOS).
% \name also achieves more than 40~fps on resource-constrained devices such as iPhone 14 Pro, matching the requirement of real time videos.

% \fyy{After the intro, the reader should know how Grace works at a high level.
% I definitely don't feel like knowing its workflow after reading the intro,
% e.g., what happens during training and inference, respectively?}
% \fyy{The last paragraph is fine but breaks the flow in my opinion. I usually prefer to state the contributions first, including "Grace is the first work to ...", before providing the results highlights.
%}
% Comparison between \name and a spectrum of state-of-the-art loss-resilient schemes shows that 
% it reduces undecodable frames by 95\% and stall duration by 90\% compared with FEC, 
% and boosts video quality over error concealment by 3~dB of SSIM. 
% Our IRB-approved user study shows \name has a 38\% higher mean opinion score (MOS), further attesting to its effectiveness.
% \name can also encode and decode efficiently on resource-constrained devices: \fillme and \fillme fps for 720{p} video on an iPhone 14 Pro at drop of only \fillme dB in SSIM.

% {\em (i)} forward error concealment (Tambur~\cite{rudow2023tambur}), 
% {\em (ii)} postprocessing error concealment by neural-net in-painting~\cite{xiang2019generative}, 
% {\em (iii)} scalable video coding (Swift~\cite{swift}), and
% {\em (iv)} selective frame skipping (Voxel~\cite{voxel} and Salsify~\cite{salsify}).
% Our key results are: 
% \begin{packeditemize}
%   \item \name achieves better quality, by 1.4-4 dB of SSIM\footnote{The definition of SSIM dB is in \S\ref{subsec:eval:setup}}, than other loss-resilient schemes at the same packet loss (between 20\% and 80\%) and bitrate (between 0.8Mbps and 4.8Mbps). 
  
%   \item \name achieves a similar average quality (in SSIM) with the codec used in WebRTC at the same bitrate. In other words, \name does not sacrifice quality when there is no packet loss. 
  
%   \item When different loss-resilient schemes are run on real network traces
%   \footnote{To be fair, we run \name and the baselines over the same congestion control (CC) algorithm, GCC~\cite{carlucci2016analysis}, which is the standard CC used in WebRTC.}
%   , \name reduces undecodable frames by 95\% and stall duration by 90\% compared with FEC; 
%   it also significantly boosts video quality over error concealment---without notably affecting other metrics in both comparisons.
  
%   \item With much less video stuttering and fewer skipped frames, our IRB-approved user study confirms that \name has \review{38}\% higher mean opinion score (MOS) than the most competitive loss-resilient schemes.
  
%   \item On a single Nvidia A40 GPU, \name can decode 480p and 720p at 120~fps and 44.1~fps, respectively and encode 480p and 720p at 87.7~fps and 31.2~fps, respectively, which is 1.5-5$\times$ faster than recent video autoencoders. 
%   On an iPhone 14 Pro, it can encode 720{p} videos at 41~fps (on par with GPU-based implementation) at only a drop of 0.5 dB in SSIM. \yc{the fps is higher than it should be, because we didn't consider the time to get h264 mv on iphone}
  
% \end{packeditemize}

% To put \name's contribution in perspective, neural video codecs have long been used in multimedia, but \name is, to our best knowledge, the first to jointly train generative NN encoder and decoder to improve loss resilience in real-time video.
% \name is closely related to using NNs to generatively reconstruct the missing data in lost packets, but they do not jointly train the encoder for loss resilience (\eg~\cite{sankisa2018video,reparo}) or handle only special content type at low resolution~\cite{reparo}.
% \name is also related to but different from an emergent technique~\cite{kurka2020deepjscc,bourtsoulatze2019deep,gunduz2019machine} which trains autoencoders to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss).
% \fyy{After the intro, the reader should know how Grace works at a high level.
% I definitely don't feel like knowing its workflow after reading the intro,
% e.g., what happens during training and inference, respectively?}
% \fyy{The last paragraph is fine but breaks the flow in my opinion. I usually prefer to state the contributions first, including "Grace is the first work to ...", before providing the results highlights.}


% \begin{itemize}
%     \item A loss-tolerant video system should deal with the following challenges: 
%     \begin{itemize}
%         \item Each packet of a frame should be independently decodable regardless of other frames -- we have per-packet entropy coding for this
%         \item Should be able to sync the states between sender and receiver to prevent error propagation -- we have state synchronization protocol
%     \end{itemize}
%     \textit{(emphasize \name is not just a NN, but a video system)}

%     \item Challenges to make NN being practical for realtime video applications
%     \begin{itemize}
%         \item too heavy for edge devices to run -- our CPU optimization for edge devices
%         \item bitrate adaptation (need to find some citations) -- backbone sharing for faster bitrate adaptation
%     \end{itemize}
%     \textit{(we are not too heavy)}

%     \item We have implemented and evaluated \name on XXX and compared it against YYY baselines. Here are the key results
%     \begin{itemize}
%         \item similar average quality (not sacrificing quality)
%         \item better quality than EC, lower stall/delay than FEC
%         \item Higher user score
%         \item Fast inference speed to match real time requirement
%     \end{itemize}

%     \item Key contribution: {\em jointly} train encoder and decoder  {\em with loss}.
% \end{itemize}
%This enhanced resilience can be attributed to \name's exposure to packet
%losses during training, which steers it to transform video into a loss-resistant
%space.

==> sections/old/intro_v0.tex <==
%-------------------------------------------------------------------------------
\tightsection{Introduction}
%-------------------------------------------------------------------------------

Usage of real-time video conferencing applications are increasing rapidly.

The goal of real time video conferencing is high visual quality and low latency. However, achieving such goal is challenging because of unavoidable and unpredictable packet losses.

Towards this problem, state-of-art solutions can be divided into 2 categories: retransmission-based method and hand-crafted loss tolerant mechanisms. However, all of those methods are not optimal...

Our goal and our design...

==> sections/old/intro_v10.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}

Real-time video communication has a long history in research, yet only recently has it become truly popular and ubiquitous in our daily lives~\cite{blum2021webrtc}, from online meetings~\cite{webrtc-vc-1,webrtc-vc-2}, cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2}, to interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2} and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
The amount of time people spend on real-time videos increases much faster than they spend on streaming videos, both live and on-demand~\cite{webrtc-trend-1,webrtc-trend-2}.
%As a result, users expect that each frame has a high quality, that no frame is skipped, and 
%that each frame is decoded on time such that the viewer sees a smooth playback (\eg under 25fps, a frame should be decoded every 40~ms). 

However, compared to on-demand video viewers, users of real-time applications are more likely to suffer poor quality and video stuttering in video calls~\cite{vca-vice} and online gaming~\cite{gaming-asurion}.
%, even when the network is connected, \eg video freezes when audio continues~\cite{??}. 
This is because real-time video applications use a shallow jitter buffer (\eg \fillme ms in WebRTC).
As a result, {\em any} lost or delayed packet may increase the {\em frame delay}---the delay between sending a frame and receiving enough data to decode it.
This is particularly damaging in long-latency links (\eg long-distance video calls or bufferbloat), where resending just one packet takes one round-trip time and can block the decoding of several frames.

Loss-resilient video coding
%which decodes a frame at a decent quality in presence of packet loss, 
is thus the key to maintaining high video quality and smooth playback of real-time videos.
The performance of a loss-resilient coding scheme can be measured in {\em compression efficiency} (quality in {\em absence} of packet loss) and {\em loss resilience} (quality in {\em presence} of packet loss).
%in {\em presence} of packet loss, whether the decoder can decode a frame soon after receiving some of its packets at a decent quality).
%The former means that in {\em absence} of packet loss, the decoded quality of a frame is high, in PSNR, SSIM or VMAF.
%The latter means that in {\em presence} of packet loss, the decoder can decode a frame soon after receiving some of its packets at a decent quality.
%, given the amount of data in the packets received before decoding.
Henceforth, we refer to 
%the delay before the receiver decodes a frame as its {\em frame delay}, and 
the fraction of data in packets that arrive after a frame's decoding as {\em data missing rate} or \rate. Note that a missing packet can be lost or delayed.


%and a packet arriving after the frame delay is referred to as a {\em missing packet}. 
%Note that a missed packet can be lost or delayed.
%%A packet of a frame is a {\em missing packet}, if it takes longer than the frame delay, and 
%We refer to the fraction of data in missing packets of a frame as {\em data missing rate} or \rate. 

Unfortunately, in real-time videos, existing loss-resilient techniques fall short on either loss resilience or compression efficiency (see \S\ref{??}).\footnote{
%Some techniques that work well in on-demand videos are much less effective in real-time videos. 
Scalable video coding (SVC~\cite{??}, FGS~\cite{??}, Swift~\cite{??}), which works well for on-demand streaming videos, is much less effective in real-time videos, because packets of a frame are sent together, rather than layer by layer (see \S\ref{??}).
For this reason, scalable video coding is not commonly used to improve unicast real-time videos~\cite{salsify}. 
%This corroborates the observation in~\cite{salsify}. 
Another line of work (\eg~\cite{voxel}) selectively skips frames that do not affect future frames (such as B-frames), but B-frames are seldom used in real-time videos, and I-frames, which stop the impact of skipped frames, are much fewer in real-time videos than in chunk-based videos. 
Nonetheless, we will still evaluate them against \name.}
%Despite many proposals, current loss-resilient techniques achieve loss resilience at the cost of lower compression efficiency (see \S\ref{??}).
%existing loss-resilient techniques improve loss resilience at the cost of lower compression efficiency.
For instance, for forward error correction (FEC) to tolerate $30\%$ \rate, (at least) $30\%$ redundancy must be added {\em before} sending the packets out~\cite{??}. 
If fewer than $30\%$ packets are actually missing (\ie~\rate is overestimated), 
%it overestimates \rate (\ie fewer than $x\%$ packets are actually missing), 
video quality will be lower than if no redundancy is added.
If \rate is underestimated, the receiver must wait longer and request the sender to resend packets, until at least 70\% of packets are received.
%(\eg FEC with \fillme\% redundancy in Figure~\ref{fig:intro-example} when \rate exceeds \fillme\%).
%(\eg FEC with \fillme\% redundancy in Figure~\ref{fig:intro-example} when \rate is below \fillme\%).
Similarly, using an older frame as encoding reference lets the decoder safely skip a frame without affecting future frames (\eg~\cite{salsify}), but older reference frame also significantly lowers compression efficiency (needs more bits to reach same quality).
As a result, most real-time Internet video systems increase loss resilience only {\em after} packet loss has affected some frames~\cite{??,??,streamingcoding}. 
%, and leaving some frames unprotected against burst of packet loss. 
%it also significantly reduces compression efficiency as older frames are more different with the current frame.




Ideally, a better solution, which we refer to as {\em Data-Scalable} ({\em DS}) video delivery, 
should gracefully degrade in presence of packet loss, without compromising quality in absence of packet loss.
%should have decent compression efficiency in presence of loss of {\em any} packets. 
Concretely, it should 
{\em (i)} reach a quality close to that of a non-loss-resilient coding algorithm (such as H.265), if all packets are received; 
{\em (ii)} be able to decode a frame if {\em any} (non-empty) subset of packets of the frame is received (\ie no retransmission unless all data are lost); and 
{\em (iii)} achieve better quality, if one more packet is received.
%As we have seen, prior work falls short on at least one front.



This paper presents {\em \name}, a real-time video system that uses {\em  autoencoders (AE)} to realize data-scalable DS video delivery for the first time.
%which explores a new approach to DS video delivery by using {\em neural-net (NN) autoencoders}.
At a high level, an autoencoder works like a standard video codec, except replacing part of the coding logic with neural networks (NNs). 
It uses an NN encoder to encode a frame ($\x$) to a {\em \aecode} ($\y$) (prior to entropy encoding), and uses an NN decoder to decode $\y$ to a reconstructed frame ($\z$) that is similar to $\x$. 


We choose autoencoders, not because off-the-shelf autoencoders are already data-scalable (DS), but because of their distinct properties that {\em could} enable DS coding. 
%\name is a particular design that harnesses these properties to enable DS coding.
Specifically, if we randomly set $n\%$ of elements in \aecode $\y$ to zeros, \ie {\em random data erasure}, the NN decoder of an autoencoder can still reconstruct the frame, and the difference in the decoding output between with and without the random data erasure grows with $n\%$. 
Thus, If we imagine the random data erasure is the impact of network packet loss on \aecode (we will explain how it could be done shortly), the above property means that video quality {\em could} degrade gradually with more packet loss.
This is in contrast to FEC, where quality does not grow with more data if packet loss rate is below a threshold but it drops abruptly once loss rate exceeds the threshold.
This relatively ``smooth'' relationship between decoder input and its output can be intuitively understood that that unlike traditional codecs, autoencoders do not have stringent structures or dependencies among the elements in a \aecodes.\footnote{Mathematically, the smoothness is a result of NN encoders and decoders having continuous derivatives everywhere. Moreover, NN decoders also resemble the architecture of variational autoencoder (VAE) which are {\em generative} models that can create realistic-looking images from random inputs.}





%Specifically, if the \aecode $\y$ is changed by a random noise $\delta$, the NN decoder of an autoencoder can always reconstruct a frame, and the difference between the decoding output of $\y$ and that of $\y+\delta$ grows with $\delta$. 
%If we imagine the noise $\delta$ as the impact of network packet loss on encoded data (we will explain how it could be done shortly), the above property means that video quality {\em could} degrade gradually with more packet loss.

Despite its promise, several key challenges remain to make autoencoders truly data-scalable in practice. 
\name addresses these challenges, and here we highlight two of them.
First, \name translates the effect of packet loss to random data erasure in \aecode, by a novel per-packet entropy encoding scheme.
Unlike standard autoencoders, we
% such that the effect of packet loss is the same as random data erasure in \aecode (\ie randomly set some elements to zeros).
%To this end, \name differently than 
randomly partitions an \aecode into sub-tensors and arithmetically codes each sub-tensor separately as a packet, and missing a packet effectively sets a random subset of elements in \aecode to zeros.
However, doing so naively can greatly inflate compressed data size due to extra space needed to encode each packet's symbol distribution. 
%Standard arithmetic coding incurs excessive size overhead per packet due to the need to store each packet's data distribution.
Instead, \name carefully coarsens the granularity of symbol distributions, which significantly reduces size inflation while preserving arithmetic coding's compression efficiency (see \S\ref{??} for details). 

Moreover, quality of existing autoencoders degrades quickly if more data is missing in an \aecode. 
This is because standard autoencoder training never trains autoencoders to decode a frame and subsequent frames in presence of substantial data loss on the encoder's output (\aecode).
\name uses a different autoencoder training process.
It applies random data erasures to each \aecode, which can simulate the effects of different \rates as explained shortly.
By varying the rate of data erasure (from 0\% to 90\%), 
%In other words, by training the NN encoder and NN decoder jointly, 
the new autoencoders not only learn how to compress frames efficiently but also how to be resilient to different \rates (see \S\ref{??} for details). 



%Second, unlike traditional codecs, autoencoders do not have stringent structures or dependencies among the elements in the encoder output (\aecodes).
%If we randomly set some elements of an \aecode to zeros (\ie random data erasures), the NN decoder can still reconstruct the whole frame with a decent quality.
%Importantly, 
%with more random data erasures on the {\em same} \aecode, video quality drops {\em gradually}, rather than abruptly as in FEC.
%% with more zeroed random elements in autoencoder-returned code (\ie higher random erasure rate).



%{\em if} packet loss is equivalent to random data erasure on \aecodes, video quality can degrade gracefully with higher \rates.
%To this end, 

\name also addresses several practical challenges associated with autoencoders, such as 
%\name also tackles other practical challenges, such as 
bitrate control, speeding up coding, and balancing the size of I-frames and P-frames.


\begin{comment}
\jc{
\begin{itemize}
\item nn property: small change doesn't dramatically change output (contrast with fec and h265) => randomness, smoothness, vae
\item but two challenges: quality drop still quite sharply, and overhead to per-packet entropy coding
\item our contributions
\end{itemize}
}

First, The NN decoder of an autoencoder {\em could} reconstruct frames from an \aecode $z$, even if some data in $z$ is lost between the encoder and the decoder.
Like many NNs which have continuous derivatives, when $z$ changes to $z+\delta_z$, autoencoder's output will change from $y$ to $y+\delta_y$ and $\delta_y$ will grow proportional with $\delta_z$.
Moreover, NN decoder resembles the architecture of variational autoencoder (VAE) which are {\em generative} models that create high-quality images even from a random input.

\end{comment}


\begin{comment}
\footnote{
The NN decoder architecture resembles a variational autoencoder (VAE), which creates realistic-looking images from a purely random tensor input!}
It can be intuitively understood that NNs having continuous derivatives, 
%\footnote{Encoder output is sometimes quantized, but quantization's effect on video quality is much less than data erasures caused by packet loss.}.


so that the decoder can loss between the encoder's output (\aecode) and the decoder's input, or handle long-term effect of packet loss. 
This is because in standard autoencoder training, the encoder output (\aecode) is almost always identical to the decoder input, and 
%have never seen any data erasure during the training. 
%To improve quality under data erasures, 



%By training the NN encoder and NN decoder jointly, they {\em could} learn to reconstruct high-quality frames in presence of random data erasures on the autoencoder-output code.


Second, unlike traditional codecs, autoencoders do not have stringent structures or dependencies among the elements in the encoder output (\aecodes).
If we randomly set some elements of an \aecode to zeros (\ie random data erasures), the NN decoder can still reconstruct the whole frame with a decent quality.
Importantly, 
with more random data erasures on the {\em same} \aecode, video quality drops {\em gradually}, rather than abruptly as in FEC.
% with more zeroed random elements in autoencoder-returned code (\ie higher random erasure rate).

Thus, {\em if} packet loss is equivalent to random data erasure on \aecodes, video quality can degrade gracefully with higher \rates.
To this end, \name runs arithmetic coding differently than standard autoencoders.
It randomly partitions an \aecode into sub-tensors and runs arithmetic coding to compress each sub-tensor as a separately decodable packet, so missing a packet only erases a random portion of the \aecode.
However, naive per-packet arithmetic coding greatly inflates data size due to extra space needed to encode each packet's symbol distribution. 
%Standard arithmetic coding incurs excessive size overhead per packet due to the need to store each packet's data distribution.
To address it, \name carefully coarsens the granularity of symbol distributions, which reduces the overhead to store symbol distribution while preserving arithmetic coding's compression efficiency (see \S\ref{??} for details). 

\name also addresses several practical challenges associated with autoencoders, such as 
%\name also tackles other practical challenges, such as 
bitrate control, speeding up coding, and balancing the size of I-frames and P-frames.

\end{comment}

\begin{comment}


First, autoencoder-output tensors do not impose stringent structures or dependencies among their elements. 
If we randomly set some elements of an autoencoder-output tensor to zeros (\ie random data erasures), the NN decoder can still reconstruct the whole frame with a decent quality (though with room for improvement).
More importantly, if we apply more random data erasures on the {\em same} autoencoder-output tensor, video quality will drop {\em gradually}, rather than abruptly as in FEC.
% with more zeroed random elements in autoencoder-returned code (\ie higher random erasure rate).
These suggest that video quality {\em could} degrade gracefully with higher \rates, {\em if} packet loss is equivalent to random data erasure on autoencoder-output tensor.

To this end, we change the arithmetic coding in standard autoencoders and classic codecs. 
%\name changes the arithmetic coding in standard autoencoders, which encodes the whole autoencoder-output tensor as a whole. 
%Instead, we 
\name first randomly partitions an autoencoder-output tensor into sub-tensors and runs arithmetic coding to compress each sub-tensor as a separately decodable packet.
Thus, missing a packet only erases a random portion of the elements in the tensor.
While seemingly straightforward, per-packet arithmetic coding, if done naively, will greatly inflate the coded data size due to extra space needed to encode the data distributions of different packets. 
%Standard arithmetic coding incurs excessive size overhead per packet due to the need to store each packet's data distribution.
To address it, \name carefully coarsen the granularity of the per-packet data distribution, which greatly reduces the overhead to store data distribution while preserving the efficiency of arithmetic coding (see \S\ref{??} for details). 
%the size overhead and efficiency of per-packet arithmetic coding 
%\jc{Yihua, a footnote on how does CABAC gets around it and why isn't it easily applicable to us?} 

Second, the NN decoder in an autoencoder could be used as a generative model. 
Theoretically, it can learn to act like a variational autoencoder (VAE), which can create realistic-looking high-quality images from a purely {\em random} tensor!
By training the NN encoder and NN decoder jointly, they {\em could} learn to reconstruct high-quality frames in presence of random data erasures on the autoencoder-output code.


Quality of existing autoencoders quality will degrade quickly with more random erasures.
This is because in standard autoencoder training, the encoder output is almost\footnote{Encoder output is sometimes quantized, but quantization's effect on video quality is much less than data erasures caused by packet loss.} always identical to the decoder input. 
%have never seen any data erasure during the training. 
%To improve quality under data erasures, 
\name uses a different autoencoder training process---it injecting random data erasures of various rates (from 0\% to 90\%) between the encoder and the decoder, which simulates the effects of different \rates.
In other words, the new autoencoders not only learn how to compress frames efficiently but also how to code them in a way resilient to different \rates (see \S\ref{??} for details). 

\end{comment}



%the rate of random erasures (more zeroed elements). 

%, which as explained in \S\ref{??} could mimic the effect of packet loss, the decoder can still decode the whole frame. 

\begin{comment}

because the elements in an autoencoder-output tensor have much less dependency among them.

To let autoencoders function under packet loss, we first change entropy encoding---instead of entropy coding the entire autoencoder-output tensor to a bitstream and then packetizing it to packets




\name chooses autoencoders, because the elements in an autoencoder-output tensor have much less dependency among them.
If we randomly select some elements of an autoencoder-returned code (\ie random erasures) and set them to zero, which as explained in \S\ref{??} could mimic the effect of packet loss, the decoder can still decode the whole frame. 
In contrast, missing information in H.264 
% will not render the whole frame undecodable. 
%does not have dramatic impact on the decoded video quality.
This is in contrast to SVC where any data loss on a low layer also affects higher layers.
Moreover, the impact of random erasures on video quality increases with the rate of random erasures (\eg more zeroed elements). 
In other words, unlike FEC needs to known \rate~{\em a priori}, the quality of autoencoders {\em could} degrade gracefully with more data loss.


We use autoencoders because they have two {\em potential} advantages.
First, there is little explicit dependency among the elements of an autoencoder-returned tensor. 
Thus, unlike in SVC where any data loss on a lower layer also affects higher layers, applying any random erasures (such as zeroing randomly selected elements) on an output tensor of an autoencoder will not have a dramatic impact on the decoded video quality.
%In other words, so the values in the tensor do not need to be received in specific order, like in SVC. 
Second, the impact of random perturbation on video quality {\em could} be further reduced by training the autoencoder to work under different random erasure rates. 
The resulting autoencoders might be better than FEC which only tolerates a pre-determined data loss rate.
%one autoencoder (a pair of NN encoder and NN decoder) could be trained to work under a {\em range} of data erasure rates and still achieve decent quality.


Yet, traditional autoencoders are ill-suited for real-time videos. 
Here, we highlight how \name addresses two specific challenges to enable autoencoder-based DS video delivery.



First, traditional autoencoder-returned code could be decoded in presence of data loss, but its quality will degrade quickly with more random erasures.
This is because in standard autoencoder training, the encoder output is almost\footnote{Encoder output is sometimes quantized (lower float precision), but quantization's effect on video quality is much less than data erasures caused by packet loss.} always identical to the decoder input. 
%have never seen any data erasure during the training. 
%To improve quality under data erasures, 
\name uses a different autoencoder training process---it injecting random data erasures of various rates (from 0\% to 90\%) between the encoder and the decoder, which simulates the effects of different \rates.
In other words, the new autoencoders not only learn how to compress frames efficiently but also how to code them in a way resilient to different \rates (see \S\ref{??} for details). 

Second, existing autoencoders and standard video codecs use arithmetic coding to compress all information of a frame to a single bitstream which will then be packetized. 
This means that any packet loss will render the data undecodable.
%If this bitstream is packetized, as done in conventional real-time video systems, any packet loss will render the data undecodable.
Instead, \name first randomly partitions the autoencoder-returned code to sub-tensors and then arithmetically codes each sub-tensor as a separate packet.
Though it sounds easy, per-packet arithmetic coding turns out to be challenging, since traditional arithmetic coding incurs excessive size overhead per packet due to the need to store each packet's data distribution. 
\name addresses it using a novel scheme to balance the size overhead and efficiency of per-packet arithmetic coding (see \S\ref{??}). 

\end{comment}

%As an end-to-end video coding framework, 
%\name also tackles other practical challenges, such as efficient bitrate control, speeding up of autoencoders, and balancing the size of I-frames and P-frames.


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/fig1-example.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/fig1-example-osdi.pdf}
        \includegraphics[width=0.99\linewidth]{figs/fig1-example-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{Example results of \name's (a) more graceful degradation in presence of packet loss than prior solutions, and (b) better tradeoffs between video quality and tail frame delay, which corroborates the subjective rating of users.
         More results can be found in \S\ref{sec:eval}. 
%         \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
    \jc{TODO: add a horizontal line to indicate the quality of H.265}
         }
%    \tightcaption{Video quality vs. \rates of different video codecs when the actual encoded bitrate is 3.6 Mbps (which includes FEC redundancy if used.)
%    Quality of \name's autoencoder degrades gracefully with higher \rates. 
%%    achieves a smoother quality degradation as packet loss rate increases.
%    More results can be found in \S\ref{sec:eval}. 
%%    \jc{Yihua, can you replot the FEC lines to use the same color (w/ diff point/line types)}
%%    \jc{Yihua, can you add (DSC) next to our solution?}
%%    \jc{Yihua, can we also replace yellow with 50\% redundancy?}
%    %\jc{YIHUA, remember to add a line of 264 without loss, and remove the part of h264 when it's undecodable}\jc{set R-D optimization to "intra-MB insertion"}
%%    \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
%%    \jc{Yihua, can you add a horizontal line to indicate the quality of H.265}
%    }
    \label{fig:intro-example}
    % \vspace{-0.5cm}
\end{figure}




We should also clarify what \name does {\em not} do.
\name decides {\em what} each packet contains, but it rate adaptation. 
Instead, it uses existing rate adaptation logics, such as GCC~\cite{??}, to decide the target bitrate of a frame and how fast to send its packets.
%, so that even if the selected bitrate overshoots the bandwidth, we can still obtain decent quality.
Moreover, \name aims at unicast video communication, rather than multi-party conferencing.

%Being a coding system, \name can work with existing congestion control (CC) logics---CC decides how fast to send packets, and \name decides {\em what} each packet contains.


To put it in context, \name is, to our best knowledge, the first to demonstrates that autoencoders could remarkably improve loss resilience in real-time communication.
Autoencoders have long been used in multimedia and data communication (see \S\ref{sec:related}) but mostly for better compression efficiency.
Swift and DeepFGS, for instance, use autoencoders to improve scalable video coding for on-demand videos~\cite{swift,??}. 
\name is also related to DeepJSCC which uses autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises~\cite{??} (rather than packet loss).
%for compressing images and signals in wireless communication and 


\begin{comment}
To put \name in perspective, autoencoders have long been used in data communication~\cite{erpek2020deep} (see \S\ref{sec:related}).
\name, which can be seen as joint-source-channel coder, is similar 
%As a joint-source-channel coder, \name's autoencoder is similar 
in spirit to DeepJSCC which uses autoencoder to compress static images (rather than real-time videos) in a way robust to wireless signal noises~\cite{??} (rather than packet loss).
%for compressing images and signals in wireless communication and 
Recently, Swift uses autoencoders to improve scalable video coding (SVC) for on-demand videos~\cite{swift}. 
To our best knowledge, \name is the first video framework to demonstrates the potential of autoencoders to improve loss resilience in real-time communication.
\end{comment}

%Much remains unknown about the limits of autoencoders as a loss-resilient coding layer.

%To our best knowledge, \name is the first end-to-end autoencoder-based video system for loss-resilient real-time videos.
%that achieves stream real-time videos in a data-scalable fashion. 



%arising from training and using autoencoders in real-time video communication.

%Many aspects of \name are also inspired by prior work. 
%That said, \name, to our best knowledge, is the first to develop custom autoencoders that realize data-scalable video delivery.

%\name aims at unicast video sessions, rather than multi-party conferences. 
%It is also important that \name's autoencoders do {\em not} achieve better compression efficiency than recent heavily engineered video codecs, such as H.265. 
%Indeed, \name's video quality is still slightly lower than H.265 at the same bitrate. 

We have implemented and evaluated \name in two aspects (Figure~\ref{fig:intro-example} gives an example). 
First, on various video content, \name's quality degrades more gracefully under packet loss than other loss-resilient coding.
%, without much compromise on quality in absence of packet loss. 
That said, in absence of packet loss, \name's quality is slightly lower than H.265 at the same bitrate. \jc{need to update this}
% which is comparable or less than adding 10\% FEC redundancy. 
%does {\em not} outperform the latest heavily engineered video codecs in quality---indeed, \name's video quality is slightly lower than H.265 at the same bitrate. 
Second, using real-world network traces and a packet-level simulator, we show that \name significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to the most competitive baselines which still have to retransmit packets or skip frames.
This greatly decreases video stuttering and skipped frames---our user study confirms that \name has much higher average subjective rating by users than the most competitive baselines.

\begin{comment}
Using real-world and synthetic network traces and a wide range of videos, we show that \name's autoencoder has a more graceful quality degradation under packet loss than baseline loss-resilient video codecs.
%, without sacrificing video quality in absence of packet loss 
(Figure~\ref{fig:intro-example} gives an example).
When comparing \name with the baselines with the same CC logic (\eg GCC~\cite{??} and Salsify-CC~\cite{??}), \name significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to prior work which has to retransmit packets or skip frames, with the comparable video quality.
To put it in perspective, \name significantly decrease the frames that arrive after user-perceivable delay (\eg 200ms for video calls) and reduces video stuttering.
\end{comment}

%Our results show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile when prior work has to retransmit packets or skip frame), with the marginally lowered video quality.
%To put it in perspective, \name can significantly reduce the chance that frames arrive after user-perceivable delay (\eg 200ms for video conferencing) and improve playback smoothness (higher frame rate).

%\jc{ae has caveats (size, speed, efficiency). }
%\jc{this paper above all shows a new design space}

\textbf{This work does not raise any ethical issues.}






%unlike SVC, the output tensor of an autoencoder does {\em not} impose a hierarchical structure among its elements, so the values in the tensor do not need to be received in specific order, like in SVC. 
%Instead, randomly perturbing a tensor in the new embedding space, such as zeroing any $\alpha\%$ of a tensor's elements, will have only a {\em limited} impact (proportional to $\alpha\%$)  on the quality of the decoded frame.
%Second, unlike FEC which only tolerates a pre-determined data loss rate, one autoencoder (a pair of NN encoder and NN decoder) could be trained to achieve desirable quality under a {\em range} of data erasure rates. 

%To be specific, each frame is supposed to be decoded at a fixed interval after the last frame was decoded, and 
%
%a packet associated with a frame will delay the rendering of a 
%To be more specific, we call a packet as a {\em missing packet}, if it arrives after when the frame it belongs to should be decoded (\eg 40ms after the last frame is decoded under 25fps), and we refer to the fraction of data in missing packets of a frame as {\em data missing rate} or \rate. 
%Note that a missed packet can be lost or delayed.






==> sections/old/intro_v11.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}

Real-time video communication has a long history in research, yet only recently has it become truly widespread in our daily lives~\cite{blum2021webrtc}, from online meetings~\cite{webrtc-vc-1,webrtc-vc-2}, cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2}, to interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2} and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
The amount of time people spend on real-time videos is growing at a much faster rate than the time spent on streaming videos, whether live and on-demand~\cite{webrtc-trend-1,webrtc-trend-2}.
%As a result, users expect that each frame has a high quality, that no frame is skipped, and 
%that each frame is decoded on time such that the viewer sees a smooth playback (\eg under 25fps, a frame should be decoded every 40~ms). 

Despite its growing popularity, users of real-time video applications (\eg video calls and online gaming) are more susceptible to poor quality and video stuttering compared to those who watch on-demand videos (\eg Netflix)~\cite{gaming-asurion, vca-vice}, especially in long-latency links (\eg long-distance video calls). 
In on-demand video streaming, the delay of retransmitting packets, which can be 100s ms or higher in long-latency links, can be concealed by the buffer, but real-time videos use a very short jitter buffer (\eg merely \fillme ms in WebRTC)~\cite{??}  in order to play each frame as soon as it is decoded.
As a result, the additional delay to wait or resend a single packet frame might block the decoding of multiple frames and cause a visual stuttering. 

\begin{comment}
resending {\em any} lost or delayed packets could increase the {\em frame delay}---the time between sending a frame and receiving enough data to decode it, 

%, even when the network is connected, \eg video freezes when audio continues~\cite{??}. 
This is because real-time video applications use a short jitter buffer (\eg \fillme ms in WebRTC).
 resending a single packet takes one round-trip time which can be a few hundreds of milliseconds, blocking the decoding of multiple frames and causing a visual stuttering. 

, which makes them more vulnerable to lost or delayed packets.
Resending {\em any} lost or delayed packets leads to increased {\em frame delay}---the time between sending a frame and receiving enough data to decode it.
This issue is particularly pronounced in long-latency links (\eg long-distance video calls or bufferbloat), where resending a single packet takes one round-trip time and block the decoding of multiple frames.
\end{comment}

Loss-resilient video coding is, thus,
%which decodes a frame at a decent quality in presence of packet loss, 
key to high quality  and smooth playback of real-time videos.
%We use {\em data missing rate} or \rate to refer to 
%%the delay before the receiver decodes a frame as its {\em frame delay}, and 
%the portion of packet data that is not received (due to packet dropping or delaying) before a frame is decoded.
Ideally, it should have high {\em compression efficiency} in {\em absence} of packet loss and {\em loss resilience} under various {\em data missing rate} or \rate, which we use to refer to
%the delay before the receiver decodes a frame as its {\em frame delay}, and 
the fraction of data that is not received (due to packet drops or queuing) before a frame is decoded.

%The effectiveness of a loss-resilient coding scheme can be evaluated by {\em compression efficiency} (quality in {\em absence} of packet loss) and {\em loss resilience} (quality in {\em presence} of packet loss).
%in {\em presence} of packet loss, whether the decoder can decode a frame soon after receiving some of its packets at a decent quality).
%The former means that in {\em absence} of packet loss, the decoded quality of a frame is high, in PSNR, SSIM or VMAF.
%The latter means that in {\em presence} of packet loss, the decoder can decode a frame soon after receiving some of its packets at a decent quality.
%, given the amount of data in the packets received before decoding.


%and a packet arriving after the frame delay is referred to as a {\em missing packet}. 
%Note that a missed packet can be lost or delayed.
%%A packet of a frame is a {\em missing packet}, if it takes longer than the frame delay, and 
%We refer to the fraction of data in missing packets of a frame as {\em data missing rate} or \rate. 


Current real-time video systems, unfortunately, achieve loss resilience by adding various redundancies, thus sacrificing compression efficiency.\footnote{
Scalable video coding (SVC~\cite{??}, FGS~\cite{??}, Swift~\cite{??}), which works well for on-demand streaming videos, will be much less effective in real-time videos which send packets of a frame together, instead of layer by layer (see \S\ref{??}).
For this reason, scalable video coding is not commonly used to improve unicast real-time videos~\cite{salsify}. 
Similarly, selective frame skipping (\eg~\cite{voxel}) might work for on-demand videos, but in real-time videos, most frames are P-frames which cause poor quality once dropped, unless I-frames are frequently inserted.
Nonetheless, we will still evaluate them against \name.}
To handle $30\%$ \rate, for instance, forward error correction (FEC) needs to add (at least) $30\%$ redundancy {\em before} transmission~\cite{??}. 
For this reason, most real-time video systems only increase FEC redundancy after packet loss has affected some frames~\cite{??,??,streamingcoding}.
For these frames whose \rate is underestimated, the receiver must still wait or request the sender to resend some packets until at least 70\% of packets have arrived.
At the same time, FEC may add too much redundancy even after the packet loss has subsided, when it happens, the video quality will be lower than it could have been with much lower or no added redundancy. 


\begin{comment}

Current real-time video systems, unfortunately, 
%fall short in either loss resilience or compression efficiency.
achieve loss resilience by adding various redundancies, thus sacrificing compression efficiency.\footnote{
%Some techniques that work well in on-demand videos are much less effective in real-time videos. 
Scalable video coding (SVC~\cite{??}, FGS~\cite{??}, Swift~\cite{??}), which works well for on-demand streaming videos, will be much less effective in real-time videos which send packets of a frame together, instead of layer by layer (see \S\ref{??}).
For this reason, scalable video coding is not commonly used to improve unicast real-time videos~\cite{salsify}. 
%This corroborates the observation in~\cite{salsify}. 
Similarly, frame skipping (\eg~\cite{voxel}) might work for on-demand videos, but in real-time videos, most frames are P-frames which cause poor quality once dropped, unless I-frames are frequently inserted.
%Another line of work (\eg~\cite{voxel}) selectively skips frames (mostly B-frames) that do not affect future frames, but B-frames are rarely used in real-time videos, and I-frames, which stop the impact of frame skipping, are much fewer in real-time videos than in chunk-based videos. 
Nonetheless, we will still evaluate them against \name.}
%Despite many proposals, current loss-resilient techniques achieve loss resilience at the cost of lower compression efficiency (see \S\ref{??}).
%existing loss-resilient techniques improve loss resilience at the cost of lower compression efficiency.
For instance, to handle $30\%$ \rate, forward error correction (FEC) needs to add (at least) $30\%$ redundancy {\em before} transmission~\cite{??}. 
If the actual \rate is below 30\%, 
%it overestimates \rate (\ie fewer than $x\%$ packets are actually missing), 
the video quality will be lower than if no redundancy is added in the first place.
If \rate is underestimated, the receiver must wait or request the sender to resend some packets until at least 70\% of packets have arrived.
%(\eg FEC with \fillme\% redundancy in Figure~\ref{fig:intro-example} when \rate exceeds \fillme\%).
%(\eg FEC with \fillme\% redundancy in Figure~\ref{fig:intro-example} when \rate is below \fillme\%).
An alternative loss resilient coding uses an older but reliably received frame as the reference frame, allowing the decoder to safely skip loss-affected frames (\eg~\cite{salsify}).
%without hurting future frames, 
However, using an old reference frame requires more encoded bits to achieve same quality as using the last reference frame (\ie low compression efficiency).
%reduces compression efficiency as more bits are needed to encode the difference between the current frame and an old frame.
For these reasons, most real-time video systems only increase loss resilience after packet loss has affected some frames~\cite{??,??,streamingcoding}, and sometimes they add too much redundancy even after the packet loss has subsided. 
%As a result, most real-time Internet video systems only increase loss resilience {\em after} packet loss has impacted some frames~\cite{??,??,streamingcoding}. 
%, and leaving some frames unprotected against burst of packet loss. 
%it also significantly reduces compression efficiency as older frames are more different with the current frame.

\end{comment}



Ideally, the quality should degrade gracefully with more packet loss (higher \rate), without compromising the quality in absence of packet loss.
Specifically, it should be able to 
{\em (i)} decode a frame as long as {\em any} (non-empty) subset of packets of the frame is received;
%(\ie no need for retransmission unless all data is lost);  
{\em (ii)} achieve better quality with the addition of each new packet (\ie lower \rate); and
{\em (iii)}  reach a quality close to a non-loss-resilient coding algorithm (such as H.265), when all packets are received.
We refer to it as {\em Data-Scalable} ({\em DS}) video coding.
FEC is not DS coding, since its quality does not improve with more data if the packet loss rate is below a threshold but the quality drops abruptly once loss rate exceeds the threshold.


\begin{comment}

An ideal solution, which we refer to as {\em Data-Scalable} ({\em DS}) video coding, should have a  graceful degradation of video quality with more packet loss (higher \rate), without compromising quality in absence of packet loss.
%should have decent compression efficiency in presence of loss of {\em any} packets. 
Specifically, it should be able to 
{\em (i)} decode a frame as long as {\em any} (non-empty) subset of packets of the frame is received;
%(\ie no need for retransmission unless all data is lost);  
{\em (ii)} achieve better quality with the addition of each new packet; and
{\em (iii)}  reach a quality level close to a non-loss-resilient coding algorithm (such as H.265), when all packets are received.
For instance, forward error correction (FEC) is not DS coding, since its quality does not improve with more data if the packet loss rate is below a threshold but the quality drops abruptly once loss rate exceeds the threshold.

\end{comment}


%{\em (i)} reach a quality level close to a non-loss-resilient coding algorithm (such as H.265), when all packets are received; 
%{\em (ii)} allowing for decoding a frame with {\em any} (non-empty) subset of packets of the frame is received (\ie no need for retransmission unless all data is lost); and 
%{\em (iii)} achieve better quality with the addition of each new packet.
%As we have seen, prior work falls short on at least one front.


\mypara{Data-scalable autoencoder}
This paper introduces {\em \name}, a real-time video system that, for the first time, uses {\em  autoencoders (AEs)} to realize data-scalable (DS) video delivery.
%which explores a new approach to DS video delivery by using {\em neural-net (NN) autoencoders}.
At a high level, autoencoders work like a standard video codec but replace some coding logic with neural networks (NNs). 
It uses an NN encoder to encode a frame to a {\em \aecode} (without entropy encoding), and an NN decoder to decode to a reconstructed frame that is similar to the original frame. 


We choose autoencoders, not because the off-the-shelf models are inherently data-scalable (DS), but due to their unique properties that {\em could} enable DS coding. 
%\name is a particular design that harnesses these properties to enable DS coding.
Specifically, the NN decoder can reconstruct a decent-quality frame, even if we {\em randomly erase} (\ie set to zeroes) a subset of $n\%$ elements in the \aecode (the output of the NN encoder).
In other words, {\em random data erasure} on the \aecode has a limited impact on the decoding quality of autoencoders. 
This can be attributed to the lack of stringent dependencies among the elements in a \aecode\footnote{
%Mathematically, this smoothness is a result of NN encoders and decoders having continuous derivatives everywhere. Moreover, 
This can also be intuitively understood that NN decoders share the architecture of {\em generative} NNs, such as variational autoencoder (VAE), which can create realistic-looking images from random inputs.}, unlike SVC where the decoding of a layer depends on the lower layers.



\begin{comment}


The implication is that {\em if} packet loss (with \rate of $n\%$) has the same effect on \aecode as random data erasure of $n\%$, then the video would be decodable under various packet loss patterns, and the quality {\em could} degrade with more packet loss.


The reason for this relatively ``smooth'' relationship between the input and output of NN decoder is that 
autoencoders, unlike SVC, do not have stringent structures or dependencies among the elements in a \aecode.\footnote{Mathematically, the smoothness is a result of NN encoders and decoders having continuous derivatives everywhere. Moreover, NN decoders also resemble the architecture of variational autoencoder (VAE) which are {\em generative} models that can create realistic-looking images from random inputs.}

 fact that that, unlike traditional codecs, autoencoders do not have stringent structures or dependencies among the elements in a \aecodes.\footnote{Mathematically, the smoothness is a result of NN encoders and decoders having continuous derivatives everywhere. Moreover, NN decoders also resemble the architecture of variational autoencoder (VAE) which are {\em generative} models that can create realistic-looking images from random inputs.}
This is also in contrast to forward error correction (FEC), where quality does not improve with more data if the packet loss rate is below a threshold but the quality drops abruptly once loss rate exceeds the threshold.


Moreover, the difference in the decoding output between with and without such random data erasure grows with $n\%$. 
This means that {\em if} packet loss (with \rate of $n\%$) has the same effect on \aecode as random data erasure of $n\%$, then video quality might degrade with more packet loss.

\end{comment}




%Specifically, if the \aecode $\y$ is changed by a random noise $\delta$, the NN decoder of an autoencoder can always reconstruct a frame, and the difference between the decoding output of $\y$ and that of $\y+\delta$ grows with $\delta$. 
%If we imagine the noise $\delta$ as the impact of network packet loss on encoded data (we will explain how it could be done shortly), the above property means that video quality {\em could} degrade gradually with more packet loss.


Despite the promise of autoencoders, several practical challenges remain.
%\name addresses several practical challenges.
Two of them will be highlighted here.

%Despite the promise of autoencoders, \name must address several practical challenges, such as improving quality under various \rates, making entropy encoding of \aecodes loss-resilient, controlling bitrate, and speeding up autoencoder coding. 
%Two of them will be highlighted here.

\begin{comment}
Despite the promise of autoencoders, several practical challenges remain, 
%to make autoencoders data-scalable in practice, 
such as improving quality under various \rates, making entropy encoding of \aecodes loss-resilient,
%packet loss to random data erasure in \aecodes, 
controlling bitrate, and speeding up autoencoder coding. %, and balancing I-frame and P-frame size. 
\name addresses these challenges, and two of them will be highlighted here.
\end{comment}


%\mypara{Adding packet loss in autoencoder training}
\mypara{Training autoencoder with packet loss}
First, the quality of standard autoencoders drops quite significantly if more data is erased from the \aecode. 
This is because the standard autoencoder training, in which  the decoder always sees the same \aecode returned by the encoder, never prepares the autoencoder to handle any data loss between the encoder and the decoder. 
\name trains autoencoders different (see \S\ref{??} for details).
It applies random data erasures to the \aecode (which could simulate the effect of packet loss as explained shortly), and by varying the rate of data erasure between [0\%, 100\%), 
%In other words, by training the NN encoder and NN decoder jointly, 
the new autoencoders not only learn how to compress high-quality frames efficiently but also to be robust to different rates of random data erasures. 

\begin{comment}
in standard autoencoder training,
%when training these autoencoders, 
the decoder sees the same \aecode returned by the encoder.
%the \aecode returned by the encoder is identical to the input of the decoder. 
Thus, the training does not prepare the autoencoder to handle any data loss between the encoder and the decoder. 
% a lossless channel between the encoder and the decoder).
%never trains autoencoders to decode a frame and subsequent frames in presence of substantial data loss on the encoder's output (\aecode).
\end{comment}

%, which simulates the effects of packet loss under different \rates (which will be explained shortly).


\mypara{Per-packet entropy coding for autoencoder}
Standard autoencoders use entropy encoding to losslessly compress a \aecode to a single bitstream and then packetize it, so any packet loss will render it undecodable.
%entropy coding used in current autoencoders cannot tolerate any packet loss. 
A naive idea is to randomly 
split the \aecode's elements to partitions,
%split a \aecode to sub-tensors, 
each separately entropy-encoded as an independently decodable packet, and if $n\%$ packets are lost, we set their elements in the \aecode to zeros, which resembles random erasure.
%effectively erases a random subset of $n\%$ elements.
%is the same as 
%random data erasure.
However, this naive per-packet entropy coding greatly increases the size of the compressed data, due to the additional space needed to store the symbol distribution (used by entropy-decoding) in each packet.
%To mitigate the size increase, 
\name carefully coarsens the granularity of symbol distributions, which significantly reduces size increase while maintaining the compression efficiency of entropy coding (see \S\ref{??} for details). 


\begin{comment}

A naive method would be 
%translate the effect of packet loss to random data erasure on \aecodes would be 
to randomly partition a \aecode into smaller sub-tensors and then arithmetically code each sub-tensor separately as a packet.
If a packet is missing, we set its elements in \aecode to zeros, which effectively mimics random data erasure.
%effectively sets a random set of elements to zeros.
However, this approach greatly increases the size of the compressed data, due to the additional space required to encode the symbol distribution of each packet.
To avoid this, \name carefully coarsens the granularity of symbol distributions, which significantly reduces size increase while maintaining the compression efficiency of arithmetic coding (as described in details in \S\ref{??}). 

\end{comment}

\begin{comment}

\name translates the effect of packet loss to random data erasure in \aecode, by a novel per-packet entropy encoding scheme.
Unlike standard autoencoders, we
% such that the effect of packet loss is the same as random data erasure in \aecode (\ie randomly set some elements to zeros).
%To this end, \name differently than 
randomly partitions an \aecode into sub-tensors and arithmetically codes each sub-tensor separately as a packet, and missing a packet effectively sets a random subset of elements in \aecode to zeros.
However, doing so naively can greatly inflate compressed data size due to extra space needed to encode each packet's symbol distribution. 
%Standard arithmetic coding incurs excessive size overhead per packet due to the need to store each packet's data distribution.
Instead, \name carefully coarsens the granularity of symbol distributions, which significantly reduces size inflation while preserving arithmetic coding's compression efficiency (see \S\ref{??} for details). 

\name also addresses several practical challenges associated with autoencoders, such as 
%\name also tackles other practical challenges, such as 
bitrate control, speeding up coding, and balancing the size of I-frames and P-frames.

\end{comment}




%Second, unlike traditional codecs, autoencoders do not have stringent structures or dependencies among the elements in the encoder output (\aecodes).
%If we randomly set some elements of an \aecode to zeros (\ie random data erasures), the NN decoder can still reconstruct the whole frame with a decent quality.
%Importantly, 
%with more random data erasures on the {\em same} \aecode, video quality drops {\em gradually}, rather than abruptly as in FEC.
%% with more zeroed random elements in autoencoder-returned code (\ie higher random erasure rate).



%{\em if} packet loss is equivalent to random data erasure on \aecodes, video quality can degrade gracefully with higher \rates.
%To this end, 

\begin{comment}
\jc{
\begin{itemize}
\item nn property: small change doesn't dramatically change output (contrast with fec and h265) => randomness, smoothness, vae
\item but two challenges: quality drop still quite sharply, and overhead to per-packet entropy coding
\item our contributions
\end{itemize}
}

First, The NN decoder of an autoencoder {\em could} reconstruct frames from an \aecode $z$, even if some data in $z$ is lost between the encoder and the decoder.
Like many NNs which have continuous derivatives, when $z$ changes to $z+\delta_z$, autoencoder's output will change from $y$ to $y+\delta_y$ and $\delta_y$ will grow proportional with $\delta_z$.
Moreover, NN decoder resembles the architecture of variational autoencoder (VAE) which are {\em generative} models that create high-quality images even from a random input.

\end{comment}


\begin{comment}
\footnote{
The NN decoder architecture resembles a variational autoencoder (VAE), which creates realistic-looking images from a purely random tensor input!}
It can be intuitively understood that NNs having continuous derivatives, 
%\footnote{Encoder output is sometimes quantized, but quantization's effect on video quality is much less than data erasures caused by packet loss.}.


so that the decoder can loss between the encoder's output (\aecode) and the decoder's input, or handle long-term effect of packet loss. 
This is because in standard autoencoder training, the encoder output (\aecode) is almost always identical to the decoder input, and 
%have never seen any data erasure during the training. 
%To improve quality under data erasures, 



%By training the NN encoder and NN decoder jointly, they {\em could} learn to reconstruct high-quality frames in presence of random data erasures on the autoencoder-output code.


Second, unlike traditional codecs, autoencoders do not have stringent structures or dependencies among the elements in the encoder output (\aecodes).
If we randomly set some elements of an \aecode to zeros (\ie random data erasures), the NN decoder can still reconstruct the whole frame with a decent quality.
Importantly, 
with more random data erasures on the {\em same} \aecode, video quality drops {\em gradually}, rather than abruptly as in FEC.
% with more zeroed random elements in autoencoder-returned code (\ie higher random erasure rate).

Thus, {\em if} packet loss is equivalent to random data erasure on \aecodes, video quality can degrade gracefully with higher \rates.
To this end, \name runs arithmetic coding differently than standard autoencoders.
It randomly partitions an \aecode into sub-tensors and runs arithmetic coding to compress each sub-tensor as a separately decodable packet, so missing a packet only erases a random portion of the \aecode.
However, naive per-packet arithmetic coding greatly inflates data size due to extra space needed to encode each packet's symbol distribution. 
%Standard arithmetic coding incurs excessive size overhead per packet due to the need to store each packet's data distribution.
To address it, \name carefully coarsens the granularity of symbol distributions, which reduces the overhead to store symbol distribution while preserving arithmetic coding's compression efficiency (see \S\ref{??} for details). 

\name also addresses several practical challenges associated with autoencoders, such as 
%\name also tackles other practical challenges, such as 
bitrate control, speeding up coding, and balancing the size of I-frames and P-frames.

\end{comment}

\begin{comment}


First, autoencoder-output tensors do not impose stringent structures or dependencies among their elements. 
If we randomly set some elements of an autoencoder-output tensor to zeros (\ie random data erasures), the NN decoder can still reconstruct the whole frame with a decent quality (though with room for improvement).
More importantly, if we apply more random data erasures on the {\em same} autoencoder-output tensor, video quality will drop {\em gradually}, rather than abruptly as in FEC.
% with more zeroed random elements in autoencoder-returned code (\ie higher random erasure rate).
These suggest that video quality {\em could} degrade gracefully with higher \rates, {\em if} packet loss is equivalent to random data erasure on autoencoder-output tensor.

To this end, we change the arithmetic coding in standard autoencoders and classic codecs. 
%\name changes the arithmetic coding in standard autoencoders, which encodes the whole autoencoder-output tensor as a whole. 
%Instead, we 
\name first randomly partitions an autoencoder-output tensor into sub-tensors and runs arithmetic coding to compress each sub-tensor as a separately decodable packet.
Thus, missing a packet only erases a random portion of the elements in the tensor.
While seemingly straightforward, per-packet arithmetic coding, if done naively, will greatly inflate the coded data size due to extra space needed to encode the data distributions of different packets. 
%Standard arithmetic coding incurs excessive size overhead per packet due to the need to store each packet's data distribution.
To address it, \name carefully coarsen the granularity of the per-packet data distribution, which greatly reduces the overhead to store data distribution while preserving the efficiency of arithmetic coding (see \S\ref{??} for details). 
%the size overhead and efficiency of per-packet arithmetic coding 
%\jc{Yihua, a footnote on how does CABAC gets around it and why isn't it easily applicable to us?} 

Second, the NN decoder in an autoencoder could be used as a generative model. 
Theoretically, it can learn to act like a variational autoencoder (VAE), which can create realistic-looking high-quality images from a purely {\em random} tensor!
By training the NN encoder and NN decoder jointly, they {\em could} learn to reconstruct high-quality frames in presence of random data erasures on the autoencoder-output code.


Quality of existing autoencoders quality will degrade quickly with more random erasures.
This is because in standard autoencoder training, the encoder output is almost\footnote{Encoder output is sometimes quantized, but quantization's effect on video quality is much less than data erasures caused by packet loss.} always identical to the decoder input. 
%have never seen any data erasure during the training. 
%To improve quality under data erasures, 
\name uses a different autoencoder training process---it injecting random data erasures of various rates (from 0\% to 90\%) between the encoder and the decoder, which simulates the effects of different \rates.
In other words, the new autoencoders not only learn how to compress frames efficiently but also how to code them in a way resilient to different \rates (see \S\ref{??} for details). 

\end{comment}



%the rate of random erasures (more zeroed elements). 

%, which as explained in \S\ref{??} could mimic the effect of packet loss, the decoder can still decode the whole frame. 

\begin{comment}

because the elements in an autoencoder-output tensor have much less dependency among them.

To let autoencoders function under packet loss, we first change entropy encoding---instead of entropy coding the entire autoencoder-output tensor to a bitstream and then packetizing it to packets




\name chooses autoencoders, because the elements in an autoencoder-output tensor have much less dependency among them.
If we randomly select some elements of an autoencoder-returned code (\ie random erasures) and set them to zero, which as explained in \S\ref{??} could mimic the effect of packet loss, the decoder can still decode the whole frame. 
In contrast, missing information in H.264 
% will not render the whole frame undecodable. 
%does not have dramatic impact on the decoded video quality.
This is in contrast to SVC where any data loss on a low layer also affects higher layers.
Moreover, the impact of random erasures on video quality increases with the rate of random erasures (\eg more zeroed elements). 
In other words, unlike FEC needs to known \rate~{\em a priori}, the quality of autoencoders {\em could} degrade gracefully with more data loss.


We use autoencoders because they have two {\em potential} advantages.
First, there is little explicit dependency among the elements of an autoencoder-returned tensor. 
Thus, unlike in SVC where any data loss on a lower layer also affects higher layers, applying any random erasures (such as zeroing randomly selected elements) on an output tensor of an autoencoder will not have a dramatic impact on the decoded video quality.
%In other words, so the values in the tensor do not need to be received in specific order, like in SVC. 
Second, the impact of random perturbation on video quality {\em could} be further reduced by training the autoencoder to work under different random erasure rates. 
The resulting autoencoders might be better than FEC which only tolerates a pre-determined data loss rate.
%one autoencoder (a pair of NN encoder and NN decoder) could be trained to work under a {\em range} of data erasure rates and still achieve decent quality.


Yet, traditional autoencoders are ill-suited for real-time videos. 
Here, we highlight how \name addresses two specific challenges to enable autoencoder-based DS video delivery.



First, traditional autoencoder-returned code could be decoded in presence of data loss, but its quality will degrade quickly with more random erasures.
This is because in standard autoencoder training, the encoder output is almost\footnote{Encoder output is sometimes quantized (lower float precision), but quantization's effect on video quality is much less than data erasures caused by packet loss.} always identical to the decoder input. 
%have never seen any data erasure during the training. 
%To improve quality under data erasures, 
\name uses a different autoencoder training process---it injecting random data erasures of various rates (from 0\% to 90\%) between the encoder and the decoder, which simulates the effects of different \rates.
In other words, the new autoencoders not only learn how to compress frames efficiently but also how to code them in a way resilient to different \rates (see \S\ref{??} for details). 

Second, existing autoencoders and standard video codecs use arithmetic coding to compress all information of a frame to a single bitstream which will then be packetized. 
This means that any packet loss will render the data undecodable.
%If this bitstream is packetized, as done in conventional real-time video systems, any packet loss will render the data undecodable.
Instead, \name first randomly partitions the autoencoder-returned code to sub-tensors and then arithmetically codes each sub-tensor as a separate packet.
Though it sounds easy, per-packet arithmetic coding turns out to be challenging, since traditional arithmetic coding incurs excessive size overhead per packet due to the need to store each packet's data distribution. 
\name addresses it using a novel scheme to balance the size overhead and efficiency of per-packet arithmetic coding (see \S\ref{??}). 

\end{comment}

%As an end-to-end video coding framework, 
%\name also tackles other practical challenges, such as efficient bitrate control, speeding up of autoencoders, and balancing the size of I-frames and P-frames.


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/fig1-example.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/fig1-example-osdi.pdf}
        \includegraphics[width=0.99\linewidth]{figs/fig1example.pdf}
         \label{fig:}
         \tightcaption{Example results of \name's (a) more graceful degradation in presence of packet loss than prior solutions, and (b) better tradeoffs between video quality and tail frame delay, which corroborates the subjective rating of users.
         More results can be found in \S\ref{sec:eval}. 
%         \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
    \jc{TODO: add a horizontal line to indicate the quality of H.265}
    \textcolor{red}{Yihua: TODO: update real values (fig1data.xlsx)}
         }
%    \tightcaption{Video quality vs. \rates of different video codecs when the actual encoded bitrate is 3.6 Mbps (which includes FEC redundancy if used.)
%    Quality of \name's autoencoder degrades gracefully with higher \rates. 
%%    achieves a smoother quality degradation as packet loss rate increases.
%    More results can be found in \S\ref{sec:eval}. 
%%    \jc{Yihua, can you replot the FEC lines to use the same color (w/ diff point/line types)}
%%    \jc{Yihua, can you add (DSC) next to our solution?}
%%    \jc{Yihua, can we also replace yellow with 50\% redundancy?}
%    %\jc{YIHUA, remember to add a line of 264 without loss, and remove the part of h264 when it's undecodable}\jc{set R-D optimization to "intra-MB insertion"}
%%    \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
%%    \jc{Yihua, can you add a horizontal line to indicate the quality of H.265}
%    }
    \label{fig:intro-example}
    % \vspace{-0.5cm}
\end{figure}

Besides achieving loss resilience on a single frame, \name uses a novel frame delivery system to approximate DS coding over a sequence of frames, speed up autoencoder coding (on GPUs and CPUs), and enable efficient bitrate control (\S\ref{??}).

%including a custom streaming protocol
%controlling bitrate, and speeding up autoencoder coding. 


It is important to note what \name does {\em not} cover.
\name does not address problems in multi-party conferencing (\eg stream forwarding); instead, it focuses on unicast video communication.
While \name decides {\em what} each packet contains, it re-uses existing logics, such as GCC~\cite{??}, to determine the target bitrate of a frame and {\em how fast} to send its packets.
%, so that even if the selected bitrate overshoots the bandwidth, we can still obtain decent quality.


%Being a coding system, \name can work with existing congestion control (CC) logics---CC decides how fast to send packets, and \name decides {\em what} each packet contains.


To put it in context, autoencoders have long been used in multimedia and data communication (see \S\ref{sec:related}) but \name is, to our best knowledge, the first to demonstrates that potential of autoencoders to remarkably improve loss resilience in real-time video.
Swift and DeepFGS, for instance, use autoencoders to improve scalable video coding (rather than loss tolerance) for on-demand (rather than real-time) videos~\cite{swift,??}. 
\name also differs to DeepJSCC which uses autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss)~\cite{??,??}.



\begin{comment}

To put it in context, \name is, to our best knowledge, the first to demonstrates that potential of autoencoders to remarkably improve loss resilience in real-time video.
Autoencoders have long been used in multimedia and data communication (see \S\ref{sec:related}) but mostly for more efficient compression.
Swift and DeepFGS, for instance, use autoencoders to improve scalable video coding for on-demand videos~\cite{swift,??}, rather than loss tolerance of real-time videos. 
\name also differs to DeepJSCC~\cite{??,??} which uses autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss).
%for compressing images and signals in wireless communication and 


To put \name in perspective, autoencoders have long been used in data communication~\cite{erpek2020deep} (see \S\ref{sec:related}).
\name, which can be seen as joint-source-channel coder, is similar 
%As a joint-source-channel coder, \name's autoencoder is similar 
in spirit to DeepJSCC which uses autoencoder to compress static images (rather than real-time videos) in a way robust to wireless signal noises~\cite{??} (rather than packet loss).
%for compressing images and signals in wireless communication and 
Recently, Swift uses autoencoders to improve scalable video coding (SVC) for on-demand videos~\cite{swift}. 
To our best knowledge, \name is the first video framework to demonstrates the potential of autoencoders to improve loss resilience in real-time communication.
\end{comment}

%Much remains unknown about the limits of autoencoders as a loss-resilient coding layer.

%To our best knowledge, \name is the first end-to-end autoencoder-based video system for loss-resilient real-time videos.
%that achieves stream real-time videos in a data-scalable fashion. 



%arising from training and using autoencoders in real-time video communication.

%Many aspects of \name are also inspired by prior work. 
%That said, \name, to our best knowledge, is the first to develop custom autoencoders that realize data-scalable video delivery.

%\name aims at unicast video sessions, rather than multi-party conferences. 
%It is also important that \name's autoencoders do {\em not} achieve better compression efficiency than recent heavily engineered video codecs, such as H.265. 
%Indeed, \name's video quality is still slightly lower than H.265 at the same bitrate. 

We have implemented \name and evaluated it under various network traces and video content. 
There are two key findings (an example of which is given in Figure~\ref{fig:intro-example}). 
First, when no packets are lost, \name's quality does not exceed H.265 at the same bitrate, but in presence of more packet loss, \name's quality degrades much more gracefully than other loss-resilient video coding.
Second, we use packet-level simulation driven by real-world bandwidth traces, and runs \name and the baseline loss-resilient coding schemes on the same congestion control logic.
We show that compared to the baselines, \name reduces the 95th-percentile frame delay (defined as the delay between encoding and decoding of a frame) by up-to \fillme$\times$ and the stall rate (defined as the fraction of inter-frame gaps that exceed \fillme~ms) by \fillme$\times$. 
%compared to the most competitive baselines which still have to retransmit packets or skip frames.
With much less video stuttering and fewer skipped frames, our user study confirms that \name has higher average subjective ratings by users than the baselines.

%First, on various video content, \name's quality degrades more gracefully under packet loss than other loss-resilient coding.
%That said, in absence of packet loss, \name's quality is slightly lower than H.265 at the same bitrate. \jc{need to update this}




%, without much compromise on quality in absence of packet loss. 
% which is comparable or less than adding 10\% FEC redundancy. 
%does {\em not} outperform the latest heavily engineered video codecs in quality---indeed, \name's video quality is slightly lower than H.265 at the same bitrate. 


\begin{comment}
Using real-world and synthetic network traces and a wide range of videos, we show that \name's autoencoder has a more graceful quality degradation under packet loss than baseline loss-resilient video codecs.
%, without sacrificing video quality in absence of packet loss 
(Figure~\ref{fig:intro-example} gives an example).
When comparing \name with the baselines with the same CC logic (\eg GCC~\cite{??} and Salsify-CC~\cite{??}), \name significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to prior work which has to retransmit packets or skip frames, with the comparable video quality.
To put it in perspective, \name significantly decrease the frames that arrive after user-perceivable delay (\eg 200ms for video calls) and reduces video stuttering.
\end{comment}

%Our results show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile when prior work has to retransmit packets or skip frame), with the marginally lowered video quality.
%To put it in perspective, \name can significantly reduce the chance that frames arrive after user-perceivable delay (\eg 200ms for video conferencing) and improve playback smoothness (higher frame rate).

%\jc{ae has caveats (size, speed, efficiency). }
%\jc{this paper above all shows a new design space}

\textbf{This work does not raise any ethical issues.}






%unlike SVC, the output tensor of an autoencoder does {\em not} impose a hierarchical structure among its elements, so the values in the tensor do not need to be received in specific order, like in SVC. 
%Instead, randomly perturbing a tensor in the new embedding space, such as zeroing any $\alpha\%$ of a tensor's elements, will have only a {\em limited} impact (proportional to $\alpha\%$)  on the quality of the decoded frame.
%Second, unlike FEC which only tolerates a pre-determined data loss rate, one autoencoder (a pair of NN encoder and NN decoder) could be trained to achieve desirable quality under a {\em range} of data erasure rates. 

%To be specific, each frame is supposed to be decoded at a fixed interval after the last frame was decoded, and 
%
%a packet associated with a frame will delay the rendering of a 
%To be more specific, we call a packet as a {\em missing packet}, if it arrives after when the frame it belongs to should be decoded (\eg 40ms after the last frame is decoded under 25fps), and we refer to the fraction of data in missing packets of a frame as {\em data missing rate} or \rate. 
%Note that a missed packet can be lost or delayed.






==> sections/old/intro_v12.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}

Real-time video communication has a long history in research, yet only recently has it become truly widespread in our daily lives~\cite{blum2021webrtc}---from online meetings~\cite{webrtc-vc-1,webrtc-vc-2}, cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2}, to interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2} and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
The amount of time people spend on real-time videos grow faster than the time spent on watching streaming videos~\cite{webrtc-trend-1,webrtc-trend-2}.
Yet, users are more susceptible to video stuttering and poor quality when using real-time video applications (\eg video calls and online gaming) than when watching on-demand videos (\eg Netflix). 
% Despite intensive research on congestion control and bitrate adaptation~\cite{salsify,sprout} for Internet videos, 
Despite many prior efforts, packet jitters and loss still remain, especially in wide-area networks that have substantial latency and bandwidth fluctuation.
% , such as long-distance video calls. 
To make it more challenging, real-time video clients use a very short buffer (\eg merely 10 ms in WebRTC~\cite{10.1145/3410449}) to render each frame as soon as they are received. 
Consequently, waiting/retransmitting a single packet, which could take 100s ms or longer, will block multiple frames and cause a visual stuttering.

% These packet retransmits may not be concealed by the short buffer---merely 10 ms in WebRTC~\cite{10.1145/3410449}, which allows frames to be played as soon as they are decoded.
% As a result, the extra delay to wait or resend a single packet frame, which could take 100s ms or longer in long-latency links, can block the decoding of multiple frames and cause a visual stuttering. 


\begin{comment}
might be conceal by the playback buffer in on-demand streaming videos, 
%In on-demand video streaming, the extra delay of packet retransmits (which could be 100s ms or higher in long-latency links) is easy to conceal by the video buffer, but 
this may not be true for 
real-time videos use a very short buffer (\eg merely \fillme ms in WebRTC)~\cite{??}  in order to play each frame as soon as it is decoded.
As a result, the additional delay to wait or resend a single packet frame might block the decoding of multiple frames and cause a visual stuttering. 
\end{comment}


Thus, loss-resilient video coding is crucial real-time videos.
% for high-quality, smooth real-time videos.
An ideal loss-resilient scheme should achieve high {\em compression efficiency}, which means high quality with fewer bits, and {\em loss resilience} under various data missing rate or {\em \rate} defined by
the fraction of data that is not received, due to packet drops or queuing, before a frame is decoded.

Unfortunately, current real-time video systems achieve loss resilience by adding various forms of redundancies, thus sacrificing compression efficiency (as elaborated in \S\ref{subsec:prior}).\footnote{
Scalable video coding (SVC~\cite{SVCFEC1}, FGS~\cite{ma2022deepfgs,li2001overview}, Swift~\cite{swift}), which works well for on-demand streaming videos, will be much less effective in real-time videos which send packets of a frame together, instead of layer by layer (see \S\ref{subsec:prior}).
For this reason, scalable video coding is not commonly used to improve unicast real-time videos~\cite{salsify}. 
Similarly, selective frame skipping (\eg~\cite{voxel}) might work for on-demand videos, but in real-time videos, most frames are P-frames which cause poor quality once dropped, unless I-frames are frequently inserted.
Nonetheless, we will still evaluate them against \name.}
To handle 30\% \rate, for instance, forward error correction (FEC) must add (at least) 30\% redundancy {\em before} transmission~\cite{holmer2013handling, uberti2015webrtc}. 
For this reason, most systems only increase FEC redundancy after packet loss has already affected some frames~\cite{holmer2013handling}, which requires packets to be resent until enough packets are received.
%For these frames whose \rate is underestimated, 
%the receiver must still request the sender to resend some packets until at least 70\% of packets have arrived.
Even after the packet loss has subsided, FEC may still add too much redundancy, thereby reducing  video quality.  
Similarly, loss resilience could be achieved by using an older but reliably received frame as the reference frame, allowing the decoder to safely skip a loss-affected frame (\eg~\cite{salsify}).
%without hurting future frames, 
However, using an old reference frame means more bits to achieve the same quality as using the last frame as reference, which lowers compression efficiency.
%\jc{add old reference frame}



This paper presents \name, a new approach to loss-resilient real-time video, by customizing {\em  autoencoders}. 
%This paper presents \name, a new end-to-end loss-resilient real-time video streaming system, by customizing {\em  autoencoders} following the idea proposed in~\cite{cheng2022grace}. 
Autoencoders work like a standard video codec but replace part of the encoder and decoder with neural networks (NNs). 
Though autoencoders have a long history in multimedia, standard autoencoders have focused on better compression efficiency (achieving higher quality in fewer bits) and are not inherently loss-resilient.
This is because, in traditional autoencoder training, the decoder always receives the {\em same} \aecode produced by the encoder, which does not prepare the autoencoders to handle any data loss during transmission. 

In \name, we show that autoencoder-based video streaming can be loss-resilient by customizing the autoencoder training process (\S\ref{sec:core}) and video streaming framework (\S\ref{sec:delivery}).

In \name's autoencoder training process (\S\ref{subsec:training}), when the NN encoder returns a \aecode, we randomly mask n\% of its elements to zeros before feeding it to the NN decoder, a process we call {\em random masking}. We vary the rate of random masking ($n\%$) between [0\%, 100\%), which as explained shortly, simulates the effect of packet loss under different \rates.
% As explained shortly, varying the rate of random masking (n%n\%) between [0\%, 100\%) simulates the effect of packet loss under different \rates.
Consequently, our trained autoencoder, {\em without} knowing the actual \rate, can encode a frame such that it can: {\em (i)} decode a frame as long as {\em any} (non-empty) subset of packets of the frame is received;
%(\ie no need for retransmission unless all data is lost);  
{\em (ii)} achieve better quality with the addition of each new packet (\ie graceful degradation with higher \rate); and
{\em (iii)} reach a quality close to a non-loss-resilient coding algorithm (such as H.265) when all packets are received.
We refer to it as {\em Data-Scalable} ({\em DS}) video coding.
In contrast, FEC is not DS coding, since its quality does not improve with more data if the \rate is below a threshold but the quality drops abruptly (due to retransmits) once the \rate exceeds the threshold.

% Our prior work of data-scalable (DS) autoencoders~\cite{cheng2022grace} suffers from multiple problems: {\em (i)} naive entropy encoding lowers compression efficiency, {\em (ii)} encoding speed insufficiently fast (<20fps) for real-time video streaming requirements, and {\em (iii)} additional quality degradation due to error propagation from packet losses.
% %To leverage the new data-scalable (DS) autoencoders, 
% To address the above challenges, \name uses a customized video streaming framework to deliver autoencoder-generated data.
% It uses a new packetization scheme with per-packet entropy encoding, which makes packet loss of $n\%$ \rate appear to have the same effect as $n\%$ random making on the \aecode (\S\ref{subsec:packetization}) with negligible size overhead. 
% \name also uses techniques for DS coding over a sequence of frames to minimize the propagation of error, as well as optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).
To leverage the new data-scalable (DS) autoencoders, \name uses a customized video streaming framework to deliver autoencoder-generated data.
It uses a new packetization scheme on randomly shuffled \aecode with per-packet entropy encoding, which makes packet loss of $n\%$ \rate appear to have the same effect as $n\%$ random making on the \aecode (\S\ref{subsec:packetization}). 
\name also uses techniques for DS coding over a sequence of frames, as well as optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).


\begin{comment}

It uses a novel packetization scheme that makes packet loss of n%n\% appear to have the same effect as n%n\% random making on the \aecode (see \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{subsec:packetization} for details). 
%Standard autoencoders entropy encode the NN encoder output (\aecode) and packetize the resulting bitstream, so any packet loss will render it undecodable by the receiver.
The basic idea is to randomly split the \aecode's elements to partitions, each separately entropy-encoded as an independently decodable packet, and if n%n\% packets are lost, we set their elements in the \aecode to zeros, which mimics random masking.
However, this naive scheme greatly increases the size of the compressed data, due to the additional space needed to store the symbol distribution (used by entropy-decoding) in each packet.
\name addresses this challenge by carefully coarsening the granularity of symbol distributions, which significantly reduces size increase while maintaining the compression efficiency of entropy coding. 

\end{comment}





\begin{comment}

Ideally, the quality should degrade gracefully with more packet loss (higher \rate), without compromising the quality in absence of packet loss.
Specifically, it should be able to 
{\em (i)} decode a frame as long as {\em any} (non-empty) subset of packets of the frame is received;
%(\ie no need for retransmission unless all data is lost);  
{\em (ii)} achieve better quality with the addition of each new packet (\ie lower \rate); and
{\em (iii)}  reach a quality close to a non-loss-resilient coding algorithm (such as H.265), when all packets are received.
We refer to it as {\em Data-Scalable} ({\em DS}) video coding.
FEC is not DS coding, since its quality does not improve with more data if the packet loss rate is below a threshold but the quality drops abruptly once loss rate exceeds the threshold.


\mypara{Data-scalable autoencoder}
This paper introduces {\em \name}, a real-time video system that, for the first time, uses {\em  autoencoders (AEs)} to realize data-scalable (DS) video delivery.
%which explores a new approach to DS video delivery by using {\em neural-net (NN) autoencoders}.
At a high level, autoencoders work like a standard video codec but replace some coding logic with neural networks (NNs). 
It uses an NN encoder to encode a frame to a {\em \aecode} (without entropy encoding), and an NN decoder to decode to a reconstructed frame that is similar to the original frame. 


We choose autoencoders, not because the off-the-shelf models are inherently data-scalable (DS), but due to their unique properties that {\em could} enable DS coding. 
%\name is a particular design that harnesses these properties to enable DS coding.
Specifically, the NN decoder can reconstruct a decent-quality frame, even if we {\em randomly erase} (\ie set to zeroes) a subset of $n\%$ elements in the \aecode (the output of the NN encoder).
In other words, {\em random data erasure} on the \aecode has a limited impact on the decoding quality of autoencoders. 
This can be attributed to the lack of stringent dependencies among the elements in a \aecode\footnote{
%Mathematically, this smoothness is a result of NN encoders and decoders having continuous derivatives everywhere. Moreover, 
This can also be intuitively understood that NN decoders share the architecture of {\em generative} NNs, such as variational autoencoder (VAE), which can create realistic-looking images from random inputs.}, unlike SVC where the decoding of a layer depends on the lower layers.


Despite the promise of autoencoders, several practical challenges remain.
%\name addresses several practical challenges.
Two of them will be highlighted here.

%Despite the promise of autoencoders, \name must address several practical challenges, such as improving quality under various \rates, making entropy encoding of \aecodes loss-resilient, controlling bitrate, and speeding up autoencoder coding. 
%Two of them will be highlighted here.


%\mypara{Adding packet loss in autoencoder training}
\mypara{Training autoencoder with packet loss}
First, the quality of standard autoencoders drops quite significantly if more data is erased from the \aecode. 
This is because the standard autoencoder training, in which  the decoder always sees the same \aecode returned by the encoder, never prepares the autoencoder to handle any data loss between the encoder and the decoder. 
\name trains autoencoders different (see \S\ref{??} for details).
It applies random data erasures to the \aecode (which could simulate the effect of packet loss as explained shortly), and by varying the rate of data erasure between [0\%, 100\%), 
%In other words, by training the NN encoder and NN decoder jointly, 
the new autoencoders not only learn how to compress high-quality frames efficiently but also to be robust to different rates of random data erasures. 

%, which simulates the effects of packet loss under different \rates (which will be explained shortly).






\mypara{Per-packet entropy coding for autoencoder}
Standard autoencoders use entropy encoding to losslessly compress a \aecode to a single bitstream and then packetize it, so any packet loss will render it undecodable.
%entropy coding used in current autoencoders cannot tolerate any packet loss. 
A naive idea is to randomly 
split the \aecode's elements to partitions,
%split a \aecode to sub-tensors, 
each separately entropy-encoded as an independently decodable packet, and if $n\%$ packets are lost, we set their elements in the \aecode to zeros, which resembles random erasure.
%effectively erases a random subset of $n\%$ elements.
%is the same as 
%random data erasure.
However, this naive per-packet entropy coding greatly increases the size of the compressed data, due to the additional space needed to store the symbol distribution (used by entropy-decoding) in each packet.
%To mitigate the size increase, 
\name carefully coarsens the granularity of symbol distributions, which significantly reduces size increase while maintaining the compression efficiency of entropy coding (see \S\ref{??} for details). 




Besides achieving loss resilience on a single frame, \name uses a novel frame delivery system to approximate DS coding over a sequence of frames, speed up autoencoder coding (on GPUs and CPUs), and enable efficient bitrate control (\S\ref{??}).




\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/fig1-example.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/fig1-example-osdi.pdf}
        \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/fig1.png}
         \caption{graceful degradation}
         \label{fig:normal-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
         \caption{delay quality tradeoff}
         \label{fig:normal-ssim-delay}
     \end{subfigure}
         \label{fig:}
         \tightcaption{Example results of \name's (a) more graceful degradation in presence of packet loss than prior solutions, and (b) better tradeoffs between video quality and tail frame delay, which corroborates the subjective rating of users.
         More results can be found in \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{sec:eval}. 
%         \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
    \jc{TODO: add a horizontal line to indicate the quality of H.265}
    \textcolor{red}{Yihua: TODO: update real values (fig1data.xlsx)}
         }
    \label{fig:intro-example}
\end{figure}

\end{comment}





\begin{figure}[t!]
    \centering
        \includegraphics[width=0.99\linewidth]{figs/intro-example-illustrative-old.pdf}
         \tightcaption{(a) An example of \name's loss resilience under packet loss of different \rates, and (b) the potential quality/delay improvement by \name. These figures are illustrative; actual figures from our evaluation and trace analysis appear
later (e.g., Figures~\ref{fig:normal-simulation}, \ref{fig:queue15-simulation}, \ref{fig:loss_by_bitrate}). }
    \label{fig:intro-example}
    % \vspace{-0.5cm}
\end{figure}

%including a custom streaming protocol
%controlling bitrate, and speeding up autoencoder coding. 


We should also clarify what \name does {\em not} cover.
First, \name does not address problems unique to multi-party conferencing (\eg stream forwarding); instead, we focus on unicast video communication.
%While \name decides {\em what} each packet contains, 
Second, \name runs on existing congestion control (CC) logics ({\em without} packet retransmits unless all packets of a frame are lost), such as GCC~\cite{carlucci2016analysis}, which decides the target frame size and how fast to send the \name-encoded packets.
Third, \name is not well-fit for resource-constraint devices, though our optimized implementation runs much faster than current autoencoders 
% and achieves lower delay than alternative solutions 
(\S\ref{subsec:fast-coding}).
%, so that even if the selected bitrate overshoots the bandwidth, we can still obtain decent quality.


%Being a coding system, \name can work with existing congestion control (CC) logics---CC decides how fast to send packets, and \name decides {\em what} each packet contains.


To put it in context, autoencoders have long been used in multimedia (see \S\ref{sec:related}) but \name is, to our best knowledge, the first to demonstrate the potential of autoencoders to improve loss resilience in real-time video.
Swift and DeepFGS, for instance, use autoencoders to improve scalable video coding (rather than loss tolerance) for on-demand (rather than real-time) videos~\cite{swift, ma2022deepfgs}. 
DeepJSCC uses an autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss)~\cite{kurka2020deepjscc}.
\name also differs from neural error concealment~\cite{sankisa2018video} which only uses NNs on the receiver, whereas \name jointly trains the encoder and decoder to handle packet loss.



%Much remains unknown about the limits of autoencoders as a loss-resilient coding layer.

%To our best knowledge, \name is the first end-to-end autoencoder-based video system for loss-resilient real-time videos.
%that achieves stream real-time videos in a data-scalable fashion. 



%arising from training and using autoencoders in real-time video communication.

%Many aspects of \name are also inspired by prior work. 
%That said, \name, to our best knowledge, is the first to develop custom autoencoders that realize data-scalable video delivery.

%\name aims at unicast video sessions, rather than multi-party conferences. 
%It is also important that \name's autoencoders do {\em not} achieve better compression efficiency than recent heavily engineered video codecs, such as H.265. 
%Indeed, \name's video quality is still slightly lower than H.265 at the same bitrate. 

We have implemented \name and evaluated it under various network traces and video content. 
There are two key findings (an example of which is given in Figure~\ref{fig:intro-example}). 
First, when no packets are lost, \name's quality does not exceed H.265 at the same bitrate, but in presence of more packet loss, \name's quality degrades much more gracefully than other loss-resilient coding schemes.
Second, we use packet-level simulation driven by real-world bandwidth traces and run \name and the baseline loss-resilient coding schemes. % on the same CC logic (retransmits disabled).
We show that compared to the baselines, \name reduces the ratio of delayed frames (defined as the frames whose delay between encoding and decoding is larger than 400~ms) by up-to 4$\times$ and the stall rate (defined as the fraction of inter-frame gaps that exceed 200~ms) by 10$\times$. 
%compared to the most competitive baselines which still have to retransmit packets or skip frames.
With much less video stuttering and fewer skipped frames, our user study confirms that \name has higher average subjective ratings by users than the baselines.

\textbf{This work does not raise any ethical issues.}








==> sections/old/intro_v13.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}

Real-time video communication has a long history in research, yet only recently has it become truly widespread in our daily lives~\cite{blum2021webrtc}---from online meetings~\cite{webrtc-vc-1,webrtc-vc-2}, cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2}, to interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2} and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
In the meantime, RTC (and WebRTC clients) has become the de-facto platform for real-time videos, just like HTTP and DASH in streaming videos, enabling more and more new applications~\cite{webrtc-trend-1,webrtc-trend-2}. 
%The amount of time people spend on real-time videos grow faster than the time spent on watching streaming videos~\cite{webrtc-trend-1,webrtc-trend-2}.


Compared to streaming videos (over HTTP), such as video-on-demand, users are at least as susceptible to video stuttering and poor quality when using real-time video applications (\eg video conferencing and online gaming). 
However, real-time video clients use a very short buffer in order to render each frame as soon as they are received.
For instance, the buffer in WebRTC is merely 10s of ms~\cite{10.1145/3410449}; in contrast, HTTP-based streaming videos, even live sports event, have a buffer of at least 10 seconds. 
To make it worse, long latencies and bandwidth fluctuations remain across wide-area networks and cellular networks, causing occasional packet loss and latency jitter. 
Waiting/retransmitting a single packet can take 100s ms or longer and block multiple frames, causing video stuttering.
Thus, loss-resilient video coding is crucial real-time videos.

%Yet, users are at least as susceptible to video stuttering and poor quality when using real-time video applications (\eg video calls and online gaming) as when watching on-demand videos (\eg Netflix). 
%% Despite intensive research on congestion control and bitrate adaptation~\cite{salsify,sprout} for Internet videos, 
%Long latencies and bandwidth fluctuations remain across wide-area networks and cellular networks.
%% , such as long-distance video calls. 
%To make it more challenging, real-time video clients use a very short buffer (\eg merely 10 ms in WebRTC~\cite{10.1145/3410449}) to render each frame as soon as they are received. 
%Consequently, waiting/retransmitting a single packet, which could take 100s ms or longer, will block multiple frames and cause a visual stuttering.

% These packet retransmits may not be concealed by the short buffer---merely 10 ms in WebRTC~\cite{10.1145/3410449}, which allows frames to be played as soon as they are decoded.
% As a result, the extra delay to wait or resend a single packet frame, which could take 100s ms or longer in long-latency links, can block the decoding of multiple frames and cause a visual stuttering. 


\begin{comment}
might be conceal by the playback buffer in on-demand streaming videos, 
%In on-demand video streaming, the extra delay of packet retransmits (which could be 100s ms or higher in long-latency links) is easy to conceal by the video buffer, but 
this may not be true for 
real-time videos use a very short buffer (\eg merely \fillme ms in WebRTC)~\cite{??}  in order to play each frame as soon as it is decoded.
As a result, the additional delay to wait or resend a single packet frame might block the decoding of multiple frames and cause a visual stuttering. 
\end{comment}


%\begin{figure}[t!]
%    \centering
%        \includegraphics[width=0.99\linewidth]{figs/intro-example-illustrative-old.pdf}
%         \tightcaption{(a) An example of \name's loss resilience under packet loss of different \rates, and (b) the potential quality/delay improvement by \name. These figures are illustrative; actual figures from our evaluation and trace analysis appear
%later (e.g., Figures~\ref{fig:normal-simulation}, \ref{fig:queue15-simulation}, \ref{fig:loss_by_bitrate}). }
%    \label{fig:intro-example}
%    % \vspace{-0.5cm}
%\end{figure}

% for high-quality, smooth real-time videos.
\mypara{Data-scalable (DS) coding}
We define the {\em Data Missing Rate} (\rate) of a frame as the fraction of packets not received before the  receiver decodes the frame\footnote{\rate is similar to packet loss rate defined on a single frame.}, \eg every 50ms at 20 frames per second (fps).
A packet can be missing due to packet drops, queuing delay or out-of-order delivery, and the missing packets can be consecutive or random.
{\em Without} knowing the actual \rate, an ideal loss-resilient coding scheme should encode a frame  such that
%Then {\em without} knowing the actual \rate, an ideal loss-resilient scheme should meet three criteria: 
\begin{packeditemize}
\item {\em (i)} the frame is decodable under any \rate below 100\% (\ie at least one packet is received), 
\item {\em (ii)} the quality is close to a non-loss-resilient codec (\eg H.265) when all packets are received, and
%as long as {\em any} (non-empty) subset of packets of the frame is received, 
%(\ie no need for retransmission unless all data is lost);  
\item {\em (iii)} quality degrades gracefully with higher \rate, \ie quality gradually improves if {\em any} more packets are received.
\end{packeditemize}
We call such a coding scheme {\em data-scalable} (DS).
DS coding is ideal for real-time video, because without retransmission, its quality degrades gracefully with more packet loss (higher \rate) while not sacrificing quality in absence of packet loss. 

Unfortunately, despite of many loss-resilience schemes, they are fundamentally ill-suited for DS coding by design.
% fall short at realizing DS coding. 
Firstly, Tambur, a state-of-the-art scheme based on forward error correction (FEC), tolerates $x$\% \rate by adding at least $x$\% redundancy {\em before} transmission~\cite{holmer2013handling, uberti2015webrtc}, thus lowering the encoded video quality even if all packets turn out to be successfully received. 
Therefore, most systems, such as WebRTC, do not add FEC redundancy by default, and increase FEC redundancy only {\em reactively}, after packet loss has affected some frames~\cite{holmer2013handling}.
%, which requires packets to be resent until enough packets are received.
%For these frames whose \rate is underestimated, 
%the receiver must still request the sender to resend some packets until at least 70\% of packets have arrived.
%Even after the packet loss has subsided, FEC may still add too much redundancy, thereby reducing  video quality.  
Secondly, DS may seem similar to the concepts of scalable video coding (SVC)~\cite{SVCFEC1} and fine granularity scalability (FGS)~\cite{ma2022deepfgs,li2001overview}, both of which improve quality as more data are received. 
However, there is a key difference: quality in DS coding depends on how many packets are received {\em regardless} of which packets, but SVC and FGS split video into layers and their quality increases only if more layers are received in a specific hierarchy.
Thirdly, receiver-side error concealment may seem to be another candidate for DS, but in order to decode any subset of packets, it must either use FEC or split a frame into independently encoded partitions, which greatly increases the bitrate to achieve the same quality~\cite{KUMAR2006425}.
In \S\ref{subsec:prior}, we will discuss more schemes (such as functional decoder and super resolution).




\tempstrike{
Some loss-resilient scheme uses an older but reliably received frame as the reference frame, allowing the decoder to safely skip a loss-affected frame (\eg~\cite{salsify}).
%without hurting future frames, 
However, using an old reference frame means more bits to achieve the same quality as using the last frame as reference, which lowers compression efficiency.
}


%achieve high {\em compression efficiency}, which means high quality with fewer bits, and {\em loss resilience} under various data missing rate or {\em \rate} defined by
%the fraction of data that is not received, due to packet drops or queuing, before a frame is decoded.

\tempstrike{
Unfortunately, current real-time video systems achieve loss resilience by adding various forms of redundancies, thus sacrificing compression efficiency (as elaborated in \S\ref{subsec:prior}).\footnote{
Scalable video coding (SVC~\cite{SVCFEC1}, FGS~\cite{ma2022deepfgs,li2001overview}, Swift~\cite{swift}), which works well for on-demand streaming videos, will be much less effective in real-time videos which send packets of a frame together, instead of layer by layer (see \S\ref{subsec:prior}).
For this reason, scalable video coding is not commonly used to improve unicast real-time videos~\cite{salsify}. 
Similarly, selective frame skipping (\eg~\cite{voxel}) might work for on-demand videos, but in real-time videos, most frames are P-frames which cause poor quality once dropped, unless I-frames are frequently inserted.
Nonetheless, we will still evaluate them against \name.}
%\jc{add old reference frame}
}

This paper presents \name, a new loss-resilient scheme for real-time video, which approximates DS coding.
The key idea is two-fold.
\begin{packedenumerate} 
\item \name uses {\em a loss-resilient autoencoder} (\S\ref{subsec:training}), a pair of {\em jointly trained} neural encoder and neural decoder, which optimizes video quality when $x$\% of values in the encoder output of a frame are randomly selected and masked (\ie set to zeros), with $x$\% between 0 to 100\%, before the masked data is fed to the decoder. 
This simulates the effect of random data masking between the encoder and the decoder.
\item \name uses a {\em novel packetization scheme} (\S\ref{subsec:packetization}) to partition the encoder output of a frame and entropy encodes each partition as an independently decodable packet, so that under any $x$\% packet loss (consecutive or not), the reconstructed input of the decoder is the encoder output except that $x$\% of randomly selected values are masked.
In short, packet loss will appear to have same effect as random data masking between the encoder and the decoder.
\end{packedenumerate} 
When put together, the two ideas help \name to optimize quality under various \rates (Figure~\ref{fig:intro-example}). 
As a result, \name better approximates DS coding than any prior solutions when tested under different \rates.
When no packets are lost, \name's quality does not exceed H.265 at the same bitrate, but in presence of higher \rates, \name's quality degrades much more gracefully than state-of-the-art loss-resilient coding schemes.


\begin{figure}[t!]
    \centering
        \includegraphics[width=0.9\linewidth]{figs/intro-example-illustrative-short.pdf}
         \tightcaption{An illustrative example of \name's data-scalable coding under packet loss of different \rates when compared with existing loss-resilient schemes. (actual figures from our evaluation appear
later (e.g., Figures~\ref{fig:loss_by_bitrate}). }
    \label{fig:intro-example}
    % \vspace{-0.5cm}
\end{figure}

To leverage the new data-scalable (DS) autoencoders, \name also includes a customized video streaming framework to delivery a sequence of frames to synchronize the encoder and decoder states in a slightly lazy fashion.
It also includes optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).
%to deliver autoencoder-generated data.
%It uses a new packetization scheme on randomly shuffled \aecode with per-packet entropy encoding, which makes packet loss of $n\%$ \rate appear to have the same effect as $n\%$ random making on the \aecode (\S\ref{subsec:packetization}). 
%\name also uses techniques for DS coding over a sequence of frames, as well as optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).




\name is not without limitations. 
First, we focus on unicast video communication, rather than problems in multi-party conferencing (\eg stream forwarding). 
%While \name decides {\em what} each packet contains, 
Second, though our optimized implementation of \name runs much faster than current autoencoders 
% and achieves lower delay than alternative solutions 
(\S\ref{subsec:fast-coding}), \name cannot run fast enough on resource-constraint devices yet. 


We have implemented \name and like other work in this space, we evaluate \name in a packet-level simulator driven by real network traces and a range of video content genres (all from different data sources from the training set) and compare it against a range of state-of-the-art loss resilient schemes, including {\em (i)} FEC (Tambur~\cite{rudow2023tambur}), {\em (ii)} error concealment (neural-net generative in-painting~\cite{xiang2019generative} and selective skipping~\cite{voxel}), {\em (iii)} Salsify's functional codec~\cite{salsify}, {\em (iv)} SVC~\cite{swift}, and {\em (v)} super resolution (SR)~\cite{??}.\footnote{\editSOCC{The main use case of SR is to enhance the decoded video quality at the receiver when the available bandwidth is low. Such technique should work for any kind of video codecs. Therefore, SR is orthogonal to \name.}} \jc{explain SR is orthogonal}
To be fair, we run \name and the baselines over the same congestion control (CC) algorithms, including GCC~\cite{carlucci2016analysis} and Salsify~\cite{salsify} (except that packet retransmission is turned off for loss-resilient decoders).
Our key results are: 
\begin{packeditemize}
\item \name achieves the similar average quality (in SSIM) with the codec used in WebRTC at the same bitrate. In other words, \name does not sacrifice quality in absence of packet loss.
\item \name achieves better quality, by \fillme-\fillme dB of SSIM, than other loss-resilient schemes at the same \rate and bitrate. 
\item When running on real network traces, \name  reduces the duration of video stalls, number of non-decodable frames, and 95th percentile frame delay by \fillme\%, \fillme\%, and \fillme\% respectively, when compared to the most competitive baselines. 
\item With much less video stuttering and fewer skipped frames, our user study confirms that \name has \fillme\% higher mean opinion score (MOS) than the most competitive loss-resilient schemes.
\item On a single \fillme GPU, \name can decode 720p and 1080p at \fillme~fps and \fillme~fps respectively, and encode 720p and 1080p at \fillme~fps and \fillme~fps respectively. This speed is on par with 
On CPUs, \name can encode \fillme{p} videos at \fillme~fps at only a drop of \fillme dB in SSIM.
\end{packeditemize}
%ratio of delayed frames (defined as the frames whose delay between encoding and decoding is larger than 400~ms) by up-to 4$\times$ and the stall rate (defined as the fraction of inter-frame gaps that exceed 200~ms) by 10$\times$. 
%compared to the most competitive baselines which still have to retransmit packets or skip frames.



To put \name's contribution in context, autoencoders have a long been used in multimedia (see \S\ref{sec:related}), but \name is, to our best knowledge, the first to demonstrate the potential of autoencoders to improve loss resilience in real-time video.
Existing autoencoders have focused on compression efficiency (achieving higher quality in fewer bits) assuming that there is no data loss between the encoder and the decoder.
Swift and DeepFGS, for instance, use autoencoders to improve scalable video coding (rather than loss tolerance) for on-demand (rather than real-time) videos~\cite{swift, ma2022deepfgs}. 
DeepJSCC uses an autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss)~\cite{kurka2020deepjscc}.
\name also differs from neural super-resolution models~\cite{neuroscaler} and neural error concealment~\cite{sankisa2018video} which only use NNs on the receiver, whereas \name jointly trains the encoder and decoder to handle packet loss.


%There are two key findings (an example of which is given in Figure~\ref{fig:intro-example}). 
%First, when no packets are lost, \name's quality does not exceed H.265 at the same bitrate, but in presence of more packet loss, \name's quality degrades much more gracefully than other loss-resilient coding schemes.
%Second, we use packet-level simulation driven by real-world bandwidth traces and run \name and the baseline loss-resilient coding schemes. % on the same CC logic (retransmits disabled).
%We show that compared to the baselines, \name reduces the ratio of delayed frames (defined as the frames whose delay between encoding and decoding is larger than 400~ms) by up-to 4$\times$ and the stall rate (defined as the fraction of inter-frame gaps that exceed 200~ms) by 10$\times$. 
%%compared to the most competitive baselines which still have to retransmit packets or skip frames.
%With much less video stuttering and fewer skipped frames, our user study confirms that \name has higher average subjective ratings by users than the baselines.
%
%Second, \name borrows existing congestion control (CC) logics {\em without} packet retransmits unless all packets of a frame are lost), such as GCC~\cite{carlucci2016analysis}, which decides the target frame size and how fast to send the \name-encoded packets.


%\textbf{This work does not raise any ethical issues.}



%Though autoencoders have a long history in multimedia, standard autoencoders have focused on better compression efficiency (achieving higher quality in fewer bits) and are not inherently loss-resilient.
%This is because, in traditional autoencoder training, the decoder always receives the {\em same} \aecode produced by the encoder, which does not prepare the autoencoders to handle any data loss during transmission. 
%
%To put it in context, neural encoders and decoders have long been used in multimedia (see \S\ref{sec:related}) but \name is, to our best knowledge, the first to demonstrate the potential of autoencoders to improve loss resilience in real-time video.
%Swift and DeepFGS, for instance, use autoencoders to improve scalable video coding (rather than loss tolerance) for on-demand (rather than real-time) videos~\cite{swift, ma2022deepfgs}. 
%DeepJSCC uses an autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss)~\cite{kurka2020deepjscc}.
%\name also differs from neural error concealment~\cite{sankisa2018video} which only uses NNs on the receiver, whereas \name jointly trains the encoder and decoder to handle packet loss.


\tempstrike{


Autoencoders work like a standard video codec but replace part of the encoder and decoder with neural networks (NNs). 
Though autoencoders have a long history in multimedia, standard autoencoders have focused on better compression efficiency (achieving higher quality in fewer bits) and are not inherently loss-resilient.
This is because, in traditional autoencoder training, the decoder always receives the {\em same} \aecode produced by the encoder, which does not prepare the autoencoders to handle any data loss during transmission. 



This paper presents \name, a new approach to loss-resilient real-time video, by customizing {\em  autoencoders}. 
%This paper presents \name, a new end-to-end loss-resilient real-time video streaming system, by customizing {\em  autoencoders} following the idea proposed in~\cite{cheng2022grace}. 

In \name, we show that autoencoder-based video streaming can be loss-resilient by customizing the autoencoder training process (\S\ref{sec:core}) and video streaming framework (\S\ref{sec:delivery}).

In \name's autoencoder training process (\S\ref{subsec:training}), when the NN encoder returns a \aecode, we randomly mask n\% of its elements to zeros before feeding it to the NN decoder, a process we call {\em random masking}. We vary the rate of random masking ($n\%$) between [0\%, 100\%), which as explained shortly, simulates the effect of packet loss under different \rates.
% As explained shortly, varying the rate of random masking (n%n\%) between [0\%, 100\%) simulates the effect of packet loss under different \rates.
Consequently, our trained autoencoder, {\em without} knowing the actual \rate, can encode a frame such that it can: {\em (i)} decode a frame as long as {\em any} (non-empty) subset of packets of the frame is received;
%(\ie no need for retransmission unless all data is lost);  
{\em (ii)} achieve better quality with the addition of each new packet (\ie graceful degradation with higher \rate); and
{\em (iii)} reach a quality close to a non-loss-resilient coding algorithm (such as H.265) when all packets are received.
We refer to it as {\em Data-Scalable} ({\em DS}) video coding.
In contrast, FEC is not DS coding, since its quality does not improve with more data if the \rate is below a threshold but the quality drops abruptly (due to retransmits) once the \rate exceeds the threshold.

}

% Our prior work of data-scalable (DS) autoencoders~\cite{cheng2022grace} suffers from multiple problems: {\em (i)} naive entropy encoding lowers compression efficiency, {\em (ii)} encoding speed insufficiently fast (<20fps) for real-time video streaming requirements, and {\em (iii)} additional quality degradation due to error propagation from packet losses.
% %To leverage the new data-scalable (DS) autoencoders, 
% To address the above challenges, \name uses a customized video streaming framework to deliver autoencoder-generated data.
% It uses a new packetization scheme with per-packet entropy encoding, which makes packet loss of $n\%$ \rate appear to have the same effect as $n\%$ random making on the \aecode (\S\ref{subsec:packetization}) with negligible size overhead. 
% \name also uses techniques for DS coding over a sequence of frames to minimize the propagation of error, as well as optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).


\begin{comment}

It uses a novel packetization scheme that makes packet loss of n%n\% appear to have the same effect as n%n\% random making on the \aecode (see \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{subsec:packetization} for details). 
%Standard autoencoders entropy encode the NN encoder output (\aecode) and packetize the resulting bitstream, so any packet loss will render it undecodable by the receiver.
The basic idea is to randomly split the \aecode's elements to partitions, each separately entropy-encoded as an independently decodable packet, and if n%n\% packets are lost, we set their elements in the \aecode to zeros, which mimics random masking.
However, this naive scheme greatly increases the size of the compressed data, due to the additional space needed to store the symbol distribution (used by entropy-decoding) in each packet.
\name addresses this challenge by carefully coarsening the granularity of symbol distributions, which significantly reduces size increase while maintaining the compression efficiency of entropy coding. 

\end{comment}





\begin{comment}

Ideally, the quality should degrade gracefully with more packet loss (higher \rate), without compromising the quality in absence of packet loss.
Specifically, it should be able to 
{\em (i)} decode a frame as long as {\em any} (non-empty) subset of packets of the frame is received;
%(\ie no need for retransmission unless all data is lost);  
{\em (ii)} achieve better quality with the addition of each new packet (\ie lower \rate); and
{\em (iii)}  reach a quality close to a non-loss-resilient coding algorithm (such as H.265), when all packets are received.
We refer to it as {\em Data-Scalable} ({\em DS}) video coding.
FEC is not DS coding, since its quality does not improve with more data if the packet loss rate is below a threshold but the quality drops abruptly once loss rate exceeds the threshold.


\mypara{Data-scalable autoencoder}
This paper introduces {\em \name}, a real-time video system that, for the first time, uses {\em  autoencoders (AEs)} to realize data-scalable (DS) video delivery.
%which explores a new approach to DS video delivery by using {\em neural-net (NN) autoencoders}.
At a high level, autoencoders work like a standard video codec but replace some coding logic with neural networks (NNs). 
It uses an NN encoder to encode a frame to a {\em \aecode} (without entropy encoding), and an NN decoder to decode to a reconstructed frame that is similar to the original frame. 


We choose autoencoders, not because the off-the-shelf models are inherently data-scalable (DS), but due to their unique properties that {\em could} enable DS coding. 
%\name is a particular design that harnesses these properties to enable DS coding.
Specifically, the NN decoder can reconstruct a decent-quality frame, even if we {\em randomly erase} (\ie set to zeroes) a subset of $n\%$ elements in the \aecode (the output of the NN encoder).
In other words, {\em random data erasure} on the \aecode has a limited impact on the decoding quality of autoencoders. 
This can be attributed to the lack of stringent dependencies among the elements in a \aecode\footnote{
%Mathematically, this smoothness is a result of NN encoders and decoders having continuous derivatives everywhere. Moreover, 
This can also be intuitively understood that NN decoders share the architecture of {\em generative} NNs, such as variational autoencoder (VAE), which can create realistic-looking images from random inputs.}, unlike SVC where the decoding of a layer depends on the lower layers.


Despite the promise of autoencoders, several practical challenges remain.
%\name addresses several practical challenges.
Two of them will be highlighted here.

%Despite the promise of autoencoders, \name must address several practical challenges, such as improving quality under various \rates, making entropy encoding of \aecodes loss-resilient, controlling bitrate, and speeding up autoencoder coding. 
%Two of them will be highlighted here.


%\mypara{Adding packet loss in autoencoder training}
\mypara{Training autoencoder with packet loss}
First, the quality of standard autoencoders drops quite significantly if more data is erased from the \aecode. 
This is because the standard autoencoder training, in which  the decoder always sees the same \aecode returned by the encoder, never prepares the autoencoder to handle any data loss between the encoder and the decoder. 
\name trains autoencoders different (see \S\ref{??} for details).
It applies random data erasures to the \aecode (which could simulate the effect of packet loss as explained shortly), and by varying the rate of data erasure between [0\%, 100\%), 
%In other words, by training the NN encoder and NN decoder jointly, 
the new autoencoders not only learn how to compress high-quality frames efficiently but also to be robust to different rates of random data erasures. 

%, which simulates the effects of packet loss under different \rates (which will be explained shortly).






\mypara{Per-packet entropy coding for autoencoder}
Standard autoencoders use entropy encoding to losslessly compress a \aecode to a single bitstream and then packetize it, so any packet loss will render it undecodable.
%entropy coding used in current autoencoders cannot tolerate any packet loss. 
A naive idea is to randomly 
split the \aecode's elements to partitions,
%split a \aecode to sub-tensors, 
each separately entropy-encoded as an independently decodable packet, and if $n\%$ packets are lost, we set their elements in the \aecode to zeros, which resembles random erasure.
%effectively erases a random subset of $n\%$ elements.
%is the same as 
%random data erasure.
However, this naive per-packet entropy coding greatly increases the size of the compressed data, due to the additional space needed to store the symbol distribution (used by entropy-decoding) in each packet.
%To mitigate the size increase, 
\name carefully coarsens the granularity of symbol distributions, which significantly reduces size increase while maintaining the compression efficiency of entropy coding (see \S\ref{??} for details). 




Besides achieving loss resilience on a single frame, \name uses a novel frame delivery system to approximate DS coding over a sequence of frames, speed up autoencoder coding (on GPUs and CPUs), and enable efficient bitrate control (\S\ref{??}).




\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/fig1-example.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/fig1-example-osdi.pdf}
        \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/fig1.png}
         \caption{graceful degradation}
         \label{fig:normal-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
         \caption{delay quality tradeoff}
         \label{fig:normal-ssim-delay}
     \end{subfigure}
         \label{fig:}
         \tightcaption{Example results of \name's (a) more graceful degradation in presence of packet loss than prior solutions, and (b) better tradeoffs between video quality and tail frame delay, which corroborates the subjective rating of users.
         More results can be found in \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{sec:eval}. 
%         \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
    \jc{TODO: add a horizontal line to indicate the quality of H.265}
    \textcolor{red}{Yihua: TODO: update real values (fig1data.xlsx)}
         }
    \label{fig:intro-example}
\end{figure}

\end{comment}






%including a custom streaming protocol
%controlling bitrate, and speeding up autoencoder coding. 


%, so that even if the selected bitrate overshoots the bandwidth, we can still obtain decent quality.


%Being a coding system, \name can work with existing congestion control (CC) logics---CC decides how fast to send packets, and \name decides {\em what} each packet contains.




%Much remains unknown about the limits of autoencoders as a loss-resilient coding layer.

%To our best knowledge, \name is the first end-to-end autoencoder-based video system for loss-resilient real-time videos.
%that achieves stream real-time videos in a data-scalable fashion. 



%arising from training and using autoencoders in real-time video communication.

%Many aspects of \name are also inspired by prior work. 
%That said, \name, to our best knowledge, is the first to develop custom autoencoders that realize data-scalable video delivery.

%\name aims at unicast video sessions, rather than multi-party conferences. 
%It is also important that \name's autoencoders do {\em not} achieve better compression efficiency than recent heavily engineered video codecs, such as H.265. 
%Indeed, \name's video quality is still slightly lower than H.265 at the same bitrate. 








==> sections/old/intro_v14.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}

Real-time video communication has a long history in research, yet only recently has it become truly widespread in our daily lives~\cite{blum2021webrtc}.
RTC (and WebRTC clients) has become the de-facto platform for real-time videos, just like HTTP and DASH in streaming videos, enabling more and more new applications~\cite{webrtc-trend-1,webrtc-trend-2}, from online meetings~\cite{webrtc-vc-1,webrtc-vc-2}, cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2}, to interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2} and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
%The amount of time people spend on real-time videos grow faster than the time spent on watching streaming videos~\cite{webrtc-trend-1,webrtc-trend-2}.





%Compared to streaming videos (over HTTP), such as video-on-demand, users are at least as susceptible to video stuttering and poor quality when using real-time video applications (\eg video conferencing and online gaming). 
%However, real-time video clients use a very short buffer in order to render each frame as soon as they are received.
%For instance, the buffer in WebRTC is merely 10s of ms~\cite{10.1145/3410449}; in contrast, HTTP-based streaming videos, even live sports event, have a buffer of at least 10 seconds. 
%To make it worse, long latencies and bandwidth fluctuations remain across wide-area networks and cellular networks, causing occasional packet loss and latency jitter. 
%Waiting/retransmitting a single packet can take 100s ms or longer and block multiple frames, causing video stuttering.
%Thus, loss-resilient video coding, which can tolerate any packet loss rate\footnote{To avoid ambiguity, we define {\em the packet loss rate on a frame} as the fraction of its packets not received before the receiver decodes the frame, \eg every 50ms at 20 frames per second (fps).
%A packet can be lost due to packet drops, queuing delay or out-of-order delivery, and the missing packets can be consecutive or random.}, is crucial for real-time videos.

Yet, users of real-time video applications still suffer from video stuttering and poor visual quality~\cite{10.1145/3487552.3487842, webrtc-performance}. 
To minimize the delay of each frame, real-time video clients use a short buffer, \eg tens of milliseconds in WebRTC~\cite{10.1145/3410449}\footnote{In contrast, HTTP-based streaming videos, even live sports events, have a buffer of at least 10 seconds, allowing streaming video players to retransmit packets without causing video stalls. 
%However, this is not possible for RTC-based real-time video clients.
}. \passed{\amz{This should read as "tens of milliseconds" not "ten seconds of milliseconds", right?}}
This means that resending {\em any} packet, especially in long-latency networks, will block the decoding of multiple frames and cause video stuttering/stalls.
Unfortunately, packet loss and high latency jitter remain common across wide-area networks and cellular networks.
Therefore, it is crucial for real-time video coding to tolerate packet loss.
Here, we define {\em packet loss} on a given frame as any packets not received before the receiver decodes the frame.
%, \eg every 50ms at 20 frames per second (fps).
Packet loss can be consecutive or random and can result from packet drops or latency jitter.\footnote{It is important to clarify that our notion of packet loss rate is {\bf\em not} network-level loss rate. Even if a packet is not dropped, it can still be counted as a packet loss, if it arrives too late. It is not rare for real-time video clients to have a high (over 50\%) packet loss rate on some frames, even if the network has a very low packet drop rate. Our definition of packet loss rate is consistent with recent papers~\cite{rudow2023tambur,google-doc-fec}.}
%queuing delay or out-of-order delivery.
\passed{\jc{rewrote to tune down the contrast with vod. see if it's better}}
\passed{\fyy{I wouldn't contrast RTC with video-on-demand streaming. Their differences are well understood, and the comparison wastes the precious space in the first page.}}

%Yet, users are at least as susceptible to video stuttering and poor quality when using real-time video applications (\eg video calls and online gaming) as when watching on-demand videos (\eg Netflix). 
%% Despite intensive research on congestion control and bitrate adaptation~\cite{salsify,sprout} for Internet videos, 
%Long latencies and bandwidth fluctuations remain across wide-area networks and cellular networks.
%% , such as long-distance video calls. 
%To make it more challenging, real-time video clients use a very short buffer (\eg merely 10 ms in WebRTC~\cite{10.1145/3410449}) to render each frame as soon as they are received. 
%Consequently, waiting/retransmitting a single packet, which could take 100s ms or longer, will block multiple frames and cause a visual stuttering.

% These packet retransmits may not be concealed by the short buffer---merely 10 ms in WebRTC~\cite{10.1145/3410449}, which allows frames to be played as soon as they are decoded.
% As a result, the extra delay to wait or resend a single packet frame, which could take 100s ms or longer in long-latency links, can block the decoding of multiple frames and cause a visual stuttering. 


\begin{comment}
might be conceal by the playback buffer in on-demand streaming videos, 
%In on-demand video streaming, the extra delay of packet retransmits (which could be 100s ms or higher in long-latency links) is easy to conceal by the video buffer, but 
this may not be true for 
real-time videos use a very short buffer (\eg merely \fillme ms in WebRTC)~\cite{??}  in order to play each frame as soon as it is decoded.
As a result, the additional delay to wait or resend a single packet frame might block the decoding of multiple frames and cause a visual stuttering. 
\end{comment}




%Despite of many loss-resilience coding schemes, they fall short in different ways. 
%% fall short at realizing DS coding. 
%First, state-of-the-art scheme based on forward error correction (FEC), such as Tambur~\cite{tambur}, can tolerate packet loss but it is difficult to set an appropriate rate of FEC redundancy. 
%To tolerate $x$\% packet loss, it must add at least $x$\% redundancy {\em before} transmission~\cite{holmer2013handling, uberti2015webrtc}, and quality will be lowered to make space for the redundancy, even if all packets turn out to be successfully received (Figure~\ref{fig:intro-example}(a)). 
%Therefore, most systems, such as WebRTC, do not add FEC redundancy by default, and increase FEC redundancy only {\em reactively}, after packet loss has affected some frames~\cite{holmer2013handling}.
%%, which requires packets to be resent until enough packets are received.
%%For these frames whose \rate is underestimated, 
%%the receiver must still request the sender to resend some packets until at least 70\% of packets have arrived.
%%Even after the packet loss has subsided, FEC may still add too much redundancy, thereby reducing  video quality.  
%%Secondly, DS may seem similar to the concepts of 
%Second, scalable video coding (SVC)~\cite{SVCFEC1} and fine granularity scalability (FGS)~\cite{ma2022deepfgs,li2001overview} in theory can improve quality as more packets are received. 
%However, these schemes split a video into a hierarchy of layers, and packet loss at a lower layer can block the decoding of higher layers (Figure~\ref{fig:intro-example}(b)).
%%and their quality increases only if packets of a higher layer received in a specific hierarchy.
%%However, there is a key difference: quality in DS coding depends on how many packets are received {\em regardless} of which packets, but SVC and FGS split video into layers and their quality increases only if more layers are received in a specific hierarchy.
%Third, receiver-side error concealment may seem promising, but in order to decode any subset of packets, it must either use FEC or split a frame into independently encoded partitions.
%As a result, it has a lower quality than traditional codec like H.265 at the same bitrate~\cite{KUMAR2006425} (Figure~\ref{fig:intro-example}(c)).



Existing loss-resilient video coding schemes generally fall in two categories~\cite{wang2000error,wang1998error}, and they each fall short in different ways. 
% https://ivpl.northwestern.edu/wp-content/uploads/2019/02/Error_resilient_video_coding_techniques.pdf, https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=664283
First, in {\em encoder-side forward} error concealment, the sender adds redundancy to each frame {\em before} sending it out.
For instance, forward-error correction (FEC), which is well-studied and used in WebRTC~\cite{holmer2013handling, xiao2012dynamic}, can tolerate any $x$\% loss of packets by adding $x$\% redundancy.
However, it is difficult to pick an appropriate portion for FEC redundancy before packet loss occurs, and adding too much FEC redundancy lowers the video quality regardless how many packets are received. 
As a result, WebRTC and other systems do not add FEC redundancy by default and add FEC redundancy only after some frames are already affected by packet loss~\cite{holmer2013handling}.
Second, in {\em decoder-side post-processing} error concealment, the decoder uses received data to reconstruct the regions or frames affected by packet loss.
However, it must sacrifice compression efficiency in order for each received packet to be independently decodable~\cite{KUMAR2006425}.
%its quality at zero packet loss is worse than traditional codec like H.265 at the same bitrate~\cite{KUMAR2006425}, because it must add redundancy bits to allow each packet to be independently decodable (Figure~\ref{fig:intro-example}(c)).
Moreover, the decoder may not be able to reconstruct all lost information at a high loss rate. 
%As a result, its quality is lower than traditional codec like H.265 at the same bitrate~\cite{KUMAR2006425}, even when all packets are received (Figure~\ref{fig:intro-example}(c)).
\S\ref{subsec:related} will discuss more schemes that might help tolerate loss but are not designed specifically for loss resilience, such as functional decoder, scalable video coding, and super-resolution.
In short, these solutions either sacrifice the quality when there is no packet loss or fail to get decent quality under high packet loss rates.

\passed{\jc{good point. SVC doesn't have to be here; it should be used to contrast DS coding later. the text is updated.}}
\passed{\fyy{SVC is never designed to be an error-resilient scheme, and thus can be pushed back to Section 2 and related work. It is still important to mention SVC after ``we will discuss more schemes'' or explicitly explain why (e.g., it does not tolerate lost packets in its base layers), in case reviewers have it in mind and get confused. Later in Section 2/related work, is it also fair to say when evaluated from the perspective of error resilience, SVC is inferior to state-of-the-art post-processing error concealment approaches? It also needs to sacrifice compression efficiency to produce enhancement layers
(so the starting point of Figure 1(b) is inaccurate).
Anyway, removing SVC will make this paragraph logically easier to understand: there are ``forward'' approaches and ``post-processing'' approaches, but Grace jointly optimizes both or you can say Grace takes an unprecedented approach.}}


\begin{figure}[t!]
    \centering
        \includegraphics[width=0.83\linewidth]{figs/intro-example-illustrative-threelines.pdf}
         \tightcaption{Illustration existing loss-resilient schemes vs. this work at the same bitrate but under different packet loss rates. 
%         \name's data-scalable coding under packet loss of different \rates when compared with existing loss-resilient schemes. 
         (actual figures from our evaluation appear
later (e.g., Figures~\ref{fig:loss_by_bitrate}). 
        % \yc{just put a note here, should we add SVC in this graph? I like it but we may need to change some text?}
        \passed{\fyy{Similarly, SVC should be removed from Figure 1; otherwise, there's too much to parse. Then, one figure with three curves would suffice. Besides, DMR is not defined yet. Can you actually get rid of that and just say packet loss rate?}}
        } 
    \label{fig:intro-example}
    \vspace{-0.2cm}
    % \vspace{-0.5cm}
\end{figure}

%\begin{figure}[t!]
%    \centering
%%        \includegraphics[width=0.9\linewidth]{figs/intro-example-illustrative-short.pdf}
%        \includegraphics[width=0.99\linewidth]{figs/intro-example-illustrative-separate.pdf}
%         \tightcaption{Illustration existing loss-resilient schemes vs. this work at the same bitrate but under different packet loss rates. 
%%         \name's data-scalable coding under packet loss of different \rates when compared with existing loss-resilient schemes. 
%         (actual figures from our evaluation appear
%later (e.g., Figures~\ref{fig:loss_by_bitrate}). 
%\fyy{Similarly, SVC should be removed from Figure 1; otherwise, there's too much to parse.
%Then, one figure with three curves would suffice.
%Besides, DMR is not defined yet. Can you actually get rid of
%that and just say packet loss rate?}}
%    \label{fig:intro-example}
%    % \vspace{-0.5cm}
%\end{figure}

%\begin{figure}[t!]
%    \centering
%        \includegraphics[width=0.99\linewidth]{figs/intro-example-illustrative-old.pdf}
%         \tightcaption{(a) An example of \name's loss resilience under packet loss of different \rates, and (b) the potential quality/delay improvement by \name. These figures are illustrative; actual figures from our evaluation and trace analysis appear
%later (e.g., Figures~\ref{fig:normal-simulation}, \ref{fig:queue15-simulation}, \ref{fig:loss_by_bitrate}). }
%    \label{fig:intro-example}
%    % \vspace{-0.5cm}
%\end{figure}

% for high-quality, smooth real-time videos.

In this paper, we present \name, a new approach that {\em jointly trains a pair of neural-net (NN) encoder and NN decoder that optimize quality under a variety of packet loss rates}. 
Our insight is that by training the NN encoder and decoder under different rates of simulated packet loss (explained shortly), the resulting NN encoder and decoder forms a {\em generative autoencoder} that tolerates the packet loss while only marginally sacrificing the quality when there is no packet loss.
With the same encoding of each frame, \name obtains quality similar to the classic codec (H.265) used in WebRTC without FEC when there is no packet loss; and with higher packet loss rates, the quality gradually degrades but still better than state-of-the-art loss-resilient schemes.
%In other words, \name's video quality degrade gracefully with more packet loss while only marginally sacrificing the quality when there is no packet loss. 
%training the autoencoder under various packet loss rates, the decoded video quality can {\em degrade gracefully with more packet loss while only marginally sacrificing the quality in absence of packet loss}. 
\passed{\amz{I find the phrase "in absence of packet loss" difficult to parse, and it's used often in the intro. Can you replace at least a few instances with "when there is no packet loss"?}}
We refer to it as {\em Data-Scalable} (DS) coding. 
Figure~\ref{fig:intro-example} illustrates the contrast between DS coding and the two prior categories of error-resilient coding.
% \yc{should we put svc here if it's in figure 1?}
More specifically, DS coding has four practical benefits:
{\em (i)} it does not need to predict the loss rate before sending the packets, 
{\em (ii)} a frame can be decodable under {\em any} loss rate, unless all packets are lost, 
{\em (iii)} quality gradually improves if more packets are received\footnote{Scalable video coding (SVC)~\cite{SVCFEC1} and fine granularity scalability (FGS)~\cite{ma2022deepfgs,li2001overview} in theory could also improve quality with more packets. 
However, they split a video into a hierarchy of layers, 
%and packet loss at a lower layer can block the decoding of higher layers. Thus, 
so unlike DS coding, a new packet may not always improve quality, if the lower layers are not fully received.}, and
{\em (iv)} when all packets are received, it reaches a quality similar to the traditional codec like H.265 used in WebRTC.
\passed{\amz{Item (iii) is confusingly written -- if I understood correctly after reading the footnote, "quality gradually improves as more packets are received" or "quality scales gradually as more packets are received" will be more clear.}}

%More specifically, \name encodes and decode each frame 
%%We present \name, a concrete example of this approach that encodes and decodes video frames 
%using a {\em novel antoencoder} whose encoder and decoder are neural nets (NNs).
To add packet loss in the training of the generative autoencoder, we simulate packet loss as follows.
%jointly train the NN encoder and NN decoder under various loss rates, 
%\name simulates packet loss as follows. 
\name uses a new packetization scheme that {\em partitions} the encoder's output tensor and {\em entropy encodes} each partition as a {\em separate} packet. 
If all packets are received, the decoder's input will be identical to the encoder's output.
If a packet is lost, the values in its partition are set to zeros (\ie {\em masked}) in the decoder's input. 
%By training under different rates of simulated packet loss, 
%By simulating the effect of packet loss on decoder's input, \name jointly trains the encoder and decoder NNs to optimize the decoded video quality under various rates of packet loss. 
\S\ref{sec:core} shows more details of our training process and packetization process. 


Once the generative autoencoder is trained, \name entails several optimizations to stream video online efficiently (\S\ref{sec:delivery}).
%entails several optimizations to stream video efficiently online (\S\ref{sec:delivery}).
%For instance, \name minimizes the size inflation caused by the design choice of entropy encoding each packet separately (rather than entropy encode the entire encoder's output). 
In particular, in order to encode each frame at a given target bitrate, \name trains multiple pre-trained 
% \yc{the word "pre-trained" is a bit confusing here, are we saying we are not doing online training?} 
encoders that produce different encoded bitrates but share most computation, so with minimum compute overhead, \name can encode a frame at multiple bitrates and then pick the encoded bitrate similar to the target bitrate. 
When the receiver decodes a frame of partially received packets, \name uses a protocol to re-synchronize the encoder and decoder states without need for retransmission.
\name also entails optimizations to run the NN encoder and decoder on CPUs and reduce the size inflation due to per-packet entropy encoding. 

%\name's per-packet entropy encoding
\passed{\amz{This sentence is confusing, since the entropy encoding scheme is not mentioned before, so I had no context for the size inflation. Flipping the sentence ("\name entropy encodes each packet separately, so we optimized the design to minimize potential size inflation" would read easier.}}
%\name also uses a customized protocol to re-synchronize the states on the sender when the receiver decodes a frame without waiting for all packets to arrive.
%\S\ref{sec:delivery} details other optimizations, such as a way to drastically reduce autoencoder overhead (on GPUs and CPUs) and efficient bitrate control to fit the encoding bitrate to target sending rate set by congestion control.
%To make \name practical, \name also includes schemes to 
%speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{subsec:fast-coding}).








\tempstrike{
\mypara{Data-scalable (DS) coding}
We define the {\em Data Missing Rate} (\rate) of a frame as the fraction of packets not received before the  receiver decodes the frame\footnote{\rate is similar to packet loss rate defined on a single frame.}, \eg every 50ms at 20 frames per second (fps).
A packet can be missing due to packet drops, queuing delay or out-of-order delivery, and the missing packets can be consecutive or random.
{\em Without} knowing the actual \rate, an ideal loss-resilient coding scheme should encode a frame  such that
%Then {\em without} knowing the actual \rate, an ideal loss-resilient scheme should meet three criteria: 
\begin{packeditemize}
\item {\em (i)} the frame is decodable under any \rate below 100\% (\ie at least one packet is received), 
\item {\em (ii)} the quality is close to a non-loss-resilient codec (\eg H.265) when all packets are received, and
%as long as {\em any} (non-empty) subset of packets of the frame is received, 
%(\ie no need for retransmission unless all data is lost);  
\item {\em (iii)} quality degrades gracefully with higher \rate, \ie quality gradually improves if {\em any} more packets are received.
\end{packeditemize}
We call such a coding scheme {\em data-scalable} (DS).
DS coding is ideal for real-time video, because without retransmission, its quality degrades gracefully with more packet loss (higher \rate) while not sacrificing quality in absence of packet loss. 
}





\tempstrike{
Some loss-resilient scheme uses an older but reliably received frame as the reference frame, allowing the decoder to safely skip a loss-affected frame (\eg~\cite{salsify}).
%without hurting future frames, 
However, using an old reference frame means more bits to achieve the same quality as using the last frame as reference, which lowers compression efficiency.
}


%achieve high {\em compression efficiency}, which means high quality with fewer bits, and {\em loss resilience} under various data missing rate or {\em \rate} defined by
%the fraction of data that is not received, due to packet drops or queuing, before a frame is decoded.

\tempstrike{
Unfortunately, current real-time video systems achieve loss resilience by adding various forms of redundancies, thus sacrificing compression efficiency (as elaborated in \S\ref{subsec:prior}).\footnote{
Scalable video coding (SVC~\cite{SVCFEC1}, FGS~\cite{ma2022deepfgs,li2001overview}, Swift~\cite{swift}), which works well for on-demand streaming videos, will be much less effective in real-time videos which send packets of a frame together, instead of layer by layer (see \S\ref{subsec:prior}).
For this reason, scalable video coding is not commonly used to improve unicast real-time videos~\cite{salsify}. 
Similarly, selective frame skipping (\eg~\cite{voxel}) might work for on-demand videos, but in real-time videos, most frames are P-frames which cause poor quality once dropped, unless I-frames are frequently inserted.
Nonetheless, we will still evaluate them against \name.}
%\jc{add old reference frame}
}



\tempstrike{
In contrast, an ideal loss-resilient coding should be {\em Data-Scalable} (DS)---{\em its quality should degrade gracefully with higher packet loss rate but without sacrificing the quality in absence of packet loss} (illustrated in Figure~\ref{fig:intro-example}(d)). 
DS coding has several benefits: 
{\em (i)} it does not need to predict loss rate before sending the packets (unlike FEC), 
{\em (ii)} a frame can be decodable under {\em any} loss rate, unless all packets are lost, 
{\em (iii)} quality gradually improves if {\em any} more packets are received (unlike SVC), and
{\em (iv)} when all packets are received, it reaches a quality similar to the traditional codec like H.265 used in WebRTC (unlike error concealment).

This paper presents \name, a new loss-resilient scheme for real-time video, which better approximates DS coding by using an autoencoder (neural encoder and neural decoder) to optimize quality under various packet loss rates.
The key idea is two-fold.
\begin{packeditemize} 
\item \name's {\em a loss-resilient autoencoder} (\S\ref{subsec:training}) consists of a pair of neural encoder and neural decoder {\em jointly trained} to optimize video quality when $x$\% of values in the encoder output of a frame are randomly selected and masked (\ie set to zeros), with $x$\% between 0 to 100\%, before the masked data is fed to the decoder. 
This simulates the effect of random data masking between the encoder and the decoder.
\item \name uses a {\em novel packetization scheme} (\S\ref{subsec:packetization}) to partition the encoder output of a frame and entropy encodes each partition as an independently decodable packet, so that losing any $x$\% packets (which can be consecutive or random) has the same effect on the input of the decoder as masking $x$\% of randomly selected values.
In short, packet loss will appear to have same effect as random data masking between the encoder and the decoder.
\end{packeditemize} 
}

%When put together, the two ideas help \name to optimize quality under various packet loss rates, so it better approximates DS coding than prior schemes.
%
%When no packet is lost, \name's quality is similar to H.265 at the same bitrate, but as loss rate increases, \name's quality degrades much more gracefully than state-of-the-art loss-resilient coding schemes.
%%(Figure~\ref{fig:intro-example}). 
%In short, \name better approximates DS coding than prior schemes when packet loss affects one frame. 
%%when tested under different \rates.



%presents a way to smooth frame size across different frame types (I-frames and P-frames)


%To leverage the new data-scalable (DS) autoencoders, \name also includes a customized video streaming framework to delivery a sequence of frames to synchronize the states on the sender and the receiver when the receiver decodes a frame without waiting for 
%%in a slightly lazy fashion.
%It also includes optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).
%to deliver autoencoder-generated data.
%It uses a new packetization scheme on randomly shuffled \aecode with per-packet entropy encoding, which makes packet loss of $n\%$ \rate appear to have the same effect as $n\%$ random making on the \aecode (\S\ref{subsec:packetization}). 
%\name also uses techniques for DS coding over a sequence of frames, as well as optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).







We have implemented \name and evaluated \name using real network traces and a range of video content genres (all from different data sources from the training set) and compare it against a range of state-of-the-art loss resilient schemes, including 
{\em (i)} forward error concealment (Tambur~\cite{rudow2023tambur}), 
{\em (ii)} postprocessing error concealment by neural-net in-painting~\cite{xiang2019generative}, 
{\em (iii)} scalable video coding (Swift~\cite{swift}), and
{\em (iv)} selective frame skipping (Voxel~\cite{voxel} and Salsify~\cite{salsify})
%å, and {\em (v)} functional codecs (Salsify~\cite{salsify}).
%{\em (i)} FEC (Tambur~\cite{rudow2023tambur}), {\em (ii)} error concealment (neural-net generative in-painting~\cite{xiang2019generative} and selective skipping~\cite{voxel}), {\em (iii)} Scalable Video Coding~\cite{swift}, and {\em (iv)} Salsify's functional codec~\cite{salsify}
To be fair, we run \name and the baselines over the same congestion control (CC) algorithm, GCC~\cite{carlucci2016analysis}, which is the standard CC used in WebRTC.
% including GCC~\cite{carlucci2016analysis} and Salsify~\cite{salsify} (except that packet retransmission is turned off for loss-resilient decoders).
Our key results are: 
\begin{packeditemize}
\item \name achieves a similar average quality (in SSIM) with the codec used in WebRTC at the same bitrate. In other words, \name does not sacrifice quality when there is no packet loss. %in absence of packet loss.
\item \name achieves better quality, by 1.4-4 dB of SSIM, than other loss-resilient schemes at the same packet loss and bitrate. 
\item When running on real network traces, \name  reduces the duration of video stalls, number of non-rendered frames, and 98$^{th}$ percentile frame delay by \review{90}\%, \review{95}\%, and \review{66}\% respectively, when compared to the most competitive baselines. 
\item With much less video stuttering and fewer skipped frames, our user study confirms that \name has \review{38}\% higher mean opinion score (MOS) than the most competitive loss-resilient schemes.
\item On a single Nvidia A40 GPU, \name can decode 480p and 720p at 120~fps and 44.1~fps respectively and encode 480p and 720p at 87.7~fps and 31.2~fps, which is 1.5-5$\times$ faster than recent video autoencoders. On CPUs, it can encode 720{p} videos at 28.5~fps (on par with GPU) at only a drop of 0.5 dB in SSIM.
\end{packeditemize}
%ratio of delayed frames (defined as the frames whose delay between encoding and decoding is larger than 400~ms) by up-to 4$\times$ and the stall rate (defined as the fraction of inter-frame gaps that exceed 200~ms) by 10$\times$. 
%compared to the most competitive baselines which still have to retransmit packets or skip frames.


To put \name's contribution in context, neural video codecs have long been used in multimedia, but \name is, to our best knowledge, the first to jointly train generative NN encoder and decoder to improve loss resilience in real-time video.
\name is closely related to using NNs to generatively reconstruct the missing data in lost packets, but they do not jointly train the encoder for loss resilience (\eg~\cite{sankisa2018video,reparo}) and handle only special content type at low resolution~\cite{reparo}.
\name is also related to but different from an emergent techniques~\cite{kurka2020deepjscc,bourtsoulatze2019deep,gunduz2019machine} which train autoencoders to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss).
%Most work on autoencoders has focused on improving {\em compression efficiency} rather than loss resilience, such as scalable video coding (Swift~\cite{swift} and DeepFGS~\cite{ma2022deepfgs}), super resolution~\cite{gemino,neuroscaler,livenas}.
%Neural networks have been used to reconstruct missing spatial blocks in lost packets (\eg~\cite{sankisa2018video,reparo}, which uses NNs on the decoder side and handles only specific video content (\eg talking head~\cite{reparo}). 
%In contrast, \name jointly trains the encoder and decoder to handle packet loss.
%\name is related to but different from an emergent techniques~\cite{kurka2020deepjscc,bourtsoulatze2019deep,gunduz2019machine} which train autoencoders to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss).

\passed{\jc{agreed that this is a bit too long. tried to shrink it.}}
\passed{\amz{I understand including so much comparison to related work to hedge the "first to our knowledge" claim, but it is quite long considering the related work comes so soon after. I would remove everything after the first sentence and put it above the limitations paragraph, or just wrap up all the citations in a "other approaches address compression efficiency, post-processing, or signal noise". }}

While \name improves quality under packet loss, the approach has limitations (\S\ref{sec:limit}). 
%\amz{This sentence is awkward, I think you can more generously say "While \name improves quality under packet loss, the approach has limitations."}
First, though our implementation of \name can run much faster than traditional autoencoders,
% and achieves lower delay than alternative solutions 
\name cannot run in real-time on resource-constraint devices yet. 
%\amz{Fast enough for what, real-time? }
Second, we focus on unicast video communication, rather than problems in multi-party conferencing (\eg stream forwarding). 
% Third, \name cannot improve the video quality when all packets are lost. 
%\amz{Cannot improve what? }
%\jc{mention that packet loss is often not 100\% given audio still continues}
%While \name decides {\em what} each packet contains, 
Our main goal is to show the potential of training generative autoencoders under different loss rates.
And these challenges are left for future work.


\tempstrike{
% \ie no data loss between the encoder and the decoder, so they need to combined with a loss-resilient scheme.
For instance, Swift~\cite{swift} and DeepFGS~\cite{ma2022deepfgs} use NN codecs to improve scalable video coding (rather than loss tolerance) for on-demand (rather than real-time) videos. 
Super-resolution (SR)~\cite{gemino,neuralscaler} enhances the decoded video quality at the receiver when the available bandwidth is low
DeepJSCC uses an autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss)~\cite{kurka2020deepjscc}.
\name also differs from neural super-resolution models~\cite{neuroscaler,livenas} and generative neural error concealment~\cite{sankisa2018video, reparo} which only trains NNs on the receiver and handles only specific video content (\eg talking head~\cite{reparo}), whereas \name jointly trains the encoder and decoder to handle packet loss.


, and {\em (v)} super resolution (SR)~\cite{??}.\footnote{\editSOCC{The main use case of SR is to enhance the decoded video quality at the receiver when the available bandwidth is low. Such technique should work for any kind of video codecs. Therefore, SR is orthogonal to \name.}} %\jc{explain SR is orthogonal}

}

%There are two key findings (an example of which is given in Figure~\ref{fig:intro-example}). 
%First, when no packets are lost, \name's quality does not exceed H.265 at the same bitrate, but in presence of more packet loss, \name's quality degrades much more gracefully than other loss-resilient coding schemes.
%Second, we use packet-level simulation driven by real-world bandwidth traces and run \name and the baseline loss-resilient coding schemes. % on the same CC logic (retransmits disabled).
%We show that compared to the baselines, \name reduces the ratio of delayed frames (defined as the frames whose delay between encoding and decoding is larger than 400~ms) by up-to 4$\times$ and the stall rate (defined as the fraction of inter-frame gaps that exceed 200~ms) by 10$\times$. 
%%compared to the most competitive baselines which still have to retransmit packets or skip frames.
%With much less video stuttering and fewer skipped frames, our user study confirms that \name has higher average subjective ratings by users than the baselines.
%
%Second, \name borrows existing congestion control (CC) logics {\em without} packet retransmits unless all packets of a frame are lost), such as GCC~\cite{carlucci2016analysis}, which decides the target frame size and how fast to send the \name-encoded packets.


%\textbf{This work does not raise any ethical issues.}



%Though autoencoders have a long history in multimedia, standard autoencoders have focused on better compression efficiency (achieving higher quality in fewer bits) and are not inherently loss-resilient.
%This is because, in traditional autoencoder training, the decoder always receives the {\em same} \aecode produced by the encoder, which does not prepare the autoencoders to handle any data loss during transmission. 
%
%To put it in context, neural encoders and decoders have long been used in multimedia (see \S\ref{sec:related}) but \name is, to our best knowledge, the first to demonstrate the potential of autoencoders to improve loss resilience in real-time video.
%Swift and DeepFGS, for instance, use autoencoders to improve scalable video coding (rather than loss tolerance) for on-demand (rather than real-time) videos~\cite{swift, ma2022deepfgs}. 
%DeepJSCC uses an autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss)~\cite{kurka2020deepjscc}.
%\name also differs from neural error concealment~\cite{sankisa2018video} which only uses NNs on the receiver, whereas \name jointly trains the encoder and decoder to handle packet loss.


\tempstrike{


Autoencoders work like a standard video codec but replace part of the encoder and decoder with neural networks (NNs). 
Though autoencoders have a long history in multimedia, standard autoencoders have focused on better compression efficiency (achieving higher quality in fewer bits) and are not inherently loss-resilient.
This is because, in traditional autoencoder training, the decoder always receives the {\em same} \aecode produced by the encoder, which does not prepare the autoencoders to handle any data loss during transmission. 



This paper presents \name, a new approach to loss-resilient real-time video, by customizing {\em  autoencoders}. 
%This paper presents \name, a new end-to-end loss-resilient real-time video streaming system, by customizing {\em  autoencoders} following the idea proposed in~\cite{cheng2022grace}. 

In \name, we show that autoencoder-based video streaming can be loss-resilient by customizing the autoencoder training process (\S\ref{sec:core}) and video streaming framework (\S\ref{sec:delivery}).

In \name's autoencoder training process (\S\ref{subsec:training}), when the NN encoder returns a \aecode, we randomly mask n\% of its elements to zeros before feeding it to the NN decoder, a process we call {\em random masking}. We vary the rate of random masking ($n\%$) between [0\%, 100\%), which as explained shortly, simulates the effect of packet loss under different \rates.
% As explained shortly, varying the rate of random masking (n%n\%) between [0\%, 100\%) simulates the effect of packet loss under different \rates.
Consequently, our trained autoencoder, {\em without} knowing the actual \rate, can encode a frame such that it can: {\em (i)} decode a frame as long as {\em any} (non-empty) subset of packets of the frame is received;
%(\ie no need for retransmission unless all data is lost);  
{\em (ii)} achieve better quality with the addition of each new packet (\ie graceful degradation with higher \rate); and
{\em (iii)} reach a quality close to a non-loss-resilient coding algorithm (such as H.265) when all packets are received.
We refer to it as {\em Data-Scalable} ({\em DS}) video coding.
In contrast, FEC is not DS coding, since its quality does not improve with more data if the \rate is below a threshold but the quality drops abruptly (due to retransmits) once the \rate exceeds the threshold.

}

% Our prior work of data-scalable (DS) autoencoders~\cite{cheng2022grace} suffers from multiple problems: {\em (i)} naive entropy encoding lowers compression efficiency, {\em (ii)} encoding speed insufficiently fast (<20fps) for real-time video streaming requirements, and {\em (iii)} additional quality degradation due to error propagation from packet losses.
% %To leverage the new data-scalable (DS) autoencoders, 
% To address the above challenges, \name uses a customized video streaming framework to deliver autoencoder-generated data.
% It uses a new packetization scheme with per-packet entropy encoding, which makes packet loss of $n\%$ \rate appear to have the same effect as $n\%$ random making on the \aecode (\S\ref{subsec:packetization}) with negligible size overhead. 
% \name also uses techniques for DS coding over a sequence of frames to minimize the propagation of error, as well as optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).


\begin{comment}

It uses a novel packetization scheme that makes packet loss of n%n\% appear to have the same effect as n%n\% random making on the \aecode (see \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{subsec:packetization} for details). 
%Standard autoencoders entropy encode the NN encoder output (\aecode) and packetize the resulting bitstream, so any packet loss will render it undecodable by the receiver.
The basic idea is to randomly split the \aecode's elements to partitions, each separately entropy-encoded as an independently decodable packet, and if n%n\% packets are lost, we set their elements in the \aecode to zeros, which mimics random masking.
However, this naive scheme greatly increases the size of the compressed data, due to the additional space needed to store the symbol distribution (used by entropy-decoding) in each packet.
\name addresses this challenge by carefully coarsening the granularity of symbol distributions, which significantly reduces size increase while maintaining the compression efficiency of entropy coding. 

\end{comment}





\begin{comment}

Ideally, the quality should degrade gracefully with more packet loss (higher \rate), without compromising the quality in absence of packet loss.
Specifically, it should be able to 
{\em (i)} decode a frame as long as {\em any} (non-empty) subset of packets of the frame is received;
%(\ie no need for retransmission unless all data is lost);  
{\em (ii)} achieve better quality with the addition of each new packet (\ie lower \rate); and
{\em (iii)}  reach a quality close to a non-loss-resilient coding algorithm (such as H.265), when all packets are received.
We refer to it as {\em Data-Scalable} ({\em DS}) video coding.
FEC is not DS coding, since its quality does not improve with more data if the packet loss rate is below a threshold but the quality drops abruptly once loss rate exceeds the threshold.


\mypara{Data-scalable autoencoder}
This paper introduces {\em \name}, a real-time video system that, for the first time, uses {\em  autoencoders (AEs)} to realize data-scalable (DS) video delivery.
%which explores a new approach to DS video delivery by using {\em neural-net (NN) autoencoders}.
At a high level, autoencoders work like a standard video codec but replace some coding logic with neural networks (NNs). 
It uses an NN encoder to encode a frame to a {\em \aecode} (without entropy encoding), and an NN decoder to decode to a reconstructed frame that is similar to the original frame. 


We choose autoencoders, not because the off-the-shelf models are inherently data-scalable (DS), but due to their unique properties that {\em could} enable DS coding. 
%\name is a particular design that harnesses these properties to enable DS coding.
Specifically, the NN decoder can reconstruct a decent-quality frame, even if we {\em randomly erase} (\ie set to zeroes) a subset of $n\%$ elements in the \aecode (the output of the NN encoder).
In other words, {\em random data erasure} on the \aecode has a limited impact on the decoding quality of autoencoders. 
This can be attributed to the lack of stringent dependencies among the elements in a \aecode\footnote{
%Mathematically, this smoothness is a result of NN encoders and decoders having continuous derivatives everywhere. Moreover, 
This can also be intuitively understood that NN decoders share the architecture of {\em generative} NNs, such as variational autoencoder (VAE), which can create realistic-looking images from random inputs.}, unlike SVC where the decoding of a layer depends on the lower layers.


Despite the promise of autoencoders, several practical challenges remain.
%\name addresses several practical challenges.
Two of them will be highlighted here.

%Despite the promise of autoencoders, \name must address several practical challenges, such as improving quality under various \rates, making entropy encoding of \aecodes loss-resilient, controlling bitrate, and speeding up autoencoder coding. 
%Two of them will be highlighted here.


%\mypara{Adding packet loss in autoencoder training}
\mypara{Training autoencoder with packet loss}
First, the quality of standard autoencoders drops quite significantly if more data is erased from the \aecode. 
This is because the standard autoencoder training, in which  the decoder always sees the same \aecode returned by the encoder, never prepares the autoencoder to handle any data loss between the encoder and the decoder. 
\name trains autoencoders different (see \S\ref{??} for details).
It applies random data erasures to the \aecode (which could simulate the effect of packet loss as explained shortly), and by varying the rate of data erasure between [0\%, 100\%), 
%In other words, by training the NN encoder and NN decoder jointly, 
the new autoencoders not only learn how to compress high-quality frames efficiently but also to be robust to different rates of random data erasures. 

%, which simulates the effects of packet loss under different \rates (which will be explained shortly).






\mypara{Per-packet entropy coding for autoencoder}
Standard autoencoders use entropy encoding to losslessly compress a \aecode to a single bitstream and then packetize it, so any packet loss will render it undecodable.
%entropy coding used in current autoencoders cannot tolerate any packet loss. 
A naive idea is to randomly 
split the \aecode's elements to partitions,
%split a \aecode to sub-tensors, 
each separately entropy-encoded as an independently decodable packet, and if $n\%$ packets are lost, we set their elements in the \aecode to zeros, which resembles random erasure.
%effectively erases a random subset of $n\%$ elements.
%is the same as 
%random data erasure.
However, this naive per-packet entropy coding greatly increases the size of the compressed data, due to the additional space needed to store the symbol distribution (used by entropy-decoding) in each packet.
%To mitigate the size increase, 
\name carefully coarsens the granularity of symbol distributions, which significantly reduces size increase while maintaining the compression efficiency of entropy coding (see \S\ref{??} for details). 




Besides achieving loss resilience on a single frame, \name uses a novel frame delivery system to approximate DS coding over a sequence of frames, speed up autoencoder coding (on GPUs and CPUs), and enable efficient bitrate control (\S\ref{??}).




\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/fig1-example.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/fig1-example-osdi.pdf}
        \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/fig1.png}
         \caption{graceful degradation}
         \label{fig:normal-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
         \caption{delay quality tradeoff}
         \label{fig:normal-ssim-delay}
     \end{subfigure}
         \label{fig:}
         \tightcaption{Example results of \name's (a) more graceful degradation in presence of packet loss than prior solutions, and (b) better tradeoffs between video quality and tail frame delay, which corroborates the subjective rating of users.
         More results can be found in \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{sec:eval}. 
%         \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
    \jc{TODO: add a horizontal line to indicate the quality of H.265}
    \textcolor{red}{Yihua: TODO: update real values (fig1data.xlsx)}
         }
    \label{fig:intro-example}
\end{figure}

\end{comment}






%including a custom streaming protocol
%controlling bitrate, and speeding up autoencoder coding. 


%, so that even if the selected bitrate overshoots the bandwidth, we can still obtain decent quality.


%Being a coding system, \name can work with existing congestion control (CC) logics---CC decides how fast to send packets, and \name decides {\em what} each packet contains.




%Much remains unknown about the limits of autoencoders as a loss-resilient coding layer.

%To our best knowledge, \name is the first end-to-end autoencoder-based video system for loss-resilient real-time videos.
%that achieves stream real-time videos in a data-scalable fashion. 



%arising from training and using autoencoders in real-time video communication.

%Many aspects of \name are also inspired by prior work. 
%That said, \name, to our best knowledge, is the first to develop custom autoencoders that realize data-scalable video delivery.

%\name aims at unicast video sessions, rather than multi-party conferences. 
%It is also important that \name's autoencoders do {\em not} achieve better compression efficiency than recent heavily engineered video codecs, such as H.265. 
%Indeed, \name's video quality is still slightly lower than H.265 at the same bitrate. 








==> sections/old/intro_v15.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}

Real-time video communication has a long history in research, yet only recently has it become truly widespread in our daily lives~\cite{blum2021webrtc}.
RTC (and WebRTC clients) has become the de-facto platform for real-time videos, just like HTTP and DASH is for streaming videos, enabling more and more new applications~\cite{webrtc-trend-1,webrtc-trend-2}, from online meetings~\cite{webrtc-vc-1,webrtc-vc-2}, cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2}, to interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2} and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
%The amount of time people spend on real-time videos grow faster than the time spent on watching streaming videos~\cite{webrtc-trend-1,webrtc-trend-2}.





%Compared to streaming videos (over HTTP), such as video-on-demand, users are at least as susceptible to video stuttering and poor quality when using real-time video applications (\eg video conferencing and online gaming). 
%However, real-time video clients use a very short buffer in order to render each frame as soon as they are received.
%For instance, the buffer in WebRTC is merely 10s of ms~\cite{10.1145/3410449}; in contrast, HTTP-based streaming videos, even live sports event, have a buffer of at least 10 seconds. 
%To make it worse, long latencies and bandwidth fluctuations remain across wide-area networks and cellular networks, causing occasional packet loss and latency jitter. 
%Waiting/retransmitting a single packet can take 100s ms or longer and block multiple frames, causing video stuttering.
%Thus, loss-resilient video coding, which can tolerate any packet loss rate\footnote{To avoid ambiguity, we define {\em the packet loss rate on a frame} as the fraction of its packets not received before the receiver decodes the frame, \eg every 50ms at 20 frames per second (fps).
%A packet can be lost due to packet drops, queuing delay or out-of-order delivery, and the missing packets can be consecutive or random.}, is crucial for real-time videos.

Yet, users of real-time video applications still has poor experience due to video stalls, low visual quality or frequent quality switches~\cite{10.1145/3487552.3487842, webrtc-performance}. 
This is because the nature of real-time applications requires the clients to have a very short buffer, \eg tens of milliseconds in WebRTC~\cite{10.1145/3410449}\footnote{In contrast, HTTP-based streaming videos, even live sports events, have a buffer of at least 10 seconds, allowing streaming video players to retransmit packets without causing video stalls. 
%However, this is not possible for RTC-based real-time video clients.
}. 
%\passed{\amz{This should read as "tens of milliseconds" not "ten seconds of milliseconds", right?}}
This means that resending {\em any} packet, especially in long-latency networks, will block the decoding of multiple frames and cause video stalls.
Hence, it is crucial to tolerate packet loss, especially since packet drops and high latency jitters remain common across wide-area and cellular networks.
% Unfortunately, packet drops and high latency jitter remain common across wide-area networks and cellular networks.
% Therefore, it is crucial for real-time video coding to tolerate packet loss.
Here, we define {\em packet loss} on a given frame as any packets not received before the receiver decodes the frame.
%, \eg every 50ms at 20 frames per second (fps).
Packet loss can be consecutive or random and can result from packet drops or latency jitter.\footnote{It is important to clarify that our notion of packet loss rate is {\bf\em not} the traditional network-level loss rate. Even if a packet is not dropped, it can still be counted as a packet loss, if it arrives too late. It is not rare for real-time video clients to have a high (over 50\%) packet loss rate on some frames, even if the network has a very low packet drop rate. Our definition of packet loss rate is consistent with recent papers~\cite{rudow2023tambur,google-doc-fec}.}
%queuing delay or out-of-order delivery.
% \passed{\jc{rewrote to tune down the contrast with vod. see if it's better}}
% \passed{\fyy{I wouldn't contrast RTC with video-on-demand streaming. Their differences are well understood, and the comparison wastes the precious space in the first page.}}

%Yet, users are at least as susceptible to video stuttering and poor quality when using real-time video applications (\eg video calls and online gaming) as when watching on-demand videos (\eg Netflix). 
%% Despite intensive research on congestion control and bitrate adaptation~\cite{salsify,sprout} for Internet videos, 
%Long latencies and bandwidth fluctuations remain across wide-area networks and cellular networks.
%% , such as long-distance video calls. 
%To make it more challenging, real-time video clients use a very short buffer (\eg merely 10 ms in WebRTC~\cite{10.1145/3410449}) to render each frame as soon as they are received. 
%Consequently, waiting/retransmitting a single packet, which could take 100s ms or longer, will block multiple frames and cause a visual stuttering.

% These packet retransmits may not be concealed by the short buffer---merely 10 ms in WebRTC~\cite{10.1145/3410449}, which allows frames to be played as soon as they are decoded.
% As a result, the extra delay to wait or resend a single packet frame, which could take 100s ms or longer in long-latency links, can block the decoding of multiple frames and cause a visual stuttering. 


\begin{comment}
might be conceal by the playback buffer in on-demand streaming videos, 
%In on-demand video streaming, the extra delay of packet retransmits (which could be 100s ms or higher in long-latency links) is easy to conceal by the video buffer, but 
this may not be true for 
real-time videos use a very short buffer (\eg merely \fillme ms in WebRTC)~\cite{??}  in order to play each frame as soon as it is decoded.
As a result, the additional delay to wait or resend a single packet frame might block the decoding of multiple frames and cause a visual stuttering. 
\end{comment}




%Despite of many loss-resilience coding schemes, they fall short in different ways. 
%% fall short at realizing DS coding. 
%First, state-of-the-art scheme based on forward error correction (FEC), such as Tambur~\cite{tambur}, can tolerate packet loss but it is difficult to set an appropriate rate of FEC redundancy. 
%To tolerate $x$\% packet loss, it must add at least $x$\% redundancy {\em before} transmission~\cite{holmer2013handling, uberti2015webrtc}, and quality will be lowered to make space for the redundancy, even if all packets turn out to be successfully received (Figure~\ref{fig:intro-example}(a)). 
%Therefore, most systems, such as WebRTC, do not add FEC redundancy by default, and increase FEC redundancy only {\em reactively}, after packet loss has affected some frames~\cite{holmer2013handling}.
%%, which requires packets to be resent until enough packets are received.
%%For these frames whose \rate is underestimated, 
%%the receiver must still request the sender to resend some packets until at least 70\% of packets have arrived.
%%Even after the packet loss has subsided, FEC may still add too much redundancy, thereby reducing  video quality.  
%%Secondly, DS may seem similar to the concepts of 
%Second, scalable video coding (SVC)~\cite{SVCFEC1} and fine granularity scalability (FGS)~\cite{ma2022deepfgs,li2001overview} in theory can improve quality as more packets are received. 
%However, these schemes split a video into a hierarchy of layers, and packet loss at a lower layer can block the decoding of higher layers (Figure~\ref{fig:intro-example}(b)).
%%and their quality increases only if packets of a higher layer received in a specific hierarchy.
%%However, there is a key difference: quality in DS coding depends on how many packets are received {\em regardless} of which packets, but SVC and FGS split video into layers and their quality increases only if more layers are received in a specific hierarchy.
%Third, receiver-side error concealment may seem promising, but in order to decode any subset of packets, it must either use FEC or split a frame into independently encoded partitions.
%As a result, it has a lower quality than traditional codec like H.265 at the same bitrate~\cite{KUMAR2006425} (Figure~\ref{fig:intro-example}(c)).



% Existing loss-resilient video coding schemes generally fall in two categories, and they each fall short in different ways. 
Two general categories of loss-resilient video coding exist, but they each fall short in different ways ~\cite{wang2000error,wang1998error}.
% https://ivpl.northwestern.edu/wp-content/uploads/2019/02/Error_resilient_video_coding_techniques.pdf, https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=664283
First, in {\em encoder-based forward} error correction, the sender adds redundancy to each frame {\em before} sending it out.
For instance, forward-error correction (FEC), which is well-studied and used in WebRTC~\cite{holmer2013handling, xiao2012dynamic}, can tolerate any $x$\% loss of packets by adding $x$\% redundancy.
However, since the redundancy must be added by the sender before knowing the packet loss rate, it is difficult to pick an appropriate amount of FEC redundancy. 
It still requires retransmission and causes video delay/stall if the redundancy is smaller than the actual packet loss, yet adding too much FEC redundancy lowers the video quality regardless of how many packets are lost. 
Because of the negative impact of FEC redundancy on quality, WebRTC and other systems do not add FEC redundancy by default and add FEC redundancy only until some frames are already affected by packet loss~\cite{holmer2013handling}. 
Second, in {\em decoder-based post-processing} error concealment, the decoder uses received data to reconstruct the regions or frames affected by packet loss.
However, the sender must sacrifice compression efficiency in order for each received packet to be independently decodable~\cite{KUMAR2006425}.
%its quality at zero packet loss is worse than traditional codec like H.265 at the same bitrate~\cite{KUMAR2006425}, because it must add redundancy bits to allow each packet to be independently decodable (Figure~\ref{fig:intro-example}(c)).
Moreover, the decoder cannot reconstruct all lost information, since the encoder is trying to include as little redundancy as possible to achieve a better compression ratio.
%As a result, its quality is lower than traditional codec like H.265 at the same bitrate~\cite{KUMAR2006425}, even when all packets are received (Figure~\ref{fig:intro-example}(c)).
\S\ref{subsec:related} will discuss more schemes that might help tolerate loss but are not designed specifically for loss resilience, such as scalable video coding, and super-resolution.
In short, these solutions either sacrifice the quality when there is no packet loss or fail to get decent quality under high packet loss rates.

% \passed{\jc{good point. SVC doesn't have to be here; it should be used to contrast DS coding later. the text is updated.}}
% \passed{\fyy{SVC is never designed to be an error-resilient scheme, and thus can be pushed back to Section 2 and related work. It is still important to mention SVC after ``we will discuss more schemes'' or explicitly explain why (e.g., it does not tolerate lost packets in its base layers), in case reviewers have it in mind and get confused. Later in Section 2/related work, is it also fair to say when evaluated from the perspective of error resilience, SVC is inferior to state-of-the-art post-processing error concealment approaches? It also needs to sacrifice compression efficiency to produce enhancement layers
% (so the starting point of Figure 1(b) is inaccurate).
% Anyway, removing SVC will make this paragraph logically easier to understand: there are ``forward'' approaches and ``post-processing'' approaches, but Grace jointly optimizes both or you can say Grace takes an unprecedented approach.}}


\begin{figure}[t]
\centering
\includegraphics[width=0.7\columnwidth]{intro-illustration.pdf}
\caption{Illustration of the video quality attained by
different loss-resilient schemes under varying packet loss rates. 
In comparison to forward error correction (FEC) and post-processing
error concealment, \name demonstrates a  more gradual and graceful 
degradation of quality as the loss rate escalates.
(The actual measured performance is presented in \S\ref{sec:eval}.)} 
\label{fig:intro-example}
\end{figure}

%\caption{Illustration existing loss-resilient schemes vs. this work at the same bitrate but under different packet loss rates. 
% \name's data-scalable coding under packet loss of different \rates when compared with existing loss-resilient schemes. 
%(actual figures from our evaluation appear
%later (e.g., Figures~\ref{fig:loss_by_bitrate}). 
% \yc{just put a note here, should we add SVC in this graph? I like it but we may need to change some text?}
%\passed{\fyy{Similarly, SVC should be removed from Figure 1; otherwise, there's too much to parse. Then, one figure with three curves would suffice. Besides, DMR is not defined yet. Can you actually get rid of that and just say packet loss rate?}}
%}

%\begin{figure}[t!]
%    \centering
%%        \includegraphics[width=0.9\linewidth]{figs/intro-example-illustrative-short.pdf}
%        \includegraphics[width=0.99\linewidth]{figs/intro-example-illustrative-separate.pdf}
%         \tightcaption{Illustration existing loss-resilient schemes vs. this work at the same bitrate but under different packet loss rates. 
%%         \name's data-scalable coding under packet loss of different \rates when compared with existing loss-resilient schemes. 
%         (actual figures from our evaluation appear
%later (e.g., Figures~\ref{fig:loss_by_bitrate}). 
%\fyy{Similarly, SVC should be removed from Figure 1; otherwise, there's too much to parse.
%Then, one figure with three curves would suffice.
%Besides, DMR is not defined yet. Can you actually get rid of
%that and just say packet loss rate?}}
%    \label{fig:intro-example}
%    % \vspace{-0.5cm}
%\end{figure}

%\begin{figure}[t!]
%    \centering
%        \includegraphics[width=0.99\linewidth]{figs/intro-example-illustrative-old.pdf}
%         \tightcaption{(a) An example of \name's loss resilience under packet loss of different \rates, and (b) the potential quality/delay improvement by \name. These figures are illustrative; actual figures from our evaluation and trace analysis appear
%later (e.g., Figures~\ref{fig:normal-simulation}, \ref{fig:queue15-simulation}, \ref{fig:loss_by_bitrate}). }
%    \label{fig:intro-example}
%    % \vspace{-0.5cm}
%\end{figure}

% for high-quality, smooth real-time videos.

In this paper, we present \name, a new approach that {\em jointly trains a pair of neural-net (NN) encoder and NN decoder to optimize quality under a variety of packet loss rates}. 
Our insight is that by training the NN encoder and decoder under different rates of simulated packet loss (explained shortly), the resulting NN encoder and decoder forms a {\em generative autoencoder} with the following property: %that tolerates the packet loss while only marginally sacrificing the quality when there is no packet loss.
{\em (i)} With the same encoding (regardless of the packet loss rate), \name obtains quality similar to the classic codec (H.265) used in WebRTC without FEC when there is no packet loss, and {\em (ii)} as the packet loss rate raises, the quality gradually degrades but is still better than state-of-the-art loss-resilient schemes.
%In other words, \name's video quality degrade gracefully with more packet loss while only marginally sacrificing the quality when there is no packet loss. 
%training the autoencoder under various packet loss rates, the decoded video quality can {\em degrade gracefully with more packet loss while only marginally sacrificing the quality in absence of packet loss}. 
\passed{\amz{I find the phrase "in absence of packet loss" difficult to parse, and it's used often in the intro. Can you replace at least a few instances with "when there is no packet loss"?}}
We refer to it as {\em Data-Scalable} (DS) coding. 
Figure~\ref{fig:intro-example} illustrates the contrast between DS coding, encoder-based forward error correction, and decoder-based post-processing error concealment.
% \yc{should we put svc here if it's in figure 1?}
More specifically, DS coding has four practical benefits:
{\em (i)} it does not need to know the loss rate before encoding each frame, 
{\em (ii)} a frame is decodable under {\em any} packet loss rate, unless all packets are lost, 
{\em (iii)} quality gradually improves if more packets are received\footnote{Scalable video coding (SVC)~\cite{SVCFEC1} and fine granularity scalability (FGS)~\cite{ma2022deepfgs,li2001overview} in theory could also improve quality with more packets. 
However, they split a video into a hierarchy of layers, 
%and packet loss at a lower layer can block the decoding of higher layers. Thus, 
so unlike DS coding, a new packet may not always improve quality, if the lower layers are not fully received.}, and
{\em (iv)} when all packets are received, it reaches a quality similar to the traditional codec like H.265 used in WebRTC.
\passed{\amz{Item (iii) is confusingly written -- if I understood correctly after reading the footnote, "quality gradually improves as more packets are received" or "quality scales gradually as more packets are received" will be more clear.}}

%More specifically, \name encodes and decode each frame 
%%We present \name, a concrete example of this approach that encodes and decodes video frames 
%using a {\em novel antoencoder} whose encoder and decoder are neural nets (NNs).
To add packet loss in the training of its generative autoencoder, \name simulates packet loss as follows.
%jointly train the NN encoder and NN decoder under various loss rates, 
%\name simulates packet loss as follows. 
Different from traditional video codec that splits the entropy-encoded byte stream into multiple packets, \name uses a new packetization scheme that first {\em partitions} the encoder's output tensor and then {\em entropy encodes} each partition as a {\em separate} packet. 
If all packets are received, the decoder's input will be identical to the encoder's output.
If a packet is lost, the values in its partition are set to zeros (\ie {\em masked}) in the decoder's input.
During training, given a packet loss rate, \name simulates such process to zeroing out elements corresponding to the lost packets.
%By training under different rates of simulated packet loss, 
%By simulating the effect of packet loss on decoder's input, \name jointly trains the encoder and decoder NNs to optimize the decoded video quality under various rates of packet loss. 
\S\ref{sec:core} shows more details of our training process and packetization process. 
\yc{revisit this paragraph, it's not really talking about how to "simulate" the packet loss. Maybe change the first sentence?}


Once its generative autoencoder is trained, \name entails several optimizations to stream video online efficiently (\S\ref{sec:delivery}).
%entails several optimizations to stream video efficiently online (\S\ref{sec:delivery}).
%For instance, \name minimizes the size inflation caused by the design choice of entropy encoding each packet separately (rather than entropy encode the entire encoder's output). 
For instance, in order to encode each frame at a given target bitrate, \name trains multiple pre-trained 
% \yc{the word "pre-trained" is a bit confusing here, are we saying we are not doing online training?} 
encoders that produce different encoded bitrates but share most computation, so with minimum compute overhead, \name can encode a frame at multiple bitrates and then pick a encoded bitrate similar to the target bitrate. 
\name's decoder can decode a partially received frame without any retransmission, and to avoid out-of-sync coding states, \name uses a protocol to re-synchronize the encoder and decoder states. 
%When the receiver decodes a frame of partially received packets, \name uses a protocol to re-synchronize the encoder and decoder states without packet retransmission.
\name also entails optimizations to run the NN encoder and decoder on CPUs and reduce the size inflation due to per-packet entropy encoding. 

%\name's per-packet entropy encoding
\passed{\amz{This sentence is confusing, since the entropy encoding scheme is not mentioned before, so I had no context for the size inflation. Flipping the sentence ("\name entropy encodes each packet separately, so we optimized the design to minimize potential size inflation" would read easier.}}
%\name also uses a customized protocol to re-synchronize the states on the sender when the receiver decodes a frame without waiting for all packets to arrive.
%\S\ref{sec:delivery} details other optimizations, such as a way to drastically reduce autoencoder overhead (on GPUs and CPUs) and efficient bitrate control to fit the encoding bitrate to target sending rate set by congestion control.
%To make \name practical, \name also includes schemes to 
%speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{subsec:fast-coding}).








\tempstrike{
\mypara{Data-scalable (DS) coding}
We define the {\em Data Missing Rate} (\rate) of a frame as the fraction of packets not received before the  receiver decodes the frame\footnote{\rate is similar to packet loss rate defined on a single frame.}, \eg every 50ms at 20 frames per second (fps).
A packet can be missing due to packet drops, queuing delay or out-of-order delivery, and the missing packets can be consecutive or random.
{\em Without} knowing the actual \rate, an ideal loss-resilient coding scheme should encode a frame  such that
%Then {\em without} knowing the actual \rate, an ideal loss-resilient scheme should meet three criteria: 
\begin{packeditemize}
\item {\em (i)} the frame is decodable under any \rate below 100\% (\ie at least one packet is received), 
\item {\em (ii)} the quality is close to a non-loss-resilient codec (\eg H.265) when all packets are received, and
%as long as {\em any} (non-empty) subset of packets of the frame is received, 
%(\ie no need for retransmission unless all data is lost);  
\item {\em (iii)} quality degrades gracefully with higher \rate, \ie quality gradually improves if {\em any} more packets are received.
\end{packeditemize}
We call such a coding scheme {\em data-scalable} (DS).
DS coding is ideal for real-time video, because without retransmission, its quality degrades gracefully with more packet loss (higher \rate) while not sacrificing quality in absence of packet loss. 
}





\tempstrike{
Some loss-resilient scheme uses an older but reliably received frame as the reference frame, allowing the decoder to safely skip a loss-affected frame (\eg~\cite{salsify}).
%without hurting future frames, 
However, using an old reference frame means more bits to achieve the same quality as using the last frame as reference, which lowers compression efficiency.
}


%achieve high {\em compression efficiency}, which means high quality with fewer bits, and {\em loss resilience} under various data missing rate or {\em \rate} defined by
%the fraction of data that is not received, due to packet drops or queuing, before a frame is decoded.

\tempstrike{
Unfortunately, current real-time video systems achieve loss resilience by adding various forms of redundancies, thus sacrificing compression efficiency (as elaborated in \S\ref{subsec:prior}).\footnote{
Scalable video coding (SVC~\cite{SVCFEC1}, FGS~\cite{ma2022deepfgs,li2001overview}, Swift~\cite{swift}), which works well for on-demand streaming videos, will be much less effective in real-time videos which send packets of a frame together, instead of layer by layer (see \S\ref{subsec:prior}).
For this reason, scalable video coding is not commonly used to improve unicast real-time videos~\cite{salsify}. 
Similarly, selective frame skipping (\eg~\cite{voxel}) might work for on-demand videos, but in real-time videos, most frames are P-frames which cause poor quality once dropped, unless I-frames are frequently inserted.
Nonetheless, we will still evaluate them against \name.}
%\jc{add old reference frame}
}



\tempstrike{
In contrast, an ideal loss-resilient coding should be {\em Data-Scalable} (DS)---{\em its quality should degrade gracefully with higher packet loss rate but without sacrificing the quality in absence of packet loss} (illustrated in Figure~\ref{fig:intro-example}(d)). 
DS coding has several benefits: 
{\em (i)} it does not need to predict loss rate before sending the packets (unlike FEC), 
{\em (ii)} a frame can be decodable under {\em any} loss rate, unless all packets are lost, 
{\em (iii)} quality gradually improves if {\em any} more packets are received (unlike SVC), and
{\em (iv)} when all packets are received, it reaches a quality similar to the traditional codec like H.265 used in WebRTC (unlike error concealment).

This paper presents \name, a new loss-resilient scheme for real-time video, which better approximates DS coding by using an autoencoder (neural encoder and neural decoder) to optimize quality under various packet loss rates.
The key idea is two-fold.
\begin{packeditemize} 
\item \name's {\em a loss-resilient autoencoder} (\S\ref{subsec:training}) consists of a pair of neural encoder and neural decoder {\em jointly trained} to optimize video quality when $x$\% of values in the encoder output of a frame are randomly selected and masked (\ie set to zeros), with $x$\% between 0 to 100\%, before the masked data is fed to the decoder. 
This simulates the effect of random data masking between the encoder and the decoder.
\item \name uses a {\em novel packetization scheme} (\S\ref{subsec:packetization}) to partition the encoder output of a frame and entropy encodes each partition as an independently decodable packet, so that losing any $x$\% packets (which can be consecutive or random) has the same effect on the input of the decoder as masking $x$\% of randomly selected values.
In short, packet loss will appear to have same effect as random data masking between the encoder and the decoder.
\end{packeditemize} 
}

%When put together, the two ideas help \name to optimize quality under various packet loss rates, so it better approximates DS coding than prior schemes.
%
%When no packet is lost, \name's quality is similar to H.265 at the same bitrate, but as loss rate increases, \name's quality degrades much more gracefully than state-of-the-art loss-resilient coding schemes.
%%(Figure~\ref{fig:intro-example}). 
%In short, \name better approximates DS coding than prior schemes when packet loss affects one frame. 
%%when tested under different \rates.



%presents a way to smooth frame size across different frame types (I-frames and P-frames)


%To leverage the new data-scalable (DS) autoencoders, \name also includes a customized video streaming framework to delivery a sequence of frames to synchronize the states on the sender and the receiver when the receiver decodes a frame without waiting for 
%%in a slightly lazy fashion.
%It also includes optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).
%to deliver autoencoder-generated data.
%It uses a new packetization scheme on randomly shuffled \aecode with per-packet entropy encoding, which makes packet loss of $n\%$ \rate appear to have the same effect as $n\%$ random making on the \aecode (\S\ref{subsec:packetization}). 
%\name also uses techniques for DS coding over a sequence of frames, as well as optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).







We have implemented \name and evaluated \name using real network traces and a range of video content genres (all from different data sources than the training set of the autoencoder) and compare it against a range of state-of-the-art variants of different loss resilient schemes, including 
{\em (i)} forward error concealment (Tambur~\cite{rudow2023tambur}), 
{\em (ii)} postprocessing error concealment by neural-net in-painting~\cite{xiang2019generative}, 
{\em (iii)} scalable video coding (Swift~\cite{swift}), and
{\em (iv)} selective frame skipping (Voxel~\cite{voxel} and Salsify~\cite{salsify}).
%å, and {\em (v)} functional codecs (Salsify~\cite{salsify}).
%{\em (i)} FEC (Tambur~\cite{rudow2023tambur}), {\em (ii)} error concealment (neural-net generative in-painting~\cite{xiang2019generative} and selective skipping~\cite{voxel}), {\em (iii)} Scalable Video Coding~\cite{swift}, and {\em (iv)} Salsify's functional codec~\cite{salsify}
% including GCC~\cite{carlucci2016analysis} and Salsify~\cite{salsify} (except that packet retransmission is turned off for loss-resilient decoders).
Our key results are: 
\begin{packeditemize}
  \item \name achieves better quality, by 1.4-4 dB of SSIM\footnote{The definition of SSIM dB is in \S\ref{subsec:eval:setup}}, than other loss-resilient schemes at the same packet loss (between 20\% and 80\%) and bitrate (between 0.8Mbps and 4.8Mbps). 
  \item \name achieves a similar average quality (in SSIM) with the codec used in WebRTC at the same bitrate. In other words, \name does not sacrifice quality when there is no packet loss. %in absence of packet loss.
  \item When different loss-resilient schemes are run on real network traces
  \footnote{To be fair, we run \name and the baselines over the same congestion control (CC) algorithm, GCC~\cite{carlucci2016analysis}, which is the standard CC used in WebRTC.}
  , \name's superior loss resilience leads to 90\% reduced duration of video stalls, 95\% reduced number of non-rendered frames, and 66\% reduced tail frame delay (98$^{th}$ percentile). 
  %\name  reduces the duration of video stalls, number of non-rendered frames, and 98$^{th}$ percentile frame delay by \review{90}\%, \review{95}\%, and \review{66}\% respectively, when compared to the most competitive baselines
  \item With much less video stuttering and fewer skipped frames, our IRB-approved user study confirms that \name has \review{38}\% higher mean opinion score (MOS) than the most competitive loss-resilient schemes.
  \item On a single Nvidia A40 GPU, \name can decode 480p and 720p at 120~fps and 44.1~fps, respectively and encode 480p and 720p at 87.7~fps and 31.2~fps, which is 1.5-5$\times$ faster than recent video autoencoders. On CPUs, it can encode 720{p} videos at 28.5~fps (on par with GPU-based implementation) at only a drop of 0.5 dB in SSIM. \yc{update the numbers to reflect Ziyi's latest results}
\end{packeditemize}
%ratio of delayed frames (defined as the frames whose delay between encoding and decoding is larger than 400~ms) by up-to 4$\times$ and the stall rate (defined as the fraction of inter-frame gaps that exceed 200~ms) by 10$\times$. 
%compared to the most competitive baselines which still have to retransmit packets or skip frames.


To put \name's contribution in perspective, neural video codecs have long been used in multimedia, but \name is, to our best knowledge, the first to jointly train generative NN encoder and decoder to improve loss resilience in real-time video.
\name is closely related to using NNs to generatively reconstruct the missing data in lost packets, but they do not jointly train the encoder for loss resilience (\eg~\cite{sankisa2018video,reparo}) or handle only special content type at low resolution~\cite{reparo}.
\name is also related to but different from an emergent technique~\cite{kurka2020deepjscc,bourtsoulatze2019deep,gunduz2019machine} which trains autoencoders to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss).
%Most work on autoencoders has focused on improving {\em compression efficiency} rather than loss resilience, such as scalable video coding (Swift~\cite{swift} and DeepFGS~\cite{ma2022deepfgs}), super resolution~\cite{gemino,neuroscaler,livenas}.
%Neural networks have been used to reconstruct missing spatial blocks in lost packets (\eg~\cite{sankisa2018video,reparo}, which uses NNs on the decoder side and handles only specific video content (\eg talking head~\cite{reparo}). 
%In contrast, \name jointly trains the encoder and decoder to handle packet loss.
%\name is related to but different from an emergent techniques~\cite{kurka2020deepjscc,bourtsoulatze2019deep,gunduz2019machine} which train autoencoders to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss).

% \passed{\jc{agreed that this is a bit too long. tried to shrink it.}}
% \passed{\amz{I understand including so much comparison to related work to hedge the "first to our knowledge" claim, but it is quite long considering the related work comes so soon after. I would remove everything after the first sentence and put it above the limitations paragraph, or just wrap up all the citations in a "other approaches address compression efficiency, post-processing, or signal noise". }}

While \name improves real-time video quality under packet loss, it has limitations (\S\ref{sec:limit}). 
%\amz{This sentence is awkward, I think you can more generously say "While \name improves quality under packet loss, the approach has limitations."}
First, though our implementation of \name can run much faster than traditional autoencoders,
% and achieves lower delay than alternative solutions 
\name cannot run in real-time on resource-constraint devices yet. 
%\amz{Fast enough for what, real-time? }
Second, we focus on unicast video communication, rather than problems in multi-party conferencing (\eg stream forwarding). 
% Third, \name cannot improve the video quality when all packets are lost. 
%\amz{Cannot improve what? }
%\jc{mention that packet loss is often not 100\% given audio still continues}
%While \name decides {\em what} each packet contains, 
Our main goal is to show the potential of training generative autoencoders under different loss rates, and we expect it will spark more efforts to tackle these limitations.


\tempstrike{
% \ie no data loss between the encoder and the decoder, so they need to combined with a loss-resilient scheme.
For instance, Swift~\cite{swift} and DeepFGS~\cite{ma2022deepfgs} use NN codecs to improve scalable video coding (rather than loss tolerance) for on-demand (rather than real-time) videos. 
Super-resolution (SR)~\cite{gemino,neuralscaler} enhances the decoded video quality at the receiver when the available bandwidth is low
DeepJSCC uses an autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss)~\cite{kurka2020deepjscc}.
\name also differs from neural super-resolution models~\cite{neuroscaler,livenas} and generative neural error concealment~\cite{sankisa2018video, reparo} which only trains NNs on the receiver and handles only specific video content (\eg talking head~\cite{reparo}), whereas \name jointly trains the encoder and decoder to handle packet loss.


, and {\em (v)} super resolution (SR)~\cite{??}.\footnote{\editSOCC{The main use case of SR is to enhance the decoded video quality at the receiver when the available bandwidth is low. Such technique should work for any kind of video codecs. Therefore, SR is orthogonal to \name.}} %\jc{explain SR is orthogonal}

}

%There are two key findings (an example of which is given in Figure~\ref{fig:intro-example}). 
%First, when no packets are lost, \name's quality does not exceed H.265 at the same bitrate, but in presence of more packet loss, \name's quality degrades much more gracefully than other loss-resilient coding schemes.
%Second, we use packet-level simulation driven by real-world bandwidth traces and run \name and the baseline loss-resilient coding schemes. % on the same CC logic (retransmits disabled).
%We show that compared to the baselines, \name reduces the ratio of delayed frames (defined as the frames whose delay between encoding and decoding is larger than 400~ms) by up-to 4$\times$ and the stall rate (defined as the fraction of inter-frame gaps that exceed 200~ms) by 10$\times$. 
%%compared to the most competitive baselines which still have to retransmit packets or skip frames.
%With much less video stuttering and fewer skipped frames, our user study confirms that \name has higher average subjective ratings by users than the baselines.
%
%Second, \name borrows existing congestion control (CC) logics {\em without} packet retransmits unless all packets of a frame are lost), such as GCC~\cite{carlucci2016analysis}, which decides the target frame size and how fast to send the \name-encoded packets.


%\textbf{This work does not raise any ethical issues.}



%Though autoencoders have a long history in multimedia, standard autoencoders have focused on better compression efficiency (achieving higher quality in fewer bits) and are not inherently loss-resilient.
%This is because, in traditional autoencoder training, the decoder always receives the {\em same} \aecode produced by the encoder, which does not prepare the autoencoders to handle any data loss during transmission. 
%
%To put it in context, neural encoders and decoders have long been used in multimedia (see \S\ref{sec:related}) but \name is, to our best knowledge, the first to demonstrate the potential of autoencoders to improve loss resilience in real-time video.
%Swift and DeepFGS, for instance, use autoencoders to improve scalable video coding (rather than loss tolerance) for on-demand (rather than real-time) videos~\cite{swift, ma2022deepfgs}. 
%DeepJSCC uses an autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises (rather than packet loss)~\cite{kurka2020deepjscc}.
%\name also differs from neural error concealment~\cite{sankisa2018video} which only uses NNs on the receiver, whereas \name jointly trains the encoder and decoder to handle packet loss.


\tempstrike{


Autoencoders work like a standard video codec but replace part of the encoder and decoder with neural networks (NNs). 
Though autoencoders have a long history in multimedia, standard autoencoders have focused on better compression efficiency (achieving higher quality in fewer bits) and are not inherently loss-resilient.
This is because, in traditional autoencoder training, the decoder always receives the {\em same} \aecode produced by the encoder, which does not prepare the autoencoders to handle any data loss during transmission. 



This paper presents \name, a new approach to loss-resilient real-time video, by customizing {\em  autoencoders}. 
%This paper presents \name, a new end-to-end loss-resilient real-time video streaming system, by customizing {\em  autoencoders} following the idea proposed in~\cite{cheng2022grace}. 

In \name, we show that autoencoder-based video streaming can be loss-resilient by customizing the autoencoder training process (\S\ref{sec:core}) and video streaming framework (\S\ref{sec:delivery}).

In \name's autoencoder training process (\S\ref{subsec:training}), when the NN encoder returns a \aecode, we randomly mask n\% of its elements to zeros before feeding it to the NN decoder, a process we call {\em random masking}. We vary the rate of random masking ($n\%$) between [0\%, 100\%), which as explained shortly, simulates the effect of packet loss under different \rates.
% As explained shortly, varying the rate of random masking (n%n\%) between [0\%, 100\%) simulates the effect of packet loss under different \rates.
Consequently, our trained autoencoder, {\em without} knowing the actual \rate, can encode a frame such that it can: {\em (i)} decode a frame as long as {\em any} (non-empty) subset of packets of the frame is received;
%(\ie no need for retransmission unless all data is lost);  
{\em (ii)} achieve better quality with the addition of each new packet (\ie graceful degradation with higher \rate); and
{\em (iii)} reach a quality close to a non-loss-resilient coding algorithm (such as H.265) when all packets are received.
We refer to it as {\em Data-Scalable} ({\em DS}) video coding.
In contrast, FEC is not DS coding, since its quality does not improve with more data if the \rate is below a threshold but the quality drops abruptly (due to retransmits) once the \rate exceeds the threshold.

}

% Our prior work of data-scalable (DS) autoencoders~\cite{cheng2022grace} suffers from multiple problems: {\em (i)} naive entropy encoding lowers compression efficiency, {\em (ii)} encoding speed insufficiently fast (<20fps) for real-time video streaming requirements, and {\em (iii)} additional quality degradation due to error propagation from packet losses.
% %To leverage the new data-scalable (DS) autoencoders, 
% To address the above challenges, \name uses a customized video streaming framework to deliver autoencoder-generated data.
% It uses a new packetization scheme with per-packet entropy encoding, which makes packet loss of $n\%$ \rate appear to have the same effect as $n\%$ random making on the \aecode (\S\ref{subsec:packetization}) with negligible size overhead. 
% \name also uses techniques for DS coding over a sequence of frames to minimize the propagation of error, as well as optimizations to speed up autoencoder coding (on GPUs and CPUs) and efficient bitrate control to allow for dynamic video quality depending on available bandwidth (\S\ref{sec:delivery}).


\begin{comment}

It uses a novel packetization scheme that makes packet loss of n%n\% appear to have the same effect as n%n\% random making on the \aecode (see \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{subsec:packetization} for details). 
%Standard autoencoders entropy encode the NN encoder output (\aecode) and packetize the resulting bitstream, so any packet loss will render it undecodable by the receiver.
The basic idea is to randomly split the \aecode's elements to partitions, each separately entropy-encoded as an independently decodable packet, and if n%n\% packets are lost, we set their elements in the \aecode to zeros, which mimics random masking.
However, this naive scheme greatly increases the size of the compressed data, due to the additional space needed to store the symbol distribution (used by entropy-decoding) in each packet.
\name addresses this challenge by carefully coarsening the granularity of symbol distributions, which significantly reduces size increase while maintaining the compression efficiency of entropy coding. 

\end{comment}





\begin{comment}

Ideally, the quality should degrade gracefully with more packet loss (higher \rate), without compromising the quality in absence of packet loss.
Specifically, it should be able to 
{\em (i)} decode a frame as long as {\em any} (non-empty) subset of packets of the frame is received;
%(\ie no need for retransmission unless all data is lost);  
{\em (ii)} achieve better quality with the addition of each new packet (\ie lower \rate); and
{\em (iii)}  reach a quality close to a non-loss-resilient coding algorithm (such as H.265), when all packets are received.
We refer to it as {\em Data-Scalable} ({\em DS}) video coding.
FEC is not DS coding, since its quality does not improve with more data if the packet loss rate is below a threshold but the quality drops abruptly once loss rate exceeds the threshold.


\mypara{Data-scalable autoencoder}
This paper introduces {\em \name}, a real-time video system that, for the first time, uses {\em  autoencoders (AEs)} to realize data-scalable (DS) video delivery.
%which explores a new approach to DS video delivery by using {\em neural-net (NN) autoencoders}.
At a high level, autoencoders work like a standard video codec but replace some coding logic with neural networks (NNs). 
It uses an NN encoder to encode a frame to a {\em \aecode} (without entropy encoding), and an NN decoder to decode to a reconstructed frame that is similar to the original frame. 


We choose autoencoders, not because the off-the-shelf models are inherently data-scalable (DS), but due to their unique properties that {\em could} enable DS coding. 
%\name is a particular design that harnesses these properties to enable DS coding.
Specifically, the NN decoder can reconstruct a decent-quality frame, even if we {\em randomly erase} (\ie set to zeroes) a subset of $n\%$ elements in the \aecode (the output of the NN encoder).
In other words, {\em random data erasure} on the \aecode has a limited impact on the decoding quality of autoencoders. 
This can be attributed to the lack of stringent dependencies among the elements in a \aecode\footnote{
%Mathematically, this smoothness is a result of NN encoders and decoders having continuous derivatives everywhere. Moreover, 
This can also be intuitively understood that NN decoders share the architecture of {\em generative} NNs, such as variational autoencoder (VAE), which can create realistic-looking images from random inputs.}, unlike SVC where the decoding of a layer depends on the lower layers.


Despite the promise of autoencoders, several practical challenges remain.
%\name addresses several practical challenges.
Two of them will be highlighted here.

%Despite the promise of autoencoders, \name must address several practical challenges, such as improving quality under various \rates, making entropy encoding of \aecodes loss-resilient, controlling bitrate, and speeding up autoencoder coding. 
%Two of them will be highlighted here.


%\mypara{Adding packet loss in autoencoder training}
\mypara{Training autoencoder with packet loss}
First, the quality of standard autoencoders drops quite significantly if more data is erased from the \aecode. 
This is because the standard autoencoder training, in which  the decoder always sees the same \aecode returned by the encoder, never prepares the autoencoder to handle any data loss between the encoder and the decoder. 
\name trains autoencoders different (see \S\ref{??} for details).
It applies random data erasures to the \aecode (which could simulate the effect of packet loss as explained shortly), and by varying the rate of data erasure between [0\%, 100\%), 
%In other words, by training the NN encoder and NN decoder jointly, 
the new autoencoders not only learn how to compress high-quality frames efficiently but also to be robust to different rates of random data erasures. 

%, which simulates the effects of packet loss under different \rates (which will be explained shortly).






\mypara{Per-packet entropy coding for autoencoder}
Standard autoencoders use entropy encoding to losslessly compress a \aecode to a single bitstream and then packetize it, so any packet loss will render it undecodable.
%entropy coding used in current autoencoders cannot tolerate any packet loss. 
A naive idea is to randomly 
split the \aecode's elements to partitions,
%split a \aecode to sub-tensors, 
each separately entropy-encoded as an independently decodable packet, and if $n\%$ packets are lost, we set their elements in the \aecode to zeros, which resembles random erasure.
%effectively erases a random subset of $n\%$ elements.
%is the same as 
%random data erasure.
However, this naive per-packet entropy coding greatly increases the size of the compressed data, due to the additional space needed to store the symbol distribution (used by entropy-decoding) in each packet.
%To mitigate the size increase, 
\name carefully coarsens the granularity of symbol distributions, which significantly reduces size increase while maintaining the compression efficiency of entropy coding (see \S\ref{??} for details). 




Besides achieving loss resilience on a single frame, \name uses a novel frame delivery system to approximate DS coding over a sequence of frames, speed up autoencoder coding (on GPUs and CPUs), and enable efficient bitrate control (\S\ref{??}).




\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/fig1-example.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/fig1-example-osdi.pdf}
        \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/fig1.png}
         \caption{graceful degradation}
         \label{fig:normal-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
         \caption{delay quality tradeoff}
         \label{fig:normal-ssim-delay}
     \end{subfigure}
         \label{fig:}
         \tightcaption{Example results of \name's (a) more graceful degradation in presence of packet loss than prior solutions, and (b) better tradeoffs between video quality and tail frame delay, which corroborates the subjective rating of users.
         More results can be found in \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{sec:eval}. 
%         \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
    \jc{TODO: add a horizontal line to indicate the quality of H.265}
    \textcolor{red}{Yihua: TODO: update real values (fig1data.xlsx)}
         }
    \label{fig:intro-example}
\end{figure}

\end{comment}






%including a custom streaming protocol
%controlling bitrate, and speeding up autoencoder coding. 


%, so that even if the selected bitrate overshoots the bandwidth, we can still obtain decent quality.


%Being a coding system, \name can work with existing congestion control (CC) logics---CC decides how fast to send packets, and \name decides {\em what} each packet contains.




%Much remains unknown about the limits of autoencoders as a loss-resilient coding layer.

%To our best knowledge, \name is the first end-to-end autoencoder-based video system for loss-resilient real-time videos.
%that achieves stream real-time videos in a data-scalable fashion. 



%arising from training and using autoencoders in real-time video communication.

%Many aspects of \name are also inspired by prior work. 
%That said, \name, to our best knowledge, is the first to develop custom autoencoders that realize data-scalable video delivery.

%\name aims at unicast video sessions, rather than multi-party conferences. 
%It is also important that \name's autoencoders do {\em not} achieve better compression efficiency than recent heavily engineered video codecs, such as H.265. 
%Indeed, \name's video quality is still slightly lower than H.265 at the same bitrate. 








==> sections/old/intro_v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\section{Introduction}

Real-time video traffic is now on par with traditional streaming videos, with applications ranging from video conferencing to emerging IoT services and cloud-based gaming~\cite{see refs from hotnets}.
Video in Chrome over WebRTC grew 100x during 2020~\cite{??}, and one global industry survey found that services based on real-time videos grew from less than 5\% to over 28\% between 2020 and 2021~\cite{\url{https://www.wowza.com/wp-content/uploads/Streaming-Video-Latency-Report-Interactive-2020.pdf},??}.
% https://f.hubspotusercontent20.net/hubfs/229276/2021%20Low%20Latency%20Report/streaming-video-latency-report-interactive-2021.pdf

With the unprecedented proliferation of real-time video, we see an emerging need for the ability to render a frame with {\em high quality} as soon as {\em any} non-empty subset of its packets is received.
The flexibility for clients to {\em balance frame-level delay and rendering quality} is particularly useful under {\em long RTT} (\eg long enough to render retransmission ineffective), and {\em intermittent} packet drops, delays or reordering, caused by bursty cross-traffic and natural variation of encoded frame sizes.\footnote{This problem so profound and urgent that serious efforts are finally being made by ISPs to offer active queue management for real-time traffic~\cite{l4s}, marking  a shift in focus from bandwidth to tail delay~\cite{report}, but wide deployment is still a long way off. Our proposed solution is complementary to this trend and can benefit from it once deployed (see \S\ref{??}).}

\jc{mention the need for high frame rate, i.e., can't skip frames!}


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
         \label{fig:}
    \caption{}
    \label{fig:intro-example}
\end{figure}

Unfortunately, current loss-resilient schemes fall short of this expectation, especially in links with long propagation RTTs and high packet jitters (\eg transient congestion and packet drops). 
For instance, FEC, the loss-resilient method ubiquitously used in WebRTC, requires a certain fraction of packets be reliably received before a frame is decodable. 
Moreover, to tolerate a higher fraction of packets being missed when decoding, more redundancy must be added {\em before} packets transmission. 
Setting an appropriate level of redundancy is, however, well-known to be hard under high packet jitters~\cite{??}---too much redundancy causes underutilization of bandwidth (\ie low video quality if all packets arrive on time), while too little redundancy forces the receiver to wait for (or resend) more packets. 
Figure~\ref{fig:intro-example} illustrates this tradeoff: the same coding cannot achieve high quality under both no packet loss and high fraction of packet loss.
Like FEC, other schemes (\eg SVC, intra-MB insertion) also must reliably deliver at least certain number of packets and add redundancy that sacrifices video quality if no packets are delayed/lost (\S\ref{??}).




We argue that a better video codec should be {\em data scalable}, which entails three requirements: 
(1) the coding of a video frame only depends on target bitrate (not predicted loss rate), 
(2) the frame is decodable once {\em any} non-empty subset of its packets are received and the decoded quality improves with more packets received, and 
(3) for any x\%, the decoded quality with x\% arrived packets is close to the classic codec (like H.265) with x\% FEC redundancy.\footnote{At first glance, this may sound like scalable video coding (SVC), whose quality ideally is proportional to throughput. Unfortunately, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets and a missing packet may disproportionally render multiple quality layers undecodable. 
In practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).}
In contrast to existing codec (including loss-resilient ones), a data-salable codec eschews the need for the sender to inject redundancy based on predicted packet jitter/losses and allows the receiver to flexibly choose when to decode a frame once one of its packets arrives while still enjoying decent video quality.


\begin{comment}

Unlike FEC which sets redundancy rate {\em before} sending data out, our goal is to encode a frame in a \rate-agnostic way and decode the frame under any \rate (less than 100\%) at a similar quality as current FEC-based coding {\em if} it knew \rate. 
In other words, 
(1) under zero \rate, the decoded video quality should be close to that of existing video coding without FEC redundancy, and 
(2) the decoded video quality should degrade gracefully with higher \rate, with a similar quality as FEC-based coding if FEC knows the \rate. 
% So without knowing \rate, it should achieve similar quality as existing real-time video systems when they know \rate. 
In short, the envisioned real-time video system eschews the need for \rate prediction.

\end{comment}


Achieving data-scalable coding is clearly a daunting task, but this paper demonstrates that it is possible. 
We explore a new approach to data-scalable codec, by borrowing and customizing the emergent deep autoencoders, a class of neural-network coder/decoders that compress multimedia data (videos and images) highly efficiently. 
Though existing autoencoders do not tolerate loss, we show that by letting them ``experience'' different rates of packet loss during training, we can create {\em data-scalable autoencoders} learn not only how to code video pixels efficiently but also how to code them in a way that is resilient to missing packets.
% Training in itself is not straightforward, since packet losses are not naturally differentiable.
While the idea of data-scalable autoencoder is arguably simple, its performance gain is quite remarkable. 
Figure~\ref{fig:intro-example} contrasts the performance of an example data-scalable autoencoder with prior loss-resilient schemes. 

Our goal is {\em not} merely showing that data-scalable autoencoders are possible. 
Instead, our main contribution is to explore key questions regarding {\em how to develop and use data-scalable autoencoders in real-time video systems} in the context of \name, a concrete system based on data-scalable autoencoders. 
These questions include
why an autoencoder could be resilient to packet losses, 
how to best incorporate packet losses in autoencoder training (given packet loss is not naturally differentiable), and
how well an autoencoder fares in unseen content {\em and} unseen \rates. 
Moreover, since the video codec is tightly connected to other components in a real-time video system, data-scalable autoencoders bring up unique design questions, such as 
how a streaming protocol designed for data-scalable autoencoders should look like (including packetization, packet scheduling, reference frame selection), and how much compute/storage overheads autoencoders would add to WebRTC and how to mitigate them. 

% This begs several immediate and critical questions.

% Instead, we try to answer these technical questions in the context of \name, a concrete system based on data-scalable autoencoders. 


% To best utilize data-scalable autoencoders in practice, they should also be  video streaming system. 


Though the concept of autoencoders has been used in video streaming~\cite{??} and image compression in wireless communication~\cite{??}, to our best knowledge, these questions have not been systematically studied.
For instance, \fillme \jc{pick one or two exciting technical contributions}



Our evaluation shows \jc{eval highlights}

\jc{outline the roadmap and highlight the contribution again}

\jc{need a forward pointer to 2.2 (caveats of autoencoders)}




==> sections/old/intro_v3.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\section{Introduction}

Real-time video traffic is on par with traditional streaming videos. 
With applications ranging from video conferencing to emerging IoT services and cloud-based gaming~\cite{see refs from hotnets}, video in Chrome over WebRTC grew 100x during 2020~\cite{??}, and one global industry survey found that services based on real-time videos grew from less than 5\% to over 28\% between 2020 and 2021~\cite{\url{https://www.wowza.com/wp-content/uploads/Streaming-Video-Latency-Report-Interactive-2020.pdf},??}.
% https://f.hubspotusercontent20.net/hubfs/229276/2021%20Low%20Latency%20Report/streaming-video-latency-report-interactive-2021.pdf

With the unprecedented proliferation, real-time video applications are expected to operate in not only low-RTT and largely stable networks, but over connections with {\em long RTT} (which renders retransmission ineffective) or {\em high packet jitters} and {\em intermittent losses} (which makes accurate rate adaptation difficult).\footnote{This problem so profound and urgent that serious efforts are finally being made by ISPs to offer active queue management for real-time traffic~\cite{l4s}, marking  a shift in focus from bandwidth to tail delay~\cite{report}, but wide deployment is still a long way off. Our proposed solution is complementary to this trend and can benefit from it once deployed (see \S\ref{??}).}
For instance, retransmitting a packet along a path with 100ms RTT will delay or skip at least three frames in a 25fps video stream (a new frame every 40ms).
Prior measurements have confirmed that such long RTT is common in video conferencing and that high packet jitters and losses are not rare, due to various reasons such as bursty cross-traffic, packet reordering, and variation of encoded frame sizes.\jc{the last sentence should be replaced with numbers cited from recent papers}

%\jc{mention the need for high frame rate, i.e., can't skip frames!}


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        \includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss.pdf}
         \label{fig:}
    \caption{Loss resilience comparison among different schemes. The encoding bitrate is set at \fillme Mbps. 
    More results can be found in \S\ref{sec:eval}.\jc{YIHUA, remember to add a line of 264 without loss.}}
    \label{fig:intro-example}
\end{figure}

Thus, to flexibly trade between video quality and video delay (without skipping frames), a client should ideally be able to decode the next frame when {\em any} non-empty subset of its packets is received and still obtain decent quality given the amount of data received. 
Unfortunately, existing loss-resilient schemes fall short of this expectation.
%, especially in links with long propagation RTTs and high packet jitters (\eg transient congestion and packet drops). 
For instance, Forward Error Correction (FEC) is ubiquitously used in WebRTC, and it requires a certain fraction of packets be reliably received before a frame is decodable. 
To tolerate a higher fraction of packets being missed when decoding, more redundancy must be added {\em before} packets transmission. 
Thus, choosing an appropriate level of redundancy is known to be difficult under high packet jitters~\cite{??}.
As illustrated in Figure~\ref{fig:intro-example}, too much redundancy would underutilize bandwidth (\ie low video quality if all packets arrive on time), while too little redundancy would drive the receiver to wait for (or resend) more packets. 
In short, the same coding cannot achieve high quality under both no packet loss and high fraction of packet loss.
As elaborated in \S\ref{??}, other schemes (\eg SVC, inter-MB insertion) also must deliver at least certain number of packets for a frame to be decodable, and/or pad video data with non-trivial redundancy in anticipation of certain packet loss rate, which hurts video quality if no packets turn out lost.

To address these limitations, we advocate for a new abstraction, referred to as {\em data-scalable} video delivery, which entails two requirements: 
(1) the coding of a video frame does not depend on an anticipated loss rate, 
(2) a frame is decodable once {\em any} non-empty subset of its packets are received and the decoded quality improves with more packets received.\footnote{At first glance, this may sound like scalable video coding (SVC), whose quality increase with throughput. However, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets and a missing packet may disproportionally render multiple quality layers undecodable. In practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).}
In other words, the decoded video quality, under no packet losses, should be similar to a classic codecs (\eg H.264, H.265) and degrade {\em gracefully} with more lost packets. 
In essence, the abstraction of data-salable video delivery eschews the need for the sender to inject redundancy based on predicted packet losses and instead allows the receiver to flexibly choose when to decode a frame once any its packets have arrived while enjoying decent video quality.


\begin{comment}

Unlike FEC which sets redundancy rate {\em before} sending data out, our goal is to encode a frame in a \rate-agnostic way and decode the frame under any \rate (less than 100\%) at a similar quality as current FEC-based coding {\em if} it knew \rate. 
In other words, 
(1) under zero \rate, the decoded video quality should be close to that of existing video coding without FEC redundancy, and 
(2) the decoded video quality should degrade gracefully with higher \rate, with a similar quality as FEC-based coding if FEC knows the \rate. 
% So without knowing \rate, it should achieve similar quality as existing real-time video systems when they know \rate. 
In short, the envisioned real-time video system eschews the need for \rate prediction.

\end{comment}


%While data-scalable coding might be possible with existing codecs, we
We explore a new approach to data-scalable coding, by borrowing and customizing the emergent neural-net autoencoders, a class of neural-network coder/decoders for multimedia data (videos and images). 
Existing autoencoders are developed with compression efficiency as the objective, but we show that by injecting emulated packet losses during autoencoder training, we can create a {\em data-scalable autoencoders}, that learn not only how to code video pixels efficiently but also how to code them in a way that is resilient to missing packets.
% Training in itself is not straightforward, since packet losses are not naturally differentiable.
%While the idea of data-scalable autoencoder is arguably simple, its performance gain is quite remarkable. 
The resulting autoencoder, though slightly less efficient at compressing videos under no packet losses than classic heavily engineered codecs, can meet the two criteria of data-scalable coding. 
Figure~\ref{fig:intro-example} shows an example result: the decoded quality at x\% packet losses should be close to that of H.264 or H.265 with x\% FEC redundancy, which can be viewed as a reference design that optimizes compression efficiency, not loss resilience.

Besides the possibility of data-scalable autoencoders, we also present the design and implementation of \name, a concrete real-time video system.
\name tackles two high-level challenges. 

First, how to train a data-scalable autoencoder to tolerate various unseen packet loss rates. 
This challenge entails several subquestions: 
how packet losses should be emulated as part of model training given that the impact of packet loss on coded data is non-differentiable, 
what packet losses should be revealed to the autoencoder during training, 
and why our autoencoder is more resilient to data losses than existing schemes.

Second, how to realize data-scalable delivery over data generated by the data-scalable autoencoder. 
This involves several design questions such as how a streaming protocol designed for data-scalable autoencoders should look like (including packetization, packet scheduling, reference frame selection), and how much compute/storage overheads autoencoders would add to WebRTC and how to mitigate them. 
Moreover, since use of autoencoders in real-time video delivery is relatively new, we also examine various strategies for bitrate adaptation and key frame insertion in the context of \name.

No individual component of \name is particularly intricate, and some are inspired by prior work. 
However, the contribution of \name lies in an end-to-end real-time video delivery framework, which tackles various challenges arising from training data-scalable autoencoder and delivering autoenocer output data.


%\jc{there's some concerns regarding autoencoders. these questions are answered for the first time}

%how to best emulate packet losses during training so that the resulting autoencoder can handle and
%how well an autoencoder fares in unseen content {\em and} unseen \rates. 
%Moreover, since the video codec is tightly connected to other components in a real-time video system, data-scalable autoencoders bring up unique design questions, such as 
%how a streaming protocol designed for data-scalable autoencoders should look like (including packetization, packet scheduling, reference frame selection), and how much compute/storage overheads autoencoders would add to WebRTC and how to mitigate them. 

% This begs several immediate and critical questions.

% Instead, we try to answer these technical questions in the context of \name, a concrete system based on data-scalable autoencoders. 


% To best utilize data-scalable autoencoders in practice, they should also be  video streaming system. 


Admittedly, we are not the first to use autoencoders in video compression. 
Applications of autoencoders can be found in wireless and data communication to compress images, video files, and signals~\cite{??}, and notably a recent work uses custom autoencoders to obtain highly efficient scalable video coding (SVC). 
However, to our best knowledge, \name is the first to use custom autoencoders to realize data-scalable video delivery.



Our evaluation shows \jc{eval highlights}

\jc{outline the roadmap and highlight the contribution again}

\jc{need a forward pointer to 2.2 (caveats of autoencoders)}

\jc{
\begin{itemize}
    \item content generalization
    \item clarify the use cases
    \item putting the improvement into context
    \item 
\end{itemize}
}





==> sections/old/intro_v4.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\section{Introduction}

Real-time videos are as important and popular as traditional streaming videos. 
With applications ranging from video conferencing to emerging IoT services and cloud-based gaming~\cite{webrtc-gaming-1,webrtc-gaming-2,webrtc-vr-1,webrtc-vr-2,webrtc-iot-1,webrtc-iot-2}, video in Chrome over WebRTC grew 100x during 2020~\cite{blum2021webrtc}, and one global industry survey found that services based on real-time videos grew from less than 5\% to over 28\% between 2020 and 2021~\cite{video-report-2020,video-report-2021}.
% ~\cite{\url{https://www.wowza.com/wp-content/uploads/Streaming-Video-Latency-Report-Interactive-2020.pdf},??}.
% https://f.hubspotusercontent20.net/hubfs/229276/2021%20Low%20Latency%20Report/streaming-video-latency-report-interactive-2021.pdf

With users increasingly depending on real-time videos, it is crucial to deliver video frames smoothly and with decent quality under a wide range of network conditions\footnote{This problem so profound and urgent that serious efforts are finally being made by ISPs to offer active queue management for real-time traffic~\cite{l4s}, marking  a shift in focus from bandwidth to tail delay~\cite{report}, but wide deployment is still a long way off. Our proposed solution is complementary to this trend and can benefit from it once deployed (see \S\ref{??}).}, including
long latency and highly dynamic network jitters, causing intermittent bursts of {\em packet losses}. 
Importantly, in real-time video, packet losses include {\bf not only} randomly dropped packets, but also those delayed (due to congestion, path fluctuation, or retransmission) and thus arriving after when the frames they belong to are supposed to be decoded (\eg 40ms after decoding the last frame if the video is 25fps)\footnote{In lack of a better term, we call them {\em packet losses}.}.
%{\em long latency}, {\em high packet jitters} and {\em intermittent bursts of packet losses}.
%Importantly, in real-time video, packet losses include {\bf not only} randomly dropped packets, but also those delayed by congestion, path fluctuation, or retransmission and arriving after when the frames they belong to are supposed to be decoded (\eg 40ms after decoding the last frame if the video is 25fps)\footnote{In lack of a better term, we call them {\em packet losses}.}.
Recent measurements shown that high packet jitters and losses are not rare in real-time video applications~\cite{jansen2018performance,concerto}; \eg a drop of bandwidth from 3Mbps to 500Kbps can make 75\% of packets missing their playback time and raise the RTT by 6$\times$.
%one study found that in \fillme sessions, packet loss rates can be up-to \fillme\% for \fillme\% frames.\jc{YIHUA, please fill the numbers}
Retransmission is often too late with long RTT, since the jitter buffer is only \fillme; \eg resending packets on a path with 100ms RTT will delay or skip at least three frames in a 25fps video stream (\ie a new frame every 40ms).

\begin{comment}
Since real-time video clients have a very shallow jitter buffer (\fillme), a packet is effectively lost as long as it is delayed long enough (due to retransmission, congestion, path fluctuation, etc) to affect the decoding of a frame (and subsequent frames).\footnote{It is important that in real-time video, packet losses {\bf not only} include packets randomly dropped by the network, but also those that are delayed due to congestion, path fluctuation, or retransmission and arrive later than when the frame it belongs to is supposed to be decoded (\eg 40ms after the last frame was decoded if the video is 25fps). In lack of a better term, we call them packet losses, and the packet loss rates can thus easily be as high as \fillme\%, as shown in recent measurements~\cite{??,??}}
For instance, retransmitting packets on a path with 100ms RTT could delay (or skip) at least three frames in a 25fps video stream (\ie a new frame every 40ms).
Prior measurements have confirmed that such long RTT is common in video conferencing and that high packet jitters and losses are not rare, due to reasons including bursty cross-traffic, packet reordering, and variation of encoded frame sizes.
\end{comment}

%\jc{mention the need for high frame rate, i.e., can't skip frames!}


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        \includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss.pdf}
         \label{fig:}
    \caption{Comparing different loss-resilient schemes when the actual encoding bitrate is set at \fillme Mbps. 
    Quality of \name's autoencoder achieves a smoother quality degradation as packet loss rate increases.
    More results can be found in \S\ref{sec:eval}.\jc{YIHUA, remember to add a line of 264 without loss, and remove the part of h264 when it's undecodable}}
    \label{fig:intro-example}
\end{figure}

%To flexibly balance video quality and video delay, ideally a client should be able to decode the next frame when {\em any} non-empty subset of its packets is received and still obtain decent quality given the amount of data received. 
Many prior techniques have been proposed to tolerate packet losses, but they still require retransmission or trade low quality for higher loss resilience. 
%
%An ideal client should therefore tolerate packet losses be able to decode the next frame when {\em any} non-empty subset of its packets is received and still obtain decent quality given the amount of data received. 
%Unfortunately, existing loss-resilient schemes fall short of this expectation.
%, especially in links with long propagation RTTs and high packet jitters (\eg transient congestion and packet drops). 
For instance, Forward Error Correction (FEC) requires a minimum fraction of packets be reliably received before a frame is decodable, and to lower this minimum fraction, more redundancy must be added, forcing the sender to encode a frame in lower quality before sending the packets out. 
As a result (illustrated in Figure~\ref{fig:intro-example}), video quality will be low if packet losses are overestimated, or delay will be high if packet losses are underestimated. 
Similar tradeoffs between quality and delay (loss resilience) manifest themselves in other schemes (\eg SVC, inter-MB insertion) as well (\S\ref{subsec:abstractions}). 

%To tolerate a higher fraction of packets being missed when decoding, more redundancy must be added {\em before} packets transmission. 
%Thus, choosing an appropriate level of redundancy is known to be difficult under high packet jitters~\cite{??}.
%As illustrated in Figure~\ref{fig:intro-example}, too much redundancy would underutilize bandwidth (\ie low video quality if all packets arrive on time), while too little redundancy would drive the receiver to wait for (or resend) more packets. 
%In short, the same coding cannot achieve high quality under both no packet loss and high fraction of packet loss.
%As elaborated in \S\ref{??}, other schemes (\eg SVC, inter-MB insertion) also must deliver at least certain number of packets for a frame to be decodable, and/or pad video data with non-trivial redundancy in anticipation of certain packet loss rate, which hurts video quality if no packets turn out lost.

To address these limitations, we advocate for a new abstraction, referred to as {\em data-scalable} video delivery, and a practical implementation of it: the same encoding of a frame can be decodable once {\em any} non-empty subset of its packets are received (as opposed to a minimum set of packets as in FEC, RS or fountain codes) and achieve higher quality with each new packet received.\footnote{At first glance, this may sound like scalable video coding (SVC), whose quality increase with throughput. However, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets and a missing packet may disproportionally render multiple quality layers undecodable. In practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).}
%, which entails two requirements: 
%(1) the coding of a video frame does not depend on an anticipated loss rate, 
%(2) a frame is decodable once {\em any} non-empty subset of its packets are received and the decoded quality improves with more packets received.
%In other words, the decoded video quality degrades {\em gracefully} with more lost packets. 
In other words, a frame is decoded at a similar quality to a classic codecs (\eg H.26x) when no packet is lost, and the quality degrades {\em gracefully} with more lost packets. 
%the decoded video quality, under no packet losses, should be similar to a classic codecs (\eg H.264, H.265) and degrade {\em gracefully} with more lost packets. 
The abstraction of data-salable delivery therefore does not need to predict packet losses before sending video packets; instead, the receiver can flexibly choose when to decode a frame once any packets have arrived while enjoying decent video quality.

%the sender to inject redundancy based on predicted packet losses; 


\begin{comment}

Unlike FEC which sets redundancy rate {\em before} sending data out, our goal is to encode a frame in a \rate-agnostic way and decode the frame under any \rate (less than 100\%) at a similar quality as current FEC-based coding {\em if} it knew \rate. 
In other words, 
(1) under zero \rate, the decoded video quality should be close to that of existing video coding without FEC redundancy, and 
(2) the decoded video quality should degrade gracefully with higher \rate, with a similar quality as FEC-based coding if FEC knows the \rate. 
% So without knowing \rate, it should achieve similar quality as existing real-time video systems when they know \rate. 
In short, the envisioned real-time video system eschews the need for \rate prediction.

\end{comment}

We explore a new approach to data-scalable delivery, inspired by the emergent neural {\em autoencoders}.
We discuss the benefits and caveats of using autoencoders in \S\ref{subsec:why-autoencoder}.
%, neural-network coder/decoders for multimedia data (videos and images). 
Thanks to their neural-network architecture, autoencoder {\em could} be data-scalable, but existing autoencoders' quality drops quite quickly with lost packets.
We show, however, that by simulating packet losses during autoencoder training, we can train {\em data-scalable autoencoders}, that learn not only how to compress video pixels efficiently but also how to code them in ways resilient to missing packets.

%While data-scalable coding might be possible with existing codecs, we
%This paper explores a new approach to data-scalable coding, by borrowing and customizing autoencoders, an emergent class of neural-net coder/decoders for multimedia data (videos and images). 
%Existing autoencoders are developed with compression efficiency as the objective, but we show that by injecting emulated packet losses during autoencoder training, we can create a {\em data-scalable autoencoders}, that learn not only how to code video pixels efficiently but also how to code them in a way that is resilient to missing packets.
%% Training in itself is not straightforward, since packet losses are not naturally differentiable.
%%While the idea of data-scalable autoencoder is arguably simple, its performance gain is quite remarkable. 
%The resulting autoencoder, though slightly less efficient at compressing videos under no packet losses than classic heavily engineered codecs, can meet the two criteria of data-scalable coding. 
%Figure~\ref{fig:intro-example} shows an example result: the decoded quality at x\% packet losses should be close to that of H.264 or H.265 with x\% FEC redundancy, which can be viewed as a reference design that optimizes compression efficiency, not loss resilience.

This work presents the design and implementation of \name, a concrete real-time video system based on data-scalable autoencoders. 
%To make data-scalable autoencoders practical, we present the design and implementation of \name, an end-to-end real-time video system.
Figure~\ref{fig:intro-example} shows an example result: its quality degrades gracefully with more packet losses, and at various packet loss rate, its quality is comparable to that of H.264 or H.265 with adequate FEC redundancy. 
%, which can be viewed as a traditional reference that optimizes compression efficiency and loss resilience.

%the decoded quality at x\% packet losses is close to that of H.264 or H.265 with x\% FEC redundancy, which can be viewed as a reference design that optimizes compression efficiency, but not loss resilience.

\name tackles two high-level challenges. 
First, how to train data-scalable autoencoders (\S\ref{sec:training}). 
We discuss design choices regarding how packet losses should be simulated as part of model training given that the impact of packet loss on coded data is non-differentiable, and
what packet losses should be revealed during autoencoder training in order to balance quality at high rates and low rates of packet losses.
We also discuss why autoencoders can be made data-scalable.


%First, how to train a data-scalable autoencoder to tolerate various unseen packet loss rates. 
%This challenge entails several subquestions, such as
%how packet losses should be simulated as part of model training given that the impact of packet loss on coded data is non-differentiable, and
%what packet losses should be revealed during autoencoder training in order to balance quality at high rates and low rates of packet losses.

%and why our autoencoder is more resilient to data losses than existing schemes.

Second, how video frames encoded by autoencoder should be streamed to realize data scalable delivery over a {\em sequence} of frames. 
\name uses custom strategies of packetization and frame scheduling, such that the (individually decodable) packets are received and decoded in a way that balances frame delay  and quality (\S\ref{sec:delivery}).
\name also provides optimizations to adapt bitrate on top of autoencoders and reduce compute and memory overheads (\S\ref{subsec:optimize}).
\name is {\em complementary} to congestion control which decides how fast packets should be sent, while \name decides {\em what} packets should be send.

%Second, how to realize data-scalable delivery over data generated by the data-scalable autoencoder. 
%This involves several design questions such as how a streaming protocol designed for data-scalable autoencoders should look like (including packetization, packet scheduling, reference frame selection), and how much compute/storage overheads autoencoders would add to WebRTC and how to mitigate them. 
%Moreover, since use of autoencoders in real-time video delivery is relatively new, we also examine various strategies for bitrate adaptation and key frame insertion in the context of \name.

%Most components of \name are inspired by prior work.
%No individual component of \name is particularly new. %, and some are inspired by prior work. 



%\jc{there's some concerns regarding autoencoders. these questions are answered for the first time}

%how to best emulate packet losses during training so that the resulting autoencoder can handle and
%how well an autoencoder fares in unseen content {\em and} unseen \rates. 
%Moreover, since the video codec is tightly connected to other components in a real-time video system, data-scalable autoencoders bring up unique design questions, such as 
%how a streaming protocol designed for data-scalable autoencoders should look like (including packetization, packet scheduling, reference frame selection), and how much compute/storage overheads autoencoders would add to WebRTC and how to mitigate them. 

% This begs several immediate and critical questions.

% Instead, we try to answer these technical questions in the context of \name, a concrete system based on data-scalable autoencoders. 


% To best utilize data-scalable autoencoders in practice, they should also be  video streaming system. 



Importantly, \name does {\em not} improve coding efficiency (higher quality with less bits), which most heavily engineered video codecs strive to optimize. 
In fact, \name's video quality is slightly lower than H.265 at same bitrate. 
However, \name enables data-scalable delivery to achieve better quality with lower delay in high jitter networks.


We are not the first to use autoencoders in video compression. 
Applications of autoencoders can be found in wireless and data communication to compress images, video files, and signals~\cite{erpek2020deep}, and notably a recent work uses custom autoencoders to obtain highly efficient scalable video coding (SVC)~\cite{swift}. 
%Many aspects of \name are also inspired by prior work. 
That said, \name, to our best knowledge, is the first to use custom autoencoders to realize data-scalable video delivery.
The contribution of \name is an end-to-end real-time video delivery framework, which tackles various challenges arising from training and using data-scalable autoencoder in real-time video communication.



We test \name and traditional loss-resilient schemes and codecs on real and synthetic network traces, as well as various genres of videos.
Our results show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces video frame delay (by 2-3$\times$ at the 95th percentile) with marginally lowered video quality (less than \fillme~dB in SSIM).
To put it in perspective, \name significantly improves playback smoothness (\fillme less stalls with a jitter buffer) and reduces the chance that frames arrive after user-perceivable delay (\eg 200ms for video conferencing).

\textbf{This work does not raise any ethical issues.}

%\jc{eval highlights}

%\jc{outline the roadmap and highlight the contribution again}

%\jc{need a forward pointer to 2.2 (caveats of autoencoders)}
%
%\jc{
%\begin{itemize}
%    \item content generalization
%    \item clarify the use cases
%    \item putting the improvement into context
%    \item 
%\end{itemize}
%}





==> sections/old/intro_v5.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}

%Real-time videos are as important and popular as traditional streaming videos. 
With applications ranging from video conferencing to emerging IoT services and cloud-based gaming~\cite{webrtc-gaming-1,webrtc-gaming-2,webrtc-vr-1,webrtc-vr-2,webrtc-iot-1,webrtc-iot-2}, real-time videos in Chrome over WebRTC (one of the most popular real-time video frameworks) grew 100x during 2020~\cite{blum2021webrtc}, and one global industry survey found that services based on real-time videos grew from less than 5\% to over 28\% between 2020 and 2021~\cite{video-report-2020,video-report-2021}.
% ~\cite{\url{https://www.wowza.com/wp-content/uploads/Streaming-Video-Latency-Report-Interactive-2020.pdf},??}.
% https://f.hubspotusercontent20.net/hubfs/229276/2021%20Low%20Latency%20Report/streaming-video-latency-report-interactive-2021.pdf

With this increasing demand for real-time videos, it is crucial to deliver the video frames smoothly and with decent quality under a wide range of network conditions\footnote{This problem is so profound and urgent that serious efforts are finally being made by ISPs to offer active queue management for real-time traffic~\cite{l4s}, marking  a shift in focus from bandwidth to tail delay~\cite{latency-report-apnic}, but wide deployment is still a long way off. Our proposed solution is complementary to this trend and can benefit from it once deployed (see \S\ref{sec:eval}).}, including
long latency and highly dynamic network jitters, causing intermittent bursts of {\em packet losses}. 
Importantly, in this work, we use packet losses to refer to both randomly dropped packets {\em and} those delayed (due to congestion, path fluctuation, or retransmission) and thus arriving after when the frames they belong to are supposed to be decoded (\eg 40ms after decoding the last frame if the video is 25fps).
%{\em long latency}, {\em high packet jitters} and {\em intermittent bursts of packet losses}.
%Importantly, in real-time video, packet losses include {\bf not only} randomly dropped packets, but also those delayed by congestion, path fluctuation, or retransmission and arriving after when the frames they belong to are supposed to be decoded (\eg 40ms after decoding the last frame if the video is 25fps)\footnote{In lack of a better term, we call them {\em packet losses}.}.
Recent measurements show that high packet jitters and losses exist widely in real-time video applications~\cite{jansen2018performance,concerto,latency-report-apnic,latency-report-iab}; \eg a drop of bandwidth from 3Mbps to 500Kbps can cause 75\% of packets missing their playback time and raise the RTT by 6$\times$.
%one study found that in \fillme sessions, packet loss rates can be up-to \fillme\% for \fillme\% frames.\jc{YIHUA, please fill the numbers}
With long RTT, retransmission is often too late since the jitter buffer is only tens of milliseconds; \eg resending packets on a path with 100ms RTT will delay or skip at least three frames in a 25fps video stream (\ie a new frame every 40ms).

\begin{comment}
Since real-time video clients have a very shallow jitter buffer (\fillme), a packet is effectively lost as long as it is delayed long enough (due to retransmission, congestion, path fluctuation, etc) to affect the decoding of a frame (and subsequent frames).\footnote{It is important that in real-time video, packet losses {\bf not only} include packets randomly dropped by the network, but also those that are delayed due to congestion, path fluctuation, or retransmission and arrive later than when the frame it belongs to is supposed to be decoded (\eg 40ms after the last frame was decoded if the video is 25fps). For lack of a better term, we call them packet losses, and the packet loss rates can thus easily be as high as \fillme\%, as shown in recent measurements~\cite{??,??}}
For instance, retransmitting packets on a path with 100ms RTT could delay (or skip) at least three frames in a 25fps video stream (\ie a new frame every 40ms).
Prior measurements have confirmed that such long RTT is common in video conferencing and that high packet jitters and losses are not rare, due to reasons including bursty cross-traffic, packet reordering, and variation of encoded frame sizes.
\end{comment}

%\jc{mention the need for high frame rate, i.e., can't skip frames!}


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        \includegraphics[width=0.85\linewidth]{figs/fig1-example.pdf}
         \label{fig:}
    \tightcaption{Comparing different loss-resilient schemes when the actual encoded bitrate (not target bitrate) is set at 3.6 Mbps. (FEC bits are included in the encoded bitrate.)
    Quality of \name's autoencoder degrades gracefully with a higher packet loss rate. 
%    achieves a smoother quality degradation as packet loss rate increases.
    More results can be found in \S\ref{sec:eval}.
    %\jc{YIHUA, remember to add a line of 264 without loss, and remove the part of h264 when it's undecodable}\jc{set R-D optimization to "intra-MB insertion"}
    }
    \label{fig:intro-example}
    % \vspace{-0.5cm}
\end{figure}

%To flexibly balance video quality and video delay, ideally a client should be able to decode the next frame when {\em any} non-empty subset of its packets is received and still obtain decent quality given the amount of data received. 
Many prior techniques have been proposed to tolerate packet losses, but they either require retransmission or trade low quality for higher loss resilience. 
%
%An ideal client should therefore tolerate packet losses be able to decode the next frame when {\em any} non-empty subset of its packets is received and still obtain decent quality given the amount of data received. 
%Unfortunately, existing loss-resilient schemes fall short of this expectation.
%, especially in links with long propagation RTTs and high packet jitters (\eg transient congestion and packet drops). 
For instance, Forward Error Correction (FEC) requires a minimum fraction of packets to be reliably received before a frame is decodable, and to lower this minimum fraction, more redundancy must be added, forcing the sender to encode a frame in lower quality before sending the packets out. 
As a result (illustrated in Figure~\ref{fig:intro-example}), the video quality will be low if packet losses are overestimated, or delay will be high if packet losses are underestimated. 
Similar tradeoffs between quality and delay (loss resilience) manifest themselves in other schemes (\eg SVC, intra-MB insertion) as well (\S\ref{subsec:abstractions}). 

%To tolerate a higher fraction of packets being missed when decoding, more redundancy must be added {\em before} packets transmission. 
%Thus, choosing an appropriate level of redundancy is known to be difficult under high packet jitters~\cite{??}.
%As illustrated in Figure~\ref{fig:intro-example}, too much redundancy would underutilize bandwidth (\ie low video quality if all packets arrive on time), while too little redundancy would drive the receiver to wait for (or resend) more packets. 
%In short, the same coding cannot achieve high quality under both no packet loss and high fraction of packet loss.
%As elaborated in \S\ref{??}, other schemes (\eg SVC, inter-MB insertion) also must deliver at least certain number of packets for a frame to be decodable, and/or pad video data with non-trivial redundancy in anticipation of certain packet loss rate, which hurts video quality if no packets turn out lost.


This paper presents the design and implementation of \name, a new real-time video system based on the emergent neural {\em autoencoders}.
%To make data-scalable autoencoders practical, we present the design and implementation of \name, an end-to-end real-time video system.
Figure~\ref{fig:intro-example} shows an example of \name's loss resilience: 
if no packet is lost, a frame can be decoded at a similar quality to classic codecs (\eg H.264), and with more packet losses, \name's quality degrades more {\em gracefully} than various baselines (explained in \S\ref{sec:eval}).

At its core, \name's new autoencoder offers a new abstraction, called {\em data-scalable delivery}:
the same encoding of a frame can be decodable once {\em any} non-empty subset of its packets are received (as opposed to a minimum set of packets required by FEC, RS or fountain codes) and achieve higher quality with each new packet received.\footnote{At first glance, this may sound like scalable video coding (SVC), whose quality increase with throughput. However, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets and a missing packet may disproportionally render multiple quality layers undecodable. In practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).}
%the decoded video quality, under no packet losses, should be similar to a classic codecs (\eg H.264, H.265) and degrade {\em gracefully} with more lost packets. 
Therefore, a sender does not need to predict packet losses; instead, the receiver can flexibly choose when to decode a frame once any packets have arrived while enjoying decent video quality.

\name customizes autoencoders because of their empirical smooth relationships between video quality and the perturbations on the coded data (\eg packet losses), which naturally arise from autoencoders' neural network structure (elaborated in \S\ref{subsec:understanding}).
However, off-the-shelf autoencoders do not yet have a graceful quality degradation under packet losses.



%of autoencoders makes them a natural fit for data-scalable delivery, thanks to the autoencoder's smooth relationship between video quality and the perturbations on the coded data (elaborated in \S\ref{sec:understanding})


\name's contribution is three-fold. 
First, we show that by simulating packet losses during autoencoder training (\S\ref{sec:training}), it is possible to train autoencoders that learn not only how to compress frames efficiently but also how to code them in ways resilient to lost packets.\footnote{\name's autoencoder is joint-source-channel coder (see \S\ref{sec:related}).}
%, in a similar spirit as~\cite{??}, which also uses autoencoders, but to code images (rather than video) to correct bit-level noises (rather packet losses).}
%We also discuss design choices regarding how packet losses should be simulated in end-to-end training and how to train autoencoders to work well on various packet loss rates. 
%, and
%what packet losses should be revealed during autoencoder training in order to balance quality at high rates and low rates of packet losses.

Second, \name presents a framework to stream autoencoder output over a {\em sequence} of frames (\S\ref{sec:delivery}). 
\name uses custom strategies to encode sequences of I-frames and P-frames and allow a receiver to determine when to decode a frame anytime after receiving the first packet, in order to balance frame delay and decoded video quality even when packet losses last for multiple frames. 
%of frame scheduling (when to decode a frame) to allow the receiver to balance frame delay and decoded video quality  are received and decoded in a way that balances frame delay and quality.
\name can work on existing congestion control algorithms, which decide how fast packets should be sent, while \name decides {\em what} packets should be sent.



Third, autoencoders are not as optimized (in speed and coding efficiency) as heavily engineered traditional codecs. 
To make it practical, \name provides optimizations to speed up the encoding/decoding, reduce compute and memory overheads, and adapt encoding bitrates under dynamic bandwidth (\S\ref{subsec:optimize}).
Importantly, \name does {\em not} improve coding efficiency (higher quality with fewer bits), which most heavily engineered video codecs strive to optimize. 
Indeed, \name's video quality is still slightly lower than H.265 at the same bitrate. 
%That said, \name enables data-scalable delivery to achieve better quality with lower delay in high jitter networks.

We are not the first to apply autoencoders to data communication. 
Autoencoders have already been used in wireless and data communication to compress images, video files, and signals~\cite{erpek2020deep}. Notably, a recent work also uses custom autoencoders to obtain highly efficient scalable video coding (SVC)~\cite{swift}. 
%Many aspects of \name are also inspired by prior work. 
That said, \name, to our best knowledge, is the first to develop custom autoencoders that realize data-scalable video delivery.
The contribution of \name is an end-to-end real-time video delivery framework, which tackles various challenges arising from training and using data-scalable autoencoder in real-time video communication.



We test \name with traditional loss-resilient schemes and codecs on real and synthetic network traces, as well as various genres of videos.
Our results show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile when prior work has to retransmit packets or skip frame), with the marginally lowered video quality.
To put it in perspective, \name can significantly reduce the chance that frames arrive after user-perceivable delay (\eg 200ms for video conferencing) and improve playback smoothness (higher frame rate).

\textbf{This work does not raise any ethical issues.}

















==> sections/old/intro_v6.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}


%Real-time videos are as important and popular as traditional streaming videos. 
With applications ranging from video conferencing to emerging IoT services and cloud-based gaming~\cite{webrtc-gaming-1,webrtc-gaming-2,webrtc-vr-1,webrtc-vr-2,webrtc-iot-1,webrtc-iot-2}, real-time videos in Chrome over WebRTC (one of the most popular real-time video frameworks) grew 100x during 2020~\cite{blum2021webrtc}.
One industry survey found that services based on real-time videos grew global-wise from less than 5\% to over 28\% between 2020 and 2021~\cite{video-report-2020,video-report-2021}.
% ~\cite{\url{https://www.wowza.com/wp-content/uploads/Streaming-Video-Latency-Report-Interactive-2020.pdf},??}.
% https://f.hubspotusercontent20.net/hubfs/229276/2021%20Low%20Latency%20Report/streaming-video-latency-report-interactive-2021.pdf

Therefore, it is crucial for real-time video systems to deliver each frame smoothly with decent quality, even under highly dynamic bandwidth (making bursts of packets unavoidable) and long latency (making packet retransmissions too costly).`\footnote{This problem is so profound and urgent that serious efforts are finally being made by ISPs to offer active queue management for real-time traffic~\cite{l4s}, marking  a shift in focus from bandwidth to tail delay~\cite{latency-report-apnic}, but wide deployment is still a long way off. Our proposed solution is complementary to this trend and can benefit from it once deployed (see \S\ref{sec:eval}).}
% presence of long latency and intermittent bursts of {\em packet losses}
% , including long latency and highly dynamic network jitters, causing.  
Here, packet losses refer to both dropped packets {\em and} packets delayed too much (due to congestion, path fluctuation, or retransmission) that they cause visual glitches---they arrive after when the frames they belong to are supposed to be decoded (\eg 40ms after decoding the last frame if the video is 25fps).
%{\em long latency}, {\em high packet jitters} and {\em intermittent bursts of packet losses}.
%Importantly, in real-time video, packet losses include {\bf not only} randomly dropped packets, but also those delayed by congestion, path fluctuation, or retransmission and arriving after when the frames they belong to are supposed to be decoded (\eg 40ms after decoding the last frame if the video is 25fps)\footnote{In lack of a better term, we call them {\em packet losses}.}.
A sudden drop of bandwidth from 3Mbps to 500Kbps can cause 75\% of packets by dropped or delayed, and 
%one study found that in \fillme sessions, packet loss rates can be up-to \fillme\% for \fillme\% frames.\jc{YIHUA, please fill the numbers}
resending these packets is often too late since the jitter buffer is only tens of milliseconds; \eg resending packets on a path with 100ms RTT will delay or skip at least three frames in a 25fps video stream (\ie a new frame every 40ms).
Recent measurements have shown that similar network conditions are not rare in real-time video applications~\cite{jansen2018performance,concerto,latency-report-apnic,latency-report-iab}.

\begin{comment}
Since real-time video clients have a very shallow jitter buffer (\fillme), a packet is effectively lost as long as it is delayed long enough (due to retransmission, congestion, path fluctuation, etc) to affect the decoding of a frame (and subsequent frames).\footnote{It is important that in real-time video, packet losses {\bf not only} include packets randomly dropped by the network, but also those that are delayed due to congestion, path fluctuation, or retransmission and arrive later than when the frame it belongs to is supposed to be decoded (\eg 40ms after the last frame was decoded if the video is 25fps). For lack of a better term, we call them packet losses, and the packet loss rates can thus easily be as high as \fillme\%, as shown in recent measurements~\cite{??,??}}
For instance, retransmitting packets on a path with 100ms RTT could delay (or skip) at least three frames in a 25fps video stream (\ie a new frame every 40ms).
Prior measurements have confirmed that such long RTT is common in video conferencing and that high packet jitters and losses are not rare, due to reasons including bursty cross-traffic, packet reordering, and variation of encoded frame sizes.
\end{comment}

%\jc{mention the need for high frame rate, i.e., can't skip frames!}


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/fig1-example.pdf}
        \includegraphics[width=0.85\linewidth]{figs/fig1-example-osdi.pdf}
         \label{fig:}
    \tightcaption{Comparing different loss-resilient schemes when the actual encoded bitrate (not target bitrate) is set at 3.6 Mbps. (FEC bits are included in the encoded bitrate.)
    Quality of \name's autoencoder degrades gracefully with a higher packet loss rate. 
%    achieves a smoother quality degradation as packet loss rate increases.
    More results can be found in \S\ref{sec:eval}. \jc{Yihua, can you replot the FEC lines to use the same color (w/ diff point/line types)}
%    \jc{Yihua, can you add (DSC) next to our solution?}
%    \jc{Yihua, can we also replace yellow with 50\% redundancy?}
    %\jc{YIHUA, remember to add a line of 264 without loss, and remove the part of h264 when it's undecodable}\jc{set R-D optimization to "intra-MB insertion"}
    \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
    \jc{Yihua, can you add a horizontal line to indicate the quality of H.265}
    }
    \label{fig:intro-example}
    % \vspace{-0.5cm}
\end{figure}

%To flexibly balance video quality and video delay, ideally a client should be able to decode the next frame when {\em any} non-empty subset of its packets is received and still obtain decent quality given the amount of data received. 

% add a pre-determined rate of redundancy to tolerate a fraction of packet losses. 
%An ideal client should therefore tolerate packet losses be able to decode the next frame when {\em any} non-empty subset of its packets is received and still obtain decent quality given the amount of data received. 
%Unfortunately, existing loss-resilient schemes fall short of this expectation.
%, especially in links with long propagation RTTs and high packet jitters (\eg transient congestion and packet drops). 

Many loss-resilient schemes have been studied, but either they work well only when the sender knows the future packet loss rate before sending packets or their quality drops quickly with more packet losses (\eg Figure~\ref{fig:intro-example}).
% Many loss-resilient schemes have been studied, but they either require a minimum number of  packets received before decoding a frame or cause substantial quality degradation to achieve loss resilience. 
A classic example is Forward Error Correction (FEC).
To tolerate $x\%$ packet losses, (at least) $x\%$ redundancy must be added {\em before} sending the packets out. 
As a result, if it underestimates packet loss rate, the client must resend some packets (or wait longer) for enough ($x\%$) packets to be received (\eg FEC with \fillme\% redundancy in Figure~\ref{fig:intro-example} when loss rate is higher than \fillme\%)
At the same time, if it overestimates packet loss rate (\ie fewer than $x\%$ packets are actually lost), video quality will be lower than what could have been achieved (\eg FEC with \fillme\% redundancy in Figure~\ref{fig:intro-example} when loss rate is lower than \fillme\%)..
Other schemes (\eg SVC, intra-MB insertion) have similar tradeoffs between quality and delay (loss resilience) as well, as will be elaborate on them in \S\ref{subsec:abstractions}. 
While more work can be done on existing loss-resilient schemes, the room to improve is likely limited after decades of research.


% This means that if more than $x\%$ packets are lost, the client must resend some packets (or wait longer) so that $(100-x)\%$ of packets must be delivered reliably (\fillme in Figure~\ref{fig:intro-example} shows an example).
% On the other hand, if fewer than $x\%$ packets are lost, video quality will be lower than what could be achieved by the amount of received data (\fillme in Figure~\ref{fig:intro-example} shows an example).
% It requires a minimum fraction of packets to be reliably received before a frame is decodable, and to lower this minimum fraction, more redundancy must be added, forcing the sender to encode a frame in lower quality before sending the packets out. 
% As a result (illustrated in Figure~\ref{fig:intro-example}), the video quality will be low if packet losses are overestimated, or delay will be high if packet losses are underestimated. 

%To tolerate a higher fraction of packets being missed when decoding, more redundancy must be added {\em before} packets transmission. 
%Thus, choosing an appropriate level of redundancy is known to be difficult under high packet jitters~\cite{??}.
%As illustrated in Figure~\ref{fig:intro-example}, too much redundancy would underutilize bandwidth (\ie low video quality if all packets arrive on time), while too little redundancy would drive the receiver to wait for (or resend) more packets. 
%In short, the same coding cannot achieve high quality under both no packet loss and high fraction of packet loss.
%As elaborated in \S\ref{??}, other schemes (\eg SVC, inter-MB insertion) also must deliver at least certain number of packets for a frame to be decodable, and/or pad video data with non-trivial redundancy in anticipation of certain packet loss rate, which hurts video quality if no packets turn out lost.

This work explores a clean-slate approach, based on the emergent {\em neural autoencoders}, to realizing a new video coding abstraction, called {\em data-scalable coding} ({\em DSC}), which entails two key properties.
{\em (i)} First, the frame is decodable once any non-empty subset of its packets are received, and quality improves with more packets received (or equivalently, the quality degrades gracefully with more packets missing). 
{\em (ii)} Second, unlike the redundancy-based coding (\eg FEC), how a frame is encoded should not depend on the prediction of future packet losses.

Figure~\ref{fig:intro-example} shows that such a codec (realized by our solution) is better than prior solutions: a frame can be decoded once {\em any} non-empty subset of its packets are received (as opposed to a minimum set of packets required by FEC, RS or fountain codes), have higher quality with more received packets, and if all packets are received, have a similar quality to classic codecs (\eg H.264).\footnote{At first glance, this may sound like scalable video coding (SVC), whose quality increase with throughput. However, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets and a missing packet may disproportionally render multiple quality layers undecodable. In practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).}
In other words, with more packet losses, \name's quality degrades more {\em gracefully} than various baselines (explained in \S\ref{sec:eval}).
Thus, a sender does not need to predict packet losses; instead, the receiver can flexibly choose when to decode a frame once any packets have arrived while enjoying decent video quality.


% based on the emergent neural {\em autoencoders}.
%
% Figure~\ref{fig:intro-example} shows an example of \name's loss resilience: 


% At its core, \name's new autoencoder offers a new abstraction, called {\em data-scalable delivery}:

We present the design and implementation of \name, an end-to-end real-time video system that realizes DSC.
\name customizes autoencoders because of their empirical smooth relationships between video quality and the perturbations on the coded data (\eg packet losses), which naturally arise from autoencoders' neural network structure (elaborated in \S\ref{subsec:understanding}).
However, off-the-shelf autoencoders do not yet have a graceful quality degradation under packet losses.



%of autoencoders makes them a natural fit for data-scalable delivery, thanks to the autoencoder's smooth relationship between video quality and the perturbations on the coded data (elaborated in \S\ref{sec:understanding})


\name's contribution is three-fold. 
First, we show that by simulating packet losses during autoencoder training (\S\ref{sec:training}), it is possible to train autoencoders that learn not only how to compress frames efficiently but also how to code them in ways resilient to lost packets.\footnote{\name's autoencoder is joint-source-channel coder (see \S\ref{sec:related}).}
%, in a similar spirit as~\cite{??}, which also uses autoencoders, but to code images (rather than video) to correct bit-level noises (rather packet losses).}
%We also discuss design choices regarding how packet losses should be simulated in end-to-end training and how to train autoencoders to work well on various packet loss rates. 
%, and
%what packet losses should be revealed during autoencoder training in order to balance quality at high rates and low rates of packet losses.

Second, \name presents a framework to stream autoencoder output over a {\em sequence} of frames (\S\ref{sec:delivery}). 
\name uses custom strategies to encode sequences of I-frames and P-frames and allow a receiver to determine when to decode a frame anytime after receiving the first packet, in order to balance frame delay and decoded video quality even when packet losses last for multiple frames. 
%of frame scheduling (when to decode a frame) to allow the receiver to balance frame delay and decoded video quality  are received and decoded in a way that balances frame delay and quality.
\name can work on existing congestion control algorithms, which decide how fast packets should be sent, while \name decides {\em what} packets should be sent.



Third, autoencoders are not as optimized (in speed and coding efficiency) as heavily engineered traditional codecs. 
To make it practical, \name provides optimizations to speed up the encoding/decoding, reduce compute and memory overheads, and adapt encoding bitrates under dynamic bandwidth (\S\ref{subsec:optimize}).
Importantly, \name does {\em not} improve coding efficiency (higher quality with fewer bits), which most heavily engineered video codecs strive to optimize. 
Indeed, \name's video quality is still slightly lower than H.265 at the same bitrate. 
%That said, \name enables data-scalable delivery to achieve better quality with lower delay in high jitter networks.

We are not the first to apply autoencoders to data communication. 
Autoencoders have already been used in wireless and data communication to compress images, video files, and signals~\cite{erpek2020deep}. Notably, a recent work also uses custom autoencoders to obtain highly efficient scalable video coding (SVC)~\cite{swift}. 
%Many aspects of \name are also inspired by prior work. 
That said, \name, to our best knowledge, is the first to develop custom autoencoders that realize data-scalable video delivery.
The contribution of \name is an end-to-end real-time video delivery framework, which tackles various challenges arising from training and using data-scalable autoencoder in real-time video communication.



We test \name with traditional loss-resilient schemes and codecs on real and synthetic network traces, as well as various genres of videos.
Our results show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile when prior work has to retransmit packets or skip frame), with the marginally lowered video quality.
To put it in perspective, \name can significantly reduce the chance that frames arrive after user-perceivable delay (\eg 200ms for video conferencing) and improve playback smoothness (higher frame rate).

\textbf{This work does not raise any ethical issues.}

















==> sections/old/intro_v7.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}

\jc{clarify multiparty and unicast}
\jc{bandwidth adaptation is different from loss protection}

Real-time video communication has a long history in research, yet only recently has it become truly popular and crucial to our daily lives~\cite{blum2021webrtc}, from online meetings~\cite{webrtc-vc-1,webrtc-vc-2}, cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2}, to interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2} and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
The amount of time users spend on real-time videos is growing much faster than watching traditional HTTP-based streaming videos~\cite{webrtc-trend-1,webrtc-trend-2}.
%As a result, users expect that each frame has a high quality, that no frame is skipped, and 
%that each frame is decoded on time such that the viewer sees a smooth playback (\eg under 25fps, a frame should be decoded every 40~ms). 

%These requirements are challenging for two reasons.
However, despite having higher available bandwidth, the users of real-time video applications still suffer poor quality and video stalls in video calls~\cite{vca-vice} and online games~\cite{gaming-asurion}, for two reasons.
First, real-time video has a {\em short} jitter buffer (0--1 frame in WebRTC)\footnote{In contrast, traditional streaming videos, even live broadcast videos, have a buffer of at least several seconds.}, so without sufficient loss protection, {\em any} delayed or lost packet 
%packet jitter, queuing delay or packet drop 
may block the encoding of a frame.
Henceforth, we call a packet as a {\em missing packet}, if it arrives after when the frame it belongs to should be decoded (\eg 40ms after the last frame is decoded under 25fps), and we refer to the fraction of data in missing packets of a frame as {\em data missing rate} or \rate. 
Note that a missed packet can be lost or delayed.

Second, it is {\em hard to know in advance} when high \rates occurs or which packets will be missing.
Real-time communication, such as video calls, often have  high network latency ($>$100~ms) and transient {\em bursts} of missing packets, arising from myriad reasons (sudden bandwidth drops, bad wireless, congestion-induced queuing buildups, routing fluctuations, etc).
As a result, for instance, a bandwidth drop from 3Mbps to 500Kbps on a 200ms-RTT link can suddenly raise \rate to 75\% and retransmission will delay or skip at least 6 frames in a 25fps video stream. 
Recent measurements have shown that such pathological scenarios are not rare in real-time video applications~\cite{jansen2018performance,concerto,latency-report-apnic,latency-report-iab}.

As non-zero \rate is hard to predict, a desirable solution for real-time videos should 
\begin{packeditemize}
\item {\em R1 (Few retransmission or frame skipping):} The receiver can decode a frame if {\em any} non-empty subset of the packets of this frame is received (\ie no retransmission or frame skipping unless all packets are missing);
\item {\em R2 (Graceful degradation):} The decoded quality gradually degrades with each missing packet; in order words, quality gradually improves with each received packet; and
\item {\em R3 (High compression efficiency):} The decoded quality reaches a quality close to that of a non-loss-resilient coding algorithm (such as H.265), if all packets are received.
%similar quality as the quality without redundancy (such as H.265), if all packets are received.
\end{packeditemize}
We call such a solution as {\em Data-Scalable} ({\em DS}) video delivery.

Over the past decades, there has been intense research towards loss-resilient video coding, but they each fall short in at least one of the three requirements.
For instance, scalable coding (such as SVC~\cite{??} and FGS~\cite{??}) violates {\em R2}, because packets must be received in a hierarchical order---from lower layers to higher layers---any lost packet on a lower layer will render higher layers undecodable even if more packets are received.
Moreover, forward error correction (FEC) violates {\em R1}, if FEC redundancy is insufficient, in which case it will have to resend or wait for some missing packets in order to decode the frame.
It also violates {\em R2}, because once the frame is decodable, more packets will not improve quality.
Finally, it violates {\em R3}, if too much FEC redundancy is used when no packets are missing, in which case not all bits are used to encode frames.
\S\ref{sec:??} will elaborate on more previous loss-resilient coding.

In contrast, we explore a new approach to DSC video delivery by encoding and decoding video frames using {\em neural-net (NN) autoencoders}.
At a high level, an NN encoder maps each frame to a point (a tensor) in a new embedding space, and the NN decoder maps the point to a reconstructed frame. 
These autoencoders, if used appropriately, could have two unique advantages.
First, unlike the output of scalable coding, an output tensor of an autoencoder does {\em not} impose a hierarchical structure among its elements. 
As a result, randomly perturbing a tensor in the new embedding space, such as zeroing any $\alpha\%$ of a tensor's elements, will have only a {\em limited} impact (proportional to $\alpha\%$)  on the quality of the decoded frame.
Second, unlike FEC which only tolerates a pre-determined data loss rate, one autoencoder (a pair of NN encoder and NN decoder) could be trained to achieve desirable quality under a {\em range} of data erasure rates. 

%erasing (by zeroing) any $\alpha\%$ of values in the output tensor has a limited impact (proportional to $\alpha\%$)  on the quality of the decoded frame.
%
%First, the output tensors of autoencoders do {\em not} impose a hierarchical structure as in scalable coding; instead, erasing (by zeroing) any $\alpha\%$ of values in the output tensor has a limited impact (proportional to $\alpha\%$)  on the quality of the decoded frame.
%Essentially, the neural network (NN) encoder maps a frame to a point in a new embedding space and the NN decoder maps the point back to a frame, where applying random perturbation (such as zeroing a random fraction of coordinates) on a point will unlikely change the decoding result dramatically.
%First, existing loss-resilient schemes obtain motion vectors and residuals from classic codecs (such as H264/265 or VP8/9), quantizes them, and runs lossless arithmetic coding. 
%First, the tensor outputs of autoencoders (before entropy coding)  ``flat'', rather than 


\begin{itemize}
\item real-time video requires: high quality, low tail delay per frame, and minimum frame skipping. why hard: cant guarantee all packets will arrive on time, and hard to predict how many and which will be late. 
\item our goal: (1) decodable at any arrived packets, (2) quality proportional to received data, and (3) high quality when all data is received
\item existing solutions miss some of them. list all solutions
\item we explore a clean-slate solution: how about autoencoder. two benefits (1) can add loss tolerance to training, and (2) flat output
\item how to train the model: a new formulation, selection of packet loss patterns in training
\item how to stream autoencoder output: entropy-encoding and packetization, i/p frame, frame scheduling
\item how to speedup autoencoder: speedup on cpu, bitrate adaptation
\item example improvement
\end{itemize}


==> sections/old/intro_v8.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}

Real-time video communication has a long history in research, yet only recently has it become truly popular and ubiquitous in our daily lives~\cite{blum2021webrtc}, from online meetings~\cite{webrtc-vc-1,webrtc-vc-2}, cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2}, to interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2} and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
The amount of time people spend on real-time videos increases much faster than they spend on streaming videos, both live and on-demand~\cite{webrtc-trend-1,webrtc-trend-2}.
%As a result, users expect that each frame has a high quality, that no frame is skipped, and 
%that each frame is decoded on time such that the viewer sees a smooth playback (\eg under 25fps, a frame should be decoded every 40~ms). 

However, compared to on-demand video viewers, users of real-time applications are more likely to suffer poor quality and video stuttering in video calls~\cite{vca-vice} and online gaming~\cite{gaming-asurion}.
%, even when the network is connected, \eg video freezes when audio continues~\cite{??}. 
This is because real-time video applications use a shallow jitter buffer (\eg \fillme ms in WebRTC).
As a result, {\em any} lost or delayed packet may increase the {\em frame delay}---the delay between sending a frame and receiving enough data to decode it.
This is particularly damaging in long-latency links (\eg long-distance video calls or bufferbloat), where resending just one packet takes one round-trip time and can block the decoding of several frames.

Loss-resilient video coding
%which decodes a frame at a decent quality in presence of packet loss, 
is thus the key to maintaining high video quality and smooth playback of real-time videos.
The performance of a loss-resilient coding scheme can be measured in {\em compression efficiency} (quality in {\em absence} of packet loss) and {\em loss resilience} (quality in {\em presence} of packet loss).
%in {\em presence} of packet loss, whether the decoder can decode a frame soon after receiving some of its packets at a decent quality).
%The former means that in {\em absence} of packet loss, the decoded quality of a frame is high, in PSNR, SSIM or VMAF.
%The latter means that in {\em presence} of packet loss, the decoder can decode a frame soon after receiving some of its packets at a decent quality.
%, given the amount of data in the packets received before decoding.
Henceforth, we refer to 
%the delay before the receiver decodes a frame as its {\em frame delay}, and 
the fraction of data in packets that arrive after a frame's decoding as {\em data missing rate} or \rate. Note that a missing packet can be lost or delayed.


%and a packet arriving after the frame delay is referred to as a {\em missing packet}. 
%Note that a missed packet can be lost or delayed.
%%A packet of a frame is a {\em missing packet}, if it takes longer than the frame delay, and 
%We refer to the fraction of data in missing packets of a frame as {\em data missing rate} or \rate. 

Unfortunately, in real-time videos, existing loss-resilient techniques fall short on either loss resilience or compression efficiency (see \S\ref{??}).\footnote{Some techniques that work well in on-demand videos are much less effective in real-time videos. 
Scalable video coding (SVC~\cite{??} or FGS~\cite{??}) is less effective, because in real-time videos, the packets of a frame are sent together, rather than layer by layer. 
This corroborates the observation in~\cite{salsify}. 
Another line of work~\cite{voxel,???} selectively skips frames that do not affect future frames (such as B-frames), but B-frames are seldom used in real-time videos, and I-frames, which stop the impact of skipped frames, are much fewer in real-time videos than in chunk-based videos. 
Nonetheless, this paper still evaluates them qualitatively and quantitatively.}
%Despite many proposals, current loss-resilient techniques achieve loss resilience at the cost of lower compression efficiency (see \S\ref{??}).
%existing loss-resilient techniques improve loss resilience at the cost of lower compression efficiency.
For instance, for forward error correction (FEC) to tolerate $30\%$ \rate, (at least) $30\%$ redundancy must be added {\em before} sending the packets out~\cite{??}. 
If fewer than $30\%$ packets are actually missing (\ie~\rate is overestimated), 
%it overestimates \rate (\ie fewer than $x\%$ packets are actually missing), 
video quality will be lower than if no redundancy is added.
If \rate is underestimated, the receiver must wait longer and request the sender to resend packets, until at least 70\% of packets are received.
%(\eg FEC with \fillme\% redundancy in Figure~\ref{fig:intro-example} when \rate exceeds \fillme\%).
%(\eg FEC with \fillme\% redundancy in Figure~\ref{fig:intro-example} when \rate is below \fillme\%).
Similarly, using an older frame as encoding reference lets the decoder safely skip a frame without affecting future frames (\eg~\cite{salsify}), but older reference frame also significantly lowers compression efficiency (needs more bits to reach same quality).
As a result, most real-time Internet video systems increase loss resilience only {\em after} packet loss has affected some frames~\cite{??,??,streamingcoding}. 
%, and leaving some frames unprotected against burst of packet loss. 
%it also significantly reduces compression efficiency as older frames are more different with the current frame.




A better solution, which we refer to as {\em Data-Scalable} ({\em DS}) video delivery, 
should gracefully degrade in presence of packet loss, without compromising quality in absence of packet loss.
%should have decent compression efficiency in presence of loss of {\em any} packets. 
Concretely, it should 
{\em (i)} reach a quality close to that of a non-loss-resilient coding algorithm (such as H.265), if all packets are received; 
{\em (ii)} be able to decode a frame if {\em any} (non-empty) subset of packets of the frame is received (\ie no retransmission unless all data are lost); and 
{\em (iii)} achieve better quality, if one more packet is received.
%As we have seen, prior work falls short on at least one front.



This paper presents \name, a real-time video system which explores a new approach to DS video delivery by using {\em neural-net (NN) autoencoders}.
At a high level, an autoencoder uses an NN encoder to encode a frame to an {\em autoencoder-output tensor} (before entropy encoding), and uses an NN decoder to decode the tensor to a reconstructed frame. 




\name chooses autoencoders, because the elements in an autoencoder-output tensor have much less dependency among them.
If we randomly select some elements of an autoencoder-returned code (\ie random erasures) and set them to zero, which as explained in \S\ref{??} could mimic the effect of packet loss, the decoder can still decode the whole frame. 
In contrast, missing information in H.264 
% will not render the whole frame undecodable. 
%does not have dramatic impact on the decoded video quality.
This is in contrast to SVC where any data loss on a low layer also affects higher layers.
Moreover, the impact of random erasures on video quality increases with the rate of random erasures (\eg more zeroed elements). 
In other words, unlike FEC needs to known \rate~{\em a priori}, the quality of autoencoders {\em could} degrade gracefully with more data loss.

\begin{comment}
We use autoencoders because they have two {\em potential} advantages.
First, there is little explicit dependency among the elements of an autoencoder-returned tensor. 
Thus, unlike in SVC where any data loss on a lower layer also affects higher layers, applying any random erasures (such as zeroing randomly selected elements) on an output tensor of an autoencoder will not have a dramatic impact on the decoded video quality.
%In other words, so the values in the tensor do not need to be received in specific order, like in SVC. 
Second, the impact of random perturbation on video quality {\em could} be further reduced by training the autoencoder to work under different random erasure rates. 
The resulting autoencoders might be better than FEC which only tolerates a pre-determined data loss rate.
%one autoencoder (a pair of NN encoder and NN decoder) could be trained to work under a {\em range} of data erasure rates and still achieve decent quality.
\end{comment}

Yet, traditional autoencoders are ill-suited for real-time videos. 
Here, we highlight how \name addresses two specific challenges to enable autoencoder-based DS video delivery.

First, traditional autoencoder-returned code could be decoded in presence of data loss, but its quality will degrade quickly with more random erasures.
This is because in standard autoencoder training, the encoder output is almost\footnote{Encoder output is sometimes quantized (lower float precision), but quantization's effect on video quality is much less than data erasures caused by packet loss.} always identical to the decoder input. 
%have never seen any data erasure during the training. 
%To improve quality under data erasures, 
\name uses a different autoencoder training process---it injecting random data erasures of various rates (from 0\% to 90\%) between the encoder and the decoder, which simulates the effects of different \rates.
In other words, the new autoencoders not only learn how to compress frames efficiently but also how to code them in a way resilient to different \rates (see \S\ref{??} for details). 

Second, existing autoencoders and standard video codecs use arithmetic coding to compress all information of a frame to a single bitstream which will then be packetized. 
This means that any packet loss will render the data undecodable.
%If this bitstream is packetized, as done in conventional real-time video systems, any packet loss will render the data undecodable.
Instead, \name first randomly partitions the autoencoder-returned code to sub-tensors and then arithmetically codes each sub-tensor as a separate packet.
Though it sounds easy, per-packet arithmetic coding turns out to be challenging, since traditional arithmetic coding incurs excessive size overhead per packet due to the need to store each packet's data distribution. 
\name addresses it using a novel scheme to balance the size overhead and efficiency of per-packet arithmetic coding (see \S\ref{??}). 

%As an end-to-end video coding framework, 
\name also tackles other practical challenges, such as efficient bitrate control, speeding up of autoencoders, and balancing the size of I-frames and P-frames.


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/fig1-example.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/fig1-example-osdi.pdf}
        \includegraphics[width=0.99\linewidth]{figs/fig1-example-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{Example results of \name's (a) more graceful degradation in presence of packet loss than prior solutions, and (b) better tradeoffs between video quality and tail frame delay, which corroborates the subjective rating of users.
         More results can be found in \S\ref{sec:eval}. 
%         \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
    \jc{TODO: add a horizontal line to indicate the quality of H.265}
         }
%    \tightcaption{Video quality vs. \rates of different video codecs when the actual encoded bitrate is 3.6 Mbps (which includes FEC redundancy if used.)
%    Quality of \name's autoencoder degrades gracefully with higher \rates. 
%%    achieves a smoother quality degradation as packet loss rate increases.
%    More results can be found in \S\ref{sec:eval}. 
%%    \jc{Yihua, can you replot the FEC lines to use the same color (w/ diff point/line types)}
%%    \jc{Yihua, can you add (DSC) next to our solution?}
%%    \jc{Yihua, can we also replace yellow with 50\% redundancy?}
%    %\jc{YIHUA, remember to add a line of 264 without loss, and remove the part of h264 when it's undecodable}\jc{set R-D optimization to "intra-MB insertion"}
%%    \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
%%    \jc{Yihua, can you add a horizontal line to indicate the quality of H.265}
%    }
    \label{fig:intro-example}
    % \vspace{-0.5cm}
\end{figure}



We should clarify that \name does {\em not} include rate adaptation, which decides the target bitrate of a frame and how fast to send its packets. 
Instead, we run \name on existing rate adaptation logics, such as GCC~\cite{??}, and use \name to decide {\em what} each packet should contain, so that even if the selected bitrate overshoots the bandwidth, we can still obtain decent quality.

\name aims at unicast video sessions, rather than multi-party conferencing, which involves other challenges such as stream distribution.

%Being a coding system, \name can work with existing congestion control (CC) logics---CC decides how fast to send packets, and \name decides {\em what} each packet contains.


To put \name in perspective, autoencoders have long been used in data communication~\cite{erpek2020deep} (see \S\ref{sec:related}).
\name, which can be seen as joint-source-channel coder, is similar 
%As a joint-source-channel coder, \name's autoencoder is similar 
in spirit to DeepJSCC which uses autoencoder to compress static images (rather than real-time videos) in a way robust to wireless signal noises~\cite{??} (rather than packet loss).
%for compressing images and signals in wireless communication and 
Recently, Swift applies autoencoders to improve scalable video coding (SVC) for on-demand streaming videos~\cite{swift}. 
To our best knowledge, \name is the first real-time video framework to demonstrates the unprecedented potential of autoencoders to improve loss resilience for real-time video communication.


%To our best knowledge, \name is the first end-to-end autoencoder-based video system for loss-resilient real-time videos.
%that achieves stream real-time videos in a data-scalable fashion. 



%arising from training and using autoencoders in real-time video communication.

%Many aspects of \name are also inspired by prior work. 
%That said, \name, to our best knowledge, is the first to develop custom autoencoders that realize data-scalable video delivery.

%\name aims at unicast video sessions, rather than multi-party conferences. 
%It is also important that \name's autoencoders do {\em not} achieve better compression efficiency than recent heavily engineered video codecs, such as H.265. 
%Indeed, \name's video quality is still slightly lower than H.265 at the same bitrate. 

We evaluate \name in two aspects (Figure~\ref{fig:intro-example} gives an example). 
First, on a variety of video content, \name's quality degrades more gracefully under packet loss than baseline loss-resilient video codecs.
%, without much compromise on quality in absence of packet loss. 
That said, in absence of packet loss, \name's quality is slightly lower than H.265 at the same bitrate, but this compromise is comparable or much less than other loss-resilient baseline (\eg adding 10\% FEC redundancy). 
%does {\em not} outperform the latest heavily engineered video codecs in quality---indeed, \name's video quality is slightly lower than H.265 at the same bitrate. 
Second, using real-world network traces and a packet-level simulator, we show that \name significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to the most competitive baselines which still have to retransmit packets or skip frames.
This greatly decreases video stuttering and skipped frames---our user study confirms that \name has much higher average subjective rating by users than the most competitive baselines.

\begin{comment}
Using real-world and synthetic network traces and a wide range of videos, we show that \name's autoencoder has a more graceful quality degradation under packet loss than baseline loss-resilient video codecs.
%, without sacrificing video quality in absence of packet loss 
(Figure~\ref{fig:intro-example} gives an example).
When comparing \name with the baselines with the same CC logic (\eg GCC~\cite{??} and Salsify-CC~\cite{??}), \name significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to prior work which has to retransmit packets or skip frames, with the comparable video quality.
To put it in perspective, \name significantly decrease the frames that arrive after user-perceivable delay (\eg 200ms for video calls) and reduces video stuttering.
\end{comment}

%Our results show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile when prior work has to retransmit packets or skip frame), with the marginally lowered video quality.
%To put it in perspective, \name can significantly reduce the chance that frames arrive after user-perceivable delay (\eg 200ms for video conferencing) and improve playback smoothness (higher frame rate).


\textbf{This work does not raise any ethical issues.}






%unlike SVC, the output tensor of an autoencoder does {\em not} impose a hierarchical structure among its elements, so the values in the tensor do not need to be received in specific order, like in SVC. 
%Instead, randomly perturbing a tensor in the new embedding space, such as zeroing any $\alpha\%$ of a tensor's elements, will have only a {\em limited} impact (proportional to $\alpha\%$)  on the quality of the decoded frame.
%Second, unlike FEC which only tolerates a pre-determined data loss rate, one autoencoder (a pair of NN encoder and NN decoder) could be trained to achieve desirable quality under a {\em range} of data erasure rates. 

%To be specific, each frame is supposed to be decoded at a fixed interval after the last frame was decoded, and 
%
%a packet associated with a frame will delay the rendering of a 
%To be more specific, we call a packet as a {\em missing packet}, if it arrives after when the frame it belongs to should be decoded (\eg 40ms after the last frame is decoded under 25fps), and we refer to the fraction of data in missing packets of a frame as {\em data missing rate} or \rate. 
%Note that a missed packet can be lost or delayed.






==> sections/old/intro_v9.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}

Real-time video communication has a long history in research, yet only recently has it become truly popular and ubiquitous in our daily lives~\cite{blum2021webrtc}, from online meetings~\cite{webrtc-vc-1,webrtc-vc-2}, cloud gaming~\cite{webrtc-gaming-1,webrtc-gaming-2}, to interactive virtual reality~\cite{webrtc-vr-1,webrtc-vr-2} and IoT applications~\cite{webrtc-iot-1,webrtc-iot-2}.
The amount of time people spend on real-time videos increases much faster than they spend on streaming videos, both live and on-demand~\cite{webrtc-trend-1,webrtc-trend-2}.
%As a result, users expect that each frame has a high quality, that no frame is skipped, and 
%that each frame is decoded on time such that the viewer sees a smooth playback (\eg under 25fps, a frame should be decoded every 40~ms). 

However, compared to on-demand video viewers, users of real-time applications are more likely to suffer poor quality and video stuttering in video calls~\cite{vca-vice} and online gaming~\cite{gaming-asurion}.
%, even when the network is connected, \eg video freezes when audio continues~\cite{??}. 
This is because real-time video applications use a shallow jitter buffer (\eg \fillme ms in WebRTC).
As a result, {\em any} lost or delayed packet may increase the {\em frame delay}---the delay between sending a frame and receiving enough data to decode it.
This is particularly damaging in long-latency links (\eg long-distance video calls or bufferbloat), where resending just one packet takes one round-trip time and can block the decoding of several frames.

Loss-resilient video coding
%which decodes a frame at a decent quality in presence of packet loss, 
is thus the key to maintaining high video quality and smooth playback of real-time videos.
The performance of a loss-resilient coding scheme can be measured in {\em compression efficiency} (quality in {\em absence} of packet loss) and {\em loss resilience} (quality in {\em presence} of packet loss).
%in {\em presence} of packet loss, whether the decoder can decode a frame soon after receiving some of its packets at a decent quality).
%The former means that in {\em absence} of packet loss, the decoded quality of a frame is high, in PSNR, SSIM or VMAF.
%The latter means that in {\em presence} of packet loss, the decoder can decode a frame soon after receiving some of its packets at a decent quality.
%, given the amount of data in the packets received before decoding.
Henceforth, we refer to 
%the delay before the receiver decodes a frame as its {\em frame delay}, and 
the fraction of data in packets that arrive after a frame's decoding as {\em data missing rate} or \rate. Note that a missing packet can be lost or delayed.


%and a packet arriving after the frame delay is referred to as a {\em missing packet}. 
%Note that a missed packet can be lost or delayed.
%%A packet of a frame is a {\em missing packet}, if it takes longer than the frame delay, and 
%We refer to the fraction of data in missing packets of a frame as {\em data missing rate} or \rate. 

Unfortunately, in real-time videos, existing loss-resilient techniques fall short on either loss resilience or compression efficiency (see \S\ref{??}).\footnote{
%Some techniques that work well in on-demand videos are much less effective in real-time videos. 
Scalable video coding (SVC~\cite{??}, FGS~\cite{??}, Swift~\cite{??}), which works well for on-demand streaming videos, is much less effective in real-time videos, because packets of a frame are sent together, rather than layer by layer (see \S\ref{??}).
For this reason, scalable video coding is not commonly used to improve unicast real-time videos~\cite{salsify}. 
%This corroborates the observation in~\cite{salsify}. 
Another line of work (\eg~\cite{voxel}) selectively skips frames that do not affect future frames (such as B-frames), but B-frames are seldom used in real-time videos, and I-frames, which stop the impact of skipped frames, are much fewer in real-time videos than in chunk-based videos. 
Nonetheless, we will still evaluate them against \name.}
%Despite many proposals, current loss-resilient techniques achieve loss resilience at the cost of lower compression efficiency (see \S\ref{??}).
%existing loss-resilient techniques improve loss resilience at the cost of lower compression efficiency.
For instance, for forward error correction (FEC) to tolerate $30\%$ \rate, (at least) $30\%$ redundancy must be added {\em before} sending the packets out~\cite{??}. 
If fewer than $30\%$ packets are actually missing (\ie~\rate is overestimated), 
%it overestimates \rate (\ie fewer than $x\%$ packets are actually missing), 
video quality will be lower than if no redundancy is added.
If \rate is underestimated, the receiver must wait longer and request the sender to resend packets, until at least 70\% of packets are received.
%(\eg FEC with \fillme\% redundancy in Figure~\ref{fig:intro-example} when \rate exceeds \fillme\%).
%(\eg FEC with \fillme\% redundancy in Figure~\ref{fig:intro-example} when \rate is below \fillme\%).
Similarly, using an older frame as encoding reference lets the decoder safely skip a frame without affecting future frames (\eg~\cite{salsify}), but older reference frame also significantly lowers compression efficiency (needs more bits to reach same quality).
As a result, most real-time Internet video systems increase loss resilience only {\em after} packet loss has affected some frames~\cite{??,??,streamingcoding}. 
%, and leaving some frames unprotected against burst of packet loss. 
%it also significantly reduces compression efficiency as older frames are more different with the current frame.




Ideally, a better solution, which we refer to as {\em Data-Scalable} ({\em DS}) video delivery, 
should gracefully degrade in presence of packet loss, without compromising quality in absence of packet loss.
%should have decent compression efficiency in presence of loss of {\em any} packets. 
Concretely, it should 
{\em (i)} reach a quality close to that of a non-loss-resilient coding algorithm (such as H.265), if all packets are received; 
{\em (ii)} be able to decode a frame if {\em any} (non-empty) subset of packets of the frame is received (\ie no retransmission unless all data are lost); and 
{\em (iii)} achieve better quality, if one more packet is received.
%As we have seen, prior work falls short on at least one front.



This paper presents {\em \name}, a real-time video system that uses {\em  autoencoders (AE)} to realize data-scalable DS video delivery for the first time.
%which explores a new approach to DS video delivery by using {\em neural-net (NN) autoencoders}.
At a high level, an autoencoder uses an NN encoder to encode a frame to an {\em \aecode} (prior to entropy/arithemetic encoding), and uses an NN decoder to decode the tensor to a reconstructed frame. 
We choose autoencoders, not because off-the-shelf autoencoders are data-scalable (DS), but because of their unique properties that {\em could} enable DS coding. 
%\name is a particular design that harnesses these properties to enable DS coding.

First, the NN decoder of an autoencoder {\em could} reconstruct frames from an \aecode $z$, even if some data in $z$ is lost between the encoder and the decoder.
Like many NNs which have continuous derivatives, when $z$ changes to $z+\delta_z$, autoencoder's output will change from $y$ to $y+\delta_y$ and $\delta_y$ will grow proportional with $\delta_z$.
Moreover, NN decoder resembles the architecture of variational autoencoder (VAE) which are {\em generative} models that create high-quality images even from a random input.

That said, quality of existing autoencoders degrades quickly if more data is missing in an \aecode. 
This is because standard autoencoder training never trains autoencoders to decode a frame and subsequent frames in presence of substantial data loss on the encoder's output (\aecode).
\name uses a different autoencoder training process.
It applies random data erasures to each \aecode, which can simulate the effects of different \rates as explained shortly.
By varying the rate of data erasure (from 0\% to 90\%), 
%In other words, by training the NN encoder and NN decoder jointly, 
the new autoencoders not only learn how to compress frames efficiently but also how to be resilient to different \rates (see \S\ref{??} for details). 

\begin{comment}
\footnote{
The NN decoder architecture resembles a variational autoencoder (VAE), which creates realistic-looking images from a purely random tensor input!}
It can be intuitively understood that NNs having continuous derivatives, 
%\footnote{Encoder output is sometimes quantized, but quantization's effect on video quality is much less than data erasures caused by packet loss.}.


so that the decoder can loss between the encoder's output (\aecode) and the decoder's input, or handle long-term effect of packet loss. 
This is because in standard autoencoder training, the encoder output (\aecode) is almost always identical to the decoder input, and 
%have never seen any data erasure during the training. 
%To improve quality under data erasures, 
\end{comment}


%By training the NN encoder and NN decoder jointly, they {\em could} learn to reconstruct high-quality frames in presence of random data erasures on the autoencoder-output code.


Second, unlike traditional codecs, autoencoders do not have stringent structures or dependencies among the elements in the encoder output (\aecodes).
If we randomly set some elements of an \aecode to zeros (\ie random data erasures), the NN decoder can still reconstruct the whole frame with a decent quality.
Importantly, 
with more random data erasures on the {\em same} \aecode, video quality drops {\em gradually}, rather than abruptly as in FEC.
% with more zeroed random elements in autoencoder-returned code (\ie higher random erasure rate).

Thus, {\em if} packet loss is equivalent to random data erasure on \aecodes, video quality can degrade gracefully with higher \rates.
To this end, \name runs arithmetic coding differently than standard autoencoders.
It randomly partitions an \aecode into sub-tensors and runs arithmetic coding to compress each sub-tensor as a separately decodable packet, so missing a packet only erases a random portion of the \aecode.
However, naive per-packet arithmetic coding greatly inflates data size due to extra space needed to encode each packet's symbol distribution. 
%Standard arithmetic coding incurs excessive size overhead per packet due to the need to store each packet's data distribution.
To address it, \name carefully coarsens the granularity of symbol distributions, which reduces the overhead to store symbol distribution while preserving arithmetic coding's compression efficiency (see \S\ref{??} for details). 

\name also addresses several practical challenges associated with autoencoders, such as 
%\name also tackles other practical challenges, such as 
bitrate control, speeding up coding, and balancing the size of I-frames and P-frames.

\begin{comment}


First, autoencoder-output tensors do not impose stringent structures or dependencies among their elements. 
If we randomly set some elements of an autoencoder-output tensor to zeros (\ie random data erasures), the NN decoder can still reconstruct the whole frame with a decent quality (though with room for improvement).
More importantly, if we apply more random data erasures on the {\em same} autoencoder-output tensor, video quality will drop {\em gradually}, rather than abruptly as in FEC.
% with more zeroed random elements in autoencoder-returned code (\ie higher random erasure rate).
These suggest that video quality {\em could} degrade gracefully with higher \rates, {\em if} packet loss is equivalent to random data erasure on autoencoder-output tensor.

To this end, we change the arithmetic coding in standard autoencoders and classic codecs. 
%\name changes the arithmetic coding in standard autoencoders, which encodes the whole autoencoder-output tensor as a whole. 
%Instead, we 
\name first randomly partitions an autoencoder-output tensor into sub-tensors and runs arithmetic coding to compress each sub-tensor as a separately decodable packet.
Thus, missing a packet only erases a random portion of the elements in the tensor.
While seemingly straightforward, per-packet arithmetic coding, if done naively, will greatly inflate the coded data size due to extra space needed to encode the data distributions of different packets. 
%Standard arithmetic coding incurs excessive size overhead per packet due to the need to store each packet's data distribution.
To address it, \name carefully coarsen the granularity of the per-packet data distribution, which greatly reduces the overhead to store data distribution while preserving the efficiency of arithmetic coding (see \S\ref{??} for details). 
%the size overhead and efficiency of per-packet arithmetic coding 
%\jc{Yihua, a footnote on how does CABAC gets around it and why isn't it easily applicable to us?} 

Second, the NN decoder in an autoencoder could be used as a generative model. 
Theoretically, it can learn to act like a variational autoencoder (VAE), which can create realistic-looking high-quality images from a purely {\em random} tensor!
By training the NN encoder and NN decoder jointly, they {\em could} learn to reconstruct high-quality frames in presence of random data erasures on the autoencoder-output code.


Quality of existing autoencoders quality will degrade quickly with more random erasures.
This is because in standard autoencoder training, the encoder output is almost\footnote{Encoder output is sometimes quantized, but quantization's effect on video quality is much less than data erasures caused by packet loss.} always identical to the decoder input. 
%have never seen any data erasure during the training. 
%To improve quality under data erasures, 
\name uses a different autoencoder training process---it injecting random data erasures of various rates (from 0\% to 90\%) between the encoder and the decoder, which simulates the effects of different \rates.
In other words, the new autoencoders not only learn how to compress frames efficiently but also how to code them in a way resilient to different \rates (see \S\ref{??} for details). 

\end{comment}



%the rate of random erasures (more zeroed elements). 

%, which as explained in \S\ref{??} could mimic the effect of packet loss, the decoder can still decode the whole frame. 

\begin{comment}

because the elements in an autoencoder-output tensor have much less dependency among them.

To let autoencoders function under packet loss, we first change entropy encoding---instead of entropy coding the entire autoencoder-output tensor to a bitstream and then packetizing it to packets




\name chooses autoencoders, because the elements in an autoencoder-output tensor have much less dependency among them.
If we randomly select some elements of an autoencoder-returned code (\ie random erasures) and set them to zero, which as explained in \S\ref{??} could mimic the effect of packet loss, the decoder can still decode the whole frame. 
In contrast, missing information in H.264 
% will not render the whole frame undecodable. 
%does not have dramatic impact on the decoded video quality.
This is in contrast to SVC where any data loss on a low layer also affects higher layers.
Moreover, the impact of random erasures on video quality increases with the rate of random erasures (\eg more zeroed elements). 
In other words, unlike FEC needs to known \rate~{\em a priori}, the quality of autoencoders {\em could} degrade gracefully with more data loss.


We use autoencoders because they have two {\em potential} advantages.
First, there is little explicit dependency among the elements of an autoencoder-returned tensor. 
Thus, unlike in SVC where any data loss on a lower layer also affects higher layers, applying any random erasures (such as zeroing randomly selected elements) on an output tensor of an autoencoder will not have a dramatic impact on the decoded video quality.
%In other words, so the values in the tensor do not need to be received in specific order, like in SVC. 
Second, the impact of random perturbation on video quality {\em could} be further reduced by training the autoencoder to work under different random erasure rates. 
The resulting autoencoders might be better than FEC which only tolerates a pre-determined data loss rate.
%one autoencoder (a pair of NN encoder and NN decoder) could be trained to work under a {\em range} of data erasure rates and still achieve decent quality.


Yet, traditional autoencoders are ill-suited for real-time videos. 
Here, we highlight how \name addresses two specific challenges to enable autoencoder-based DS video delivery.



First, traditional autoencoder-returned code could be decoded in presence of data loss, but its quality will degrade quickly with more random erasures.
This is because in standard autoencoder training, the encoder output is almost\footnote{Encoder output is sometimes quantized (lower float precision), but quantization's effect on video quality is much less than data erasures caused by packet loss.} always identical to the decoder input. 
%have never seen any data erasure during the training. 
%To improve quality under data erasures, 
\name uses a different autoencoder training process---it injecting random data erasures of various rates (from 0\% to 90\%) between the encoder and the decoder, which simulates the effects of different \rates.
In other words, the new autoencoders not only learn how to compress frames efficiently but also how to code them in a way resilient to different \rates (see \S\ref{??} for details). 

Second, existing autoencoders and standard video codecs use arithmetic coding to compress all information of a frame to a single bitstream which will then be packetized. 
This means that any packet loss will render the data undecodable.
%If this bitstream is packetized, as done in conventional real-time video systems, any packet loss will render the data undecodable.
Instead, \name first randomly partitions the autoencoder-returned code to sub-tensors and then arithmetically codes each sub-tensor as a separate packet.
Though it sounds easy, per-packet arithmetic coding turns out to be challenging, since traditional arithmetic coding incurs excessive size overhead per packet due to the need to store each packet's data distribution. 
\name addresses it using a novel scheme to balance the size overhead and efficiency of per-packet arithmetic coding (see \S\ref{??}). 

\end{comment}

%As an end-to-end video coding framework, 
%\name also tackles other practical challenges, such as efficient bitrate control, speeding up of autoencoders, and balancing the size of I-frames and P-frames.


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/intro_loss_resilience_v1.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/psnr-vs-loss-example.pdf}
        %\includegraphics[width=0.85\linewidth]{figs/fig1-example.pdf}
%        \includegraphics[width=0.85\linewidth]{figs/fig1-example-osdi.pdf}
        \includegraphics[width=0.99\linewidth]{figs/fig1-example-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{Example results of \name's (a) more graceful degradation in presence of packet loss than prior solutions, and (b) better tradeoffs between video quality and tail frame delay, which corroborates the subjective rating of users.
         More results can be found in \S\ref{sec:eval}. 
%         \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
    \jc{TODO: add a horizontal line to indicate the quality of H.265}
         }
%    \tightcaption{Video quality vs. \rates of different video codecs when the actual encoded bitrate is 3.6 Mbps (which includes FEC redundancy if used.)
%    Quality of \name's autoencoder degrades gracefully with higher \rates. 
%%    achieves a smoother quality degradation as packet loss rate increases.
%    More results can be found in \S\ref{sec:eval}. 
%%    \jc{Yihua, can you replot the FEC lines to use the same color (w/ diff point/line types)}
%%    \jc{Yihua, can you add (DSC) next to our solution?}
%%    \jc{Yihua, can we also replace yellow with 50\% redundancy?}
%    %\jc{YIHUA, remember to add a line of 264 without loss, and remove the part of h264 when it's undecodable}\jc{set R-D optimization to "intra-MB insertion"}
%%    \jc{Yihua, can you explain why DSC is better than pre-trained model even under zero loss ratio?}
%%    \jc{Yihua, can you add a horizontal line to indicate the quality of H.265}
%    }
    \label{fig:intro-example}
    % \vspace{-0.5cm}
\end{figure}




We should also clarify what \name does {\em not} do.
\name decides {\em what} each packet contains, but it rate adaptation. 
Instead, it uses existing rate adaptation logics, such as GCC~\cite{??}, to decide the target bitrate of a frame and how fast to send its packets.
%, so that even if the selected bitrate overshoots the bandwidth, we can still obtain decent quality.
Moreover, \name aims at unicast video communication, rather than multi-party conferencing.

%Being a coding system, \name can work with existing congestion control (CC) logics---CC decides how fast to send packets, and \name decides {\em what} each packet contains.


To put it in context, \name is, to our best knowledge, the first to demonstrates that autoencoders could remarkably improve loss resilience in real-time communication.
Autoencoders have long been used in multimedia and data communication (see \S\ref{sec:related}) but mostly for better compression efficiency.
Swift and DeepFGS, for instance, use autoencoders to improve scalable video coding for on-demand videos~\cite{swift,??}. 
\name is also related to DeepJSCC which uses autoencoder to compress images (rather than real-time videos) in a way robust to link signal noises~\cite{??} (rather than packet loss).
%for compressing images and signals in wireless communication and 


\begin{comment}
To put \name in perspective, autoencoders have long been used in data communication~\cite{erpek2020deep} (see \S\ref{sec:related}).
\name, which can be seen as joint-source-channel coder, is similar 
%As a joint-source-channel coder, \name's autoencoder is similar 
in spirit to DeepJSCC which uses autoencoder to compress static images (rather than real-time videos) in a way robust to wireless signal noises~\cite{??} (rather than packet loss).
%for compressing images and signals in wireless communication and 
Recently, Swift uses autoencoders to improve scalable video coding (SVC) for on-demand videos~\cite{swift}. 
To our best knowledge, \name is the first video framework to demonstrates the potential of autoencoders to improve loss resilience in real-time communication.
\end{comment}

%Much remains unknown about the limits of autoencoders as a loss-resilient coding layer.

%To our best knowledge, \name is the first end-to-end autoencoder-based video system for loss-resilient real-time videos.
%that achieves stream real-time videos in a data-scalable fashion. 



%arising from training and using autoencoders in real-time video communication.

%Many aspects of \name are also inspired by prior work. 
%That said, \name, to our best knowledge, is the first to develop custom autoencoders that realize data-scalable video delivery.

%\name aims at unicast video sessions, rather than multi-party conferences. 
%It is also important that \name's autoencoders do {\em not} achieve better compression efficiency than recent heavily engineered video codecs, such as H.265. 
%Indeed, \name's video quality is still slightly lower than H.265 at the same bitrate. 

We have implemented and evaluated \name in two aspects (Figure~\ref{fig:intro-example} gives an example). 
First, on various video content, \name's quality degrades more gracefully under packet loss than other loss-resilient coding.
%, without much compromise on quality in absence of packet loss. 
That said, in absence of packet loss, \name's quality is slightly lower than H.265 at the same bitrate. \jc{need to update this}
% which is comparable or less than adding 10\% FEC redundancy. 
%does {\em not} outperform the latest heavily engineered video codecs in quality---indeed, \name's video quality is slightly lower than H.265 at the same bitrate. 
Second, using real-world network traces and a packet-level simulator, we show that \name significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to the most competitive baselines which still have to retransmit packets or skip frames.
This greatly decreases video stuttering and skipped frames---our user study confirms that \name has much higher average subjective rating by users than the most competitive baselines.

\begin{comment}
Using real-world and synthetic network traces and a wide range of videos, we show that \name's autoencoder has a more graceful quality degradation under packet loss than baseline loss-resilient video codecs.
%, without sacrificing video quality in absence of packet loss 
(Figure~\ref{fig:intro-example} gives an example).
When comparing \name with the baselines with the same CC logic (\eg GCC~\cite{??} and Salsify-CC~\cite{??}), \name significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile) compared to prior work which has to retransmit packets or skip frames, with the comparable video quality.
To put it in perspective, \name significantly decrease the frames that arrive after user-perceivable delay (\eg 200ms for video calls) and reduces video stuttering.
\end{comment}

%Our results show that while \name's compression efficiency is slightly worse than heavily engineered video codecs, it significantly reduces {\em tail} frame delay (by 2$\times$ at the 95th percentile when prior work has to retransmit packets or skip frame), with the marginally lowered video quality.
%To put it in perspective, \name can significantly reduce the chance that frames arrive after user-perceivable delay (\eg 200ms for video conferencing) and improve playback smoothness (higher frame rate).

%\jc{ae has caveats (size, speed, efficiency). }
%\jc{this paper above all shows a new design space}

\textbf{This work does not raise any ethical issues.}






%unlike SVC, the output tensor of an autoencoder does {\em not} impose a hierarchical structure among its elements, so the values in the tensor do not need to be received in specific order, like in SVC. 
%Instead, randomly perturbing a tensor in the new embedding space, such as zeroing any $\alpha\%$ of a tensor's elements, will have only a {\em limited} impact (proportional to $\alpha\%$)  on the quality of the decoded frame.
%Second, unlike FEC which only tolerates a pre-determined data loss rate, one autoencoder (a pair of NN encoder and NN decoder) could be trained to achieve desirable quality under a {\em range} of data erasure rates. 

%To be specific, each frame is supposed to be decoded at a fixed interval after the last frame was decoded, and 
%
%a packet associated with a frame will delay the rendering of a 
%To be more specific, we call a packet as a {\em missing packet}, if it arrives after when the frame it belongs to should be decoded (\eg 40ms after the last frame is decoded under 25fps), and we refer to the fraction of data in missing packets of a frame as {\em data missing rate} or \rate. 
%Note that a missed packet can be lost or delayed.






==> sections/old/motivate-nsdi-v1.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\tightsection{Background}
\label{sec:motivate}

%Video coding has a rich history of research and it is hard to fit a comprehensive overview in a limited space.
%Nonetheless, 

\vspace{0.2cm}

\tightsubsection{Real-time video coding}
\label{subsec:background}

To help explain \name's design, we first introduce some key concepts of real-time video coding relevant to this work. 
%before explaining the need for a different approach (\S\ref{subsec:ds},\ref{subsec:prior}). 
%The video sender runs a rate adaptation logic to dynamically set the frame rate and bitrate of the encoded video.
The sender encodes the video at a given frame rate and bitrate, \eg
%A video stream is encoded at certain frame rate and bitrate, both are controlled by an adaptation logic in the player.
at a frame rate of 25~fps (frames per second) and bitrate of 3~Mbps, the encoder should on average generate a 15~KB frame every 40~ms.
%, though the actual frame size varies.
%depends on the {\em type} of a frame
A video stream consists of multiple groups of consecutive frames (called a group of pictures or GoP), and each GoP starts with an I-frame (or key-frame) followed by P-frames (or inter-frames)\footnote{On-demand videos also use B-frames (bidirectional predicted frames), which 
% are smaller than P-frames since they 
refer to both past and future P-frames. However, real-time video rarely uses B-frames in order to render frames as soon as possible.
% However, to render frames as soon as possible, real-time video rarely uses B-frames~\cite{??}, since they refer to future frames to be decoded.
}.
% and B-frames (bidirectional predicted frames). 
I-frames are encoded and decoded independently without referring to other frames, so they have a bigger size than P-frames, which only encode the differences with other {\em reference} frames.
In real-time videos, most frames are P-frames to reduce the frame size.
Figure~\ref{fig:codec-workflow} shows the workflow of encoding a P-frame. 
Given a new frame, the encoder 
(1) calculates its motion vectors (MVs) and residuals per macroblock (MB), each of 4×4,8×8,\dots, 
(2) then transforms and quantizes them, 
(3) entropy encodes the transformed data, 
(4) splits the entropy-coded data into packets, and 
(5) sends them out by a congestion control logic, such as GCC~\cite{carlucci2016analysis} used by WebRTC. 
%To encode a frame, the encoder first calculates the differences (\eg motion vectors and residuals) among macroblocks (4×4,8×8,…4\times4,8\times8,\dots) in the current frame and reference frames (or within an I-frame),  then transforms and quantizes these differences to a more compact form, and finally losslessly encodes the data using arithmetic coding. 
%The entropy-encoded data is then packetized and sent out by the transport layer, which tries to deliver as many packets as possible 
%% (though not always all packets) 
%to the receiver by the time when the frame is decoded.
%algorithm decides how fast to send a frame's packets, 
%in order to ensure enough data be delivered to the receiver when the frame is decoded. 
Similarly, the receiver depacketizes and decodes the received data to 
% runs a reverse process (depacketization and decoding) to 
reconstruct each frame from received packets. 

% Thus, I-frames are used infrequently (\eg only when content shifts dramatically) with 10s or more P-frames between two I-frames.

%and each GoP consists of 10s to 100s of P-frames. 
%I-frames are encoded independently, and P-frames and B-frames encode the differences between them and other {\em reference} frames: a P-frame refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames. 
%Importantly, to render each frame as soon as its packets are received, real-time videos almost never use B-frames which refer to future frames~\cite{??}. 
%Since I-frames do not need other frames to decode, their sizes in standard video codecs are much bigger than B-/P-frames, so I-frames are typically used only when content shifts dramatically and each GoP consists of 10s to 100s of frames. 

%As we will see in \Sref{??}, our new video coding system follows the same frame definitions, though the optimal GoP size will be much smaller. 


%Different {\em frame types} often have different frame sizes.
%An I-frame (intra-frames) is encoded independently and is followed by P-frames (predicted frames) and B-frames (bidirectional predicted frames), each of which encodes the differences between it and some other frames.
%A frame used as a reference for decoding other frames is called a {\em reference} frame: a P-frame only refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames.
%Since I-frames do not need other frames to decode, their sizes are typically bigger than B-/P-frames.


%In real-time videos, to render each frame as soon as its packets are received, B-frames, which refer to future frames, are rarely used~\cite{??}. 
%This precludes several loss-resilient techniques such as B-frame skipping (see \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{??}).

%, and  , each encoding the difference with the previous and future I-/P-frames.
%Thus, I-frames are typically bigger than P-frames and B-frames, but decoding I-frames does not depend on any other frame, while decoding P-frames or B-frames must refer to other frames. 
%fewer other frames than decoding a B-frame.


%A decoded frame is put in a very short {\em buffer} before playing to conceal transient latency jitters.
% (due to queuing or retransmits).


\begin{figure}[t!]
         \hspace{-0.2cm}
        \includegraphics[width=1.05\linewidth]{figs/codec-workflow-new.pdf}
         \label{fig:}
         \tightcaption{A typical workflow to encode a frame.
         \fyy{I prefer not to use "tightcaption" or italics for the caption. Regular USENIX template looks much nicer. Leave ample vertical space after each figure.}}
    \label{fig:codec-workflow}
    % \vspace{-0.25cm}
\end{figure}

A key metric in real-time video is frame delay, the time between the encoding and the rendering of a frame.
To reduce frame delay, real-time video clients commonly make two choices~\cite{10.1145/3410449,salsify} that are different from streaming videos, such as Netflix, ESPN Live: %\footnote{\jc{any exceptions?}}:
% that affect the requirements of a desirable video coding scheme.
\begin{packeditemize}
\item Packets of a frame are sent in a burst (without waiting for acks), and %without waiting for acknowledgement.
{\em any} packets in the middle of a frame could be delayed or dropped when the receiver tries to decode the frame.
By contrast, streaming videos are sent by chunks (each consisting of 10's to 100's of frames) over the HTTP/TCP protocol.
\item The buffer in real-time videos is much {\em shorter} (\eg 10's~ms) than that of on-demand videos, whose buffer is over 10 seconds, and live broadcast videos, whose buffer is still several seconds. %\amz{I swapped the "10s" in this section to "10's" to reduce confusion, please revert if undesired. }
% This short buffer often cannot conceal retransmission delay in long-latency networks.
%With a short buffer, any missing packet might delay a frame longer than the jitter buffer can conceal.
\end{packeditemize}

Congestion control and bitrate adaptation logics are often used by video clients employ to cope with bandwidth fluctuation, such as GCC~\cite{carlucci2016analysis},  Salsify~\cite{salsify}, and NADA~\cite{zhu2016nada}.
Ideally, these adaptation logics should reduce packet loss.
However, because it is difficult to predict bandwidth drops or packet loss in advance, they cannot completely eliminate packet loss.
\name is complementary to this line of work, and our results show \name improves loss resilience under different congestion control logics (Figure~\ref{fig:appgcc-delay-simulation}). %\yc{is it okay to put the forward reference to appendix here?}

\passed{\jc{need to smooth the text here}}
%Here, we define {\em packet loss} on a given frame as any packets not received before the receiver decodes the frame. \yc{the prior sentence is replicated from intro}
%, \eg every 50ms at 20 frames per second (fps).
The packet loss, defined {\em per frame as any packets not received before the receiver decodes the frame},
can be consecutive or random and can result from packet drops or latency jitter. 
This definition is consistent with recent papers~\cite{rudow2023tambur,cheng2023abrf,holmer2013handling}. 
It is important to clarify that our notion of packet loss rate is {\bf \em not} network-level loss rate (which rarely exceeds 1\%). 
Even if a packet is not dropped, it can {\em still} be counted as a packet loss, if it arrives too late. 
Therefore, it is {\em not rare} for real-time video clients to have a high (over 50\%) packet loss rate on some frames, even if the network has a very low packet loss rate.
The high packet loss rate per frame also corroborates recent papers in this space~\cite{cheng2023abrf,rudow2023tambur,cheng2020deeprs}.
\fyy{avoid over-emphasizing in this paragraph; use italics and bold only when necessary}


\tightsubsection{Related work}
\label{subsec:related}

As retransmission delay is difficult to conceal by the buffer, particularly in long-latency networks, many schemes for error resilience have been studied. 
\passed{\jc{Yihua, please add more citations. }}
\passed{\jc{this section should also be made more technical. Yihua, ping me if you can spend some time on this part}\yc{added a bit words, but maybe not enough}}


\myparashort{Forward error coding}adds redundancy to the encoded data at the sender before sending to the network. 
This is also known as error-resilient channel coding. 
Examples include FEC, Reed-Solomon code, LDPC and fountain codes~\cite{mackay1997near,mackay2005fountain}, rateless coding~\cite{castura2006rateless}, streaming code~\cite{badr2017fec,rudow2023tambur}, and recent ones based on DNNs~\cite{7926071, 8919799}.
Moreover, video codecs also supports data partitioning and apply unequal protection using forward error correction (also known as UEP~\cite{zhao2010rd, abdallah2019h}), \ie having higher redundancy for more important information such as codec configuration and frame metadata.
However, these schemes need to know how many packets will arrive before sending the data out. 
If the loss rate is underestimated, the redundancy will be insufficient to tolerate missing packets and the receiver must either wait for more packets or retransmitted packets.
On the other hand, once the received packets are decodable, receiving more packets does not improve the quality, so even if all packets are received, quality will be lower than without redundancy. 




\myparashort{Postprocessing error concealment}reconstructs missing data in lost packets on the decoder side by solving the following two problems.

First, decoding the partially received frame requires partitioning a video frame into independently decodable packets.
Modern video encoders use a few techniques to achieve this, including \texttt{INTRA}-mode macroblock encoding~\cite{660830}, slice interleaving~\cite{ismaeil2000efficient} or flexible macroblock ordering~\cite{lambert2006flexible} 
However, such methods limit the encoder's ability to exploit redundancies across neighboring MBs, because adjacent MBs need to be split into different packets in a checkerboard manner~\cite{kumar2006error, lambert2006flexible} or based on ROI detection~\cite{tan2011new}, or be encoded by \texttt{INTRA} mode.
Therefore, these methods reduce the compression efficiency, and the encoded frame size typically inflates by 10\%-50\%~\cite{kumar2006error, wenger2002scattered, 4494082, dhondt2004flexible}. 

% First, to make the partially received packets decodable, some macroblocks (MBs) need to be set in \texttt{INTRA} mode~\cite{660830, lambert2006flexible}, and adjacent MBs need to be split into different packets in a checkerboard manner~\cite{kumar2006error, lambert2006flexible} or based on ROI detection~\cite{tan2011new}. This reduces the compression efficiency, 
% %limits the encoder's ability to exploits redundancies across neighboring MBs, so 
% and the encoded frame size typically inflates by 10\%-50\%~\cite{kumar2006error, wenger2002scattered, 4494082, dhondt2004flexible}. 
% INTRA mode, FMO, slice interleaving and the size inflation problem

Second, the receiver needs to reconstruct data in the lost packets after decoding the received packets. 
Such reconstruction can be done by classic heuristics (\eg Motion vectors interpolation~\cite{kolkeri2009error, zhou2010efficient, wang2013novel} and Intra-block refreshing~\cite{kumar2006error} in H.264) and NN-based inpainting (\eg~\cite{xiang2019generative,kang2022error, sankisa2018video, mathieu2015deep,reparo}).
Recent works~\cite{??, reparo} also try to use vision transformers~\cite{dosovitskiy2020image, arnab2021vivit} to directly predict the missing values in the lost packets before decoding the frame.
However, since the encoder in these schemes is agnostic to the decoder post-processing, it will aggressively compress each frame, and as a result, each packet contains little redundant information to help reconstruct motion vectors or residuals in other packets.
Thus when a packet is lost, the task of in-painting or reconstruction must guess the missing data (similar to constrained hallucination~\cite{liu2020brief, santos2020single}).
Even recent techniques still see a notable quality drop (\eg PSNR drops from 38 dB to 25 dB at 20\% packet loss~\cite{nam2020novel}). 
In contrast, \name jointly trains the NN encoder and NN decoder, which allows the encoder to produce data that is easier to reconstruct accurately when partially received. 


% Motion-vector recovery techniques, for instance, recover the motion vector (MV) of an MB~\cite{yihua?} by searching surrounding MBs whose MVs are not lost, and copying the one that causes least pixel differences (``glitches'')~\cite{??}. 
%The encoder splits each frame into partitions (also known as slices) and encodes each partition separately. 
% Modern encoders can split each frame into partitions and encode each partition separately (\eg slice interleaving~\cite{ismaeil2000efficient} or flexible macroblock ordering~\cite{lambert2006flexible} technique used in H.264). 
% The receiver first decodes the partitions (motion vectors and residuals) in the received packets  and use them to reconstruct data in the lost packets. 
% Such reconstruction can be done by classic heuristics (\eg Motion vectors interpolation~\cite{kolkeri2009error, zhou2010efficient, wang2013novel} and Intra-block refreshing~\cite{kumar2006error} in H.264) and NN-based inpainting (\eg~\cite{xiang2019generative,kang2022error, sankisa2018video, mathieu2015deep,reparo}).
% However, it has two problems. 
% First, to make the partially received packets decodable, some macroblocks (MBs) need to be set in \texttt{INTRA} mode~\cite{660830, lambert2006flexible}, and adjacent MBs need to be split into different packets in a checkerboard manner~\cite{kumar2006error, lambert2006flexible} or based on ROI detection~\cite{tan2011new}. This reduces the compression efficiency, 
% %limits the encoder's ability to exploits redundancies across neighboring MBs, so 
% and the encoded frame size typically inflates by 10\%-50\%~\cite{kumar2006error, wenger2002scattered, 4494082, dhondt2004flexible}. 
% Moreover, since the encoder in these schemes is agnostic to the decoder post-processing, it will aggressively compress each frame, and as a result, each packet contains little redundant information to help reconstruct motion vectors or residuals in other packets.
% Thus when a packet is lost, the task of in-painting or reconstruction must guess the missing data (similar to constrained hallucination~\cite{liu2020brief, santos2020single}).
% Even recent techniques still see a notable quality drop (\eg PSNR drops from 38 dB to 25 dB at even 20\% packet loss~\cite{nam2020novel}). 
% \passed{\jc{Yihua, please read the sentences above. see if the new text makes sense to you}\yc{yeah!}}
% % Moreover, the encoder is agnostic to the post-processing, so the encode data (encoded motion vectors and residuals) contains little redundant information.
% % When some blocks are missing, the in-painting task is inherently ``underspecified'' (\ie reconstruction is error-prone). 
% \passed{\amz{This sentence is a bit vague and hard to follow. I also am not convinced it is needed, unless this "underspecification" of the inpainting comes up later. } }
% In contrast, \name jointly trains the NN encoder and NN decoder, which allows the encoder to produce data that is easier to be reconstructed accurately when partially received. 
% % Moreover, \name's encoded file size does not grow with more packets. 
% \passed{\yc{to make it clear: empirically, even the sota dnn method is not working well + reasoning (citation): inpainting is hallucinating}
% \yc{encoder is agnostic to loss/inpainting, so every bit have some information. if packet is lost, the information is not recoverable. inpainting is trying to generate the missing information (movement) by hallucinating}}

\mypara{Other schemes}
Several other techniques might help mitigate the impact of packet loss, but their primary goals are not loss resilience, so they are less resilient to packet loss than the aforementioned schemes. 
But for completeness, we discuss some notable schemes here and also qualitatively compare \name against several of them in \S\ref{sec:eval}.


Scalable video coding (SVC)~\cite{schwarz2007overview, schierl2007mobile, swift} and fine-granularity scalability (FGS)~\cite{li2001overview,ma2022deepfgs} 
%\amz{same citation twice here}
 optimize the notion of rate-distortion (RD) tradeoff---video quality achieved by a single encoded bitstream under different received bitrates.
%Recent work also shows that neural encoders can improve SVC compression~\cite{swift}.
SVC encodes a video in multiple quality layers and sends data {\em layer by layer}.
This works well for on-demand videos~\cite{swift,grad}, but real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{subsec:background}), so a packet loss can occur to any layer, and a new packet may not always improve quality, if the lower layers are not fully received.
For this reason, SVC is rarely used to improve unicast real-time video (though it is used widely by multicast videos to serve users with heterogeneous network capacities~\cite{schierl2007mobile}).

%so that each newly received packet (or layer) will incrementally improve quality. 
%However, because it imposes a hierarchical order among the packets of a frame, 
%one missing packet can affect all higher quality layers, even if more packets are received in the higher quality layers.
%Though sending each layer reliably one by one is possible in on-demand videos~\cite{swift,grad}, real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{subsec:background}), so packet loss can affect any layer.
%As a result, SVC is rarely used to improve unicast real-time video (though it is used widely by multicast videos to serve users with heterogeneous network capacities~\cite{schierl2007mobile}).


Frame skipping might be another option if other error concealment schemes are not available.
%The encoder and decoder can work jointly to decide when skipping a frame does not hurt quality and the decoding states. 
For instance, Salsify~\cite{salsify} uses an older but reliably received frame, instead of the last frame, as the reference frame, so the decoder can safely skip a loss-affected frame without hurting subsequent frames.
However, it needs more bits to encode the same quality than using the last frame (which has a much smaller difference from the current frame) as the reference frame
(\eg the P-frames between every other frame are 40\% greater in size than between two consecutive frames).
Long-term reference frame (LTR) technique~\cite{zhang2008error} makes each P-frame individually decodable if the long-term reference is received, no matter whether there is packet loss in between or not. 
However, it shares a similar problem of large size overhead as Salsify.
Voxel~\cite{voxel} lets the decoder skip a loss-affected frame if the encoder indicates that skipping the frame does not affect video quality.
It works well for on-demand videos where B-frames can be safely skipped, and the impact of a skipped frame will stop at the next chunk within a few seconds. 
Unfortunately, neither apply to real-time videos. 


Deep learning has long been used in multimedia. 
It has been used to improve compression efficiency (\eg~\cite{dvc,elf,hu2021fvc,swift, NEURIPS2021_96b250a9}), enhance quality (\eg super resolution~\cite{sivaraman2022gemino,kim2020neural,neuroscaler}), scalable video coding (\eg~\cite{swift,ma2022deepfgs}) and postprocessing error concealment (\eg~\cite{reparo, xiang2019generative, kang2022error, sankisa2018video, mathieu2015deep}).
However, the fundamental limitations of these approaches remain despite the use of deep learning.

Loss resilience has also been studied under specific assumptions, such as availability of multiple paths~\cite{meng2022achieving}, early retransmission driven by router feedback~\cite{zuo2022deadline}, and low-latency networks~\cite{ray2022sqp}.
We do not make special assumptions in this work.




\tightsubsection{Neural video codec background}
\label{subsec:ae-background}

% \jc{this section needs more work}

%\jc{refer to fig~\ref{fig:dvc-arch}}


Our work is based on neural video codecs (\textbf{NVC}s),  which use learned neural networks (\textbf{NN}s) instead of handcrafted logic, to encode and decode video frames.
NVCs have recently reached competitive and even better compression efficiency than traditional video codecs. 
Several factors contribute to this advance.
First, rather than encoding a frame with a monolithic NN, recent NVCs take advantage of logical components commonly found in classic video codecs (\S\ref{subsec:background}),
% \footnote{For this reason, most autoencoder-based video coding focuses on inter-frames, the most common frame type in real-time videos. Our work also focuses on inter-frame coding and will include I-frame in \S\ref{subsec:protocol}.}, 
such as motion estimation, compensation, and transformation compression of residual and motion vectors.
Then they replace the handcrafted heuristics of classic codecs with NNs that can learn more complex algorithms from data.
Second, these NVCs are trained on a large corpus of videos (\eg Vimeo-90K~\cite{vimeo-dataset}), so their compression efficiency can reasonably generalize across a variety of video content (which we also observe in our evaluation \S\ref{sec:eval}).
For these reasons, NVCs attract increasing attention in the multimedia community~\cite{dvc, swift, hu2021fvc}.

% % (We will discuss I-frame in \S\ref{subsec:protocol}, and B-frames are rarely used in real-time videos~\cite{ffmpegstreaming}.)
% It is comprised of steps (\eg motion and residual estimation) typically found in a traditional video codec (\S\ref{subsec:background}) but  uses NNs to replace
% %Most recent video autoencoders~\cite{??,??,??} combine useful concepts from traditional codecs (\eg motion vectors and residuals) and replace 
% handcrafted heuristics for motion estimation, compensation, and \st{transformation} \edit{compression} of residual and motion vectors.
% %, and they achieve compression efficiency comparable to recent video codecs.
% %, and achieve comparable compression efficiency as recent compression algorithms.

%\mypara{Limitations}



\begin{figure*}[t!]
    \centering
         \centering
        %\includegraphics[width=0.97\linewidth]{figs/dvc-arch-v3.pdf}
        % \includegraphics[width=0.93\linewidth]{figs/dvc-arch-v3.pdf}
        %\includegraphics[width=0.93\linewidth]{figs/dvc-arch-v4.pdf}
        \includegraphics[width=0.93\linewidth]{figs/workflow-new.pdf}
    \tightcaption{Workflow of \name's neural video codec \yc{their might be a better name other than "frame prediction". If we changed the name, remember to also change the corresponding locations in section 4!}}
    \label{fig:dvc-arch}
\end{figure*}

Our work adopts the DVC architecture~\cite{dvc}, a popular NVC. %(depicted in Figure~\ref{fig:dvc-arch}).
Two properties of NVCs make them particularly suitable for loss resilience.
\begin{packeditemize}

\item {\bf Generative:} The decoding part in NVCs, such as DVC, can {\em generate} frames with any vector in the encoded latent space as input. 
In other words, it can decode not only the encoder's output but also other vectors that look similar to the encoder's output. 
This means that if we randomly perturb the values in the encoder output (such as zeroing some random values or adding a Gaussian noise), the NN decoder can still successfully decode the frame, though the quality will have a non-trivial drop compared to without the perturbation.
\yc{We need to change this, this paragraph sounds like "decoder itself can already provide pretty good loss resilience", which is not ture}

\item {\bf Learnable:} NVCs can decode any vector in the encoded latent space but the decoded quality can be quite poor. 
Fortunately, the encoder and the decoder are {\em learnable} NNs that can be trained to optimize decoded quality in the presence of perturbations like random zeroing. 
For instance, the decoder can learn to be less sensitive to perturbed values, and the encoder can learn to add slight redundancy that helps the decoder accurately correct perturbed values.

\end{packeditemize}

Nonetheless, existing NVCs as-is still lack tolerance to packet loss for two reasons.
%still requires traditional schemes (like FEC) to handle packet loss. 
%Their lack of packet loss tolerance is due to two reasons.
First, the standard NVCs training implicitly assumes that the encoder's output equals the decoder's input,
% \footnote{A recent work~\cite{??,??} adds Gaussian random noise\jc{check!} between the encoder and decoder to simulate wireless signal noise, but this is different from packet loss which masks a fraction of the data.}, 
so it does not prepare the NVC to handle data loss between the encoder and decoder. 
Second, entropy encoding used in NVCs compresses the whole encoder output as a single bitstream, so any data loss will render it undecodeable.

\name is an attempt at transforming NVCs to be resilient to packet loss at different rates.
Our work is related to an emerging line of work on deep joint source-channel coding~\cite{kurka2020deepjscc, pmlr-v97-choi19a, bourtsoulatze2019deep} which trains an NVC to code images in a representation that is both compact and robust to signal noises.
\name differs on two key fronts. 
First, they target physical layer protection against signal noises.
% is different from (and complementary to) transport-/application-layer protection against packet losses. 
While physical-layer noises can be modeled as differentiable linear transformations (as in~\cite{bourtsoulatze2019deep,gunduz2019machine}), packet drops are not naturally differentiable and need to be handled differently. % (see \S\ref{subsec:sim-losses}). 
Second, unlike compressing individual images, frames in a streaming video cannot be treated separately, otherwise, any error on one frame may propagate to future frames. 


\tightsubsection{Summary}

In summary, traditional error-resilient methods fall short to optimize quality under a range of packet loss rates.
On one hand, encoder-based forward error coding (FEC) optimizes quality only under a pre-determined loss rate, and decoder-based postprocessing for error concealment suffers suboptimal quality under high loss rates.
On the other hand, NVCs can potentially tolerate data perturbation at any rate, but they cannot tolerate packet loss.

\begin{comment}

By contrast, a better coding scheme should optimize quality under different packet loss rates. 
We call it {\em data-scalable (DS) coding}.
With the same encoding of each frame, DS coding obtains quality similar to the classic codec (H.265) used in WebRTC without FEC when there is no packet loss; and with higher packet loss rates, the quality gradually degrades but is still better than state-of-the-art loss-resilient schemes.
In the next two sections, we will describe an autoencoder-based solution to approximate the effect of DS coding.

\end{comment}

%the aforementioned solutions either sacrifice the quality in absence of packet loss or fail to get decent quality in presence of high packet loss rates.
%As we will see, \name shows a more desirable relationship between quality and packet loss rate.





==> sections/old/motivate.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\tightsection{Background}
\label{sec:motivate}

%Video coding has a rich history of research and it is hard to fit a comprehensive overview in a limited space.
%Nonetheless, 

\vspace{0.2cm}

\tightsubsection{Real-time video coding}
\label{subsec:background}

To help explain \name's design, we first introduce some key concepts of real-time video coding (\S\ref{subsec:background}) relevant to this work. 
%before explaining the need for a different approach (\S\ref{subsec:ds},\ref{subsec:prior}). 
%The video sender runs a rate adaptation logic to dynamically set the frame rate and bitrate of the encoded video.
The sender encodes the video at a given frame rate and bitrate, \eg
%A video stream is encoded at certain frame rate and bitrate, both are controlled by an adaptation logic in the player.
at a frame rate of 25fps (frames per second) and bitrate of 3Mbps, the encoder should on average generate a 15KB frame every 40ms.
%, though the actual frame size varies.
%depends on the {\em type} of a frame
A video stream consists of multiple groups of consecutive frames (called a group of pictures or GoP), and each GoP starts with an I-frame (or key-frame) followed by P-frames (or inter-frames)\footnote{On-demand videos also use B-frames (bidirectional predicted frames), which 
% are smaller than P-frames since they 
refer to both past and future P-frames. However, real-time video rarely uses B-frames in order to render frames as soon as possible.
% However, to render frames as soon as possible, real-time video rarely uses B-frames~\cite{??}, since they refer to future frames to be decoded.
}.
% and B-frames (bidirectional predicted frames). 
I-frames are encoded and decoded independently without referring to other frames, so they have a bigger size than P-frames, which only encode the differences with other {\em reference} frames.
In real-time videos, most frames are P-frames to reduce the frame size.
Figure~\ref{fig:codec-workflow} shows the workflow of encoding a P-frame. 
Given a new frame, the encoder 
(1) calculates its motion vectors (MVs) and residuals per macroblock (MB), each of 4×4,8×8,\dots, 
(2) then transforms and quantizes them, 
(3) entropy encodes the transformed data, 
(4) splits the entropy-coded data into packets, and 
(5) sends them out by a congestion control logic, such as GCC~\cite{carlucci2016analysis} used by WebRTC. 
%To encode a frame, the encoder first calculates the differences (\eg motion vectors and residuals) among macroblocks (4×4,8×8,…4\times4,8\times8,\dots) in the current frame and reference frames (or within an I-frame),  then transforms and quantizes these differences to a more compact form, and finally losslessly encodes the data using arithmetic coding. 
%The entropy-encoded data is then packetized and sent out by the transport layer, which tries to deliver as many packets as possible 
%% (though not always all packets) 
%to the receiver by the time when the frame is decoded.
%algorithm decides how fast to send a frame's packets, 
%in order to ensure enough data be delivered to the receiver when the frame is decoded. 
Similarly, the receiver depacketizes and decodes the received data to 
% runs a reverse process (depacketization and decoding) to 
reconstruct each frame from received packets. 

% Thus, I-frames are used infrequently (\eg only when content shifts dramatically) with 10s or more P-frames between two I-frames.

%and each GoP consists of 10s to 100s of P-frames. 
%I-frames are encoded independently, and P-frames and B-frames encode the differences between them and other {\em reference} frames: a P-frame refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames. 
%Importantly, to render each frame as soon as its packets are received, real-time videos almost never use B-frames which refer to future frames~\cite{??}. 
%Since I-frames do not need other frames to decode, their sizes in standard video codecs are much bigger than B-/P-frames, so I-frames are typically used only when content shifts dramatically and each GoP consists of 10s to 100s of frames. 

%As we will see in \Sref{??}, our new video coding system follows the same frame definitions, though the optimal GoP size will be much smaller. 


%Different {\em frame types} often have different frame sizes.
%An I-frame (intra-frames) is encoded independently and is followed by P-frames (predicted frames) and B-frames (bidirectional predicted frames), each of which encodes the differences between it and some other frames.
%A frame used as a reference for decoding other frames is called a {\em reference} frame: a P-frame only refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames.
%Since I-frames do not need other frames to decode, their sizes are typically bigger than B-/P-frames.


%In real-time videos, to render each frame as soon as its packets are received, B-frames, which refer to future frames, are rarely used~\cite{??}. 
%This precludes several loss-resilient techniques such as B-frame skipping (see \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{??}).

%, and  , each encoding the difference with the previous and future I-/P-frames.
%Thus, I-frames are typically bigger than P-frames and B-frames, but decoding I-frames does not depend on any other frame, while decoding P-frames or B-frames must refer to other frames. 
%fewer other frames than decoding a B-frame.


%A decoded frame is put in a very short {\em buffer} before playing to conceal transient latency jitters.
% (due to queuing or retransmits).


\begin{figure}[t!]
    \centering
         \centering
         %\includegraphics[width=0.85\linewidth]{figs/fig2-workflow-newplaceholder.pdf}
        \includegraphics[width=0.77\linewidth]{figs/fig2-workflow-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{A typical workflow to encode a frame.}
    \label{fig:codec-workflow}
    \vspace{-0.25cm}
\end{figure}

A key metric in real-time video is frame delay, the time between the encoding and the rendering of a frame.
To reduce frame delay, real-time video clients commonly make two choices~\cite{10.1145/3410449,salsify} that are different from streaming videos, such as Netflix, ESPN Live: %\footnote{\jc{any exceptions?}}:
% that affect the requirements of a desirable video coding scheme.
\begin{packeditemize}
\item Packets of a frame are sent in a burst (without waiting for acks), and %without waiting for acknowledgement.
{\em any} packets in the middle of a frame could be delayed or dropped when the receiver tries to decode the frame.
By contrast, streaming videos are sent by chunks (each consisting of 10's to 100's of frames) over the HTTP/TCP protocol.
\item The buffer in real-time videos is much {\em shorter} (\eg 10's~ms) than that of on-demand videos, whose buffer is over 10 seconds, and live broadcast videos, whose buffer is still several seconds. %\amz{I swapped the "10s" in this section to "10's" to reduce confusion, please revert if undesired. }
% This short buffer often cannot conceal retransmission delay in long-latency networks.
%With a short buffer, any missing packet might delay a frame longer than the jitter buffer can conceal.
\end{packeditemize}

Congestion control and bitrate adaptation logics are often used by video clients employ to cope with bandwidth fluctuation, such as GCC~\cite{carlucci2016analysis},  Salsify~\cite{salsify}, and NADA~\cite{zhu2016nada}.
Ideally, these adaptation logics should reduce packet loss.
However, because it is difficult to predict bandwidth drops or packet loss in advance, they cannot completely eliminate packet loss.
\name is complementary to this line of work, and our results show \name improves loss resilience under different congestion control logics (Figure~\ref{fig:appgcc-delay-simulation}). %\yc{is it okay to put the forward reference to appendix here?}

\passed{\jc{need to smooth the text here}}
%Here, we define {\em packet loss} on a given frame as any packets not received before the receiver decodes the frame. \yc{the prior sentence is replicated from intro}
%, \eg every 50ms at 20 frames per second (fps).
The packet loss, defined {\em per frame as any packets not received before the receiver decodes the frame}, can be consecutive or random and can result from packet drops or latency jitter. 
This definition is consistent with recent papers~\cite{rudow2023tambur,cheng2023abrf,holmer2013handling}. 
It is important to clarify that our notion of packet loss rate is {\bf \em not} network-level loss rate (which rarely exceeds 1\%). 
Even if a packet is not dropped, it can {\em still} be counted as a packet loss, if it arrives too late. 
Therefore, it is {\em not rare} for real-time video clients to have a high (over 50\%) packet loss rate on some frames, even if the network has a very low packet loss rate.
The high packet loss rate per frame also corroborates recent papers in this space~\cite{cheng2023abrf,rudow2023tambur,cheng2020deeprs}.



\tightsubsection{Related work}
\label{subsec:related}

As retransmission delay is difficult to conceal by the buffer, particularly in long-latency networks, many schemes for error resilience have been studied. 
\passed{\jc{Yihua, please add more citations. }}
\passed{\jc{this section should also be made more technical. Yihua, ping me if you can spend some time on this part}\yc{added a bit words, but maybe not enough}}


\myparashort{Forward error coding}adds redundancy to the encoded data at the sender before sending to the network. 
This is also known as error-resilient channel coding. 
Examples include FEC, Reed-Solomon code, LDPC and fountain codes~\cite{mackay1997near,mackay2005fountain}, rateless coding~\cite{castura2006rateless}, streaming code~\cite{badr2017fec,rudow2023tambur}, and recent ones based on DNNs~\cite{7926071, 8919799}.
Moreover, video codecs also supports data partitioning and apply unequal protection using forward error correction (also known as UEP~\cite{zhao2010rd, abdallah2019h}), \ie having higher redundancy for more important information such as codec configuration and frame metadata.
However, these schemes need to know how many packets will arrive before sending the data out. 
If the loss rate is underestimated, the redundancy will be insufficient to tolerate missing packets and the receiver must either wait for more packets or retransmitted packets.
On the other hand, once the received packets are decodable, receiving more packets does not improve the quality, so even if all packets are received, quality will be lower than without the redundancy. 




\myparashort{Postprocessing error concealment}reconstructs missing data in lost packets on the decoder side. 
% Motion-vector recovery techniques, for instance, recover the motion vector (MV) of an MB~\cite{yihua?} by searching surrounding MBs whose MVs are not lost, and copying the one that causes least pixel differences (``glitches'')~\cite{??}. 
%The encoder splits each frame into partitions (also known as slices) and encodes each partition separately. 
Modern encoders can split each frame into partitions and encode each partition separately (\eg slice interleaving~\cite{ismaeil2000efficient} or flexible macroblock ordering~\cite{lambert2006flexible} technique used in H.264). 
The receiver first decodes the partitions (motion vectors and residuals) in the received packets  and use them to reconstruct data in the lost packets. 
Such reconstruction can be done by classic heuristics (\eg Motion vectors interpolation~\cite{kolkeri2009error, zhou2010efficient, wang2013novel} and Intra-block refreshing~\cite{kumar2006error} in H.264) and NN-based inpainting (\eg~\cite{xiang2019generative,kang2022error, sankisa2018video, mathieu2015deep,reparo}).
However, it has two problems. 
First, to make the partially received packets decodable, some macroblocks (MBs) need to be set in \texttt{INTRA} mode~\cite{660830, lambert2006flexible}, and adjacent MBs need to be split into different packets in a checkerboard manner~\cite{kumar2006error, lambert2006flexible} or based on ROI detection~\cite{tan2011new}. This reduces the compression efficiency, 
%limits the encoder's ability to exploits redundancies across neighboring MBs, so 
and the encoded frame size typically inflates by 10\%-50\%~\cite{kumar2006error, wenger2002scattered, 4494082, dhondt2004flexible}. 
Moreover, since the encoder in these schemes is agnostic to the decoder post-processing, it will aggressively compress each frame, and as a result, each packet contains little redundant information to help reconstruct motion vectors or residuals in other packets.
Thus when a packet is lost, the task of in-painting or reconstruction must guess the missing data (similar to constrained hallucination~\cite{liu2020brief, santos2020single}).
Even recent techniques still see a notable quality drop (\eg PSNR drops from 38 dB to 25 dB at even 20\% packet loss~\cite{nam2020novel}). 
\passed{\jc{Yihua, please read the sentences above. see if the new text makes sense to you}\yc{yeah!}}
% Moreover, the encoder is agnostic to the post-processing, so the encode data (encoded motion vectors and residuals) contains little redundant information.
% When some blocks are missing, the in-painting task is inherently ``underspecified'' (\ie reconstruction is error-prone). 
\passed{\amz{This sentence is a bit vague and hard to follow. I also am not convinced it is needed, unless this "underspecification" of the inpainting comes up later. } }
In contrast, \name jointly trains the NN encoder and NN decoder, which allows the encoder to produce data that is easier to be reconstructed accurately when partially received. 
% Moreover, \name's encoded file size does not grow with more packets. 
\passed{\yc{to make it clear: empirically, even the sota dnn method is not working well + reasoning (citation): inpainting is hallucinating}
\yc{encoder is agnostic to loss/inpainting, so every bit have some information. if packet is lost, the information is not recoverable. inpainting is trying to generate the missing information (movement) by hallucinating}}

\mypara{Other schemes}
There are several other techniques that are might help mitigate the impact of packet loss, but their primary goals are not loss resilience, so they are less resilient to packet loss than the aforementioned schemes. 
But for completeness, we discuss some notable schemes here and also qualitatively compare \name against several of them in \S\ref{sec:eval}.

\passed{\jc{the following paras should be greatly tightened}\yc{already looks good to me}}

Scalable video coding (SVC)~\cite{schwarz2007overview, schierl2007mobile, swift} and fine-granularity scalability (FGS)~\cite{li2001overview,ma2022deepfgs} 
%\amz{same citation twice here}
 optimize the notion of rate-distortion (RD) tradeoff---video quality achieved by a single encoded bitstream under different received bitrates.
%Recent work also shows that neural encoders can improve SVC compression~\cite{swift}.
SVC encodes a video in multiple quality layers and sends data {\em layer by layer}.
This works well for on-demand videos~\cite{swift,grad}, but real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{subsec:background}), so a packet loss can occur to any layer, and a new packet may not always improve quality, if the lower layers are not fully received.
For this reason, SVC is rarely used to improve unicast real-time video (though it is used widely by multicast videos to serve users with heterogeneous network capacities~\cite{schierl2007mobile}).

%so that each newly received packet (or layer) will incrementally improve quality. 
%However, because it imposes a hierarchical order among the packets of a frame, 
%one missing packet can affect all higher quality layers, even if more packets are received in the higher quality layers.
%Though sending each layer reliably one by one is possible in on-demand videos~\cite{swift,grad}, real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{subsec:background}), so packet loss can affect any layer.
%As a result, SVC is rarely used to improve unicast real-time video (though it is used widely by multicast videos to serve users with heterogeneous network capacities~\cite{schierl2007mobile}).


Frame skipping might be another option if other error concealment schemes are not available.
%The encoder and decoder can work jointly to decide when skipping a frame does not hurt quality and the decoding states. 
For instance, Salsify~\cite{salsify} uses an older but reliably received frame, instead of the last frame, as the reference frame, so the decoder can safely skip a loss-affected frame without hurting subsequent frames.
However, it needs more bits to encode the same quality than using the last frame (which has a much smaller difference from the current frame) as the reference frame
(\eg the P-frames between every other frame are 40\% greater in size than between two consecutive frames).
Long-term reference frame (LTR) technique~\cite{zhang2008error} makes each P-frame individually decodable if the long-term reference is received, no matter whether there is packet loss in between or not. 
However, it shares a similar problem of large size overhead as Salsify.
Voxel~\cite{voxel} lets the decoder skip a loss-affected frame if the encoder indicates that skipping the frame does not affect video quality.
It works well for on-demand videos where B-frames can be safely skipped, and the impact of a skipped frame will stop at the next chunk within a few seconds. 
Unfortunately, neither apply to real-time videos. 


Deep learning has long been used in multimedia. 
It has been used to improve compression efficiency (\eg~\cite{dvc,elf,hu2021fvc,swift, NEURIPS2021_96b250a9}), enhance quality (\eg super resolution~\cite{sivaraman2022gemino,kim2020neural,neuroscaler}), scalable video coding (\eg~\cite{swift,ma2022deepfgs}) and postprocessing error concealment (\eg~\cite{reparo, xiang2019generative, kang2022error, sankisa2018video, mathieu2015deep}).
However, the fundamental limitations of these approaches remain despite the use of deep learning.

Loss resilience has also been studied under specific assumptions, such as availability of multiple paths~\cite{meng2022achieving}, early retransmission driven by router feedback~\cite{zuo2022deadline}, and low-latency networks~\cite{ray2022sqp}.
We do not make special assumptions in this work.



\tightsubsection{Autoencoder background}
\label{subsec:ae-background}

% \jc{this section needs more work}

%\jc{refer to fig~\ref{fig:dvc-arch}}


Our work is based on autoencoders, which use learned NNs instead of handcrafted logic, to encode and decode video frames.
Autoencoders have recently reached competitive and even better compression efficiency than traditional video codecs. 
Several factors contribute to this advance.
First, rather than encoding a frame with a monolithic NN, recent autoencoders take advantage of logical components commonly found in classic video codecs (\S\ref{subsec:background}),
% \footnote{For this reason, most autoencoder-based video coding focuses on inter-frames, the most common frame type in real-time videos. Our work also focuses on inter-frame coding and will include I-frame in \S\ref{subsec:protocol}.}, 
such as motion estimation, compensation, and transformation compression of residual and motion vectors.
Then they replace the handcrafted heuristics of classic codecs with NNs that can learn more complex algorithms from data.
Second, these autoencoders are trained on a large corpus of videos (\eg Vimeo-90K~\cite{vimeo-dataset}), so their compression efficiency can reasonably generalize across a variety of video content (which we also observe in our evaluation \S\ref{sec:eval}).
For these reasons, autoencoders attract increasing attention in the multimedia community~\cite{dvc, swift, hu2021fvc}.

% % (We will discuss I-frame in \S\ref{subsec:protocol}, and B-frames are rarely used in real-time videos~\cite{ffmpegstreaming}.)
% It is comprised of steps (\eg motion and residual estimation) typically found in a traditional video codec (\S\ref{subsec:background}) but  uses NNs to replace
% %Most recent video autoencoders~\cite{??,??,??} combine useful concepts from traditional codecs (\eg motion vectors and residuals) and replace 
% handcrafted heuristics for motion estimation, compensation, and \st{transformation} \edit{compression} of residual and motion vectors.
% %, and they achieve compression efficiency comparable to recent video codecs.
% %, and achieve comparable compression efficiency as recent compression algorithms.

%\mypara{Limitations}



\begin{figure*}[t!]
    \centering
         \centering
        %\includegraphics[width=0.97\linewidth]{figs/dvc-arch-v3.pdf}
        % \includegraphics[width=0.93\linewidth]{figs/dvc-arch-v3.pdf}
        \includegraphics[width=0.93\linewidth]{figs/dvc-arch-v4.pdf}
    \tightcaption{Workflow of the autoencoder in \name.}
    \label{fig:dvc-arch}
\end{figure*}

Our work adopts the DVC architecture~\cite{dvc}, a popular autoencoder (depicted in Figure~\ref{fig:dvc-arch}).
Two properties of autoencoders make them particularly suitable for loss resilience.
\begin{packeditemize}

\item {\bf Generative:} The decoding part in autoencoders, such as DVC, can {\em generate} frames with any vector in the encoded latent space as input. 
In other words, it can decode not only the encoder's output but also other vectors that look similar to the encoder's output. 
This means that if we randomly perturb the values in the encoder output (such as zeroing some random values or adding a Gaussian noise), the NN decoder can still successfully decode the frame, though the quality will have a non-trivial drop compared to without the perturbation.

\item {\bf Learnable:} Autoencoders can decode any vector in the encoded latent space but the decoded quality can be quite poor. 
Fortunately, the encoder and the decoder are {\em learnable} NNs that can be trained to optimize decoded quality in the presence of perturbations like random zeroing. 
For instance, the decoder can learn to be less sensitive to perturbed values, and the encoder can learn to add slight redundancy that helps the decoder accurately correct perturbed values.

\end{packeditemize}

Nonetheless, existing autoencoders as-is still lack tolerance to packet loss for two reasons.
%still requires traditional schemes (like FEC) to handle packet loss. 
%Their lack of packet loss tolerance is due to two reasons.
First, the standard autoencoder training implicitly assumes that the encoder's output equals the decoder's input,
% \footnote{A recent work~\cite{??,??} adds Gaussian random noise\jc{check!} between the encoder and decoder to simulate wireless signal noise, but this is different from packet loss which masks a fraction of the data.}, 
so it does not prepare the autoencoder to handle data loss between the encoder and decoder. 
Second, entropy encoding used in autoencoders compresses the whole encoder output as a single bitstream, so any data loss will render it undecodeable.

\name is an attempt at transforming autoencoders to be resilient to packet loss at different rates.
Our work is related to an emerging line of work on deep joint source-channel coding~\cite{kurka2020deepjscc, pmlr-v97-choi19a} which trains an autoencoder to code images in a representation that is both compact and robust to signal noises.
\name differs on two key fronts. 
First, they target physical-layer protection against signal noises.
% is different from (and complementary to) transport-/application-layer protection against packet losses. 
While physical-layer noises can be modeled as differentiable linear transformations (as in~\cite{bourtsoulatze2019deep,gunduz2019machine}), packet drops are not naturally differentiable and need to be handled differently. % (see \S\ref{subsec:sim-losses}). 
Second, unlike compressing individual images, frames in a streaming video cannot be treated separately, otherwise, any error on one frame may propagate to future frames. 


\tightsubsection{Summary}

In summary, traditional error-resilient methods fall short to optimize quality under different packet loss rates.
On one hand, forward error coding optimizes quality only under a pre-determined loss rate, and postprocessing error concealment suffers suboptimal quality under a range of loss rates.
On the other hand, autoencoders can potentially tolerate data perturbation at any rate, but they cannot tolerate packet loss.

By contrast, a better coding scheme should optimize quality under different packet loss rates. 
We call it {\em data-scalable (DS) coding}.
With the same encoding of each frame, DS coding obtains quality similar to the classic codec (H.265) used in WebRTC without FEC when there is no packet loss; and with higher packet loss rates, the quality gradually degrades but is still better than state-of-the-art loss-resilient schemes.
In the next two sections, we will describe an autoencoder-based solution to approximate the effect of DS coding.

%the aforementioned solutions either sacrifice the quality in absence of packet loss or fail to get decent quality in presence of high packet loss rates.
%As we will see, \name shows a more desirable relationship between quality and packet loss rate.





==> sections/old/motivate_v10.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\tightsection{Motivation}
\label{sec:motivate}

%Video coding has a rich history of research and it is hard to fit a comprehensive overview in a limited space.
%Nonetheless, 

\vspace{0.2cm}

\tightsubsection{Background of video coding}
\label{subsec:background}

To help explin \name's design, we first introduce some key concepts of real-time video coding (\S\ref{subsec:background}) relevant to this work. 
%before explaining the need for a different approach (\S\ref{subsec:ds},\ref{subsec:prior}). 
%The video sender runs a rate adaptation logic to dynamically set the frame rate and bitrate of the encoded video.
The sender encodes the video at a given frame rate and bitrate, \eg
%A video stream is encoded at certain frame rate and bitrate, both are controlled by an adaptation logic in the player.
at a frame rate of 25fps (frames per second) and bitrate of 3Mbps, the encoder should on average generate a 15KB frame every 40ms.
%, though the actual frame size varies.
%depends on the {\em type} of a frame
A video stream consists of multiple groups of consecutive frames (called group of pictures or GoP), and each GoP starts with an I-frame (intra-frame) followed by P-frames (predicted frames)\footnote{On-demand videos also use B-frames (bidirectional predicted frames), which 
% are smaller than P-frames since they 
refer to both past and future P-frames. However, real-time video rarely uses B-frames in order to render frames as soon as possible.
% However, to render frames as soon as possible, real-time video rarely uses B-frames~\cite{??}, since they refer to future frames to be decoded.
}.
% and B-frames (bidirectional predicted frames). 
I-frames are encoded and decoded independently without referring to other frames, so they have a bigger size than P-frames, which only encode the differences with other {\em reference} frames.

% Thus, I-frames are used infrequently (\eg only when content shifts dramatically) with 10s or more P-frames between two I-frames.

%and each GoP consists of 10s to 100s of P-frames. 
%I-frames are encoded independently, and P-frames and B-frames encode the differences between them and other {\em reference} frames: a P-frame refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames. 
%Importantly, to render each frame as soon as its packets are received, real-time videos almost never use B-frames which refer to future frames~\cite{??}. 
%Since I-frames do not need other frames to decode, their sizes in standard video codecs are much bigger than B-/P-frames, so I-frames are typically used only when content shifts dramatically and each GoP consists of 10s to 100s of frames. 

%As we will see in \Sref{??}, our new video coding system follows the same frame definitions, though the optimal GoP size will be much smaller. 


%Different {\em frame types} often have different frame sizes.
%An I-frame (intra-frames) is encoded independently and is followed by P-frames (predicted frames) and B-frames (bidirectional predicted frames), each of which encodes the differences between it and some other frames.
%A frame used as a reference for decoding other frames is called a {\em reference} frame: a P-frame only refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames.
%Since I-frames do not need other frames to decode, their sizes are typically bigger than B-/P-frames.


%In real-time videos, to render each frame as soon as its packets are received, B-frames, which refer to future frames, are rarely used~\cite{??}. 
%This precludes several loss-resilient techniques such as B-frame skipping (see \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{??}).

%, and  , each encoding the difference with the previous and future I-/P-frames.
%Thus, I-frames are typically bigger than P-frames and B-frames, but decoding I-frames does not depend on any other frame, while decoding P-frames or B-frames must refer to other frames. 
%fewer other frames than decoding a B-frame.


Most frames are P-frames.
Figure~\ref{fig:codec-workflow} shows the workflow. 
Given a new frame, the encoder 
(1) calculates its motion vectors (MVs) and residuals per macroblock (MB), each of 4×4,8×8,\dots, 
(2) then transforms and quantizes them, 
(3) entropy encodes the transformed data, 
(4) splits the entropy-coded data into packets, and 
(5) sends them out by a congestion control logic, such as GCC~\cite{carlucci2016analysis} used by WebRTC. 
%To encode a frame, the encoder first calculates the differences (\eg motion vectors and residuals) among macroblocks (4×4,8×8,…4\times4,8\times8,\dots) in the current frame and reference frames (or within an I-frame),  then transforms and quantizes these differences to a more compact form, and finally losslessly encodes the data using arithmetic coding. 
%The entropy-encoded data is then packetized and sent out by the transport layer, which tries to deliver as many packets as possible 
%% (though not always all packets) 
%to the receiver by the time when the frame is decoded.
%algorithm decides how fast to send a frame's packets, 
%in order to ensure enough data be delivered to the receiver when the frame is decoded. 
Similarly, the receiver depacketizes and decodes the received data to 
% runs a reverse process (depacketization and decoding) to 
reconstruct each frame from received packets. 
%A decoded frame is put in a very short {\em buffer} before playing to conceal transient latency jitters.
% (due to queuing or retransmits).


\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/fig2-workflow-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{A typical workflow to encode a frame.}
    \label{fig:codec-workflow}
\end{figure}


To reduce frame delay (defined by the time between the encoding and the rendering of a frame), real-time video clients make two common choices~\cite{10.1145/3410449,salsify} that are different from streaming videos, such as Netflix, ESPN live: %\footnote{\jc{any exceptions?}}:
% that affect the requirements of a desirable video coding scheme.
\begin{packeditemize}
\item Packets of a frame are sent in a burst (without waiting for acks), and %without waiting for acknowledgement.
{\em any} packets in the middle of a frame could be delayed or dropped when the receiver tries to decode the frame.
By contrast, streaming videos are sent by chunks (each consisting of 10s to 100s of frames) over the HTTP/TCP protocol.
\item The buffer in real-time videos is much {\em shorter} (\eg 10s~ms) than that of on-demand videos, whose buffer is over 10 seconds, and live broadcast videos, whose buffer is still several seconds.
Thus, retransmission delay is more difficult to conceal, particularly in long-latency networks.
% This short buffer often cannot conceal retransmission delay in long-latency networks.
%With a short buffer, any missing packet might delay a frame longer than the jitter buffer can conceal.
\end{packeditemize}
Therefore, tolerating packet loss is crucial.
%Therefore, it is at least as important to tolerate packet loss as enhancing quality through better compression algorithm or super resolution~\cite{neuroscaler,nas}. 

%loss resilience is vital for real-time video coding!

%real-time videos use  loss resilience of video coding is needed to ensure smooth and high-quality video in presence of packet loss.



 
%Loss-resilient video coding is particularly crucial in real-time videos.\footnote{\jc{clarify real-time video, conversational video, low-latency video}}
%This is because
%%Since packet loss might happen anytime, loss resilience of video coding is needed to maintain smoothness and high quality. 
%%Loss resilience is particularly important for real-time videos, because 
%to maintain high interactivity, real-time videos use a much shorter jitter buffer (just 1-2 frames or 10s~ms) than on-demand or live broadcast videos, whose buffers are likely at least a few seconds.
%With such a short buffer, {\em any packet queuing or retransmit} might block the decoding of a frame after the short buffer is depleted. 


%, which can be caused by either dropped packets or delayed packets.

%To capture the effect of dropped packets and delayed packets on decoding, 

%\tightsubsection{\hspace{-0.2cm}Desirable loss-resilient coding for real-time videos}
\tightsubsection{Data-Scalable Coding}
\label{subsec:ds}

\mypara{Data-missing rate (\rate)}
\fyy{Not sure it's necessary to introduce a new concept.
Since all schemes are allowed to consume the same amount of
bandwidth using the same total size of packets, their latencies should also be the same (unless undecodable at all).
Packet loss rate seems perfectly fine to use?}
We define data-missing rate (\rate) as the fraction of packets of a frame that have not arrived when the frame is decoded.
\jc{effectively packet loss rate but defined per frame}
A missing packet can be due to queuing or retransmission.
%\footnote{\rate can be seen as deadline missing rate, if the deadline is when the decoder decides to decode a frame.}
High \rates arise from various reasons. 
For instance, a sudden bandwidth drop from 3Mbps to 500Kbps on a 200ms-RTT link can quickly raise \rate to 75\% and retransmission will delay or skip at least 6 frames in a 25fps video stream. 
Previous measurements have shown that 
%if frames are decoded with a fixed intervals (\eg every 40ms for a 25~fps video), 
transient high \rates (\eg $>30\%$) are not rare and are difficult to precisely predict in advance~\cite{macmillan2021measuring}. 
Note that our work does {\bf not} assume that high \rates are persistent in presence of a rate adaptation logic.

\mypara{Data-Scalable (DS) coding}
In a desirable video coding, which we refer to as {\em data-scalable} ({\em DS} for short) coding, quality should gracefully degrade in {\em presence} of more packet loss, without compromising the quality in {\em absence} of packet loss.
We breakdown this to three specific requirements:

\begin{packeditemize}
\item {\bf (\RDecodable)} 
The receiver can decode a frame if {\em any} non-empty subset of the packets of this frame is received---{\em minimum need for retransmission or frame skipping}.
%In real-time videos, the delay of a retransmit (at least a round-trip time) is sometimes longer than the jitter buffer (10s~ms), so any retransmit may cause a user-perceivable lag or skipped frames. 
%(\ie no retransmission or frame skipping unless no packet is received);

\item {\bf (\RGraceful)} 
%{\em Graceful degradation:} 
The quality should gradually improve with the addition of any received packet---{\em graceful degradation with higher \rates}.
%(\ie the decoded quality should gracefully degrades with higher \rates).

\item {\bf (\REfficient)} 
%{\em Compression efficiency:} 
If all packets are received, the decoded video will reach a quality close to that of a non-loss-resilient coding algorithm (such as H.265)---{\em high compression efficiency}.
%similar quality as the quality without redundancy (such as H.265), if all packets are received.

\end{packeditemize}




\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/fig2-dmr-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{Illustrative example of the ideal data-scalable coding under dynamic data-missing rates (\rates).
%         \jc{maybe replace it with real values of autoencoder and FEC? }
         }
    \label{fig:codec-dmr}
\end{figure}

\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.97\linewidth]{figs/big-comparison-v2.pdf}
         \label{fig:}
         \tightcaption{Limitations of current loss-resilient solutions under three packet arrival patterns (no loss and one packet missing at different positions). \greencheck marks both high quality (encoding bitrate approximates the throughput) and low delay (no retransmission).}
    \label{fig:comparison}
\end{figure*}

Figure~\ref{fig:codec-dmr} illustrates the effect of DS coding in action. % in presence of bursts of high \rates.
% due to bandwidth fluctuations.
We assume that the bandwidth is mostly stable with intermittent high-\rate spikes caused by transient bandwidth drops and that the encoding bitrate matches the actual bandwidth.
As \rate varies over time, the quality of DS coding is high \rate is low (zero) and drops gracefully when \rate is high.

%To deliver each frame as quickly as possible, the sender often sends all packets of a frame in {\em one batch}. As a result, {\em any} packets might be missing. 






%in DS, quality grows with the number of {\em any} received packets, whereas in RD, the quality grows with consecutive packets in their sending order. 

%an RD-optimized sender sends packets in specific sending order and its quality grows with only received packets that are before the first missing packet in the sending order.

% assumes that packets are sent in order and packet loss only happens to the latter packets.
%DS is more realistic in real-time videos, because in long-latency networks, the sender should send all packets of a frame in one burst, and loss can happen to any packets, rather than just the last few packets (as shown in Figure~\ref{??}). 


%Second, to reduce frame delay in long-latency networks, the sender often sends all packets of a frame in one burst, rather than multiple congestion windows.
%%Thus loss and delaying can happen to any packets within the burst. 
%This diminishes the benefit of layered coding (introduced shortly) which encodes a video in multiple layers and must deliver the layers in a specific order (see \S\ref{??}).

\tightsubsection{Why not existing loss-resilient schemes?}
\label{subsec:prior}

\fyy{I suppose this overly defensive section is added to address reviewers' concerns upfront. However, it is currently very heavy and requires a lot of brainpower to process. Following Figure 4's examples is not pleasant at all. Consider writing a standard background subsection on loss-resilient schemes, and another subsection for autoencoders? After reading through Section 2, the reader should have a better intuition about why autoencoders are suitable, and how they overcome the problems of existing approaches. Be prepared for reviewers who skip Section 3 and beyond.}

Next, we will explain why it is difficult to achieve DS coding using current loss-resilience schemes, including FEC, SVC, and error concealment.
% rate-distortion optimization
% and the difference between DS and other similar notions (\eg rate-distortion optimization).


%Next, we examine several representative loss-resilient coding schemes through the lens of the requirements of DS. 
%explain why they fall short of at least one of the three requirements of DS coding.

%Loss resilience has long been an important research topic. 
%Given the sheer amount of prior work in this space, we only highlight those that are most representative or closest to the goal of DS coding. % (see~\cite{??} for a complete survey).
%For ease of comparison, Figure~????????????\ref{fig:primitive-table}  shows how video quality varies with received data (packets) in different loss-resilient techniques. 

%these abstractions also influence the interaction with the remaining parts of a real-time video application, such as congestion control and bitrate adaptation.




\myparaq{Why not bitrate adaptation over TCP}
First, most streaming video systems today rely on congestion control and bitrate adaptation logics to {\em react} to bandwidth fluctuation and rely on \st{TCP to retransmit} \edit{retransmission to recover from} lost packets. 
They use highly efficient codec (\eg H265), so {\em if} all packets are received on time (\ie retransmission is fast enough), 
%the highly efficient codec (\eg H265) 
they will reach  a high quality with fewer bits. 
%This is well-suited for very low latency (with RTT of a few milliseconds) to allow fast retransmission.
However, it violates \RDecodable because these codecs are not inherently loss tolerant, so a frame cannot be decoded until all packets are received (\eg packet outcome \#2 and \#3 in Figure~\ref{fig:comparison}). 
%In real-time videos, retransmission delays can sometimes be longer than the jitter buffer (10s~ms), causing a visually perceivable lag or a skipped frame.

%re-sending a packet takes longer than the jitter buffer, this can also cause a visually perceivable lag or a skipped frame.

%Essentially, bitrate adaptation is {\em reactive}---if bandwidth suddenly drops, some frames will have already been affected by packet delays/drops before the sender/receiver lowers the bitrate.
%Without a proper loss-resilient scheme, it violates all three requirements of DS coding for real-time videos.

%---it lowers the encoding bitrate {\em after} a bandwidth drop is detected

%Packet retransmission is a conventional loss-resilient scheme. 

\begin{comment}
Frames are coded by a highly efficient codec (\eg H.265), and once all packets are received, the quality will be equal to the original encoded quality.
However, since these codecs optimize for compression, not loss resilience, any lost packets must be resent until all packets are reliably received, which violates {\em \RDecodable}.
If re-sending a packet takes longer than the jitter buffer, this can also cause a visually perceivable lag or a skipped frame.




\myparaq{Why not bitrate adaptation}
Bitrate adaptation lowers the target bitrate of {\em future} video chunks/frames {\em after} a bandwidth drop is detected. %, and then the video encoder will code the future video chunk or frame at the lowered target bitrate. 
Thus, bitrate adaptation is fundamentally {\em reactive}: 
when bandwidth suddenly drops, some frames have already experienced packet delays or drops before the sender/receiver can lower its target bitrate.
Given the short jitter buffer, this can directly hurt user experience, as in Figure~\ref{fig:trace}(a).
Without a proper loss-resilient scheme, it violates all three requirements of DS coding.

\end{comment}

\myparaq{Why not scalable video coding (SVC)}
SVC tries to optimize the classic notion of rate-distortion (RD) tradeoff, which which represents video quality achieved by a single encoded bitstream under different received bitrates and was studied intensively around 2000~\cite{schwarz2007overview, schierl2007mobile}.
SVC encodes a video at multiple quality layers and  sends data {\em layer by layer}, so that
%and if the packets are received in order, 
each newly received packet (or layer) will incrementally improve quality. % and when all packets are received, quality will be close to that of H.265. 
SVC-based techniques have made remarkable progress towards RD-optimized quality in on-demand video streaming, \eg fine-grained scalability (FSG)~\cite{li2001overview} and more recently, DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift}.


\begin{comment}
such that the decoder can reach the $i$-th quality layer, once the packets of $i$-th layer and lower layers are received, and the quality can be incrementally improved to the $(i+1)$-th layer, if the packets of the $(i+1)$-th layer are received.
%as long as the packets belong to the $i$-th layer and lower layers are received, we can obtain the quality of the $i$-th layer.
% and gradually improve quality with more received layers.
SVC-based techniques have made remarkable progress towards RD-optimized quality, especially in on-demand video streaming, \eg fine-grained scalability (FSG)~\cite{li2001overview} and more recently, DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift}.
Unlike TCP-based bitrate adaptation, an SVC sender sends data {\em layer by layer}, and 
%and if the packets are received in order, 
each newly received packet (or layer) will incrementally improve quality and when all packets are received, quality will be close to that of H.265. 
Thus, SVC can greatly benefit multicast videos which serve receivers that have heterogeneous network capacities~\cite{??}.
\end{comment}

However, SVC does not meet {\em \RGraceful}, because it imposes a hierarchical order among the packets of a frame; one missing packet can affect all higher quality layers, even if more packets are received in the higher quality layers (\eg packet outcome \#2 in Figure~\ref{fig:comparison}).
Though sending each layer reliably one by one is possible in on-demand videos~\cite{swift,grad}, real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{subsec:background}), so packet loss can affect any layer.
As a result, SVC is rarely used to improve unicast real-time video (though it is used widely by multicast videos to serve users with heterogeneous network capacities~\cite{schierl2007mobile}).
Essentially, DS coding differs from RD optimization on a key aspect---the quality of DS coding depends on {\em how many} packets, not {\em which} packets, are received.


\begin{comment}

There have been many SVC techniques---notably, fine-grained scalability (FSG)~\cite{li2001overview} and more recently, DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift} achieve near-optimal rate-distortion (RD) tradeoffs: if the packets are received in order, each newly received packet will incrementally improve quality and when all packets are received, quality will be close to that of H.265. 
%realize the following effect: if the packets are received in order, each new packet will incrementally improve quality, and when all packets are received, the quality is similar to H.265. 
Therefore, SVC can greatly benefit multicast videos as a way to serve receivers that have heterogeneous network capacities~\cite{??}.

However, SVC imposes a hierarchical order among packets that one missing packet can render all higher quality layers undecodable, even if more packets are received on higher quality layers~\cite{chen2006frame}; in other words, it violates {\em \RGraceful}.
Though sending each layer reliably one by one is possible in on-demand videos~\cite{swift,grad,etc}, real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{??}), so packet loss can affect any layer.
For this reason, SVC is not widely used to improve quality of unicast real-time video sessions~\cite{??}.


Note that DS is different from the classic notion of rate-distortion (RD) optimization, which was studied intensively around 2000~\cite{??,??}. 
%DS video coding may sound similar to the classic rate-distortion (RD) tradeoff, which was intensively studied around early 2000s~\cite{??,??}. 
RD optimizes video quality achieved by a single encoded bitstream under different received bitrates.
%, and ideally, with a single encoded bitstream, the decoding quality of the received data naturally increase if more data of the bitstream is received.
DS differs on a key aspect.
%The quality of DS coding grows with more received packets, regardless of their positions in the original sending order.
The quality of DS coding depends on {\em how many} packets, not {\em which} packets, are received.
In contrast, RD assumes that the packets have some dependencies and its quality increases with more packets received before the first missing packet in the original sending order. 
For instance, suppose that three packets are sent and the 2nd packet is the first missing packet. If the 3rd packet is received, then the quality of DS coding will grow but the quality of RD coding will not, since only one packet before the missing packet is received.
DS coding is more suitable for real-time videos, because as said earlier, senders of real-time videos burst packets of each frame, so loss can happen to any packets, rather than just the last packets.

\end{comment}


\begin{comment}

This makes sense in on-demand videos where different layers can be sent reliably one by one~\cite{??}.
In addition, 

However, SVC imposes a hierarchical order that one missing packet can render all higher quality layers undecodable, it violates requirement {\em \RGraceful}~\cite{chen2006frame}.
In unicast real-time video communication, however, senders often send all packets of a frame in {\em one batch}, rather than layer by layer, because the round-trip time is often higher than jitter buffer, 
As a result, {\em any} packets can be lost. 



with non-trivial network latency, so to reduce each frame's delay, most senders send packets of a frame as one batch.

SVC imposes a hierarchical order that one missing packet can render all higher quality layers undecodable, it violates requirement {\em \RGraceful}~\cite{chen2006frame}.
%\footnote{The classic SVC violates both requirement {\em (ii)} and {\em (iii)} of DS coding, though {\em (iii)} is mitigated by an autoencoder-based codec~\cite{swift} proposed recently.}
Even if the base (lowest) layer is padded with redundancy (\eg FEC, explained shortly)~\cite{SVCFEC1, schierl2007using,wang2000error}, it does not protect other layers from packet losses.\footnote{\jc{move this footnote to SVC later}The state-of-the-art solution, which is also based on neural-network autoencoders~\cite{swift}, can generate a single encoded bitstream to  {\em approximate} the optimal RD tradeoff, though still with a substantial margin.}

Other than SVC, there have been several other proposals that aim for finer-grained scalability.
Notably, fine-grained scalability (FSG)~\cite{li2001overview} and more recently DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift} strive to realize the following effect: if the packets are received in order, each new packet will incrementally improve quality, and when all packets are received, the quality is similar to H.265. 
Though they are better than classic SVC, they still impose a hierarchical structure over packets, which violates requirement {\em \RGraceful}---if a low-quality-layer packet of is missing, higher-quality-layer packets are not useful.\footnote{It should be clarified that SVC does achieve coding scalability with on-demand videos, which has enough buffer to allow packet retransmission.
%, where the sender usually makes sure one layer is fully received before sending the next one.
}

\jc{old text}
 (\eg as we will explain shortly, in scalable coding, data of lower coding layer is reliably received before fetching higher layers). 
With this assumption, RD-optimized coding can still greatly improve multicast service (\eg in multi-party video conferencing) and on-demand videos where different layers can be received one by one. 
Our paper aims at unicast real-time video communication with non-trivial network latency, so to reduce each frame's delay, most senders send packets of a frame as one batch.

\end{comment}

%one single lost packet of a lower layer will make all higher layers undecoded. 
%This violates requirement {\em (ii)} of DS coding.
%While the base (lowest-quality) layer of SVC is often padded with redundancy (\eg FEC, explained shortly)~\cite{wang2000error}, it does not protect other layers from packet losses.
%






\myparaq{Why not error correction coding (\eg FEC)}
The most common loss-resilient coding in real-time video is forward error correction (FEC).
% and its recent variants (\eg streaming code~\cite{??} and rateless fountain code~\cite{??}). 
%These redundancy-based schemes essentially trade coding efficiency for loss resilience. 
Given a target frame size RR, FEC encodes frames at N%⋅RN\%\cdot R, with the remaining (1−N%)⋅R(1-N\%)\cdot R used for redundancy. (1−N%)(1-N\%) is the {\em redundancy rate}.
The frame will be decodable, once {\em any} N%N\% of packets are received.
FEC differs from SVC in that SVC depends on {\em which data} is received, whereas FEC depends on {\em how much} data is received.

However, FEC-based schemes, including rateless coding~\cite{castura2006rateless} and streaming code~\cite{badr2017fec}, must know in advance how much data will arrive before the receiver decodes a frame; otherwise it will add either too much redundancy or still need to retransmit. 
% \footnote{\jc{some words on why rateless doesn't help here} \jc{also a parallel work tumbr has the same problem}} must know \rate~{\em before} sending the data; otherwise it will add either too much redundancy or still need to retransmit. 
%they work better only if \rate is known {\em before} FEC encodes the data. 
%must know \rate in advance to avoid packet retransmission and too much redundancy.
If redundancy is not enough to conceal missing packets in time (\ie~\rate is underestimated), some packets must be waited or retransmitted in order to decode the frame, which violates {\em \RDecodable} (\eg 10\% FEC in Figure~\ref{fig:comparison}).
Once the received packets are decodable, more packets will not improve the quality, which violates {\em \RGraceful}.
And if all packets are received (\ie~\rate is overestimated), the redundancy will lower the video quality, which violates {\em \REfficient} (\eg FEC 33\% with packet outcome \#1 in Figure~\ref{fig:comparison}).

%if much redundancy is added while all packets are received (\ie loss rate is overestimated), the decoded quality will be much lower than it could have been without redundancy (which violates {\em \REfficient}).

%\jc{include streaming code}




\myparaq{Why not redundant video coding}
%Source-coding-based schemes do not explicitly add redundancy like FEC. 
Besides FEC which adds redundancy to the video encoder output, the video coding itself can increase loss resilience.
% \footnote{In the video coding literature, the former (\eg FEC) refers to channel coding, while the latter refers to source coding.}.
% can be made more resilient to packet loss.
%Two examples are intra-MB insertion and reference selection, but both methods do not meet {\em \REfficient}, because they also add redundancy and have much lower quality if no packet turns out missing. 
%Intra-MB insertion~\cite{??} sets more macroblocks (MBs) in \texttt{INTRA} mode which makes their decoding not dependant on other frames, so missing one MB will affect fewer other MBs.
%However, doing so fails to exploit similar MBs across different frames, their quality will be lower than without intra-MB insertion at the same bitrate.
For instance, if we use an older but reliably received frame, instead of the last frame, as the reference frame, the decoder can safely skip a loss-affected frame (\eg~\cite{salsify}) without hurting subsequent frames.
However, this method also needs more bits to encode the same quality than using the last frame (which has a much smaller difference with the current from) as the reference frame
% , because the difference between two consecutive frames is much less than other history frames 
(\eg the P-frames between every other frames are 40\% greater in size than between two consecutive frames).

Without redundancy in coded data, one can still choose to skip a loss-affected frame, if skipping it does not affect future quality (\eg Voxel~\cite{voxel}). 
It works well for on-demand videos where (1) B-frames can be safely skipped, (2) the impact of a skipped frame will stop at the next chunk within a few seconds, and (3) the content is known in advance to profile the impact of skipping each frame on future frames. 
Unfortunately, none of them apply to real-time videos. %, in which B-frames are rarely used in and I-frames are used less often.



%\mypara{Receiver-side loss concealment}
\myparaq{Why not error concealment}
Error concealment by the video receiver has been intensively studied in multimedia. 
% Motion-vector recovery techniques, for instance, recover the motion vector (MV) of an MB~\cite{yihua?} by searching surrounding MBs whose MVs are not lost, and copying the one that causes least pixel differences (``glitches'')~\cite{??}. 
including recent work that uses neural networks (NN) to recover lost motion vectors (MVs) or use inpainting techniques to recover lost residuals~\cite{zhou2010efficient, xiang2019generative}. 
The key problem of these error concealment strategies is two-fold.
First, more macroblocks (MBs) need to be set in \texttt{INTRA} mode (independently decodable) and neighboring MBs should ideally be in different packets to facilitate recovery during packet losses.
However, all of these increase the frame size (\eg~30\% for four packets) and this inflation increases with more packets, since 
% in order for each packet to be decodable, but this greatly increases the frame size (\eg~\fillme\% for four packets) and this inflation increases with more packets.
they fail to leverage similarity among MBs---they do not meet {\em \REfficient}.
% , their quality will be lower than without intra-MB insertion at the same bitrate. 
% Like redundant video coding, this means they fall shorts on {\em \REfficient}.
Second, since the sender still uses a standard codec, there is minimum redundancy in the encoded MVs and residuals, and thus the MV recovery or inpainting tasks are inherently ``underspecified''.
% \footnote{This is why they often train the NN model per video~\cite{??,??,??}, but it is infeasible in real-time videos.}
As a result, their quality degrades quickly with higher \rates, which corroborates our results in \S\ref{sec:eval}.

\yihua{update a paragraph about sr here -- need to iterate}
\myparaq{Why not super-resolution (SR)}
Previous works have employed the super-resolution (SR) technique to enhance video quality in low-bandwidth conditions for on-demand and live video streaming~\cite{??, ??, ??}. However, SR does not fulfill the requirements of data-scalable coding; it fails if the base frame is incomplete or undecodable, contravening \RDecodable and \RGraceful.
SR can potentially enhance real-time video quality in two ways: {\em (i)} directly improving decoded video quality, and {\em (ii)} preserving quality while transmitting less data, thereby averting possible network congestion or allocating more bandwidth for additional redundancy.
However, approach {\em (i)} is codec-agnostic and hence unrelated to the design space of DS codecs. Approach {\em (ii)} is also non-data-scalable; if the transmission bitrate is excessively low, quality will deteriorate, and if the bitrate is set higher to preserve quality, network congestion cannot be completely mitigated.

In contrast, this work~{\em jointly} trains the NN encoder and NN decoder, allowing slight amount of redundancy in the coded data to facilitate error concealment by decoding.
%Moreover, its per-packet entropy encoding adds much less overhead than 


%In summary, none of the existing loss-resilient schemes achieve the goal of DS video coding. 
%We will also show preliminary results that quantitatively compare them with our proposal in later sections.


%can reconstruct lost motion vector (MV) of a macroblock (MB) by the MVs of surrounding MBs.
%For instance, one method to 

\begin{comment}

We empirically observe that such recovery is less effective than the NN-based coding proposed in this work.\jc{yihua, any pointer to an evidence?} to recover it and this may not always be effective (see \S\ref{??}).


Moreover, when the information of an MB is missing, they use handcrafted heuristics 

Receiver-side solution is to use image inpainting algorithms to restore a partially received frame. 
However, this is doable only {\em if} part of a frame can be decoded based on received data, which must rely on some other techniques mentioned earlier. 
For these reasons, they are not commonly used in real-time videos.



Alternatively, can also choose to skip a loss-affected frame, if skipping it does not affect future quality. 
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) B-frames can naturally be safely skipped, (2) the impact of a skipped frame will stop at next chunk (in a few seconds) when a new I-frame starts, and (3) the impact of skipping each frame on future frames can be pre-determined offline. 
Unfortunately, none of them is true for real-time videos, in which B-frames are rarely used in and I-frames are used less often.


\end{comment}



\begin{comment}
Reference selection uses an older frame already received by the receiver, instead of the last frame, as the reference to encode a new frame (\eg~\cite{salsify}), so any frame undecodable due to packet losses can be safely skipped without affecting future frames.
%setting its reference frame to some history frame that has been received by the receiver, rather than the last frame~\cite{salsify}. 
%This way, a frame that is undecodable due to packet losses can just be safely skipped without affecting future frames.

Both methods, however, do not meet {\em \REfficient}, because they use redundancy and have much lower quality if all packets are received. 
%In both cases, however, they have to sacrifice some compression efficiency if all packets are received, which violates {\em \REfficient}.
Intra-MB insertion fails to exploit similar MBs across different frames, their quality will be lower than without intra-MB insertion at the same bitrate.
%Like intra-MB insertion, 
Reference selection needs more bits to encode the same quality level, because the difference between two consecutive frames is much less than other history frames (\eg the P-frames between every other frames are \fillme\% greater in size than between two consecutive frames).

Both error-correction coding and redundant video coding must choose between compression efficiency (quality in absence of packet loss) and loss resilient (quality in presence of packet loss). 
For this reason, in practice, they are used {\em after} packet loss occurs---FEC is activated by WebRTC or the reference frame is changed by Salsify, only after the first packet loss is detected by the sender, which is at least one round-trip time after the packet loss occurs.
%Figure~\ref{fig:codec-dmr} shows an example of FEC. 
%The sender typically only adds redundancy {\em after} packet loss or delay increase affect a few frames, and when they may also add too much redundancy even after the \rate drops, resulting in low quality.

\end{comment}


\begin{comment}

reduce the inter-dependencies between macroblocks (MBs).
% that are potentially similar to each other. 
Intra-MB insertion, for instance, sets more MBs in \texttt{INTRA} mode, so that a lost MB will affect fewer other MBs.
%they are independently decodable, even if other MBs are lost.
However, because they do not leverage similarity across MBs, their quality will be much lower than without intra-MB insertion at the same bitrate which violates {\em \REfficient}.
%compression at the same bitrate is significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.
%and others that refer to them decodable, even if other data is lost.
%\footnote{Packet losses can also be tolerated by choosing a better reference frame to allow the receiver to skip undecodable frames without affecting subsequent frames, such as in Salsify~\cite{salsify}. These techniques can be used jointly with this proposal to select better quality reference frames.}
%Both intra-MB insertion and FEC must lower coding efficiency: FEC adds redundancy data and intra-MB insertion keeps more inter-macroblock redundancy.

Several other loss-resilient schemes exist that work without changing the video codecs, though they are less efficient than SVC, FEC at handling transient packet losses. 



\myparaq{Why not reference-frame selection} 
When encoding the next frame, the sender can set the reference frame to be a history frame that has been completely received by the receiver, rather than the last frame. 
This way, a frame that is undecodable due to packet losses can just be skipped without affecting future frames.
However, like intra-MB insertion, its quality will be much lower at the same bitrate than using the last frame as the reference, which violates {\em \REfficient}.
%its compression at the same bitrate will be significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.
An exception is Salsify~\cite{salsify}, which changes to a history frame (not the last one) as reference only {\em after} a loss is detected. 
As a result, however, it must skip several frames before encoding starts with a new reference frame.

\end{comment}


%requires techniques like intra-MB insertion are used, which has its own limitations as discussed earlier. For this reason, they are not commonly used in real-time videos.



\begin{comment}

The receiver can also choose to skip a frame depending on the frame's impact on future quality, but for frames whose absence will greatly affect the quality of other frames, this violates at least requirements of  $\RDecodable$ and $\RGraceful$.
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) the impact of a dropped frame will stop at next chunk (in a few seconds) which starts with a new I-frame, and (2) the impact of a skipped frame on future frames can be pre-determined offline. 
Unfortunately, both are not true for real-time videos.

\end{comment}


\begin{comment}

\myparaq{Why not selective frame dropping} 
Even if dropping a frame may affect future frames, the receiver can still choose to do that if the impact on the future frame's quality is relatively small.
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) the impact of a dropped frame will stop at the next chunk, which will start in a few seconds with a new i-frame, and (2) the impact of a skipped frame on future frames can be pre-determined offline. 
Unfortunately, both are not true for real-time videos. 


\myparaq{Why not computer vision-based error concealment}
Finally, image inpainting and super-resolution techniques could restore a partial frame. 
Unfortunately, this is doable only {\em if} part of a frame can be decoded based on received data.
This is usually not doable unless techniques like intra-MB insertion are used, which has its own limitations as discussed earlier. For this reason, they are not commonly used in real-time videos.
%different parts of a frame is encoded independently, which at the same bitrate will be significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.

\end{comment}


%\jc{is \name compatible with multi-party calls}


\begin{comment}



\myparaq{What's new in real-time video}
While this general workflow applies to most video streaming systems, real-time videos are distinctive in that they seek to reduce the {\em frame delay} between sending a frame and decoding it.
This profoundly affects their design choices in three ways.
%have three features distinct from others, which profoundly affect their designs. 
%short jitter buffer, no b frame, packets sent toghether, all of which have profound impact
\begin{packeditemize}
\item {\em Short jitter buffer:} First, real-time videos use a much shorter jitter buffer (just 1-2 frames or 10s of milliseconds) than even live broadcast videos, which have a buffer of at least a few seconds.
While increasing interactivity between clients, the short buffer makes the receiver potentially vulnerable to {\em any packet queuing or retransmit} that blocks the decoding of a frame after the short buffer is depleted. 


\item {\em Each frame sent in one batch:} Second, to reduce frame delay in long-latency networks, the sender often sends all packets of a frame in one burst, rather than multiple congestion windows.
%Thus loss and delaying can happen to any packets within the burst. 
This diminishes the benefit of layered coding (introduced shortly) which encodes a video in multiple layers and must deliver the layers in a specific order (see \S\ref{??}).


\item {\em Avoid B-frames:} Third, as each frame should be decoded as soon as its packets are received, B-frames are rarely used in real-time videos~\cite{??}, since they require future frames to be received. 
This precludes several loss-resilient techniques such as B-frame skipping (see \S\ref{??}).
\end{packeditemize}



\begin{itemize}
\item 2.1 Background
\begin{itemize}
\item basics: video, encoder, decoder, packets
\item real-time video: small jitter buffer, all packets must be sent together
\item concept of loss-resilient coding
\end{itemize}

\item 2.2 Ideal coding for real-time video
\begin{itemize}
\item given that 
\end{itemize}

\item 2.3 Limitations
\begin{itemize}
\item type 1: scalable coding
\item type 2: fec (rateless versions), reference selection, recover
\end{itemize}
\end{itemize}

We begin with why loss-resilient video coding is particularly important to real-time video and what an ideal scheme should achieve. 
We then explain the limitations of existing approaches.

Despite more bandwidth, many recent studies have shown that real-time video communication is plagued with intermittent packet loss and jitter~\cite{macmillan2021measuring,jansen2018performance,concerto,moulay2018experimental,latency-report-iab,latency-report-iab-2,latency-report-apnic}.
%induced by congestion, wireless, bufferbloat, etc.
\jc{yihua, can we find a few good pointers for this?}
%Adapting bitrate (ABR), which {\em reacts} to fluctuations of network conditions, is not enough to completely prevent packet loss, without using an extremely conservative bitrate. 
Since real-time video clients have very shallow jitter buffers, there is little time for packet retransmission before each frame should be decoded. 
So unlike in traditional streaming videos (which has a buffer of at least several seconds),
%Having shallow jitter buffers means that adapting bitrate or sending rate alone is not enough for clients to be immune to packet loss. 
%This leaves little time for packet retransmission, so 
{\em any} dropped or queued packets could delay the decoding of a frame, causing video stuttering and frame skipping in real-time video applications. 

%Having shallow jitter buffers also means that adapting bitrate or sending rate alone is not adequate to make real-time video client immune to packet loss.
%
%
%It is hard to predict how many packets will be dropped 
%Thus, the ability to decode a frame with a decent quality in presence of packet loss is crucial.




%\jc{Relationship with bitrate adaptation}

\end{comment}

==> sections/old/motivate_v11.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\tightsection{Background}
\label{sec:motivate}

%Video coding has a rich history of research and it is hard to fit a comprehensive overview in a limited space.
%Nonetheless, 

\vspace{0.2cm}

\tightsubsection{Real-time video coding}
\label{subsec:background}

To help explain \name's design, we first introduce some key concepts of real-time video coding (\S\ref{subsec:background}) relevant to this work. 
%before explaining the need for a different approach (\S\ref{subsec:ds},\ref{subsec:prior}). 
%The video sender runs a rate adaptation logic to dynamically set the frame rate and bitrate of the encoded video.
The sender encodes the video at a given frame rate and bitrate, \eg
%A video stream is encoded at certain frame rate and bitrate, both are controlled by an adaptation logic in the player.
at a frame rate of 25fps (frames per second) and bitrate of 3Mbps, the encoder should on average generate a 15KB frame every 40ms.
%, though the actual frame size varies.
%depends on the {\em type} of a frame
A video stream consists of multiple groups of consecutive frames (called a group of pictures or GoP), and each GoP starts with an I-frame (or key-frame) followed by P-frames (or inter-frames)\footnote{On-demand videos also use B-frames (bidirectional predicted frames), which 
% are smaller than P-frames since they 
refer to both past and future P-frames. However, real-time video rarely uses B-frames in order to render frames as soon as possible.
% However, to render frames as soon as possible, real-time video rarely uses B-frames~\cite{??}, since they refer to future frames to be decoded.
}.
% and B-frames (bidirectional predicted frames). 
I-frames are encoded and decoded independently without referring to other frames, so they have a bigger size than P-frames, which only encode the differences with other {\em reference} frames.
In real-time videos, most frames are P-frames to reduce the frame size.
Figure~\ref{fig:codec-workflow} shows the workflow of encoding a P-frame. 
Given a new frame, the encoder 
(1) calculates its motion vectors (MVs) and residuals per macroblock (MB), each of 4×4,8×8,\dots, 
(2) then transforms and quantizes them, 
(3) entropy encodes the transformed data, 
(4) splits the entropy-coded data into packets, and 
(5) sends them out by a congestion control logic, such as GCC~\cite{carlucci2016analysis} used by WebRTC. 
%To encode a frame, the encoder first calculates the differences (\eg motion vectors and residuals) among macroblocks (4×4,8×8,…4\times4,8\times8,\dots) in the current frame and reference frames (or within an I-frame),  then transforms and quantizes these differences to a more compact form, and finally losslessly encodes the data using arithmetic coding. 
%The entropy-encoded data is then packetized and sent out by the transport layer, which tries to deliver as many packets as possible 
%% (though not always all packets) 
%to the receiver by the time when the frame is decoded.
%algorithm decides how fast to send a frame's packets, 
%in order to ensure enough data be delivered to the receiver when the frame is decoded. 
Similarly, the receiver depacketizes and decodes the received data to 
% runs a reverse process (depacketization and decoding) to 
reconstruct each frame from received packets. 

% Thus, I-frames are used infrequently (\eg only when content shifts dramatically) with 10s or more P-frames between two I-frames.

%and each GoP consists of 10s to 100s of P-frames. 
%I-frames are encoded independently, and P-frames and B-frames encode the differences between them and other {\em reference} frames: a P-frame refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames. 
%Importantly, to render each frame as soon as its packets are received, real-time videos almost never use B-frames which refer to future frames~\cite{??}. 
%Since I-frames do not need other frames to decode, their sizes in standard video codecs are much bigger than B-/P-frames, so I-frames are typically used only when content shifts dramatically and each GoP consists of 10s to 100s of frames. 

%As we will see in \Sref{??}, our new video coding system follows the same frame definitions, though the optimal GoP size will be much smaller. 


%Different {\em frame types} often have different frame sizes.
%An I-frame (intra-frames) is encoded independently and is followed by P-frames (predicted frames) and B-frames (bidirectional predicted frames), each of which encodes the differences between it and some other frames.
%A frame used as a reference for decoding other frames is called a {\em reference} frame: a P-frame only refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames.
%Since I-frames do not need other frames to decode, their sizes are typically bigger than B-/P-frames.


%In real-time videos, to render each frame as soon as its packets are received, B-frames, which refer to future frames, are rarely used~\cite{??}. 
%This precludes several loss-resilient techniques such as B-frame skipping (see \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{??}).

%, and  , each encoding the difference with the previous and future I-/P-frames.
%Thus, I-frames are typically bigger than P-frames and B-frames, but decoding I-frames does not depend on any other frame, while decoding P-frames or B-frames must refer to other frames. 
%fewer other frames than decoding a B-frame.


%A decoded frame is put in a very short {\em buffer} before playing to conceal transient latency jitters.
% (due to queuing or retransmits).


\begin{figure}[t!]
    \centering
         \centering
         %\includegraphics[width=0.85\linewidth]{figs/fig2-workflow-newplaceholder.pdf}
        \includegraphics[width=0.77\linewidth]{figs/fig2-workflow-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{A typical workflow to encode a frame.}
    \label{fig:codec-workflow}
    \vspace{-0.25cm}
\end{figure}

A key metric in real-time video is frame delay, the time between the encoding and the rendering of a frame.
To reduce frame delay, real-time video clients commonly make two choices~\cite{10.1145/3410449,salsify} that are different from streaming videos, such as Netflix, ESPN Live: %\footnote{\jc{any exceptions?}}:
% that affect the requirements of a desirable video coding scheme.
\begin{packeditemize}
\item Packets of a frame are sent in a burst (without waiting for acks), and %without waiting for acknowledgement.
{\em any} packets in the middle of a frame could be delayed or dropped when the receiver tries to decode the frame.
By contrast, streaming videos are sent by chunks (each consisting of 10's to 100's of frames) over the HTTP/TCP protocol.
\item The buffer in real-time videos is much {\em shorter} (\eg 10's~ms) than that of on-demand videos, whose buffer is over 10 seconds, and live broadcast videos, whose buffer is still several seconds. %\amz{I swapped the "10s" in this section to "10's" to reduce confusion, please revert if undesired. }
% This short buffer often cannot conceal retransmission delay in long-latency networks.
%With a short buffer, any missing packet might delay a frame longer than the jitter buffer can conceal.
\end{packeditemize}

Congestion control and bitrate adaptation logics are often used by video clients employ to cope with bandwidth fluctuation, such as GCC~\cite{carlucci2016analysis},  Salsify~\cite{salsify}, and NADA~\cite{zhu2016nada}.
Ideally, these adaptation logics should reduce packet loss.
However, because it is difficult to predict bandwidth drops or packet loss in advance, they cannot completely eliminate packet loss.
\name is complementary to this line of work, and our results show \name improves loss resilience under different congestion control logics (Figure~\ref{fig:appgcc-delay-simulation}). %\yc{is it okay to put the forward reference to appendix here?}

\passed{\jc{need to smooth the text here}}
%Here, we define {\em packet loss} on a given frame as any packets not received before the receiver decodes the frame. \yc{the prior sentence is replicated from intro}
%, \eg every 50ms at 20 frames per second (fps).
The packet loss, defined {\em per frame as any packets not received before the receiver decodes the frame}, can be consecutive or random and can result from packet drops or latency jitter. 
This definition is consistent with recent papers~\cite{rudow2023tambur,cheng2023abrf,holmer2013handling}. 
It is important to clarify that our notion of packet loss rate is {\bf \em not} network-level loss rate (which rarely exceeds 1\%). 
Even if a packet is not dropped, it can {\em still} be counted as a packet loss, if it arrives too late. 
Therefore, it is {\em not rare} for real-time video clients to have a high (over 50\%) packet loss rate on some frames, even if the network has a very low packet loss rate.
The high packet loss rate per frame also corroborates recent papers in this space~\cite{cheng2023abrf,rudow2023tambur,cheng2020deeprs}.



\tightsubsection{Related work}
\label{subsec:related}

As retransmission delay is difficult to conceal by the buffer, particularly in long-latency networks, many schemes for error resilience have been studied. 
\passed{\jc{Yihua, please add more citations. }}
\passed{\jc{this section should also be made more technical. Yihua, ping me if you can spend some time on this part}\yc{added a bit words, but maybe not enough}}


\myparashort{Forward error coding}adds redundancy to the encoded data at the sender before sending to the network. 
This is also known as error-resilient channel coding. 
Examples include FEC, Reed-Solomon code, LDPC and fountain codes~\cite{mackay1997near,mackay2005fountain}, rateless coding~\cite{castura2006rateless}, streaming code~\cite{badr2017fec,rudow2023tambur}, and recent ones based on DNNs~\cite{7926071, 8919799}.
Moreover, video codecs also supports data partitioning and apply unequal protection using forward error correction (also known as UEP~\cite{zhao2010rd, abdallah2019h}), \ie having higher redundancy for more important information such as codec configuration and frame metadata.
However, these schemes need to know how many packets will arrive before sending the data out. 
If the loss rate is underestimated, the redundancy will be insufficient to tolerate missing packets and the receiver must either wait for more packets or retransmitted packets.
On the other hand, once the received packets are decodable, receiving more packets does not improve the quality, so even if all packets are received, quality will be lower than without the redundancy. 




\myparashort{Postprocessing error concealment}reconstructs missing data in lost packets on the decoder side. 
% Motion-vector recovery techniques, for instance, recover the motion vector (MV) of an MB~\cite{yihua?} by searching surrounding MBs whose MVs are not lost, and copying the one that causes least pixel differences (``glitches'')~\cite{??}. 
%The encoder splits each frame into partitions (also known as slices) and encodes each partition separately. 
Modern encoders can split each frame into partitions and encode each partition separately (\eg slice interleaving~\cite{ismaeil2000efficient} or flexible macroblock ordering~\cite{lambert2006flexible} technique used in H.264). 
The receiver first decodes the partitions (motion vectors and residuals) in the received packets  and use them to reconstruct data in the lost packets. 
Such reconstruction can be done by classic heuristics (\eg Motion vectors interpolation~\cite{kolkeri2009error, zhou2010efficient, wang2013novel} and Intra-block refreshing~\cite{kumar2006error} in H.264) and NN-based inpainting (\eg~\cite{xiang2019generative,kang2022error, sankisa2018video, mathieu2015deep,reparo}).
However, it has two problems. 
First, to make the partially received packets decodable, some macroblocks (MBs) need to be set in \texttt{INTRA} mode~\cite{660830, lambert2006flexible}, and adjacent MBs need to be split into different packets in a checkerboard manner~\cite{kumar2006error, lambert2006flexible} or based on ROI detection~\cite{tan2011new}. This reduces the compression efficiency, 
%limits the encoder's ability to exploits redundancies across neighboring MBs, so 
and the encoded frame size typically inflates by 10\%-50\%~\cite{kumar2006error, wenger2002scattered, 4494082, dhondt2004flexible}. 
Moreover, since the encoder in these schemes is agnostic to the decoder post-processing, it will aggressively compress each frame, and as a result, each packet contains little redundant information to help reconstruct motion vectors or residuals in other packets.
Thus when a packet is lost, the task of in-painting or reconstruction must guess the missing data (similar to constrained hallucination~\cite{liu2020brief, santos2020single}).
Even recent techniques still see a notable quality drop (\eg PSNR drops from 38 dB to 25 dB at even 20\% packet loss~\cite{nam2020novel}). 
\passed{\jc{Yihua, please read the sentences above. see if the new text makes sense to you}\yc{yeah!}}
% Moreover, the encoder is agnostic to the post-processing, so the encode data (encoded motion vectors and residuals) contains little redundant information.
% When some blocks are missing, the in-painting task is inherently ``underspecified'' (\ie reconstruction is error-prone). 
\passed{\amz{This sentence is a bit vague and hard to follow. I also am not convinced it is needed, unless this "underspecification" of the inpainting comes up later. } }
In contrast, \name jointly trains the NN encoder and NN decoder, which allows the encoder to produce data that is easier to be reconstructed accurately when partially received. 
% Moreover, \name's encoded file size does not grow with more packets. 
\passed{\yc{to make it clear: empirically, even the sota dnn method is not working well + reasoning (citation): inpainting is hallucinating}
\yc{encoder is agnostic to loss/inpainting, so every bit have some information. if packet is lost, the information is not recoverable. inpainting is trying to generate the missing information (movement) by hallucinating}}

\mypara{Other schemes}
There are several other techniques that are might help mitigate the impact of packet loss, but their primary goals are not loss resilience, so they are less resilient to packet loss than the aforementioned schemes. 
But for completeness, we discuss some notable schemes here and also qualitatively compare \name against several of them in \S\ref{sec:eval}.

\passed{\jc{the following paras should be greatly tightened}\yc{already looks good to me}}

Scalable video coding (SVC)~\cite{schwarz2007overview, schierl2007mobile, swift} and fine-granularity scalability (FGS)~\cite{li2001overview,ma2022deepfgs} 
%\amz{same citation twice here}
 optimize the notion of rate-distortion (RD) tradeoff---video quality achieved by a single encoded bitstream under different received bitrates.
%Recent work also shows that neural encoders can improve SVC compression~\cite{swift}.
SVC encodes a video in multiple quality layers and sends data {\em layer by layer}.
This works well for on-demand videos~\cite{swift,grad}, but real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{subsec:background}), so a packet loss can occur to any layer, and a new packet may not always improve quality, if the lower layers are not fully received.
For this reason, SVC is rarely used to improve unicast real-time video (though it is used widely by multicast videos to serve users with heterogeneous network capacities~\cite{schierl2007mobile}).

%so that each newly received packet (or layer) will incrementally improve quality. 
%However, because it imposes a hierarchical order among the packets of a frame, 
%one missing packet can affect all higher quality layers, even if more packets are received in the higher quality layers.
%Though sending each layer reliably one by one is possible in on-demand videos~\cite{swift,grad}, real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{subsec:background}), so packet loss can affect any layer.
%As a result, SVC is rarely used to improve unicast real-time video (though it is used widely by multicast videos to serve users with heterogeneous network capacities~\cite{schierl2007mobile}).


Frame skipping might be another option if other error concealment schemes are not available.
%The encoder and decoder can work jointly to decide when skipping a frame does not hurt quality and the decoding states. 
For instance, Salsify~\cite{salsify} uses an older but reliably received frame, instead of the last frame, as the reference frame, so the decoder can safely skip a loss-affected frame without hurting subsequent frames.
However, it needs more bits to encode the same quality than using the last frame (which has a much smaller difference from the current frame) as the reference frame
(\eg the P-frames between every other frame are 40\% greater in size than between two consecutive frames).
Long-term reference frame (LTR) technique~\cite{zhang2008error} makes each P-frame individually decodable if the long-term reference is received, no matter whether there is packet loss in between or not. 
However, it shares a similar problem of large size overhead as Salsify.
Voxel~\cite{voxel} lets the decoder skip a loss-affected frame if the encoder indicates that skipping the frame does not affect video quality.
It works well for on-demand videos where B-frames can be safely skipped, and the impact of a skipped frame will stop at the next chunk within a few seconds. 
Unfortunately, neither apply to real-time videos. 


Deep learning has long been used in multimedia. 
It has been used to improve compression efficiency (\eg~\cite{dvc,elf,hu2021fvc,swift, NEURIPS2021_96b250a9}), enhance quality (\eg super resolution~\cite{sivaraman2022gemino,kim2020neural,neuroscaler}), scalable video coding (\eg~\cite{swift,ma2022deepfgs}) and postprocessing error concealment (\eg~\cite{reparo, xiang2019generative, kang2022error, sankisa2018video, mathieu2015deep}).
However, the fundamental limitations of these approaches remain despite the use of deep learning.

Loss resilience has also been studied under specific assumptions, such as availability of multiple paths~\cite{meng2022achieving}, early retransmission driven by router feedback~\cite{zuo2022deadline}, and low-latency networks~\cite{ray2022sqp}.
We do not make special assumptions in this work.



\tightsubsection{Autoencoder background}
\label{subsec:ae-background}

% \jc{this section needs more work}

%\jc{refer to fig~\ref{fig:dvc-arch}}


Our work is based on autoencoders, which use learned NNs instead of handcrafted logic, to encode and decode video frames.
Autoencoders have recently reached competitive and even better compression efficiency than traditional video codecs. 
Several factors contribute to this advance.
First, rather than encoding a frame with a monolithic NN, recent autoencoders take advantage of logical components commonly found in classic video codecs (\S\ref{subsec:background}),
% \footnote{For this reason, most autoencoder-based video coding focuses on inter-frames, the most common frame type in real-time videos. Our work also focuses on inter-frame coding and will include I-frame in \S\ref{subsec:protocol}.}, 
such as motion estimation, compensation, and transformation compression of residual and motion vectors.
Then they replace the handcrafted heuristics of classic codecs with NNs that can learn more complex algorithms from data.
Second, these autoencoders are trained on a large corpus of videos (\eg Vimeo-90K~\cite{vimeo-dataset}), so their compression efficiency can reasonably generalize across a variety of video content (which we also observe in our evaluation \S\ref{sec:eval}).
For these reasons, autoencoders attract increasing attention in the multimedia community~\cite{dvc, swift, hu2021fvc}.

% % (We will discuss I-frame in \S\ref{subsec:protocol}, and B-frames are rarely used in real-time videos~\cite{ffmpegstreaming}.)
% It is comprised of steps (\eg motion and residual estimation) typically found in a traditional video codec (\S\ref{subsec:background}) but  uses NNs to replace
% %Most recent video autoencoders~\cite{??,??,??} combine useful concepts from traditional codecs (\eg motion vectors and residuals) and replace 
% handcrafted heuristics for motion estimation, compensation, and \st{transformation} \edit{compression} of residual and motion vectors.
% %, and they achieve compression efficiency comparable to recent video codecs.
% %, and achieve comparable compression efficiency as recent compression algorithms.

%\mypara{Limitations}



\begin{figure*}[t!]
    \centering
         \centering
        %\includegraphics[width=0.97\linewidth]{figs/dvc-arch-v3.pdf}
        % \includegraphics[width=0.93\linewidth]{figs/dvc-arch-v3.pdf}
        \includegraphics[width=0.93\linewidth]{figs/dvc-arch-v4.pdf}
    \tightcaption{Workflow of the autoencoder in \name.}
    \label{fig:dvc-arch}
\end{figure*}

Our work adopts the DVC architecture~\cite{dvc}, a popular autoencoder (depicted in Figure~\ref{fig:dvc-arch}).
Two properties of autoencoders make them particularly suitable for loss resilience.
\begin{packeditemize}

\item {\bf Generative:} The decoding part in autoencoders, such as DVC, can {\em generate} frames with any vector in the encoded latent space as input. 
In other words, it can decode not only the encoder's output but also other vectors that look similar to the encoder's output. 
This means that if we randomly perturb the values in the encoder output (such as zeroing some random values or adding a Gaussian noise), the NN decoder can still successfully decode the frame, though the quality will have a non-trivial drop compared to without the perturbation.

\item {\bf Learnable:} Autoencoders can decode any vector in the encoded latent space but the decoded quality can be quite poor. 
Fortunately, the encoder and the decoder are {\em learnable} NNs that can be trained to optimize decoded quality in the presence of perturbations like random zeroing. 
For instance, the decoder can learn to be less sensitive to perturbed values, and the encoder can learn to add slight redundancy that helps the decoder accurately correct perturbed values.

\end{packeditemize}

Nonetheless, existing autoencoders as-is still lack tolerance to packet loss for two reasons.
%still requires traditional schemes (like FEC) to handle packet loss. 
%Their lack of packet loss tolerance is due to two reasons.
First, the standard autoencoder training implicitly assumes that the encoder's output equals the decoder's input,
% \footnote{A recent work~\cite{??,??} adds Gaussian random noise\jc{check!} between the encoder and decoder to simulate wireless signal noise, but this is different from packet loss which masks a fraction of the data.}, 
so it does not prepare the autoencoder to handle data loss between the encoder and decoder. 
Second, entropy encoding used in autoencoders compresses the whole encoder output as a single bitstream, so any data loss will render it undecodeable.

\name is an attempt at transforming autoencoders to be resilient to packet loss at different rates.
Our work is related to an emerging line of work on deep joint source-channel coding~\cite{kurka2020deepjscc, pmlr-v97-choi19a} which trains an autoencoder to code images in a representation that is both compact and robust to signal noises.
\name differs on two key fronts. 
First, they target physical-layer protection against signal noises.
% is different from (and complementary to) transport-/application-layer protection against packet losses. 
While physical-layer noises can be modeled as differentiable linear transformations (as in~\cite{bourtsoulatze2019deep,gunduz2019machine}), packet drops are not naturally differentiable and need to be handled differently. % (see \S\ref{subsec:sim-losses}). 
Second, unlike compressing individual images, frames in a streaming video cannot be treated separately, otherwise, any error on one frame may propagate to future frames. 


\tightsubsection{Summary}

In summary, traditional error-resilient methods fall short to optimize quality under different packet loss rates.
On one hand, forward error coding optimizes quality only under a pre-determined loss rate, and postprocessing error concealment suffers suboptimal quality under a range of loss rates.
On the other hand, autoencoders can potentially tolerate data perturbation at any rate, but they cannot tolerate packet loss.

By contrast, a better coding scheme should optimize quality under different packet loss rates. 
We call it {\em data-scalable (DS) coding}.
With the same encoding of each frame, DS coding obtains quality similar to the classic codec (H.265) used in WebRTC without FEC when there is no packet loss; and with higher packet loss rates, the quality gradually degrades but is still better than state-of-the-art loss-resilient schemes.
In the next two sections, we will describe an autoencoder-based solution to approximate the effect of DS coding.

%the aforementioned solutions either sacrifice the quality in absence of packet loss or fail to get decent quality in presence of high packet loss rates.
%As we will see, \name shows a more desirable relationship between quality and packet loss rate.





==> sections/old/motivate_v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\section{Background}



% Real-time video, it is crucial that enough data is timely received for each frame, so that the high-quality frames can be rendered at a fixed interval (\eg every 50ms for 20fps). 
% However, as most packet networks have occasional congestion, delay jitter and packet losses, not all packets of a frame may arrive timely.
% Retransmitting missing packets is also inefficient if the round trip time is long.
% Therefore, loss-resilient schemes are required to ensure that a frame can be decoded at a high quality even if a fraction of its packets have not arrived when it is supposed to be decoded, \ie non-zero deadline-missing rate or \rate. 



\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.85\linewidth]{figs/motivate_example_placeholder.pdf}
         \label{fig:}
    \caption{}
    \label{fig:motivate-example}
\end{figure}

\subsection{Prior Loss-Resilient Schemes}


With occasional congestion and packet jitter and losses in most packet networks, it is desirable that a real-time video client can decode and render the next frame as soon as a subset of its packets are received.
Therefore, loss-resilient techniques have seen intensive research for over two decades, despite that other types of streaming videos (YouTube, Netfliex) have long become TCP-based. 

\mypara{Forward error correction (FEC)}
We start with FEC as it is the most widely used loss-resilient scheme in today's real-time video systems (mostly WebRTC-based). 
(Other loss-resilient schemes (\fillme) will be discussed shortly.)
Put simply, an optimal FEC takes any file of size $M$ bytes, codes it with redundancy bits, and sends the coded data out.
The receiver can then decode the coded data as long as {\em any} $M$ bytes are received. 
Fountain code is a variant of FEC that does not limit the size of the coded data, so the sender can send as many bytes as it wants, and the receiver can decode it once $M$ bytes have arrive. 
Readers can refer to~\cite{??,??} for a more in-depth introduction of FEC.
FEC has been studied intensively in the IEEE multimedia community, with \fillme and \fillme achieving near-ideal performance of FEC and fountain codes.
For simplicity, this paper assumes ideal FEC (\ie the coded data generated from $M$ bytes is decodable once any $M$ bytes are received)\footnote{\jc{a footnote on the suboptimal use of fec in webrtc}}.


FEC is known to have the ``cliff effect'': for a given data (a frame or chunk encoded by a video coder like H.265), no matter how FEC adds redundancy, at least as many bytes as in the original data must be delivered.
And since the decoded video quality remains the same even if more bytes arrive (Figure~\ref{fig:intro-example}), the video coder should encode the video at the highest sustainable bitrate. 
If we know that under the sending rate of $c$, $r$ fraction of data will not arrive timely (\eg when a frame should be rendered), then ideally, the video should be encoded at bitrate $c\cdot(1-r)$ and sent with redundancy rate $r$. 
With less redundancy, the receiver must wait longer for more packets to arrive or retransmit; with more redundancy, the video bitrate will be lowered.
Thus, {\em FEC will be most effective {\bf if} the sender knows how many bytes can be timely delivered in advance.} 
% For a link of 4Mbps and negligible RTT, to deliver a frame within 100ms, the ideal frame size cannot exceed 50KB; otherwise, no matter how FEC adds redundancy, it always takes longer than 100ms for FEC to get enough bytes to decode the frame. 
% To see why this may be problematic, consider streaming a video of 20fps over a hypothetical network connection of 5Mbps (with zero RTT). 
% over a link of 4Mbps and negligible RTT, no matter how FEC adds redundancy, it will always take about one second to deliver 200KB of data required for FEC to recreate the frame data. 
% Otherwise, the frame has to be skipped, and the last decoded frame will fill in, causing degraded visual quality\jc{need a citation or some justification}. 
% To pick an appropriate redundancy rate, FEC-based loss-resilient schemes have developed various algorithms to predict future \rate based on history network conditions and current sending rate (\eg~\cite{??,??,??}). 
% , in order to determine how fast data should be sent out ($c$) and how much redundancy should be introduced ($r$), such that $c\cdot(1-r)$ matches the receiving data rate at the receiver.
Despite many efforts to predict packet loss rate, pick a desirable redundancy rate before knowing the future \rate is hard, especially
% But since $r$ is picked {\em before} the data is sent, it is hard to always pick a desirable \rate, 
if \rate changes dynamically and non-stationarily in packet networks.\footnote{In fairness, FEC is effective at concealing random packet losses in wireless channels with a largely stable erasure rate.
Moreover, the FEC redundancy can help the sender to quickly probe bandwidth~\cite{??}.}



% Given a target sending rate $w$ decided by a congestion control logic, if the estimated \rate (the fraction of data not arriving by the time decoder wishes to decodes the data) is $r$, a video frame will be compressed by a video encoder at a bitrate $b=w\cdot(1-r)$ and then coded by FEC with redundancy of $c\cdot r$.
% An adaptive logic is then needed to determine the FEC redundancy rate (\eg~\cite{??,??,??}).
% % This is feasible when the \rate $r$ for a sending rate $w$ is reliably estimated, but 
% However, \rate often changes dynamically and non-stationarily in packet networks.

\jc{an example figure of dmr over time here, with fec logic}

Figure~\ref{??} gives an example of why setting the FEC redundancy rate is difficult. 
We run WebRTC against a bandwidth trace sample from \fillme over a network link of RTT \fillme and a droptail queue of \fillme.\footnote{We enable the \fillme option\jc{bw probing and fec} to allow fast sending adaptation, and the FEC redundancy rate is dynamically determined by the default history-based logic. \cite{??, ??} offer a comprehensive description of WebRTC's congestion control and FEC logic.}
Figure~\ref{??} shows that the frame delays (the time between sending a frame and enough bytes received to decode it) is littered with sporadic periods of sudden spikes.
When bandwidth suddenly drops, the sending rate and the FEC redundancy rate cannot adjust timely, causing many packets to arrive late and delaying the rendering of several subsequent frames. 
The long delays could have been mitigated, if we let FEC adapt more conservatively (\eg increase redundancy faster but decrease it more slowly), as shown \fillme. But this is at the cost of much lower video quality, as more bytes are used for redundancy.
Techniques like dynamic reference selection~\cite{salsify} may mitigate this issue, but could not have avoided the congestion and delay of the first few frames as elaborated in \S\ref{??}.

\jc{mention the findings corroborate with \cite{\url{https://docs.google.com/document/d/1Hg1SaLEl6T4rEU9j-isovCo8VEjjnuCPTcLNJewj7Nk/edit}}}


\jc{need a figure here to clarify different between video coder and fec coder}

\mypara{Loss-resilient video coding}
In addition to FEC (and other channel-coding schemes), prior work has also studied loss-resilient video coding techniques, which add redundancy during the video codec (\eg H.265) rather than after. 
These schemes are usually called ``source coding'' in the multimedia literature.
For instance, \jc{explain R/D optimization, unequal protection, and dynamic reference selection}




\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.6\linewidth]{figs/motivate_regime.pdf}
         \label{fig:}
    \caption{}
    \label{fig:motivate-regime}
\end{figure}


\mypara{Compression efficiency vs. loss resilience}
Both FEC-based schemes and loss-resilient video coding face a fundamental limitation:
compared to traditional coder (\eg H.265) that are optimized for video coding efficiency (less bits for higher quality), these loss-resilient coders are less efficient in that they use more bits (\ie redundancy) to obtain same quality in the absence of any packet loss (\ie zero \rate).
In other words, they must trade compression efficiency for loss resilience, so the rate of redundancy is highly sensitive to \rate prediction. 
\jc{a few more examples on how various video coders trades compression efficiency for loss resilience}



\jc{add a figure of unpredictable dmr vs long delay}

Figure~\ref{fig:??} illustrates when existing schemes are effective.
When the RTT of the connection is low compared to the desirable frame delay, packet retransmission would be sufficient to conceal any packet losses.
When the \rate of the next frame is stationary or largely predictable, FEC-based schemes will be sufficient. However, current solutions will fall short in the case of high RTT and highly dynamic \rates.



Connections with dynamic \rates and high RTT are not rare in practice. 
For instance, we can run a ``what-if'' analysis over the trace of Figure~\ref{??} to reveal the \rate of each frame if a maximum frame delay of \fillme is imposed. 
We keep the same congestion control logic and measure how much data of each frame arrive at the receiver after the maximum frame delay. 
We see \rate varies just as much as the frame delays, especially when bandwidth suddenly drops.
It is not surprise then that existing FEC logic in WebRTC cannot always set an appropriate FEC redundancy rate that is high enough to maintain a low tail frame delay, but not too high to sacrifice video bitrate.
% if a frame has a \rate of 30\%, the optimal FEC redundancy rates would have been 30\% (\ie video encoding bitrate is 70\% of the sending rate, if such encoding is available). 
% We can see that the optimal redundancy rates can be just as highly dynamic as the frame delays.


In summary, existing loss-resilient schemes encode video based on estimated \rate and are most effective only when the estimation is accurate. 
Overestimation leads to too much redundancy and low video quality, but underestimation cause more retransmission and video frame delays.



\subsection{Autoencoders}


This work is framework built on autoencoders, an emergent class of learned coders for video frames, including I-frames and P-frames.
Compared to early autoencoder variants, recent autoencoders obtain much better compression efficiency, thanks to higher-capacity encoder/decoder DNN architectures that can be trained on large set of videos (\eg Vimeo-90K~\cite{??}). 
Like traditional codecs, recent video autoencoders compute and compress motion vector estimation and residuals separately, rather than compressing each frame from scratch. 
These optimizations improve not only compression efficiency but also generalization of these NN-based autoencoders.


\mypara{Caveats}
Though various autoencoders are studied extensively in the computer vision community, there has been surprisingly little attention given to careful comparison between autoencoders and traditional codecs (H.265 and H.264), leading to biased (and sometimes exaggerated) perception of autoencoders's performance. 
Traditional video codecs have been extremely heavily engineered, but if one tests an autoencoder and H.265 under the same small (4-10) GoP, autoencoders can outperform H.265, because small GoPs align better with how autoencoders are trained but are not what H.265 is designed for. 
Such comparison can be unfavorable to autoencoders as well.
For instance, H.26x obtains better motion vector estimation and smaller residuals by searching for {\em multiple} reference frames, whereas most designs of autoencoders derive motion vectors and residuals only a {\em single} reference frame (which is not a fundamental constraint), but instead focus on better compression of the motion vectors and residuals.
To make it more complicated, autoencoders are trained to optimize PSNR (pixel distortion) whereas traditional codecs are designed with YUV-SSIM in mind\cite{some citation?}.

With these caveats in mind, we try our best to avoid such pitfalls in our evaluation of autoencoders and their baselines. (For space limitation, we elaborate the details in \S\ref{??}.)
For instance, we evaluate them in both PSNR and YUV-SSIM and do not limit the GoP of H.26x, but use their default encoding setting instead (\eg GoP of \fillme). 
We also disable B-frames (0 bframe and rc-lookahead) and use \texttt{fast} preset in H.26x, as in most real-time videos~\cite{??,??}\footnote{To be clear, we make sure that this is still unfavorable to autoencoders, since H.26x can still use multiple history frames as reference, but autoencoders only use one.}.
\jc{yihua: please find some citation/pointers to justify this choice.}
The bottom line is that our pre-trained autoencoder~\cite{??,??} (which \name customizes) is worse than H.265 with all optimizations, but without b-frame optimization, it is on par with H.265 and better than H.264.


Despite being emergent and relatively less engineered than traditional codecs, autoencoders are increasingly applied by the signal processing community for image compression~\cite{??,??} and wireless communication~\cite{??,??}, by multimedia community for high-volumetric video compression~\cite{??,??} and recently by the networking community to improve chunk-based video streaming~\cite{swift}.
Unlike this work, however, these efforts still rely on packets retransmission or traditional schemes (like FEC) to handle packet losses. 


==> sections/old/motivate_v3.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\section{Loss tolerance for real-time video}

\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.92\linewidth]{figs/primitive_table_new.pdf}
    \caption{Abstractions of different loss-resilient schemes. The differences are: 
    (1) unlike redundancy-based schemes, data-scalable coding does not depend on prediction of packet loss rate; and 
    (2) unlike retransmission-based or redundancy-based schemes which must retransmit lost packets until some {\em predefined set} or {\em minimum number} of packets are received, data-scalable delivery can decode a frame with any non-empty set of packets, and the quality gradually improves with every new packet.}
    \label{fig:primitive-table}
\end{figure*}


% Real-time video, it is crucial that enough data is timely received for each frame, so that the high-quality frames can be rendered at a fixed interval (\eg every 50ms for 20fps). 
% However, as most packet networks have occasional congestion, delay jitter and packet losses, not all packets of a frame may arrive timely.
% Retransmitting missing packets is also inefficient if the round trip time is long.
% Therefore, loss-resilient schemes are required to ensure that a frame can be decoded at a high quality even if a fraction of its packets have not arrived when it is supposed to be decoded, \ie non-zero deadline-missing rate or \rate. 



Many recent studies (\eg~\cite{??,??,??,??})\jc{YIHUA, please find more reference} have shown that intermittent congestion, packet jitter, and packet drops are not rare for real-time video applications in the wild. 
Consequently, a client may not have received all packets of a frame when the frame is due for decoding (\eg 40ms after the last frame was decoded if the video is 25fps).

Thus, the ability to tolerate packet losses\footnote{In this work, a packet loss can occur even if the packet is not dropped by the network; a packet is lost if it is delayed (due to congestion, path fluctuation, etc) and arrives after the receiver decodes the frame it belongs to.} is pressingly needed to allow a real-time video client to decode and render the next frame when only a subset of its packets are received.



\subsection{\hspace{-0.3cm}Abstractions of prior loss-resilience schemes}
\label{subsec:abstractions}


%This section revisits three general approaches to loss resilience taken by prior work.  

%\subsection{Prior Loss-Resilient Schemes}

Loss resilience has long been an important research topic. 
While the details vary greatly among different loss-resilient techniques, it helps to view them through the lens of the high-level abstractions that characterize how packets (coded data) are encoded and how {\em decoded video quality of a frame changes with received data (packets)}.
These abstractions also influence the interaction with the remaining of a real-time video application, such as congestion control and bitrate adaptation.


\begin{comment}
they have followed some high-level abstractions that characterize how packets (coded data) are encoded and how {\em decoded video quality of a frame changes with received data (packets)}.
%\vspace{-0.05cm}
%\begin{align}
%\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) & \rightarrow \{\texttt{pkts}\}_{sent}\\
%\texttt{\bf Decode}(\{\texttt{pkts}\}_{received}) & \rightarrow \texttt{quality}
%\label{eq:abstraction}
%\vspace{-0.05cm}
%\end{align}
%of certain loss-resilient performance in terms of video quality as a function of received data (packets). 
Viewing them through the lens of abstractions helps us understand their high-level loss-resilience behavior and  with the remaining of a real-time video application, such as congestion control and bitrate adaptation.

\end{comment}

\mypara{Retransmission-based loss resilience}
Packet retransmission is a conventional loss-resilient scheme. 
A client must retransmit packets until a {\em pre-determined set} of packets is reliably delivered. 
Thus the abstraction of retransmission-based loss resilience is:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(\{\texttt{pkts}\}_{received}\subseteq\{\texttt{pkts}\}_{predefined}) &\rightarrow \texttt{quality}\nonumber
\vspace{-0.05cm}
\end{align}
To make it more concrete, we discuss two representative types of retransmission-based schemes.

\smallskip
{\em Single-bitrate coding} must retransmit every lost packet of a video frame for the frame to be decodable. 
When all packets arrive the quality is as high as the original encoded quality.
%This RTX's abstraction can be viewed as ``a frame is non-decodable until all its packets are received, at which point the quality is as high as the original encoded quality.''
This basic scheme is known to have high tail delays if a few packets are resent between two clients whose RTT is higher than inter-frame interval. 

\smallskip
{\em Scalable video coding (SVC)} encodes a video in multiple quality layers, in a way that if a packet of one layer is lost while all packets of lower layers are received, the lower layers can still be decoded.\footnote{\jc{a note on why we dont consider the redundancies in svc}}
Thus, the abstraction of SVC is that ``quality reaches that of the layer $i$ if all packets belonging $i$ and all lower layers have been received.''
That said, a packet loss in SVC can render all higher layers non-decodable. 
For this reason, the base (lowest) layer is often protected by FEC, \ie unequal-protected (UEP) SVC~\cite{wang2000error}, but any packet loss at any other layers can still affect multiple layers. 

Because a pre-determined set of packets will be always be reliably delivered by retransmission, the video coding can focus on compression efficiency (maximal quality under a given target bitrate without any redundancy). 
However, in lack of any redundancy-based techniques, a frame is decodable only if a certain set of packets are received in its entirety, so any lost packets might block the decoding of a frame, making retransmission inevitable in many cases. 
For this reason, most real-time video systems use retransmission together with some redundancy-based loss-resilient techniques, so only a selective set of lost packets need to be resent. 




\mypara{Redundancy-based loss resilience}
Unlike retransmission, redundancy-based techniques trade compression efficiency for loss resilience. 
As long as an enough {\em number} of packets are received, the frame will be decodable at a decent quality. 
The abstraction of redundancy-based loss resilience is characterized by:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}, \texttt{redun}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}},\texttt{redun}) &\rightarrow \texttt{quality}\nonumber
\nonumber
\vspace{-0.05cm}
\end{align}
This equation entails the efficiency-resilience tradeoff: higher redundancy \texttt{redun} leads to lower $\alpha_{\texttt{redun}}$ (\ie higher loss resilience), but it also means lower resulting quality if $|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}}$ (\ie lower coding efficiency).
Here, we discuss two concrete redundancy-based schemes.

\smallskip
{\em Forward error correction (FEC)} is widely used in most WebRTC-based real-time video systems.\footnote{\jc{a footnote on the suboptimal use of fec in webrtc}}
Put simply, an idealized FEC takes an encoded video frame (or any file) of size $M$ packets, codes it with redundancy bits, such that the receiver can then recover the data as long as {\em any} $M$ packets\footnote{This work assume equal-sized packets. This is aligned with existing applications, \fillme} are received. 
FEC has been studied intensively in the IEEE multimedia community, with \fillme and \fillme achieving near-ideal performance of FEC and fountain codes. (\cite{??,??} give a more in-depth introduction of FEC.)
Therefore, FEC's abstraction can be described as ``the quality of a frame is low (undecodable) until {\em any} $M$ packets are received.''

FEC suffers the well-known ``cliff effect''. 
For a given data (a frame or chunk encoded by a video coder like H.265), no matter how much redundancy is added, at least as many bytes as in the original data must be delivered, and the decoded video quality remains the same even if more bytes arrive.
Thus, the video encoder should ideally encode each video frame at exact the bitrate that matches the amount of data received when the frame is decoded. 
As a consequence, {\em FEC is effective {\bf if} the sender knows how many bytes can be timely delivered in advance.} 
With less redundancy, the receiver must wait for more packets to arrive or be retransmitted; with more redundancy, the video quality will be low.



\smallskip
{\em Intra-MB insertion}
The multimedia community has also proposed techniques to make video coding (\eg H.264) resilient to packet losses by keep more existing pixel-level redundancy during the video coding process (as opposed to FEC which adds redundancy on top of an encoded frame).
The idea is to reduce the inter-dependencies between macroblocks that are potentially similar to each other. 
For instance, \jc{Yihua, explain R/D optimization, intra-MB insertion, dynamic reference selection, etc}
\jc{need a footnote here to describe how entropy encoding can be stopped at the boundary between packets. }

Like FEC, with more pixel-level redundancy preserved, data erasures have less impact, but compression efficiency is lowered at the same time. 
In practice, with all packets, the decoded quality of intra-MB insertion is lower than that of the coding algorithm that is optimized for coding efficiency (\ie no redundancy), and while a small fraction of data losses can be efficiently tolerated, a high loss rate (more than 40\% data erasure) will still render a frame undecodable~\cite{??,??}. 

\jc{need a footnote to discuss frame skipping and reference frame selection!!!}


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.85\linewidth]{figs/motivate_example_placeholder.pdf}
         \label{fig:}
    \caption{\jc{YIHUA, let's run WebRTC (with FEC adaptation turned on) on a simple bandwidth trace like this.}}
    \label{fig:motivate-example}
\end{figure}


\mypara{Limitations}
Retransmission-based schemes become less effective than redundancy-based schemes under longer propagation delays between clients. 
However, compared to traditional coders (\eg H.265) that are optimized for video coding efficiency (less bits for higher quality), the redundancy-based abstractions are less efficient in that they use more bits to obtain same quality in the absence of any packet loss.
%That is, they must trade compression efficiency for loss resilience, so the rate of redundancy is highly sensitive to \rate prediction. 
Thus, these abstractions of loss resilience are effective only if they can predict future packet loss rate and jitter, which is not always possible in practice. 

Figure~\ref{fig:motivate-example} gives an example of why setting the FEC redundancy rate is difficult. 
We run WebRTC against a simple bandwidth trace over a network link of RTT \fillme and a droptail queue of \fillme.\footnote{We enable the \fillme option\jc{bw probing and fec} to allow fast sending adaptation, and the FEC redundancy rate is dynamically determined by the default history-based logic. \cite{??, ??} offer a comprehensive description of WebRTC's congestion control and FEC logic.}
%Figure~\ref{??} shows that the frame delays (the time between sending a frame and enough bytes received to decode it) is littered with sporadic periods of sudden spikes.
When bandwidth suddenly drops, the sending rate and the FEC redundancy rate can adjust only after any sign of congestion is returned to the sender (after at least one RTT), causing many packets to arrive late and delaying the rendering of several subsequent frames. 
The long delays could have been mitigated, if FEC adapts more conservatively (\eg increase redundancy faster but decrease it more slowly). 
But this is at the cost of much lower video quality, as more bytes are used for redundancy when bandwidth is stable.
Techniques like dynamic reference selection~\cite{salsify} may mitigate this issue, but could not have avoided the congestion and delay of the first few frames as elaborated in \S\ref{??}.

\jc{mention the findings corroborate with \cite{\url{https://docs.google.com/document/d/1Hg1SaLEl6T4rEU9j-isovCo8VEjjnuCPTcLNJewj7Nk/edit}}}


\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.6\linewidth]{figs/motivate_regime.pdf}
    \caption{Traditional abstractions (retransmission-based and redundancy-based) for loss resilience are suitable for connections with low latency or predictable packet loss rates, respectively. However, they are less effective if latency is long and packet loss rate is highly dynamic.}
    \label{fig:motivate-regime}
\end{figure}

To summarize, Figure~\ref{fig:motivate-regime} illustrates when existing schemes are effective.
When the RTT of the connection is low compared to the desirable frame delay, packet retransmission would be sufficient to conceal any packet losses.
When the packet loss rate of the next frame is largely predictable, FEC-based schemes will be sufficient. 
In short, current abstractions fall short in the case of high RTT and highly dynamic packet jitters and losses.



\subsection{Data-scalable video delivery}

To overcome the limitations of prior loss-resilient schemes, we envision a new abstraction of loss resilience---{\em data-scalable} delivery, which entails two specific requirements.
{\em (i)} First, a frame is encoded in a way that is not dependent on the prediction of future packet losses.
%{\em (ii)} Second, the decoded quality with {\em any} $x\%$ ($x>0$) received packets is lower but still comparable to classic codec (\eg H.265) with $x\%$ FEC redundancy.
%Note that classic coder $x\%$ with  can be viewed as a reference design that optimizes compression efficiency, not loss resilience.
{\em (ii)} The frame is decodable once {\em any} non-empty subset of its packets are received and the quality improves with more packets received.
%\item 
%\end{packeditemize}
Using the form of prior loss-resilience abstractions, data-scalable delivery is:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}|) &\rightarrow \texttt{quality}\nonumber
\nonumber
\vspace{-0.05cm}
\end{align}

Figure~\ref{fig:primitive-table} illustrates the difference between data-scalable delivery and other loss-resilient techniques.
%,  illustrates an example frame whose coded data is delivered in six packets arriving at the receiver at an arbitrary order. 
The most noticeable benefit of data-scalable delivery is that, while the exact arrival time of each packet is unknown to the receiver, data-scalable delivery offers the receiver the {\em flexibility} to decode a frame anytime after receiving any one of the packets. 
Moreover, each new packet strictly improves quality.

It helps to compare data-scalable delivery with SVC whose quality increase with throughput. 
However, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets.
As a result, each new packet does not always improve quality until all packets of a higher layer (and all layers below it) have been received. 
In other words, a missing packet may disproportionally render multiple quality layers undecodable. 
For this reason, in practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).




\subsection{Why autoencoder?}
\label{subsec:why-autoencoder}

This work is framework built on autoencoders, an emergent class of learned coders for video frames, including I-frames and P-frames.
Compared to early autoencoder variants, recent autoencoders obtain much better compression efficiency, thanks to higher-capacity encoder/decoder DNN architectures that can be trained on large set of videos (\eg Vimeo-90K~\cite{??}). 
Like traditional codecs, recent video autoencoders compute and compress motion vector estimation and residuals separately, rather than compressing each frame from scratch. 
These optimizations improve not only compression efficiency but also generalization of these NN-based autoencoders.

\mypara{Autoencoder-based data-scalable coding}
We base our approach on autoencoder, not only because of its potential compression efficiency, but more importantly, the performance of several autoencoders (albeit suboptimal) naturally fits the definition of data-scalable delivery. 
For example, we consider a pre-trained I-frame autoencoder~\cite{??} and a pre-trained P-frame autoencoder~\cite{??}. 
To emulate the effect of packet losses, we randomly erase \fillme\% of values in the autoencoder-returned data (without entropy encoding). 
We will explain how this random data erasure simulates packet losses in \S\ref{??}.
Figure~\ref{fig:autoencoder-pretrained} shows that as more data is received, the decoded quality gradually improves. (The test is on a different video dataset than the training dataset.)
It is very encouraging that even the pre-trained autoencoders produce data-scalable delivery.


\begin{figure}[t!]
    \centering
%    \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/psnr-loss-vs-pretrained.pdf}
%         \caption{P-frame model}
%         \label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/autoencoder_pretrained_qmap_v1.png}
%         \caption{I-frame model}
%         \label{fig:}
%     \end{subfigure}

         \includegraphics[width=0.6\linewidth]{figs/psnr-loss-vs-pretrained.pdf}

    \caption{Loss resilience of an example pre-trained autoencoder (red). It is already data-scalable (decodable with any subset of packets), but the quality drops much faster than the graceful degradation observed in our solution. \jc{YIHUA, make the figure wider. Swap the order of the legend to "Pre-trained autoencoder" and "Our custom autoencoder"}
%    Our models has a more graceful quality degradation under packet losses comparing to pretrained models
    }
    \label{fig:autoencoder-pretrained}
\end{figure}

However, with these pre-trained autoencoders, the quality grows quite {\em slowly} only a few packets are received. 
This is expected, since these autoencoders are not trained to realize data-scalable delivery. 
Our goal in the remaining of the paper is two-fold: (1) creating better data-scalable autoencoders that produce better quality under various packet losses, and (2) designing a custom real-time video delivery system on top autoencoders as a codec, which strikes better balance between frame delay and video quality. 

\mypara{Caveats of autoencoders}
Though various autoencoders are studied extensively in the computer vision community, there has been surprisingly little attention given to careful comparison between autoencoders and traditional codecs (H.265 and H.264), leading to biased (and sometimes exaggerated) perception of autoencoders's performance. 
Traditional video codecs have been extremely heavily engineered, but if one tests an autoencoder and H.265 under the same small (4-10) GoP, autoencoders can outperform H.265, because small GoPs align better with how autoencoders are trained but are not what H.265 is designed for. 
Such comparison can be unfavorable to autoencoders as well.
For instance, H.26x obtains better motion vector estimation and smaller residuals by searching for {\em multiple} reference frames, whereas most designs of autoencoders derive motion vectors and residuals only a {\em single} reference frame (which is not a fundamental constraint), but instead focus on better compression of the motion vectors and residuals.
To make it more complicated, autoencoders are trained to optimize PSNR (pixel distortion) whereas traditional codecs are designed with YUV-SSIM in mind\cite{some citation?}.

With these caveats in mind, we try our best to avoid such pitfalls in our evaluation of autoencoders and their baselines. (For space limitation, we elaborate the details in \S\ref{??}.)
For instance, we evaluate them in both PSNR and YUV-SSIM and do not limit the GoP of H.26x, but use their default encoding setting instead (\eg GoP of \fillme). 
We also disable B-frames (0 bframe and rc-lookahead) and use \texttt{fast} preset in H.26x, as in most real-time videos~\cite{??,??}\footnote{To be clear, we make sure that this is still unfavorable to autoencoders, since H.26x can still use multiple history frames as reference, but autoencoders only use one.}.
\jc{yihua: please find some citation/pointers to justify this choice.}
Moreover, we always train autoencoders on the same dataset (Vimeo-90K~\cite{??}) but report the test result on different datasets.
The bottom line is that our pre-trained autoencoder~\cite{??,??} (which \name customizes) is worse than H.265 with all optimizations, but without b-frame optimization, it is on par with H.265 and better than H.264.


Despite being emergent and relatively less engineered than traditional codecs, autoencoders are increasingly applied by the signal processing community for image compression~\cite{??,??} and wireless communication~\cite{??,??}, by multimedia community for high-volumetric video compression~\cite{??,??} and recently by the networking community to improve chunk-based video streaming~\cite{swift}.
Unlike this work, however, these efforts still rely on packets retransmission or traditional schemes (like FEC) to handle packet losses. 




% \begin{figure}[t!]
%     \centering
%          \centering
%         \includegraphics[width=0.99\linewidth]{figs/primitive_example.pdf}
%     \caption{}
%     \label{fig:primitive_example}
% \end{figure}

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.99\linewidth]{figs/primitive_example_new.pdf}
%    \caption{}
%    \label{fig:primitive_example}
%\end{figure*}




%
%
%\jc{need to elaborate on this! need a "functional" description of the data-scalable primitive}
%

\begin{comment}


To  the limitations of the traditional loss-resilient schemes, we choose a different approach, by borrowing the concept of deep autoencoder and exploring its design choices in the context of \name, the first autoencoder-based real-time video system.
% We first describe the design choices of its autoencoder-based codec.

Before delving into the detailed design, we posit two requirements that should be met by an ideal codec for real-time video systems, which we refer to as {\em data-scalable} codec: 
\begin{packeditemize}
\item The video coding should be \rate-agnostic, and 
\item At any \rate ($<100\%$)\footnote{Importantly, the second requirement does {\em not} include \rate of 100\% (no data received).}, the decoded quality is near that of FEC-based loss protection if FEC knows the \rate. 
\end{packeditemize}
For instance, (see Figure~\ref{fig:intro-example}), \name's codec achieves similar quality as H.265 without FEC-based protection
% An example of such codec is the one we developed as part of \name.
As shown in Figure~\ref{??}, when \rate is zero, the quality is similar to that of H.265 without FEC-based protection, and as fewer packets are received (higher \rate) quality degrade {\em gracefully}, achieving similar quality as H.265 protected by an FEC redundancy rate that matches the \rate. 
\end{comment}


% This section introduces the basic design of our data-scalable video codec, and the next few sections will examine its design choices and how it should be used in an end-to-end real-time video system.






==> sections/old/motivate_v4.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\section{Loss tolerance for real-time video}

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.92\linewidth]{figs/primitive_table_new.pdf}
%    \caption{Abstractions of different loss-resilient schemes. The differences are: 
%    (1) unlike redundancy-based schemes, data-scalable coding does not depend on prediction of packet loss rate; and 
%    (2) unlike retransmission-based or redundancy-based schemes which must retransmit lost packets until some {\em predefined set} or {\em minimum number} of packets are received, data-scalable delivery can decode a frame with any non-empty set of packets, and the quality gradually improves with every new packet.}
%    \label{fig:primitive-table}
%\end{figure*}


% Real-time video, it is crucial that enough data is timely received for each frame, so that the high-quality frames can be rendered at a fixed interval (\eg every 50ms for 20fps). 
% However, as most packet networks have occasional congestion, delay jitter and packet losses, not all packets of a frame may arrive timely.
% Retransmitting missing packets is also inefficient if the round trip time is long.
% Therefore, loss-resilient schemes are required to ensure that a frame can be decoded at a high quality even if a fraction of its packets have not arrived when it is supposed to be decoded, \ie non-zero deadline-missing rate or \rate. 



Many recent studies (\eg~\cite{macmillan2021measuring,jansen2018performance,concerto,moulay2018experimental}) have shown that intermittent congestion, packet jitter, and packet drops are not rare and can cause long tail delay and low frame rate for real-time video applications. 
Consequently, a client may not have received all packets of a frame when the frame is due for decoding (\eg 40ms after the last frame was decoded if the video is 25fps).
Thus, the ability to decode a frame, despite packet losses (including those dropped or those delayed by congestion), is pressingly needed. 

\begin{comment}
Thus, the ability to tolerate packet losses\footnote{In this work, a packet loss can occur even if the packet is not dropped by the network; a packet is lost if it is delayed (due to congestion, path fluctuation, etc) and arrives after the receiver decodes the frame it belongs to.} is pressingly needed to allow a real-time video client to decode and render the next frame when only a subset of its packets are received.
\end{comment}


\subsection{\hspace{-0.3cm}Abstractions of prior loss-resilience schemes}
\label{subsec:abstractions}


%This section revisits three general approaches to loss resilience taken by prior work.  

%\subsection{Prior Loss-Resilient Schemes}

Loss resilience has long been an important research topic. 
While the details vary greatly among different loss-resilient techniques, it helps to view them through the lens of the high-level abstractions (summarized in Figure~\ref{fig:primitive-table}) that characterize how packets (coded data) are encoded and how {\em decoded video quality of a frame changes with received data (packets)}.
These abstractions also influence the interaction with the remaining of a real-time video application, such as congestion control and bitrate adaptation.


\begin{comment}
they have followed some high-level abstractions that characterize how packets (coded data) are encoded and how {\em decoded video quality of a frame changes with received data (packets)}.
%\vspace{-0.05cm}
%\begin{align}
%\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) & \rightarrow \{\texttt{pkts}\}_{sent}\\
%\texttt{\bf Decode}(\{\texttt{pkts}\}_{received}) & \rightarrow \texttt{quality}
%\label{eq:abstraction}
%\vspace{-0.05cm}
%\end{align}
%of certain loss-resilient performance in terms of video quality as a function of received data (packets). 
Viewing them through the lens of abstractions helps us understand their high-level loss-resilience behavior and  with the remaining of a real-time video application, such as congestion control and bitrate adaptation.

\end{comment}

\mypara{Retransmission-based schemes}
%Packet retransmission is a conventional loss-resilient scheme. 
A retransmission-based client takes in a video frame encoded by a traditional codec (\eg H.264) under a target bitrate, and it must resend lost packets until a {\em pre-defined set} of packets (pre-determined before the frame's packets are sent) is reliably delivered. 
This abstraction can be written as:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(\{\texttt{pkts}\}_{received}\supseteq\{\texttt{pkts}\}_{predefined}) &\rightarrow \texttt{quality}\nonumber
\vspace{-0.05cm}
\end{align}
To make the discussion more concrete, we consider two typical retransmission-based schemes.

\smallskip
{\em Basic TCP-based delivery} must retransmit every lost packet for a frame to be decodable. 
Once all packets are received, the quality will equal the original encoded quality.
%This RTX's abstraction can be viewed as ``a frame is non-decodable until all its packets are received, at which point the quality is as high as the original encoded quality.''
This scheme is known to suffer high tail delays, if the connection has an RTT longer than inter-frame interval.
%if a few packets are resent between two clients whose RTT is higher than inter-frame interval. 

\smallskip
{\em Scalable video coding (SVC)} encodes a video with multiple quality layers, such that a quality layer can be decoded as long as packets of this layer and all lower layers are received.
% \footnote{\jc{a note on why we dont consider the redundancies in svc}}
%if a packet of one layer is lost while all packets of lower layers are received, the lower layers can still be decoded.
%Thus, the abstraction of SVC is that ``quality reaches that of the layer $i$ if all packets belonging $i$ and all lower layers have been received.''
That said, a lost packet can render all higher layers non-decodable. 
Even if the base (lowest) layer is often padded with redundancy (\eg FEC, explained shortly)~\cite{wang2000error}, any packet loss at any other layers can still affect multiple layers. 

The advantage of the retransmission-based approach is that video coding can focus on compression efficiency (maximal quality under a given target bitrate), because a pre-determined set of packets will be always reliably delivered.
However, without any redundancy, a frame is decodable only if a pre-defined set of packets (all packets or those of a few layers) are received in its entirety. 
%any lost packets might block the decoding of a frame, making retransmission inevitable in many cases. 
To avoid blocking the decoding by a missing packet, retransmission is inevitable, but retransmission can be very slow in long-RTT networks, especially when the extra delay to request a lost packet is longer than the jitter buffer (\fillme), which result in a visually perceivable lag or skipped frame.
Therefore, retransmission is also complemented by some redundancy-based loss-resilient techniques, so only fewer lost packets need to be resent. 





\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.995\linewidth]{figs/primitive_table_new_v3.pdf}
    \caption{
Different abstractions of loss-resilient schemes. 
    Retransmission-based schemes (TCP, SVC) obtain high quality (the red horizontal line) but only if a predefined minimum {\em set} of packets are received.
    Redundancy-based ones (FEC, intra-MB) tolerate a pre-defined maximum packet loss rate by adding more redundancy (thus lower quality when all packets are received).
    In contrast, data-scalable delivery can decode a frame from any non-empty set of packets, gradually improves quality with {\em each} new packet, and achieves a high quality when all packets arrive. 
%    The differences are: 
%    (1) unlike redundancy-based schemes, data-scalable delivery does not need to add more redundancy to tolerate more predicted packet losses, and
%    (2) unlike retransmission-based schemes which must receive a predefined minimum {\em set} of packets, data-scalable delivery can decode a frame with any non-empty set of packets.
%    Comparing different abstractions of loss-resilient schemes. The differences are: 
%    (1) unlike redundancy-based schemes, data-scalable coding does not depend on prediction of packet loss rate; and 
%    (2) unlike retransmission-based schemes which must receive a predefined minimum {\em set} of packets, data-scalable delivery can decode a frame with any non-empty set of packets, and the quality gradually improves with every new packet.
%    (3) unlike redundancy-based ones which must receive a minimum number of packets, data-scalable delivery can decode a frame with 
    }
    \label{fig:primitive-table}
\end{figure}




\mypara{Redundancy-based schemes}
A frame is decodable when at least $N\%$ packets are received, but the decoded quality is lower with a smaller $N$.
Here, $(1-N\%)$ represents the redundancy rate, which depends on the predicted packet loss rate.
Effectively, redundancy-based schemes trade coding efficiency (more bits to obtain same quality) for loss resilience. 
The abstraction is:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}, N\%) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}| \geq N\%,N) &\rightarrow \texttt{quality}\nonumber
\nonumber
\vspace{-0.05cm}
\end{align}
%This equation entails the efficiency-resilience tradeoff: higher redundancy \texttt{redun} leads to lower $\alpha_{\texttt{redun}}$ (\ie higher loss resilience), but it also means lower resulting quality if $|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}}$ (\ie lower coding efficiency).
Redundancy-based schemes have been studied intensively in the IEEE multimedia community~\cite{??,??}.
Two typical redundancy-based schemes are FEC and intra-MB insertion.

%The abstraction of redundancy-based loss resilience is characterized by:
%\vspace{-0.05cm}
%\begin{align}
%\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}, \texttt{redun}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
%\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}},\texttt{redun}) &\rightarrow \texttt{quality}\nonumber
%\nonumber
%\vspace{-0.05cm}
%\end{align}
%This equation entails the efficiency-resilience tradeoff: higher redundancy \texttt{redun} leads to lower $\alpha_{\texttt{redun}}$ (\ie higher loss resilience), but it also means lower resulting quality if $|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}}$ (\ie lower coding efficiency).
%Here, we discuss two concrete redundancy-based schemes.

\smallskip
{\em Forward error correction (FEC)} is widely used in WebRTC-based applications.\footnote{\jc{a footnote on the suboptimal use of fec in webrtc}}. %(see \cite{??,??} for an in-depth discussion).
Ideally, FEC takes an encoded video/frame of size $M$ packets, codes it with redundancy bits, and the receiver can then recover the data if {\em any} $M$ packets\footnote{This work assume equal-sized packets. This is aligned with existing applications, \fillme} are received. 
%, with \fillme and \fillme achieving near-ideal performance of FEC and fountain codes. 
%Therefore, FEC's abstraction can be described as ``the quality of a frame is low (undecodable) until {\em any} $M$ packets are received.''
FEC suffers the well-known ``cliff effect''. 
To send a piece of data,
%(a frame or chunk encoded by a video coder like H.265), 
no matter how much redundancy is added, at least as many bytes as in the original data must be delivered, and the decoded video quality remains the same even if more data are received.
Thus, with less redundancy, the receiver must wait for more packets to arrive or be retransmitted; with more redundancy, the video quality will be low.
%Thus, the video encoder should ideally encode each video frame at exact the bitrate that matches the amount of data received when the frame is decoded. 



\smallskip
{\em Intra-MB insertion} does not explicitly add redundancy like FEC. 
% has also proposed techniques to make video coding (\eg H.264) resilient to packet losses by keep more existing pixel-level redundancy during the video coding process (as opposed to FEC which adds redundancy on top of an encoded frame).
Instead, it reduces the inter-dependencies between macroblocks that are potentially similar to each other. 
For instance, \jc{Yihua, explain R/D optimization, intra-MB insertion, dynamic reference selection, etc}
\jc{need a footnote here to describe how entropy encoding can be stopped at the boundary between packets. }


\jc{need a footnote to discuss frame skipping and reference frame selection!!!}


To tolerate packet losses, both intra-MB insertion and FEC must lower coding efficiency: FEC adds redundancy data and intra-MB insertion keeps more inter-macroblock redundancy.
Thus, {\em they are most effective, {\em if} the sender knows how many bytes can be timely delivered in advance}.



\begin{figure}[t!]
    \centering
      \begin{subfigure}[b]{0.8\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/webrtc-rate.pdf}
         \caption{Bandwidth and bitrate}
         \label{fig:}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.8\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/webrtc-delay.pdf}
         \caption{Frame delay}
         \label{fig:}
     \end{subfigure}
        \label{fig:}
    \caption{\jc{YIHUA, let's run WebRTC (with FEC adaptation turned on) on a simple bandwidth trace like this.}}
    \label{fig:motivate-example}
\end{figure}


Unfortunately, predicting how many packets will not arrive by time is hard. 
Figure~\ref{fig:motivate-example} gives an example of why setting the FEC redundancy rate is difficult. 
We run WebRTC against a simple bandwidth trace over a network link of RTT \fillme and a droptail queue of \fillme.\footnote{We enable the \fillme option\jc{bw probing and fec} to allow fast sending adaptation, and the FEC redundancy rate is dynamically determined by the default history-based logic. \cite{??, ??} offer a comprehensive description of WebRTC's congestion control and FEC logic.}
%Figure~\ref{??} shows that the frame delays (the time between sending a frame and enough bytes received to decode it) is littered with sporadic periods of sudden spikes.
When bandwidth suddenly drops, the sending rate and the FEC redundancy rate can adjust only after any sign of congestion is returned to the sender (after at least one RTT), causing many packets to arrive late and delaying the rendering of several subsequent frames. 
The long delays could have been mitigated, if FEC adapts more conservatively (\eg increase redundancy faster but decrease it more slowly). 
But this is at the cost of much lower video quality, as more bytes are used for redundancy when bandwidth is stable.
Techniques like dynamic reference selection~\cite{salsify} may mitigate this issue, but could not have avoided the congestion and delay of the first few frames as elaborated in \S\ref{??}.

\jc{mention the findings corroborate with \cite{\url{https://docs.google.com/document/d/1Hg1SaLEl6T4rEU9j-isovCo8VEjjnuCPTcLNJewj7Nk/edit}}}

\jc{also mention that fec is not native in webrtc. this is google implementation}

%Like FEC, with more pixel-level redundancy preserved, data erasures have less impact, but compression efficiency is lowered at the same time. 
%In practice, with all packets, the decoded quality of intra-MB insertion is lower than that of the coding algorithm that is optimized for coding efficiency (\ie no redundancy), and while a small fraction of data losses can be efficiently tolerated, a high loss rate (more than 40\% data erasure) will still render a frame undecodable~\cite{??,??}. 


\begin{comment}

\mypara{Limitations}
Retransmission-based schemes become less effective than redundancy-based schemes under longer propagation delays between clients. 
However, compared to traditional coders (\eg H.265) that are optimized for video coding efficiency (less bits for higher quality), the redundancy-based abstractions are less efficient in that they use more bits to obtain same quality in the absence of any packet loss.
%That is, they must trade compression efficiency for loss resilience, so the rate of redundancy is highly sensitive to \rate prediction. 
Thus, these abstractions of loss resilience are effective only if they can predict future packet loss rate and jitter, which is not always possible in practice. 

Figure~\ref{fig:motivate-example} gives an example of why setting the FEC redundancy rate is difficult. 
We run WebRTC against a simple bandwidth trace over a network link of RTT \fillme and a droptail queue of \fillme.\footnote{We enable the \fillme option\jc{bw probing and fec} to allow fast sending adaptation, and the FEC redundancy rate is dynamically determined by the default history-based logic. \cite{??, ??} offer a comprehensive description of WebRTC's congestion control and FEC logic.}
%Figure~\ref{??} shows that the frame delays (the time between sending a frame and enough bytes received to decode it) is littered with sporadic periods of sudden spikes.
When bandwidth suddenly drops, the sending rate and the FEC redundancy rate can adjust only after any sign of congestion is returned to the sender (after at least one RTT), causing many packets to arrive late and delaying the rendering of several subsequent frames. 
The long delays could have been mitigated, if FEC adapts more conservatively (\eg increase redundancy faster but decrease it more slowly). 
But this is at the cost of much lower video quality, as more bytes are used for redundancy when bandwidth is stable.
Techniques like dynamic reference selection~\cite{salsify} may mitigate this issue, but could not have avoided the congestion and delay of the first few frames as elaborated in \S\ref{??}.




\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.6\linewidth]{figs/motivate_regime.pdf}
    \caption{Traditional abstractions (retransmission-based and redundancy-based) for loss resilience are suitable for connections with low latency or predictable packet loss rates, respectively. However, they are less effective if latency is long and packet loss rate is highly dynamic.}
    \label{fig:motivate-regime}
\end{figure}

\end{comment}


%Figure~\ref{fig:motivate-regime} illustrates when existing schemes are effective.
In short, retransmission-based schemes are sufficient if the RTT between the clients is low enough to conceal the retransmission delay. 
%compared to the desirable frame delay, packet retransmission would be sufficient to conceal any packet losses.
Redundancy-based schemes are suitable to connections with largely predictable packet loss rate.
% of the next frame is largely predictable, FEC-based schemes will be sufficient. 
However, both of them fall short under high RTT and highly dynamic packet jitters and losses.



\subsection{New abstraction: Data-scalable delivery}

To overcome the limitations of prior loss-resilient schemes, we envision a new abstraction of loss resilience---{\em data-scalable} delivery, which entails two specific requirements.
{\em (i)} First, the frame is decodable once {\em any} non-empty subset of its packets are received, and quality improves with more packets received (or equivalently, quality degrades gracefully with more packets missing).
{\em (ii)} Second, unlike the redundancy-based approach, how a frame is encoded should not depend on the prediction of future packet losses.
%{\em (ii)} Second, the decoded quality with {\em any} $x\%$ ($x>0$) received packets is lower but still comparable to classic codec (\eg H.265) with $x\%$ FEC redundancy.
%Note that classic coder $x\%$ with  can be viewed as a reference design that optimizes compression efficiency, not loss resilience.
%\item 
%\end{packeditemize}
Using the form of prior loss-resilience abstractions, data-scalable delivery is:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}|) &\rightarrow \texttt{quality}\nonumber
\nonumber
\vspace{-0.05cm}
\end{align}

Figure~\ref{fig:primitive-table} illustrates the difference between data-scalable delivery and other loss-resilient techniques.
%,  illustrates an example frame whose coded data is delivered in six packets arriving at the receiver at an arbitrary order. 
The most noticeable benefit of data-scalable delivery is that, while the exact arrival time of each packet is unknown to the receiver, data-scalable delivery offers the receiver the {\em flexibility} to decode a frame anytime after receiving any one of the packets. 
Moreover, each new packet strictly improves quality.

It helps to highlight the difference between data-scalable delivery and SVC whose quality also increases with more packets. 
However, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets.
As we will show in \S\ref{sec:eval}, SVC (even with FEC-protection on the base layer as commonly used~\cite{??,??}) does not always improve quality with each new packet, until all packets of a higher layer (and all layers below it) have been received. 
In other words, a missing packet may render multiple quality layers undecodable. 
%For this reason, in practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).




\subsection{Why autoencoder?}
\label{subsec:why-autoencoder}

Our work is built on autoencoders, an emergent class of neural network coders for video frames, including I-frames and P-frames.
The recent autoencoders borrow ideas from traditional codecs (\eg compressing motion vectors and residuals separately, rather than compressing each frame from scratch), but replace handcrafted heuristics with multi-layer neural nets (NNs) which are trained on large sets of videos (\eg Vimeo-90K~\cite{??}). 
Thanks to these trends, their compression efficiency and generalization have been improving over the recent years.

%Recent autoencoders have improved their compression efficiency, thanks to higher-capacity encoder/decoder DNN architectures, which can be trained on large set of videos (\eg Vimeo-90K~\cite{??}). 
%
%%Like traditional codecs, recent video autoencoders compute and compress motion vector estimation and residuals separately, rather than compressing each frame from scratch. 
%These optimizations improve not only compression efficiency but also generalization of these NN-based autoencoders.

\mypara{Autoencoder-based data-scalable coding}
We base our approach on autoencoders, not because of their compression efficiency, but because their performance (albeit suboptimal) potentially fits the definition of data-scalable delivery. 
For example, we consider a pre-trained P-frame autoencoder~\cite{dvc}. 
To emulate the effect of different packet loss rates, we randomly zero \fillme-\fillme\% of values in the autoencoder-returned data (before entropy encoding). 
(We will explain how such random data erasure simulates packet losses in \S\ref{??}.)
Figure~\ref{fig:autoencoder-pretrained} (red curve) shows that as more data is received, the decoded quality gradually improves. 
(To avoid overfitting, we test it on a different video dataset than the training dataset.)
%It is very encouraging that even a pre-trained autoencoder leads to a (suboptimal) data-scalable delivery.


\begin{figure}[t!]
    \centering
%    \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/psnr-loss-vs-pretrained.pdf}
%         \caption{P-frame model}
%         \label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/autoencoder_pretrained_qmap_v1.png}
%         \caption{I-frame model}
%         \label{fig:}
%     \end{subfigure}

         \includegraphics[width=0.6\linewidth]{figs/psnr-loss-vs-pretrained.pdf}

    \caption{Loss resilience of an example pre-trained autoencoder (red). It is already data-scalable (decodable with any subset of packets), but the quality drops much faster than the graceful degradation observed in our solution. \jc{YIHUA, make the figure wider. Swap the order of the legend to "Pre-trained autoencoder" and "Our custom autoencoder"} \jc{also add a horizontal line of H.264/265 without loss}
%    Our models has a more graceful quality degradation under packet losses comparing to pretrained models
    }
    \label{fig:autoencoder-pretrained}
\end{figure}

However, the quality of the pre-trained autoencoder grows quite {\em slowly} when only a few packets are received. 
This is expected, since these autoencoders are not trained to realize data-scalable delivery. 
Our goal in the remaining of the paper is two-fold: (1) creating better data-scalable autoencoders that produce better quality under various packet losses (see the blue line in Figure~\ref{fig:autoencoder-pretrained}), and (2) designing a custom real-time video delivery system that uses autoencoders as a codec, to better balance between frame delay and video quality. 

Despite being emergent and relatively less engineered than traditional codecs, autoencoders are increasingly applied by the signal processing community for image compression~\cite{??,??} and wireless communication~\cite{??,??}, by multimedia community for high-volumetric video compression~\cite{??,??} and recently by the networking community to improve chunk-based video streaming~\cite{swift}.
Unlike this work, however, these efforts still rely on packets retransmission or traditional schemes (like FEC) to handle packet losses. 


\subsection{Caveats of using autoencoders}

Though autoencoders are studied extensively in the computer vision community, there has been surprisingly little attention given to a thorough comparison between autoencoders and traditional codecs (H.265 and H.264), which have been extremely heavily engineered in the multimedia community.
We are aware of that this leads to potentially biased (and sometimes exaggerated) perception of autoencoders's performance. 
%Traditional video codecs have been extremely heavily engineered, but 
For instance, if one tests an autoencoder and H.265 under the same small (4-10) GoP, autoencoders will outperform H.265, because small GoPs align better with how autoencoders are trained but are not what H.265 is designed for. 
On the other hand, a comparison can be unfavorable to autoencoders as well.
For instance, H.26x obtains better motion vector estimation and smaller residuals by using {\em multiple} reference frames, whereas most autoencoders derive motion vectors and residuals only a {\em single} reference frame (which is not a fundamental constraint) and instead focus on better compression of the motion vectors and residuals.
To make it more complicated, autoencoders can optimize either PSNR or SSIM (in RGB or YUV), so research on autoencoders typically evaluate only the metric that the model is trained on.
%whereas traditional codecs are designed with YUV-SSIM in mind\cite{some citation?}.

In this project, we have spent great effort to improvement the performance of autoencoder-based real-time videos (some key optimizations are explained in \S\ref{subsec:optimize}).
We have also tried our best to avoid such pitfalls in our evaluation of autoencoders and their baselines. (For space limitation, we elaborate the details in \S\ref{??}.)
For instance, we evaluate them in various metrics (PSNR and SSIM) and use H.26x's default encoding setting without limiting GoP, and stress-test autoencoders on video sets different from the training set.
We also disable B-frames (0 bframe and rc-lookahead) and use \texttt{fast} preset in H.26x, as in most real-time videos~\cite{??,??}.
\jc{yihua: please find some citation/pointers to justify this choice.}
%train autoencoders on the same dataset (Vimeo-90K~\cite{??}) but report the test result on different datasets.
%Moreover, we allow H.26x can still use multiple history frames as reference, but only one frame as reference in autoencoders. 
%To be clear, we make sure that this is still unfavorable to autoencoders, since H.26x can still use multiple history frames as reference, but autoencoders only use one.
The bottom line is that in our testing, our pre-trained autoencoder~\cite{??,??} (which \name customizes) it is on par with H.265 and better than H.264, and we have also confirmed that in the most aggressive encoding mode (\eg with B-frames and \texttt{fast}), H.265 achieves higher compression efficiency than autoencoders. 

We hope to present a balanced view in this work: even though the autoencoders have lower coding efficiency than the heavily engineered video codecs like H.265, we believe that their potential to reduce tail delay (via data-scalable delivery) outweighs the slightly lowered quality, which is also being constantly improved by better neural-network models.




% \begin{figure}[t!]
%     \centering
%          \centering
%         \includegraphics[width=0.99\linewidth]{figs/primitive_example.pdf}
%     \caption{}
%     \label{fig:primitive_example}
% \end{figure}

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.99\linewidth]{figs/primitive_example_new.pdf}
%    \caption{}
%    \label{fig:primitive_example}
%\end{figure*}




%
%
%\jc{need to elaborate on this! need a "functional" description of the data-scalable primitive}
%

\begin{comment}


To  the limitations of the traditional loss-resilient schemes, we choose a different approach, by borrowing the concept of deep autoencoder and exploring its design choices in the context of \name, the first autoencoder-based real-time video system.
% We first describe the design choices of its autoencoder-based codec.

Before delving into the detailed design, we posit two requirements that should be met by an ideal codec for real-time video systems, which we refer to as {\em data-scalable} codec: 
\begin{packeditemize}
\item The video coding should be \rate-agnostic, and 
\item At any \rate ($<100\%$)\footnote{Importantly, the second requirement does {\em not} include \rate of 100\% (no data received).}, the decoded quality is near that of FEC-based loss protection if FEC knows the \rate. 
\end{packeditemize}
For instance, (see Figure~\ref{fig:intro-example}), \name's codec achieves similar quality as H.265 without FEC-based protection
% An example of such codec is the one we developed as part of \name.
As shown in Figure~\ref{??}, when \rate is zero, the quality is similar to that of H.265 without FEC-based protection, and as fewer packets are received (higher \rate) quality degrade {\em gracefully}, achieving similar quality as H.265 protected by an FEC redundancy rate that matches the \rate. 
\end{comment}


% This section introduces the basic design of our data-scalable video codec, and the next few sections will examine its design choices and how it should be used in an end-to-end real-time video system.






==> sections/old/motivate_v5.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\tightsection{Loss tolerance for real-time video}

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.92\linewidth]{figs/primitive_table_new.pdf}
%    \caption{Abstractions of different loss-resilient schemes. The differences are: 
%    (1) unlike redundancy-based schemes, data-scalable coding does not depend on prediction of packet loss rate; and 
%    (2) unlike retransmission-based or redundancy-based schemes which must retransmit lost packets until some {\em predefined set} or {\em minimum number} of packets are received, data-scalable delivery can decode a frame with any non-empty set of packets, and the quality gradually improves with every new packet.}
%    \label{fig:primitive-table}
%\end{figure*}


% Real-time video, it is crucial that enough data is timely received for each frame, so that the high-quality frames can be rendered at a fixed interval (\eg every 50ms for 20fps). 
% However, as most packet networks have occasional congestion, delay jitter and packet losses, not all packets of a frame may arrive timely.
% Retransmitting missing packets is also inefficient if the round trip time is long.
% Therefore, loss-resilient schemes are required to ensure that a frame can be decoded at a high quality even if a fraction of its packets have not arrived when it is supposed to be decoded, \ie non-zero deadline-missing rate or \rate. 



Many recent studies (\eg~\cite{macmillan2021measuring,jansen2018performance,concerto,moulay2018experimental}) have shown that intermittent congestion, packet jitter, and packet drops widely exist and often cause long tail delay and low frame rate in real-time video applications. 
Consequently, a client may not be able to receive all packets of a frame before the frame is due for decoding (\eg 40ms after the last frame was decoded if the video is 25fps).
Thus, the ability to decode a frame, despite packet losses (including those dropped or those delayed by congestion), is pressingly needed. 

\begin{comment}
Thus, the ability to tolerate packet losses\footnote{In this work, a packet loss can occur even if the packet is not dropped by the network; a packet is lost if it is delayed (due to congestion, path fluctuation, etc) and arrives after the receiver decodes the frame it belongs to.} is pressingly needed to allow a real-time video client to decode and render the next frame when only a subset of its packets are received.
\end{comment}


\tightsubsection{Prior loss-resilience schemes}
\label{subsec:abstractions}


%This section revisits three general approaches to loss resilience taken by prior work.  

%\subsection{Prior Loss-Resilient Schemes}

Loss resilience has long been an important research topic. 
While the details vary greatly among different loss-resilient techniques, it helps to view them through the lens of the high-level abstractions (summarized in Figure~\ref{fig:primitive-table}) that characterize how packets (coded data) are encoded and how {\em decoded video quality of a frame changes with received data (packets)}.
These abstractions also influence the interaction with the remaining parts of a real-time video application, such as congestion control and bitrate adaptation.


\begin{comment}
they have followed some high-level abstractions that characterize how packets (coded data) are encoded and how {\em decoded video quality of a frame changes with received data (packets)}.
%\vspace{-0.05cm}
%\begin{align}
%\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) & \rightarrow \{\texttt{pkts}\}_{sent}\\
%\texttt{\bf Decode}(\{\texttt{pkts}\}_{received}) & \rightarrow \texttt{quality}
%\label{eq:abstraction}
%\vspace{-0.05cm}
%\end{align}
%of certain loss-resilient performance in terms of video quality as a function of received data (packets). 
Viewing them through the lens of abstractions helps us understand their high-level loss-resilience behavior and  with the remaining of a real-time video application, such as congestion control and bitrate adaptation.

\end{comment}

\myparashort{Retransmission-based}clients
%Packet retransmission is a conventional loss-resilient scheme. 
encode a video frame by a traditional codec (\eg H.264) with a target bitrate and must resend lost packets until a {\em pre-defined set} of packets (pre-determined during video coding) is reliably received. 
%This abstraction can be written as:
%\vspace{-0.05cm}
%\begin{align}
%\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
%\texttt{\bf Decode}(\{\texttt{pkts}\}_{received}\supseteq\{\texttt{pkts}\}_{predefined}) &\rightarrow \texttt{quality}\nonumber
%\vspace{-0.05cm}
%\end{align}
There are two typical retransmission-based schemes.

\smallskip
{\em Basic TCP-based delivery} must retransmit every lost packet for a frame to be decodable. 
Once all packets are received, the quality will be equal to the original encoded quality.
%This RTX's abstraction can be viewed as ``a frame is non-decodable until all its packets are received, at which point the quality is as high as the original encoded quality.''
%if a few packets are resent between two clients whose RTT is higher than inter-frame interval. 

\smallskip
{\em Scalable video coding (SVC)} encodes a video at multiple quality layers such that a quality layer can be decoded as long as packets of this layer and all lower layers are received. %\footnote{\jc{a note on why we dont consider the redundancies in svc}}
%if a packet of one layer is lost while all packets of lower layers are received, the lower layers can still be decoded.
%Thus, the abstraction of SVC is that ``quality reaches that of the layer $i$ if all packets belonging $i$ and all lower layers have been received.''
However, one single lost packet of a lower layer prevents all higher layers from being decoded. 

With retransmission, video codecs can focus on coding efficiency (\ie maximal quality under a given target bitrate). But it also suffers high tail delays when re-sending a packet takes longer than the jitter buffer\footnote{Usually around 50 milliseconds in WebRTC} and frame interval, causing a visually perceivable lag or a skipped frame.
Even if the base (lowest) layer is padded with redundancy (\eg FEC, explained shortly)~\cite{wang2000error}, any packet loss can still be retransmitted to reach higher quality layers. 
%since a pre-determined set of packets will be always reliably delivered

%However, without any redundancy-based protection, a frame is not decodable unless a pre-defined set of packets (all packets or those of some layers) are received in its entirety. 
%%any lost packets might block the decoding of a frame, making retransmission inevitable in many cases. 
%Thus, retransmission is often inevitable, and retransmission can be very slow in long-RTT networks, especially when the extra delay to request a lost packet is longer than the jitter buffer (\fillme), which result in a visually perceivable lag or skipped frame.
%Therefore, retransmission is also complemented by some redundancy-based loss-resilient techniques, so only fewer lost packets need to be resent. 





\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.999\linewidth]{figs/primitive_table_new_v4.pdf}
    \tightcaption{
Summary of loss-resilient schemes. 
    Retransmission-based schemes (TCP, SVC) obtain high quality (the red horizontal line) only if a predefined {\em set} of packets are received.
    Redundancy-based ones (FEC, intra-MB) tolerate a pre-defined maximum number of packet losses by adding redundancy (thus lowering quality when all packets are received).
    In contrast, data-scalable delivery decodes a frame from any non-empty set of packets, improves quality with {\em each} new packet, and has high quality when all packets arrive. 
%    The differences are: 
%    (1) unlike redundancy-based schemes, data-scalable delivery does not need to add more redundancy to tolerate more predicted packet losses, and
%    (2) unlike retransmission-based schemes which must receive a predefined minimum {\em set} of packets, data-scalable delivery can decode a frame with any non-empty set of packets.
%    Comparing different abstractions of loss-resilient schemes. The differences are: 
%    (1) unlike redundancy-based schemes, data-scalable coding does not depend on prediction of packet loss rate; and 
%    (2) unlike retransmission-based schemes which must receive a predefined minimum {\em set} of packets, data-scalable delivery can decode a frame with any non-empty set of packets, and the quality gradually improves with every new packet.
%    (3) unlike redundancy-based ones which must receive a minimum number of packets, data-scalable delivery can decode a frame with 
    }
    \label{fig:primitive-table}
\end{figure}




\myparashort{Redundancy-based}schemes are used in complement to retransmission-based techniques. 
%are often also complemented with some redundancy-based loss-resilient techniques, so only fewer lost packets need to be resent. 
With this technique, a frame is decodable when at least $N\%$ packets are received. However, the decoded quality is lower with a smaller $N$.
Here, $(1-N\%)$ represents the redundancy rate.
Redundancy-based schemes essentially trade coding efficiency for loss resilience. 
%The abstraction is:
%\vspace{-0.05cm}
%\begin{align}
%\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}, N\%) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
%\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}| \geq N\%,N) &\rightarrow \texttt{quality}\nonumber
%\nonumber
%\vspace{-0.05cm}
%\end{align}
Redundancy-based schemes have been studied intensively.
% in the IEEE multimedia community.
%Two typical redundancy-based schemes are FEC and intra-MB insertion.


%This equation entails the efficiency-resilience tradeoff: higher redundancy \texttt{redun} leads to lower $\alpha_{\texttt{redun}}$ (\ie higher loss resilience), but it also means lower resulting quality if $|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}}$ (\ie lower coding efficiency).

%The abstraction of redundancy-based loss resilience is characterized by:
%\vspace{-0.05cm}
%\begin{align}
%\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}, \texttt{redun}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
%\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}},\texttt{redun}) &\rightarrow \texttt{quality}\nonumber
%\nonumber
%\vspace{-0.05cm}
%\end{align}
%This equation entails the efficiency-resilience tradeoff: higher redundancy \texttt{redun} leads to lower $\alpha_{\texttt{redun}}$ (\ie higher loss resilience), but it also means lower resulting quality if $|\{\texttt{pkts}\}_{received}| \geq \alpha_{\texttt{redun}}$ (\ie lower coding efficiency).
%Here, we discuss two concrete redundancy-based schemes.

\smallskip
{\em Forward error correction (FEC)} and Reed-Soloman and Fountain Codes~\cite{mackay2005fountain} are often used in real-time applications.\footnote{FEC is not in the standard of WebRTC. Our evaluation uses the FEC logic implemented in Google's open-source repository~\cite{WEBRTCSRC}.
% \jc{a footnote on the suboptimal use of fec in webrtc}
} %(see \cite{??,??} for an in-depth discussion).
Ideally, these FEC schemes take an encoded video/frame and code it with redundancy bits, and the receiver can recover the data if {\em any} packets contain the same amount of bytes as the original data 
% This is aligned with existing applications, \fillme
that was received. 
%, with \fillme and \fillme achieving near-ideal performance of FEC and fountain codes. 
%Therefore, FEC's abstraction can be described as ``the quality of a frame is low (undecodable) until {\em any} $M$ packets are received.''

FEC is known to have the ``cliff effect''. 
%(a frame or chunk encoded by a video coder like H.265), 
No matter how much redundancy is added, the decoder has to receive at least as many bytes as in the encoded video file, \ie retransmission cannot be avoided if the encoding video bitrate already exceeds the network capacity.
Moreover, the decoded video quality is pre-decided by the video encoder and remains the same even if more data arrives.
Thus, with too little redundancy, the receiver must wait for more packets to arrive or be retransmitted; with too much redundancy, the video quality will be low.
Thus, {\em they are most effective, {\em if} the sender knows how many bytes can be timely delivered in advance}.

%Thus, the video encoder should ideally encode each video frame at exact the bitrate that matches the amount of data received when the frame is decoded. 

%These issues affect Reed-Soloman and fountain codes: that they cannot decode a frame only when a minimum number of packets are received, and the quality will not increase with more arrived packets. 




\begin{figure}[t!]
    \centering
      \begin{subfigure}[b]{0.6\linewidth}
         \centering
         \includegraphics[width=1.1\linewidth]{figs/webrtc-rate.pdf}
         \caption{Bandwidth and bitrate}
         \label{fig:}
     \end{subfigure}
     \begin{subfigure}[b]{0.6\linewidth}
         \centering
         \includegraphics[width=1.1\linewidth]{figs/webrtc-delay.pdf}
         \caption{Frame delay}
         \label{fig:}
     \end{subfigure}
    \tightcaption{An WebRTC run with a sudden bandwidth drop}
    \label{fig:motivate-example}
    % \vspace{-0.5cm}
\end{figure}


Unfortunately, it is not always possible to predict the number of missing packets before the receiver decodes a frame. 
Figure~\ref{fig:motivate-example} gives an example showing why setting the FEC redundancy rate is difficult. 
We run WebRTC against a simple bandwidth trace over a network link of RTT 300ms and a drop-tail queue of 1024 packets.\footnote{By default, bandwidth probing and FEC are enabled by WebRTC to allow fast sending adaptation, and the FEC redundancy rate is dynamically determined by the packet loss in the last a few seconds. \cite{holmer2013handling} offer a comprehensive description of WebRTC's congestion control and FEC logic.
}
%Figure~\ref{??} shows that the frame delays (the time between sending a frame and enough bytes received to decode it) is littered with sporadic periods of sudden spikes.
When bandwidth suddenly drops, the sending rate and the FEC redundancy rate adjust only after any sign of congestion is returned to the sender (after at least one RTT), causing many packets to be dropped and delaying subsequent frames. 
The long delays could have been mitigated, if FEC adapts more conservatively (\eg increase redundancy faster but decrease it more slowly). But this will cause lower video quality as more bytes are used for redundancy when bandwidth is stable.
Techniques like dynamic reference selection~\cite{salsify} may mitigate this issue, but could not have avoided the congestion and delay of the first few frames. %as elaborated in \S\ref{??}.
This corroborates the findings in the literature (\eg~\cite{google-doc-fec})



Source-coding-based schemes (\eg intra-MB insertion) do not explicitly add redundancy like FEC. 
% has also proposed techniques to make video coding (\eg H.264) resilient to packet losses by keep more existing pixel-level redundancy during the video coding process (as opposed to FEC which adds redundancy on top of an encoded frame).
Instead, it reduces the inter-dependencies between macroblocks (MBs) that are potentially similar to each other. 
For instance, intra-MB insertion adaptively sets more MBs in \texttt{INTRA} mode, making these MBs and others that refer to them decodable, even if other data is lost.\footnote{Packet losses can also be tolerated by choosing a better reference frame to allow the receiver to skip undecodable frames without affecting subsequent frames, such as in Salsify~\cite{salsify}. These techniques can be used jointly with \name to select better quality reference frames.}
%For instance, \jc{Yihua, explain R/D optimization, intra-MB insertion, dynamic reference selection, etc}
%\jc{need a footnote here to describe how entropy encoding can be stopped at the boundary between packets. }
Both intra-MB insertion and FEC must lower coding efficiency: FEC adds redundancy data and intra-MB insertion keeps more inter-macroblock redundancy.
%Figure~\ref{fig:motivate-regime} illustrates when existing schemes are effective.

In short, retransmission-based schemes are sufficient if the RTT between the clients is low enough to conceal the retransmission delay. 
%compared to the desirable frame delay, packet retransmission would be sufficient to conceal any packet losses.
Redundancy-based schemes are suitable for connections with largely predictable packet loss rates.
% of the next frame is largely predictable, FEC-based schemes will be sufficient. 
However, both of them fall short under high RTT and highly dynamic packet jitters and losses.



%\jc{need a footnote to discuss frame skipping and reference frame selection!!!}





% \jc{mention the findings corroborate with \cite{\url{https://docs.google.com/document/d/1Hg1SaLEl6T4rEU9j-isovCo8VEjjnuCPTcLNJewj7Nk/edit}}}

% \jc{also mention that fec is not native in webrtc. this is google implementation}

%Like FEC, with more pixel-level redundancy preserved, data erasures have less impact, but compression efficiency is lowered at the same time. 
%In practice, with all packets, the decoded quality of intra-MB insertion is lower than that of the coding algorithm that is optimized for coding efficiency (\ie no redundancy), and while a small fraction of data losses can be efficiently tolerated, a high loss rate (more than 40\% data erasure) will still render a frame undecodable~\cite{??,??}. 


\begin{comment}

\mypara{Limitations}
Retransmission-based schemes become less effective than redundancy-based schemes under longer propagation delays between clients. 
However, compared to traditional coders (\eg H.265) that are optimized for video coding efficiency (fewer bits for higher quality), the redundancy-based abstractions are less efficient in that they use more bits to obtain the same quality in the absence of any packet loss.
%That is, they must trade compression efficiency for loss resilience, so the rate of redundancy is highly sensitive to \rate prediction. 
Thus, these abstractions of loss resilience are effective only if they can predict future packet loss rates and jitter, which is not always possible in practice. 

Figure~\ref{fig:motivate-example} gives an example of why setting the FEC redundancy rate is difficult. 
We run WebRTC against a simple bandwidth trace over a network link of RTT \fillme and a drop-tail queue of \fillme.\footnote{We enable the \fillme option\jc{bw probing and fec} to allow fast sending adaptation, and the FEC redundancy rate is dynamically determined by the default history-based logic. \cite{??, ??} offer a comprehensive description of WebRTC's congestion control and FEC logic.}
%Figure~\ref{??} shows that the frame delays (the time between sending a frame and enough bytes received to decode it) is littered with sporadic periods of sudden spikes.
When bandwidth suddenly drops, the sending rate and the FEC redundancy rate can adjust only after any sign of congestion is returned to the sender (after at least one RTT), causing many packets to arrive late and delaying the rendering of several subsequent frames. 
The long delays could have been mitigated, if FEC adapts more conservatively (\eg increase redundancy faster but decrease it more slowly). 
But this is at the cost of much lower video quality, as more bytes are used for redundancy when bandwidth is stable.
Techniques like dynamic reference selection~\cite{salsify} may mitigate this issue, but could not have avoided the congestion and delay of the first few frames as elaborated in \S\ref{??}.




\begin{figure}[t!]
    \centering
         \centering
        %  \includegraphics[width=0.85\linewidth]{figs/intro-example-placeholder.pdf}
        \includegraphics[width=0.6\linewidth]{figs/motivate_regime.pdf}
    \caption{Traditional abstractions (retransmission-based and redundancy-based) for loss resilience are suitable for connections with low latency or predictable packet loss rates, respectively. However, they are less effective if latency is long and packet loss rate is highly dynamic.}
    \label{fig:motivate-regime}
\end{figure}

\end{comment}



\tightsubsection{A new abstraction: Data-scalable delivery}

%To overcome the limitations of prior loss-resilient schemes, 
This work envisions a new abstraction of loss resilience, {\em data-scalable} delivery, and presents a concrete implementation (\S\ref{sec:training}).
Data-scalable delivery should meet two criteria.
{\em (i)} First, the frame is decodable once {\em any} non-empty subset of its packets are received, and quality improves with more packets received (or equivalently, the quality degrades gracefully with more packets missing).
{\em (ii)} Second, unlike the redundancy-based approach, how a frame is encoded should not depend on the prediction of future packet losses.
%{\em (ii)} Second, the decoded quality with {\em any} $x\%$ ($x>0$) received packets is lower but still comparable to classic codec (\eg H.265) with $x\%$ FEC redundancy.
%Note that classic coder $x\%$ with  can be viewed as a reference design that optimizes compression efficiency, not loss resilience.
%\item 
%\end{packeditemize}
At a high level, this new abstraction can be expressed as follows:
\vspace{-0.05cm}
\begin{align}
\texttt{\bf Encode}(\texttt{frame}, \texttt{bitrate}_{target}) &\rightarrow \{\texttt{pkts}\}_{sent}\nonumber\\
\texttt{\bf Decode}(|\{\texttt{pkts}\}_{received}|) &\rightarrow \texttt{quality}\nonumber
\nonumber
\vspace{-0.05cm}
\end{align}

\myparaq{What's new}
Figure~\ref{fig:primitive-table} contrasts data-scalable delivery with other loss-resilient techniques.
\begin{packeditemize}
\item
Unlike FEC (RS or Fountain Code), data-scalable delivery allows the receiver to decode after receiving any packet and obtain higher quality with each new packet received.

\item
While SVC might increase quality with more received packets, it is not data-scalable, because it imposes a hierarchical structure of packets. 
One missing packet may render multiple quality layers undecodable (even if the base layer is protected by FEC~\cite{SVCFEC1, schierl2007using}).
%Each new packet does not always improve quality, until all packets of a layer and the lowers layers have been received. 
%As we will show in \S\ref{sec:eval}, SVC (even with FEC-protection on the base layer as commonly used~\cite{??,??}) does not always improve quality with each new packet, until all packets of a higher layer (and all layers below it) have been received. 
%In other words, a missing packet may render multiple quality layers undecodable. 

\end{packeditemize}

We should stress that any loss resilience comes at the expense of coding efficiency, and {\em data-scalable delivery is no exception}.
We expect that the quality in absence of any packet losses will be slightly lower than traditional codecs.

%,  illustrates an example frame whose coded data is delivered in six packets arriving at the receiver at an arbitrary order. 

%It helps to highlight the difference between data-scalable delivery and SVC whose quality also increases with more packets. 
%However, SVC is not exactly data-scalable, because it imposes a strict hierarchy among packets.
%As we will show in \S\ref{sec:eval}, SVC (even with FEC-protection on the base layer as commonly used~\cite{??,??}) does not always improve quality with each new packet, until all packets of a higher layer (and all layers below it) have been received. 
%In other words, a missing packet may render multiple quality layers undecodable. 

%For this reason, in practice, SVC often employs extra loss-protection like FEC but only to protect its base layer (known as unequal error protection).




%The most noticeable benefit of data-scalable delivery is that, 
%Therefore, while the exact arrival time of each packet is unknown to the receiver, 
%Data-scalable delivery offers the receiver the {\em flexibility} to decode a frame anytime after receiving at least one packet of the frame, and the quality always improves with each new packet.


%We should clarify that this work does {\em not} invent a new loss tolerant paradigm. 


\tightsubsection{Why autoencoder?}
\label{subsec:why-autoencoder}

Our approach to data-scalable delivery is based on autoencoders, an emergent class of neural-network coders for video (I-frames and P-frames).
The recent autoencoders borrow ideas from traditional codecs (\eg compressing motion vectors and residuals separately, rather than compressing each frame from scratch), and replace handcrafted heuristics with multi-layer neural nets (NNs) which are trained on large sets of videos (\eg Vimeo-90K~\cite{vimeo-dataset}). 
Recent autoencoders' performance has significantly improved~\cite{dvc, elf}. 
%Thanks to these trends, their compression efficiency and generalization have been improving over the recent years.

%Recent autoencoders have improved their compression efficiency, thanks to higher-capacity encoder/decoder DNN architectures, which can be trained on large set of videos (\eg Vimeo-90K~\cite{??}). 
%
%%Like traditional codecs, recent video autoencoders compute and compress motion vector estimation and residuals separately, rather than compressing each frame from scratch. 
%These optimizations improve not only compression efficiency but also generalization of these NN-based autoencoders.

%\mypara{Autoencoder-based data-scalable coding}
We choose to use autoencoders not because of their coding efficiency (which comes with caveats discussed shortly), but because their quality under data erasure (albeit suboptimal) {\em might} fit the definition of data-scalable delivery. 
Figure~\ref{fig:autoencoder-pretrained} shows an example: we use a pre-trained P-frame autoencoder~\cite{dvc} to encode frames from a video (not from the training set) and test its decoded quality with an increasing rate of random data erasure (we will explain how this simulates packet losses in \S\ref{subsec:sim-losses}). 
%To emulate the effect of different packet loss rates, we randomly zero \fillme-\fillme\% of values in the autoencoder-returned data (before entropy encoding). 
The red curve shows that as more data is received, the decoded quality gradually improves. 
%(To avoid overfitting, we test it on a different video dataset than the training dataset.)
%It is very encouraging that even a pre-trained autoencoder leads to a (suboptimal) data-scalable delivery.


\begin{figure}[t!]
    \centering
%    \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/psnr-loss-vs-pretrained.pdf}
%         \caption{P-frame model}
%         \label{fig:}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figs/autoencoder_pretrained_qmap_v1.png}
%         \caption{I-frame model}
%         \label{fig:}
%     \end{subfigure}

         \includegraphics[width=0.5\linewidth]{figs/psnr-loss-vs-pretrained.pdf}

    \tightcaption{Loss resilience of an example pre-trained autoencoder (red). It is already data-scalable (decodable with any subset of packets), but the quality drops much faster than the graceful degradation observed in our solution. 
    % \jc{YIHUA, make the figure wider. Swap the order of the legend to "Pre-trained autoencoder" and "Our custom autoencoder"} \jc{also add a horizontal line of H.264/265 without loss}
%    Our models has a more graceful quality degradation under packet losses comparing to pretrained models
    }
    \label{fig:autoencoder-pretrained}
\end{figure}

However, as the figure shows, the pre-trained autoencoder degrades quite sharply with more data erasure. 
(After all, these autoencoders are not trained to perform well under random data erasure.) 
In \S\ref{sec:training}, we will show how to train data-scalable autoencoders that produce better quality under various packet losses (\eg the blue line in Figure~\ref{fig:autoencoder-pretrained}).
%Our goal in the remaining of the paper is two-fold: (1) creating better data-scalable autoencoders that produce better quality under various packet losses (see the blue line in Figure~\ref{fig:autoencoder-pretrained}), and (2) designing a custom real-time video delivery system that uses autoencoders as a codec, to better balance between frame delay and video quality. 




\tightsubsection{Caveats of using autoencoders}

Despite being emergent and not as heavily optimized as traditional codecs, autoencoders have gained increasing attention in the signal processing community for image compression~\cite{bourtsoulatze2019deep,gunduz2019machine} and wireless communication~\cite{erpek2020deep,dai2020deep}, by the multimedia community for high-volumetric video compression~\cite{le2022mobilecodec,li20213d}, and recently by the networking community for chunk-based video streaming~\cite{swift}, though these efforts still rely on traditional schemes (like FEC) to handle packet losses. 

Though autoencoders are studied extensively, there has been much less attention given to a thorough comparison between autoencoders and traditional codecs (H.265 and H.264, which have been extremely optimized in speed and efficiency).
This could lead to potentially biased (and sometimes exaggerated) perceptions of autoencoders' performance. 
%Traditional video codecs have been extremely heavily engineered, but 
For instance, if one tests an autoencoder and H.265 under the same small (4-10) GoP, autoencoders will outperform H.265 because small GoPs align better with how autoencoders are trained but not with H.265.
These comparisons could also be unfair to autoencoders as well.
For instance, H.26x searches optimal reference MBs from {\em multiple} frames to reduce residuals, whereas most autoencoders derive motion vectors and residuals from a {\em single} reference frame (which is not a fundamental constraint) and instead, they focus on compression of given motion vectors and residuals.
Moreover, autoencoders can be trained to optimize either PSNR or SSIM, so papers evaluate only the metric that the model is trained for.
%whereas traditional codecs are designed with YUV-SSIM in mind\cite{some citation?}.

This work reports our efforts to make autoencoders loss resilient (\S\ref{sec:training},\ref{sec:delivery}) as well as practical (in speed and memory usage) for real-time videos (\S\ref{subsec:optimize}).
In our evaluation of autoencoders, we have tried our best to avoid pitfalls (\eg those listed in~\cite{codec-eval-pitfalls}). (For space limitation, we elaborate the details in \S\ref{subsec:eval:setup}.)
For instance, we report both PSNR and SSIM and use H.26x's default encoding setting without limiting GoP, and stress-test autoencoders on video sets different from the training set.
We also use a common setting of real-time video~\cite{ZEROLAT1,ZEROLAT2} with the \texttt{fast} preset in H.265 and no B-frames or rc-lookahead.
%disable B-frames (0 bframe and rc-lookahead) and use \texttt{fast} preset in H.265.
% \jc{yihua: please find some citation/pointers to justify this choice.}
%train autoencoders on the same dataset (Vimeo-90K~\cite{??}) but report the test result on different datasets.
%Moreover, we allow H.26x can still use multiple history frames as reference, but only one frame as reference in autoencoders. 
%To be clear, we make sure that this is still unfavorable to autoencoders, since H.26x can still use multiple history frames as reference, but autoencoders only use one.
%The bottom line is that in our testing, our pre-trained autoencoder~\cite{??,??} (which \name customizes) it is on par with H.265 and better than H.264, and we have also confirmed that in the most aggressive encoding mode (\eg with B-frames and \texttt{fast}), H.265 achieves higher compression efficiency than autoencoders. 

We hope to present a balanced view in this work: even though the autoencoders have lower coding efficiency than the heavily engineered video codecs like H.265, we believe that their potential to reduce tail delay (via data-scalable delivery) outweighs the slightly lowered quality, which is also being constantly improved by better neural-network models.




% \begin{figure}[t!]
%     \centering
%          \centering
%         \includegraphics[width=0.99\linewidth]{figs/primitive_example.pdf}
%     \caption{}
%     \label{fig:primitive_example}
% \end{figure}

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.99\linewidth]{figs/primitive_example_new.pdf}
%    \caption{}
%    \label{fig:primitive_example}
%\end{figure*}




%
%
%\jc{need to elaborate on this! need a "functional" description of the data-scalable primitive}
%

\begin{comment}


To  the limitations of the traditional loss-resilient schemes, we choose a different approach, by borrowing the concept of deep autoencoder and exploring its design choices in the context of \name, the first autoencoder-based real-time video system.
% We first describe the design choices of its autoencoder-based codec.

Before delving into the detailed design, we posit two requirements that should be met by an ideal codec for real-time video systems, which we refer to as {\em data-scalable} codec: 
\begin{packeditemize}
\item The video coding should be \rate-agnostic, and 
\item At any \rate ($<100\%$)\footnote{Importantly, the second requirement does {\em not} include \rate of 100\% (no data received).}, the decoded quality is near that of FEC-based loss protection if FEC knows the \rate. 
\end{packeditemize}
For instance, (see Figure~\ref{fig:intro-example}), \name's codec achieves similar quality as H.265 without FEC-based protection
% An example of such codec is the one we developed as part of \name.
As shown in Figure~\ref{??}, when \rate is zero, the quality is similar to that of H.265 without FEC-based protection, and as fewer packets are received (higher \rate) quality degrade {\em gracefully}, achieving similar quality as H.265 protected by an FEC redundancy rate that matches the \rate. 
\end{comment}


% This section introduces the basic design of our data-scalable video codec, and the next few sections will examine its design choices and how it should be used in an end-to-end real-time video system.






==> sections/old/motivate_v6.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\tightsection{Motivation}


Video coding has a rich history of research, and it would be hard to fit a comprehensive overview of video coding in limited space.
However, for people new to this topic, it will help to introduce the key concepts pertinent to this paper (\S\ref{??}) before explaining why better solution is needed (\S\ref{??}). 

\tightsubsection{Background of video coding}

When encoding a video stream, the sender uses rate adaptation logic to dynamically set the frame rate and bitrate used to encode video frames.
%A video stream is encoded at certain frame rate and bitrate, both are controlled by an adaptation logic in the player.
For a frame rate of 25~fps (frames per second) and bitrate of 3Mbps, for instance, the encoder should on average generate a 150KB frame every 40ms, though actual size of a frame depends on the {\em frame type}.
%Different {\em frame types} often have different frame sizes.
An I-frame (intra-frames), encoded independently, is followed by P-frames (predicted frames), each encoding only the differences with previous I-/P-frames, and B-frames (bidirectional predicted frames), each encoding the difference with the previous and future I-/P-frames.
Thus, I-frames are typically bigger than P-frames and B-frames, but decoding I-frames does not depend on any other frame, while decoding P-frames or B-frames must refer to other frames. 
%fewer other frames than decoding a B-frame.
A frame used as a reference for decoding other frames is called a {\em reference frame}.


\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/fig2-workflow-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{}
    \label{fig:codec-workflow}
\end{figure}

To encode each frame, the encoder first calculates the differences (\eg motion vectors and residuals) among macroblocks ($4\times4,8\times8,\dots$) in the current frame and reference frames (or within an I-frame),  then transform and quantize these differences to a more compact form, and finally losslessly code the data using arithmetic coding. 
The compressed data of each frame is then packetized and sent through the network by the transport layer, which controls how fast the packets need to be sent 
%algorithm decides how fast to send a frame's packets, 
in order to ensure enough data be delivered to the receiver by the time the frame is decoded. 

The receiver runs a reverse process (depacketization and decoding) to reconstruct each frame when all or some of its packets arrive. 
Once a frame is decoded, it might not be rendered immediately; instead, it will be put in a {\em (jitter) buffer} first, so that latency jitter, due to queuing or retransmits, will not directly affect video smoothness.

\jc{clarify real-time video, conversational video, low-latency video}




\tightsubsection{Goal: data-scalable coding}

Since packet loss might happen anytime, loss resilience of video coding is critical to maintain smoothness and high quality. 
This is particularly important in real-time videos, because they use a much shorter jitter buffer (just 1-2 frames or 10s of milliseconds) than even live broadcast videos, which have a buffer of at least a few seconds.
While increasing interactivity between clients, the short buffer makes the receiver potentially vulnerable to {\em any packet queuing or retransmit} that blocks the decoding of a frame after the short buffer is depleted. 

As both lost packets and delayed packets affect decoding, for simplicity, we use {\em data-missing rate} (or {\em \rate} for short) to denote the fraction data (packets) of a frame that arrive after when the frame is decoded.
Previous measurements have shown that if frames are decoded with a fixed intervals (\eg every 40ms for a 25~fps video), \rate can vary between \fillme, and is hard to predict in advance~\cite{??,??,??}. 
For instance, a bandwidth drop from 3Mbps to 500Kbps on a 200ms-RTT link can suddenly raise \rate to 75\% and retransmission will delay or skip at least 6 frames in a 25fps video stream. 

A desirable video coding system, therefore, should encode video frames such that the quality gracefully degrade in presence of packet loss, without compromising quality in absence of packet loss. 
Concretely, it should meet three requirements:
\begin{packeditemize}
\item {\em \RDecodable (Minimum retransmission and frame skipping):} The receiver can decode a frame if {\em any} non-empty subset of the packets of this frame is received.
%(\ie no retransmission or frame skipping unless no packet is received);
\item {\em \RGraceful (Graceful degradation):} quality gradually improves with each received packet; in order words, the decoded quality gradually degrades with each missing packet; and
\item {\em \REfficient (High compression efficiency):} The decoded quality reaches a quality close to that of a non-loss-resilient coding algorithm (such as H.265), if all packets are received.
%similar quality as the quality without redundancy (such as H.265), if all packets are received.
\end{packeditemize}
We refer to this as {\em data-scalable} (or {\em DS} for short) video coding and delivery.


\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/fig2-dmr-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{}
    \label{fig:codec-dmr}
\end{figure}


DS video coding may sound similar to the classic rate-distortion (RD) tradeoff, which was intensively studied around early 2000s~\cite{??,??}. 
Similar to DS, RD represents the optimal video quality (minimum distortion) under different receiving bitrate, and ideally, with a single encoded bitstream, the decoding quality of the received data naturally increase if more data of the bitstream is received.
However, there is a key difference: DS does not assume the data is received in any specific order, but RD assumes that data of lower coding layer is received before higher layers. 
With this assumption, RD-optimized coding can still greatly improve multicast service (\eg in multi-party video conferencing) and on-demand videos where different layers can be received one by one. 
Our paper aims at unicast real-time video communication with non-trivial network latency, so to reduce each frame's delay, most senders send packets of a frame as one batch.


\myparaq{What's new in real-time video}
While this general workflow applies to most video streaming systems, real-time videos are distinctive in that they seek to reduce the {\em frame delay} between sending a frame and decoding it.
This profoundly affects their design choices in three ways.
%have three features distinct from others, which profoundly affect their designs. 
%short jitter buffer, no b frame, packets sent toghether, all of which have profound impact
\begin{packeditemize}
\item {\em Short jitter buffer:} First, real-time videos use a much shorter jitter buffer (just 1-2 frames or 10s of milliseconds) than even live broadcast videos, which have a buffer of at least a few seconds.
While increasing interactivity between clients, the short buffer makes the receiver potentially vulnerable to {\em any packet queuing or retransmit} that blocks the decoding of a frame after the short buffer is depleted. 


\item {\em Each frame sent in one batch:} Second, to reduce frame delay in long-latency networks, the sender often sends all packets of a frame in one burst, rather than multiple congestion windows.
%Thus loss and delaying can happen to any packets within the burst. 
This diminishes the benefit of layered coding (introduced shortly) which encodes a video in multiple layers and must deliver the layers in a specific order (see \S\ref{??}).


\item {\em Avoid B-frames:} Third, as each frame should be decoded as soon as its packets are received, B-frames are rarely used in real-time videos~\cite{??}, since they require future frames to be received. 
This precludes several loss-resilient techniques such as B-frame skipping (see \S\ref{??}).
\end{packeditemize}



\begin{itemize}
\item 2.1 Background
\begin{itemize}
\item basics: video, encoder, decoder, packets
\item real-time video: small jitter buffer, all packets must be sent together
\item concept of loss-resilient coding
\end{itemize}

\item 2.2 Ideal coding for real-time video
\begin{itemize}
\item given that 
\end{itemize}

\item 2.3 Limitations
\begin{itemize}
\item type 1: scalable coding
\item type 2: fec (rateless versions), reference selection, recover
\end{itemize}
\end{itemize}

We begin with why loss-resilient video coding is particularly important to real-time video and what an ideal scheme should achieve. 
We then explain the limitations of existing approaches.

Despite more bandwidth, many recent studies have shown that real-time video communication is plagued with intermittent packet loss and jitter~\cite{macmillan2021measuring,jansen2018performance,concerto,moulay2018experimental,latency-report-iab,latency-report-iab-2,latency-report-apnic}.
%induced by congestion, wireless, bufferbloat, etc.
\jc{yihua, can we find a few good pointers for this?}
%Adapting bitrate (ABR), which {\em reacts} to fluctuations of network conditions, is not enough to completely prevent packet loss, without using an extremely conservative bitrate. 
Since real-time video clients have very shallow jitter buffers, there is little time for packet retransmission before each frame should be decoded. 
So unlike in traditional streaming videos (which has a buffer of at least several seconds),
%Having shallow jitter buffers means that adapting bitrate or sending rate alone is not enough for clients to be immune to packet loss. 
%This leaves little time for packet retransmission, so 
{\em any} dropped or queued packets could delay the decoding of a frame, causing video stuttering and frame skipping in real-time video applications. 

%Having shallow jitter buffers also means that adapting bitrate or sending rate alone is not adequate to make real-time video client immune to packet loss.
%
%
%It is hard to predict how many packets will be dropped 
%Thus, the ability to decode a frame with a decent quality in presence of packet loss is crucial.




%\jc{Relationship with bitrate adaptation}

\tightsubsection{Problems of current loss-resilient coding}

Loss resilience has long been an important research topic. 
Given the sheer amount of prior work in this space, we only highlight those that are most representative or closest to the goal of DS coding. % (see~\cite{??} for a complete survey).
For ease of comparison, Figure~\ref{fig:primitive-table}  shows how video quality varies with received data (packets) in different loss-resilient techniques. 

%these abstractions also influence the interaction with the remaining parts of a real-time video application, such as congestion control and bitrate adaptation.




\myparaq{Why not retransmission-based recovery}
%Packet retransmission is a conventional loss-resilient scheme. 
Frames are coded by a highly efficient codec (\eg H.265), and once all packets are received, the quality will be equal to the original encoded quality.
However, since these codecs optimize for compression, not loss resilience, any lost packets must be resent until all packets are reliably received, which violates {\em \RDecodable}.
If re-sending a packet takes longer than the jitter buffer, this can also cause a visually perceivable lag or a skipped frame.




\myparaq{Why not bitrate adaptation}
Bitrate adaptation lowers the target bitrate of {\em future} video chunks/frames {\em after} a bandwidth drop is detected. %, and then the video encoder will code the future video chunk or frame at the lowered target bitrate. 
Thus, bitrate adaptation is fundamentally {\em reactive}: 
when bandwidth suddenly drops, some frames have already experienced packet delays or drops before the sender/receiver can lower its target bitrate.
Given the short jitter buffer, this can directly hurt user experience, as in Figure~\ref{fig:trace}(a).
Without a proper loss-resilient scheme, it violates all three requirements of DS coding.

\myparaq{Why not scalable video coding (SVC)}
SVC encodes a video at multiple quality layers such that a layer can be decoded as long as the packets of this layer and all lower layers are received.
However, because SVC imposes a hierarchical order that one missing packet can render all higher quality layers undecodable, it violates requirement {\em \RGraceful}~\cite{chen2006frame}.
%\footnote{The classic SVC violates both requirement {\em (ii)} and {\em (iii)} of DS coding, though {\em (iii)} is mitigated by an autoencoder-based codec~\cite{swift} proposed recently.}
Even if the base (lowest) layer is padded with redundancy (\eg FEC, explained shortly)~\cite{SVCFEC1, schierl2007using,wang2000error}, it does not protect other layers from packet losses.

Other than SVC, there have been several other proposals that aim for finer-grained scalability.
Notably, fine-grained scalability (FSG)~\cite{li2001overview} and more recently DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift} strive to realize the following effect: if the packets are received in order, each new packet will incrementally improve quality, and when all packets are received, the quality is similar to H.265. 
Though they are better than classic SVC, they still impose a hierarchical structure over packets, which violates requirement {\em \RGraceful}---if a low-quality-layer packet of is missing, higher-quality-layer packets are not useful.\footnote{It should be clarified that SVC does achieve coding scalability with on-demand videos, which has enough buffer to allow packet retransmission.
%, where the sender usually makes sure one layer is fully received before sending the next one.
}

%one single lost packet of a lower layer will make all higher layers undecoded. 
%This violates requirement {\em (ii)} of DS coding.
%While the base (lowest-quality) layer of SVC is often padded with redundancy (\eg FEC, explained shortly)~\cite{wang2000error}, it does not protect other layers from packet losses.
%






\myparaq{Why not redundancy-based coding (FEC, RS, fountain codes)} \jc{include streaming code}
%These redundancy-based schemes essentially trade coding efficiency for loss resilience. 
Given a target bitrate $R$, redundancy-based schemes encode a frame at bitrate $N\%\cdot R$, with the remaining $(1-N\%)\cdot R$ used for redundancy code. $(1-N\%)$ is the {\em redundancy rate}.
Then the frame is decodable, once at least {\em any} $N\%$ of packets are received.
A key distinction with SVC is that the quality of SVC depends on {\em which data} is received, whereas the quality of FEC depends on {\em how much} data is received, which is more flexible.
However, they must know \rate in advance to avoid packet retransmission and too much redundancy.
Otherwise, if insufficient redundancy is used (\ie more packets are lost than expected), some packets still must be retransmitted in order to decode the frame (which violates {\em \RDecodable}).
Once the received packets are decodable, more packets will not improve the quality of FEC (which violates {\em \RGraceful}).
And if much redundancy is added while all packets are received (\ie loss rate is overestimated), the decoded quality will be much lower than it could have been without redundancy (which violates {\em \REfficient}).



\myparaq{Why not loss-resilient source coding (\eg intra-MB insertion)}
%Source-coding-based schemes do not explicitly add redundancy like FEC. 
Instead of adding redundancy like FEC, they reduce the inter-dependencies between macroblocks (MBs).
% that are potentially similar to each other. 
Intra-MB insertion, for instance, sets more MBs in \texttt{INTRA} mode, so that a lost MB will affect fewer other MBs.
%they are independently decodable, even if other MBs are lost.
However, because they do not leverage similarity across MBs, their quality will be much lower than without intra-MB insertion at the same bitrate which violates {\em \REfficient}.
%compression at the same bitrate is significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.
%and others that refer to them decodable, even if other data is lost.
%\footnote{Packet losses can also be tolerated by choosing a better reference frame to allow the receiver to skip undecodable frames without affecting subsequent frames, such as in Salsify~\cite{salsify}. These techniques can be used jointly with this proposal to select better quality reference frames.}
%Both intra-MB insertion and FEC must lower coding efficiency: FEC adds redundancy data and intra-MB insertion keeps more inter-macroblock redundancy.

Several other loss-resilient schemes exist that work without changing the video codecs, though they are less efficient than SVC, FEC at handling transient packet losses. 

\myparaq{Why not reference-frame selection} 
When encoding the next frame, the sender can set the reference frame to be a history frame that has been completely received by the receiver, rather than the last frame. 
This way, a frame that is undecodable due to packet losses can just be skipped without affecting future frames.
However, like intra-MB insertion, its quality will be much lower at the same bitrate than using the last frame as the reference, which violates {\em \REfficient}.
%its compression at the same bitrate will be significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.
An exception is Salsify~\cite{salsify}, which changes to a history frame (not the last one) as reference only {\em after} a loss is detected. 
As a result, however, it must skip several frames before encoding starts with a new reference frame.

\myparaq{Why not selective frame dropping} 
Even if dropping a frame may affect future frames, the receiver can still choose to do that if the impact on the future frame's quality is relatively small.
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) the impact of a dropped frame will stop at the next chunk, which will start in a few seconds with a new i-frame, and (2) the impact of a skipped frame on future frames can be pre-determined offline. 
Unfortunately, both are not true for real-time videos. 


\myparaq{Why not computer vision-based error concealment}
Finally, image inpainting and super-resolution techniques could restore a partial frame. 
Unfortunately, this is doable only {\em if} part of a frame can be decoded based on received data.
This is usually not doable unless techniques like intra-MB insertion are used, which has its own limitations as discussed earlier. For this reason, they are not commonly used in real-time videos.
%different parts of a frame is encoded independently, which at the same bitrate will be significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.


In short, none of the existing loss-resilient schemes achieve the goal of DS video coding and delivery. 
We will also show preliminary results that quantitatively compare them with our proposal in later sections.

==> sections/old/motivate_v7.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\tightsection{Motivation}
\label{sec:motivate}

Video coding has a rich history of research and it is hard to fit a comprehensive overview in limited space.
However, for people unfamiliar with this topic, it helps to introduce the key concepts pertinent to this paper (\S\ref{subsec:background}) before explaining why a different approach is needed (\S\ref{subsec:prior}). 


\tightsubsection{Background of video coding}
\label{subsec:background}

To stream a video, the sender runs a rate adaptation logic to dynamically set the frame rate and bitrate of the encoded video.
%A video stream is encoded at certain frame rate and bitrate, both are controlled by an adaptation logic in the player.
With a frame rate of 25fps (frames per second) and bitrate of 3Mbps, for instance, the encoder should on average generate a 15KB frame every 40ms, though the actual frame size varies.
%depends on the {\em type} of a frame.
A video stream consists of multiple groups of consecutive frames (called group of pictures or GoP), each starting with an I-frame (intra-frame) followed by P-frames (predicted frames) and B-frames (bidirectional predicted frames). 
I-frames are encoded independently (\ie they can be decoded without referring to other frames), so their sizes are often much bigger than P-frames, which only encode the differences between them and other {\em reference} frames.\footnote{On-demand videos also use B-frames, which are smaller than P-frames since they refer to both past and future P-frames. However, to render frames as soon as possible, real-time video rarely use B-frames~\cite{??}, since they refer to future frames to be decoded.}
Thus, I-frames are used infrequently (\eg only when content shifts dramatically) with 10s or more P-frames between two I-frames.
%and each GoP consists of 10s to 100s of P-frames. 
%I-frames are encoded independently, and P-frames and B-frames encode the differences between them and other {\em reference} frames: a P-frame refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames. 
%Importantly, to render each frame as soon as its packets are received, real-time videos almost never use B-frames which refer to future frames~\cite{??}. 
%Since I-frames do not need other frames to decode, their sizes in standard video codecs are much bigger than B-/P-frames, so I-frames are typically used only when content shifts dramatically and each GoP consists of 10s to 100s of frames. 

%As we will see in \S\ref{??}, our new video coding system follows the same frame definitions, though the optimal GoP size will be much smaller. 


%Different {\em frame types} often have different frame sizes.
%An I-frame (intra-frames) is encoded independently and is followed by P-frames (predicted frames) and B-frames (bidirectional predicted frames), each of which encodes the differences between it and some other frames.
%A frame used as a reference for decoding other frames is called a {\em reference} frame: a P-frame only refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames.
%Since I-frames do not need other frames to decode, their sizes are typically bigger than B-/P-frames.


%In real-time videos, to render each frame as soon as its packets are received, B-frames, which refer to future frames, are rarely used~\cite{??}. 
%This precludes several loss-resilient techniques such as B-frame skipping (see \S\ref{??}).

%, and  , each encoding the difference with the previous and future I-/P-frames.
%Thus, I-frames are typically bigger than P-frames and B-frames, but decoding I-frames does not depend on any other frame, while decoding P-frames or B-frames must refer to other frames. 
%fewer other frames than decoding a B-frame.


\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.92\linewidth]{figs/fig2-workflow-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{A typical workflow of a video encoder.}
    \label{fig:codec-workflow}
\end{figure}

To encode a P-frame (Figure~\ref{fig:codec-workflow}), the encoder first calculates motion vectors (MVs) and residuals between macroblocks ($4\times4,8\times8,\dots$) in the current frame and reference frames, then transforms and quantizes them to a more compact form, and finally entropy encodes the data.
%To encode a frame, the encoder first calculates the differences (\eg motion vectors and residuals) among macroblocks ($4\times4,8\times8,\dots$) in the current frame and reference frames (or within an I-frame),  then transforms and quantizes these differences to a more compact form, and finally losslessly encodes the data using arithmetic coding. 
The entropy-encoded data is then packetized and sent out by the transport layer, which tries to deliver as many packets as possible (though not always all packets) to the receiver by the time when the frame is decoded.
%algorithm decides how fast to send a frame's packets, 
%in order to ensure enough data be delivered to the receiver when the frame is decoded. 
The receiver runs a reverse process (depacketization and decoding) to reconstruct each frame from received packets. 
Once a frame is decoded, it will be put in a {\em (jitter) buffer} to conceal transient latency jitter. 
% (due to queuing or retransmits).

That said, to reduce frame delay under long latency, real-time video clients make two common choices~\cite{??}\footnote{\jc{any exceptions?}}:
% that affect the requirements of a desirable video coding scheme.
\begin{packeditemize}
\item Packets of a frame are sent in a burst (without waiting for acks), so %without waiting for acknowledgement.
{\em any} packets in the middle of a frame could be missing when the receiver decodes a frame.
\item The jitter buffer is much {\em shorter} (\eg 10s~ms) than that of on-demand or live broadcast videos (whose buffer is at least a few seconds).
This short buffer often cannot conceal retransmission delay in long-latency networks.
%With a short buffer, any missing packet might delay a frame longer than the jitter buffer can conceal.
\end{packeditemize}
Therefore, loss resilience is vital for real-time video coding!

%real-time videos use  loss resilience of video coding is needed to ensure smooth and high-quality video in presence of packet loss.



 
%Loss-resilient video coding is particularly crucial in real-time videos.\footnote{\jc{clarify real-time video, conversational video, low-latency video}}
%This is because
%%Since packet loss might happen anytime, loss resilience of video coding is needed to maintain smoothness and high quality. 
%%Loss resilience is particularly important for real-time videos, because 
%to maintain high interactivity, real-time videos use a much shorter jitter buffer (just 1-2 frames or 10s~ms) than on-demand or live broadcast videos, whose buffers are likely at least a few seconds.
%With such a short buffer, {\em any packet queuing or retransmit} might block the decoding of a frame after the short buffer is depleted. 


%, which can be caused by either dropped packets or delayed packets.

%To capture the effect of dropped packets and delayed packets on decoding, 

\tightsubsection{\hspace{-0.2cm}Desirable loss-resilient coding for real-time videos}

\mypara{Data-missing rate (\rate)}
We define {\em data-missing rate} ({\em \rate}) as the fraction of data in a frame which, due to queuing or retransmission, have not arrived when the frame is decoded.
%\footnote{\rate can be seen as deadline missing rate, if the deadline is when the decoder decides to decode a frame.}
High \rates can arise from various reasons. 
For instance, a sudden bandwidth drop from 3Mbps to 500Kbps on a 200ms-RTT link can quickly raise \rate to 75\% and retransmission will delay or skip at least 6 frames in a 25fps video stream. 
Previous measurements have shown that 
%if frames are decoded with a fixed intervals (\eg every 40ms for a 25~fps video), 
transient high \rates (\eg $>30\%$) are not rare and are difficult to precisely predict in advance~\cite{??,??,??}. 

\mypara{Data-Scalable (DS) coding}
A desirable video coding, which we refer to as {\em data-scalable} ({\em DS} for short) coding, quality should gracefully degrade in {\em presence} of more packet loss, without compromising the quality in {\em absence} of packet loss.
We breakdown this to three specific requirements:

\begin{packeditemize}
\item {\bf (\RDecodable)} 
The receiver can decode a frame if {\em any} non-empty subset of the packets of this frame is received---{\em minimum need for retransmission or frame skipping}.
%In real-time videos, the delay of a retransmit (at least a round-trip time) is sometimes longer than the jitter buffer (10s~ms), so any retransmit may cause a user-perceivable lag or skipped frames. 
%(\ie no retransmission or frame skipping unless no packet is received);

\item {\bf (\RGraceful)} 
%{\em Graceful degradation:} 
The quality should gradually improve with the addition of any received packet---{\em graceful degradation with higher \rates}.
%(\ie the decoded quality should gracefully degrades with higher \rates).

\item {\bf (\REfficient)} 
%{\em Compression efficiency:} 
If all packets are received, the decoded video will reach a quality close to that of a non-loss-resilient coding algorithm (such as H.265)---{\em high compression efficiency}.
%similar quality as the quality without redundancy (such as H.265), if all packets are received.

\end{packeditemize}




\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/fig2-dmr-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{Illustrative example of the ideal data-scalable coding under dynamic data-missing rates (\rates).
%         \jc{maybe replace it with real values of autoencoder and FEC? }
         }
    \label{fig:codec-dmr}
\end{figure}

\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/big-comparison-v2.pdf}
         \label{fig:}
         \tightcaption{Limitations of current loss-resilient solutions under three packet arrival patterns (no loss and one packet missing at different positions). \greencheck marks both high quality (encoding bitrate approximates the throughput) and low delay (no retransmission).}
    \label{fig:comparison}
\end{figure*}

Figure~\ref{fig:codec-dmr} illustrates the effect of DS coding in action in presence of bursts of high \rates.
% due to bandwidth fluctuations.
We assume that the bandwidth is mostly stable with the high \rates caused by transient bandwidth drops, and that the encoding bitrate matches the actual bandwidth.
As \rate varies over time, the quality of DS coding drops gracefully when \rate is high, but remains high when \rate is low (zero).

%To deliver each frame as quickly as possible, the sender often sends all packets of a frame in {\em one batch}. As a result, {\em any} packets might be missing. 






%in DS, quality grows with the number of {\em any} received packets, whereas in RD, the quality grows with consecutive packets in their sending order. 

%an RD-optimized sender sends packets in specific sending order and its quality grows with only received packets that are before the first missing packet in the sending order.

% assumes that packets are sent in order and packet loss only happens to the latter packets.
%DS is more realistic in real-time videos, because in long-latency networks, the sender should send all packets of a frame in one burst, and loss can happen to any packets, rather than just the last few packets (as shown in Figure~\ref{??}). 


%Second, to reduce frame delay in long-latency networks, the sender often sends all packets of a frame in one burst, rather than multiple congestion windows.
%%Thus loss and delaying can happen to any packets within the burst. 
%This diminishes the benefit of layered coding (introduced shortly) which encodes a video in multiple layers and must deliver the layers in a specific order (see \S\ref{??}).

\tightsubsection{Limitations of prior solutions}
\label{subsec:prior}

Next, we will explain why it is difficult to achieve DS coding using current loss-resilience schemes (such as FEC and rate-distortion optimization).
% and the difference between DS and other similar notions (\eg rate-distortion optimization).


%Next, we examine several representative loss-resilient coding schemes through the lens of the requirements of DS. 
%explain why they fall short of at least one of the three requirements of DS coding.

%Loss resilience has long been an important research topic. 
%Given the sheer amount of prior work in this space, we only highlight those that are most representative or closest to the goal of DS coding. % (see~\cite{??} for a complete survey).
%For ease of comparison, Figure~\ref{fig:primitive-table}  shows how video quality varies with received data (packets) in different loss-resilient techniques. 

%these abstractions also influence the interaction with the remaining parts of a real-time video application, such as congestion control and bitrate adaptation.




\myparaq{Why not bitrate adaptation over TCP}
First, most streaming video systems today rely on congestion control and bitrate adaptation logics to {\em react} to bandwidth fluctuation and rely on TCP to retransmit lost packets. 
They use highly efficient codec (\eg H265), so {\em if} all packets are received on time (\ie retransmission is fast enough), 
%the highly efficient codec (\eg H265) 
they will reach  a high quality with fewer bits. 
%This is well-suited for very low latency (with RTT of a few milliseconds) to allow fast retransmission.
However, it violates \RDecodable because these codecs are not inherently loss tolerant, so a frame cannot be decoded until all packets are received (\eg packet outcome \#2 and \#3 in Figure~\ref{fig:comparison}). 
%In real-time videos, retransmission delays can sometimes be longer than the jitter buffer (10s~ms), causing a visually perceivable lag or a skipped frame.

%re-sending a packet takes longer than the jitter buffer, this can also cause a visually perceivable lag or a skipped frame.

%Essentially, bitrate adaptation is {\em reactive}---if bandwidth suddenly drops, some frames will have already been affected by packet delays/drops before the sender/receiver lowers the bitrate.
%Without a proper loss-resilient scheme, it violates all three requirements of DS coding for real-time videos.

%---it lowers the encoding bitrate {\em after} a bandwidth drop is detected

%Packet retransmission is a conventional loss-resilient scheme. 

\begin{comment}
Frames are coded by a highly efficient codec (\eg H.265), and once all packets are received, the quality will be equal to the original encoded quality.
However, since these codecs optimize for compression, not loss resilience, any lost packets must be resent until all packets are reliably received, which violates {\em \RDecodable}.
If re-sending a packet takes longer than the jitter buffer, this can also cause a visually perceivable lag or a skipped frame.




\myparaq{Why not bitrate adaptation}
Bitrate adaptation lowers the target bitrate of {\em future} video chunks/frames {\em after} a bandwidth drop is detected. %, and then the video encoder will code the future video chunk or frame at the lowered target bitrate. 
Thus, bitrate adaptation is fundamentally {\em reactive}: 
when bandwidth suddenly drops, some frames have already experienced packet delays or drops before the sender/receiver can lower its target bitrate.
Given the short jitter buffer, this can directly hurt user experience, as in Figure~\ref{fig:trace}(a).
Without a proper loss-resilient scheme, it violates all three requirements of DS coding.

\end{comment}

\myparaq{Why not scalable video coding (SVC)}
SVC is aimed at optimizing the classic notion of rate-distortion (RD) tradeoff, which was studied intensively around 2000~\cite{??,??}.
RD optimizes video quality achieved by a single encoded bitstream under different received bitrates.
SVC encodes a video at multiple quality layers, and unlike TCP-based bitrate adaptation, it sends data {\em layer by layer}, and 
%and if the packets are received in order, 
each newly received packet (or layer) will incrementally improve quality and when all packets are received, quality will be close to that of H.265. 
SVC-based techniques have made remarkable progress towards RD-optimized quality in on-demand video streaming, \eg fine-grained scalability (FSG)~\cite{li2001overview} and more recently, DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift}.


\begin{comment}
such that the decoder can reach the $i$-th quality layer, once the packets of $i$-th layer and lower layers are received, and the quality can be incrementally improved to the $(i+1)$-th layer, if the packets of the $(i+1)$-th layer are received.
%as long as the packets belong to the $i$-th layer and lower layers are received, we can obtain the quality of the $i$-th layer.
% and gradually improve quality with more received layers.
SVC-based techniques have made remarkable progress towards RD-optimized quality, especially in on-demand video streaming, \eg fine-grained scalability (FSG)~\cite{li2001overview} and more recently, DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift}.
Unlike TCP-based bitrate adaptation, an SVC sender sends data {\em layer by layer}, and 
%and if the packets are received in order, 
each newly received packet (or layer) will incrementally improve quality and when all packets are received, quality will be close to that of H.265. 
Thus, SVC can greatly benefit multicast videos which serve receivers that have heterogeneous network capacities~\cite{??}.
\end{comment}

However, SVC does not meet {\em \RGraceful}, because it imposes a hierarchical order among the packets of a frame; one missing packet can render all higher quality layers undecodable, even if more packets are received in the higher quality layers~\cite{chen2006frame} (\eg packet outcome \#2 in Figure~\ref{fig:comparison}).
Though sending each layer reliably one by one is possible in on-demand videos~\cite{swift,grad,etc}, real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{subsec:background}), so packet loss can affect any layer.
Thus SVC is rarely used for unicast real-time video sessions~\cite{??} (though SVC still greatly benefits multicast videos to serve users with heterogeneous network capacities~\cite{??}).
Essentially, DS coding differs from RD optimization on a key aspect---the quality of DS coding depends on {\em how many} packets, not {\em which} packets, are received.


\begin{comment}

There have been many SVC techniques---notably, fine-grained scalability (FSG)~\cite{li2001overview} and more recently, DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift} achieve near-optimal rate-distortion (RD) tradeoffs: if the packets are received in order, each newly received packet will incrementally improve quality and when all packets are received, quality will be close to that of H.265. 
%realize the following effect: if the packets are received in order, each new packet will incrementally improve quality, and when all packets are received, the quality is similar to H.265. 
Therefore, SVC can greatly benefit multicast videos as a way to serve receivers that have heterogeneous network capacities~\cite{??}.

However, SVC imposes a hierarchical order among packets that one missing packet can render all higher quality layers undecodable, even if more packets are received on higher quality layers~\cite{chen2006frame}; in other words, it violates {\em \RGraceful}.
Though sending each layer reliably one by one is possible in on-demand videos~\cite{swift,grad,etc}, real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{??}), so packet loss can affect any layer.
For this reason, SVC is not widely used to improve quality of unicast real-time video sessions~\cite{??}.


Note that DS is different from the classic notion of rate-distortion (RD) optimization, which was studied intensively around 2000~\cite{??,??}. 
%DS video coding may sound similar to the classic rate-distortion (RD) tradeoff, which was intensively studied around early 2000s~\cite{??,??}. 
RD optimizes video quality achieved by a single encoded bitstream under different received bitrates.
%, and ideally, with a single encoded bitstream, the decoding quality of the received data naturally increase if more data of the bitstream is received.
DS differs on a key aspect.
%The quality of DS coding grows with more received packets, regardless of their positions in the original sending order.
The quality of DS coding depends on {\em how many} packets, not {\em which} packets, are received.
In contrast, RD assumes that the packets have some dependencies and its quality increases with more packets received before the first missing packet in the original sending order. 
For instance, suppose that three packets are sent and the 2nd packet is the first missing packet. If the 3rd packet is received, then the quality of DS coding will grow but the quality of RD coding will not, since only one packet before the missing packet is received.
DS coding is more suitable for real-time videos, because as said earlier, senders of real-time videos burst packets of each frame, so loss can happen to any packets, rather than just the last packets.

\end{comment}


\begin{comment}

This makes sense in on-demand videos where different layers can be sent reliably one by one~\cite{??}.
In addition, 

However, SVC imposes a hierarchical order that one missing packet can render all higher quality layers undecodable, it violates requirement {\em \RGraceful}~\cite{chen2006frame}.
In unicast real-time video communication, however, senders often send all packets of a frame in {\em one batch}, rather than layer by layer, because the round-trip time is often higher than jitter buffer, 
As a result, {\em any} packets can be lost. 



with non-trivial network latency, so to reduce each frame's delay, most senders send packets of a frame as one batch.

SVC imposes a hierarchical order that one missing packet can render all higher quality layers undecodable, it violates requirement {\em \RGraceful}~\cite{chen2006frame}.
%\footnote{The classic SVC violates both requirement {\em (ii)} and {\em (iii)} of DS coding, though {\em (iii)} is mitigated by an autoencoder-based codec~\cite{swift} proposed recently.}
Even if the base (lowest) layer is padded with redundancy (\eg FEC, explained shortly)~\cite{SVCFEC1, schierl2007using,wang2000error}, it does not protect other layers from packet losses.\footnote{\jc{move this footnote to SVC later}The state-of-the-art solution, which is also based on neural-network autoencoders~\cite{swift}, can generate a single encoded bitstream to  {\em approximate} the optimal RD tradeoff, though still with a substantial margin.}

Other than SVC, there have been several other proposals that aim for finer-grained scalability.
Notably, fine-grained scalability (FSG)~\cite{li2001overview} and more recently DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift} strive to realize the following effect: if the packets are received in order, each new packet will incrementally improve quality, and when all packets are received, the quality is similar to H.265. 
Though they are better than classic SVC, they still impose a hierarchical structure over packets, which violates requirement {\em \RGraceful}---if a low-quality-layer packet of is missing, higher-quality-layer packets are not useful.\footnote{It should be clarified that SVC does achieve coding scalability with on-demand videos, which has enough buffer to allow packet retransmission.
%, where the sender usually makes sure one layer is fully received before sending the next one.
}

\jc{old text}
 (\eg as we will explain shortly, in scalable coding, data of lower coding layer is reliably received before fetching higher layers). 
With this assumption, RD-optimized coding can still greatly improve multicast service (\eg in multi-party video conferencing) and on-demand videos where different layers can be received one by one. 
Our paper aims at unicast real-time video communication with non-trivial network latency, so to reduce each frame's delay, most senders send packets of a frame as one batch.

\end{comment}

%one single lost packet of a lower layer will make all higher layers undecoded. 
%This violates requirement {\em (ii)} of DS coding.
%While the base (lowest-quality) layer of SVC is often padded with redundancy (\eg FEC, explained shortly)~\cite{wang2000error}, it does not protect other layers from packet losses.
%






\myparaq{Why not error correction coding (\eg FEC)}
The most common loss-resilient coding in real-time video is forward error correction (FEC) and its recent variants (\eg streaming code~\cite{??} and rateless fountain code~\cite{??}). 
%These redundancy-based schemes essentially trade coding efficiency for loss resilience. 
Given a target frame size $R$, FEC encodes frames at $N\%\cdot R$, with the remaining $(1-N\%)\cdot R$ used for redundancy. $(1-N\%)$ is the {\em redundancy rate}.
The frame will be decodable, once {\em any} $N\%$ of packets are received.
FEC differs from SVC in that SVC depends on {\em which data} is received, whereas FEC depends on {\em how much} data is received.

However, FEC-based schemes\footnote{\jc{some words on why rateless doesn't help here} \jc{also a parallel work tumbr has the same problem}} must know \rate~{\em before} sending the data; otherwise it will add either too much redundancy or still need to retransmit. 
%they work better only if \rate is known {\em before} FEC encodes the data. 
%must know \rate in advance to avoid packet retransmission and too much redundancy.
If redundancy is not enough to conceal missing packets in time (\ie~\rate is underestimated), some packets must be waited or retransmitted in order to decode the frame, which violates {\em \RDecodable} (\eg 10\% FEC in Figure~\ref{fig:comparison}).
Once the received packets are decodable, more packets will not improve the quality, which violates {\em \RGraceful}.
And if all packets are received (\ie~\rate is overestimated), the redundancy will lower the video quality, which violates {\em \REfficient} (\eg FEC 33\% with packet outcome \#1 in Figure~\ref{fig:comparison}).

%if much redundancy is added while all packets are received (\ie loss rate is overestimated), the decoded quality will be much lower than it could have been without redundancy (which violates {\em \REfficient}).

%\jc{include streaming code}




\myparaq{Why not redundant video coding}
%Source-coding-based schemes do not explicitly add redundancy like FEC. 
Besides FEC which adds redundancy to video encoder output, the video coding itself can be made more resilient to packet loss\footnote{In the video coding literature, the former (\eg FEC) refers to channel coding, while the latter refers to source coding.}.
Two examples are intra-MB insertion and reference selection, but both methods do not meet {\em \REfficient}, because they also add redundancy and have much lower quality if no packet turns out missing. 
Intra-MB insertion~\cite{??} sets more macroblocks (MBs) in \texttt{INTRA} mode which makes their decoding not dependant on other frames, so missing one MB will affect fewer other MBs.
However, doing so fails to exploit similar MBs across different frames, their quality will be lower than without intra-MB insertion at the same bitrate.
Moreover, when the information of an MB is missing, they use handcrafted heuristics\footnote{For instance, one method to recover the motion vector (MV) of an MB~\cite{yihua?} is to search surrounding MBs whose MVs are not lost, and copy the one that causes least pixel differences (``glitches''). We empirically observe that such recovery is less effective than the NN-based coding proposed in this work.\jc{yihua, any pointer to an evidence?}} to recover it and this may not always be effective (see \S\ref{??}).

Reference selection uses an older but reliably received frame, instead of the last frame, as the reference frame, allowing the decoder to safely skip a loss-affected frame (\eg~\cite{salsify}).
However, this method also needs more bits to encode the same quality than using the last frame as reference, because the difference between two consecutive frames is much less than other history frames (\eg the P-frames between every other frames are \fillme\% greater in size than between two consecutive frames).

\begin{comment}
Reference selection uses an older frame already received by the receiver, instead of the last frame, as the reference to encode a new frame (\eg~\cite{salsify}), so any frame undecodable due to packet losses can be safely skipped without affecting future frames.
%setting its reference frame to some history frame that has been received by the receiver, rather than the last frame~\cite{salsify}. 
%This way, a frame that is undecodable due to packet losses can just be safely skipped without affecting future frames.

Both methods, however, do not meet {\em \REfficient}, because they use redundancy and have much lower quality if all packets are received. 
%In both cases, however, they have to sacrifice some compression efficiency if all packets are received, which violates {\em \REfficient}.
Intra-MB insertion fails to exploit similar MBs across different frames, their quality will be lower than without intra-MB insertion at the same bitrate.
%Like intra-MB insertion, 
Reference selection needs more bits to encode the same quality level, because the difference between two consecutive frames is much less than other history frames (\eg the P-frames between every other frames are \fillme\% greater in size than between two consecutive frames).

Both error-correction coding and redundant video coding must choose between compression efficiency (quality in absence of packet loss) and loss resilient (quality in presence of packet loss). 
For this reason, in practice, they are used {\em after} packet loss occurs---FEC is activated by WebRTC or the reference frame is changed by Salsify, only after the first packet loss is detected by the sender, which is at least one round-trip time after the packet loss occurs.
%Figure~\ref{fig:codec-dmr} shows an example of FEC. 
%The sender typically only adds redundancy {\em after} packet loss or delay increase affect a few frames, and when they may also add too much redundancy even after the \rate drops, resulting in low quality.

\end{comment}


\begin{comment}

reduce the inter-dependencies between macroblocks (MBs).
% that are potentially similar to each other. 
Intra-MB insertion, for instance, sets more MBs in \texttt{INTRA} mode, so that a lost MB will affect fewer other MBs.
%they are independently decodable, even if other MBs are lost.
However, because they do not leverage similarity across MBs, their quality will be much lower than without intra-MB insertion at the same bitrate which violates {\em \REfficient}.
%compression at the same bitrate is significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.
%and others that refer to them decodable, even if other data is lost.
%\footnote{Packet losses can also be tolerated by choosing a better reference frame to allow the receiver to skip undecodable frames without affecting subsequent frames, such as in Salsify~\cite{salsify}. These techniques can be used jointly with this proposal to select better quality reference frames.}
%Both intra-MB insertion and FEC must lower coding efficiency: FEC adds redundancy data and intra-MB insertion keeps more inter-macroblock redundancy.

Several other loss-resilient schemes exist that work without changing the video codecs, though they are less efficient than SVC, FEC at handling transient packet losses. 



\myparaq{Why not reference-frame selection} 
When encoding the next frame, the sender can set the reference frame to be a history frame that has been completely received by the receiver, rather than the last frame. 
This way, a frame that is undecodable due to packet losses can just be skipped without affecting future frames.
However, like intra-MB insertion, its quality will be much lower at the same bitrate than using the last frame as the reference, which violates {\em \REfficient}.
%its compression at the same bitrate will be significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.
An exception is Salsify~\cite{salsify}, which changes to a history frame (not the last one) as reference only {\em after} a loss is detected. 
As a result, however, it must skip several frames before encoding starts with a new reference frame.

\end{comment}

%\mypara{Receiver-side loss concealment}
\mypara{Error concealment by receiver}
The receiver can also choose to skip a loss-affected frame, if skipping it does not affect future quality. 
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) B-frames can naturally be safely skipped, (2) the impact of a skipped frame will stop at next chunk (in a few seconds) when a new I-frame starts, and (3) the impact of skipping each frame on future frames can be pre-determined offline. 
Unfortunately, none of them is true for real-time videos, in which B-frames are rarely used in and I-frames are used less often.
Another receiver-side solution is to use image inpainting algorithms to restore a partially received frame. 
However, this is doable only {\em if} part of a frame can be decoded based on received data, which must rely on some other techniques mentioned earlier. 
For these reasons, they are not commonly used in real-time videos.


%requires techniques like intra-MB insertion are used, which has its own limitations as discussed earlier. For this reason, they are not commonly used in real-time videos.



\begin{comment}

The receiver can also choose to skip a frame depending on the frame's impact on future quality, but for frames whose absence will greatly affect the quality of other frames, this violates at least requirements of  $\RDecodable$ and $\RGraceful$.
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) the impact of a dropped frame will stop at next chunk (in a few seconds) which starts with a new I-frame, and (2) the impact of a skipped frame on future frames can be pre-determined offline. 
Unfortunately, both are not true for real-time videos.

\end{comment}


\begin{comment}

\myparaq{Why not selective frame dropping} 
Even if dropping a frame may affect future frames, the receiver can still choose to do that if the impact on the future frame's quality is relatively small.
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) the impact of a dropped frame will stop at the next chunk, which will start in a few seconds with a new i-frame, and (2) the impact of a skipped frame on future frames can be pre-determined offline. 
Unfortunately, both are not true for real-time videos. 


\myparaq{Why not computer vision-based error concealment}
Finally, image inpainting and super-resolution techniques could restore a partial frame. 
Unfortunately, this is doable only {\em if} part of a frame can be decoded based on received data.
This is usually not doable unless techniques like intra-MB insertion are used, which has its own limitations as discussed earlier. For this reason, they are not commonly used in real-time videos.
%different parts of a frame is encoded independently, which at the same bitrate will be significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.

\end{comment}

In summary, none of the existing loss-resilient schemes achieve the goal of DS video coding. 
%We will also show preliminary results that quantitatively compare them with our proposal in later sections.

%\jc{is \name compatible with multi-party calls}


\begin{comment}



\myparaq{What's new in real-time video}
While this general workflow applies to most video streaming systems, real-time videos are distinctive in that they seek to reduce the {\em frame delay} between sending a frame and decoding it.
This profoundly affects their design choices in three ways.
%have three features distinct from others, which profoundly affect their designs. 
%short jitter buffer, no b frame, packets sent toghether, all of which have profound impact
\begin{packeditemize}
\item {\em Short jitter buffer:} First, real-time videos use a much shorter jitter buffer (just 1-2 frames or 10s of milliseconds) than even live broadcast videos, which have a buffer of at least a few seconds.
While increasing interactivity between clients, the short buffer makes the receiver potentially vulnerable to {\em any packet queuing or retransmit} that blocks the decoding of a frame after the short buffer is depleted. 


\item {\em Each frame sent in one batch:} Second, to reduce frame delay in long-latency networks, the sender often sends all packets of a frame in one burst, rather than multiple congestion windows.
%Thus loss and delaying can happen to any packets within the burst. 
This diminishes the benefit of layered coding (introduced shortly) which encodes a video in multiple layers and must deliver the layers in a specific order (see \S\ref{??}).


\item {\em Avoid B-frames:} Third, as each frame should be decoded as soon as its packets are received, B-frames are rarely used in real-time videos~\cite{??}, since they require future frames to be received. 
This precludes several loss-resilient techniques such as B-frame skipping (see \S\ref{??}).
\end{packeditemize}



\begin{itemize}
\item 2.1 Background
\begin{itemize}
\item basics: video, encoder, decoder, packets
\item real-time video: small jitter buffer, all packets must be sent together
\item concept of loss-resilient coding
\end{itemize}

\item 2.2 Ideal coding for real-time video
\begin{itemize}
\item given that 
\end{itemize}

\item 2.3 Limitations
\begin{itemize}
\item type 1: scalable coding
\item type 2: fec (rateless versions), reference selection, recover
\end{itemize}
\end{itemize}

We begin with why loss-resilient video coding is particularly important to real-time video and what an ideal scheme should achieve. 
We then explain the limitations of existing approaches.

Despite more bandwidth, many recent studies have shown that real-time video communication is plagued with intermittent packet loss and jitter~\cite{macmillan2021measuring,jansen2018performance,concerto,moulay2018experimental,latency-report-iab,latency-report-iab-2,latency-report-apnic}.
%induced by congestion, wireless, bufferbloat, etc.
\jc{yihua, can we find a few good pointers for this?}
%Adapting bitrate (ABR), which {\em reacts} to fluctuations of network conditions, is not enough to completely prevent packet loss, without using an extremely conservative bitrate. 
Since real-time video clients have very shallow jitter buffers, there is little time for packet retransmission before each frame should be decoded. 
So unlike in traditional streaming videos (which has a buffer of at least several seconds),
%Having shallow jitter buffers means that adapting bitrate or sending rate alone is not enough for clients to be immune to packet loss. 
%This leaves little time for packet retransmission, so 
{\em any} dropped or queued packets could delay the decoding of a frame, causing video stuttering and frame skipping in real-time video applications. 

%Having shallow jitter buffers also means that adapting bitrate or sending rate alone is not adequate to make real-time video client immune to packet loss.
%
%
%It is hard to predict how many packets will be dropped 
%Thus, the ability to decode a frame with a decent quality in presence of packet loss is crucial.




%\jc{Relationship with bitrate adaptation}

\end{comment}

==> sections/old/motivate_v8.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\tightsection{Motivation}
\label{sec:motivate}

Video coding has a rich history of research and it is hard to fit a comprehensive overview in a limited space.
Nonetheless, for those who are unfamiliar with this topic, it is beneficial to introduce the key concepts relevant to this paper (\S\ref{subsec:background}) before explaining the need for a different approach (\S\ref{subsec:ds},\ref{subsec:prior}). 


\tightsubsection{Background of video coding}
\label{subsec:background}

The video sender runs a rate adaptation logic to dynamically set the frame rate and bitrate of the encoded video.
%A video stream is encoded at certain frame rate and bitrate, both are controlled by an adaptation logic in the player.
With a frame rate of 25fps (frames per second) and bitrate of 3Mbps, for instance, the encoder should on average generate a 15KB frame every 40ms, though the actual frame size varies.
%depends on the {\em type} of a frame
A video stream consists of multiple groups of consecutive frames (called group of pictures or GoP), each starting with an I-frame (intra-frame) followed by P-frames (predicted frames) and B-frames (bidirectional predicted frames). 
I-frames are encoded independently (\ie they can be decoded without referring to other frames), so their sizes are often much bigger than P-frames, which only encode the differences between themselves and other {\em reference} frames.\footnote{On-demand videos also use B-frames, which 
% are smaller than P-frames since they 
refer to both past and future P-frames. However, real-time video rarely uses B-frames in order to render frames as soon as possible.
% However, to render frames as soon as possible, real-time video rarely uses B-frames~\cite{??}, since they refer to future frames to be decoded.
}

% Thus, I-frames are used infrequently (\eg only when content shifts dramatically) with 10s or more P-frames between two I-frames.

%and each GoP consists of 10s to 100s of P-frames. 
%I-frames are encoded independently, and P-frames and B-frames encode the differences between them and other {\em reference} frames: a P-frame refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames. 
%Importantly, to render each frame as soon as its packets are received, real-time videos almost never use B-frames which refer to future frames~\cite{??}. 
%Since I-frames do not need other frames to decode, their sizes in standard video codecs are much bigger than B-/P-frames, so I-frames are typically used only when content shifts dramatically and each GoP consists of 10s to 100s of frames. 

%As we will see in \Sref{??}, our new video coding system follows the same frame definitions, though the optimal GoP size will be much smaller. 


%Different {\em frame types} often have different frame sizes.
%An I-frame (intra-frames) is encoded independently and is followed by P-frames (predicted frames) and B-frames (bidirectional predicted frames), each of which encodes the differences between it and some other frames.
%A frame used as a reference for decoding other frames is called a {\em reference} frame: a P-frame only refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames.
%Since I-frames do not need other frames to decode, their sizes are typically bigger than B-/P-frames.


%In real-time videos, to render each frame as soon as its packets are received, B-frames, which refer to future frames, are rarely used~\cite{??}. 
%This precludes several loss-resilient techniques such as B-frame skipping (see \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{??}).

%, and  , each encoding the difference with the previous and future I-/P-frames.
%Thus, I-frames are typically bigger than P-frames and B-frames, but decoding I-frames does not depend on any other frame, while decoding P-frames or B-frames must refer to other frames. 
%fewer other frames than decoding a B-frame.


\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/fig2-workflow-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{A typical workflow of a video encoder.}
    \label{fig:codec-workflow}
\end{figure}

To encode a P-frame (Figure~\ref{fig:codec-workflow}), the encoder first calculates motion vectors (MVs) and residuals of each macroblock (MB, each of 4×4,8×8,\dots) in the current frame, then transforms and quantizes them to a more compact form, and finally, entropy encodes the data.
%To encode a frame, the encoder first calculates the differences (\eg motion vectors and residuals) among macroblocks (4×4,8×8,…4\times4,8\times8,\dots) in the current frame and reference frames (or within an I-frame),  then transforms and quantizes these differences to a more compact form, and finally losslessly encodes the data using arithmetic coding. 
The entropy-encoded data is then packetized and sent out by the transport layer, which tries to deliver as many packets as possible 
% (though not always all packets) 
to the receiver by the time when the frame is decoded.
%algorithm decides how fast to send a frame's packets, 
%in order to ensure enough data be delivered to the receiver when the frame is decoded. 
Similarly, the receiver depacketizes and decodes the received data to 
% runs a reverse process (depacketization and decoding) to 
reconstruct each frame from received packets. 
A decoded frame is put in a {\em buffer} before playing to conceal transient latency jitters. 
% (due to queuing or retransmits).

To reduce frame delay under long latency, real-time video clients make two common choices~\cite{10.1145/3410449,salsify}: %\footnote{\jc{any exceptions?}}:
% that affect the requirements of a desirable video coding scheme.
\begin{packeditemize}
\item Packets of a frame are sent in a burst (without waiting for acks), so %without waiting for acknowledgement.
{\em any} packets in the middle of a frame could be missing (delayed or dropped) when the receiver tries to decode the frame.
\item The jitter buffer is much {\em shorter} (\eg 10s~ms) than that of on-demand or live broadcast videos (whose buffer is at least a few seconds).
Thus, retransmission delay often cannot be concealed, particularly in long-latency networks.
% This short buffer often cannot conceal retransmission delay in long-latency networks.
%With a short buffer, any missing packet might delay a frame longer than the jitter buffer can conceal.
\end{packeditemize}
Therefore, loss resilience is vital for real-time video coding!

%real-time videos use  loss resilience of video coding is needed to ensure smooth and high-quality video in presence of packet loss.



 
%Loss-resilient video coding is particularly crucial in real-time videos.\footnote{\jc{clarify real-time video, conversational video, low-latency video}}
%This is because
%%Since packet loss might happen anytime, loss resilience of video coding is needed to maintain smoothness and high quality. 
%%Loss resilience is particularly important for real-time videos, because 
%to maintain high interactivity, real-time videos use a much shorter jitter buffer (just 1-2 frames or 10s~ms) than on-demand or live broadcast videos, whose buffers are likely at least a few seconds.
%With such a short buffer, {\em any packet queuing or retransmit} might block the decoding of a frame after the short buffer is depleted. 


%, which can be caused by either dropped packets or delayed packets.

%To capture the effect of dropped packets and delayed packets on decoding, 

\tightsubsection{\hspace{-0.2cm}Desirable loss-resilient coding for real-time videos}
\label{subsec:ds}

\mypara{Data-missing rate (\rate)}
We define data-missing rate (\rate) as the fraction of packets of a frame that have not arrived when the frame is decoded.
A missing packet can be due to queuing or retransmission.
%\footnote{\rate can be seen as deadline missing rate, if the deadline is when the decoder decides to decode a frame.}
High \rates arise from various reasons. 
For instance, a sudden bandwidth drop from 3Mbps to 500Kbps on a 200ms-RTT link can quickly raise \rate to 75\% and retransmission will delay or skip at least 6 frames in a 25fps video stream. 
Previous measurements have shown that 
%if frames are decoded with a fixed intervals (\eg every 40ms for a 25~fps video), 
transient high \rates (\eg $>30\%$) are not rare and are difficult to precisely predict in advance~\cite{macmillan2021measuring}. 
Note that our work does {\bf not} assume that high \rates are persistent in presence of a rate adaptation logic.

\mypara{Data-Scalable (DS) coding}
In a desirable video coding, which we refer to as {\em data-scalable} ({\em DS} for short) coding, quality should gracefully degrade in {\em presence} of more packet loss, without compromising the quality in {\em absence} of packet loss.
We breakdown this to three specific requirements:

\begin{packeditemize}
\item {\bf (\RDecodable)} 
The receiver can decode a frame if {\em any} non-empty subset of the packets of this frame is received---{\em minimum need for retransmission or frame skipping}.
%In real-time videos, the delay of a retransmit (at least a round-trip time) is sometimes longer than the jitter buffer (10s~ms), so any retransmit may cause a user-perceivable lag or skipped frames. 
%(\ie no retransmission or frame skipping unless no packet is received);

\item {\bf (\RGraceful)} 
%{\em Graceful degradation:} 
The quality should gradually improve with the addition of any received packet---{\em graceful degradation with higher \rates}.
%(\ie the decoded quality should gracefully degrades with higher \rates).

\item {\bf (\REfficient)} 
%{\em Compression efficiency:} 
If all packets are received, the decoded video will reach a quality close to that of a non-loss-resilient coding algorithm (such as H.265)---{\em high compression efficiency}.
%similar quality as the quality without redundancy (such as H.265), if all packets are received.

\end{packeditemize}




\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/fig2-dmr-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{Illustrative example of the ideal data-scalable coding under dynamic data-missing rates (\rates).
%         \jc{maybe replace it with real values of autoencoder and FEC? }
         }
    \label{fig:codec-dmr}
\end{figure}

\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.97\linewidth]{figs/big-comparison-v2.pdf}
         \label{fig:}
         \tightcaption{Limitations of current loss-resilient solutions under three packet arrival patterns (no loss and one packet missing at different positions). \greencheck marks both high quality (encoding bitrate approximates the throughput) and low delay (no retransmission).}
    \label{fig:comparison}
\end{figure*}

Figure~\ref{fig:codec-dmr} illustrates the effect of DS coding in action. % in presence of bursts of high \rates.
% due to bandwidth fluctuations.
We assume that the bandwidth is mostly stable with intermittent high-\rate spikes caused by transient bandwidth drops and that the encoding bitrate matches the actual bandwidth.
As \rate varies over time, the quality of DS coding is high \rate is low (zero) and drops gracefully when \rate is high.

%To deliver each frame as quickly as possible, the sender often sends all packets of a frame in {\em one batch}. As a result, {\em any} packets might be missing. 






%in DS, quality grows with the number of {\em any} received packets, whereas in RD, the quality grows with consecutive packets in their sending order. 

%an RD-optimized sender sends packets in specific sending order and its quality grows with only received packets that are before the first missing packet in the sending order.

% assumes that packets are sent in order and packet loss only happens to the latter packets.
%DS is more realistic in real-time videos, because in long-latency networks, the sender should send all packets of a frame in one burst, and loss can happen to any packets, rather than just the last few packets (as shown in Figure~\ref{??}). 


%Second, to reduce frame delay in long-latency networks, the sender often sends all packets of a frame in one burst, rather than multiple congestion windows.
%%Thus loss and delaying can happen to any packets within the burst. 
%This diminishes the benefit of layered coding (introduced shortly) which encodes a video in multiple layers and must deliver the layers in a specific order (see \S\ref{??}).

\tightsubsection{Limitations of prior solutions}
\label{subsec:prior}

Next, we will explain why it is difficult to achieve DS coding using current loss-resilience schemes, including FEC, SVC, and error concealment.
% rate-distortion optimization
% and the difference between DS and other similar notions (\eg rate-distortion optimization).


%Next, we examine several representative loss-resilient coding schemes through the lens of the requirements of DS. 
%explain why they fall short of at least one of the three requirements of DS coding.

%Loss resilience has long been an important research topic. 
%Given the sheer amount of prior work in this space, we only highlight those that are most representative or closest to the goal of DS coding. % (see~\cite{??} for a complete survey).
%For ease of comparison, Figure~????????????\ref{fig:primitive-table}  shows how video quality varies with received data (packets) in different loss-resilient techniques. 

%these abstractions also influence the interaction with the remaining parts of a real-time video application, such as congestion control and bitrate adaptation.




\myparaq{Why not bitrate adaptation over TCP}
First, most streaming video systems today rely on congestion control and bitrate adaptation logics to {\em react} to bandwidth fluctuation and rely on \st{TCP to retransmit} \edit{retransmission to recover from} lost packets. 
They use highly efficient codec (\eg H265), so {\em if} all packets are received on time (\ie retransmission is fast enough), 
%the highly efficient codec (\eg H265) 
they will reach  a high quality with fewer bits. 
%This is well-suited for very low latency (with RTT of a few milliseconds) to allow fast retransmission.
However, it violates \RDecodable because these codecs are not inherently loss tolerant, so a frame cannot be decoded until all packets are received (\eg packet outcome \#2 and \#3 in Figure~\ref{fig:comparison}). 
%In real-time videos, retransmission delays can sometimes be longer than the jitter buffer (10s~ms), causing a visually perceivable lag or a skipped frame.

%re-sending a packet takes longer than the jitter buffer, this can also cause a visually perceivable lag or a skipped frame.

%Essentially, bitrate adaptation is {\em reactive}---if bandwidth suddenly drops, some frames will have already been affected by packet delays/drops before the sender/receiver lowers the bitrate.
%Without a proper loss-resilient scheme, it violates all three requirements of DS coding for real-time videos.

%---it lowers the encoding bitrate {\em after} a bandwidth drop is detected

%Packet retransmission is a conventional loss-resilient scheme. 

\begin{comment}
Frames are coded by a highly efficient codec (\eg H.265), and once all packets are received, the quality will be equal to the original encoded quality.
However, since these codecs optimize for compression, not loss resilience, any lost packets must be resent until all packets are reliably received, which violates {\em \RDecodable}.
If re-sending a packet takes longer than the jitter buffer, this can also cause a visually perceivable lag or a skipped frame.




\myparaq{Why not bitrate adaptation}
Bitrate adaptation lowers the target bitrate of {\em future} video chunks/frames {\em after} a bandwidth drop is detected. %, and then the video encoder will code the future video chunk or frame at the lowered target bitrate. 
Thus, bitrate adaptation is fundamentally {\em reactive}: 
when bandwidth suddenly drops, some frames have already experienced packet delays or drops before the sender/receiver can lower its target bitrate.
Given the short jitter buffer, this can directly hurt user experience, as in Figure~\ref{fig:trace}(a).
Without a proper loss-resilient scheme, it violates all three requirements of DS coding.

\end{comment}

\myparaq{Why not scalable video coding (SVC)}
SVC tries to optimize the classic notion of rate-distortion (RD) tradeoff, which which represents video quality achieved by a single encoded bitstream under different received bitrates and was studied intensively around 2000~\cite{schwarz2007overview, schierl2007mobile}.
SVC encodes a video at multiple quality layers and  sends data {\em layer by layer}, so that
%and if the packets are received in order, 
each newly received packet (or layer) will incrementally improve quality. % and when all packets are received, quality will be close to that of H.265. 
SVC-based techniques have made remarkable progress towards RD-optimized quality in on-demand video streaming, \eg fine-grained scalability (FSG)~\cite{li2001overview} and more recently, DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift}.


\begin{comment}
such that the decoder can reach the $i$-th quality layer, once the packets of $i$-th layer and lower layers are received, and the quality can be incrementally improved to the $(i+1)$-th layer, if the packets of the $(i+1)$-th layer are received.
%as long as the packets belong to the $i$-th layer and lower layers are received, we can obtain the quality of the $i$-th layer.
% and gradually improve quality with more received layers.
SVC-based techniques have made remarkable progress towards RD-optimized quality, especially in on-demand video streaming, \eg fine-grained scalability (FSG)~\cite{li2001overview} and more recently, DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift}.
Unlike TCP-based bitrate adaptation, an SVC sender sends data {\em layer by layer}, and 
%and if the packets are received in order, 
each newly received packet (or layer) will incrementally improve quality and when all packets are received, quality will be close to that of H.265. 
Thus, SVC can greatly benefit multicast videos which serve receivers that have heterogeneous network capacities~\cite{??}.
\end{comment}

However, SVC does not meet {\em \RGraceful}, because it imposes a hierarchical order among the packets of a frame; one missing packet can affect all higher quality layers, even if more packets are received in the higher quality layers (\eg packet outcome \#2 in Figure~\ref{fig:comparison}).
Though sending each layer reliably one by one is possible in on-demand videos~\cite{swift,grad}, real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{subsec:background}), so packet loss can affect any layer.
As a result, SVC is rarely used to improve unicast real-time video (though it is used widely by multicast videos to serve users with heterogeneous network capacities~\cite{schierl2007mobile}).
Essentially, DS coding differs from RD optimization on a key aspect---the quality of DS coding depends on {\em how many} packets, not {\em which} packets, are received.


\begin{comment}

There have been many SVC techniques---notably, fine-grained scalability (FSG)~\cite{li2001overview} and more recently, DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift} achieve near-optimal rate-distortion (RD) tradeoffs: if the packets are received in order, each newly received packet will incrementally improve quality and when all packets are received, quality will be close to that of H.265. 
%realize the following effect: if the packets are received in order, each new packet will incrementally improve quality, and when all packets are received, the quality is similar to H.265. 
Therefore, SVC can greatly benefit multicast videos as a way to serve receivers that have heterogeneous network capacities~\cite{??}.

However, SVC imposes a hierarchical order among packets that one missing packet can render all higher quality layers undecodable, even if more packets are received on higher quality layers~\cite{chen2006frame}; in other words, it violates {\em \RGraceful}.
Though sending each layer reliably one by one is possible in on-demand videos~\cite{swift,grad,etc}, real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{??}), so packet loss can affect any layer.
For this reason, SVC is not widely used to improve quality of unicast real-time video sessions~\cite{??}.


Note that DS is different from the classic notion of rate-distortion (RD) optimization, which was studied intensively around 2000~\cite{??,??}. 
%DS video coding may sound similar to the classic rate-distortion (RD) tradeoff, which was intensively studied around early 2000s~\cite{??,??}. 
RD optimizes video quality achieved by a single encoded bitstream under different received bitrates.
%, and ideally, with a single encoded bitstream, the decoding quality of the received data naturally increase if more data of the bitstream is received.
DS differs on a key aspect.
%The quality of DS coding grows with more received packets, regardless of their positions in the original sending order.
The quality of DS coding depends on {\em how many} packets, not {\em which} packets, are received.
In contrast, RD assumes that the packets have some dependencies and its quality increases with more packets received before the first missing packet in the original sending order. 
For instance, suppose that three packets are sent and the 2nd packet is the first missing packet. If the 3rd packet is received, then the quality of DS coding will grow but the quality of RD coding will not, since only one packet before the missing packet is received.
DS coding is more suitable for real-time videos, because as said earlier, senders of real-time videos burst packets of each frame, so loss can happen to any packets, rather than just the last packets.

\end{comment}


\begin{comment}

This makes sense in on-demand videos where different layers can be sent reliably one by one~\cite{??}.
In addition, 

However, SVC imposes a hierarchical order that one missing packet can render all higher quality layers undecodable, it violates requirement {\em \RGraceful}~\cite{chen2006frame}.
In unicast real-time video communication, however, senders often send all packets of a frame in {\em one batch}, rather than layer by layer, because the round-trip time is often higher than jitter buffer, 
As a result, {\em any} packets can be lost. 



with non-trivial network latency, so to reduce each frame's delay, most senders send packets of a frame as one batch.

SVC imposes a hierarchical order that one missing packet can render all higher quality layers undecodable, it violates requirement {\em \RGraceful}~\cite{chen2006frame}.
%\footnote{The classic SVC violates both requirement {\em (ii)} and {\em (iii)} of DS coding, though {\em (iii)} is mitigated by an autoencoder-based codec~\cite{swift} proposed recently.}
Even if the base (lowest) layer is padded with redundancy (\eg FEC, explained shortly)~\cite{SVCFEC1, schierl2007using,wang2000error}, it does not protect other layers from packet losses.\footnote{\jc{move this footnote to SVC later}The state-of-the-art solution, which is also based on neural-network autoencoders~\cite{swift}, can generate a single encoded bitstream to  {\em approximate} the optimal RD tradeoff, though still with a substantial margin.}

Other than SVC, there have been several other proposals that aim for finer-grained scalability.
Notably, fine-grained scalability (FSG)~\cite{li2001overview} and more recently DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift} strive to realize the following effect: if the packets are received in order, each new packet will incrementally improve quality, and when all packets are received, the quality is similar to H.265. 
Though they are better than classic SVC, they still impose a hierarchical structure over packets, which violates requirement {\em \RGraceful}---if a low-quality-layer packet of is missing, higher-quality-layer packets are not useful.\footnote{It should be clarified that SVC does achieve coding scalability with on-demand videos, which has enough buffer to allow packet retransmission.
%, where the sender usually makes sure one layer is fully received before sending the next one.
}

\jc{old text}
 (\eg as we will explain shortly, in scalable coding, data of lower coding layer is reliably received before fetching higher layers). 
With this assumption, RD-optimized coding can still greatly improve multicast service (\eg in multi-party video conferencing) and on-demand videos where different layers can be received one by one. 
Our paper aims at unicast real-time video communication with non-trivial network latency, so to reduce each frame's delay, most senders send packets of a frame as one batch.

\end{comment}

%one single lost packet of a lower layer will make all higher layers undecoded. 
%This violates requirement {\em (ii)} of DS coding.
%While the base (lowest-quality) layer of SVC is often padded with redundancy (\eg FEC, explained shortly)~\cite{wang2000error}, it does not protect other layers from packet losses.
%






\myparaq{Why not error correction coding (\eg FEC)}
The most common loss-resilient coding in real-time video is forward error correction (FEC).
% and its recent variants (\eg streaming code~\cite{??} and rateless fountain code~\cite{??}). 
%These redundancy-based schemes essentially trade coding efficiency for loss resilience. 
Given a target frame size RR, FEC encodes frames at N%⋅RN\%\cdot R, with the remaining (1−N%)⋅R(1-N\%)\cdot R used for redundancy. (1−N%)(1-N\%) is the {\em redundancy rate}.
The frame will be decodable, once {\em any} N%N\% of packets are received.
FEC differs from SVC in that SVC depends on {\em which data} is received, whereas FEC depends on {\em how much} data is received.

However, FEC-based schemes, including rateless coding~\cite{castura2006rateless} and streaming code~\cite{badr2017fec}, must know in advance how much data will arrive before the receiver decodes a frame; otherwise it will add either too much redundancy or still need to retransmit. 
% \footnote{\jc{some words on why rateless doesn't help here} \jc{also a parallel work tumbr has the same problem}} must know \rate~{\em before} sending the data; otherwise it will add either too much redundancy or still need to retransmit. 
%they work better only if \rate is known {\em before} FEC encodes the data. 
%must know \rate in advance to avoid packet retransmission and too much redundancy.
If redundancy is not enough to conceal missing packets in time (\ie~\rate is underestimated), some packets must be waited or retransmitted in order to decode the frame, which violates {\em \RDecodable} (\eg 10\% FEC in Figure~\ref{fig:comparison}).
Once the received packets are decodable, more packets will not improve the quality, which violates {\em \RGraceful}.
And if all packets are received (\ie~\rate is overestimated), the redundancy will lower the video quality, which violates {\em \REfficient} (\eg FEC 33\% with packet outcome \#1 in Figure~\ref{fig:comparison}).

%if much redundancy is added while all packets are received (\ie loss rate is overestimated), the decoded quality will be much lower than it could have been without redundancy (which violates {\em \REfficient}).

%\jc{include streaming code}




\myparaq{Why not redundant video coding}
%Source-coding-based schemes do not explicitly add redundancy like FEC. 
Besides FEC which adds redundancy to the video encoder output, the video coding itself can increase loss resilience.
% \footnote{In the video coding literature, the former (\eg FEC) refers to channel coding, while the latter refers to source coding.}.
% can be made more resilient to packet loss.
%Two examples are intra-MB insertion and reference selection, but both methods do not meet {\em \REfficient}, because they also add redundancy and have much lower quality if no packet turns out missing. 
%Intra-MB insertion~\cite{??} sets more macroblocks (MBs) in \texttt{INTRA} mode which makes their decoding not dependant on other frames, so missing one MB will affect fewer other MBs.
%However, doing so fails to exploit similar MBs across different frames, their quality will be lower than without intra-MB insertion at the same bitrate.
For instance, if we use an older but reliably received frame, instead of the last frame, as the reference frame, the decoder can safely skip a loss-affected frame (\eg~\cite{salsify}) without hurting subsequent frames.
However, this method also needs more bits to encode the same quality than using the last frame (which has a much smaller difference with the current from) as the reference frame
% , because the difference between two consecutive frames is much less than other history frames 
(\eg the P-frames between every other frames are 40\% greater in size than between two consecutive frames).

Without redundancy in coded data, one can still choose to skip a loss-affected frame, if skipping it does not affect future quality (\eg Voxel~\cite{voxel}). 
It works well for on-demand videos where (1) B-frames can be safely skipped, (2) the impact of a skipped frame will stop at the next chunk within a few seconds, and (3) the content is known in advance to profile the impact of skipping each frame on future frames. 
Unfortunately, none of them apply to real-time videos. %, in which B-frames are rarely used in and I-frames are used less often.



%\mypara{Receiver-side loss concealment}
\myparaq{Why not error concealment}
Error concealment by the video receiver has been intensively studied in multimedia. 
% Motion-vector recovery techniques, for instance, recover the motion vector (MV) of an MB~\cite{yihua?} by searching surrounding MBs whose MVs are not lost, and copying the one that causes least pixel differences (``glitches'')~\cite{??}. 
including recent work that uses neural networks (NN) to recover lost motion vectors (MVs) or use inpainting techniques to recover lost residuals~\cite{zhou2010efficient, xiang2019generative}. 
The key problem of these error concealment strategies is two-fold.
First, more macroblocks (MBs) need to be set in \texttt{INTRA} mode (independently decodable) and neighboring MBs should ideally be in different packets to facilitate recovery during packet losses.
However, all of these increase the frame size (\eg~30\% for four packets) and this inflation increases with more packets, since 
% in order for each packet to be decodable, but this greatly increases the frame size (\eg~\fillme\% for four packets) and this inflation increases with more packets.
they fail to leverage similarity among MBs---they do not meet {\em \REfficient}.
% , their quality will be lower than without intra-MB insertion at the same bitrate. 
% Like redundant video coding, this means they fall shorts on {\em \REfficient}.
Second, since the sender still uses a standard codec, there is minimum redundancy in the encoded MVs and residuals, and thus the MV recovery or inpainting tasks are inherently ``underspecified''.
% \footnote{This is why they often train the NN model per video~\cite{??,??,??}, but it is infeasible in real-time videos.}
As a result, their quality degrades quickly with higher \rates, which corroborates our results in \S\ref{sec:eval}.


In contrast, this work~{\em jointly} trains the NN encoder and NN decoder, allowing slight amount of redundancy in the coded data to facilitate error concealment by decoding.
%Moreover, its per-packet entropy encoding adds much less overhead than 


%In summary, none of the existing loss-resilient schemes achieve the goal of DS video coding. 
%We will also show preliminary results that quantitatively compare them with our proposal in later sections.


%can reconstruct lost motion vector (MV) of a macroblock (MB) by the MVs of surrounding MBs.
%For instance, one method to 

\begin{comment}

We empirically observe that such recovery is less effective than the NN-based coding proposed in this work.\jc{yihua, any pointer to an evidence?} to recover it and this may not always be effective (see \S\ref{??}).


Moreover, when the information of an MB is missing, they use handcrafted heuristics 

Receiver-side solution is to use image inpainting algorithms to restore a partially received frame. 
However, this is doable only {\em if} part of a frame can be decoded based on received data, which must rely on some other techniques mentioned earlier. 
For these reasons, they are not commonly used in real-time videos.



Alternatively, can also choose to skip a loss-affected frame, if skipping it does not affect future quality. 
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) B-frames can naturally be safely skipped, (2) the impact of a skipped frame will stop at next chunk (in a few seconds) when a new I-frame starts, and (3) the impact of skipping each frame on future frames can be pre-determined offline. 
Unfortunately, none of them is true for real-time videos, in which B-frames are rarely used in and I-frames are used less often.


\end{comment}



\begin{comment}
Reference selection uses an older frame already received by the receiver, instead of the last frame, as the reference to encode a new frame (\eg~\cite{salsify}), so any frame undecodable due to packet losses can be safely skipped without affecting future frames.
%setting its reference frame to some history frame that has been received by the receiver, rather than the last frame~\cite{salsify}. 
%This way, a frame that is undecodable due to packet losses can just be safely skipped without affecting future frames.

Both methods, however, do not meet {\em \REfficient}, because they use redundancy and have much lower quality if all packets are received. 
%In both cases, however, they have to sacrifice some compression efficiency if all packets are received, which violates {\em \REfficient}.
Intra-MB insertion fails to exploit similar MBs across different frames, their quality will be lower than without intra-MB insertion at the same bitrate.
%Like intra-MB insertion, 
Reference selection needs more bits to encode the same quality level, because the difference between two consecutive frames is much less than other history frames (\eg the P-frames between every other frames are \fillme\% greater in size than between two consecutive frames).

Both error-correction coding and redundant video coding must choose between compression efficiency (quality in absence of packet loss) and loss resilient (quality in presence of packet loss). 
For this reason, in practice, they are used {\em after} packet loss occurs---FEC is activated by WebRTC or the reference frame is changed by Salsify, only after the first packet loss is detected by the sender, which is at least one round-trip time after the packet loss occurs.
%Figure~\ref{fig:codec-dmr} shows an example of FEC. 
%The sender typically only adds redundancy {\em after} packet loss or delay increase affect a few frames, and when they may also add too much redundancy even after the \rate drops, resulting in low quality.

\end{comment}


\begin{comment}

reduce the inter-dependencies between macroblocks (MBs).
% that are potentially similar to each other. 
Intra-MB insertion, for instance, sets more MBs in \texttt{INTRA} mode, so that a lost MB will affect fewer other MBs.
%they are independently decodable, even if other MBs are lost.
However, because they do not leverage similarity across MBs, their quality will be much lower than without intra-MB insertion at the same bitrate which violates {\em \REfficient}.
%compression at the same bitrate is significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.
%and others that refer to them decodable, even if other data is lost.
%\footnote{Packet losses can also be tolerated by choosing a better reference frame to allow the receiver to skip undecodable frames without affecting subsequent frames, such as in Salsify~\cite{salsify}. These techniques can be used jointly with this proposal to select better quality reference frames.}
%Both intra-MB insertion and FEC must lower coding efficiency: FEC adds redundancy data and intra-MB insertion keeps more inter-macroblock redundancy.

Several other loss-resilient schemes exist that work without changing the video codecs, though they are less efficient than SVC, FEC at handling transient packet losses. 



\myparaq{Why not reference-frame selection} 
When encoding the next frame, the sender can set the reference frame to be a history frame that has been completely received by the receiver, rather than the last frame. 
This way, a frame that is undecodable due to packet losses can just be skipped without affecting future frames.
However, like intra-MB insertion, its quality will be much lower at the same bitrate than using the last frame as the reference, which violates {\em \REfficient}.
%its compression at the same bitrate will be significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.
An exception is Salsify~\cite{salsify}, which changes to a history frame (not the last one) as reference only {\em after} a loss is detected. 
As a result, however, it must skip several frames before encoding starts with a new reference frame.

\end{comment}


%requires techniques like intra-MB insertion are used, which has its own limitations as discussed earlier. For this reason, they are not commonly used in real-time videos.



\begin{comment}

The receiver can also choose to skip a frame depending on the frame's impact on future quality, but for frames whose absence will greatly affect the quality of other frames, this violates at least requirements of  $\RDecodable$ and $\RGraceful$.
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) the impact of a dropped frame will stop at next chunk (in a few seconds) which starts with a new I-frame, and (2) the impact of a skipped frame on future frames can be pre-determined offline. 
Unfortunately, both are not true for real-time videos.

\end{comment}


\begin{comment}

\myparaq{Why not selective frame dropping} 
Even if dropping a frame may affect future frames, the receiver can still choose to do that if the impact on the future frame's quality is relatively small.
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) the impact of a dropped frame will stop at the next chunk, which will start in a few seconds with a new i-frame, and (2) the impact of a skipped frame on future frames can be pre-determined offline. 
Unfortunately, both are not true for real-time videos. 


\myparaq{Why not computer vision-based error concealment}
Finally, image inpainting and super-resolution techniques could restore a partial frame. 
Unfortunately, this is doable only {\em if} part of a frame can be decoded based on received data.
This is usually not doable unless techniques like intra-MB insertion are used, which has its own limitations as discussed earlier. For this reason, they are not commonly used in real-time videos.
%different parts of a frame is encoded independently, which at the same bitrate will be significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.

\end{comment}


%\jc{is \name compatible with multi-party calls}


\begin{comment}



\myparaq{What's new in real-time video}
While this general workflow applies to most video streaming systems, real-time videos are distinctive in that they seek to reduce the {\em frame delay} between sending a frame and decoding it.
This profoundly affects their design choices in three ways.
%have three features distinct from others, which profoundly affect their designs. 
%short jitter buffer, no b frame, packets sent toghether, all of which have profound impact
\begin{packeditemize}
\item {\em Short jitter buffer:} First, real-time videos use a much shorter jitter buffer (just 1-2 frames or 10s of milliseconds) than even live broadcast videos, which have a buffer of at least a few seconds.
While increasing interactivity between clients, the short buffer makes the receiver potentially vulnerable to {\em any packet queuing or retransmit} that blocks the decoding of a frame after the short buffer is depleted. 


\item {\em Each frame sent in one batch:} Second, to reduce frame delay in long-latency networks, the sender often sends all packets of a frame in one burst, rather than multiple congestion windows.
%Thus loss and delaying can happen to any packets within the burst. 
This diminishes the benefit of layered coding (introduced shortly) which encodes a video in multiple layers and must deliver the layers in a specific order (see \S\ref{??}).


\item {\em Avoid B-frames:} Third, as each frame should be decoded as soon as its packets are received, B-frames are rarely used in real-time videos~\cite{??}, since they require future frames to be received. 
This precludes several loss-resilient techniques such as B-frame skipping (see \S\ref{??}).
\end{packeditemize}



\begin{itemize}
\item 2.1 Background
\begin{itemize}
\item basics: video, encoder, decoder, packets
\item real-time video: small jitter buffer, all packets must be sent together
\item concept of loss-resilient coding
\end{itemize}

\item 2.2 Ideal coding for real-time video
\begin{itemize}
\item given that 
\end{itemize}

\item 2.3 Limitations
\begin{itemize}
\item type 1: scalable coding
\item type 2: fec (rateless versions), reference selection, recover
\end{itemize}
\end{itemize}

We begin with why loss-resilient video coding is particularly important to real-time video and what an ideal scheme should achieve. 
We then explain the limitations of existing approaches.

Despite more bandwidth, many recent studies have shown that real-time video communication is plagued with intermittent packet loss and jitter~\cite{macmillan2021measuring,jansen2018performance,concerto,moulay2018experimental,latency-report-iab,latency-report-iab-2,latency-report-apnic}.
%induced by congestion, wireless, bufferbloat, etc.
\jc{yihua, can we find a few good pointers for this?}
%Adapting bitrate (ABR), which {\em reacts} to fluctuations of network conditions, is not enough to completely prevent packet loss, without using an extremely conservative bitrate. 
Since real-time video clients have very shallow jitter buffers, there is little time for packet retransmission before each frame should be decoded. 
So unlike in traditional streaming videos (which has a buffer of at least several seconds),
%Having shallow jitter buffers means that adapting bitrate or sending rate alone is not enough for clients to be immune to packet loss. 
%This leaves little time for packet retransmission, so 
{\em any} dropped or queued packets could delay the decoding of a frame, causing video stuttering and frame skipping in real-time video applications. 

%Having shallow jitter buffers also means that adapting bitrate or sending rate alone is not adequate to make real-time video client immune to packet loss.
%
%
%It is hard to predict how many packets will be dropped 
%Thus, the ability to decode a frame with a decent quality in presence of packet loss is crucial.




%\jc{Relationship with bitrate adaptation}

\end{comment}

==> sections/old/motivate_v9.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\tightsection{Motivation}
\label{sec:motivate}

Video coding has a rich history of research and it is hard to fit a comprehensive overview in a limited space.
Nonetheless, for those who are unfamiliar with this topic, it is beneficial to introduce the key concepts relevant to this paper (\S\ref{subsec:background}) before explaining the need for a different approach (\S\ref{subsec:ds},\ref{subsec:prior}). 


\tightsubsection{Background of video coding}
\label{subsec:background}

The video sender runs a rate adaptation logic to dynamically set the frame rate and bitrate of the encoded video.
%A video stream is encoded at certain frame rate and bitrate, both are controlled by an adaptation logic in the player.
With a frame rate of 25fps (frames per second) and bitrate of 3Mbps, for instance, the encoder should on average generate a 15KB frame every 40ms, though the actual frame size varies.
%depends on the {\em type} of a frame
A video stream consists of multiple groups of consecutive frames (called group of pictures or GoP), each starting with an I-frame (intra-frame) followed by P-frames (predicted frames) and B-frames (bidirectional predicted frames). 
I-frames are encoded independently (\ie they can be decoded without referring to other frames), so their sizes are often much bigger than P-frames, which only encode the differences between themselves and other {\em reference} frames.\footnote{On-demand videos also use B-frames, which 
% are smaller than P-frames since they 
refer to both past and future P-frames. However, real-time video rarely uses B-frames in order to render frames as soon as possible.
% However, to render frames as soon as possible, real-time video rarely uses B-frames~\cite{??}, since they refer to future frames to be decoded.
}

% Thus, I-frames are used infrequently (\eg only when content shifts dramatically) with 10s or more P-frames between two I-frames.

%and each GoP consists of 10s to 100s of P-frames. 
%I-frames are encoded independently, and P-frames and B-frames encode the differences between them and other {\em reference} frames: a P-frame refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames. 
%Importantly, to render each frame as soon as its packets are received, real-time videos almost never use B-frames which refer to future frames~\cite{??}. 
%Since I-frames do not need other frames to decode, their sizes in standard video codecs are much bigger than B-/P-frames, so I-frames are typically used only when content shifts dramatically and each GoP consists of 10s to 100s of frames. 

%As we will see in \Sref{??}, our new video coding system follows the same frame definitions, though the optimal GoP size will be much smaller. 


%Different {\em frame types} often have different frame sizes.
%An I-frame (intra-frames) is encoded independently and is followed by P-frames (predicted frames) and B-frames (bidirectional predicted frames), each of which encodes the differences between it and some other frames.
%A frame used as a reference for decoding other frames is called a {\em reference} frame: a P-frame only refers to the latest I-frames or P-frames, whereas a B-frame refers to both past and future P-frames.
%Since I-frames do not need other frames to decode, their sizes are typically bigger than B-/P-frames.


%In real-time videos, to render each frame as soon as its packets are received, B-frames, which refer to future frames, are rarely used~\cite{??}. 
%This precludes several loss-resilient techniques such as B-frame skipping (see \S??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{??}).

%, and  , each encoding the difference with the previous and future I-/P-frames.
%Thus, I-frames are typically bigger than P-frames and B-frames, but decoding I-frames does not depend on any other frame, while decoding P-frames or B-frames must refer to other frames. 
%fewer other frames than decoding a B-frame.


\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/fig2-workflow-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{A typical workflow of a video encoder.}
    \label{fig:codec-workflow}
\end{figure}

To encode a P-frame (Figure~\ref{fig:codec-workflow}), the encoder first calculates motion vectors (MVs) and residuals of each macroblock (MB, each of 4×4,8×8,\dots) in the current frame, then transforms and quantizes them to a more compact form, and finally, entropy encodes the data.
%To encode a frame, the encoder first calculates the differences (\eg motion vectors and residuals) among macroblocks (4×4,8×8,…4\times4,8\times8,\dots) in the current frame and reference frames (or within an I-frame),  then transforms and quantizes these differences to a more compact form, and finally losslessly encodes the data using arithmetic coding. 
The entropy-encoded data is then packetized and sent out by the transport layer, which tries to deliver as many packets as possible 
% (though not always all packets) 
to the receiver by the time when the frame is decoded.
%algorithm decides how fast to send a frame's packets, 
%in order to ensure enough data be delivered to the receiver when the frame is decoded. 
Similarly, the receiver depacketizes and decodes the received data to 
% runs a reverse process (depacketization and decoding) to 
reconstruct each frame from received packets. 
A decoded frame is put in a {\em buffer} before playing to conceal transient latency jitters. 
% (due to queuing or retransmits).

To reduce frame delay under long latency, real-time video clients make two common choices~\cite{10.1145/3410449,salsify}: %\footnote{\jc{any exceptions?}}:
% that affect the requirements of a desirable video coding scheme.
\begin{packeditemize}
\item Packets of a frame are sent in a burst (without waiting for acks), so %without waiting for acknowledgement.
{\em any} packets in the middle of a frame could be missing (delayed or dropped) when the receiver tries to decode the frame.
\item The jitter buffer is much {\em shorter} (\eg 10s~ms) than that of on-demand or live broadcast videos (whose buffer is at least a few seconds).
Thus, retransmission delay often cannot be concealed, particularly in long-latency networks.
% This short buffer often cannot conceal retransmission delay in long-latency networks.
%With a short buffer, any missing packet might delay a frame longer than the jitter buffer can conceal.
\end{packeditemize}
Therefore, loss resilience is vital for real-time video coding!

%real-time videos use  loss resilience of video coding is needed to ensure smooth and high-quality video in presence of packet loss.



 
%Loss-resilient video coding is particularly crucial in real-time videos.\footnote{\jc{clarify real-time video, conversational video, low-latency video}}
%This is because
%%Since packet loss might happen anytime, loss resilience of video coding is needed to maintain smoothness and high quality. 
%%Loss resilience is particularly important for real-time videos, because 
%to maintain high interactivity, real-time videos use a much shorter jitter buffer (just 1-2 frames or 10s~ms) than on-demand or live broadcast videos, whose buffers are likely at least a few seconds.
%With such a short buffer, {\em any packet queuing or retransmit} might block the decoding of a frame after the short buffer is depleted. 


%, which can be caused by either dropped packets or delayed packets.

%To capture the effect of dropped packets and delayed packets on decoding, 

\tightsubsection{\hspace{-0.2cm}Desirable loss-resilient coding for real-time videos}
\label{subsec:ds}

\mypara{Data-missing rate (\rate)}
We define data-missing rate (\rate) as the fraction of packets of a frame that have not arrived when the frame is decoded.
A missing packet can be due to queuing or retransmission.
%\footnote{\rate can be seen as deadline missing rate, if the deadline is when the decoder decides to decode a frame.}
High \rates arise from various reasons. 
For instance, a sudden bandwidth drop from 3Mbps to 500Kbps on a 200ms-RTT link can quickly raise \rate to 75\% and retransmission will delay or skip at least 6 frames in a 25fps video stream. 
Previous measurements have shown that 
%if frames are decoded with a fixed intervals (\eg every 40ms for a 25~fps video), 
transient high \rates (\eg $>30\%$) are not rare and are difficult to precisely predict in advance~\cite{macmillan2021measuring}. 
Note that our work does {\bf not} assume that high \rates are persistent in presence of a rate adaptation logic.

\mypara{Data-Scalable (DS) coding}
In a desirable video coding, which we refer to as {\em data-scalable} ({\em DS} for short) coding, quality should gracefully degrade in {\em presence} of more packet loss, without compromising the quality in {\em absence} of packet loss.
We breakdown this to three specific requirements:

\begin{packeditemize}
\item {\bf (\RDecodable)} 
The receiver can decode a frame if {\em any} non-empty subset of the packets of this frame is received---{\em minimum need for retransmission or frame skipping}.
%In real-time videos, the delay of a retransmit (at least a round-trip time) is sometimes longer than the jitter buffer (10s~ms), so any retransmit may cause a user-perceivable lag or skipped frames. 
%(\ie no retransmission or frame skipping unless no packet is received);

\item {\bf (\RGraceful)} 
%{\em Graceful degradation:} 
The quality should gradually improve with the addition of any received packet---{\em graceful degradation with higher \rates}.
%(\ie the decoded quality should gracefully degrades with higher \rates).

\item {\bf (\REfficient)} 
%{\em Compression efficiency:} 
If all packets are received, the decoded video will reach a quality close to that of a non-loss-resilient coding algorithm (such as H.265)---{\em high compression efficiency}.
%similar quality as the quality without redundancy (such as H.265), if all packets are received.

\end{packeditemize}




\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/fig2-dmr-newplaceholder.pdf}
         \label{fig:}
         \tightcaption{Illustrative example of the ideal data-scalable coding under dynamic data-missing rates (\rates).
%         \jc{maybe replace it with real values of autoencoder and FEC? }
         }
    \label{fig:codec-dmr}
\end{figure}

\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.97\linewidth]{figs/big-comparison-v2.pdf}
         \label{fig:}
         \tightcaption{Limitations of current loss-resilient solutions under three packet arrival patterns (no loss and one packet missing at different positions). \greencheck marks both high quality (encoding bitrate approximates the throughput) and low delay (no retransmission).}
    \label{fig:comparison}
\end{figure*}

Figure~\ref{fig:codec-dmr} illustrates the effect of DS coding in action. % in presence of bursts of high \rates.
% due to bandwidth fluctuations.
We assume that the bandwidth is mostly stable with intermittent high-\rate spikes caused by transient bandwidth drops and that the encoding bitrate matches the actual bandwidth.
As \rate varies over time, the quality of DS coding is high \rate is low (zero) and drops gracefully when \rate is high.

%To deliver each frame as quickly as possible, the sender often sends all packets of a frame in {\em one batch}. As a result, {\em any} packets might be missing. 






%in DS, quality grows with the number of {\em any} received packets, whereas in RD, the quality grows with consecutive packets in their sending order. 

%an RD-optimized sender sends packets in specific sending order and its quality grows with only received packets that are before the first missing packet in the sending order.

% assumes that packets are sent in order and packet loss only happens to the latter packets.
%DS is more realistic in real-time videos, because in long-latency networks, the sender should send all packets of a frame in one burst, and loss can happen to any packets, rather than just the last few packets (as shown in Figure~\ref{??}). 


%Second, to reduce frame delay in long-latency networks, the sender often sends all packets of a frame in one burst, rather than multiple congestion windows.
%%Thus loss and delaying can happen to any packets within the burst. 
%This diminishes the benefit of layered coding (introduced shortly) which encodes a video in multiple layers and must deliver the layers in a specific order (see \S\ref{??}).

\tightsubsection{Limitations of prior solutions}
\label{subsec:prior}

Next, we will explain why it is difficult to achieve DS coding using current loss-resilience schemes, including FEC, SVC, and error concealment.
% rate-distortion optimization
% and the difference between DS and other similar notions (\eg rate-distortion optimization).


%Next, we examine several representative loss-resilient coding schemes through the lens of the requirements of DS. 
%explain why they fall short of at least one of the three requirements of DS coding.

%Loss resilience has long been an important research topic. 
%Given the sheer amount of prior work in this space, we only highlight those that are most representative or closest to the goal of DS coding. % (see~\cite{??} for a complete survey).
%For ease of comparison, Figure~????????????\ref{fig:primitive-table}  shows how video quality varies with received data (packets) in different loss-resilient techniques. 

%these abstractions also influence the interaction with the remaining parts of a real-time video application, such as congestion control and bitrate adaptation.




\myparaq{Why not bitrate adaptation over TCP}
First, most streaming video systems today rely on congestion control and bitrate adaptation logics to {\em react} to bandwidth fluctuation and rely on \st{TCP to retransmit} \edit{retransmission to recover from} lost packets. 
They use highly efficient codec (\eg H265), so {\em if} all packets are received on time (\ie retransmission is fast enough), 
%the highly efficient codec (\eg H265) 
they will reach  a high quality with fewer bits. 
%This is well-suited for very low latency (with RTT of a few milliseconds) to allow fast retransmission.
However, it violates \RDecodable because these codecs are not inherently loss tolerant, so a frame cannot be decoded until all packets are received (\eg packet outcome \#2 and \#3 in Figure~\ref{fig:comparison}). 
%In real-time videos, retransmission delays can sometimes be longer than the jitter buffer (10s~ms), causing a visually perceivable lag or a skipped frame.

%re-sending a packet takes longer than the jitter buffer, this can also cause a visually perceivable lag or a skipped frame.

%Essentially, bitrate adaptation is {\em reactive}---if bandwidth suddenly drops, some frames will have already been affected by packet delays/drops before the sender/receiver lowers the bitrate.
%Without a proper loss-resilient scheme, it violates all three requirements of DS coding for real-time videos.

%---it lowers the encoding bitrate {\em after} a bandwidth drop is detected

%Packet retransmission is a conventional loss-resilient scheme. 

\begin{comment}
Frames are coded by a highly efficient codec (\eg H.265), and once all packets are received, the quality will be equal to the original encoded quality.
However, since these codecs optimize for compression, not loss resilience, any lost packets must be resent until all packets are reliably received, which violates {\em \RDecodable}.
If re-sending a packet takes longer than the jitter buffer, this can also cause a visually perceivable lag or a skipped frame.




\myparaq{Why not bitrate adaptation}
Bitrate adaptation lowers the target bitrate of {\em future} video chunks/frames {\em after} a bandwidth drop is detected. %, and then the video encoder will code the future video chunk or frame at the lowered target bitrate. 
Thus, bitrate adaptation is fundamentally {\em reactive}: 
when bandwidth suddenly drops, some frames have already experienced packet delays or drops before the sender/receiver can lower its target bitrate.
Given the short jitter buffer, this can directly hurt user experience, as in Figure~\ref{fig:trace}(a).
Without a proper loss-resilient scheme, it violates all three requirements of DS coding.

\end{comment}

\myparaq{Why not scalable video coding (SVC)}
SVC tries to optimize the classic notion of rate-distortion (RD) tradeoff, which which represents video quality achieved by a single encoded bitstream under different received bitrates and was studied intensively around 2000~\cite{schwarz2007overview, schierl2007mobile}.
SVC encodes a video at multiple quality layers and  sends data {\em layer by layer}, so that
%and if the packets are received in order, 
each newly received packet (or layer) will incrementally improve quality. % and when all packets are received, quality will be close to that of H.265. 
SVC-based techniques have made remarkable progress towards RD-optimized quality in on-demand video streaming, \eg fine-grained scalability (FSG)~\cite{li2001overview} and more recently, DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift}.


\begin{comment}
such that the decoder can reach the $i$-th quality layer, once the packets of $i$-th layer and lower layers are received, and the quality can be incrementally improved to the $(i+1)$-th layer, if the packets of the $(i+1)$-th layer are received.
%as long as the packets belong to the $i$-th layer and lower layers are received, we can obtain the quality of the $i$-th layer.
% and gradually improve quality with more received layers.
SVC-based techniques have made remarkable progress towards RD-optimized quality, especially in on-demand video streaming, \eg fine-grained scalability (FSG)~\cite{li2001overview} and more recently, DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift}.
Unlike TCP-based bitrate adaptation, an SVC sender sends data {\em layer by layer}, and 
%and if the packets are received in order, 
each newly received packet (or layer) will incrementally improve quality and when all packets are received, quality will be close to that of H.265. 
Thus, SVC can greatly benefit multicast videos which serve receivers that have heterogeneous network capacities~\cite{??}.
\end{comment}

However, SVC does not meet {\em \RGraceful}, because it imposes a hierarchical order among the packets of a frame; one missing packet can affect all higher quality layers, even if more packets are received in the higher quality layers (\eg packet outcome \#2 in Figure~\ref{fig:comparison}).
Though sending each layer reliably one by one is possible in on-demand videos~\cite{swift,grad}, real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{subsec:background}), so packet loss can affect any layer.
As a result, SVC is rarely used to improve unicast real-time video (though it is used widely by multicast videos to serve users with heterogeneous network capacities~\cite{schierl2007mobile}).
Essentially, DS coding differs from RD optimization on a key aspect---the quality of DS coding depends on {\em how many} packets, not {\em which} packets, are received.


\begin{comment}

There have been many SVC techniques---notably, fine-grained scalability (FSG)~\cite{li2001overview} and more recently, DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift} achieve near-optimal rate-distortion (RD) tradeoffs: if the packets are received in order, each newly received packet will incrementally improve quality and when all packets are received, quality will be close to that of H.265. 
%realize the following effect: if the packets are received in order, each new packet will incrementally improve quality, and when all packets are received, the quality is similar to H.265. 
Therefore, SVC can greatly benefit multicast videos as a way to serve receivers that have heterogeneous network capacities~\cite{??}.

However, SVC imposes a hierarchical order among packets that one missing packet can render all higher quality layers undecodable, even if more packets are received on higher quality layers~\cite{chen2006frame}; in other words, it violates {\em \RGraceful}.
Though sending each layer reliably one by one is possible in on-demand videos~\cite{swift,grad,etc}, real-time video clients send each frame as one burst to reduce frame delay (as explained in \S\ref{??}), so packet loss can affect any layer.
For this reason, SVC is not widely used to improve quality of unicast real-time video sessions~\cite{??}.


Note that DS is different from the classic notion of rate-distortion (RD) optimization, which was studied intensively around 2000~\cite{??,??}. 
%DS video coding may sound similar to the classic rate-distortion (RD) tradeoff, which was intensively studied around early 2000s~\cite{??,??}. 
RD optimizes video quality achieved by a single encoded bitstream under different received bitrates.
%, and ideally, with a single encoded bitstream, the decoding quality of the received data naturally increase if more data of the bitstream is received.
DS differs on a key aspect.
%The quality of DS coding grows with more received packets, regardless of their positions in the original sending order.
The quality of DS coding depends on {\em how many} packets, not {\em which} packets, are received.
In contrast, RD assumes that the packets have some dependencies and its quality increases with more packets received before the first missing packet in the original sending order. 
For instance, suppose that three packets are sent and the 2nd packet is the first missing packet. If the 3rd packet is received, then the quality of DS coding will grow but the quality of RD coding will not, since only one packet before the missing packet is received.
DS coding is more suitable for real-time videos, because as said earlier, senders of real-time videos burst packets of each frame, so loss can happen to any packets, rather than just the last packets.

\end{comment}


\begin{comment}

This makes sense in on-demand videos where different layers can be sent reliably one by one~\cite{??}.
In addition, 

However, SVC imposes a hierarchical order that one missing packet can render all higher quality layers undecodable, it violates requirement {\em \RGraceful}~\cite{chen2006frame}.
In unicast real-time video communication, however, senders often send all packets of a frame in {\em one batch}, rather than layer by layer, because the round-trip time is often higher than jitter buffer, 
As a result, {\em any} packets can be lost. 



with non-trivial network latency, so to reduce each frame's delay, most senders send packets of a frame as one batch.

SVC imposes a hierarchical order that one missing packet can render all higher quality layers undecodable, it violates requirement {\em \RGraceful}~\cite{chen2006frame}.
%\footnote{The classic SVC violates both requirement {\em (ii)} and {\em (iii)} of DS coding, though {\em (iii)} is mitigated by an autoencoder-based codec~\cite{swift} proposed recently.}
Even if the base (lowest) layer is padded with redundancy (\eg FEC, explained shortly)~\cite{SVCFEC1, schierl2007using,wang2000error}, it does not protect other layers from packet losses.\footnote{\jc{move this footnote to SVC later}The state-of-the-art solution, which is also based on neural-network autoencoders~\cite{swift}, can generate a single encoded bitstream to  {\em approximate} the optimal RD tradeoff, though still with a substantial margin.}

Other than SVC, there have been several other proposals that aim for finer-grained scalability.
Notably, fine-grained scalability (FSG)~\cite{li2001overview} and more recently DeepFSG~\cite{ma2022deepfgs} and Swift~\cite{swift} strive to realize the following effect: if the packets are received in order, each new packet will incrementally improve quality, and when all packets are received, the quality is similar to H.265. 
Though they are better than classic SVC, they still impose a hierarchical structure over packets, which violates requirement {\em \RGraceful}---if a low-quality-layer packet of is missing, higher-quality-layer packets are not useful.\footnote{It should be clarified that SVC does achieve coding scalability with on-demand videos, which has enough buffer to allow packet retransmission.
%, where the sender usually makes sure one layer is fully received before sending the next one.
}

\jc{old text}
 (\eg as we will explain shortly, in scalable coding, data of lower coding layer is reliably received before fetching higher layers). 
With this assumption, RD-optimized coding can still greatly improve multicast service (\eg in multi-party video conferencing) and on-demand videos where different layers can be received one by one. 
Our paper aims at unicast real-time video communication with non-trivial network latency, so to reduce each frame's delay, most senders send packets of a frame as one batch.

\end{comment}

%one single lost packet of a lower layer will make all higher layers undecoded. 
%This violates requirement {\em (ii)} of DS coding.
%While the base (lowest-quality) layer of SVC is often padded with redundancy (\eg FEC, explained shortly)~\cite{wang2000error}, it does not protect other layers from packet losses.
%






\myparaq{Why not error correction coding (\eg FEC)}
The most common loss-resilient coding in real-time video is forward error correction (FEC).
% and its recent variants (\eg streaming code~\cite{??} and rateless fountain code~\cite{??}). 
%These redundancy-based schemes essentially trade coding efficiency for loss resilience. 
Given a target frame size RR, FEC encodes frames at N%⋅RN\%\cdot R, with the remaining (1−N%)⋅R(1-N\%)\cdot R used for redundancy. (1−N%)(1-N\%) is the {\em redundancy rate}.
The frame will be decodable, once {\em any} N%N\% of packets are received.
FEC differs from SVC in that SVC depends on {\em which data} is received, whereas FEC depends on {\em how much} data is received.

However, FEC-based schemes, including rateless coding~\cite{castura2006rateless} and streaming code~\cite{badr2017fec}, must know in advance how much data will arrive before the receiver decodes a frame; otherwise it will add either too much redundancy or still need to retransmit. 
% \footnote{\jc{some words on why rateless doesn't help here} \jc{also a parallel work tumbr has the same problem}} must know \rate~{\em before} sending the data; otherwise it will add either too much redundancy or still need to retransmit. 
%they work better only if \rate is known {\em before} FEC encodes the data. 
%must know \rate in advance to avoid packet retransmission and too much redundancy.
If redundancy is not enough to conceal missing packets in time (\ie~\rate is underestimated), some packets must be waited or retransmitted in order to decode the frame, which violates {\em \RDecodable} (\eg 10\% FEC in Figure~\ref{fig:comparison}).
Once the received packets are decodable, more packets will not improve the quality, which violates {\em \RGraceful}.
And if all packets are received (\ie~\rate is overestimated), the redundancy will lower the video quality, which violates {\em \REfficient} (\eg FEC 33\% with packet outcome \#1 in Figure~\ref{fig:comparison}).

%if much redundancy is added while all packets are received (\ie loss rate is overestimated), the decoded quality will be much lower than it could have been without redundancy (which violates {\em \REfficient}).

%\jc{include streaming code}




\myparaq{Why not redundant video coding}
%Source-coding-based schemes do not explicitly add redundancy like FEC. 
Besides FEC which adds redundancy to the video encoder output, the video coding itself can increase loss resilience.
% \footnote{In the video coding literature, the former (\eg FEC) refers to channel coding, while the latter refers to source coding.}.
% can be made more resilient to packet loss.
%Two examples are intra-MB insertion and reference selection, but both methods do not meet {\em \REfficient}, because they also add redundancy and have much lower quality if no packet turns out missing. 
%Intra-MB insertion~\cite{??} sets more macroblocks (MBs) in \texttt{INTRA} mode which makes their decoding not dependant on other frames, so missing one MB will affect fewer other MBs.
%However, doing so fails to exploit similar MBs across different frames, their quality will be lower than without intra-MB insertion at the same bitrate.
For instance, if we use an older but reliably received frame, instead of the last frame, as the reference frame, the decoder can safely skip a loss-affected frame (\eg~\cite{salsify}) without hurting subsequent frames.
However, this method also needs more bits to encode the same quality than using the last frame (which has a much smaller difference with the current from) as the reference frame
% , because the difference between two consecutive frames is much less than other history frames 
(\eg the P-frames between every other frames are 40\% greater in size than between two consecutive frames).

Without redundancy in coded data, one can still choose to skip a loss-affected frame, if skipping it does not affect future quality (\eg Voxel~\cite{voxel}). 
It works well for on-demand videos where (1) B-frames can be safely skipped, (2) the impact of a skipped frame will stop at the next chunk within a few seconds, and (3) the content is known in advance to profile the impact of skipping each frame on future frames. 
Unfortunately, none of them apply to real-time videos. %, in which B-frames are rarely used in and I-frames are used less often.



%\mypara{Receiver-side loss concealment}
\myparaq{Why not error concealment}
Error concealment by the video receiver has been intensively studied in multimedia. 
% Motion-vector recovery techniques, for instance, recover the motion vector (MV) of an MB~\cite{yihua?} by searching surrounding MBs whose MVs are not lost, and copying the one that causes least pixel differences (``glitches'')~\cite{??}. 
including recent work that uses neural networks (NN) to recover lost motion vectors (MVs) or use inpainting techniques to recover lost residuals~\cite{zhou2010efficient, xiang2019generative}. 
The key problem of these error concealment strategies is two-fold.
First, more macroblocks (MBs) need to be set in \texttt{INTRA} mode (independently decodable) and neighboring MBs should ideally be in different packets to facilitate recovery during packet losses.
However, all of these increase the frame size (\eg~30\% for four packets) and this inflation increases with more packets, since 
% in order for each packet to be decodable, but this greatly increases the frame size (\eg~\fillme\% for four packets) and this inflation increases with more packets.
they fail to leverage similarity among MBs---they do not meet {\em \REfficient}.
% , their quality will be lower than without intra-MB insertion at the same bitrate. 
% Like redundant video coding, this means they fall shorts on {\em \REfficient}.
Second, since the sender still uses a standard codec, there is minimum redundancy in the encoded MVs and residuals, and thus the MV recovery or inpainting tasks are inherently ``underspecified''.
% \footnote{This is why they often train the NN model per video~\cite{??,??,??}, but it is infeasible in real-time videos.}
As a result, their quality degrades quickly with higher \rates, which corroborates our results in \S\ref{sec:eval}.

\yihua{update a paragraph about sr here -- need to iterate}
\myparaq{Why not super-resolution (SR)}
Previous works have employed the super-resolution (SR) technique to enhance video quality in low-bandwidth conditions for on-demand and live video streaming~\cite{??, ??, ??}. However, SR does not fulfill the requirements of data-scalable coding; it fails if the base frame is incomplete or undecodable, contravening \RDecodable and \RGraceful.
SR can potentially enhance real-time video quality in two ways: {\em (i)} directly improving decoded video quality, and {\em (ii)} preserving quality while transmitting less data, thereby averting possible network congestion or allocating more bandwidth for additional redundancy.
However, approach {\em (i)} is codec-agnostic and hence unrelated to the design space of DS codecs. Approach {\em (ii)} is also non-data-scalable; if the transmission bitrate is excessively low, quality will deteriorate, and if the bitrate is set higher to preserve quality, network congestion cannot be completely mitigated.

In contrast, this work~{\em jointly} trains the NN encoder and NN decoder, allowing slight amount of redundancy in the coded data to facilitate error concealment by decoding.
%Moreover, its per-packet entropy encoding adds much less overhead than 


%In summary, none of the existing loss-resilient schemes achieve the goal of DS video coding. 
%We will also show preliminary results that quantitatively compare them with our proposal in later sections.


%can reconstruct lost motion vector (MV) of a macroblock (MB) by the MVs of surrounding MBs.
%For instance, one method to 

\begin{comment}

We empirically observe that such recovery is less effective than the NN-based coding proposed in this work.\jc{yihua, any pointer to an evidence?} to recover it and this may not always be effective (see \S\ref{??}).


Moreover, when the information of an MB is missing, they use handcrafted heuristics 

Receiver-side solution is to use image inpainting algorithms to restore a partially received frame. 
However, this is doable only {\em if} part of a frame can be decoded based on received data, which must rely on some other techniques mentioned earlier. 
For these reasons, they are not commonly used in real-time videos.



Alternatively, can also choose to skip a loss-affected frame, if skipping it does not affect future quality. 
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) B-frames can naturally be safely skipped, (2) the impact of a skipped frame will stop at next chunk (in a few seconds) when a new I-frame starts, and (3) the impact of skipping each frame on future frames can be pre-determined offline. 
Unfortunately, none of them is true for real-time videos, in which B-frames are rarely used in and I-frames are used less often.


\end{comment}



\begin{comment}
Reference selection uses an older frame already received by the receiver, instead of the last frame, as the reference to encode a new frame (\eg~\cite{salsify}), so any frame undecodable due to packet losses can be safely skipped without affecting future frames.
%setting its reference frame to some history frame that has been received by the receiver, rather than the last frame~\cite{salsify}. 
%This way, a frame that is undecodable due to packet losses can just be safely skipped without affecting future frames.

Both methods, however, do not meet {\em \REfficient}, because they use redundancy and have much lower quality if all packets are received. 
%In both cases, however, they have to sacrifice some compression efficiency if all packets are received, which violates {\em \REfficient}.
Intra-MB insertion fails to exploit similar MBs across different frames, their quality will be lower than without intra-MB insertion at the same bitrate.
%Like intra-MB insertion, 
Reference selection needs more bits to encode the same quality level, because the difference between two consecutive frames is much less than other history frames (\eg the P-frames between every other frames are \fillme\% greater in size than between two consecutive frames).

Both error-correction coding and redundant video coding must choose between compression efficiency (quality in absence of packet loss) and loss resilient (quality in presence of packet loss). 
For this reason, in practice, they are used {\em after} packet loss occurs---FEC is activated by WebRTC or the reference frame is changed by Salsify, only after the first packet loss is detected by the sender, which is at least one round-trip time after the packet loss occurs.
%Figure~\ref{fig:codec-dmr} shows an example of FEC. 
%The sender typically only adds redundancy {\em after} packet loss or delay increase affect a few frames, and when they may also add too much redundancy even after the \rate drops, resulting in low quality.

\end{comment}


\begin{comment}

reduce the inter-dependencies between macroblocks (MBs).
% that are potentially similar to each other. 
Intra-MB insertion, for instance, sets more MBs in \texttt{INTRA} mode, so that a lost MB will affect fewer other MBs.
%they are independently decodable, even if other MBs are lost.
However, because they do not leverage similarity across MBs, their quality will be much lower than without intra-MB insertion at the same bitrate which violates {\em \REfficient}.
%compression at the same bitrate is significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.
%and others that refer to them decodable, even if other data is lost.
%\footnote{Packet losses can also be tolerated by choosing a better reference frame to allow the receiver to skip undecodable frames without affecting subsequent frames, such as in Salsify~\cite{salsify}. These techniques can be used jointly with this proposal to select better quality reference frames.}
%Both intra-MB insertion and FEC must lower coding efficiency: FEC adds redundancy data and intra-MB insertion keeps more inter-macroblock redundancy.

Several other loss-resilient schemes exist that work without changing the video codecs, though they are less efficient than SVC, FEC at handling transient packet losses. 



\myparaq{Why not reference-frame selection} 
When encoding the next frame, the sender can set the reference frame to be a history frame that has been completely received by the receiver, rather than the last frame. 
This way, a frame that is undecodable due to packet losses can just be skipped without affecting future frames.
However, like intra-MB insertion, its quality will be much lower at the same bitrate than using the last frame as the reference, which violates {\em \REfficient}.
%its compression at the same bitrate will be significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.
An exception is Salsify~\cite{salsify}, which changes to a history frame (not the last one) as reference only {\em after} a loss is detected. 
As a result, however, it must skip several frames before encoding starts with a new reference frame.

\end{comment}


%requires techniques like intra-MB insertion are used, which has its own limitations as discussed earlier. For this reason, they are not commonly used in real-time videos.



\begin{comment}

The receiver can also choose to skip a frame depending on the frame's impact on future quality, but for frames whose absence will greatly affect the quality of other frames, this violates at least requirements of  $\RDecodable$ and $\RGraceful$.
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) the impact of a dropped frame will stop at next chunk (in a few seconds) which starts with a new I-frame, and (2) the impact of a skipped frame on future frames can be pre-determined offline. 
Unfortunately, both are not true for real-time videos.

\end{comment}


\begin{comment}

\myparaq{Why not selective frame dropping} 
Even if dropping a frame may affect future frames, the receiver can still choose to do that if the impact on the future frame's quality is relatively small.
It may work well for on-demand chunk-based videos (\eg Voxel~\cite{palmer2021voxel}), because (1) the impact of a dropped frame will stop at the next chunk, which will start in a few seconds with a new i-frame, and (2) the impact of a skipped frame on future frames can be pre-determined offline. 
Unfortunately, both are not true for real-time videos. 


\myparaq{Why not computer vision-based error concealment}
Finally, image inpainting and super-resolution techniques could restore a partial frame. 
Unfortunately, this is doable only {\em if} part of a frame can be decoded based on received data.
This is usually not doable unless techniques like intra-MB insertion are used, which has its own limitations as discussed earlier. For this reason, they are not commonly used in real-time videos.
%different parts of a frame is encoded independently, which at the same bitrate will be significantly less efficient (\ie much lower quality when all packets are received), compared to using the last frame as reference, which violates {\em (iii)}.

\end{comment}


%\jc{is \name compatible with multi-party calls}


\begin{comment}



\myparaq{What's new in real-time video}
While this general workflow applies to most video streaming systems, real-time videos are distinctive in that they seek to reduce the {\em frame delay} between sending a frame and decoding it.
This profoundly affects their design choices in three ways.
%have three features distinct from others, which profoundly affect their designs. 
%short jitter buffer, no b frame, packets sent toghether, all of which have profound impact
\begin{packeditemize}
\item {\em Short jitter buffer:} First, real-time videos use a much shorter jitter buffer (just 1-2 frames or 10s of milliseconds) than even live broadcast videos, which have a buffer of at least a few seconds.
While increasing interactivity between clients, the short buffer makes the receiver potentially vulnerable to {\em any packet queuing or retransmit} that blocks the decoding of a frame after the short buffer is depleted. 


\item {\em Each frame sent in one batch:} Second, to reduce frame delay in long-latency networks, the sender often sends all packets of a frame in one burst, rather than multiple congestion windows.
%Thus loss and delaying can happen to any packets within the burst. 
This diminishes the benefit of layered coding (introduced shortly) which encodes a video in multiple layers and must deliver the layers in a specific order (see \S\ref{??}).


\item {\em Avoid B-frames:} Third, as each frame should be decoded as soon as its packets are received, B-frames are rarely used in real-time videos~\cite{??}, since they require future frames to be received. 
This precludes several loss-resilient techniques such as B-frame skipping (see \S\ref{??}).
\end{packeditemize}



\begin{itemize}
\item 2.1 Background
\begin{itemize}
\item basics: video, encoder, decoder, packets
\item real-time video: small jitter buffer, all packets must be sent together
\item concept of loss-resilient coding
\end{itemize}

\item 2.2 Ideal coding for real-time video
\begin{itemize}
\item given that 
\end{itemize}

\item 2.3 Limitations
\begin{itemize}
\item type 1: scalable coding
\item type 2: fec (rateless versions), reference selection, recover
\end{itemize}
\end{itemize}

We begin with why loss-resilient video coding is particularly important to real-time video and what an ideal scheme should achieve. 
We then explain the limitations of existing approaches.

Despite more bandwidth, many recent studies have shown that real-time video communication is plagued with intermittent packet loss and jitter~\cite{macmillan2021measuring,jansen2018performance,concerto,moulay2018experimental,latency-report-iab,latency-report-iab-2,latency-report-apnic}.
%induced by congestion, wireless, bufferbloat, etc.
\jc{yihua, can we find a few good pointers for this?}
%Adapting bitrate (ABR), which {\em reacts} to fluctuations of network conditions, is not enough to completely prevent packet loss, without using an extremely conservative bitrate. 
Since real-time video clients have very shallow jitter buffers, there is little time for packet retransmission before each frame should be decoded. 
So unlike in traditional streaming videos (which has a buffer of at least several seconds),
%Having shallow jitter buffers means that adapting bitrate or sending rate alone is not enough for clients to be immune to packet loss. 
%This leaves little time for packet retransmission, so 
{\em any} dropped or queued packets could delay the decoding of a frame, causing video stuttering and frame skipping in real-time video applications. 

%Having shallow jitter buffers also means that adapting bitrate or sending rate alone is not adequate to make real-time video client immune to packet loss.
%
%
%It is hard to predict how many packets will be dropped 
%Thus, the ability to decode a frame with a decent quality in presence of packet loss is crucial.




%\jc{Relationship with bitrate adaptation}

\end{comment}

==> sections/old/motivation.tex <==
\tightsection{Motivation}

\tightsubsection{Architecture of real-time video conferencing systems}

Propose a model to describe the system. (Video -> encoding algorithm -> packets -> lossy network -> packets' -> decoding algorithm -> reconstructed video)

\tightsubsection{Impact of packet losses}

Some measurements and experiments to show that
\begin{itemize}
    \item packet loss is unavoidable and unpredictable
    \item current hand-crafted methods cannot perform well: RTX-based method cause huge delay. Loss recovery mechanisms may have big quality degradation under some scenarios.
\end{itemize}

\tightsubsection{Goal of our design}
Have a graceful quality without retransmission under packet losses.

==> sections/old/overview.tex <==
\tightsection{Autoencoder: A learning-based solution}
To achieve the goals proposed above, we consider the autoencoder, a learning based approach for codecs. In this sections, we ...

\tightsubsection{What to learn}
\begin{itemize}
    \item An autoencoder which still delivers decent quality under packet losses
\end{itemize}

\tightsubsection{Why learning}

\begin{itemize}
    \item During training, autoencoder can see various loss patterns from the data. Therefore, it has a better potential to deal with varying loss rates.
    \item Autoencoders can automatically learn which part of data is more critical to the quality in an end-to-end manner. 
    \item ...
\end{itemize}

\tightsubsection{How to learn}
Present an overview of our training process -- how to train with loss.

==> sections/old/protocol-nsdi-v1.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US





\tightsection{Real-time video framework}
\label{sec:delivery}

%\jc{
%\begin{itemize}
%\item coding of i-frames (compression)
%\item bitrate control (speed)
%\item speedup on cpu (speed)
%\item end-to-end protocol (why no synchronization, interaction with tcp and abr) (resilience)
%\end{itemize}
%}

%\jc{a table mapping the techniques to effects
%\begin{itemize}
%\item compression: i-frames, per-packet entropy
%\item speed: bitrate control, cpu speedup
%\item resilience: retraining, end-to-end protocol
%\end{itemize}
%}

With the training techniques proposed in \S\ref{sec:core}, \name's NVC is highly resilient to simulated packet losses.
This section presents how to use such NVC in a real-time video delivery framework. 
In particular,
\begin{packeditemize}
\item How to entropy encode NVC encoder's output into packets (\S\ref{subsec:packetization}), 
\item How to stream a sequence of frames (\S\ref{subsec:protocol}), and
\item How to speed up encoding/decoding on resource-constrained devices without sacrificing loss resilience (\S\ref{subsec:fast-coding}).
\end{packeditemize}
% \yc{I moved entropy coding to 4.1, since I feel this is more smooth: first talking about tensor -> packets for each frame, then discuss how we stream sequence of frames, finally some optimizations}

\tightsubsection{Entropy encoding the encoder's output}\label{subsec:packetization}
As mentioned in \S\ref{sec:core}, \name randomly splits the encoder's output into subtensors, and each subtensor corresponds to an individual packet.
Like classic codecs of H.264 and VP9, each subtensor also needs to be losslessly compressed into a bitstream using an arithmetic (entropy) coding scheme.
An arithmetic encoder uses an underlying symbol distribution to compress the value at each position of the tensor.
Unlike classic codecs that use hand-tuned heuristics like CABAC, neural video codecs, including DVC, often train a distribution estimator jointly with the NN encoder and decoder to have a better distributional representation of the values in the encoder output. 
Since the decoder later uses the same symbol distributions to decode the bitstream, the symbol distribution is also sent together within the packet. 
However, putting such distribution in each packet incurs an overhead, and may greatly inflate the packet size if the data of a frame is split into many packets. 
%However, because \name divides the encoder's output tensor into subtensors, each being separately entropy encoded into a packet, thus each packet must include a copy of its own symbol distribution.
%This will greatly increase the size if the data of a frame is split into many packets. 

We reduce this per-packet overhead by carefully choosing the precision of symbol distribution, which governs the tradeoff between the size of a symbol distribution and the size of the entropy-encoded data.
A coarser-grained symbol distribution needs fewer bits to store, but it may yield a higher size of the entropy-encoded data. 
\name's insight is that we can train the NN encoder in a way that regularizes the distribution of values in each encoder's output channel\footnote{Each encoder output tensor has 224 channels} to conform to a zero-mean Laplace distribution.
This way, the symbol distribution only needs to store the variance within each channel while still perfectly compressing the encoder output tensor. 
As a result, the symbol distribution takes only $\sim$50 bytes to store per packet (a reduction from 40\% of the packet size to 5\%), without hurting the compression efficiency of entropy coding.


\tightsubsection{Streaming protocol}
\label{subsec:protocol}

%\jc{this subsection is a bit too long. tighten it please.}

% To extend the P-frame DS autoencoder trained in \S\ref{subsec:training} for multiple frames, the first challenge is potential out-of-sync {\em states} between the encoder and decoder when packet loss occurs.
%Two challenges arise when extending the P-frame DS autoencoder trained in \S\ref{subsec:??} to the delivery of multiple frames: (1) potential out-of-sync coding state between the encoder and decoder when packet loss occurs, and (2) how to encode I-frames and how frequently to add I-frames.



\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v3.pdf}
        % \includegraphics[width=0.99\linewidth]{figs/state-sync-v2.pdf}
        \includegraphics[width=0.92\linewidth]{figs/state-sync-v3.pdf}
    \tightcaption{Examples of how to deal with loss-affected frames: 
    (a) delayed by retransmission, (b) ignoring out-of-sync encoder/decoder states, and (c) 
    \name's frame optimistic encoding and state re-sync.}
    \label{fig:state-sync}
    \vspace{-0.1cm}
\end{figure}



\mypara{Basic protocol of \name}
%When any packet of the next frame is received by the decoder, the decoder will try to decode the current frame based 
The encoder encodes a new frame with a fixed interval, and % (by default, 40ms or 25fps).
when any packet of the next frame is received, the decoder will decode the current frame using the neural decoder, if at least one packet of the current frame is received.
If no packet of the current frame is received, then it will request the sender to send the frame again.
%\begin{packeditemize}
%If no packet of the current frame is received, then it will request the sender to send the frame again;
%If at least one packet of the current frame is received, then it will decode the frame.
%\item If a subset of the packets of the current frame are received, then it will decode the frame and send a ``re-sync'' signal to the sender.
%\end{packeditemize}

%\mypara{Encoding reference state}
%However, if we directly replace the traditional codec with the new autoencoder, it could cause low quality on a frame even if all of its packets arrive on time. 
However, this basic protocol can degrade quality even on frames where all packets arrive on time. 
This is because if a reference frame is decoded using a subset of packets, the encoder/decoder state will be ``out-of-sync''---the encoding of the next frame will use a different reference image than its decoding.
%---the reference image used to encode the next frame is different from the reference used by the decoder to decode the next frame.
% This can affect all subsequent frames if not handled appropriately.
% Figure~\ref{fig:state-sync} shows an example. 
%In standard video coding, 
For instance, to encode the $7^{\textrm{th}}$ frame, the sender uses the decoded $6^{\textrm{th}}$ frame as the reference to encode the $7^{\textrm{th}}$ frame, so that the receiver can decode the $7^{\textrm{th}}$ frame using the same reference. 
%To encode the $7^{\textrm{th}}$ frame, the sender uses the decoded result of the $6^{\textrm{th}}$ frame as the reference to encode the $7^{\textrm{th}}$ frame, and the receiver will use the same reference to decode the $7^{\textrm{th}}$ frame. 
However, when \name's decoder decodes the $6^{\textrm{th}}$ frame based on a subset of its packets (Figure~\ref{fig:state-sync}(a)), it will be a different image than the reference image used by encoder to encode the $7^{\textrm{th}}$ frame. 
As a result, the $7^{\textrm{th}}$ frame will have slightly lower quality even if all of its packets are received, because its encoding uses a different image than its decoding. 
% it will see a different reference when decoding the $7^{\textrm{th}}$ frame than what the encoder has assumed when encoding the $7^{\textrm{th}}$ frame.
%Thus, even if all packets of the $7^{\textrm{th}}$ are received, its quality will be slightly lower than it should be.
Similarly, since the $7^{\textrm{th}}$ is also out of sync with the sender's state, the $8^{\textrm{th}}$ frame will suffer too, and so forth.
%In short, the quality of many frames with zero \rate might still be affected.

%the naive method of using \name (Figure~\ref{fig:state-sync}(b)) will affect quality degradation on frames that do not have 

%the reference frame used by the receiver to decode the 10th10^{\textrm{th}} frame will differ from what the encoder has assumed. 
%
%, and without knowing which of the 9th9^{\textrm{th}} frame's packets will be lost, it will assume that the 9th9^{\textrm{th}} frame is decoded with all packets being received. (This is common to classic codecs and autoencoders.)
%However, if the receiver decodes the 9th9^{\textrm{th}} frame with only a subset of its packets, the actual reference frame used to decode the 10th10^{\textrm{th}} will differ from what the encoder has assumed. 
%Thus, most codecs require all packets of the 9th9^{\textrm{th}} frame to be received before decoding it (thus longer delay), or let the sender encode the 10th10^{\textrm{th}} based on an earlier reference (say the 5th5^{\textrm{th}}) whose lost packets are already known to the sender. 
%The latter {\em synchronizes} the encoding and decoding states (like in Salsify~\cite{salsify} during packet losses), but it also inflates the frame size, since the difference between the 10th10^{\textrm{th}} and the 5th5^{\textrm{th}} frames  is much greater than between the 10th10^{\textrm{th}} and the 9th9^{\textrm{th}} frames. 


%\begin{figure*}[t!]
%    \centering
%         \centering
%%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v3.pdf}
%        \includegraphics[width=0.9\linewidth]{figs/state-sync-v1.pdf}
%    \tightcaption{}
%    \label{fig:per-packet}
%\end{figure*}


A strawman is that the encoder and decoder synchronize on each frame.
% ---if the receiver decodes a frame with a subset of packets, the sender should always know which packets are used in order to reconstruct the same reference frame seen by the decoder. 
However, this will negate the benefit of \name's generative autoencoder, as the sender will wait until the receiver acknowledges after each frame, taking at least an RTT.
% for the acknowledgment from the receiver (at least an RTT) after each frame, 

\mypara{Optimistic encoding with dynamic state re-sync}
%Rather than syncing-up the reference state every frame, 
Instead, \name's sender (and decoder) optimistically encode (and decode) frames without syncing the coding states.
However, when a frame is decoded using a subset of packets, the receiver will not stop, but it also notifies the sender which packets have been used to decode recent frames. 
On receiving this feedback, the sender will quickly 
%However, once receiving the feedback that the decoder decodes a frame using a subset of its packets, the sender will quickly 
re-decode the recent frames with the same decoded frame as seen by the decoder to reconstruct the same reference frame seen by the decoder. 
%As explained shortly, such re-decoding can be greatly sped-up.
For instance, in Figure~\ref{fig:state-sync}(b), the sender is about to encode the $9^{\textrm{th}}$ when it gets the feedback that says the $6^{\textrm{th}}$ was decoded with a certain subset of packets, then the encoder will quickly re-decode the frames from the $6^{\textrm{th}}$ (with the same subset of packets) to $8^{\textrm{th}}$ frames and use the new decoded $8^{\textrm{th}}$ frame as the reference to encode the $9^{\textrm{th}}$ frame.




%\name's autoencoder can decode frames with inconsistent coding states for a handful of frames, though the quality will deteriorate over time if the coding state is left unsynced for too long. \jc{need a visualization in eval}
%However, our fast re-sync scheme makes sure that 

%The basic insight is that without synchronizing the reference frames, \name's autoencoder can decode frames with high quality for a handful of frames. \jc{need a visualization here}
%
%Therefore, the sender does not need to wait for the feedback from the receiver; instead, it can optimistically encode the next frame assuming the packets of the previous frames are completely received, until it receives a feedback from the receiver that a previous frame was not decoded with all packets (this feedback can be like an NACK in WebRTC).
%Suppose that the sender is about to encode the $9^{\textrm{th}}$ when it gets a feedback that says the $6^{\textrm{th}}$ was decoded with certain subset of packets (illustrated in Figure~\ref{fig:state-sync}(c)), then the encoder will quickly re-decode the frames from the $6^{\textrm{th}}$ to $8^{\textrm{th}}$ frames (this step can be greatly sped-up shortly), and use the new decoded $8^{\textrm{th}}$ frame as the reference to encode the $9^{\textrm{th}}$ frame.



A potential speed bottleneck is re-decoding reference frames (\eg from $6^{\textrm{th}}$ to $8^{\textrm{th}}$ frames in Figure~\ref{fig:state-sync}(c)) during re-sync. 
Fortunately, both the encoder and the decoder can re-decode these frames much faster than the normal decoding, by skipping both motion-estimation NN and the frame-prediction NN (Figure~\ref{fig:dvc-arch}).
This saves 93\% of encoding time per frame.
The insight is two-fold.
First, these frames have been decoded once, and the re-decoding simply needs to estimate the incremental changes caused by the lost packets, so it can be much faster. 
Second, skipping the frame-prediction NN does reduce the compression efficiency on the last frame (\eg the $9^{\textrm{th}}$ frame in  Figure~\ref{fig:state-sync}(c)), but it only affects only one frame.
The formal proof of why the re-decoding works can be found in \S\ref{app:resync}.%\jc{YIHUA!}

% re-synchronization does not have to have the highest quality, which allows us to skip the motion-smoothing NN in frame prediction. In addition, this is also a unique benefit of autoencoders.
% The formal proof can be found in \S\ref{??}.

\tempstrike{
    
% \footnote{\edit{The motion smoothing NN is trained to smooth the predicted frame, so that the residual will be smaller and thus easier to compress.}} 
% in the frame prediction \st{NN} \edit{step} (shown in Figure~\ref{fig:dvc-arch}), 
which takes up \fillme\% of the decoding time per frame. 
The new $8^{\textrm{th}}$ frame will be used to encode the $9^{\textrm{th}}$ frame in  Figure~\ref{fig:state-sync}(c), and when the receiver receives the encoded $9^{\textrm{th}}$ frame, it also re-decodes the frames from 6-8 {\em without} the \edit{motion-smoothing NN}.
% \st{frame prediction NN} (not shown in figure), 
Since both re-encoding and re-decoding skip the time-consuming motion-smoothing NN, the overhead is minimum 
but since this is much faster, it will not add much new overhead. 
The insight behind it is that re-synchronization does not have to have the highest quality, which allows us to skip the motion-smoothing NN in frame prediction. In addition, this is also a unique benefit of autoencoders.
%which is unique to the benefit of autoencoders

}

%allowing it to re-decode these frames using a different but faster method.
%The insight is that the decoding does not have to have the highest quality, which allows us to skip the motion-smoothing NN in motion compensation (Figure~\ref{??}) which significantly reduces the delay by \fillme\%.\jc{need a few words on why}
%For this optimization to work, the receiver also needs to re-decode the frames from 6-8 without the motion-smoothing NN, but since this is much faster, it will not add much new overhead. 

    

%, but it leverages the loss resilience of the new autoencoders.
% Like \name, NACK and Salsify allow senders to burst packets without waiting for acks, and when packet loss happens, NACK retransmits lost packets which delays the decoding of future frames and Salsify rewinds the encoder to an old state to generate the next P-frame, allowing the decoder to skip loss-affected frames.
% However, \name's key difference is that 

The dynamic state re-sync described above highlights a key advantage of \name's decoder---it does not need to skip or block the decoding of loss-affected frames; instead, it still decodes loss-affected frames with decent quality {\em before} encoder/decoder states are synchronized, so it reduces frame delay while maintaining decent quality. 
% This makes \name's optimistic encoding with dynamic state re-sync 
This is fundamentally different from  NACK (negative ack) in WebRTC (which blocks the decoding of loss-affected frames) and the encoder/decoder state synchronization in Salsify (which skips the loss-affected frames).
% , where the latter methods need to either wait for or skip the loss affected frames.

%Although \name's optimistic encoding with dynamic state re-sync may sound similar to NACK (negative ack) in WebRTC and the encoder/decoder state synchronization in Salsify, but it has a key difference. 
%The receiver in \name does not need to skip or block the decoding of loss-affected frames; instead can still decode loss-affected frames with decent quality before encoder/decoder states are synchronized, so it reduces frame delay while maintaining high quality. 
\passed{\amz{This is also framed in a roundabout way, but is also a key insight of this work IMO -- using your packetization allows for decoding lossy frames with less delay. Switching these sentences ("Another benefit of \name is that the receiver does not need to skip... This differentiates our dynamic state re-sync from NACK and Salsify")} \yc{reorganized the contents}}
%wait for the retransmission (in NACK) or the new P-frame (in Salsify) to decode the next frame frame; instead, it can still decode loss-affected frames with decent quality before encoder/decoder states are synchronized, so it reduces frame delay while maintaining high quality.


%Like NACK (negative ack) which WebRTC senders use to burst packets without waiting for acks until an NACK is received, 
%% from the receiver that some packets must be retransmitted in order to decode previous frames. 
%This is similar to Salsify which uses a similar on-demand re-sync scheme to use an old coding state to generate the next frame, allowing the decoder to skip loss-affected frames.
%However, the key difference is
%
%
% insight of on-demand re-sync is that the out-of-sync coding states will {\em affect only frames within an RTT}. 
%However, optimistic encoding with fast re-sync differ in that the receiver does not need to wait for the retransmission (in NACK) or the new P-frame (in Salsify) to decode the next frame frame; instead, it can still decode loss-affected frames with decent quality before encoder/decoder states are synchronized, so it reduces frame delay while maintaining high quality.


%\begin{itemize}
%\item synchronizing every frame will kill the benefit of DS
%\item however, the insight: its ok to be out of sync for a few frames
%\item idea: lazy synchronization. 
%\item to put it in perspective, salsify?
%\end{itemize}


%\jc{add a short para on when to decode a frame}
%
%\jc{what if all packets of a frame are lost}

\begin{comment}

\mypara{Balancing quality and frame delay}
%\mypara{Choosing when to decode a frame}
The data-scalable abstraction allows the receiver to flexibly decide, as packets arrive at the receiver, whether to decode the frame using currently arrived packets or wait for more packets in hope of improving the quality. 
(In contrast, with FEC, the receiver will always wait until enough data is received.)
%(In other loss-resilient schemes (\S\ref{??}), the receiver must wait for more packets until the data is decodable.) 
%\name embraces this flexibility with the following logic to trade frame delay with decoded quality. 



To make this decision, \name defines the {\em utility} of a frame as a linear combination of decoding quality and frame delay (since the natural decoding time) on each frame: $Q(|\{\textrm{pkts before }t\}|)-\beta\cdot t$, where $t$ is when the frame is decoded, $Q(n)$ is the frame's decoding quality with $n$ packets 
The precise values of $Q(n)$ are frame-dependent, but they are roughly similar across frames, so \name estimates $Q(n)$ using history frames.
%, and $\tau$ is the frame's natural decoding time (\eg 40ms after the last frame was decoded with frame rate 25fps).
%In our experiment, we set parameter $\beta=\fillme$.
This objective works well in practice, though there might be other objectives that better capture users' quality perception. An optimal design of such utility is beyond the scope of this paper. 

With this utility in mind, Figure~\ref{fig:decode-time} illustrates \name's logic: on receiving the $i^{\textrm{th}}$ packets of a frame (not necessarily the $i^{\textrm{th}}$ sent packet) at time $t_i$, the receiver will immediately decode the frame if all packets of the frame have arrived; otherwise, it will wait for the next packet of the frame until a deadline $t^*=t_i+\frac{1}{\beta}\cdot(Q(i+1)-Q(i))$, and if it has not received the $(i+1)^{\textrm{th}}$ packet by then, it will decode the frame with $i$ packets. 
The reason is that if the next packet comes at time $t_{i+1}$ after $t^*$, the utility $Q(i+1)-\beta\cdot (t_{i+1}-\tau)$ will be lower than the utility $Q(i)-\beta\cdot (t_i-\tau)$ if the receiver does not wait at all\footnote{This is because {\scriptsize $Q(i+1)-\beta\cdot (t_{i+1}-\tau)<Q(i+1)-\beta\cdot (t^*-\tau)=Q(i)-\beta\cdot (t_i-\tau)$}}. 
%Here, $\beta$ is a tunable parameter, and $Q(n)$ is the quality of the frame based on $n$ packets.
This strategy makes intuitive sense: the receiver will wait longer if the improvement in quality by getting one more packet (\ie $Q(n+1)-Q(n)$) is higher, but it will not wait for too long.



\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.995\linewidth]{figs/decode_time.pdf}
        \includegraphics[width=0.995\linewidth]{figs/decode_time_v2.pdf}
    \tightcaption{
    \name waits for the next frame until a deadline $t^*$, after which the utility is lower even if the next packet arrives. }
    \label{fig:decode-time}
\end{figure}


\end{comment}

%Readers may realize a potential problem arising from encoding and decoding being asynchronous. 


% However, we still need to design a practical packetization and entropy encoding scheme to make {\em entropy each encoded packet individually decodable} and do so {\em without an increase of data size}.
% This is not possible with standard autoencoders such as~\cite{dvc}, which entropy codes the entire \aecode to a single bitstream before packetization.
% As a result, any missing packet will render the bitstream undecodable. 
 


% Traditional codecs do have techniques to make each packet individually decodable, such as flexible macroblock ordering~\cite{lambert2006flexible} in H.264. These techniques divids the input frame into independent, non-overlapping partitions. Each partition is encoded separately, packed into its own entropy-encoded packet, enabling decodability if the corresponding packet arrives, as there's no dependency on other packets.

% However, this method leads to substantial size inflation, up to \editSOCC{50\%}~\cite{???}, due to the loss of compression efficiency inherent in traditional codecs' exploitation of content dependencies. For example, if two adjacent macroblocks share identical motion vectors (which is common in practice), H.264 can transmit the motion values once. But, if these macroblocks are separated into different partitions, each partition must send the value, resulting in size inflation.

% \name employs a different method as shown in Figure~\ref{fig:per-packet}. Instead of dividing the input frame, it {\em randomly} splits the elements in the coded tensor into sub-tensors and entropy encodes each sub-tensor separately. 
% The entropy coding in \name necessitates storing the symbol distribution of elements in the coded tensors for efficient compression. This means that, unlike methods that only send the symbol distribution once, our method requires storing it in every packet, potentially leading to additional overhead.
% However, this overhead is mitigated by the autoencoder training, which regularizes the distribution of elements in each coded tensor's channel to adhere to a zero-mean Laplace distribution. The variance value of each channel can be efficiently encapsulated with just a few bits. As a result, the overhead of including the symbol distribution in each packet remains minimal: even with 20 packets, the symbol distribution's size does not exceed 5\% of the total frame size.

% In \name, if a packet goes missing, we zero its elements in the original coded tensor. Given the random selection of these elements during encoding, this process effectively emulates random element masking, which matches the technique implemented during training. 
% Importantly, this approach ensures that the loss of any packet simulates a uniform random mask on the encoded tensor.

% The key difference between the per-packet entropy coding method used in traditional codecs and our method is that we don't have size inflation. This is because \name is not exploiting the dependency between elements for a better compression ratio, instead, it has fewer elements in the encoded data than traditional codecs. More specifically, in traditional codecs like H.264, each pixel has its motion vector and residual encoded in the bytestream, but \name's autoencoder will map the motion vector (or residual) of multiple pixels into the same element in the coded tensor. Therefore, \name can achieve the same size as traditional codecs without using dependencies between elements. During training, the autoencoder also learns to generate details to ensure that the quality does not drop even if we are sending less information than the traditional codecs.






\tightsubsection{Efficient coding and bitrate control}
\label{subsec:fast-coding}

\jc{the i-patch and i-frame discussion has been moved to appendix. Yihua, please do a thorough check to (1) make sure all essential discussion on iframes are still covered, to avoid comments like they only explained p-frames and what if i-frame is not loss resilient, etc, 
and (2) redirect all mentioning of iframe and ipatch to the appendix section}

\jc{some reorg: move efficient bitrate after speedup (i.e., explain how we speed up one pass of encoding, and then multiple passes. i'm not sure we need to separately explain gpu-based speedup. it's true we also make the original DVC faster on GPUs, but 1.5x seems quite marginal to be highlighted?}

%\tightsubsection{Reducing compute overhead}

%\mypara{Speed bottleneck}
% Most autoencoder research has been focused on video compression efficiency (using fewer bits to get higher quality), and their NN-based encoding and decoding are typically slower than the highly-optimized standard codecs like H.265.
% To be practical for real-time video streaming, \name entails a few additional optimizations to significantly speed up encoder and decoder and allow efficient re-encoding of a frame to match a given target bitrate. 


% I-patches are not protected by loss

% When the decoder fully receives an I-patch, it will notify the sender

% when an I-patch is fully received, the future P-frame will be based on the I-patch. 
% is still sent I-patches


% the effect of using I-patch on the frame sizes when $k=10$. It shows that I-patch effectively avoids sudden size increase caused by I-frames. 
% \passed{\amz{What is $k$ set to in Figure~\ref{fig:keyframe_smooth} ? }}
%\edit{In practice, we use BPG~\cite{bpg} to encode/decode the I-patch.}
%Depending on the original frame size, kk varies between 6 and 20. 
% This scheme effectively ``amortizes'' the size of I-frames across $k$ frames, thus smoothing the frame size as well as quality across frames.
% Moreover, since the I-frame autoencoder's encoding delay is proportional to the input size, encoding a small I-patch adds only a small compute overhead for each frame.

% (\S???????????????????????????????????????????????????????????????????????????????????????????????????\ref{app:??} shows an example).
% \footnote{We should clarify that design choice of frequent I-frames works well for autoencoders, but it is unnecessary for classic codecs due to two reasons. First, an I-frame generated by our autoencoder is only 2-5×\times bigger than a P-frame, whereas this ratio in H.264 is 4-10×\times. Second, the P-frame quality in H.264 is relatively stable, whereas the quality of a P-frame is high following an I-frame (or an I-patch).}

%\jc{mention which I frame model, and why not jpeg?}



%\jc{need a paragraph to explain why frequent i-patches actually make a lot of sense}


%\jc{how to deal with scene change?}



\begin{figure}[t!]
    \centering
         \centering
        %\includegraphics[width=0.92\linewidth]{figs/speedup.pdf}
        \includegraphics[width=0.92\linewidth]{figs/speedup.pdf}
    \tightcaption{How the autoencoder is changed for efficient bitrate control and speedup on CPUs.}
    \label{fig:speedup}
    \vspace{-0.3cm}
\end{figure}


\mypara{Efficient bitrate control}
Any video encoder must encode a frame at a size barely below the target frame size.
% Typically this can be done either by a heuristic to predict which quality level can yield the right frame size
%  encoding (as in H.264~\cite{OPENH264}) or encoding the frame multiple times at different quality levels (as in Salsify~\cite{salsify}). 
Similar to~\cite{salsify}, \name encodes a frame multiple times at different quality levels but does so faster than encoding the frame from scratch for multiple times 
% doing the whole encoding process on a frame multiple times 
(illustrated in Figure~\ref{fig:speedup}(b)). 
\name trains multiple autoencoders each with a different $\alpha$ (in Eq.~\ref{eq:2}) to achieve different quality/size tradeoff.
During the training phase, modifications were confined to the residual encoders and decoders, while other NN weights remained fixed. 
Thus, once a frame is encoded, both the motion vector (MV) and residual are reusable, with the residual undergoing further encoding through different encoders each producing a different frame size. 
This procedure, taking under 3ms, can encode a frame multiple times via residual encoders of distinct $\alpha$ values. Residual sizes in practice can span from 0.1$\times$ to 10$\times$ the MV size, thereby allowing \name to encompass a wide range of bitrates (see to \S\ref{subsec:eval:resilience}).
%but when we train these autoencoders, we {\em only} change their residual encoders and decoders, while freezing the weights of the MV encoder and decoder NNs.
%As a result, once a frame is encoded once, we can re-use the MV and residual but {\em only} re-encode the residual using a higher quality encoder, so encoding a frame the second time only takes less than 5ms. 
%This allows us to encode a frame multiple times (with the residual encoder of different $\alpha$s).
% Empirically, \name encodes each frame 1-2 times before getting a frame whose size is the highest but below the target frame size.

%Fortunately, we show that on a single NVIDIA GeForce 3080 GPU, \name's encoding speed can be greatly improved: from 5~fps on 720p HD (and 11~fps on 480p) videos by the off-the-shelf implementation to 18~fps (and 40~fps). More results in \S?????????\ref{subsec:eval:system}. 
%\name achieves such speedup by downsizing the image (by default 4×4\times) during motion-vector estimation and motion compensation, and then upsample the motion-compensated image before calculating and encoding the residuals. 
%This speeds up encoding because motion-vector estimation and motion compensation are the slowest steps during P-frame encoding and their delays are proportional to the input size.
%Thus, the overall encoding delay will be reduced if they are fed with downsized images. 
%At the same time, because the residuals are still computed between the full-resolution image and the motion-compensated image, the coding efficiency is not affected by this change for most frames.


\mypara{CPU-based speedup}
We have implemented a faster version of \name on CPUs.
% while preserving the loss-resilience autoencoder. 
It differs from the GPU-based autoencoder in two key aspects (Figure~\ref{fig:speedup}(c)): 
we (1) re-use the motion prediction logic in H.264 to generate MVs, and % (and re-train the encoder/decoder of both MV and residual), and
(2) remove the frame prediction NN from the motion compensation step. 
% As a result, with 32 threads, it takes 35ms to encode a 720p HD frame (and 17.2ms on 480p) on Intel Xeon 4216 CPU. \passed{\yc{need ziyi's input, how many threads?}} %\jc{on what CPUs?}. 
We deploy this modified \name to mobile devices using CoreML~\cite{coreml}, which is a tool optimizing on-device performance for iOS/macOS with CPU, GPU, and Neural Engine (on Apple devices).
It only takes \review{24.4ms} to encode a 720p HD frame (and 8.4ms on 480p) with CoreML on an iPhone 14 Pro. \yc{Note: this number is not accurate since it does not consider the h264 mv time}
As shown in \S\ref{subsec:eval:system}, the resulting autoencoder has slightly worse compression efficiency, but still achieves low frame delay in the presence of packet loss.
% obtains most of the benefit of a data-scalable coding system (\eg low frame delay in the presence of packet loss). 


\mypara{GPU-based speedup}
We use two ideas to speed up autoencoder on GPUs: 
(1) it uses Pytorch's just-in-time compiler~\cite{torchcompile} to optimize the NN encoder and NN decoder, and 
(2) it reduces the NN float-point precision from 32-bit to 16-bit. %\jc{Yihua/Ziyi, of all NNs or some NNs?} \zy{added}
As shown in \S\ref{subsec:eval:system}, on an NVIDIA A40 GPU, our implementation speeds up the encoder from 19.8 fps on 720p HD (and 39.5 fps on 480p) videos by the off-the-shelf implementation to 31.2 fps (and 87.7 fps on 480p), roughly a 1.5$\times$ speedup. More results in \S\ref{subsec:eval:system}.
This speed is on par with the speed-optimized proprietary autoencoders~\cite{elf}, and it still achieves desirable loss resilience and compression efficiency.
\passed{\amz{An obvious question here is "why not use the same optimization from CPU's MV on the GPU's NVENC"? I expect it would not actually provide a big benefit, since using the NVENC hardware on the GPU during inference will likely incur additional data movement between buffers, but if there’s a way you can head off that inquiry that might help. If you haven't tried it maybe add such an optimization as future work?} \yc{opticflow accelerator: https://developer.nvidia.com/blog/harnessing-the-nvidia-ada-architecture-for-frame-rate-up-conversion-in-the-nvidia-optical-flow-sdk/}}




%\mypara{Downscaling motion-vector operations}

\begin{comment}
\mypara{Speeding up on GPUs}
Most of the delay of \name's encoder and decoder can be attributed to motion related operations, including motion estimation, motion vector (MV) encoding, MV decoding, and motion compensation (see Figure~??????\ref{fig:dvc-arch}). 
%For example, to encode and decode a 720p frame (1280x720) on a \fillme GPU, these motion-related operations take \fillme\% of encoding delay and \fillme\% of decoding delay. 
Since most operations in MV encoding and decoding are mostly convolutional, \name speeds up these motion-related operations by downscaling the MV (by 4×4\times, by default) which speeds up the MV encoding and decoding by 4×\times.
In addition, \name uses Pytorch's just-in-time compiler to optimize the implementation of the encoder and decoder. 
\end{comment}


%At the same time, because the residuals are still computed between the full-resolution image and the motion-compensated image, the coding efficiency is not affected by this change for most frames.


%\name speeds up the encoding and decoding of its autoencoders 
%
%%\begin{packeditemize}
%%\item {\em Downscaling motion vectors:} 
%
%Since most motion-related operations are convolutional, their compute overheads are proportional to the dimension of the input frames. 
%Thus, \name speeds up motion-related operations by downsizing ($4\times$ in default) the input frame and the reference frames, and then upscale the motion-compensated image to compute the full-scale residual.
%%\item {\em Efficient bitrate control}
%%\end{packeditemize}




%\tightsubsection{Bitrate control}





%\jc{yihua, ziyi, fill in the text}




\begin{comment}

As a video coding system, the target frame size for \name to encode a frame is determined by an external adaptation, such as GCC, typically to match the estimated throughput.
To cope with fluctuations of network condition, throughput estimation can vary even between two consecutive frames.
As a result, \name should encode each frame at a size barely below the target frame size.
%This has been a challenge with traditional codecs.
%Thus, it is important that most frames are smaller than the target size set by congestion control, but traditional codecs are not able to do that. 
%This has been observed in \cite{salsify}, which proposes to encode each frame at multiple quality levels in order to find an encoding that fits the target bitrate. 

To encode frame at a size below a given target, \name employs a bitrate-control method similar as~\cite{salsify} and encodes each frame twice and picks the frame that has the closest size to the target. 
To do so, we need to (1) train multiple autoencoders whose frame sizes cover a wide range, and (2) run two of them as fast as possible. 

% to encode a frame with a maximum size below a target. 
First, \name trains multiple autoencoders, each using a different weight of frame size $\alpha$ in its training loss function (\S\ref{subsec:sim-losses}).
These resulting autoencoders cover a range of bitrate range. \jc{some numbers}
%\fillme$\times$ difference between the highest bitrate and lowest bitrate. (A wider bitrate range is possible with more autoencoders.)
As long as the target bitrate is within this range, \name should be able to select the autoencoder whose encoded frame size is barely lower than the target. 

Next, \name avoids the excessive compute overhead by re-using the motion-compensated image to get the residuals, and only run different versions of residual encoders to encode the residuals with different bitrates.
Since residual encoder is faster than the motion estimation and compensation, the speed up is significant. \jc{some numbers}
%A naive solution will run multiple autoencoders (like~\cite{salsify}), but the compute overhead will increase linearly.
%Fortunately, we can again re-use 

\jc{explain hanchen's bitrate control logic}

\end{comment}




% Figure~\ref{fig:e2e} puts the various pieces of \name in an end-to-end workflow, and  Table~\ref{tab:mapping} summarizes the effect of each components of \name. 

%generates the downscaled motion-vector coded tensor (\S\ref{??}) and the I-patch coded tensor (\S\ref{??}).
%It then uses the bitrate controller (\S\ref{??}) to pick the residual encoder NN so that the resulting frame size closely matches the target bitrate. 
%On the receiver side, \name uses the logic described in \S\ref{??} to determine when to decode a frame.

%\mypara{Relationship with congestion control}
\name is {\em complementary} to existing congestion control (CC) algorithms. 
When combined with \name, the CC algorithm does {\em not} need to retransmit packets, unless no packets of a frame are received.
%The choice of the congestion control (CC) logic is {\em complementary} to \name.
CC determines how fast the packets should be sent out and the target bitrate of the next frame, whereas \name decides what should be in each packet. 
\S\ref{app:salcc} evaluates \name with GCC in WebRTC~\cite{carlucci2016analysis} and Salsify CC~\cite{salsify}. 
\jc{the last sentence is a bit misplaced. can we actually say anything interesting about it?}
\S\ref{app:webrtc} discusses how to integrate \name in WebRTC.
% to run with the GCC algorithm while disabling the packet retransmission.
%Since it does not change the CC logic, \name can be readily integrated in WebRTC. We will discuss details .






%\jc{need an end-to-end figure here}


%\begin{figure}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.99\linewidth]{figs/technique-mapping.pdf}
%    \tightcaption{}
%    \label{fig:technique-mapping}
%\end{figure}



\begin{comment}

At a high level, the \name encoder and decoder feed packets to congestion control (CC) which determines how fast the packets should be sent out and the target bitrate (size) of the next frame. 
\name can work with different CC logics that have this interface.
These include GCC~\cite{??} and Salsify's CC logic~\cite{??} both of which are used as CC when we test \name and other video codecs in \S\ref{sec:eval}.
It should be noted that \name does not use FEC. 



\mypara{Interaction with transport layers}
%\name is built on the data-scalable autoencoder \name. 
%\name is a concrete real-time video communication system built on a data-scalable autoencoder (\name).
We focus on unique issues arising from the use of \name as the codec, including how to deliver each frame to strike a desirable delay-quality tradeoff, and how to deliver a sequence of frames when congestion or packet losses affect multiple frames. 
The choice of the congestion control logic is complementary to \name. 
In \S\ref{subsec:eval:e2e}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{carlucci2016analysis} or Salsify CC~\cite{salsify}. 
We do not claim that \name's strategies are new (\eg reference frame synchronization has been used in~\cite{salsify}). 
Nonetheless, \name integrates concrete design choices driven by the need, in order to unleash the full potential of \name and its data-scalable codec primitive.


\jc{interface?}

\end{comment}
%\jc{TODO}









==> sections/old/protocol.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US





\tightsection{Real-time video framework}
\label{sec:delivery}

%\jc{
%\begin{itemize}
%\item coding of i-frames (compression)
%\item bitrate control (speed)
%\item speedup on cpu (speed)
%\item end-to-end protocol (why no synchronization, interaction with tcp and abr) (resilience)
%\end{itemize}
%}

%\jc{a table mapping the techniques to effects
%\begin{itemize}
%\item compression: i-frames, per-packet entropy
%\item speed: bitrate control, cpu speedup
%\item resilience: retraining, end-to-end protocol
%\end{itemize}
%}

The new autoencoder described in \S\ref{sec:core} can achieve data-scalable (DS) coding on a {\em single} frame under simulated packet loss. 
This section presents \name's online video delivery framework. 
In particular,
\begin{packeditemize}
\item How to entropy encode autoencoder output into packets (\S\ref{subsec:packetization}), 
\item How to stream a sequence of frames (\S\ref{subsec:protocol}), and
\item How to speed up encoding/decoding on GPUs and CPUs without sacrificing loss resilience (\S\ref{subsec:fast-coding}).
\end{packeditemize}
% \yc{I moved entropy coding to 4.1, since I feel this is more smooth: first talking about tensor -> packets for each frame, then discuss how we stream sequence of frames, finally some optimizations}

\tightsubsection{Entropy encoding the encoder's output}\label{subsec:packetization}
Like classic codecs of H.264 and VP9, the NN encoder's output tensor also needs to be losslessly compressed into a bitstream using an arithmetic (entropy) coding scheme.
An arithmetic encoder uses an underlying symbol distribution to compress the value at each position of the tensor.
Unlike classic codecs that use hand-tuned heuristics like CABAC, autoencoders, including DVC, often train the value distribution jointly with the NN encoder and decoder to learn a better distributional representation of the values in the NN encoder output. 
Since the decoder later uses the same symbol distributions to recover the tensor, the symbol distribution is also sent together with the data. 
However, because \name divides the encoder's output tensor into subtensors, each being separately entropy encoded into a packet, thus each packet must include a copy of its own symbol distribution.
This will greatly increase the size if the data of a frame is split into many packets. 

We reduce this per-packet overhead by carefully choosing the precision of symbol distribution, which governs the tradeoff between the size of a symbol distribution and the size of the entropy-encoded data.
A coarser-grained symbol distribution needs fewer bits to store, but it may yield a higher size of the entropy-encoded data. 
\name's insight is that we can train the NN encoder in a way that regularizes the distribution of values in each encoder's output channel to conform to a zero-mean Laplace distribution. 
(Each encoder output tensor has 224 channels.)
This way, the symbol distribution only needs to store the variance within each channel while still perfectly compressing the encoder output tensor. 
As a result, the symbol distribution takes only $\sim$50 bytes to store per packet (a reduction from 40\% of the packet size to 5\%), without hurting the compression efficiency of entropy coding.

\begin{comment}
\tempstrike{
As described in \S\ref{sec:core}, \name uses a reversible pseudo-random mapping to divide the encoder's output tensor into packets. 
Practically, we further compress each packet's subtensor into a more compact bytestream via individual entropy encoding, reducing the bytes transmitted through the network.

Similar to traditional codecs and prior autoencoders~\cite{dvc}, \name uses arithmetic coding~\cite{??} to entropy encode the subtensor into a compressed byte stream. 
The entropy encoder takes two inputs: the subtensor itself and the distribution for each element in the subtensor. 
To correctly decode the original subtensor at the decoder side, the distribution should also be sent to the receiver in the same packet.
It is worth noting that there is a trade-off between the size of the encoded subtensor and the size of the distribution:
The size of the entropy-encoded subtensor will be smaller if the distribution is closer to the real distribution of the subtensor, however, it may significantly increase the size of the distribution, resulting in worse compression efficiency.
\name mitigates this during training by regularizing each coded tensor channel's distribution to conform to a zero-mean Laplace distribution. 
Furthermore, the variance of each channel can be efficiently represented using minimal bits, adding a trifling overhead of approximately 50 bytes per packet. \yc{``overhead'' may not be a good word here?} 

To get the distribution during runtime, traditional codecs, like H.264, use a hard-coded distribution table~\cite{??cabac} for different input elements.
In contrast, \name uses a small neural network to estimate the variance of each channel. This small neural network is also jointly trained with the encoder during training, making it able to estimate the distribution more accurately.
TTo ensure each entropy-encoded packet aligns with a predetermined packet size, \name estimates the frame size prior to partitioning the output tensor into subtensors, by calculating the distribution's entropy. The accuracy of this size estimation is reinforced by the consistent use of the same distribution for entropy encoding the tensor\yc{we should explain why the estimated size is accurate, but this sentence is not clear}. 
In practice, the error of the estimated distribution is never larger than 2\%.
}
\end{comment}


\tightsubsection{Streaming protocol}
\label{subsec:protocol}

% To extend the P-frame DS autoencoder trained in \S\ref{subsec:training} for multiple frames, the first challenge is potential out-of-sync {\em states} between the encoder and decoder when packet loss occurs.
%Two challenges arise when extending the P-frame DS autoencoder trained in \S\ref{subsec:??} to the delivery of multiple frames: (1) potential out-of-sync coding state between the encoder and decoder when packet loss occurs, and (2) how to encode I-frames and how frequently to add I-frames.



\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v3.pdf}
        % \includegraphics[width=0.99\linewidth]{figs/state-sync-v2.pdf}
        \includegraphics[width=0.92\linewidth]{figs/state-sync-v3.pdf}
    \tightcaption{Examples of how to deal with loss-affected frames: 
    (a) delayed by retransmission, (b) ignoring out-of-sync encoder/decoder states, and (c) 
    \name's frame optimistic encoding and state re-sync.}
    \label{fig:state-sync}
    \vspace{-0.1cm}
\end{figure}

\mypara{Basic protocol}
The \name encoder encodes a new frame with a fixed interval, and % (by default, 40ms or 25fps).
the decoder tries to decode a frame when the first packet of the next frame is received using the following logic:
\begin{packeditemize}
\item If no packet of the current frame is received, then it will request the sender to send the frame again;
\item Otherwise (at least one packet of the current frame is received), then it will decode the frame.
%\item If a subset of the packets of the current frame are received, then it will decode the frame and send a ``re-sync'' signal to the sender.
\end{packeditemize}

%\mypara{Encoding reference state}
However, if we directly replace the traditional codec with the new autoencoder, it could cause low quality on a frame even if all of its packets arrive on time. 
This is because if a reference frame is decoded using a subset of packets, the state will be ``out-of-sync'' between the encoder and decoder---the reference image used to encode the next frame is different from the reference used by the decoder.
% This can affect all subsequent frames if not handled appropriately.
% Figure~\ref{fig:state-sync} shows an example. 
In standard video coding, to encode the $7^{\textrm{th}}$ frame, the sender uses the decoded result of the $6^{\textrm{th}}$ frame as the reference to compute motion vectors and residual of the $7^{\textrm{th}}$ frame, and the receiver will use the same reference frame to decode the $7^{\textrm{th}}$ frame. 
However, if the receiver uses \name autoencoder to decode the $6^{\textrm{th}}$ frame using only a subset of its packets (Figure~\ref{fig:state-sync}(a)), it will see a different reference frame when decoding the $7^{\textrm{th}}$ frame than what the encoder has assumed when encoding the $7^{\textrm{th}}$ frame.
Thus, even if all packets of the $7^{\textrm{th}}$ are received, its quality will be slightly lower than it should be.
Similarly, since the $7^{\textrm{th}}$ is also out of sync with the sender's state, the $8^{\textrm{th}}$ frame will suffer too, and so forth.
%In short, the quality of many frames with zero \rate might still be affected.

%the naive method of using \name (Figure~\ref{fig:state-sync}(b)) will affect quality degradation on frames that do not have 

%the reference frame used by the receiver to decode the 10th10^{\textrm{th}} frame will differ from what the encoder has assumed. 
%
%, and without knowing which of the 9th9^{\textrm{th}} frame's packets will be lost, it will assume that the 9th9^{\textrm{th}} frame is decoded with all packets being received. (This is common to classic codecs and autoencoders.)
%However, if the receiver decodes the 9th9^{\textrm{th}} frame with only a subset of its packets, the actual reference frame used to decode the 10th10^{\textrm{th}} will differ from what the encoder has assumed. 
%Thus, most codecs require all packets of the 9th9^{\textrm{th}} frame to be received before decoding it (thus longer delay), or let the sender encode the 10th10^{\textrm{th}} based on an earlier reference (say the 5th5^{\textrm{th}}) whose lost packets are already known to the sender. 
%The latter {\em synchronizes} the encoding and decoding states (like in Salsify~\cite{salsify} during packet losses), but it also inflates the frame size, since the difference between the 10th10^{\textrm{th}} and the 5th5^{\textrm{th}} frames  is much greater than between the 10th10^{\textrm{th}} and the 9th9^{\textrm{th}} frames. 


%\begin{figure*}[t!]
%    \centering
%         \centering
%%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v3.pdf}
%        \includegraphics[width=0.9\linewidth]{figs/state-sync-v1.pdf}
%    \tightcaption{}
%    \label{fig:per-packet}
%\end{figure*}


A strawman solution is that the encoder and decoder synchronize on each frame.
% ---if the receiver decodes a frame with a subset of packets, the sender should always know which packets are used in order to reconstruct the same reference frame seen by the decoder. 
However, this will negate the benefit of \name's generative autoencoder, as the sender will wait until the receiver acknowledges after each frame which takes at least an RTT.
% for the acknowledgment from the receiver (at least an RTT) after each frame, 

\mypara{Optimistic encoding with dynamic state re-sync}
%Rather than syncing-up the reference state every frame, 
Instead, \name lets the sender optimistically encode frames without syncing the coding states.
However, once receiving the feedback that the decoder decodes a frame using a subset of its packets, the sender will quickly re-decode the recent frames with the same decoded frame as seen by the decoder to reconstruct the same reference frame seen by the decoder. 
(Explained shortly, such re-decoding can be greatly sped-up.)
For instance, in Figure~\ref{fig:state-sync}(b), the sender is about to encode the $9^{\textrm{th}}$ when it gets the feedback that says the $6^{\textrm{th}}$ was decoded with a certain subset of packets, then the encoder will quickly re-decode the frames from the $6^{\textrm{th}}$ (with the same subset of packets) to $8^{\textrm{th}}$ frames and use the new decoded $8^{\textrm{th}}$ frame as the reference to encode the $9^{\textrm{th}}$ frame.




%\name's autoencoder can decode frames with inconsistent coding states for a handful of frames, though the quality will deteriorate over time if the coding state is left unsynced for too long. \jc{need a visualization in eval}
%However, our fast re-sync scheme makes sure that 

%The basic insight is that without synchronizing the reference frames, \name's autoencoder can decode frames with high quality for a handful of frames. \jc{need a visualization here}
%
%Therefore, the sender does not need to wait for the feedback from the receiver; instead, it can optimistically encode the next frame assuming the packets of the previous frames are completely received, until it receives a feedback from the receiver that a previous frame was not decoded with all packets (this feedback can be like an NACK in WebRTC).
%Suppose that the sender is about to encode the $9^{\textrm{th}}$ when it gets a feedback that says the $6^{\textrm{th}}$ was decoded with certain subset of packets (illustrated in Figure~\ref{fig:state-sync}(c)), then the encoder will quickly re-decode the frames from the $6^{\textrm{th}}$ to $8^{\textrm{th}}$ frames (this step can be greatly sped-up shortly), and use the new decoded $8^{\textrm{th}}$ frame as the reference to encode the $9^{\textrm{th}}$ frame.



A potential speed bottleneck is re-decoding reference frames (\eg from $6^{\textrm{th}}$ to $8^{\textrm{th}}$ frames in Figure~\ref{fig:state-sync}(c)) during re-sync. 
Fortunately, both the encoder and the decoder can re-decode these frames much faster than the normal decoding, by skipping both motion-estimation NN and the frame-prediction NN (Figure~\ref{fig:dvc-arch}).
This saves 93\% of encoding time per frame.
The insight is two-fold.
First, these frames have been decoded once, and the re-decoding simply needs to estimate the incremental changes caused by the lost packets, so it can be much faster. 
Second, skipping the frame-prediction NN does reduce the compression efficiency on the last frame (\eg the $9^{\textrm{th}}$ frame in  Figure~\ref{fig:state-sync}(c)), but it only affects only one frame.
The formal proof of why the re-decoding works can be found in \S\ref{app:resync}.%\jc{YIHUA!}

% re-synchronization does not have to have the highest quality, which allows us to skip the motion-smoothing NN in frame prediction. In addition, this is also a unique benefit of autoencoders.
% The formal proof can be found in \S\ref{??}.

\tempstrike{
    
% \footnote{\edit{The motion smoothing NN is trained to smooth the predicted frame, so that the residual will be smaller and thus easier to compress.}} 
% in the frame prediction \st{NN} \edit{step} (shown in Figure~\ref{fig:dvc-arch}), 
which takes up \fillme\% of the decoding time per frame. 
The new $8^{\textrm{th}}$ frame will be used to encode the $9^{\textrm{th}}$ frame in  Figure~\ref{fig:state-sync}(c), and when the receiver receives the encoded $9^{\textrm{th}}$ frame, it also re-decodes the frames from 6-8 {\em without} the \edit{motion-smoothing NN}.
% \st{frame prediction NN} (not shown in figure), 
Since both re-encoding and re-decoding skip the time-consuming motion-smoothing NN, the overhead is minimum 
but since this is much faster, it will not add much new overhead. 
The insight behind it is that re-synchronization does not have to have the highest quality, which allows us to skip the motion-smoothing NN in frame prediction. In addition, this is also a unique benefit of autoencoders.
%which is unique to the benefit of autoencoders

}

%allowing it to re-decode these frames using a different but faster method.
%The insight is that the decoding does not have to have the highest quality, which allows us to skip the motion-smoothing NN in motion compensation (Figure~\ref{??}) which significantly reduces the delay by \fillme\%.\jc{need a few words on why}
%For this optimization to work, the receiver also needs to re-decode the frames from 6-8 without the motion-smoothing NN, but since this is much faster, it will not add much new overhead. 

    

%, but it leverages the loss resilience of the new autoencoders.
% Like \name, NACK and Salsify allow senders to burst packets without waiting for acks, and when packet loss happens, NACK retransmits lost packets which delays the decoding of future frames and Salsify rewinds the encoder to an old state to generate the next P-frame, allowing the decoder to skip loss-affected frames.
% However, \name's key difference is that 

The dynamic state re-sync described above highlights a key advantage of \name's decoder---it does not need to skip or block the decoding of loss-affected frames; instead, it still decodes loss-affected frames with decent quality {\em before} encoder/decoder states are synchronized, so it reduces frame delay while maintaining decent quality. 
% This makes \name's optimistic encoding with dynamic state re-sync 
This is fundamentally different from  NACK (negative ack) in WebRTC (which blocks the decoding of loss-affected frames) and the encoder/decoder state synchronization in Salsify (which skips the loss-affected frames).
% , where the latter methods need to either wait for or skip the loss affected frames.

%Although \name's optimistic encoding with dynamic state re-sync may sound similar to NACK (negative ack) in WebRTC and the encoder/decoder state synchronization in Salsify, but it has a key difference. 
%The receiver in \name does not need to skip or block the decoding of loss-affected frames; instead can still decode loss-affected frames with decent quality before encoder/decoder states are synchronized, so it reduces frame delay while maintaining high quality. 
\passed{\amz{This is also framed in a roundabout way, but is also a key insight of this work IMO -- using your packetization allows for decoding lossy frames with less delay. Switching these sentences ("Another benefit of \name is that the receiver does not need to skip... This differentiates our dynamic state re-sync from NACK and Salsify")} \yc{reorganized the contents}}
%wait for the retransmission (in NACK) or the new P-frame (in Salsify) to decode the next frame frame; instead, it can still decode loss-affected frames with decent quality before encoder/decoder states are synchronized, so it reduces frame delay while maintaining high quality.


%Like NACK (negative ack) which WebRTC senders use to burst packets without waiting for acks until an NACK is received, 
%% from the receiver that some packets must be retransmitted in order to decode previous frames. 
%This is similar to Salsify which uses a similar on-demand re-sync scheme to use an old coding state to generate the next frame, allowing the decoder to skip loss-affected frames.
%However, the key difference is
%
%
% insight of on-demand re-sync is that the out-of-sync coding states will {\em affect only frames within an RTT}. 
%However, optimistic encoding with fast re-sync differ in that the receiver does not need to wait for the retransmission (in NACK) or the new P-frame (in Salsify) to decode the next frame frame; instead, it can still decode loss-affected frames with decent quality before encoder/decoder states are synchronized, so it reduces frame delay while maintaining high quality.


%\begin{itemize}
%\item synchronizing every frame will kill the benefit of DS
%\item however, the insight: its ok to be out of sync for a few frames
%\item idea: lazy synchronization. 
%\item to put it in perspective, salsify?
%\end{itemize}


%\jc{add a short para on when to decode a frame}
%
%\jc{what if all packets of a frame are lost}

\begin{comment}

\mypara{Balancing quality and frame delay}
%\mypara{Choosing when to decode a frame}
The data-scalable abstraction allows the receiver to flexibly decide, as packets arrive at the receiver, whether to decode the frame using currently arrived packets or wait for more packets in hope of improving the quality. 
(In contrast, with FEC, the receiver will always wait until enough data is received.)
%(In other loss-resilient schemes (\S\ref{??}), the receiver must wait for more packets until the data is decodable.) 
%\name embraces this flexibility with the following logic to trade frame delay with decoded quality. 



To make this decision, \name defines the {\em utility} of a frame as a linear combination of decoding quality and frame delay (since the natural decoding time) on each frame: $Q(|\{\textrm{pkts before }t\}|)-\beta\cdot t$, where $t$ is when the frame is decoded, $Q(n)$ is the frame's decoding quality with $n$ packets 
The precise values of $Q(n)$ are frame-dependent, but they are roughly similar across frames, so \name estimates $Q(n)$ using history frames.
%, and $\tau$ is the frame's natural decoding time (\eg 40ms after the last frame was decoded with frame rate 25fps).
%In our experiment, we set parameter $\beta=\fillme$.
This objective works well in practice, though there might be other objectives that better capture users' quality perception. An optimal design of such utility is beyond the scope of this paper. 

With this utility in mind, Figure~\ref{fig:decode-time} illustrates \name's logic: on receiving the $i^{\textrm{th}}$ packets of a frame (not necessarily the $i^{\textrm{th}}$ sent packet) at time $t_i$, the receiver will immediately decode the frame if all packets of the frame have arrived; otherwise, it will wait for the next packet of the frame until a deadline $t^*=t_i+\frac{1}{\beta}\cdot(Q(i+1)-Q(i))$, and if it has not received the $(i+1)^{\textrm{th}}$ packet by then, it will decode the frame with $i$ packets. 
The reason is that if the next packet comes at time $t_{i+1}$ after $t^*$, the utility $Q(i+1)-\beta\cdot (t_{i+1}-\tau)$ will be lower than the utility $Q(i)-\beta\cdot (t_i-\tau)$ if the receiver does not wait at all\footnote{This is because {\scriptsize $Q(i+1)-\beta\cdot (t_{i+1}-\tau)<Q(i+1)-\beta\cdot (t^*-\tau)=Q(i)-\beta\cdot (t_i-\tau)$}}. 
%Here, $\beta$ is a tunable parameter, and $Q(n)$ is the quality of the frame based on $n$ packets.
This strategy makes intuitive sense: the receiver will wait longer if the improvement in quality by getting one more packet (\ie $Q(n+1)-Q(n)$) is higher, but it will not wait for too long.



\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.995\linewidth]{figs/decode_time.pdf}
        \includegraphics[width=0.995\linewidth]{figs/decode_time_v2.pdf}
    \tightcaption{
    \name waits for the next frame until a deadline $t^*$, after which the utility is lower even if the next packet arrives. }
    \label{fig:decode-time}
\end{figure}


\end{comment}

%Readers may realize a potential problem arising from encoding and decoding being asynchronous. 


% However, we still need to design a practical packetization and entropy encoding scheme to make {\em entropy each encoded packet individually decodable} and do so {\em without an increase of data size}.
% This is not possible with standard autoencoders such as~\cite{dvc}, which entropy codes the entire \aecode to a single bitstream before packetization.
% As a result, any missing packet will render the bitstream undecodable. 
 


% Traditional codecs do have techniques to make each packet individually decodable, such as flexible macroblock ordering~\cite{lambert2006flexible} in H.264. These techniques divids the input frame into independent, non-overlapping partitions. Each partition is encoded separately, packed into its own entropy-encoded packet, enabling decodability if the corresponding packet arrives, as there's no dependency on other packets.

% However, this method leads to substantial size inflation, up to \editSOCC{50\%}~\cite{???}, due to the loss of compression efficiency inherent in traditional codecs' exploitation of content dependencies. For example, if two adjacent macroblocks share identical motion vectors (which is common in practice), H.264 can transmit the motion values once. But, if these macroblocks are separated into different partitions, each partition must send the value, resulting in size inflation.

% \name employs a different method as shown in Figure~\ref{fig:per-packet}. Instead of dividing the input frame, it {\em randomly} splits the elements in the coded tensor into sub-tensors and entropy encodes each sub-tensor separately. 
% The entropy coding in \name necessitates storing the symbol distribution of elements in the coded tensors for efficient compression. This means that, unlike methods that only send the symbol distribution once, our method requires storing it in every packet, potentially leading to additional overhead.
% However, this overhead is mitigated by the autoencoder training, which regularizes the distribution of elements in each coded tensor's channel to adhere to a zero-mean Laplace distribution. The variance value of each channel can be efficiently encapsulated with just a few bits. As a result, the overhead of including the symbol distribution in each packet remains minimal: even with 20 packets, the symbol distribution's size does not exceed 5\% of the total frame size.

% In \name, if a packet goes missing, we zero its elements in the original coded tensor. Given the random selection of these elements during encoding, this process effectively emulates random element masking, which matches the technique implemented during training. 
% Importantly, this approach ensures that the loss of any packet simulates a uniform random mask on the encoded tensor.

% The key difference between the per-packet entropy coding method used in traditional codecs and our method is that we don't have size inflation. This is because \name is not exploiting the dependency between elements for a better compression ratio, instead, it has fewer elements in the encoded data than traditional codecs. More specifically, in traditional codecs like H.264, each pixel has its motion vector and residual encoded in the bytestream, but \name's autoencoder will map the motion vector (or residual) of multiple pixels into the same element in the coded tensor. Therefore, \name can achieve the same size as traditional codecs without using dependencies between elements. During training, the autoencoder also learns to generate details to ensure that the quality does not drop even if we are sending less information than the traditional codecs.






\tightsubsection{Efficient coding and bitrate control}
\label{subsec:fast-coding}

%\tightsubsection{Reducing compute overhead}

%\mypara{Speed bottleneck}
% Most autoencoder research has been focused on video compression efficiency (using fewer bits to get higher quality), and their NN-based encoding and decoding are typically slower than the highly-optimized standard codecs like H.265.
% To be practical for real-time video streaming, \name entails a few additional optimizations to significantly speed up encoder and decoder and allow efficient re-encoding of a frame to match a given target bitrate. 

\begin{figure}[t!]
    \centering
        %\includegraphics[width=0.85\linewidth]{figs/split-iframe-size.pdf}
    \includegraphics[width=0.75\linewidth]{figs/split-iframe-size.pdf}
    \tightcaption{Encoding each P-frame with a small I-patch leads to smoother frame sizes than naively inserting I-frames.}
    \label{fig:keyframe_smooth}
\end{figure}

\mypara{I-frames}
In many autoencoders (including DVC), 
%Placement of I-frames poses a particular challenge for \name's autoencoders (both pre-trained and re-trained), because while 
the quality of P-frames will gradually degrade after an I-frame.
%, quality gradually degrades after about 10 frames. 
%for two reasons: (1) I-frames are generally bigger in size than P-frames, and 
%(2)  while the first few P-frames after an I-frame enjoy high quality, quality gradually degrades after about 10 frames. 
If we add I-frames frequently (\eg every 10 frames), we can achieve similar average compression efficiency with  H.264 and H.265 when they use an optimal I-frame interval.
% \footnote{Many computer-vision papers on autoencoders have conveniently used a small GoP when compared against H.265, but the implication of large I-frame size for congestion control is rarely discussed.}, 
% which strikes a better tradeoff between quality and {\em average} bitrate (comparable to H.264 and H.265 with large I-frame intervals).
However, since I-frames are larger than P-frames, adding too many I-frames causes frequent spikes in frame size. %, so it is difficult for congestion control to utilize network capacity. %at a fixed frame interval. 
%make it difficult for congestion control to send the frames at a fixed interval (inversely proportional to the frame rate).
Instead, \name uses an {\em extra} small square-sized patch as a tiny I-frame, called {\em I-patch}, on {\em every P frame}.
We split each frame into $k$ patches, and for a window of $k$ frames, each frame is sent with an extra I-patch at a different location, so I-patch ``scan through'' the whole frame every $k$ frame. 
By default, $k=30$ though we empirically found any value between 10 and 30 works well.
% the location of the I-patch on a frame changes over time, so that the I-patch will scan through the whole frame size every $k$ frames. 
With I-patch, \name does not need to send any I-frames (except the first frame). 
We use BPG~\cite{bpg} to encode/decode the I-patch. 
% , and found that as long as $k$ is between 10 and 30, the compression efficiency is roughly the same. 
Figure~\ref{fig:keyframe_smooth} shows that when $k=10$, I-patch mitigates the sudden size increase caused by I-frames. 

%\tightsubsection{Encoding a sequence of frames}
%\label{subsec:delivery:iframe}

%To stream a sequence of video frames, a key question is how often I-frames should be inserted in P-frames. 
%(As explained in \S???????????????????????????????????????????????????????????????????????????????????????????????????\ref{subsec:ae-background}, \name uses only I-/P-frames, as in most real-time video systems.)
%For the P-frame autoencoder we have tried, we observe that the decoded quality can be very high right after each I-frame but it gradually degrades after about 10 frames. 


%To add I-frames frequently without the intermittent bitrate spikes caused by the I-frames, 
% (128$\times$128 to 512$\times$512) 


It is worth noting that though I-patch encoding can also use a loss-resilient autoencoder, we do not protect their packet loss to simplify the system design. 
This is because if each patch will see an I-patch every $k$ frames, so even if one patch is lost, its impact is confined to the next $k$ frames, and empirically, even this impact is marginal since P-frames are still delivered.

% I-patches are not protected by loss

% When the decoder fully receives an I-patch, it will notify the sender

% when an I-patch is fully received, the future P-frame will be based on the I-patch. 
% is still sent I-patches


% the effect of using I-patch on the frame sizes when $k=10$. It shows that I-patch effectively avoids sudden size increase caused by I-frames. 
% \passed{\amz{What is $k$ set to in Figure~\ref{fig:keyframe_smooth} ? }}
%\edit{In practice, we use BPG~\cite{bpg} to encode/decode the I-patch.}
%Depending on the original frame size, kk varies between 6 and 20. 
% This scheme effectively ``amortizes'' the size of I-frames across $k$ frames, thus smoothing the frame size as well as quality across frames.
% Moreover, since the I-frame autoencoder's encoding delay is proportional to the input size, encoding a small I-patch adds only a small compute overhead for each frame.

% (\S???????????????????????????????????????????????????????????????????????????????????????????????????\ref{app:??} shows an example).
% \footnote{We should clarify that design choice of frequent I-frames works well for autoencoders, but it is unnecessary for classic codecs due to two reasons. First, an I-frame generated by our autoencoder is only 2-5×\times bigger than a P-frame, whereas this ratio in H.264 is 4-10×\times. Second, the P-frame quality in H.264 is relatively stable, whereas the quality of a P-frame is high following an I-frame (or an I-patch).}

%\jc{mention which I frame model, and why not jpeg?}



%\jc{need a paragraph to explain why frequent i-patches actually make a lot of sense}


%\jc{how to deal with scene change?}



\begin{figure}[t!]
    \centering
         \centering
        %\includegraphics[width=0.92\linewidth]{figs/speedup.pdf}
        \includegraphics[width=0.92\linewidth]{figs/speedup.pdf}
    \tightcaption{How the autoencoder is changed for efficient bitrate control and speedup on CPUs.}
    \label{fig:speedup}
    \vspace{-0.3cm}
\end{figure}


\mypara{Efficient bitrate control}
Any video encoder must encode a frame at a size barely below the target frame size.
% Typically this can be done either by a heuristic to predict which quality level can yield the right frame size
%  encoding (as in H.264~\cite{OPENH264}) or encoding the frame multiple times at different quality levels (as in Salsify~\cite{salsify}). 
Similar to~\cite{salsify}, \name encodes a frame multiple times at different quality levels but does so faster than encoding the frame from scratch for multiple times 
% doing the whole encoding process on a frame multiple times 
(illustrated in Figure~\ref{fig:speedup}(b)). 
\name trains multiple autoencoders each with a different $\alpha$ (in Eq.~\ref{eq:2}) to achieve different quality/size tradeoff.
\edit{During the training phase, modifications were confined to the residual encoders and decoders, while other NN weights remained fixed. 
Thus, once a frame is encoded, both the motion vector (MV) and residual are reusable, with the residual undergoing further encoding through different encoders each producing a different frame size. 
This procedure, taking under 3ms, can encode a frame multiple times via residual encoders of distinct $\alpha$ values. Residual sizes in practice can span from 0.1$\times$ to 10$\times$ the MV size, thereby allowing \name to encompass a wide range of bitrates (see to \S\ref{subsec:eval:resilience}).}
%but when we train these autoencoders, we {\em only} change their residual encoders and decoders, while freezing the weights of the MV encoder and decoder NNs.
%As a result, once a frame is encoded once, we can re-use the MV and residual but {\em only} re-encode the residual using a higher quality encoder, so encoding a frame the second time only takes less than 5ms. 
%This allows us to encode a frame multiple times (with the residual encoder of different $\alpha$s).
% Empirically, \name encodes each frame 1-2 times before getting a frame whose size is the highest but below the target frame size.

%Fortunately, we show that on a single NVIDIA GeForce 3080 GPU, \name's encoding speed can be greatly improved: from 5~fps on 720p HD (and 11~fps on 480p) videos by the off-the-shelf implementation to 18~fps (and 40~fps). More results in \S?????????\ref{subsec:eval:system}. 
%\name achieves such speedup by downsizing the image (by default 4×4\times) during motion-vector estimation and motion compensation, and then upsample the motion-compensated image before calculating and encoding the residuals. 
%This speeds up encoding because motion-vector estimation and motion compensation are the slowest steps during P-frame encoding and their delays are proportional to the input size.
%Thus, the overall encoding delay will be reduced if they are fed with downsized images. 
%At the same time, because the residuals are still computed between the full-resolution image and the motion-compensated image, the coding efficiency is not affected by this change for most frames.


\mypara{CPU-based speedup}
We have implemented a faster version of \name on CPUs.
% while preserving the loss-resilience autoencoder. 
It differs from the GPU-based autoencoder in two key aspects (Figure~\ref{fig:speedup}(c)): 
we (1) re-use the motion prediction logic in H.264 to generate MVs, and % (and re-train the encoder/decoder of both MV and residual), and
(2) remove the frame prediction NN from the motion compensation step. 
As a result, with 32 threads, it takes 35ms to encode a 720p HD frame (and 17.2ms on 480p) on Intel Xeon 4216 CPU. \passed{\yc{need ziyi's input, how many threads?}} %\jc{on what CPUs?}. 
As shown in \S\ref{subsec:eval:system}, the resulting autoencoder has slightly worse compression efficiency, but still achieves low frame delay in the presence of packet loss.
% obtains most of the benefit of a data-scalable coding system (\eg low frame delay in the presence of packet loss). 


\mypara{GPU-based speedup}
We use two ideas to speed up autoencoder on GPUs: 
(1) it uses Pytorch's just-in-time compiler~\cite{torchcompile} to optimize the NN encoder and NN decoder, and 
(2) it reduces the NN float-point precision from 32-bit to 16-bit. %\jc{Yihua/Ziyi, of all NNs or some NNs?} \zy{added}
As shown in \S\ref{subsec:eval:system}, on an NVIDIA A40 GPU, our implementation speeds up the encoder from 19.8 fps on 720p HD (and 39.5 fps on 480p) videos by the off-the-shelf implementation to 31.2 fps (and 87.7 fps on 480p), roughly a 1.5$\times$ speedup. More results in \S\ref{subsec:eval:system}.
This speed is on par with the speed-optimized proprietary autoencoders~\cite{elf}, and it still achieves desirable loss resilience and compression efficiency.
\passed{\amz{An obvious question here is "why not use the same optimization from CPU's MV on the GPU's NVENC"? I expect it would not actually provide a big benefit, since using the NVENC hardware on the GPU during inference will likely incur additional data movement between buffers, but if there’s a way you can head off that inquiry that might help. If you haven't tried it maybe add such an optimization as future work?} \yc{opticflow accelerator: https://developer.nvidia.com/blog/harnessing-the-nvidia-ada-architecture-for-frame-rate-up-conversion-in-the-nvidia-optical-flow-sdk/}}




%\mypara{Downscaling motion-vector operations}

\begin{comment}
\mypara{Speeding up on GPUs}
Most of the delay of \name's encoder and decoder can be attributed to motion related operations, including motion estimation, motion vector (MV) encoding, MV decoding, and motion compensation (see Figure~??????\ref{fig:dvc-arch}). 
%For example, to encode and decode a 720p frame (1280x720) on a \fillme GPU, these motion-related operations take \fillme\% of encoding delay and \fillme\% of decoding delay. 
Since most operations in MV encoding and decoding are mostly convolutional, \name speeds up these motion-related operations by downscaling the MV (by 4×4\times, by default) which speeds up the MV encoding and decoding by 4×\times.
In addition, \name uses Pytorch's just-in-time compiler to optimize the implementation of the encoder and decoder. 
\end{comment}


%At the same time, because the residuals are still computed between the full-resolution image and the motion-compensated image, the coding efficiency is not affected by this change for most frames.


%\name speeds up the encoding and decoding of its autoencoders 
%
%%\begin{packeditemize}
%%\item {\em Downscaling motion vectors:} 
%
%Since most motion-related operations are convolutional, their compute overheads are proportional to the dimension of the input frames. 
%Thus, \name speeds up motion-related operations by downsizing ($4\times$ in default) the input frame and the reference frames, and then upscale the motion-compensated image to compute the full-scale residual.
%%\item {\em Efficient bitrate control}
%%\end{packeditemize}




%\tightsubsection{Bitrate control}





%\jc{yihua, ziyi, fill in the text}




\begin{comment}

As a video coding system, the target frame size for \name to encode a frame is determined by an external adaptation, such as GCC, typically to match the estimated throughput.
To cope with fluctuations of network condition, throughput estimation can vary even between two consecutive frames.
As a result, \name should encode each frame at a size barely below the target frame size.
%This has been a challenge with traditional codecs.
%Thus, it is important that most frames are smaller than the target size set by congestion control, but traditional codecs are not able to do that. 
%This has been observed in \cite{salsify}, which proposes to encode each frame at multiple quality levels in order to find an encoding that fits the target bitrate. 

To encode frame at a size below a given target, \name employs a bitrate-control method similar as~\cite{salsify} and encodes each frame twice and picks the frame that has the closest size to the target. 
To do so, we need to (1) train multiple autoencoders whose frame sizes cover a wide range, and (2) run two of them as fast as possible. 

% to encode a frame with a maximum size below a target. 
First, \name trains multiple autoencoders, each using a different weight of frame size $\alpha$ in its training loss function (\S\ref{subsec:sim-losses}).
These resulting autoencoders cover a range of bitrate range. \jc{some numbers}
%\fillme$\times$ difference between the highest bitrate and lowest bitrate. (A wider bitrate range is possible with more autoencoders.)
As long as the target bitrate is within this range, \name should be able to select the autoencoder whose encoded frame size is barely lower than the target. 

Next, \name avoids the excessive compute overhead by re-using the motion-compensated image to get the residuals, and only run different versions of residual encoders to encode the residuals with different bitrates.
Since residual encoder is faster than the motion estimation and compensation, the speed up is significant. \jc{some numbers}
%A naive solution will run multiple autoencoders (like~\cite{salsify}), but the compute overhead will increase linearly.
%Fortunately, we can again re-use 

\jc{explain hanchen's bitrate control logic}

\end{comment}




% Figure~\ref{fig:e2e} puts the various pieces of \name in an end-to-end workflow, and  Table~\ref{tab:mapping} summarizes the effect of each components of \name. 

%generates the downscaled motion-vector coded tensor (\S\ref{??}) and the I-patch coded tensor (\S\ref{??}).
%It then uses the bitrate controller (\S\ref{??}) to pick the residual encoder NN so that the resulting frame size closely matches the target bitrate. 
%On the receiver side, \name uses the logic described in \S\ref{??} to determine when to decode a frame.

%\mypara{Relationship with congestion control}
\name is {\em complementary} to existing congestion control (CC) algorithms. 
When combined with \name, the CC algorithm does {\em not} need to retransmit packets, unless no packets of a frame are received.
%The choice of the congestion control (CC) logic is {\em complementary} to \name.
CC determines how fast the packets should be sent out and the target bitrate of the next frame, whereas \name decides what should be in each packet. 
\S\ref{app:salcc} evaluates \name with GCC in WebRTC~\cite{carlucci2016analysis} and Salsify CC~\cite{salsify}. 
\S\ref{app:webrtc} discusses how to integrate \name in WebRTC.
% to run with the GCC algorithm while disabling the packet retransmission.
%Since it does not change the CC logic, \name can be readily integrated in WebRTC. We will discuss details .






%\jc{need an end-to-end figure here}


%\begin{figure}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.99\linewidth]{figs/technique-mapping.pdf}
%    \tightcaption{}
%    \label{fig:technique-mapping}
%\end{figure}



\begin{comment}

At a high level, the \name encoder and decoder feed packets to congestion control (CC) which determines how fast the packets should be sent out and the target bitrate (size) of the next frame. 
\name can work with different CC logics that have this interface.
These include GCC~\cite{??} and Salsify's CC logic~\cite{??} both of which are used as CC when we test \name and other video codecs in \S\ref{sec:eval}.
It should be noted that \name does not use FEC. 



\mypara{Interaction with transport layers}
%\name is built on the data-scalable autoencoder \name. 
%\name is a concrete real-time video communication system built on a data-scalable autoencoder (\name).
We focus on unique issues arising from the use of \name as the codec, including how to deliver each frame to strike a desirable delay-quality tradeoff, and how to deliver a sequence of frames when congestion or packet losses affect multiple frames. 
The choice of the congestion control logic is complementary to \name. 
In \S\ref{subsec:eval:e2e}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{carlucci2016analysis} or Salsify CC~\cite{salsify}. 
We do not claim that \name's strategies are new (\eg reference frame synchronization has been used in~\cite{salsify}). 
Nonetheless, \name integrates concrete design choices driven by the need, in order to unleash the full potential of \name and its data-scalable codec primitive.


\jc{interface?}

\end{comment}
%\jc{TODO}









==> sections/old/protocol_v7.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US






\tightsection{Real-time video delivery over \newae}
\label{sec:delivery}

%\jc{
%\begin{itemize}
%\item coding of i-frames (compression)
%\item bitrate control (speed)
%\item speedup on cpu (speed)
%\item end-to-end protocol (why no synchronization, interaction with tcp and abr) (resilience)
%\end{itemize}
%}

%\jc{a table mapping the techniques to effects
%\begin{itemize}
%\item compression: i-frames, per-packet entropy
%\item speed: bitrate control, cpu speedup
%\item resilience: retraining, end-to-end protocol
%\end{itemize}
%}

This section addresses several practical challenges of \name, focusing on its coding speed and streaming protocol. 

\tightsubsection{Efficient coding and bitrate control}
\label{subsec:fast-coding}

%\tightsubsection{Reducing compute overhead}

%\mypara{Speed bottleneck}
Most research on autoencoder focuses on compression (using fewer bits to get higher quality), but their encoding and decoding are typically slower than the heavily-engineered standard codecs like H.264.
In the autoencoder of \name, the delay to encode and decode a frame is mostly attributed to motion related operations, including motion estimation, motion vector (MV) encoding, MV decoding, and motion compensation (see Figure~\ref{fig:dvc-arch}). 
For example, to encode and decode a 720p frame on a \fillme GPU, these motion-related operations take \fillme\% of encoding delay and \fillme\% of decoding delay. 

%Fortunately, we show that on a single NVIDIA GeForce 3080 GPU, \name's encoding speed can be greatly improved: from 5~fps on 720p HD (and 11~fps on 480p) videos by the off-the-shelf implementation to 18~fps (and 40~fps). More results in \S\ref{subsec:eval:system}. 
%\name achieves such speedup by downsizing the image (by default $4\times$) during motion-vector estimation and motion compensation, and then upsample the motion-compensated image before calculating and encoding the residuals. 
%This speeds up encoding because motion-vector estimation and motion compensation are the slowest steps during P-frame encoding and their delays are proportional to the input size.
%Thus, the overall encoding delay will be reduced if they are fed with downsized images. 
%At the same time, because the residuals are still computed between the full-resolution image and the motion-compensated image, the coding efficiency is not affected by this change for most frames.


\mypara{Downscaling motion-vector operations}
Because most layers in the motion-related operations are convolutional, their compute overheads are proportional to the dimension of the input frames. 
Inspired by this, \name speeds up motion-related operations by downsizing ($4\times$ in default) the input frame and the reference frames, and then upscale the motion-compensated image to compute the full-scale residual.
For example, on a single NVIDIA GeForce 3080 GPU, the downscaling of motion input can speed up the \name encoding speed from 5~fps on 720p HD (and 11~fps on 480p) videos by the off-the-shelf implementation to 18~fps (and 40~fps). More results in \S\ref{subsec:eval:system}. 
At the same time, because the residuals are still computed between the full-resolution image and the motion-compensated image, the coding efficiency is not affected by this change for most frames.


%\tightsubsection{Bitrate control}


\mypara{Speed-up on CPUs}
Besides optimizing \name's coding speed on a GPU, we have also implemented a faster version of \name which runs at \fillme ms per frame on CPUs. 
\jc{yihua, ziyi, fill in the text}


\mypara{Efficient bitrate control}
As a video coding system, the target frame size for \name to encode a frame is determined by an external adaptation, such as GCC, typically to match the estimated throughput.
To cope with fluctuations of network condition, throughput estimation can vary even between two consecutive frames.
As a result, \name should encode each frame at a size barely below the target frame size.
%This has been a challenge with traditional codecs.
%Thus, it is important that most frames are smaller than the target size set by congestion control, but traditional codecs are not able to do that. 
%This has been observed in \cite{salsify}, which proposes to encode each frame at multiple quality levels in order to find an encoding that fits the target bitrate. 

To encode frame at a size below a given target, \name employs a bitrate-control method similar as~\cite{salsify} and encodes each frame twice and picks the frame that has the closest size to the target. 
To do so, we need to (1) train multiple autoencoders whose frame sizes cover a wide range, and (2) run two of them as fast as possible. 

% to encode a frame with a maximum size below a target. 
First, \name trains multiple autoencoders, each using a different weight of frame size $\alpha$ in its training loss function (\S\ref{subsec:sim-losses}).
These resulting autoencoders cover a range of bitrate range. \jc{some numbers}
%\fillme$\times$ difference between the highest bitrate and lowest bitrate. (A wider bitrate range is possible with more autoencoders.)
As long as the target bitrate is within this range, \name should be able to select the autoencoder whose encoded frame size is barely lower than the target. 

Next, \name avoids the excessive compute overhead by re-using the motion-compensated image to get the residuals, and only run different versions of residual encoders to encode the residuals with different bitrates.
Since residual encoder is faster than the motion estimation and compensation, the speed up is significant. \jc{some numbers}
%A naive solution will run multiple autoencoders (like~\cite{salsify}), but the compute overhead will increase linearly.
%Fortunately, we can again re-use 

\jc{explain hanchen's bitrate control logic}




%\jc{TODO}







\tightsubsection{Streaming protocol}
\label{subsec:protocol}


%\mypara{I-frame coding and state synchronization}
\mypara{I-frame coding}
Placement of I-frames poses a particular challenge for \name's autoencoders (both pre-trained and re-trained), because while the first few P-frames after an I-frame enjoy high quality, quality gradually degrades after about 10 frames. 
%for two reasons: (1) I-frames are generally bigger in size than P-frames, and 
%(2)  while the first few P-frames after an I-frame enjoy high quality, quality gradually degrades after about 10 frames. 
A strawman would add I-frames frequently (say every 10 frames)\footnote{Many computer-vision papers on autoencoders have conveniently used a small GoP when compared against H.265, but the implication of large I-frame size for congestion control is rarely discussed.}.
Even though this might achieve a decent tradeoff between quality and {\em average} bitrate (comparable to H.264 and H.265 with large I-frame intervals), sending I-frames (which have bigger sizes than the P-frames in between) frequently will make it difficult for congestion control to send the frames at a fixed interval (inversely proportional to the frame rate).

%\tightsubsection{Encoding a sequence of frames}
%\label{subsec:delivery:iframe}

%To stream a sequence of video frames, a key question is how often I-frames should be inserted in P-frames. 
%(As explained in \S\ref{subsec:ae-background}, \name uses only I-/P-frames, as in most real-time video systems.)
%For the P-frame autoencoder we have tried, we observe that the decoded quality can be very high right after each I-frame but it gradually degrades after about 10 frames. 


To add I-frames frequently without the intermittent bitrate spikes caused by the I-frames, \name encodes a small patch (about 128$\times$128 to 512$\times$512) as a tiny I-frame, which we call {\em I-patch}, on {\em every frame} (the pixels outside the I-patch will be encoded as a P-frame), and the location of the I-patch on a frame changes over time such that the I-patch will scan through the whole frame size every $k$ frames. 
Depending on the original frame size, $k$ varies between 6 and 20. 
This scheme effectively ``amortizes'' the size of I-frames across $k$ frames, thus smoothing the frame size as well as quality across frames (illustrated in Figure~\ref{fig:keyframe_smooth}).
Moreover, since the I-frame autoencoder's encoding delay is proportional to the input size, encoding a small I-patch adds only a small compute overhead for each frame.\footnote{We should clarify that design choice of frequent I-frames works well for autoencoders, but {\em not} for classic codecs for two reasons. First, an I-frame generated by our autoencoder is only 2-5$\times$ bigger than a P-frame, whereas this ratio in H.264 is 4-10$\times$. Second, the P-frame quality in H.264 is relatively stable, whereas the quality of a P-frame is high following an I-frame (or an I-patch).}


\begin{figure}[t!]
    \centering
    
        \includegraphics[width=0.85\linewidth]{figs/split-iframe-size.pdf}
    \tightcaption{Encoding each P-frame with a small I-patch leads to smoother frame sizes than naively inserting I-frames.}
    \label{fig:keyframe_smooth}
\end{figure}

\jc{need a paragraph to explain why frequent i-patches actually make a lot of sense}


\jc{how to deal with scene change?}


An important benefit of adding an I-patch (a tiny patch encoded as an I-frame without referring to previous frames) at a different place in each frame is: each patch will be encoded as an I-patch every $k$ frames. 
This means that \name can use the frequent I-patches (explained in \S\ref{subsec:delivery:iframe}) to synchronize the encoding/decoding states in each patch-size region. 
This works for two reasons.
First, without synchronizing the encoding and decoding states, \newae's quality degradation increases only marginally when multiple consecutive frames (less than about 10) are affected by packet losses.
For instance, applying a 50\% packet loss rate on one single frame can reduce PSNR by 3-4, and applying the same loss rate on 5 consecutive frames reduces PSNR by 7-9. 
%\jc{this corroborates our empirical improvements in \S\ref{??}}
%quality degrades by \fillme\% when 10 consecutive frames are affected by 50\% packet losses without the clients synchronizing their encoding/decoding states. 
Second, each patch will be encoded as an I-patch every $k$ frames ($k$ is between 6 and 20), so the impact of packet losses will not last for more than $k$ frames if the next I-patch is not lost. 
That said, in the worst case, if the I-patches of the same region are dropped persistently, this could cause bad decoded pixel values (\ie a small patch of white pixels), though we have observed it extremely rarely.



%This has a significant implication for loss resilience over multiple consecutive frames. 
%This allows \name to use a simple yet efficient solution---it does not always synchronize the encoding/decoding state on every single frame; instead, it relies 
%
%An acute reader may realize a potential problem arising from encoding and decoding being asynchronous. 
%For instance, when the sender encodes the $10^{\textrm{th}}$ frame as a P-frame, it needs the decoded the $9^{\textrm{th}}$ frame as the reference (to compute motion vectors and residuals), and without knowing which of the $9^{\textrm{th}}$ frame's packets will be lost, it will assume that the $9^{\textrm{th}}$ frame is decoded with all packets being received. (This is common to classic codecs and autoencoders.)
%However, if the receiver decodes the $9^{\textrm{th}}$ frame with only a subset of its packets, the actual reference frame used to decode the $10^{\textrm{th}}$ will differ from what the encoder has assumed. 
%Thus, most codecs require all packets of the $9^{\textrm{th}}$ frame to be received before decoding it (thus longer delay), or let the sender encode the $10^{\textrm{th}}$ based on an earlier reference (say the $5^{\textrm{th}}$) whose lost packets are already known to the sender. 
%The latter {\em synchronizes} the encoding and decoding states (like in Salsify~\cite{salsify} during packet losses), but it also inflates the frame size, since the difference between the $10^{\textrm{th}}$ and the $5^{\textrm{th}}$ frames  is much greater than between the $10^{\textrm{th}}$ and the $9^{\textrm{th}}$ frames. 








\mypara{Timing for decoding}
%\mypara{Choosing when to decode a frame}
The data-scalable abstraction allows the receiver to flexibly decide, as packets arrive at the receiver, whether to decode the frame using currently arrived packets or wait for more packets in hope of improving the quality. 
(In contrast, with FEC, the receiver will always wait until enough data is received.)
%(In other loss-resilient schemes (\S\ref{??}), the receiver must wait for more packets until the data is decodable.) 
%\name embraces this flexibility with the following logic to trade frame delay with decoded quality. 


\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.995\linewidth]{figs/decode_time.pdf}
        \includegraphics[width=0.995\linewidth]{figs/decode_time_v2.pdf}
    \tightcaption{
    \name waits for the next frame until a deadline $t^*$, after which the utility is lower even if the next packet arrives. }
    \label{fig:decode-time}
\end{figure}

To make this decision, \name defines the {\em utility} of a frame as a linear combination of decoding quality and frame delay (since the natural decoding time) on each frame: $Q(|\{\textrm{pkts before }t\}|)-\beta\cdot t$, where $t$ is when the frame is decoded, $Q(n)$ is the frame's decoding quality with $n$ packets 
The precise values of $Q(n)$ are frame-dependent, but they are roughly similar across frames, so \name estimates $Q(n)$ using history frames.
%, and $\tau$ is the frame's natural decoding time (\eg 40ms after the last frame was decoded with frame rate 25fps).
%In our experiment, we set parameter $\beta=\fillme$.
This objective works well in practice, though there might be other objectives that better capture users' quality perception. An optimal design of such utility is beyond the scope of this paper. 

With this utility in mind, Figure~\ref{fig:decode-time} illustrates \name's logic: on receiving the $i^{\textrm{th}}$ packets of a frame (not necessarily the $i^{\textrm{th}}$ sent packet) at time $t_i$, the receiver will immediately decode the frame if all packets of the frame have arrived; otherwise, it will wait for the next packet of the frame until a deadline $t^*=t_i+\frac{1}{\beta}\cdot(Q(i+1)-Q(i))$, and if it has not received the $(i+1)^{\textrm{th}}$ packet by then, it will decode the frame with $i$ packets. 
The reason is that if the next packet comes at time $t_{i+1}$ after $t^*$, the utility $Q(i+1)-\beta\cdot (t_{i+1}-\tau)$ will be lower than the utility $Q(i)-\beta\cdot (t_i-\tau)$ if the receiver does not wait at all\footnote{This is because {\scriptsize $Q(i+1)-\beta\cdot (t_{i+1}-\tau)<Q(i+1)-\beta\cdot (t^*-\tau)=Q(i)-\beta\cdot (t_i-\tau)$}}. 
%Here, $\beta$ is a tunable parameter, and $Q(n)$ is the quality of the frame based on $n$ packets.
This strategy makes intuitive sense: the receiver will wait longer if the improvement in quality by getting one more packet (\ie $Q(n+1)-Q(n)$) is higher, but it will not wait for too long.



\mypara{Interaction with transport layers}
%\name is built on the data-scalable autoencoder \newae. 
%\name is a concrete real-time video communication system built on a data-scalable autoencoder (\newae).
We focus on unique issues arising from the use of \newae as the codec, including how to deliver each frame to strike a desirable delay-quality tradeoff, and how to deliver a sequence of frames when congestion or packet losses affect multiple frames. 
The choice of the congestion control logic is complementary to \newae. 
In \S\ref{subsec:eval:e2e}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{carlucci2016analysis} or Salsify CC~\cite{salsify}. 
We do not claim that \name's strategies are new (\eg reference frame synchronization has been used in~\cite{salsify}). 
Nonetheless, \name integrates concrete design choices driven by the need, in order to unleash the full potential of \newae and its data-scalable codec primitive.


\jc{interface?}

%\ding{52}



\tightsubsection{Putting the pieces together}

\mypara{End-to-end workflow}
Figure~\ref{fig:e2e} puts together the various techniques of \name in an end-to-end workflow. 
At a high level, the \name encoder and decoder feed packets to congestion control (CC) which determines how fast the packets should be sent out and the target bitrate (size) of the next frame. 
\name can work with different CC logics that have this interface.
These include GCC~\cite{??} and Salsify's CC logic~\cite{??} both of which are used as CC when we test \name and other video codecs in \S\ref{sec:eval}.
It should be noted that \name does not use FEC. 

On the encoder side, \name first generates the downscaled motion-vector coded tensor (\S\ref{??}) and the I-patch coded tensor (\S\ref{??}).
It then uses the bitrate controller (\S\ref{??}) to pick the residual encoder NN so that the resulting frame size closely matches the target bitrate. 
On the receiver side, \name uses the logic described in \S\ref{??} to determine when to decode a frame.

%\jc{need an end-to-end figure here}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.97\linewidth]{figs/e2e.pdf}
    \tightcaption{}
    \label{fig:e2e}
\end{figure}

%\begin{figure}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.99\linewidth]{figs/technique-mapping.pdf}
%    \tightcaption{}
%    \label{fig:technique-mapping}
%\end{figure}

\begin{table}[]
\small
\begin{tabular}{cccc}
\hline
                                                                                      & \begin{tabular}[c]{@{}c@{}}Loss\\ Resilience\end{tabular} & \begin{tabular}[c]{@{}c@{}}Compression\\ Efficiency\end{tabular} & \begin{tabular}[c]{@{}c@{}}Coding \\ Speed\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}Training NN coders with\\random data erasure (\S\ref{subsec:retraining})\end{tabular} & \ding{52}                                                 &                                                                  &                                                         \\ \hline
\begin{tabular}[c]{@{}c@{}}Per-packet entropy\\ coding (\S\ref{subsec:per-packet})\end{tabular}                  & \ding{52}                                                 & \ding{52}                                                        &                                                         \\ \hline
\begin{tabular}[c]{@{}c@{}}Motion operations on \\ downscaled input (\S\ref{subsec:fast-coding})\end{tabular}      &                                                           & \ding{52}                                                        & \ding{52}                                               \\ \hline
\begin{tabular}[c]{@{}c@{}}Bitrate control by reusing\\motion vector (\S\ref{subsec:fast-coding})\end{tabular}    &                                                           &                                                                  & \ding{52}                                               \\ \hline
\begin{tabular}[c]{@{}c@{}}I-frame coding by \\ moving I-patches (\S\ref{subsec:protocol})\end{tabular}         & \ding{52}                                                 &                                                                  &                                                         \\ \hline
\end{tabular}
\end{table}

\mypara{Integration in WebRTC}
\name is implemented with 3K lines of code, in both Python (mostly for autoencoder NNs) and C++ (for frame delivery and WebRTC integration). The code and trained model of \name will be made public upon the publication of this paper.
The integration with WebRTC is logically straightforward since \newae (including I-frame and P-frame encodings) exposes similar interface as the default codec in WebRTC. 
%\jc{Ziyi, please fill in the details}

We substitute the libvpx VP8 Encoder/Decoder in WebRTC with our \newae implementation. When the sender encodes a frame, it parses the image data from the \texttt{VideoFrame} data structure (YUV format) into \texttt{torch.Tensor} (RGB format) and feed it into our \newae encoder, which will return the encoded result as a byte array. Then the encoded bytes are stored into an \texttt{EncodedImage} (class in WebRTC) and sent through the network to the receiver as RTP packets. 
% \zy{I could also add several sentences about packetization logic (commented out below)}
% The encoded bytes are then packetized as RTP packets and sent through the network to the receiver. 
We modify the built-in \texttt{RtpVideoStreamReceiver} (class in WebRTC) so that the receiver could flexibly decode the received packets even when not all the packets are received. When the receiver decides to decode the frame, it depacketizes the received packets into encoded data. Then it will use the \newae decoder to decode the image into RGB format and then convert it back to YUV for displaying on the receiver side.

%\newpage
%
%
%\tightsubsection{Streaming protocol}






%If a packet comes, the utility will be $Q(n)-1/\beta\cdot \beta\cdot(Q(n+1)-Q(n))$






%\jc{need to explain the gains are not directly from the entropy encoder or motion vector estimation}


\begin{comment}

\tightsubsection{Optimizations}
\label{subsec:optimize}

While \newae is functionally similar to traditional codecs, it faces a few technical challenges to function as the codec in a real-time video client.
Note that these challenges are not specific to loss resilience, so we do not consider packet losses in the rest of the section. 






\mypara{Reducing memory footprint}
For the client to switch between multiple autoencoders (with different bitrates), their memory footprint should be minimized, so more of them can be loaded into GPU memory to avoid the delay of loading and unloading models. 
\name trains multiple autoencoders by fine-tuning the last 10-25\% layers of the same model (\ie they share the backbone layers), so only the one autoencoder and the last few layers of different autoencoders need to be loaded in GPU memory. 
This reduces the memory footprint of the models by 60\% compared to when all models are trained separately without sharing any layers.
A similar idea has also been used in Swift~\cite{swift} in multiple SVC layer encoders.

\end{comment}




==> sections/old/protocol_v8.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US





\tightsection{Real-time video framework}
\label{sec:delivery}

%\jc{
%\begin{itemize}
%\item coding of i-frames (compression)
%\item bitrate control (speed)
%\item speedup on cpu (speed)
%\item end-to-end protocol (why no synchronization, interaction with tcp and abr) (resilience)
%\end{itemize}
%}

%\jc{a table mapping the techniques to effects
%\begin{itemize}
%\item compression: i-frames, per-packet entropy
%\item speed: bitrate control, cpu speedup
%\item resilience: retraining, end-to-end protocol
%\end{itemize}
%}

The new autoencoder described in \S\ref{sec:core} can achieve data-scalable (DS) coding on a {\em single} frame under simulated packet loss. 
This section presents \name's online video delivery framework. 
In particular,
\begin{packeditemize}
\item How to entropy encode autoencoder output into packets (\S\ref{subsec:packetization}), 
\item How to stream a sequence of frames (\S\ref{subsec:protocol}), and
\item How to speed up encoding/decoding on GPUs and CPUs without sacrificing loss resilience (\S\ref{subsec:fast-coding}).
\end{packeditemize}
% \yc{I moved entropy coding to 4.1, since I feel this is more smooth: first talking about tensor -> packets for each frame, then discuss how we stream sequence of frames, finally some optimizations}

\tightsubsection{Entropy encoding the encoder's output}\label{subsec:packetization}
Like classic codecs of H.264 and VP9, the NN encoder's output tensor also needs to be losslessly compressed into a bitstream using an arithmetic (entropy) coding scheme.
An arithmetic encoder uses an underlying symbol distribution to compress the value at each position of the tensor.
Unlike classic codecs that use hand-tuned heuristics like CABAC, autoencoders, including DVC, often train the value distribution jointly with the NN encoder and decoder to learn a better distributional representation of the values in the NN encoder output. 
Since the decoder later uses the same symbol distributions to recover the tensor, the symbol distribution is also sent together with the data. 
However, because \name divides the encoder's output tensor into subtensors, each being separately entropy encoded into a packet, thus each packet must include a copy of its own symbol distribution.
This will greatly increase the size if the data of a frame is split into many packets. 

We reduce this per-packet overhead by carefully choosing the precision of symbol distribution, which governs the tradeoff between the size of a symbol distribution and the size of the entropy-encoded data.
A coarser-grained symbol distribution needs fewer bits to store, but it may yield a higher size of the entropy-encoded data. 
\name's insight is that we can train the NN encoder in a way that regularizes the distribution of values in each encoder's output channel to conform to a zero-mean Laplace distribution. 
(Each encoder output tensor has 224 channels.)
This way, the symbol distribution only needs to store the variance within each channel while still perfectly compressing the encoder output tensor. 
As a result, the symbol distribution takes only $\sim$50 bytes to store per packet (a reduction from 40\% of the packet size to 5\%), without hurting the compression efficiency of entropy coding.

\begin{comment}
\tempstrike{
As described in \S\ref{sec:core}, \name uses a reversible pseudo-random mapping to divide the encoder's output tensor into packets. 
Practically, we further compress each packet's subtensor into a more compact bytestream via individual entropy encoding, reducing the bytes transmitted through the network.

Similar to traditional codecs and prior autoencoders~\cite{dvc}, \name uses arithmetic coding~\cite{??} to entropy encode the subtensor into a compressed byte stream. 
The entropy encoder takes two inputs: the subtensor itself and the distribution for each element in the subtensor. 
To correctly decode the original subtensor at the decoder side, the distribution should also be sent to the receiver in the same packet.
It is worth noting that there is a trade-off between the size of the encoded subtensor and the size of the distribution:
The size of the entropy-encoded subtensor will be smaller if the distribution is closer to the real distribution of the subtensor, however, it may significantly increase the size of the distribution, resulting in worse compression efficiency.
\name mitigates this during training by regularizing each coded tensor channel's distribution to conform to a zero-mean Laplace distribution. 
Furthermore, the variance of each channel can be efficiently represented using minimal bits, adding a trifling overhead of approximately 50 bytes per packet. \yc{``overhead'' may not be a good word here?} 

To get the distribution during runtime, traditional codecs, like H.264, use a hard-coded distribution table~\cite{??cabac} for different input elements.
In contrast, \name uses a small neural network to estimate the variance of each channel. This small neural network is also jointly trained with the encoder during training, making it able to estimate the distribution more accurately.
TTo ensure each entropy-encoded packet aligns with a predetermined packet size, \name estimates the frame size prior to partitioning the output tensor into subtensors, by calculating the distribution's entropy. The accuracy of this size estimation is reinforced by the consistent use of the same distribution for entropy encoding the tensor\yc{we should explain why the estimated size is accurate, but this sentence is not clear}. 
In practice, the error of the estimated distribution is never larger than 2\%.
}
\end{comment}


\tightsubsection{Streaming protocol}
\label{subsec:protocol}

% To extend the P-frame DS autoencoder trained in \S\ref{subsec:training} for multiple frames, the first challenge is potential out-of-sync {\em states} between the encoder and decoder when packet loss occurs.
%Two challenges arise when extending the P-frame DS autoencoder trained in \S\ref{subsec:??} to the delivery of multiple frames: (1) potential out-of-sync coding state between the encoder and decoder when packet loss occurs, and (2) how to encode I-frames and how frequently to add I-frames.



\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v3.pdf}
        % \includegraphics[width=0.99\linewidth]{figs/state-sync-v2.pdf}
        \includegraphics[width=0.92\linewidth]{figs/state-sync-v3.pdf}
    \tightcaption{Examples of how to deal with loss-affected frames: 
    (a) delayed by retransmission, (b) ignoring out-of-sync encoder/decoder states, and (c) 
    \name's frame optimistic encoding and state re-sync.}
    \label{fig:state-sync}
    \vspace{-0.1cm}
\end{figure}

\mypara{Basic protocol}
The \name encoder encodes a new frame with a fixed interval, and % (by default, 40ms or 25fps).
the decoder tries to decode a frame when the first packet of the next frame is received using the following logic:
\begin{packeditemize}
\item If no packet of the current frame is received, then it will request the sender to send the frame again;
\item Otherwise (at least one packet of the current frame is received), then it will decode the frame.
%\item If a subset of the packets of the current frame are received, then it will decode the frame and send a ``re-sync'' signal to the sender.
\end{packeditemize}

%\mypara{Encoding reference state}
However, if we directly replace the traditional codec with the new autoencoder, it could cause low quality on a frame even if all of its packets arrive on time. 
This is because if a reference frame is decoded using a subset of packets, the state will be ``out-of-sync'' between the encoder and decoder---the reference image used to encode the next frame is different from the reference used by the decoder.
% This can affect all subsequent frames if not handled appropriately.
% Figure~\ref{fig:state-sync} shows an example. 
In standard video coding, to encode the $7^{\textrm{th}}$ frame, the sender uses the decoded result of the $6^{\textrm{th}}$ frame as the reference to compute motion vectors and residual of the $7^{\textrm{th}}$ frame, and the receiver will use the same reference frame to decode the $7^{\textrm{th}}$ frame. 
However, if the receiver uses \name autoencoder to decode the $6^{\textrm{th}}$ frame using only a subset of its packets (Figure~\ref{fig:state-sync}(a)), it will see a different reference frame when decoding the $7^{\textrm{th}}$ frame than what the encoder has assumed when encoding the $7^{\textrm{th}}$ frame.
Thus, even if all packets of the $7^{\textrm{th}}$ are received, its quality will be slightly lower than it should be.
Similarly, since the $7^{\textrm{th}}$ is also out of sync with the sender's state, the $8^{\textrm{th}}$ frame will suffer too, and so forth.
%In short, the quality of many frames with zero \rate might still be affected.

%the naive method of using \name (Figure~\ref{fig:state-sync}(b)) will affect quality degradation on frames that do not have 

%the reference frame used by the receiver to decode the 10th10^{\textrm{th}} frame will differ from what the encoder has assumed. 
%
%, and without knowing which of the 9th9^{\textrm{th}} frame's packets will be lost, it will assume that the 9th9^{\textrm{th}} frame is decoded with all packets being received. (This is common to classic codecs and autoencoders.)
%However, if the receiver decodes the 9th9^{\textrm{th}} frame with only a subset of its packets, the actual reference frame used to decode the 10th10^{\textrm{th}} will differ from what the encoder has assumed. 
%Thus, most codecs require all packets of the 9th9^{\textrm{th}} frame to be received before decoding it (thus longer delay), or let the sender encode the 10th10^{\textrm{th}} based on an earlier reference (say the 5th5^{\textrm{th}}) whose lost packets are already known to the sender. 
%The latter {\em synchronizes} the encoding and decoding states (like in Salsify~\cite{salsify} during packet losses), but it also inflates the frame size, since the difference between the 10th10^{\textrm{th}} and the 5th5^{\textrm{th}} frames  is much greater than between the 10th10^{\textrm{th}} and the 9th9^{\textrm{th}} frames. 


%\begin{figure*}[t!]
%    \centering
%         \centering
%%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v3.pdf}
%        \includegraphics[width=0.9\linewidth]{figs/state-sync-v1.pdf}
%    \tightcaption{}
%    \label{fig:per-packet}
%\end{figure*}


A strawman solution is that the encoder and decoder synchronize on each frame.
% ---if the receiver decodes a frame with a subset of packets, the sender should always know which packets are used in order to reconstruct the same reference frame seen by the decoder. 
However, this will negate the benefit of \name's generative autoencoder, as the sender will wait until the receiver acknowledges after each frame which takes at least an RTT.
% for the acknowledgment from the receiver (at least an RTT) after each frame, 

\mypara{Optimistic encoding with dynamic state re-sync}
%Rather than syncing-up the reference state every frame, 
Instead, \name lets the sender optimistically encode frames without syncing the coding states.
However, once receiving the feedback that the decoder decodes a frame using a subset of its packets, the sender will quickly re-decode the recent frames with the same decoded frame as seen by the decoder to reconstruct the same reference frame seen by the decoder. 
(Explained shortly, such re-decoding can be greatly sped-up.)
For instance, in Figure~\ref{fig:state-sync}(b), the sender is about to encode the $9^{\textrm{th}}$ when it gets the feedback that says the $6^{\textrm{th}}$ was decoded with a certain subset of packets, then the encoder will quickly re-decode the frames from the $6^{\textrm{th}}$ (with the same subset of packets) to $8^{\textrm{th}}$ frames and use the new decoded $8^{\textrm{th}}$ frame as the reference to encode the $9^{\textrm{th}}$ frame.




%\name's autoencoder can decode frames with inconsistent coding states for a handful of frames, though the quality will deteriorate over time if the coding state is left unsynced for too long. \jc{need a visualization in eval}
%However, our fast re-sync scheme makes sure that 

%The basic insight is that without synchronizing the reference frames, \name's autoencoder can decode frames with high quality for a handful of frames. \jc{need a visualization here}
%
%Therefore, the sender does not need to wait for the feedback from the receiver; instead, it can optimistically encode the next frame assuming the packets of the previous frames are completely received, until it receives a feedback from the receiver that a previous frame was not decoded with all packets (this feedback can be like an NACK in WebRTC).
%Suppose that the sender is about to encode the $9^{\textrm{th}}$ when it gets a feedback that says the $6^{\textrm{th}}$ was decoded with certain subset of packets (illustrated in Figure~\ref{fig:state-sync}(c)), then the encoder will quickly re-decode the frames from the $6^{\textrm{th}}$ to $8^{\textrm{th}}$ frames (this step can be greatly sped-up shortly), and use the new decoded $8^{\textrm{th}}$ frame as the reference to encode the $9^{\textrm{th}}$ frame.



A potential speed bottleneck is re-decoding reference frames (\eg from $6^{\textrm{th}}$ to $8^{\textrm{th}}$ frames in Figure~\ref{fig:state-sync}(c)) during re-sync. 
Fortunately, both the encoder and the decoder can re-decode these frames much faster than the normal decoding, by skipping both motion-estimation NN and the frame-prediction NN (Figure~\ref{fig:dvc-arch}).
This saves 93\% of encoding time per frame.
The insight is two-fold.
First, these frames have been decoded once, and the re-decoding simply needs to estimate the incremental changes caused by the lost packets, so it can be much faster. 
Second, skipping the frame-prediction NN does reduce the compression efficiency on the last frame (\eg the $9^{\textrm{th}}$ frame in  Figure~\ref{fig:state-sync}(c)), but it only affects only one frame.
The formal proof of why the re-decoding works can be found in \S\ref{app:resync}.%\jc{YIHUA!}

% re-synchronization does not have to have the highest quality, which allows us to skip the motion-smoothing NN in frame prediction. In addition, this is also a unique benefit of autoencoders.
% The formal proof can be found in \S\ref{??}.

\tempstrike{
    
% \footnote{\edit{The motion smoothing NN is trained to smooth the predicted frame, so that the residual will be smaller and thus easier to compress.}} 
% in the frame prediction \st{NN} \edit{step} (shown in Figure~\ref{fig:dvc-arch}), 
which takes up \fillme\% of the decoding time per frame. 
The new $8^{\textrm{th}}$ frame will be used to encode the $9^{\textrm{th}}$ frame in  Figure~\ref{fig:state-sync}(c), and when the receiver receives the encoded $9^{\textrm{th}}$ frame, it also re-decodes the frames from 6-8 {\em without} the \edit{motion-smoothing NN}.
% \st{frame prediction NN} (not shown in figure), 
Since both re-encoding and re-decoding skip the time-consuming motion-smoothing NN, the overhead is minimum 
but since this is much faster, it will not add much new overhead. 
The insight behind it is that re-synchronization does not have to have the highest quality, which allows us to skip the motion-smoothing NN in frame prediction. In addition, this is also a unique benefit of autoencoders.
%which is unique to the benefit of autoencoders

}

%allowing it to re-decode these frames using a different but faster method.
%The insight is that the decoding does not have to have the highest quality, which allows us to skip the motion-smoothing NN in motion compensation (Figure~\ref{??}) which significantly reduces the delay by \fillme\%.\jc{need a few words on why}
%For this optimization to work, the receiver also needs to re-decode the frames from 6-8 without the motion-smoothing NN, but since this is much faster, it will not add much new overhead. 

    

%, but it leverages the loss resilience of the new autoencoders.
% Like \name, NACK and Salsify allow senders to burst packets without waiting for acks, and when packet loss happens, NACK retransmits lost packets which delays the decoding of future frames and Salsify rewinds the encoder to an old state to generate the next P-frame, allowing the decoder to skip loss-affected frames.
% However, \name's key difference is that 

The dynamic state re-sync described above highlights a key advantage of \name's decoder---it does not need to skip or block the decoding of loss-affected frames; instead, it still decodes loss-affected frames with decent quality {\em before} encoder/decoder states are synchronized, so it reduces frame delay while maintaining decent quality. 
% This makes \name's optimistic encoding with dynamic state re-sync 
This is fundamentally different from  NACK (negative ack) in WebRTC (which blocks the decoding of loss-affected frames) and the encoder/decoder state synchronization in Salsify (which skips the loss-affected frames).
% , where the latter methods need to either wait for or skip the loss affected frames.

%Although \name's optimistic encoding with dynamic state re-sync may sound similar to NACK (negative ack) in WebRTC and the encoder/decoder state synchronization in Salsify, but it has a key difference. 
%The receiver in \name does not need to skip or block the decoding of loss-affected frames; instead can still decode loss-affected frames with decent quality before encoder/decoder states are synchronized, so it reduces frame delay while maintaining high quality. 
\passed{\amz{This is also framed in a roundabout way, but is also a key insight of this work IMO -- using your packetization allows for decoding lossy frames with less delay. Switching these sentences ("Another benefit of \name is that the receiver does not need to skip... This differentiates our dynamic state re-sync from NACK and Salsify")} \yc{reorganized the contents}}
%wait for the retransmission (in NACK) or the new P-frame (in Salsify) to decode the next frame frame; instead, it can still decode loss-affected frames with decent quality before encoder/decoder states are synchronized, so it reduces frame delay while maintaining high quality.


%Like NACK (negative ack) which WebRTC senders use to burst packets without waiting for acks until an NACK is received, 
%% from the receiver that some packets must be retransmitted in order to decode previous frames. 
%This is similar to Salsify which uses a similar on-demand re-sync scheme to use an old coding state to generate the next frame, allowing the decoder to skip loss-affected frames.
%However, the key difference is
%
%
% insight of on-demand re-sync is that the out-of-sync coding states will {\em affect only frames within an RTT}. 
%However, optimistic encoding with fast re-sync differ in that the receiver does not need to wait for the retransmission (in NACK) or the new P-frame (in Salsify) to decode the next frame frame; instead, it can still decode loss-affected frames with decent quality before encoder/decoder states are synchronized, so it reduces frame delay while maintaining high quality.


%\begin{itemize}
%\item synchronizing every frame will kill the benefit of DS
%\item however, the insight: its ok to be out of sync for a few frames
%\item idea: lazy synchronization. 
%\item to put it in perspective, salsify?
%\end{itemize}


%\jc{add a short para on when to decode a frame}
%
%\jc{what if all packets of a frame are lost}

\begin{comment}

\mypara{Balancing quality and frame delay}
%\mypara{Choosing when to decode a frame}
The data-scalable abstraction allows the receiver to flexibly decide, as packets arrive at the receiver, whether to decode the frame using currently arrived packets or wait for more packets in hope of improving the quality. 
(In contrast, with FEC, the receiver will always wait until enough data is received.)
%(In other loss-resilient schemes (\S\ref{??}), the receiver must wait for more packets until the data is decodable.) 
%\name embraces this flexibility with the following logic to trade frame delay with decoded quality. 



To make this decision, \name defines the {\em utility} of a frame as a linear combination of decoding quality and frame delay (since the natural decoding time) on each frame: $Q(|\{\textrm{pkts before }t\}|)-\beta\cdot t$, where $t$ is when the frame is decoded, $Q(n)$ is the frame's decoding quality with $n$ packets 
The precise values of $Q(n)$ are frame-dependent, but they are roughly similar across frames, so \name estimates $Q(n)$ using history frames.
%, and $\tau$ is the frame's natural decoding time (\eg 40ms after the last frame was decoded with frame rate 25fps).
%In our experiment, we set parameter $\beta=\fillme$.
This objective works well in practice, though there might be other objectives that better capture users' quality perception. An optimal design of such utility is beyond the scope of this paper. 

With this utility in mind, Figure~\ref{fig:decode-time} illustrates \name's logic: on receiving the $i^{\textrm{th}}$ packets of a frame (not necessarily the $i^{\textrm{th}}$ sent packet) at time $t_i$, the receiver will immediately decode the frame if all packets of the frame have arrived; otherwise, it will wait for the next packet of the frame until a deadline $t^*=t_i+\frac{1}{\beta}\cdot(Q(i+1)-Q(i))$, and if it has not received the $(i+1)^{\textrm{th}}$ packet by then, it will decode the frame with $i$ packets. 
The reason is that if the next packet comes at time $t_{i+1}$ after $t^*$, the utility $Q(i+1)-\beta\cdot (t_{i+1}-\tau)$ will be lower than the utility $Q(i)-\beta\cdot (t_i-\tau)$ if the receiver does not wait at all\footnote{This is because {\scriptsize $Q(i+1)-\beta\cdot (t_{i+1}-\tau)<Q(i+1)-\beta\cdot (t^*-\tau)=Q(i)-\beta\cdot (t_i-\tau)$}}. 
%Here, $\beta$ is a tunable parameter, and $Q(n)$ is the quality of the frame based on $n$ packets.
This strategy makes intuitive sense: the receiver will wait longer if the improvement in quality by getting one more packet (\ie $Q(n+1)-Q(n)$) is higher, but it will not wait for too long.



\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.995\linewidth]{figs/decode_time.pdf}
        \includegraphics[width=0.995\linewidth]{figs/decode_time_v2.pdf}
    \tightcaption{
    \name waits for the next frame until a deadline $t^*$, after which the utility is lower even if the next packet arrives. }
    \label{fig:decode-time}
\end{figure}


\end{comment}

%Readers may realize a potential problem arising from encoding and decoding being asynchronous. 


% However, we still need to design a practical packetization and entropy encoding scheme to make {\em entropy each encoded packet individually decodable} and do so {\em without an increase of data size}.
% This is not possible with standard autoencoders such as~\cite{dvc}, which entropy codes the entire \aecode to a single bitstream before packetization.
% As a result, any missing packet will render the bitstream undecodable. 
 


% Traditional codecs do have techniques to make each packet individually decodable, such as flexible macroblock ordering~\cite{lambert2006flexible} in H.264. These techniques divids the input frame into independent, non-overlapping partitions. Each partition is encoded separately, packed into its own entropy-encoded packet, enabling decodability if the corresponding packet arrives, as there's no dependency on other packets.

% However, this method leads to substantial size inflation, up to \editSOCC{50\%}~\cite{???}, due to the loss of compression efficiency inherent in traditional codecs' exploitation of content dependencies. For example, if two adjacent macroblocks share identical motion vectors (which is common in practice), H.264 can transmit the motion values once. But, if these macroblocks are separated into different partitions, each partition must send the value, resulting in size inflation.

% \name employs a different method as shown in Figure~\ref{fig:per-packet}. Instead of dividing the input frame, it {\em randomly} splits the elements in the coded tensor into sub-tensors and entropy encodes each sub-tensor separately. 
% The entropy coding in \name necessitates storing the symbol distribution of elements in the coded tensors for efficient compression. This means that, unlike methods that only send the symbol distribution once, our method requires storing it in every packet, potentially leading to additional overhead.
% However, this overhead is mitigated by the autoencoder training, which regularizes the distribution of elements in each coded tensor's channel to adhere to a zero-mean Laplace distribution. The variance value of each channel can be efficiently encapsulated with just a few bits. As a result, the overhead of including the symbol distribution in each packet remains minimal: even with 20 packets, the symbol distribution's size does not exceed 5\% of the total frame size.

% In \name, if a packet goes missing, we zero its elements in the original coded tensor. Given the random selection of these elements during encoding, this process effectively emulates random element masking, which matches the technique implemented during training. 
% Importantly, this approach ensures that the loss of any packet simulates a uniform random mask on the encoded tensor.

% The key difference between the per-packet entropy coding method used in traditional codecs and our method is that we don't have size inflation. This is because \name is not exploiting the dependency between elements for a better compression ratio, instead, it has fewer elements in the encoded data than traditional codecs. More specifically, in traditional codecs like H.264, each pixel has its motion vector and residual encoded in the bytestream, but \name's autoencoder will map the motion vector (or residual) of multiple pixels into the same element in the coded tensor. Therefore, \name can achieve the same size as traditional codecs without using dependencies between elements. During training, the autoencoder also learns to generate details to ensure that the quality does not drop even if we are sending less information than the traditional codecs.






\tightsubsection{Efficient coding and bitrate control}
\label{subsec:fast-coding}

%\tightsubsection{Reducing compute overhead}

%\mypara{Speed bottleneck}
% Most autoencoder research has been focused on video compression efficiency (using fewer bits to get higher quality), and their NN-based encoding and decoding are typically slower than the highly-optimized standard codecs like H.265.
% To be practical for real-time video streaming, \name entails a few additional optimizations to significantly speed up encoder and decoder and allow efficient re-encoding of a frame to match a given target bitrate. 

\begin{figure}[t!]
    \centering
        %\includegraphics[width=0.85\linewidth]{figs/split-iframe-size.pdf}
    \includegraphics[width=0.75\linewidth]{figs/split-iframe-size.pdf}
    \tightcaption{Encoding each P-frame with a small I-patch leads to smoother frame sizes than naively inserting I-frames.}
    \label{fig:keyframe_smooth}
\end{figure}

\mypara{I-frames}
In many autoencoders (including DVC), 
%Placement of I-frames poses a particular challenge for \name's autoencoders (both pre-trained and re-trained), because while 
the quality of P-frames will gradually degrade after an I-frame.
%, quality gradually degrades after about 10 frames. 
%for two reasons: (1) I-frames are generally bigger in size than P-frames, and 
%(2)  while the first few P-frames after an I-frame enjoy high quality, quality gradually degrades after about 10 frames. 
If we add I-frames frequently (\eg every 10 frames), we can achieve similar average compression efficiency with  H.264 and H.265 when they use an optimal I-frame interval.
% \footnote{Many computer-vision papers on autoencoders have conveniently used a small GoP when compared against H.265, but the implication of large I-frame size for congestion control is rarely discussed.}, 
% which strikes a better tradeoff between quality and {\em average} bitrate (comparable to H.264 and H.265 with large I-frame intervals).
However, since I-frames are larger than P-frames, adding too many I-frames causes frequent spikes in frame size. %, so it is difficult for congestion control to utilize network capacity. %at a fixed frame interval. 
%make it difficult for congestion control to send the frames at a fixed interval (inversely proportional to the frame rate).
Instead, \name uses an {\em extra} small square-sized patch as a tiny I-frame, called {\em I-patch}, on {\em every P frame}.
We split each frame into $k$ patches, and for a window of $k$ frames, each frame is sent with an extra I-patch at a different location, so I-patch ``scan through'' the whole frame every $k$ frame. 
By default, $k=30$ though we empirically found any value between 10 and 30 works well.
% the location of the I-patch on a frame changes over time, so that the I-patch will scan through the whole frame size every $k$ frames. 
With I-patch, \name does not need to send any I-frames (except the first frame). 
We use BPG~\cite{bpg} to encode/decode the I-patch. 
% , and found that as long as $k$ is between 10 and 30, the compression efficiency is roughly the same. 
Figure~\ref{fig:keyframe_smooth} shows that when $k=10$, I-patch mitigates the sudden size increase caused by I-frames. 

%\tightsubsection{Encoding a sequence of frames}
%\label{subsec:delivery:iframe}

%To stream a sequence of video frames, a key question is how often I-frames should be inserted in P-frames. 
%(As explained in \S???????????????????????????????????????????????????????????????????????????????????????????????????\ref{subsec:ae-background}, \name uses only I-/P-frames, as in most real-time video systems.)
%For the P-frame autoencoder we have tried, we observe that the decoded quality can be very high right after each I-frame but it gradually degrades after about 10 frames. 


%To add I-frames frequently without the intermittent bitrate spikes caused by the I-frames, 
% (128$\times$128 to 512$\times$512) 


It is worth noting that though I-patch encoding can also use a loss-resilient autoencoder, we do not protect their packet loss to simplify the system design. 
This is because if each patch will see an I-patch every $k$ frames, so even if one patch is lost, its impact is confined to the next $k$ frames, and empirically, even this impact is marginal since P-frames are still delivered.

% I-patches are not protected by loss

% When the decoder fully receives an I-patch, it will notify the sender

% when an I-patch is fully received, the future P-frame will be based on the I-patch. 
% is still sent I-patches


% the effect of using I-patch on the frame sizes when $k=10$. It shows that I-patch effectively avoids sudden size increase caused by I-frames. 
% \passed{\amz{What is $k$ set to in Figure~\ref{fig:keyframe_smooth} ? }}
%\edit{In practice, we use BPG~\cite{bpg} to encode/decode the I-patch.}
%Depending on the original frame size, kk varies between 6 and 20. 
% This scheme effectively ``amortizes'' the size of I-frames across $k$ frames, thus smoothing the frame size as well as quality across frames.
% Moreover, since the I-frame autoencoder's encoding delay is proportional to the input size, encoding a small I-patch adds only a small compute overhead for each frame.

% (\S???????????????????????????????????????????????????????????????????????????????????????????????????\ref{app:??} shows an example).
% \footnote{We should clarify that design choice of frequent I-frames works well for autoencoders, but it is unnecessary for classic codecs due to two reasons. First, an I-frame generated by our autoencoder is only 2-5×\times bigger than a P-frame, whereas this ratio in H.264 is 4-10×\times. Second, the P-frame quality in H.264 is relatively stable, whereas the quality of a P-frame is high following an I-frame (or an I-patch).}

%\jc{mention which I frame model, and why not jpeg?}



%\jc{need a paragraph to explain why frequent i-patches actually make a lot of sense}


%\jc{how to deal with scene change?}



\begin{figure}[t!]
    \centering
         \centering
        %\includegraphics[width=0.92\linewidth]{figs/speedup.pdf}
        \includegraphics[width=0.92\linewidth]{figs/speedup.pdf}
    \tightcaption{How the autoencoder is changed for efficient bitrate control and speedup on CPUs.}
    \label{fig:speedup}
    \vspace{-0.3cm}
\end{figure}


\mypara{Efficient bitrate control}
Any video encoder must encode a frame at a size barely below the target frame size.
% Typically this can be done either by a heuristic to predict which quality level can yield the right frame size
%  encoding (as in H.264~\cite{OPENH264}) or encoding the frame multiple times at different quality levels (as in Salsify~\cite{salsify}). 
Similar to~\cite{salsify}, \name encodes a frame multiple times at different quality levels but does so faster than encoding the frame from scratch for multiple times 
% doing the whole encoding process on a frame multiple times 
(illustrated in Figure~\ref{fig:speedup}(b)). 
\name trains multiple autoencoders each with a different $\alpha$ (in Eq.~\ref{eq:2}) to achieve different quality/size tradeoff.
\edit{During the training phase, modifications were confined to the residual encoders and decoders, while other NN weights remained fixed. 
Thus, once a frame is encoded, both the motion vector (MV) and residual are reusable, with the residual undergoing further encoding through different encoders each producing a different frame size. 
This procedure, taking under 3ms, can encode a frame multiple times via residual encoders of distinct $\alpha$ values. Residual sizes in practice can span from 0.1$\times$ to 10$\times$ the MV size, thereby allowing \name to encompass a wide range of bitrates (see to \S\ref{subsec:eval:resilience}).}
%but when we train these autoencoders, we {\em only} change their residual encoders and decoders, while freezing the weights of the MV encoder and decoder NNs.
%As a result, once a frame is encoded once, we can re-use the MV and residual but {\em only} re-encode the residual using a higher quality encoder, so encoding a frame the second time only takes less than 5ms. 
%This allows us to encode a frame multiple times (with the residual encoder of different $\alpha$s).
% Empirically, \name encodes each frame 1-2 times before getting a frame whose size is the highest but below the target frame size.

%Fortunately, we show that on a single NVIDIA GeForce 3080 GPU, \name's encoding speed can be greatly improved: from 5~fps on 720p HD (and 11~fps on 480p) videos by the off-the-shelf implementation to 18~fps (and 40~fps). More results in \S?????????\ref{subsec:eval:system}. 
%\name achieves such speedup by downsizing the image (by default 4×4\times) during motion-vector estimation and motion compensation, and then upsample the motion-compensated image before calculating and encoding the residuals. 
%This speeds up encoding because motion-vector estimation and motion compensation are the slowest steps during P-frame encoding and their delays are proportional to the input size.
%Thus, the overall encoding delay will be reduced if they are fed with downsized images. 
%At the same time, because the residuals are still computed between the full-resolution image and the motion-compensated image, the coding efficiency is not affected by this change for most frames.


\mypara{CPU-based speedup}
We have implemented a faster version of \name on CPUs.
% while preserving the loss-resilience autoencoder. 
It differs from the GPU-based autoencoder in two key aspects (Figure~\ref{fig:speedup}(c)): 
we (1) re-use the motion prediction logic in H.264 to generate MVs, and % (and re-train the encoder/decoder of both MV and residual), and
(2) remove the frame prediction NN from the motion compensation step. 
As a result, with 32 threads, it takes 35ms to encode a 720p HD frame (and 17.2ms on 480p) on Intel Xeon 4216 CPU. \passed{\yc{need ziyi's input, how many threads?}} %\jc{on what CPUs?}. 
As shown in \S\ref{subsec:eval:system}, the resulting autoencoder has slightly worse compression efficiency, but still achieves low frame delay in the presence of packet loss.
% obtains most of the benefit of a data-scalable coding system (\eg low frame delay in the presence of packet loss). 


\mypara{GPU-based speedup}
We use two ideas to speed up autoencoder on GPUs: 
(1) it uses Pytorch's just-in-time compiler~\cite{torchcompile} to optimize the NN encoder and NN decoder, and 
(2) it reduces the NN float-point precision from 32-bit to 16-bit. %\jc{Yihua/Ziyi, of all NNs or some NNs?} \zy{added}
As shown in \S\ref{subsec:eval:system}, on an NVIDIA A40 GPU, our implementation speeds up the encoder from 19.8 fps on 720p HD (and 39.5 fps on 480p) videos by the off-the-shelf implementation to 31.2 fps (and 87.7 fps on 480p), roughly a 1.5$\times$ speedup. More results in \S\ref{subsec:eval:system}.
This speed is on par with the speed-optimized proprietary autoencoders~\cite{elf}, and it still achieves desirable loss resilience and compression efficiency.
\passed{\amz{An obvious question here is "why not use the same optimization from CPU's MV on the GPU's NVENC"? I expect it would not actually provide a big benefit, since using the NVENC hardware on the GPU during inference will likely incur additional data movement between buffers, but if there’s a way you can head off that inquiry that might help. If you haven't tried it maybe add such an optimization as future work?} \yc{opticflow accelerator: https://developer.nvidia.com/blog/harnessing-the-nvidia-ada-architecture-for-frame-rate-up-conversion-in-the-nvidia-optical-flow-sdk/}}




%\mypara{Downscaling motion-vector operations}

\begin{comment}
\mypara{Speeding up on GPUs}
Most of the delay of \name's encoder and decoder can be attributed to motion related operations, including motion estimation, motion vector (MV) encoding, MV decoding, and motion compensation (see Figure~??????\ref{fig:dvc-arch}). 
%For example, to encode and decode a 720p frame (1280x720) on a \fillme GPU, these motion-related operations take \fillme\% of encoding delay and \fillme\% of decoding delay. 
Since most operations in MV encoding and decoding are mostly convolutional, \name speeds up these motion-related operations by downscaling the MV (by 4×4\times, by default) which speeds up the MV encoding and decoding by 4×\times.
In addition, \name uses Pytorch's just-in-time compiler to optimize the implementation of the encoder and decoder. 
\end{comment}


%At the same time, because the residuals are still computed between the full-resolution image and the motion-compensated image, the coding efficiency is not affected by this change for most frames.


%\name speeds up the encoding and decoding of its autoencoders 
%
%%\begin{packeditemize}
%%\item {\em Downscaling motion vectors:} 
%
%Since most motion-related operations are convolutional, their compute overheads are proportional to the dimension of the input frames. 
%Thus, \name speeds up motion-related operations by downsizing ($4\times$ in default) the input frame and the reference frames, and then upscale the motion-compensated image to compute the full-scale residual.
%%\item {\em Efficient bitrate control}
%%\end{packeditemize}




%\tightsubsection{Bitrate control}





%\jc{yihua, ziyi, fill in the text}




\begin{comment}

As a video coding system, the target frame size for \name to encode a frame is determined by an external adaptation, such as GCC, typically to match the estimated throughput.
To cope with fluctuations of network condition, throughput estimation can vary even between two consecutive frames.
As a result, \name should encode each frame at a size barely below the target frame size.
%This has been a challenge with traditional codecs.
%Thus, it is important that most frames are smaller than the target size set by congestion control, but traditional codecs are not able to do that. 
%This has been observed in \cite{salsify}, which proposes to encode each frame at multiple quality levels in order to find an encoding that fits the target bitrate. 

To encode frame at a size below a given target, \name employs a bitrate-control method similar as~\cite{salsify} and encodes each frame twice and picks the frame that has the closest size to the target. 
To do so, we need to (1) train multiple autoencoders whose frame sizes cover a wide range, and (2) run two of them as fast as possible. 

% to encode a frame with a maximum size below a target. 
First, \name trains multiple autoencoders, each using a different weight of frame size $\alpha$ in its training loss function (\S\ref{subsec:sim-losses}).
These resulting autoencoders cover a range of bitrate range. \jc{some numbers}
%\fillme$\times$ difference between the highest bitrate and lowest bitrate. (A wider bitrate range is possible with more autoencoders.)
As long as the target bitrate is within this range, \name should be able to select the autoencoder whose encoded frame size is barely lower than the target. 

Next, \name avoids the excessive compute overhead by re-using the motion-compensated image to get the residuals, and only run different versions of residual encoders to encode the residuals with different bitrates.
Since residual encoder is faster than the motion estimation and compensation, the speed up is significant. \jc{some numbers}
%A naive solution will run multiple autoencoders (like~\cite{salsify}), but the compute overhead will increase linearly.
%Fortunately, we can again re-use 

\jc{explain hanchen's bitrate control logic}

\end{comment}




% Figure~\ref{fig:e2e} puts the various pieces of \name in an end-to-end workflow, and  Table~\ref{tab:mapping} summarizes the effect of each components of \name. 

%generates the downscaled motion-vector coded tensor (\S\ref{??}) and the I-patch coded tensor (\S\ref{??}).
%It then uses the bitrate controller (\S\ref{??}) to pick the residual encoder NN so that the resulting frame size closely matches the target bitrate. 
%On the receiver side, \name uses the logic described in \S\ref{??} to determine when to decode a frame.

%\mypara{Relationship with congestion control}
\name is {\em complementary} to existing congestion control (CC) algorithms. 
When combined with \name, the CC algorithm does {\em not} need to retransmit packets, unless no packets of a frame are received.
%The choice of the congestion control (CC) logic is {\em complementary} to \name.
CC determines how fast the packets should be sent out and the target bitrate of the next frame, whereas \name decides what should be in each packet. 
\S\ref{app:salcc} evaluates \name with GCC in WebRTC~\cite{carlucci2016analysis} and Salsify CC~\cite{salsify}. 
\S\ref{app:webrtc} discusses how to integrate \name in WebRTC.
% to run with the GCC algorithm while disabling the packet retransmission.
%Since it does not change the CC logic, \name can be readily integrated in WebRTC. We will discuss details .






%\jc{need an end-to-end figure here}


%\begin{figure}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.99\linewidth]{figs/technique-mapping.pdf}
%    \tightcaption{}
%    \label{fig:technique-mapping}
%\end{figure}



\begin{comment}

At a high level, the \name encoder and decoder feed packets to congestion control (CC) which determines how fast the packets should be sent out and the target bitrate (size) of the next frame. 
\name can work with different CC logics that have this interface.
These include GCC~\cite{??} and Salsify's CC logic~\cite{??} both of which are used as CC when we test \name and other video codecs in \S\ref{sec:eval}.
It should be noted that \name does not use FEC. 



\mypara{Interaction with transport layers}
%\name is built on the data-scalable autoencoder \name. 
%\name is a concrete real-time video communication system built on a data-scalable autoencoder (\name).
We focus on unique issues arising from the use of \name as the codec, including how to deliver each frame to strike a desirable delay-quality tradeoff, and how to deliver a sequence of frames when congestion or packet losses affect multiple frames. 
The choice of the congestion control logic is complementary to \name. 
In \S\ref{subsec:eval:e2e}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{carlucci2016analysis} or Salsify CC~\cite{salsify}. 
We do not claim that \name's strategies are new (\eg reference frame synchronization has been used in~\cite{salsify}). 
Nonetheless, \name integrates concrete design choices driven by the need, in order to unleash the full potential of \name and its data-scalable codec primitive.


\jc{interface?}

\end{comment}
%\jc{TODO}









==> sections/old/related_v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Related Work}
\label{sec:related}

% \begin{itemize}
% \item loss resilient schemes
% \item adaptive streaming: cc, fec rate, bitrate, etc.
% \item autoencoders
% \end{itemize}

% Other than the prior work elaborated elsewhere, we want to briefly mention a few other related techniques.


\mypara{Adaptive video streaming}
Loss-resilient video coding can be codec-specific (\eg~\cite{rdo,salsify} discussed in \S\ref{sec:motivate}) or adapt
% As the codecs become standardized and widely used in popular platforms like WebRTC, recent efforts shift focus to adapting 
common configurations of codecs or error correction (\eg FEC)~\cite{holmer2013handling}.
There has been intense research on adaptive video streaming, including performance analysis of commercial players (\eg~\cite{macmillan2021measuring,carlucci2016analysis}) and how to better adapt packet retransmission (\eg~\cite{feamster2002packet,yang2005unequal}), sending rate (\eg~\cite{sprout,concerto}), encoding bitrate (\eg~\cite{salsify,xiao2018two,zhang2021loki}) and FEC redundancy rate (\eg~\cite{nagy2014congestion,fong2019low}), which seek to predict future network conditions and/or quickly react to any changes. 
However, these predictions are not always accurate. %, due to occasional packet losses/delaying. 
% as the tail delay is susceptible to occasional packet losses/delaying or bandwidth drops. 
% While they achieve good performance with accurate predictions, it not easy to always be accurate, and thus the tail quality and delay is susceptible to occasional packet losses/delaying or bandwidth drops. 
In contrast, data-scalable coding is complementary to rate adaptation, but they eschew the need for accurate loss prediction and instead gracefully degrade their quality with more packet losses.

\begin{comment}

\mypara{Loss-resilient video coding}
Most early work on loss-resilient video coding focuses on modifying traditional codec (\eg H.26x) so that the decoder can reconstruct frames at decent quality in lossy networks (see FEC~\cite{holmer2013handling}, RDO~\cite{rdo}, and stateful encoding~\cite{salsify} for specific examples in \S\ref{sec:motivate}).
As the codecs become standardized and widely deployed in devices, recent efforts shift focus to adapting configurations (\eg reference frames, target bitrate) of these codecs and block error correction (FEC) to enhance loss resilience~\cite{holmer2013handling}.
% For instance, FEC is supported in WebRTC and other commercial video players~\cite{holmer2013handling}.

As elaborated in \S\ref{sec:motivate}, to obtain robustness to potential packet losses, these techniques must sacrifice encoded quality under no losses.
While \name trades quality for resilience, the tradeoffs are much more favorable, as the compression and loss resilience are jointly optimized.

\mypara{Adaptive video streaming}
There has been intense research on adaptive video streaming, including detailed performance measurements of commercial players (\eg~\cite{macmillan2021measuring,carlucci2016analysis}) and how to better adapt packet retransmission (\eg~\cite{feamster2002packet,yang2005unequal}), sending rate (\eg~\cite{sprout,concerto}), encoding bitrate (\eg~\cite{salsify,xiao2018two}) and FEC redundancy rate (\eg~\cite{nagy2014congestion,fong2019low}) to predict the future network conditions and quickly react to any changes. 
However, these predictions may not be always accurate, as the tail quality and delay is susceptible to occasional packet losses/delaying or bandwidth drops. 
% While they achieve good performance with accurate predictions, it not easy to always be accurate, and thus the tail quality and delay is susceptible to occasional packet losses/delaying or bandwidth drops. 
In contrast, \name eschews the need for accurate loss prediction and instead gracefully degrades its quality with more packet losses.
% since packet losses have a relatively mild impact on video quality and frame delay.

\end{comment}

\mypara{Autoencoder in signal processing}
% Like many deep-learning techniques, applications of neural autoencoders is an active  topic. %~\cite{??,??,??}.
Our work is related to two autoencoder applications in the signal processing community. % are most relevant to this work.
One improves lossy channel communication by training the decoder as a classifier~\cite{erpek2020deep,dai2020deep}. 
To send a message from a set of $n$ messages, the sender encodes a one-hot vector (with the index of the message set to one), and the decoder classifies (possibly corrupted) data to predict which message it is. 
The other uses autoencoders to code images in a representation that is both compact and robust to signal noises~\cite{bourtsoulatze2019deep,gunduz2019machine}.
Like us, it combines data (image) compression with robustness to low SNR in the physical layer. 

Our work differs on two key fronts. 
The first is that they target a different network layer.
Physical-layer protection against signal noises is different from (and complementary to) transport-/application-layer protection against packet losses.
%Physical-layer noises affected data transmission differently than drops/queuing of data packets on which modern real-time video applications (\eg WebRTC) operate. 
Moreover, though physical-layer noises can be modeled as differentiable linear transformations (as in~\cite{bourtsoulatze2019deep,gunduz2019machine}), packet drops (\rate) are not differentiable and need to be handled differently (see \S\ref{sec:design}). 
The second is compressing and streaming videos is different from (if not more difficult than) compressing individual images. 
Video frames cannot be treated separately, because any error on one frame may propagate to future frames. 
While more research is needed, we believe that we have taken a significant step forward in showing the promise of autoencoders in real-time videos and outlining the concrete technical steps that should be pursued. 

\jc{add more on fountain coding}


\section{Limitations}

\mypara{At least one packet has to arrive}
\name cannot decode a frame with no received packet, rather it allows the receiver to choose when to decode {\em after} the first packet arrives. 
This means \name will not help during network disconnection or severe congestion that block any packet arrivals.
One potential way to avoid such extreme situation is leverage multiple concurrent connections and run \name over multipath TCP (with custom packet scheduling to discard or deprioritize untimely packets.)


\mypara{Bounded by autoencoder's performance}
Though \S\ref{sec:eval} shows that \newae's compression efficiency is comparable to H.264 under no packet loss, its quality-bitrate tradeoff is bounded by that of the pre-trained autoencoders. 
This is expected, since we choose not to modify the autoencoder architecture, and instead only train them to be data-scalable. 
Similarly, \newae does not improve the generalization of pre-trained autoencoders on unseen videos, because we train them using the pre-trained models' training data (Vimeo-90K and \fillme).
That said, autoencoders are being constantly improved to obtain higher compression efficiency (\eg via using more reference frames like in traditional codecs) and work better on new videos (\eg via model adaptation).

\mypara{No multi-party support (yet)}


\mypara{First I-frame must be lossless}

\mypara{Frames are rarely skipped}


\mypara{Compute and power overhead}





==> sections/old/related_v3.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US


\tightsection{Related work}
\label{sec:related}

% \begin{itemize}
% \item loss resilient schemes
% \item adaptive streaming: cc, fec rate, bitrate, etc.
% \item autoencoders
% \end{itemize}

Other than the prior work elaborated elsewhere, we want to briefly mention a few other related techniques.

\yihua{re-organize the content and extend the error concealment part.}
\mypara{Loss resilience}
Loss resilience techniques fall into four categories: error concealment, channel coding, source coding, and joint-source-channel coding.
Error concealment techniques allow the decoder to decode the corrupted bytestream and smartly recover the missing content.
The techniques include flexible macroblock ordering~\cite{660830, lambert2006flexible}, reference frame selection~\cite{wenger1998error, tsai2013error}, motion-vector reconstruction~\cite{varsa2001non, lee2001error, zhou2010efficient}.
Channel coding includes FEC techniques, Reed-Solomon code, LDPC and fountain codes~\cite{mackay1997near,mackay2005fountain}.
There are also recent works using neural networks for channel coding~\cite{7926071, 8919799}.
%An ideal fountain code sends as many bytes as possible and can reconstruct the original file once same number of bytes of the original file have been received. 
As elaborated in \S\ref{subsec:prior}, 
% While the (ideal) ability to reconstruct video of bitrate kk from any received data of bitrate kk is appealing, it means that some packets must be delayed/retransmitted if the encoded video bitrate already exceeds the link capacity, so using 
channel coding alone is not ideal for real-time video applications~\cite{fong2019low}.
Source coding adds redundancy during the video coding process, such as Intra-MB insertion~\cite{cote2000optimal, chen2015adaptive} and ROI-based protection~\cite{7265015, 5535201}. 
% which encodes some macroblocks (MBs) in a P-frame without referring to previous frames, making them decodable in absence of the reference frame.
A more promising approach to loss-resilient video coding is joint-source-channel coding~\cite{kurka2020deepjscc, pmlr-v97-choi19a}, and our \name belongs to this category.
The closest related work is DeepJSCC~\cite{kurka2020deepjscc} which trains an autoencoder to code images in a representation that is both compact and robust to signal noises~\cite{bourtsoulatze2019deep,gunduz2019machine}.
%It combines data (image) compression with robustness to low SNR in the physical layer
\name differs from DeepJSCC on two key fronts. 
First, they target physical-layer protection against signal noises.
% is different from (and complementary to) transport-/application-layer protection against packet losses. 
While physical-layer noises can be modeled as differentiable linear transformations (as in~\cite{bourtsoulatze2019deep,gunduz2019machine}), packet drops (\rate) are not differentiable and need to be handled differently. % (see \S\ref{subsec:sim-losses}). 
Second, unlike compressing individual images, frames in a streaming video cannot be treated separately, otherwise, any error on one frame may propagate to future frames. 
%While more research is needed, we believe that we have taken a significant step forward in showing the promise of autoencoders in real-time videos and outlining the concrete technical steps that should be pursued. 
% \yihua{where to put FGS?}


\mypara{Video compression}
Obtaining loss resilience must sacrifice coding efficiency (lower quality in absence of packet losses), and \name is no exception.
Most commercial video coding techniques are based on classic codecs, such as H.265 and VP9. 
Though video autoencoders (\eg~\cite{dvc,hu2021fvc}) have greatly improved their coding efficiency, it remains unclear if they outperform heavily engineered state-of-the-art video codecs, which do not limit the search for optimal reference MB and can run multiple passes on a video to optimize coding efficiency. 
Our evaluation focus on a specific setting (H.26x without B-frames and the ``fast'' preset) and shows that \name's coding efficiency is comparable with H.26x.
In a recent work~\cite{swift, NEURIPS2021_96b250a9}, autoencoders' coding efficiency is also shown to be comparable with H.265. 
% That said, we choose to build \name on autoencoders not for its coding efficiency, but for its potential to realize data-scalable delivery.

\begin{comment}
\mypara{Data-scalable autoencoders}
Our preceding study~\cite{cheng2022grace} similarly investigated the utility of autoencoders in data-scalable video codecs. Nevertheless, \name distinguishes itself from this past work via the following enhancements:
\begin{packeditemize}
    \item {\em Enhanced per-packet entropy encoding}: The prior work's per-packet entropy coding solution mapped tensor elements to individual packets randomly, which led to divergent element distributions within each packet due to the random shuffling, thereby reducing compression efficiency. \name rectifies this by regulating the distribution of elements within each channel as outlined in \S\ref{subsec:packetization}.
    \item {\em Accelerated encoding/decoding speed}: In the former study, encoding a 720p frame on a GPU using the AE encoder took over 50ms, and more than 5s on a CPU. This is insufficient for real-time 25fps video streaming. \name harnesses various strategies to optimize encoding speed (\S\ref{subsec:fast-coding}), enabling the encoding of a 720p frame at 25fps on both CPU and GPU.
    \item {\em Improved bitrate control}: In order to conform to the target bitrate, the same frame may need to be encoded by multiple models. While previous work reduced computation by sharing ~70\% of the weights, it still required more than 10ms to encode the same frame using a new model. \name further reduces computation by reusing the entire motion vector (\S\ref{subsec:fast-coding}), taking approximately 2ms to encode the same frame at a different bitrate (\S\ref{subsec:eval:system}).
    \item {\em Optimized state re-sync heuristics}: \name's state re-sync protocol (\S\ref{subsec:protocol}) minimizes error propagation due to encoder-decoder asynchrony, thereby improving average quality in comparison to our previous work (\S\ref{subsec:eval:e2e}).
\end{packeditemize}
Furthermore, we conducted an extensive evaluation of more error resilience baselines in \S\ref{sec:eval}, including smart FEC~\cite{rudow2023tambur}, smart error concealment~\cite{kang2022error}, Voxel~\cite{voxel}, and SVC, providing a comprehensive comparison between \name and potential error-resilient baselines.
\end{comment}


\begin{comment}
    

\mypara{Adaptive video streaming}
There has been intense research on adaptive streaming, including adapting sending rate (\eg~\cite{sprout,concerto, kurdoglu2016real, fang2019reinforcement}), encoding bitrate (\eg~\cite{salsify,xiao2018two,zhang2021loki, 9786839, 8943150}) and FEC redundancy rate (\eg~\cite{nagy2014congestion,fong2019low,holmer2013handling}).
These congestion control and bitrate adaptation algorithms are essentially reactive to intermittent congestion and packet losses. 
\name is complementary to them in that data-scalable delivery eschews the need for accurate loss prediction.
% and instead gracefully degrades their quality with more packet losses.
% as the tail delay is susceptible to occasional packet losses/delaying or bandwidth drops. 
% While they achieve good performance with accurate predictions, it not easy to always be accurate, and thus the tail quality and delay is susceptible to occasional packet losses/delaying or bandwidth drops. 
%In contrast, data-scalable coding is complementary to rate adaptation, but they eschew the need for accurate loss prediction and instead gracefully degrade their quality with more packet losses.


\end{comment}

% \tightsection{Conclusion}

% to deliver video frames in a data-scalable manner (decodable with any non-empty subset of packets and graceful improvement with more packets).
% Though in absence of packet losses, \name has lower coding efficiency than traditional codecs, we show that \name allows clients to better balance video quality and frame delay.

\tightsection{Discussion and Conclusion}

This paper presents \name, a new real-time video system that specifically trains autoencoders to tolerate a range of packet loss rates.
As a result, its quality gracefully degrades in {\em presence} of packet loss, with marginal compromise on quality in {\em absence} of packet loss.


Much remains unknown about the full potential and limits of autoencoder-based data communication. 
% Our work shows autoencoders can achieve decent packet loss for real-time videos. 
Although \name appears to work well for the packet loss patterns in our tested network traces--even beating many traditional loss-resilient video coding algorithms--we do not yet understand clearly why they are resilient to packet loss, other than the observation that across a range of videos, their quality seems to degrade gracefully with higher \rates.

% One fundamental question appears to be how to simulate the packet loss in the training process so the autoencoder can adequately learn to deal with vagaries in real-world network conditions. 
% We empirically observe that compared to uniformly selecting the rate of random masking from 0 to 100\%, the training will converge faster and achieve better quality if the training uses fewer specific rates of masking (\eg \{0\%, 30\%, 60\%\}).
% This suggests that more research is needed to systematically explore the design space of loss-resilient autoencoders.



%focusing on fewer possible rates of random data erasure (\eg 0\%, 30\%, 60\%) seem to  under high and low \rate than .
%cramming more rates of random data erasure (\eg a uniform distribution from 0 to 99\%). 



Our approach {\em increases} application complexity in order to {\em reduce} friction between networking and networked applications. 
Traditional optimizations for networking, including recent ML-based ones, have focused on low-level control knobs (like sending rate, bitrate, path selection) which only {\em indirectly} affect what a {\em user} perceives.
By contrast, our {\em autoencoder-based} approach focuses on maximizing the user-perceived quality of networked applications by training an NN-based data coding layer with packet loss and possibly a broader set of network objectives.

% For instance, an autoencoder {\em could} learn to also facilitate congestion control, \eg mildly overshooting estimated bandwidth to probe network capacities when content is more loss-tolerant.

% More research questions are opened by this approach.
% \begin{packeditemize}
% \item First, can autoencoders learn to also facilitate congestion control, \eg mildly overshooting estimated bandwidth to probe network capacities when content is more loss-tolerant?
% \item Second, can autoencoders learn to accommodate other applications such as generative AI which cares more about the quality of generated text or images?
% \end{packeditemize}
% But many dots need to be connected before the 

\begin{comment}


explores a new opportunity of ML for networking. 

By contrast, autoencoders 

The proposed loss-resilient autoencoder can also be extended to help determining sending rate (by varying the encoded frame sizes) to jointly adapt to variation of video content and network conditions.
It enables new optimizations, such as raising sending rate over estimated bandwidth only when the autoencoder-encoded frames are more loss-tolerant. 


\jc{
\begin{itemize}
\item this is a new data representation. not clear what its true potential is
\item unclear how to set training loss rate
\item unexploited flexibility: integration with congestion control
\item coding is old, but mostly case by case. autoencoder goes beyond video (generative AI?)
\end{itemize}
}

\end{comment}


\begin{comment}
    

\tightsection{Limitations}

\mypara{At least one packet has to arrive}
\name allows the receiver to choose when to decode {\em after} the first packet arrives, but it cannot decode a frame with no received packet. 
This means \name will not help during network disconnection or severe congestion that blocks any packet arrivals.
One potential way to avoid  such extreme situation is to leverage multiple concurrent connections and run \name over multipath TCP (with custom packet scheduling to discard or deprioritize untimely packets.)


% \mypara{Bounded by autoencoder's performance}
% Though \S\ref{sec:eval} shows that \newae's compression efficiency is comparable to H.264 under no packet loss, its quality-bitrate tradeoff is bounded by that of the pre-trained autoencoders. 
% This is expected, since we choose not to modify the autoencoder architecture, and instead only train them to be data-scalable. 
% Similarly, \newae does not improve the generalization of pre-trained autoencoders on unseen videos, because we train them using the pre-trained models' training data (Vimeo-90K~\cite{vimeo-dataset} and COCO\cite{coco-dataset}).
% That said, autoencoders are being constantly improved to obtain higher compression efficiency (\eg via using more reference frames like in traditional codecs) and work better on new videos (\eg via model adaptation).


%\mypara{No multi-party support (yet)}

%\mypara{First I-frame must be lossless}

\mypara{Frame skipping}
\name rarely skips a frame, unless no packet is received at all.  
This is a unique benefit of data-scalable delivery. 
However, we acknowledge that this is not necessarily the optimal choice.
We believe more user studies are needed to understand if people prefer frames decoded at a slightly lower quality (due to packet losses) or skip a few frames in hope of improving the quality of future frames.


\mypara{Compute and power overhead}
\name belongs to the line of work (\eg~\cite{nas,swift}) that embraces the trend of more hardware NN accelerators. 
That said, \newae as-is runs much more slowly than the heavily engineered codecs, so it is not applicable to low-power devices.
\jc{autoencoder is not for cheap devices}

\end{comment}

==> sections/old/technical-nsdi-v1.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US







\tightsection{Training \name's autoencoder}
\label{sec:core}


The next two sections present \name's training process of its autoencoder and online video delivery framework, respectively.
The key idea is to achieve DS coding by {\em jointly training the NN encoder and NN decoder of an autoencoder under different packet loss rates}.
We begin with how to simulate packet loss, and then
% such that losing one out of $n$ packets has the same effect as randomly zeroing $1/n$ values in the encoder's output. 
describe \name training process to optimize quality under various packet loss rates.

%In this section, we will first describe the training procedure with the assumption that packet loss appears to be setting values at random positions of the encoder output to zeros. 
%Then we will present a concrete packetization scheme realizes this assumption, so that the trained autoencoder effectively learns how to decode data affected by packet loss.

%
%\jc{this section needs more work}
%
%%\name is a concrete instantiation of data-scalable delivery. 
%We present, \name, a new {\em autoencoder}-based video coding system.
%This section presents the training  make \name data-scalable when packet loss affects only one frame.
%%---the new autoencoder training to tolerate random data erasure (\S???\ref{subsec:??}) and a custom scheme of packetization and entropy encoding to equate packet loss and data erasure (\S???\ref{subsec:??}).
%The next section will describe the video delivery framework over \name's autoencoder.

%designed to achieve close-to-optimal data-scalable coding. 

%and a custom delivery framework for the new autoencoder (\S???\ref{sec:delivery}).
%We will describe the autoencoder design in this section, followed by the delivery framework in the next section. 

%\tightsubsection{Training loss}

\mypara{Terminology}
Figure~\ref{fig:dvc-arch} shows the workflow of \name's encoder (sender) and decoder (receiver).
The encoder's output is a coded tensor that entails both encoded motion vector (MV) and encoded residuals. 
(We provide details of these tensors in Appendix~\ref{app:details}.
We denote the encoder by $\Coder$ (with its NN weights $\phi$) and the decoder by $\Decoder$ (with its NN weights $\theta$).
The encoder encodes a frame $\x$ to a {\em \aecode} $\y=\Coder(\x)$, and the decoder decodes $\y$ to a reconstructed frame $\hat{\x}=\Decoder(\y)$.
Traditionally, autoencoder training minimizes the following training loss function:% over inputs from training frames \X\X:
\vspace{-0.04cm}
\begin{align}
%\textrm{\bf min~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\y), \y, \x)\textrm{, where }\y = \Coder(\x)
%\textrm{\bf min~~} \mathbb{E}_{\x} \Distort(\Decoder(\y), \x)+\alpha\cdot\Size(\y)\textrm{, where }\y = \Coder(\x)\\
%\textrm{\bf min~} 
\mathbb{E}_{\x} {\color{black}\underbrace{\highlight{black}{$\Distort(\Decoder(\y), \x)$}}_{\text{\sf \footnotesize \textcolor{black!85}{Pixel error}}}}+
\alpha{\cdot}{\color{black}\underbrace{\highlight{black}{$\Size(\y)$}}_{\text{\sf \footnotesize \textcolor{black!85}{Encoded size}}}}\textrm{, where }\y = \Coder(\x)
\label{eq:1}
\vspace{-0.08cm}
\end{align}
Here, $\Distort(\hat{\x},\x)$ is the pixel-level reconstruction error of the decoded frame $\hat{\x}$ (by default, L2-norm\footnote{
Note that L2-norm (or mean squared error) of $\hat{\x}$ and $\x$ are closely related to PSNR of $\hat{\x}$. To avoid this bias, 
our evaluation in \S\ref{sec:eval} measures the quality improvement in SSIM and user subjective studies.
% To avoid bias towards PSNR, our evaluation in \S\ref{sec:eval} measures the quality improvement in not only PSNR, but also SSIM and user subjective studies.
% Following the common practice of autoencoder training, the training loss function also includes the reconstruction loss of the motion-compensated prediction. 
%Pixel-wise distortion may not be the best way to capture human perception of reconstructed images, but it is often used in autoencoder training for its differentiability. We will evaluate the trained autoencoders in terms of more standard metrics, such as SSIM and PSNR (in RGB and YUV).
} of $\hat{\x}-\x$), and $Size(\y)$ is the entropy-coded data size of $\y$ in bit-per-pixel (BPP).
The parameter $\alpha$ governs the size-quality tradeoff: a higher $\alpha$ leads to smaller frame size ($Size(\hat{x})$) but higher distortion (\ie poorer quality) of the reconstructed frame $\hat{\x}$.
% will tend to have better visual quality in $\Decoder(\z)$ but also higher bitrate. 
%In Eq.~\ref{eq:1}, s
Since all of the functions---$\Coder$, $\Decoder$, $\Distort$ and $\Size$ (which is approximated by a pre-trained NN~\cite{dvc})---are differentiable, the NN weights $\phi$ and $\theta$ can be trained jointly to minimize Eq.~\ref{eq:1}.
%For an input frame \x\x (a c×w×hc\times w\times h tensor), the \aecode is the output of the encoder \y=\Coder(\x)\y=\Coder(\x)  will be sent to the receiver, which then runs the decoder to reconstruct the original frame from \y\y: ^\x=\Decoder(\y)\hat{\x}=\Decoder(\y).



\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v3.pdf}
%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v4.pdf}
        %\includegraphics[width=0.95\linewidth]{figs/per-packet-encoding-v5.pdf}
        \includegraphics[width=0.9\linewidth]{figs/per-packet-encoding-v5.pdf}
    \tightcaption{Example of \name's packetization.
    % and per-packet entropy encoding. 
    When a packet is lost, the elements mapped to it will be set to zeros. \yc{this figure mentions "packetization". Consider either changing the text (prefetch "packetization" in section 3) or changing this figure}}
    \label{fig:per-packet}
\end{figure}

\jc{how about we get directly to "how packet loss affects the training objective of neural codecs" next?
it's important to explain "how" to simulate packet loss, but it seems to break the flow. 
also, it seems more natural to explain how packet loss is simulated in training and how it is done in testing together?}
\mypara{Simulating packet loss}
Figure~\ref{fig:per-packet} shows how \name splits the encoder's output into individual packets.
\name's sender first splits the encoded tensor to multiple subtensors by a uniform random mapping. We use a reversible pseudo-random function to generate the mapping so that the receiver can correctly recover the original tensor with the same random seed. 
More specifically, we map the $i^{\textrm{th}}$ element to the $j=(i*p\textrm{ mod }n)^{\textrm{th}}$ packet at the $(i*p-j)/n^{\textrm{th}}$ position, where $n$ is the number of packets and $p$ is a prime number.
%\footnote{A reversible mapping allows the decoder to map elements from packets (including lost packets) back to the vector $\z$. An example can be mapping the $i^{\textrm{th}}$ element to the $j=(i*p\textrm{ mod }n)^{\textrm{th}}$ packet at the $(i*p-j)/n^{\textrm{th}}$ position, where $n$ is the number of packets and $p$ is a prime number.} 
%\jc{Yihua, please fill in here. how is the encoded tensor split into subtensors? how is the psuedo random split done?}
If a packet is lost, the decoder will set each element whose position is mapped to the lost packet to zero. 
As a result, a $x$\% packet loss rate will be translated to randomly zeroing $x$\% values in the encoder's output tensor.
\S\ref{subsec:packetization} will explain how each subtensor is losslessly compressed via entropy encoded into the bitstream of a packet, but such lossless compression is bypassed during simulation.
% In practice, each subtensor will then be entropy encoded into an individual packet and sent through the network.
%\jc{Yihua please fill in here}



\mypara{Training loss function}
During training, \name simply simulates packet loss at a rate randomly selected from a distribution of packet loss rates (explained shortly), rather than running a packet-level simulator. \passed{\amz{why not use a simulator? seems like it would introduce the burst-y distribution you explicitly induce later, but perhaps is not differentiable? Might be helpful to explain explicitly, this is one of the big contributions of this section IMO.}}
Given a packet loss rate distribution, \name jointly trains the encoder and decoder NNs to minimize: 
\passed{\yc{maybe we just say we use the simulation for packet losses that is the same as the packetization}}
%which uses a random distribution \loss\loss to simulate the effect of packet loss on the encoder's output:
\vspace{-0.04cm}
\begin{align}
%\textrm{\bf min~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\y), \x)\textrm{, where }
%\color{blue}\underbrace{\highlight{blue}{\y∼\loss(\y|\Coder(\x))\y\sim \loss(\y | \Coder(\x))}}_{\text{\sf \footnotesize \textcolor{blue!85}{Simulating packet loss}}}
\mathbb{E}_{\x} \Distort(\Decoder(\y), \x)+\alpha{\cdot}\Size(\y)\textrm{, where }
\color{blue}\underbrace{\highlight{newblue}{$\y\sim \loss(\y | \Coder(\x))$}}_{\text{\sf  \footnotesize \textcolor{blue}{Simulate packet loss}}}
\label{eq:2}
\vspace{-0.04cm}
\end{align}
%where the change is highlighted in color.
The key difference between this and the traditional loss function Eq.~\ref{eq:1} (highlighted in blue) is the distribution function $\loss$, which characterizes the distribution of decoder input under packet loss.
%Given the encoder output \Coder(\x)\Coder(\x), \loss\loss represents the data distribution seen by the decoder. 
%Remember that 
For instance, with a 
loss rate of 33\%, $\loss(\y | \Coder(\x))$ is the probability of $\y$ being the result of randomly zeroing 33\% of elements in $\Coder(\x)$.
 % An example of such random masking between \name's encoder and decoder can be found in Figure~\ref{fig:grace-training}.
% trains its autoencoder and the traditional autoencoder training.
%each \y\y drawn from the distribution \loss(\y|\Coder(\x))\loss(\y | \Coder(\x)) is a result of randomly setting 30\% of elements in \Coder(\x)\Coder(\x) to zeros.

It should be noticed that the random probability distribution $\loss$ may not be expressed as a  function of $\phi$ and is thus not differentiable with respect to $\phi$.
To train the weights in $\phi$, we use the REINFORCE trick~\cite{Kingma2014} to approximate this gradient by Monte Carlo Sampling. This is commonly used in reinforcement learning~\cite{zhang2021sample, peters2008reinforcement}.

\begin{figure}[t]
    \centering
%    \includegraphics[width=0.99\linewidth]{figs/ae-arch-v2.pdf}
    %\includegraphics[width=0.9\linewidth]{figs/ae-arch-v3.pdf}
    \includegraphics[width=0.85\linewidth]{figs/ae-arch-v3.pdf}
    \tightcaption{\name applies {\em random masking} (setting a fraction of randomly selected elements to zeros) to the NN encoder output, whereas the traditional autoencoder training has no data loss between the encoder and the decoder.
    Random masking can be made equivalent to packet loss as shown in \S\ref{subsec:packetization}.}
%    Contrasting the proposed loss-resilient design of autoencoders with traditional autoencoders.}
    \label{fig:grace-training}
\end{figure}



\mypara{Choosing simulated packet loss rates}
%A key design choice in \name is the function \loss that governs what random data erasure rate the autoencoder learns to handle during training. 
To prepare \name's neural codec to handle a range of loss rates, we should simulate a wide range of packet loss rates in training.
One idea is to draw loss rate uniformly from [0, 100\%) and apply it on the encoder output $\Coder(\x)$, but interestingly, the resulting codec performs poorly especially under loss rates. 
We empirically found that if high loss rates (\eg over 80\%) are selected even only for a fraction of time, the quality under high loss rates does get marginally improved but at the expense of significant degradation of quality under low loss rates. 
This might be because the encoder will learn to add more redundant information to prepare for high loss rates and it becomes difficult to learn a decent NN encoder when the loss rate is low.
Instead, \name uses the following distribution to pick the simulated loss rate:
with 80\% probability, the loss rate is set to 0\%; with 20\% probability, the loss rate randomly chosen from \{10\%,20\%,30\%,40\%,50\%,60\%\}.
Other loss rate distributions are possible, but we leave a more thorough examination to future work.

\begin{comment}
\mypara{Distribution of simulated packet loss rates}
%A key design choice in \name is the function \loss that governs what random data erasure rate the autoencoder learns to handle during training. 
Intuitively, in order to prepare \name's neural codec to handle a range of loss rates, we should simulate a wide range of packet loss rates in training.
% not use a fixed rate of random masking; instead, we should include many different rates of random masking from the range [0, 100\%).
% as it will rarely see 0\% masking, which translates to \rate of 0\%, while 0\% \rate is the common case in practice. 
\name uses the following distribution to pick the simulated loss rate:
with 80\% probability, the loss rate is set to 0\%; with 20\% probability, the loss rate randomly chosen from \{10\%,20\%,30\%,40\%,50\%,60\%\}.
%In \S\ref{subsec:??}, we will compare it with other training distributions of random erasure rate

It is worth some words to explain why we do not choose packet loss rate uniformly from [0, 100\%).
Empirically, we found that if a high loss rate (over 80\%) is selected for a fraction of time, the quality during 90\% packet loss will slightly improve, but it will also hurt the quality at low loss rates. 
This is because the encoder will learn to add more redundant information to prepare for high loss rates and it becomes difficult to learn a decent NN encoder when the loss rate is low.

\end{comment}

\jc{Since the key messages now become "training with loss" and "joint training", how about we explain their benefits separately? 
For example, "training with loss" makes the decoder less susceptible to zeros (since zeros could be due to loss) but instead focus more on non-zero values. 
Similarly, "joint training" makes the encoder add more non-zero values to encode redundant information to facilitate decoding. 
Here, we can put the example comparison between reconstruction under pre-trained, training only decoder, and joint training.}
\myparaq{Why is \name loss tolerant}
% As we will show in \S\ref{subsec:eval:resilience}, the quality of \name's autoencoder degrades much more gracefully than both the standard DVC autoencoders as well as other loss-resilient baselines under different rates of random masking. 
There are two intuitive reasons.
% The jointly trained NN encoder and decoder can tolerate packet loss for three reasons.
(1) The NN encoder output has little stringent dependencies between its elements, so setting elements at random positions is less impactful on the decoding result than in H.265 output. 
(2) We empirically found that the \name-trained NN encoder learns to output more non-zero values than the original DVC, which makes it easier for the decoder to tell which values are affected by packet loss. 
The increased number of non-zero values also means the encoder might learn to add redundancy in the encoded data to allow more accurate decoder reconstruction. 
This is a unique benefit of jointly training NN encoder and decoder. 
This corroborates our empirical result in \S\ref{subsec:eval:micro} that if only the decoder is trained with packet loss (with the encoder weights fixed), the quality will be worse than \name.
% \edit{both added some redundancy to the $\y$ and} allows the decoder to easily distinguish  zeroed (masked) elements.
% (3) \name's training also prepares the NN decoder to recover the zeroed elements from unmasked elements. 
% \name's autoencoder can be intuitively understood as between a traditional autoencoder and generative NNs.
% \S\ref{subsec:eval:resilience} shows empirical evidence that \name exhibits better loss resilience than baselines. 


% However, picking the masking rate uniformly from [0, 100\%) does not work well.

% \jc{need to explain why this particular distribution of simulated loss rates}










==> sections/old/technical.tex <==
\tightsection{\name: a loss-resilient autoencoder}
In this section, we describe the design and implementation of our system.

\begin{itemize}
\item 4.1 Basic design of a loss-resilient autoencoder
\begin{itemize}
    \item architecture: i-frame, p-frames, etc
    \item (the difference might be here)
    \item training process: emulate losses and quantization, and what's the loss function
    \item inference process: how to apply entropy encoding (at the per-packet level). only basic design here, we will cover rate adaptation later
    \item how is it different from other autoencoders? (architecture, training, inference)
\end{itemize}
\item 4.2 Understanding the design choices
\begin{itemize}
    \item show a few examples of "graceful degradation" vs. training loss rate
    \item how to set the loss rate in training?
\end{itemize}
\item 5. practical issues
\begin{itemize}
    \item 5.1 bitrate adaptation (qp for rate adaptation)
    \item 5.2 adapting coding overhead (resizing for compute/delay budget)
    \item 5.3 streaming protocol for reference frame synchronization
    \item 5.4 
\end{itemize}
\item 6. Implementation
this could be folded to 5.4 if not too much to say
\begin{itemize}
    \item putting it together in webrtc: interface with webrtc (including rate adaptation, compute adaptation, frame-sync protocol). 
    \item implementation optimization
\end{itemize}
\end{itemize}


\tightsubsection{Basic design of \name}
Figure~\ref{?} presents a high-level overview of \name. It consists of three main components: an I-frame encoder/decoder, a P-frame encoder/decoder, and an entropy coder. 
For the I-frame encoder/decoder, we leverage the design proposed by Song \etal\cite{QMAP}. Figure~\ref{?} presents its workflow. The I-frame encoder takes a single image as the input and outputs a latent vector as the encoded frame. The latent vector will then be compressed into packets via lossless entropy coding (will introduce shortly) and sent out to the network. On the receiver side, it will first perform entropy decoding to restore the latent vector, which will then be fed into the decoder neural network to reconstruct the image.

To encode/decode the P-frames, we use the design from Lu \etal\cite{DVC} as shown in Figure~\ref{?}. The input to the P-frame encoder includes two parts: (i) the image to be encoded, and (ii) the reference image. The output latent vector of the P-frame encoder will also be compressed via entropy encoding and decompressed at the receiver side. The P-frame decoder takes the received latent vector as well as the reference frame as the input and outputs the reconstructed image
%We note that unlike H.264 which uses the previous image as the reference\cite{?}, the reference image selection for the our P-frame encoder/decoder is much more flexible. It can be any image comes before the current one.

\yh{TODO: describe the entropy coding component}
\yh{TODO: describe the differences of our design compared with Qmap and DVC}

\mypara{Training strategy} To make our codec loss resilient, we retrain both the I-frame codec and the P-frame codec with emulated packet losses. More specifically, \yh{describe how we add loss and why that is differentiable (every byte in the latent vector has \fillme\% of the chance to be zeroed-out)}. We use ADAM optimizer to retrain the I-frame codec and the P-frame codec for \fillme and \fillme iterations respectively on an Nvidia 3080 GPU. We train the I-frame codec using the \fillme dataset and the P-frame codec is trained on the Vimeo-90K dataset\cite{xue2019video}. All the training images are cropped into 256x256 pieces to fit the GPU memory. We adopt the loss function and the quantization method from the previous works \cite{DVC, QMAP}.

\mypara{Inference strategy} In \name, we use entropy coding to provide lossless compression for the latent vector. Usually, a P-frame with 720P resolution will be compressed into \fillme packets. However, the loss of a single packet can break the entropy coding and make the compressed latent vector unrecoverable on the receiver side. To address this problem, we apply a per-packet entropy coding mechanism. That is, we partition the latent vector into multiple chunks and apply entropy coding for each chunk independently. We adjust the size of each chunk based on the number of bytes after entropy coding so that they can fit into one packet. Per-packet entropy coding may incur an overhead when compared with one-time entropy coding. However, as we will show in section \fillme, such overhead is negligible.

Besides entropy coding, packet loss can still cause another problem: loss of one packet will zero out a large consecutive area in the latent vector, which may make the decoder hard to reconstruct the original image in practice. To address this problem, we apply a reordering algorithm to the latent vector before entropy coding. \yh{describe this algorithm in a mathematical way.}  After reordering, the packet loss will zero out multiple small chunks spread uniformly across the whole latent vector. The experiment result (in section \fillme) shows that adding the reordering algorithm can improve {\fillme}db in PSNR when comparing to the default pipeline without reordering.

To cooperate with the congestion control component in video conferencing applications, \name also provides an interface for bitrate adaptation during inference. It takes a value, $Q$, between 0 and 1 as the input and adjust the quality-size trade-off. When $Q = 0$, \name will encode the frame with the lowest quality and thus with the smallest size. When $Q=1$, \name will encode the frame with highest quality and largest size. We will introduce the detailed bitrate adaptation mechanism in section \fillme.

%Although the model trained with loss can handle information loss in the latent vector during training, packet loss can 
%Besides the lost of information, packet losses during inference can cause two extra problems: \emph{(i)} packet losses will break the entropy coding, and \emph{(ii)} data loss of consecutive-area in latent vector is hard to recover. 

 
\begin{figure}[t!]
    \centering
         \centering
         \includegraphics[width=0.75\linewidth]{figs/design-choice-placeholder.png}
         \label{fig:}
    \caption{(placeholder) Autoencoders can tolerate a much larger loss rate during inference when training with a relatively smaller loss rate. \yh{adding a line/subgraph showing if loss during training is too high, performance will be bad} \yh{add Qmap}}
    \label{fig:design-choice-profiling}
\end{figure} 

\tightsubsection{Design choices in \name}
As we discussed above, training with loss can help the model become loss resilient. However, there are still two unanswered question: 
\begin{packeditemize}
    \item How much improvement in image quality does the model trained with loss have, comparing to the model trained without loss.
    \item How much loss rate we should use during training?
\end{packeditemize}

Figure~\ref{fig:design-choice-profiling} shows the image quality measured in PSNR under different loss rate during inference. The key insight is: models trained with a low loss rate (such as 20\% and 30\%) is good enough to handle a much higher loss rate (such as 50\% and 60\%) during inference. For I-frame codec, \yh{add experiment for Qmap}.  For P-frame codecs, when we apply 60\% loss during inference, the PSNR of decoded image is \review{35}db when using a model trained with 30\% loss, while the model trainied without loss only provide a image of \review{28.5}db PSNR.

Therefore, we choose \fillme\% and \review{30}\% of loss for training the I-frame codec and the P-frame codec respectively. 

\tightsection{Practical issues}
\yh{think about a better name!}

\tightsubsection{Adapting to varying bitrates}

\tightsubsection{Adapting for coding overhead}

\tightsubsection{Synchronizing reference frames between encoder and decoder}

\tightsection{Implementation}

\begin{comment}
\tightsubsection{Handling packet losses with \name}
\begin{itemize}
    \item In practice, packet loss will bring multiple challenges to the codec
    \begin{itemize}
        \item packet loss will break the entropy coding
        \item Lost of consecutive-area in latent vector is hard to recover
        \item Error caused by packet losses may propagate along P-frames and cause persistent quality degradations
    \end{itemize}
    \item To address those challenges, we propose the following mechanisms: per-packet entropy coding, reorder the latent vector, and explicit synchronization of reference frame between encoder and decoder  
\end{itemize}

\tightsubsection{Bitrate adaptation}
\begin{itemize}
    \item In a video conferencing system, the codec should be able to cooperate with underlying congestion-control system by adjusting its output bitrate.
    \item Our bitrate adaptation mechanism is similar to Salsify (can encode multiple times to choose a suitable encoding parameter)
    \item Encode a single frame for multiple times may incur performance issues. We apply XXX optimization. As we shown in evaluation xxx, \name can provide a decent encoding speed while doing a good adaption to varying target bitrates. 
\end{itemize}

\tightsubsection{Implementation}
How autoencoder is integrated into ffmpeg
\end{comment}

==> sections/old/technical_v0.tex <==
\tightsection{\name: a loss-resilient autoencoder}
In this section, we describe the design and implementation of our system.

\begin{itemize}
\item 4.1 Basic design of a loss-resilient autoencoder
\begin{itemize}
    \item architecture: i-frame, p-frames, etc
    \item (the difference might be here)
    \item training process: emulate losses and quantization, and what's the loss function
    \item inference process: how to apply entropy encoding (at the per-packet level). only basic design here, we will cover rate adaptation later
    \item how is it different from other autoencoders? (architecture, training, inference)
\end{itemize}
\item 4.2 Understanding the design choices
\begin{itemize}
    \item show a few examples of "graceful degradation" vs. training loss rate
    \item how to set the loss rate in training?
\end{itemize}
\item 5. practical issues
\begin{itemize}
    \item 5.1 bitrate adaptation (qp for rate adaptation)
    \item 5.2 adapting coding overhead (resizing for compute/delay budget)
    \item 5.3 streaming protocol for reference frame synchronization
    \item 5.4 
\end{itemize}
\item 6. Implementation
this could be folded to 5.4 if not too much to say
\begin{itemize}
    \item putting it together in webrtc: interface with webrtc (including rate adaptation, compute adaptation, frame-sync protocol). 
    \item implementation optimization
\end{itemize}
\end{itemize}


\tightsubsection{Basic design of \name}
Figure~\ref{?} presents a high-level overview of \name. It consists of three main components: an I-frame encoder/decoder, a P-frame encoder/decoder, and an entropy coder. 
For the I-frame encoder/decoder, we leverage the design proposed by Song \etal\cite{QMAP}. Figure~\ref{?} presents its workflow. The I-frame encoder takes a single image as the input and outputs a latent vector as the encoded frame. The latent vector will then be compressed into packets via lossless entropy coding (will introduce shortly) and sent out to the network. On the receiver side, it will first perform entropy decoding to restore the latent vector, which will then be fed into the decoder neural network to reconstruct the image.

To encode/decode the P-frames, we use the design from Lu \etal\cite{DVC} as shown in Figure~\ref{?}. The input to the P-frame encoder includes two parts: (i) the image to be encoded, and (ii) the reference image. The output latent vector of the P-frame encoder will also be compressed via entropy encoding and decompressed at the receiver side. The P-frame decoder takes the received latent vector as well as the reference frame as the input and outputs the reconstructed image
%We note that unlike H.264 which uses the previous image as the reference\cite{?}, the reference image selection for the our P-frame encoder/decoder is much more flexible. It can be any image comes before the current one.

\yh{TODO: describe the entropy coding component}
\yh{TODO: describe the differences of our design compared with Qmap and DVC}

\mypara{Training strategy} To make our codec loss resilient, we retrain both the I-frame codec and the P-frame codec with emulated packet losses. More specifically, \yh{describe how we add loss and why that is differentiable (every byte in the latent vector has \fillme\% of the chance to be zeroed-out)}. We use ADAM optimizer to retrain the I-frame codec and the P-frame codec for \fillme and \fillme iterations respectively on an Nvidia 3080 GPU. We train the I-frame codec using the \fillme dataset and the P-frame codec is trained on the Vimeo-90K dataset\cite{xue2019video}. All the training images are cropped into 256x256 pieces to fit the GPU memory. We adopt the loss function and the quantization method from the previous works \cite{DVC, QMAP}.

\mypara{Inference strategy} In \name, we use entropy coding to provide lossless compression for the latent vector. Usually, a P-frame with 720P resolution will be compressed into \fillme packets. However, the loss of a single packet can break the entropy coding and make the compressed latent vector unrecoverable on the receiver side. To address this problem, we apply a per-packet entropy coding mechanism. That is, we partition the latent vector into multiple chunks and apply entropy coding for each chunk independently. We adjust the size of each chunk based on the number of bytes after entropy coding so that they can fit into one packet. Per-packet entropy coding may incur an overhead when compared with one-time entropy coding. However, as we will show in section \fillme, such overhead is negligible.

Besides entropy coding, packet loss can still cause another problem: loss of one packet will zero out a large consecutive area in the latent vector, which may make the decoder hard to reconstruct the original image in practice. To address this problem, we apply a reordering algorithm to the latent vector before entropy coding. \yh{describe this algorithm in a mathematical way.}  After reordering, the packet loss will zero out multiple small chunks spread uniformly across the whole latent vector. The experiment result (in section \fillme) shows that adding the reordering algorithm can improve {\fillme}db in PSNR when comparing to the default pipeline without reordering.

To cooperate with the congestion control component in video conferencing applications, \name also provides an interface for bitrate adaptation during inference. It takes a value, $Q$, between 0 and 1 as the input and adjust the quality-size trade-off. When $Q = 0$, \name will encode the frame with the lowest quality and thus with the smallest size. When $Q=1$, \name will encode the frame with highest quality and largest size. We will introduce the detailed bitrate adaptation mechanism in section \fillme.

%Although the model trained with loss can handle information loss in the latent vector during training, packet loss can 
%Besides the lost of information, packet losses during inference can cause two extra problems: \emph{(i)} packet losses will break the entropy coding, and \emph{(ii)} data loss of consecutive-area in latent vector is hard to recover. 

 
\begin{figure}[t!]
    \centering
         \centering
         \includegraphics[width=0.75\linewidth]{figs/design-choice-placeholder.png}
         \label{fig:}
    \caption{(placeholder) Autoencoders can tolerate a much larger loss rate during inference when training with a relatively smaller loss rate. \yh{adding a line/subgraph showing if loss during training is too high, performance will be bad} \yh{add Qmap}}
    \label{fig:design-choice-profiling}
\end{figure} 

\tightsubsection{Design choices in \name}
As we discussed above, training with loss can help the model become loss resilient. However, there are still two unanswered question: 
\begin{packeditemize}
    \item How much improvement in image quality does the model trained with loss have, comparing to the model trained without loss.
    \item How much loss rate we should use during training?
\end{packeditemize}

Figure~\ref{fig:design-choice-profiling} shows the image quality measured in PSNR under different loss rate during inference. The key insight is: models trained with a low loss rate (such as 20\% and 30\%) is good enough to handle a much higher loss rate (such as 50\% and 60\%) during inference. For I-frame codec, \yh{add experiment for Qmap}.  For P-frame codecs, when we apply 60\% loss during inference, the PSNR of decoded image is \review{35}db when using a model trained with 30\% loss, while the model trainied without loss only provide a image of \review{28.5}db PSNR.

Therefore, we choose \fillme\% and \review{30}\% of loss for training the I-frame codec and the P-frame codec respectively. 

\tightsection{Practical issues}
\yh{think about a better name!}

\tightsubsection{Adapting to varying bitrates}

\tightsubsection{Adapting for coding overhead}

\tightsubsection{Synchronizing reference frames between encoder and decoder}

\tightsection{Implementation}

\begin{comment}
\tightsubsection{Handling packet losses with \name}
\begin{itemize}
    \item In practice, packet loss will bring multiple challenges to the codec
    \begin{itemize}
        \item packet loss will break the entropy coding
        \item Lost of consecutive-area in latent vector is hard to recover
        \item Error caused by packet losses may propagate along P-frames and cause persistent quality degradations
    \end{itemize}
    \item To address those challenges, we propose the following mechanisms: per-packet entropy coding, reorder the latent vector, and explicit synchronization of reference frame between encoder and decoder  
\end{itemize}

\tightsubsection{Bitrate adaptation}
\begin{itemize}
    \item In a video conferencing system, the codec should be able to cooperate with underlying congestion-control system by adjusting its output bitrate.
    \item Our bitrate adaptation mechanism is similar to Salsify (can encode multiple times to choose a suitable encoding parameter)
    \item Encode a single frame for multiple times may incur performance issues. We apply XXX optimization. As we shown in evaluation xxx, \name can provide a decent encoding speed while doing a good adaption to varying target bitrates. 
\end{itemize}

\tightsubsection{Implementation}
How autoencoder is integrated into ffmpeg
\end{comment}

==> sections/old/technical_v2.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\newcommand{\Coder}{\ensuremath{C_\phi}\xspace}
\newcommand{\Decoder}{\ensuremath{D_\theta}\xspace}
\newcommand{\Quality}{\ensuremath{F}\xspace}
\newcommand{\Packetize}{\ensuremath{A}\xspace}
\newcommand{\X}{\ensuremath{\mathbb{X}}\xspace}
\newcommand{\x}{\ensuremath{\textbf{x}}\xspace}
\newcommand{\y}{\ensuremath{\textbf{y}}\xspace}
\newcommand{\z}{\ensuremath{\textbf{z}}\xspace}
\newcommand{\loss}{\ensuremath{p_{\textrm{loss}}}\xspace}




\section{\newae: Data-Scalable Autoencoder}

\name is a concrete instantiation of data-scalable delivery. 
At a high level, \name entails a new autoencoder, \newae, and a custom delivery framework that leverages the properties of \newae.
We will describe \newae in this section, followed by the delivery framework in the next section. 

We begin with the basic terminology of autoencoders. 
We denote the coder (a neural network parameterized by weights $\phi$) by $\Coder$ and the decoder (a neural network parameterized by weights $\theta$) by $\Decoder$.
For an input frame $\x$ in the space of $\X$, the coded data $\z=\Coder(\x)$ will be sent to the receiver, which then decodes $\z$ to reconstruct the original frame $\hat{\x}=\Decoder(\z)$.
Note that the coder and decoder functions do not include the lossless entropy coding and FEC coding; instead, they perform the lossy compression, like the block-based motion estimation and residual computation. 


The compression efficiency of the output $\hat{\x}$ is measured a function $\Quality(\hat{\x},\x)$ by a weighted sum of its visual quality (\eg PSNR) and its entropy-coded size (\eg estimated by a pre-trained neural net), with the weight of visual quality being $\alpha$. 
With a higher value of $\alpha$, the trained $\Coder(\x)$ will produce output $\z$ that naturally leads to better visual quality in $\Decoder(\z)$ but higher file size. 
To adapt to the dynamic sending rate, we train multiple versions of the autoencoders with different weight $\alpha$. (See \name's bitrate adaptation in \S\ref{??}.) 
% A higher $\Quality$ value is better (higher visual quality and/or lower entropy-coded size).


\subsection{Basic formulation of \newae training}

Unlike existing applications of autoencoders, we want to train a {\em data-scalable autoencoder} that not only improves compression efficiency but also is resilient to packet losses.
To this end, we make a few critical changes to the training process of autoencoders.
We customize two existing autoencoder architectures, \cite{dvc} for P-frames (with motion vectors and residuals as input) and \cite{qmap} for I-frames (with a static image as input).\footnote{We do not consider B-frames are they are not commonly used in low-latency videos.} 
We borrow their neural network architectures (their architectures in details in \jc{need an appendix on how dvc creates input \x from two frames, and which part of it was trained by us, which part are not.}).
Since they share the same conceptual framework described above, we do not discuss them separately unless necessary.

The fact that $\Coder$, $\Decoder$, and $\Quality$ are differentiable allows end-to-end training of the autoencoder architecture~\cite{??,??,??}.
Mathematically, given a training set $\X$, our goal is 
\vspace{-0.05cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\z = \Coder(\x)
\label{eq:1}
\vspace{-0.05cm}
\end{align}


This traditional training process (Eq.~\ref{eq:1}) can be viewed as having zero \rate, \ie the input to the decoder is the same as the output of the encoder. 
To incorporate non-zero \rate, \name proposes a custom training process for autoencoders, by adding a random distribution $\loss$:
\vspace{-0.05cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\highlight{blue}{$\z\sim \loss(\z | \Coder(\x))$}
\label{eq:2}
\vspace{-0.05cm}
\end{align}

We highlight the change in color. 
Based on coder output $\Coder(\x)$, $\loss$ returns a distribution over the possible received data seen by the decoder (after packet erasures under non-zero \rate). 
This randomization effectively lets the training process see the effect of non-zero \rate. 




% \section{Simulating \rates in autoencoder training}



% \mypara{How to simulate packet losses}

\mypara{Key issues of simulating \rates in autoencoder training}
Training a data-scalable autoencoder using Eq.~\ref{eq:2} entails three key questions:
\begin{packedenumerate}
\item How to make Eq.~\ref{eq:2} differentiable for a wide range of $\loss$ that simulates various packet loss patterns?
\item How to convert $\Coder(\x)$ to data packets? This decides how losing a packet would affect the data seen by the decoder.
\item What \rates should be simulated in training, so that the trained model can deal with a range of unseen \rates?
\end{packedenumerate}
% The first question concerns packetization of the coder output and the second question concerns what \rates should be used to train the model that can deal with a range of \rates.
These questions are not involved in canonical autoencoder training, but they become critical here for the need to simulate packet losses in the training process.
% , so that the trained model can handle packet losses of various \rates in real networks. 

\subsection{How to make \newae trainable?}

An immediate challenge imposed by Eq.~\ref{eq:2} is how to train an autoencoder (the weights in $\theta$ and $\phi$), despite that the random distribution $\loss$ is not a naturally differentiable step. 

% that the expected value of $\Quality$ may not always be written in a closed, differentiable form, so before we discuss how \loss simulate packet losses with a non-zero \rate, we must first be able to run backpropagation for weights $\theta$ and $\phi$ in Eq.~\ref{eq:2}. 


\jc{Yihua/Anton, please explain how you used REINFORCE trick here.
\begin{itemize}
    \item this may look like VAE, so a natural solution is reparameterization. it doesn't work because the expectation of $\Quality$ cannot be writtein in a closed, differentiable form
    \item we use reinforce trick.. how does it work?
\end{itemize}}


\subsection{How to simulate packet losses in training?}

\jc{start with how WE do packetization, including per-packet entropy coding, and then list the alternatives}

\jc{an illustration figure here}

As illustrated in Figure~\ref{??} packetization of \name first uses an assignment function $\Packetize$ to map each element of $\z=\Coder(\x)$ to $k$ non-overlapping sublists, and then losslessly encodes each sublist to get the bit stream of a packet.
Conversely, depacketization of \name first losslessly decodes each packet to a sublist and maps the sublists back to $\z$ by the inverse function $\Packetize^{-1}$.
Each packet is numbered so if a packet has not arrived when decoding, the elements mapped it will be set to zero (this is a natural choice, though we will discuss alternatives in \S\ref{??}). 

The key to a good packetization lies in the assignment function $\Packetize$, because it decides how missing one packet would affect the coded data seen by the receiver. 
The lossless coding can use any off-the-shelf entropy coder, and the entropy-encoded bit stream should fit in the size of a packet (1.5KB).
We will discuss our choice of the entropy coder in more details in \S\ref{??}.

We consider three design choices for $\Packetize$:
\begin{packeditemize}
\item Block-based assignment splits $\z$ to {\em contiguous} blocks so elements close together will be encoded in the same packet, much the same way video data is packetized today. 
This serves a reference design point.
\item Interleaving assignment assigns the $i^{\textrm{th}}$ element to the $(i\textrm{ mod }k)^{\textrm{th}}$ packet, where $k$ is the number of packets.
Interleaving-based packetization is recommended by some traditional loss-resilient schemes~\cite{??}.
\item Randomized assignment uses a pseudo-random mapping $\Packetize_{random}$ to assign each element in $\z$ to its position in a packet. 
An inverse function $\Packetize_{random}^{-1}$ (\eg\fillme) can then be used to map the packet data back to $\z$). 
\end{packeditemize}
Once the packetization method is selected, packet losses can then be simulated by zeroing the elements assigned to certain number of packets (based on \rates selected in \S\ref{??}). 


\myparaq{Why randomized assignment}
\name chooses randomized assignment over the block-based and the interleaving ones. 
The intuitive reason is that 

\jc{\begin{itemize}
    \item why better than block-based? some elements in autoencoder output are more important than others and the important ones are sometimes put together
    \item why better than interleaving? the elements in autoencoder output have structures that align with tensors, etc. so interleaving may destroy some channels entirely.
\end{itemize}}

Figure~\ref{??} empirically compares these schemes (while fixing other factors, such as packet loss rate and training and testing data).
\jc{Some initial results.}


\subsection{Choice of \rates in autoencoder training}

A desirable autoencoder should fare well under a wide range of \rates, so at first glance, we should simulate as many possible \rate values during training as possible.
Nonetheless, adding too much randomness in \loss may make the training converge more slowly and even to suboptimal autoencoder models. 

It remains an open question how to rigorously pick the best \rates in training.
That said, we try our best to empirically examine different choices of \rates in training.

\jc{
\begin{itemize}
    \item experiment setup
    \item empirical findings: 
    (1) must have zero loss rate
    (2) more \rates doesn't help
\end{itemize}
}



\subsection{Rate adaptation over \newae}

\jc{
\begin{itemize}
    \item explain the rate adaptation logic. how we estimate frame size from complexity
    \item show empirical correlation between complexity and frame size
    \item connect it with rate control in h264.
    \item talk about shared backbone to save memory footprint.
\end{itemize}
}


\subsection{Understanding \newae's loss resilience}

\jc{
\begin{itemize}
    \item \newae's performance is surprising, but can be explained.
    \item flat relationship among elements, no strict hierarchy/dependencies like in svc or fec
    \item saliency is more robust to losses: figure~\ref{fig:per-frame}
\end{itemize}
}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/per_frame_quality_degradation_v1.pdf}
         \label{fig:}
    \caption{}
    \label{fig:per-frame}
\end{figure}


\subsection{Key frame insertion}

\jc{
\begin{itemize}
    \item start with the need for more key frames (more than that in h265).
    \item we "amortize" key frames in different frames. (better also to explain why this isn't possible in h264)
    \item give a simple back-of-envelope estimate of the new size. figure~\ref{fig:keyframe_smooth}
\end{itemize}
}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/keyframe_smooth.pdf}
    \caption{}
    \label{fig:keyframe_smooth}
\end{figure}



\section{Real-time video delivery over \newae}

Next, we present the design of \name, a concrete real-time video communication system based on \newae.
In designing \name, we focus primarily on unique issues that arise from using \newae as the codec. 
We group these issues in two categories. 
\begin{packeditemize}
\item First, optimizing the delivery of a single frame to optimize the delay-quality tradeoff. 
\item Second, optimizing the delivery of a sequence of frames when congestion or packet losses persist.
% synchronize the coding/decoding states between the sender and receiver?
\end{packeditemize}


\subsection{Workflow}

Figure~\ref{??} depicts \name's framework, which comprises of three high-level modules: the codec (\newae), the congestion controller, and the transmission controller.
The congestion controller decides the sending rate, and the choice of the congestion control logic is complementary to \newae. 
In \S\ref{??}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{??} or Salsify CC~\cite{??}. 

The transmission controller determines how to packetize \newae coder's output (coded data), deliver the packets, and depacketize all or a subset of packets to the input of \newae's decoder. 
The transmission control module is where \name makes simple yet critical modifications, in order to unleash the full potential of \newae and its data-scalable codec primitive. 
Here, we dive into more details on four major modifications. 
% \jc{we logically separate the system into two level: delivering each single frame and delivering a sequence of frames. }

\jc{emphasize that none of these techniques are exactly new, but the particular design is driven by \newae}

\jc{we don't specify the protocol as they follow naturally from the design and is not our main contribution}


\subsection{Saliency-based redundancy}

Recall from \S\ref{??} that with data-scalable primitive, the quality of a frame depends on the fraction of packets received (under a fixed coder state). 
Thus, it would be ideal to packetize the \newae coder's output in a way that improves the quality when a certain fraction of packets are received.

To this end, \name uses a novel strategy based on the randomization packetization used in \newae training (\S\ref{??}), but optimizes the quality under a given number of packets by leveraging the {\em skew distribution} of high-saliency elements in \newae coded data. 
Here, saliency is defined in the same way as Eq.~\ref{eq:3}, \ie if an element has a high saliency, changing it has a higher impact on the decoded quality than other elements. 
To motive our strategy, we run an analysis across \fillme videos in our dataset and the \newae models of \fillme different quality levels. 
Overall, the sum of saliency of the top \fillme-\fillme\% of elements is higher than the sum of saliency of all remaining elements. \jc{need a few words on why saliency is skewed? will it contradict fig~\ref{fig:per-frame}?}

These skewed distributions of saliency suggest that giving the high-saliency elements more protection can improve decoded quality, even at a cost of slightly more bytes. 
\name employs a simple yet efficient strategy of duplicating the top \fillme\% elements with the highest saliency. 
\jc{more details of the exact strategy}


\subsection{Choosing when to decode a frame}

As new packets arrive at the receiver queue (jitter buffer), the data-scalable primitive offers the receiver in \name a choice; decode now using currently arrived packets or waiting for more packets in hope of improving the quality. 
In contrast, with FEC-based loss-resilient schemes and other H.26x-based schemes (\fillme), the receiver simply has to wait for more packets until the data is decodable. 

\name embraces the primitive of data-scalable coding by carefully trading frame delay with decoded quality. 
When there is at least one more packet missing, the receiver estimates the distribution of the interval to the next packet arrival using past inter-packet intervals.
With this distribution and the quality-packet profile (Eq.~\ref{eq:3}) of the \newae that encodes the frame, \name's receiver chooses to decode a frame when \jc{an equation here}

This strategy is a well-defined, in sense that it will not decode a frame when new packets are expected to arrive, nor will it wait for more packets if the next packet arrives a long time later. 
\jc{can we also use an illustrative example to help people understand it?}


\subsection{Packet prioritization by sender}


In a WebRTC's sender, retransmitted packets (specified in selective ack) are always prioritized over new packets, simply because selectively retransmitted packets are required by the receiver to decode a prior (reference) frame.\footnote{There are exceptions, such as Salsify which may choose to skip certain frames, but they still prioritize retransmitted packets if the frame they belong to is not skipped.}
However, \name rethinks this seemingly natural choice, and instead prioritize new packets in order to leverage the primitive of data-scalable coding.
The intuitive reason is that a retransmitted packet may not be useful if arrives after the receiver decides to decode the frame. 
In contrast, each packet of a new frame, if delivered, is more likely to arrive before the receiver decodes the new frame and can thus improve its quality. 



\mypara{Extension with multi-path TCP}
\jc{more text}


\subsection{Reference frame synchronization}

An acute reader may have realized an unresolved issue, arising from encoding and decoding being asynchronous. 
If the $(i+1)^{\textrm{th}}$ frame is a P-frame, by default the sender will encode it with the decoded $i^{\textrm{th}}$ frame as the reference (used to compute motion vectors and residuals) with the assumption that the $i^{\textrm{th}}$ was fully received by the receiver. 
Now, if the receiver decodes the $i^{\textrm{th}}$ frame with only a subset of its packets, the P-frame encoding of the $(i+1)^{\textrm{th}}$ frame have a low quality when being decoded with a different reference frame than the encoder has assumed. 

A natural strawman to prevent such quality degradation is always letting the receiver piggyback ``which frame was recently decoded using which packets (just the packet IDs would be sufficient)''. 
With this knowledge, the sender can reconstruct the identical latest frame decoded by the receiver (autoencoder decoding is deterministic), and use this reconstructed frame, rather than the immediate last frame, as the reference of the next P-frame.
However, this means that there will be a non-trivial gap between the reference frame and the frame being encoded, making the P-frame significantly bigger than if the very last frame is used as the reference. 
Such gap between the two frames is usually 3-5 frames (though the exact value depends on the propagation delay), and the P-frames are about \fillme$\times$ bigger. 


To prevent quality degradation with minimum frame size inflation, \name leverages the loss-resilience of \newae. 
Empirically, \newae can tolerate out-of-sync encoding/decoding states for several consecutive frames. 
Figure~\ref{??} \jc{more text}

Inspired by these empirical observations, \name uses a simple logic, referred to as lazy synchronization, to 


% \begin{comment}


% As we have seen, a data-scalable autoencoder is well-suited for connections with dynamic \rates, since its quality is near-optimal under no missing packets but degrade gracefully under higher \rates. 
% While the proposed autoencoders can be functionally integrated in WebRTC or other real-time video platforms by simply replacing the video codec, \name makes several logically simple yet crucial modifications to the video streaming system, to maximally embrace the advantages of data-scalable autoencoders.



% \subsection{Optimizing delivery of individual frames}

% A direct implication of the autoencoder's graceful quality degradation (Figure~\ref{??}) is the ability for the receiver (decoder) to trade delay for quality or vice versa, in a finer granularity than prior solutions. 
% Waiting for one more packet, which may slightly delay the rendering of a frame, always incrementally improve the quality of the frame, allowing the receiver to move along the quality-delay tradeoff in presence of delay/loss of multiple packets.
% In contrast, systems using FEC-based coding have to wait for a certain number of packets, due to the cliff effect (\S\ref{??}) of FEC.

% This property of data-salable autoencoder naturally lands itself to a transport mechanism in between UDP and reliably delivering every packet (or a fixed fraction of packets).
% The example in Figure~\ref{??} illustrates the workflow of how \name determines 



% \jc{
% \begin{itemize}
%     \item on coding a frame: i or p? which ref frame? which model?
%     \item on sending a frame: target sending rate or bitrate?
%     \item on receiving a frame: when to decode a frame?
%     \item on packet loss
% \end{itemize}
% }

% \jc{
% \begin{itemize}
%     \item explain our single-frame delivery module: 
%     \item (1) saliency-based redundancy
%     \item (2) selective retransmission
%     \item (3) multipath tcp extension
%     \item why? plot the impact of zeroing top k values
%     \item compare the original ae vs. new ae
%     \item takeaway: high-impact elements are rare, and impact of each packet is similar
% \end{itemize}
% }



% \subsection{Delivering a sequence of frames}

% \jc{
% \begin{itemize}
%     \item we have to think about long-term effects (propagation effects of \rate)
%     \item (1) packet prioritization in \name: evenly split among new packets.
%     \item contrast it with prioritizing retransmission in webrtc
%     \item (2) \name's way of selecting ref frame (on-demand synchronization)
%     \item explain the tradeoff: always sync-up (high overhead), always not sync-up (low quality)
%     \item empirical result: quality vs. \# of high-\rate frames
%     \item (3) bitrate adaptation: 
% \end{itemize}
% }

% \end{comment}


\section{Implementation}

\name is implemented with \fillme lines of Python (mostly for autoencoder NNs) and \fillme lines of C++ (for frame delivery and WebRTC integration). 
We use the method described in \S\ref{??} to fine-tune \fillme to get \newae's P-frame codec and \fillme to get \newae's I-frame codec. 
The per-packet entropy encoder is implemented by \fillme. 

The code and trained model of \name will be made public upon the publication of this paper.

\mypara{Integration}
The integration with WebRTC is logically straightforward, since \newae (including I-frame and P-frame encodings) exposes very similar interface as the default codec in WebRTC. 
\jc{Ziyi, please fill in the details}

\jc{need to explain the gains are not directly from the entropy encoder or motion vector estimation}

\mypara{Overhead}
Despite that sharing most NN layers (\S\ref{??}) greatly reduces the memory footprint of the multi-bitrate autoencoders, the compute overhead of autoencoder NNs remains substantial---100ms to encode a frame of \fillme$\times$\fillme on a \fillme GPU (though decoding can be much faster). 
Note that this is already faster than the autoencoder used in a recent work for video streaming.
Fortunately, because \name's autoencoder contains shallow NNs, the encoding and decoding of \newae can be greatly accelerated by OpenVino~\cite{??} and achieve \fillme even on CPUs. 
\jc{kuntai/ziyi, fill in the details here}



% \jc{
% \begin{itemize}
%     \item how to integrate it in webrtc: same logical interface for video coding, packetization. replacing vp8
    
%     \item autoencoder highlight: entropy encoder, i-frame model, p-frame model
    
%     \item use of intel vino to reduce overhead
% \end{itemize}
% }




==> sections/old/technical_v3.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\newcommand{\Coder}{\ensuremath{C_\phi}\xspace}
\newcommand{\Decoder}{\ensuremath{D_\theta}\xspace}
\newcommand{\Quality}{\ensuremath{F}\xspace}
\newcommand{\Packetize}{\ensuremath{A}\xspace}
\newcommand{\X}{\ensuremath{\mathbb{X}}\xspace}
\newcommand{\x}{\ensuremath{\textbf{x}}\xspace}
\newcommand{\y}{\ensuremath{\textbf{y}}\xspace}
\newcommand{\z}{\ensuremath{\textbf{z}}\xspace}
\newcommand{\loss}{\ensuremath{p_{\textrm{loss}}}\xspace}




\section{\newae: Data-Scalable Autoencoder}

\name is a concrete instantiation of data-scalable delivery. 
At a high level, it entails a new data-scalable autoencoder, \newae (presented in this section), and a custom delivery framework that leverages the new autoencoder (discussed in the next section).
%We will describe the autoencoder design in this section, followed by the delivery framework in the next section. 

\subsection{Autoencoder background}


We begin with the basic terminology of autoencoders. 
We denote the encoder (a neural network parameterized by weights $\phi$) by $\Coder$ and the decoder (a neural network parameterized by weights $\theta$) by $\Decoder$.
For an input frame $\x$ (a $c\times w\times h$ tensor), the coded data $\z=\Coder(\x)$ will be sent to the receiver, which then runs the decoder to reconstruct the original frame from $\z$: $\hat{\x}=\Decoder(\z)$.
Note that the encoder and decoder perform the lossy compression and are {\em separate} from the lossless entropy coding or FEC coding. (We will discuss entropy encoding and packetization in \S\ref{??}.)

We customize two existing autoencoder architectures, \cite{dvc} for P-frames (with motion vectors and residuals as input) and \cite{qmap} for I-frames (with a static image as input).\footnote{We do not consider B-frames are they are not commonly used in low-latency videos.} 
We borrow their neural network architectures (their architectures in details in \jc{need an appendix on how dvc creates input \x from two frames, and which part of it was trained by us, which part are not.}).
Since they share the same conceptual framework described above, we do not discuss them separately unless necessary.


The compression efficiency of the output $\hat{\x}$ is measured by a function $\Quality(\hat{\x},\x)$, which is a weighted sum of its visual quality (\ie the difference between $\hat{\x}$ and $\x$)\footnote{It is true that pixel-wise distortion is not the best way to capture human perception of compression artifacts, but it is often used in autoencoder training for its differentiability. Our empirical evaluation also shows that the trained autoencoder performs competitively in terms of more standard metrics, such as SSIM and PSNR (both RGB and YUV-based).} and its entropy-coded size (\eg estimated by a pre-trained neural net), with the weight of visual quality being $\alpha$. 
With a higher value of $\alpha$, the trained $\Coder(\x)$ will produce output $\z$ that naturally leads to better visual quality in $\Decoder(\z)$ but higher file size. 
To adapt to the dynamic sending rate, multiple versions of the autoencoders are trained, each with a different weight $\alpha$, and they share most (backbone) layers, which significantly reduces the memory footprint when switching between bitrates. (See \name's bitrate adaptation in \S\ref{??}.) 
% A higher $\Quality$ value is better (higher visual quality and/or lower entropy-coded size).

The fact that $\Coder$, $\Decoder$, and $\Quality$ are differentiable allows end-to-end training of the autoencoder architecture~\cite{??,??,??}.
Mathematically, given a training set $\X$, our goal is 
\vspace{-0.05cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\z = \Coder(\x)
\label{eq:1}
\vspace{-0.05cm}
\end{align}

\subsection{Basic formulation of \newae training}

To train a {\em data-scalable autoencoder}, the training process should not only focus on compression efficiency (low bitrate and low reconstruction distortion) but also do so under various packet loss rates.
To this end, we make a few critical changes to the training process of autoencoders.


This traditional training process (Eq.~\ref{eq:1}) can be viewed as having zero packet loss, \ie the input to the decoder is the same as the output of the encoder. 
To incorporate different loss rates, \name proposes a custom training process for autoencoders, by adding a random distribution $\loss$:
\vspace{-0.05cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\highlight{blue}{$\z\sim \loss(\z | \Coder(\x))$}
\label{eq:2}
\vspace{-0.05cm}
\end{align}
where the change is highlighted in color.
$\loss$ takes the encoder output $\Coder(\x)$ and returns a distribution over the possible received data seen by the decoder (after packet erasures under non-zero \rate). 
As we will see next, with appropriate randomization, $\loss$ can simulate the effect of packet losses on data received by the decoder.


Simulating packet losses in Eq.~\ref{eq:2} entails three questions:
\begin{packedenumerate}
\item How should $\loss$ convert $\Coder(\x)$ to data packets and change the coded data if packets are randomly dropped? 
%This decides what data seen by the decoder would be if packets are randomly dropped. 
\item Given that the general form of $\loss$ is not differentiable, so how to train autoencoders with Eq.~\ref{eq:2} in presence of the $\loss$ function? 
\item What packet loss rate should be simulated in training, so that the trained model can deal with a range of unseen loss rates?
\end{packedenumerate}
It is important to note that these questions are not involved in canonical autoencoder training, but they become critical here for the need to simulate packet losses in the training process.
% \section{Simulating \rates in autoencoder training}



% \mypara{How to simulate packet losses}

%\mypara{Simulating packet losses in autoencoder training}
%Training a data-scalable autoencoder using Eq.~\ref{eq:2} faces three key questions:
%\begin{packedenumerate}
%\item How to make Eq.~\ref{eq:2} differentiable for a wide range of $\loss$ that simulates various packet loss patterns?
%\item How to convert $\Coder(\x)$ to data packets? This decides how losing a packet would affect the data seen by the decoder.
%\item What \rates should be simulated in training, so that the trained model can deal with a range of unseen \rates?
%\end{packedenumerate}
% The first question concerns packetization of the coder output and the second question concerns what \rates should be used to train the model that can deal with a range of \rates.

% , so that the trained model can handle packet losses of various \rates in real networks. 

\subsection{How to make \newae trainable?}

An immediate challenge imposed by Eq.~\ref{eq:2} is how to train the weights ($\theta$ and $\phi$) of the autoencoder, despite that the random distribution $\loss$ is not a naturally differentiable step. 

% that the expected value of $\Quality$ may not always be written in a closed, differentiable form, so before we discuss how \loss simulate packet losses with a non-zero \rate, we must first be able to run backpropagation for weights $\theta$ and $\phi$ in Eq.~\ref{eq:2}. 


\jc{Yihua/Anton, please explain how you used REINFORCE trick here.
\begin{itemize}
    \item this may look like VAE, so a natural solution is reparameterization. it doesn't work because the expectation of $\Quality$ cannot be writtein in a closed, differentiable form
    \item we use reinforce trick.. how does it work?
\end{itemize}}


\subsection{How to simulate packet losses in autoencoder training?}

\mypara{Packetizing autoencoder output}


\jc{start with how WE do packetization, including per-packet entropy coding, and then list the alternatives}

\jc{an illustration figure here}

As illustrated in Figure~\ref{??} packetization of \name first uses an assignment function $\Packetize$ to map each element of $\z=\Coder(\x)$ to $k$ non-overlapping sublists, and then losslessly encodes each sublist to get the bit stream of a packet.
Conversely, depacketization of \name first losslessly decodes each packet to a sublist and maps the sublists back to $\z$ by the inverse function $\Packetize^{-1}$.
Each packet is numbered so if a packet has not arrived when decoding, the elements mapped it will be set to zero (this is a natural choice, though we will discuss alternatives in \S\ref{??}). 

The key to a good packetization lies in the assignment function $\Packetize$, because it decides how missing one packet would affect the coded data seen by the receiver. 
The lossless coding can use any off-the-shelf entropy coder, and the entropy-encoded bit stream should fit in the size of a packet (1.5KB).
We will discuss our choice of the entropy coder in more details in \S\ref{??}.

We consider three design choices for $\Packetize$:
\begin{packeditemize}
\item Block-based assignment splits $\z$ to {\em contiguous} blocks so elements close together will be encoded in the same packet, much the same way video data is packetized today. 
This serves a reference design point.
\item Interleaving assignment assigns the $i^{\textrm{th}}$ element to the $(i\textrm{ mod }k)^{\textrm{th}}$ packet, where $k$ is the number of packets.
Interleaving-based packetization is recommended by some traditional loss-resilient schemes~\cite{??}.
\item Randomized assignment uses a pseudo-random mapping $\Packetize_{random}$ to assign each element in $\z$ to its position in a packet. 
An inverse function $\Packetize_{random}^{-1}$ (\eg\fillme) can then be used to map the packet data back to $\z$). 
\end{packeditemize}
Once the packetization method is selected, packet losses can then be simulated by zeroing the elements assigned to certain number of packets (based on \rates selected in \S\ref{??}). 


\myparaq{Why randomized assignment}
\name chooses randomized assignment over the block-based and the interleaving ones. 
The intuitive reason is that 

\jc{\begin{itemize}
    \item why better than block-based? some elements in autoencoder output are more important than others and the important ones are sometimes put together
    \item why better than interleaving? the elements in autoencoder output have structures that align with tensors, etc. so interleaving may destroy some channels entirely.
\end{itemize}}

Figure~\ref{??} empirically compares these schemes (while fixing other factors, such as packet loss rate and training and testing data).
\jc{Some initial results.}


\subsection{Choice of \rates in autoencoder training}

A desirable autoencoder should fare well under a wide range of \rates, so at first glance, we should simulate as many possible \rate values during training as possible.
Nonetheless, adding too much randomness in \loss may make the training converge more slowly and even to suboptimal autoencoder models. 

It remains an open question how to rigorously pick the best \rates in training.
That said, we try our best to empirically examine different choices of \rates in training.

\jc{
\begin{itemize}
    \item experiment setup
    \item empirical findings: 
    (1) must have zero loss rate
    (2) more \rates doesn't help
\end{itemize}
}



\subsection{Rate adaptation over \newae}

\jc{
\begin{itemize}
    \item explain the rate adaptation logic. how we estimate frame size from complexity
    \item show empirical correlation between complexity and frame size
    \item connect it with rate control in h264.
    \item talk about shared backbone to save memory footprint.
\end{itemize}
}


\subsection{Understanding \newae's loss resilience}

\jc{
\begin{itemize}
    \item \newae's performance is surprising, but can be explained.
    \item flat relationship among elements, no strict hierarchy/dependencies like in svc or fec
    \item saliency is more robust to losses: figure~\ref{fig:per-frame}
\end{itemize}
}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/per_frame_quality_degradation_v1.pdf}
         \label{fig:}
    \caption{}
    \label{fig:per-frame}
\end{figure}


\subsection{Key frame insertion}

\jc{
\begin{itemize}
    \item start with the need for more key frames (more than that in h265).
    \item we "amortize" key frames in different frames. (better also to explain why this isn't possible in h264)
    \item give a simple back-of-envelope estimate of the new size. figure~\ref{fig:keyframe_smooth}
\end{itemize}
}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/keyframe_smooth.pdf}
    \caption{}
    \label{fig:keyframe_smooth}
\end{figure}



\section{Real-time video delivery over \newae}

Next, we present the design of \name, a concrete real-time video communication system based on \newae.
In designing \name, we focus primarily on unique issues that arise from using \newae as the codec. 
We group these issues in two categories. 
\begin{packeditemize}
\item First, optimizing the delivery of a single frame to optimize the delay-quality tradeoff. 
\item Second, optimizing the delivery of a sequence of frames when congestion or packet losses persist.
% synchronize the coding/decoding states between the sender and receiver?
\end{packeditemize}


\subsection{Workflow}

Figure~\ref{??} depicts \name's framework, which comprises of three high-level modules: the codec (\newae), the congestion controller, and the transmission controller.
The congestion controller decides the sending rate, and the choice of the congestion control logic is complementary to \newae. 
In \S\ref{??}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{??} or Salsify CC~\cite{??}. 

The transmission controller determines how to packetize \newae coder's output (coded data), deliver the packets, and depacketize all or a subset of packets to the input of \newae's decoder. 
The transmission control module is where \name makes simple yet critical modifications, in order to unleash the full potential of \newae and its data-scalable codec primitive. 
Here, we dive into more details on four major modifications. 
% \jc{we logically separate the system into two level: delivering each single frame and delivering a sequence of frames. }

\jc{emphasize that none of these techniques are exactly new, but the particular design is driven by \newae}

\jc{we don't specify the protocol as they follow naturally from the design and is not our main contribution}


\subsection{Saliency-based redundancy}

Recall from \S\ref{??} that with data-scalable primitive, the quality of a frame depends on the fraction of packets received (under a fixed coder state). 
Thus, it would be ideal to packetize the \newae coder's output in a way that improves the quality when a certain fraction of packets are received.

To this end, \name uses a novel strategy based on the randomization packetization used in \newae training (\S\ref{??}), but optimizes the quality under a given number of packets by leveraging the {\em skew distribution} of high-saliency elements in \newae coded data. 
Here, saliency is defined in the same way as Eq.~\ref{eq:3}, \ie if an element has a high saliency, changing it has a higher impact on the decoded quality than other elements. 
To motive our strategy, we run an analysis across \fillme videos in our dataset and the \newae models of \fillme different quality levels. 
Overall, the sum of saliency of the top \fillme-\fillme\% of elements is higher than the sum of saliency of all remaining elements. \jc{need a few words on why saliency is skewed? will it contradict fig~\ref{fig:per-frame}?}

These skewed distributions of saliency suggest that giving the high-saliency elements more protection can improve decoded quality, even at a cost of slightly more bytes. 
\name employs a simple yet efficient strategy of duplicating the top \fillme\% elements with the highest saliency. 
\jc{more details of the exact strategy}


\subsection{Choosing when to decode a frame}

As new packets arrive at the receiver queue (jitter buffer), the data-scalable primitive offers the receiver in \name a choice; decode now using currently arrived packets or waiting for more packets in hope of improving the quality. 
In contrast, with FEC-based loss-resilient schemes and other H.26x-based schemes (\fillme), the receiver simply has to wait for more packets until the data is decodable. 

\name embraces the primitive of data-scalable coding by carefully trading frame delay with decoded quality. 
When there is at least one more packet missing, the receiver estimates the distribution of the interval to the next packet arrival using past inter-packet intervals.
With this distribution and the quality-packet profile (Eq.~\ref{eq:3}) of the \newae that encodes the frame, \name's receiver chooses to decode a frame when \jc{an equation here}

This strategy is a well-defined, in sense that it will not decode a frame when new packets are expected to arrive, nor will it wait for more packets if the next packet arrives a long time later. 
\jc{can we also use an illustrative example to help people understand it?}


\subsection{Packet prioritization by sender}


In a WebRTC's sender, retransmitted packets (specified in selective ack) are always prioritized over new packets, simply because selectively retransmitted packets are required by the receiver to decode a prior (reference) frame.\footnote{There are exceptions, such as Salsify which may choose to skip certain frames, but they still prioritize retransmitted packets if the frame they belong to is not skipped.}
However, \name rethinks this seemingly natural choice, and instead prioritize new packets in order to leverage the primitive of data-scalable coding.
The intuitive reason is that a retransmitted packet may not be useful if arrives after the receiver decides to decode the frame. 
In contrast, each packet of a new frame, if delivered, is more likely to arrive before the receiver decodes the new frame and can thus improve its quality. 



\mypara{Extension with multi-path TCP}
\jc{more text}


\subsection{Reference frame synchronization}

An acute reader may have realized an unresolved issue, arising from encoding and decoding being asynchronous. 
If the $(i+1)^{\textrm{th}}$ frame is a P-frame, by default the sender will encode it with the decoded $i^{\textrm{th}}$ frame as the reference (used to compute motion vectors and residuals) with the assumption that the $i^{\textrm{th}}$ was fully received by the receiver. 
Now, if the receiver decodes the $i^{\textrm{th}}$ frame with only a subset of its packets, the P-frame encoding of the $(i+1)^{\textrm{th}}$ frame have a low quality when being decoded with a different reference frame than the encoder has assumed. 

A natural strawman to prevent such quality degradation is always letting the receiver piggyback ``which frame was recently decoded using which packets (just the packet IDs would be sufficient)''. 
With this knowledge, the sender can reconstruct the identical latest frame decoded by the receiver (autoencoder decoding is deterministic), and use this reconstructed frame, rather than the immediate last frame, as the reference of the next P-frame.
However, this means that there will be a non-trivial gap between the reference frame and the frame being encoded, making the P-frame significantly bigger than if the very last frame is used as the reference. 
Such gap between the two frames is usually 3-5 frames (though the exact value depends on the propagation delay), and the P-frames are about \fillme$\times$ bigger. 


To prevent quality degradation with minimum frame size inflation, \name leverages the loss-resilience of \newae. 
Empirically, \newae can tolerate out-of-sync encoding/decoding states for several consecutive frames. 
Figure~\ref{??} \jc{more text}

Inspired by these empirical observations, \name uses a simple logic, referred to as lazy synchronization, to 


% \begin{comment}


% As we have seen, a data-scalable autoencoder is well-suited for connections with dynamic \rates, since its quality is near-optimal under no missing packets but degrade gracefully under higher \rates. 
% While the proposed autoencoders can be functionally integrated in WebRTC or other real-time video platforms by simply replacing the video codec, \name makes several logically simple yet crucial modifications to the video streaming system, to maximally embrace the advantages of data-scalable autoencoders.



% \subsection{Optimizing delivery of individual frames}

% A direct implication of the autoencoder's graceful quality degradation (Figure~\ref{??}) is the ability for the receiver (decoder) to trade delay for quality or vice versa, in a finer granularity than prior solutions. 
% Waiting for one more packet, which may slightly delay the rendering of a frame, always incrementally improve the quality of the frame, allowing the receiver to move along the quality-delay tradeoff in presence of delay/loss of multiple packets.
% In contrast, systems using FEC-based coding have to wait for a certain number of packets, due to the cliff effect (\S\ref{??}) of FEC.

% This property of data-salable autoencoder naturally lands itself to a transport mechanism in between UDP and reliably delivering every packet (or a fixed fraction of packets).
% The example in Figure~\ref{??} illustrates the workflow of how \name determines 



% \jc{
% \begin{itemize}
%     \item on coding a frame: i or p? which ref frame? which model?
%     \item on sending a frame: target sending rate or bitrate?
%     \item on receiving a frame: when to decode a frame?
%     \item on packet loss
% \end{itemize}
% }

% \jc{
% \begin{itemize}
%     \item explain our single-frame delivery module: 
%     \item (1) saliency-based redundancy
%     \item (2) selective retransmission
%     \item (3) multipath tcp extension
%     \item why? plot the impact of zeroing top k values
%     \item compare the original ae vs. new ae
%     \item takeaway: high-impact elements are rare, and impact of each packet is similar
% \end{itemize}
% }



% \subsection{Delivering a sequence of frames}

% \jc{
% \begin{itemize}
%     \item we have to think about long-term effects (propagation effects of \rate)
%     \item (1) packet prioritization in \name: evenly split among new packets.
%     \item contrast it with prioritizing retransmission in webrtc
%     \item (2) \name's way of selecting ref frame (on-demand synchronization)
%     \item explain the tradeoff: always sync-up (high overhead), always not sync-up (low quality)
%     \item empirical result: quality vs. \# of high-\rate frames
%     \item (3) bitrate adaptation: 
% \end{itemize}
% }

% \end{comment}


\section{Implementation}

\name is implemented with \fillme lines of Python (mostly for autoencoder NNs) and \fillme lines of C++ (for frame delivery and WebRTC integration). 
We use the method described in \S\ref{??} to fine-tune \fillme to get \newae's P-frame codec and \fillme to get \newae's I-frame codec. 
The per-packet entropy encoder is implemented by \fillme. 

The code and trained model of \name will be made public upon the publication of this paper.

\mypara{Integration}
The integration with WebRTC is logically straightforward, since \newae (including I-frame and P-frame encodings) exposes very similar interface as the default codec in WebRTC. 
\jc{Ziyi, please fill in the details}

\jc{need to explain the gains are not directly from the entropy encoder or motion vector estimation}

\mypara{Overhead}
Despite that sharing most NN layers (\S\ref{??}) greatly reduces the memory footprint of the multi-bitrate autoencoders, the compute overhead of autoencoder NNs remains substantial---100ms to encode a frame of \fillme$\times$\fillme on a \fillme GPU (though decoding can be much faster). 
Note that this is already faster than the autoencoder used in a recent work for video streaming.
Fortunately, because \name's autoencoder contains shallow NNs, the encoding and decoding of \newae can be greatly accelerated by OpenVino~\cite{??} and achieve \fillme even on CPUs. 
\jc{kuntai/ziyi, fill in the details here}



% \jc{
% \begin{itemize}
%     \item how to integrate it in webrtc: same logical interface for video coding, packetization. replacing vp8
    
%     \item autoencoder highlight: entropy encoder, i-frame model, p-frame model
    
%     \item use of intel vino to reduce overhead
% \end{itemize}
% }




==> sections/old/technical_v4.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\newcommand{\Coder}{\ensuremath{C_\phi}\xspace}
\newcommand{\Decoder}{\ensuremath{D_\theta}\xspace}
\newcommand{\Quality}{\ensuremath{F}\xspace}
\newcommand{\Packetize}{\ensuremath{A}\xspace}
\newcommand{\X}{\ensuremath{\mathbb{X}}\xspace}
\newcommand{\x}{\ensuremath{\textbf{x}}\xspace}
\newcommand{\y}{\ensuremath{\textbf{y}}\xspace}
\newcommand{\z}{\ensuremath{\textbf{z}}\xspace}
\newcommand{\loss}{\ensuremath{p_{\textrm{loss}}}\xspace}




\section{\newae: Data-Scalable Autoencoder}

\name is a concrete instantiation of data-scalable delivery. 
At a high level, it entails a new data-scalable autoencoder, \newae (presented in this section), and a custom delivery framework that leverages the new autoencoder (discussed in the next section).
%We will describe the autoencoder design in this section, followed by the delivery framework in the next section. 

\subsection{Autoencoder background}


We begin with the basic terminology of autoencoders. 
We denote the encoder (a neural network parameterized by weights $\phi$) by $\Coder$ and the decoder (a neural network parameterized by weights $\theta$) by $\Decoder$.
For an input frame $\x$ (a $c\times w\times h$ tensor), the coded data $\z=\Coder(\x)$ will be sent to the receiver, which then runs the decoder to reconstruct the original frame from $\z$: $\hat{\x}=\Decoder(\z)$.
Note that the encoder and decoder perform the lossy compression and are {\em separate} from the lossless entropy coding or FEC coding. (We will discuss entropy encoding and packetization in \S\ref{??}.)

We customize two existing autoencoder architectures, \cite{dvc} for P-frames (with motion vectors and residuals as input) and \cite{qmap} for I-frames (with a static image as input).\footnote{We do not consider B-frames are they are not commonly used in low-latency videos.} 
We borrow their neural network architectures (their architectures in details in \jc{need an appendix on how dvc creates input \x from two frames, and which part of it was trained by us, which part are not.}).
Since they share the same conceptual framework described above, we do not discuss them separately unless necessary.


The compression efficiency of the output $\hat{\x}$ is measured by a function $\Quality(\hat{\x},\x)$, which is a weighted sum of its pixel-distortion $Distortion(\hat{\x},\x)$, (\ie the difference between $\hat{\x}$ and $\x$)\footnote{It is true that pixel-wise distortion is not the best way to capture human perception of compression artifacts, but it is often used in autoencoder training for its differentiability. Our empirical evaluation also shows that the trained autoencoder performs competitively in terms of more standard metrics, such as SSIM and PSNR (both RGB and YUV-based).} and its entropy-encoded size $Size(\hat{x})$ (\eg estimated by a pre-trained neural net), with the weight of size being $\alpha$: $\Quality(\hat{\x},\x)= Distortion(\hat{\x},\x)+\alpha\cdot Size(\hat{\x})$
With a higher value of $\alpha$, the trained $\Coder(\x)$ will produce output $\z$ that naturally leads to better visual quality in $\Decoder(\z)$ but higher file size. 
To adapt to the dynamic sending rate, multiple versions of the autoencoders are trained, each with a different weight $\alpha$, and they share most (backbone) layers, which significantly reduces the memory footprint when switching between bitrates. (See \name's bitrate adaptation in \S\ref{??}.) 
% A higher $\Quality$ value is better (higher visual quality and/or lower entropy-coded size).

The fact that $\Coder$, $\Decoder$, and $\Quality$ are differentiable allows end-to-end training of the autoencoder architecture~\cite{??,??,??}.
Mathematically, given a training set $\X$, our goal is 
\vspace{-0.05cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\z = \Coder(\x)
\label{eq:1}
\vspace{-0.05cm}
\end{align}

\jc{anton/yihua, can you draw a simplified figure to depict the input/output of the used autoencoders? the figure should also include the tensor dimensions of the input and output. }

\subsection{Basic formulation of \newae training}

To train a {\em data-scalable autoencoder}, the training process should not only focus on compression efficiency (low bitrate and low reconstruction distortion) but also do so under various packet loss rates.
To this end, we make a few critical changes to the training process of autoencoders.


This traditional training process (Eq.~\ref{eq:1}) can be viewed as having zero packet loss, \ie the input to the decoder is the same as the output of the encoder. 
To incorporate different loss rates, \name proposes a custom training process for autoencoders, by adding a random distribution $\loss$:
\vspace{-0.05cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\highlight{blue}{$\z\sim \loss(\z | \Coder(\x))$}
\label{eq:2}
\vspace{-0.05cm}
\end{align}
where the change is highlighted in color.
$\loss$ takes the encoder output $\Coder(\x)$ and returns a distribution over the possible received data seen by the decoder (after packet erasures under non-zero \rate). 
As we will see next, with appropriate randomization, $\loss$ can simulate the effect of packet losses on data received by the decoder.


Simulating packet losses in Eq.~\ref{eq:2} entails three questions, which we will address in the remaining of this section.
\begin{packedenumerate}
\item How should $\loss$ convert $\Coder(\x)$ to data packets and change the coded data if packets are randomly dropped (\S\ref{subsec:sim-losses})? 
%This decides what data seen by the decoder would be if packets are randomly dropped. 
\item Given that the general form of $\loss$ is not differentiable, so how to train autoencoders with Eq.~\ref{eq:2} in presence of the $\loss$ function (\S\ref{subsec:sim-trainable})? 
\item What packet loss rate should be simulated in training, so that the trained model can deal with a range of unseen loss rates (\S\ref{subsec:sim-lossrate})?
\end{packedenumerate}
It is important to note that these questions are not involved in canonical autoencoder training, but they become critical here for the need to simulate packet losses in the training process.
% \section{Simulating \rates in autoencoder training}



% \mypara{How to simulate packet losses}

%\mypara{Simulating packet losses in autoencoder training}
%Training a data-scalable autoencoder using Eq.~\ref{eq:2} faces three key questions:
%\begin{packedenumerate}
%\item How to make Eq.~\ref{eq:2} differentiable for a wide range of $\loss$ that simulates various packet loss patterns?
%\item How to convert $\Coder(\x)$ to data packets? This decides how losing a packet would affect the data seen by the decoder.
%\item What \rates should be simulated in training, so that the trained model can deal with a range of unseen \rates?
%\end{packedenumerate}
% The first question concerns packetization of the coder output and the second question concerns what \rates should be used to train the model that can deal with a range of \rates.

% , so that the trained model can handle packet losses of various \rates in real networks. 



\subsection{Simulating packet losses over autoencoders}
\label{subsec:sim-losses}

To simulate the impact of losing a packet, we first explain how \name packetizes the encoder output $\z=\Coder(\x)$.

\jc{an illustration figure here}

As illustrated in Figure~\ref{??}, \name first uses a {\em packetization function} $\Packetize$ to map each element position in $\z=\Coder(\x)$ (a 3-D or 4-D tensor) to $k$ non-overlapping lists (\name uses \fillme) and then losslessly encodes the elements in each list to produce the bitstream of a packet.\footnote{It is important to note that \name's {\em per-packet} entropy coding makes each packets individually decodable. 
This is different from typical autoencoders which entropy encodes the whole $\z$ tensor before packetization and thus any lost packet will make the received data not decodable by the entropy decoder. 
Moreover, since we use arithmetic coding (\fillme), so the total size of individually encoded packets is similar to the output of coding $\z$, if the elements in each packet share the same distribution as all elements in $\z$ (which is fortuitously ensured by random mapping). 
}
Conversely, depacketization in \name first losslessly decodes each packet to a list of elements and maps element back to their original positions in $\z$ by the inverse function $\Packetize^{-1}$.
One can use an off-the-shelf entropy coder to losslessly code the elements in a packet to a bitstream. (We discuss in \S\ref{??} \jc{need an appendix here} how to fit the bitstream in the normal packet size of 1.4KB.)


If a packet is lost, each element whose position is mapped by $\Packetize$ to the lost packet will be set to zero (this is a natural choice, though there are alternatives, which will be discussed in \S\ref{??}). 
 The choice of the packetization function $\Packetize$ is thus critical, since it decides how missing one packet would affect the coded data seen by the receiver.  
\name's packetization function is a {\em random} mapping; specifically, the pseudo-random function \fillme which has a reverse mapping. 
As a result, if the random packet loss rate is 30\%, then $\loss(\z|\Coder(\x))$ will produce a distribution of $\z$ that result from randomly setting 30\% of elements in $\z$ to be zeros. 

The use of randomized packetization seems straightforward, but it empirically works better than alternatives, for two reasons. 
\begin{packeditemize}
\item Some elements in autoencoder output $\z$ are more important than others (see \S\ref{??} for some examples), and zeroing each important element has disproportionally higher impact on the decoded quality than zeroing other elements.
A random mapping makes sure that losing $x\%$ packets will affect $x\%$ important elements (whereas a non-randomized packetization may affect more than $x\%$ important elements).
\item A random mapping ensures that all elements in $\z$ has the same distribution as those mapped to each packet. This makes it easier to maintain roughly same entropy-encoded size of each packet. 
\end{packeditemize}

In \S\ref{subsec:??}, we will empirically compare \newae trained with the random packetization and \newae trained with some alternative packetization schemes, such as block-based packetization (\ie each packet contains a contiguous block of elements in $\z$) and interleaving-based packetization. 
Both are suboptimal, since important elements can be next to each other and have a fixed distance with each other under $\z$'s specific tensor structure, so in the worst case both block-based packetization and interleaving packetization can drop higher fraction of important elements than packet loss rate.



%\name uses a {\em random} mapping $\Packetize_{random}$ 
%
%This choice of  $\Packetize$ is driven by two reasons. 
%An inverse function $\Packetize_{random}^{-1}$ (\eg\fillme) can then be used to map the packet data back to $\z$). 
%Once the packetization method is selected, packet losses can then be simulated by zeroing the elements assigned to certain number of packets (we will discuss the choice of packet loss rates used in training shortly). 
%Each packet is numbered so if a packet has not arrived when decoding, the elements mapped to it will be set to zero (this is a natural choice, though we will discuss alternatives in \S\ref{??}). 
%
%%\jc{start with how WE do packetization, including per-packet entropy coding, and then list the alternatives}
%
%We compare the choice of random assignment with two strawmen:
%\begin{packeditemize}
%\item Block-based assignment splits $\z$ to {\em contiguous} blocks so elements close together will be encoded in the same packet, much the same way video data is packetized today. 
%This serves a reference design point.
%\item Interleaving assignment assigns the $i^{\textrm{th}}$ element to the $(i\textrm{ mod }k)^{\textrm{th}}$ packet, where $k$ is the number of packets.
%Interleaving-based packetization is recommended by some traditional loss-resilient schemes~\cite{??}.
%\end{packeditemize}
%Once the packetization method is selected, packet losses can then be simulated by zeroing the elements assigned to certain number of packets (based on \rates selected in \S\ref{??}). 


%\myparaq{Why randomized assignment}
%\name chooses randomized assignment over the block-based and the interleaving ones. 
%The intuitive reason is that 
%
%\jc{\begin{itemize}
%\item why better than block-based? some elements in autoencoder output are more important than others and the important ones are sometimes put together
%\item why better than interleaving? the elements in autoencoder output have structures that align with tensors, etc. so interleaving may destroy some channels entirely.
%\end{itemize}}
%
%Figure~\ref{??} empirically compares these schemes (while fixing other factors, such as packet loss rate and training and testing data).
%\jc{Some initial results.}



\subsection{How to make \newae trainable?}
\label{subsec:sim-trainable}

Next, we need to make Eq.~\ref{eq:2} trainable for the weights ($\theta$ and $\phi$) when $\loss$ is a random function. 
%A challenge imposed by Eq.~\ref{eq:2} is how to train the weights ($\theta$ and $\phi$) of the autoencoder, despite that the random distribution $\loss$ is not a naturally differentiable step. 

% that the expected value of $\Quality$ may not always be written in a closed, differentiable form, so before we discuss how \loss simulate packet losses with a non-zero \rate, we must first be able to run backpropagation for weights $\theta$ and $\phi$ in Eq.~\ref{eq:2}. 


\jc{Yihua/Anton, please explain how you used REINFORCE trick here.
\begin{itemize}
    \item this may look like VAE, so a natural solution is reparameterization. it doesn't work because the expectation of $\Quality$ cannot be writtein in a closed, differentiable form
    \item we use reinforce trick.. how does it work?
\end{itemize}}

\subsection{Choice of packet loss rate in training}
\label{subsec:sim-lossrate}

As the packet loss rate varies over time, a desirable autoencoder should fare well under unseen packet loss rates.
We acknowledge that it remains an open question what packet loss rates should be used to train \newae to obtain ideal generalization under unseen packet loss rates. 
But we try our best to explore different strategies of setting packet loss rates. 

At first glance, we should simulate as many packet loss rates during training as possible.
However, we found that adding too much randomness in \loss might make the training converge more slowly and even to suboptimal autoencoder models. 
Specifically, our empirical results show that (1) training \newae with just a few values of packet loss rates generalizes better than with a wide range of packet loss rates, even on unseen test packet loss rates, and (2) the packet loss rates in training should include 0\% (otherwise the trained autoencoder will perform significantly worse than the pre-trained autoencoder on low packet loss rates. 

\jc{yihua/anton, please add a figure here to compare psnr-vs-loss under different training loss distributions}

To illustrate them, Figure~\ref{??} compares three choices of training packet loss rates.
\begin{packeditemize}
\item {\em Distribution-1:} \fillme
\item {\em Distribution-2:} \fillme
\item {\em Distribution-3:} \fillme
\end{packeditemize}
\name uses Distribution-1. 
\jc{yihua/anton, please fill in a short para on the read of the figure}

The intuition that more training packet loss rates might not help is that \fillme

%\jc{
%\begin{itemize}
%    \item experiment setup
%    \item empirical findings: 
%    (1) must have zero loss rate
%    (2) more \rates doesn't help
%\end{itemize}
%}


\subsection{Understanding \newae's loss resilience}

As illustrated in Figure~\ref{fig:autoencoder-pretrained}, compared to the pre-trained autoencoder (which is already data-scalable), \newae (re-trained on the same video dataset but with packet losses) achieves much higher quality on unseen videos under various test packet loss rates, even those that are {\em not} seen during training. 
This remarkable improvement begs the question why \newae can be much more resilient to packet losses. We believe that the reasons are two-fold. 


First, compared to SVC, FEC or H.26x-based coding, the elements in \newae's encoding output (before entropy encoding) does not impose any strict structure (\eg hierarchy or dependencies). 
Instead, the relationship between elements in \newae output is ``flat'', and changing any element (to zeo) would not render the frame non-decodable. 

Second, compared to the pre-trained autoencoder, the custom training process described in \S\ref{??} reduces the sensitivity of decoding quality to individual elements.
Though this effect is hard to directly show, we can illustrate it as follows.
We first calculate the ``gradient'' of decoding quality with respect to each element in $\z$ (defined shortly).
Mathematically, the gradient of decoding quality with respect to elements in $\z$ is a vector:
\vspace{-0.05cm}
\begin{align}
\vec{g}=\frac{\partial \Quality(\Decoder(\z),\x)}{\partial\z}
\vspace{-0.05cm}
\end{align}
Figure~\ref{fig:per-frame} shows the incremental impact on decoding quality if more elements are zeroed in descending order of the gradient.
As more elements are zeroed, we can see that quality of the pre-trained autoencoder drops sharply, whereas that of \newae drops much more slowly. 



%\jc{
%\begin{itemize}
%    \item \newae's performance is surprising, but can be explained.
%    \item flat relationship among elements, no strict hierarchy/dependencies like in svc or fec
%    \item saliency is more robust to losses: figure~\ref{fig:per-frame}
%\end{itemize}
%}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/per_frame_quality_degradation_v1.pdf}
         \label{fig:}
    \caption{}
    \label{fig:per-frame}
\end{figure}


\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.92\linewidth]{figs/transmission_overview.pdf}
    \caption{}
    \label{fig:overview}
\end{figure*}


\section{Real-time video delivery over \newae}

\name is a concrete real-time video communication system built on a data-scalable autoencoder (\newae).
In designing \name, we focus primarily on unique issues  arising from the use of \newae as the codec, including how to delivery each frame to strike a desirable delay-quality tradeoff (without skipping frames), and how to delivery a sequence of frames when congestion or packet losses affect multiple frames. 
%We group these issues in two categories. 
%\begin{packeditemize}
%\item First, optimizing the delivery of a single frame to optimize the delay-quality tradeoff. 
%\item Second, optimizing the delivery of a sequence of frames when congestion or packet losses persist.
%% synchronize the coding/decoding states between the sender and receiver?
%\end{packeditemize}


%\mypara{Workflow and modules}
Figure~\ref{fig:overview} depicts \name's framework, which comprises of three high-level modules: the codec (\newae), the congestion controller, and the transmission controller.
The congestion controller decides the sending rate, and the choice of the congestion control logic is complementary to \newae. 
In \S\ref{??}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{??} or Salsify CC~\cite{??}. 

The transmission controller determines how to packetize \newae coder's output (coded data), deliver the packets, and depacketize all or a subset of packets to the input of \newae's decoder. 
Other than the codec (\newae), most \name's changes are made in the transmission module. 
We do not claim that any of the modifications is exactly new (\eg a variant of reference frame synchronization has been used in~\cite(salsify)). 
Nonetheless, \name integrates concrete design choices driven by the need, in order to unleash the full potential of \newae and its data-scalable codec primitive.

% \jc{we logically separate the system into two level: delivering each single frame and delivering a sequence of frames. }

Here, we highlight on on four major modifications (more optimizations are discussed in \S\ref{??}).

%\jc{we don't specify the protocol as they follow naturally from the design and is not our main contribution}

\begin{comment}
\subsection{Saliency-based redundancy}

Recall from \S\ref{??} that with data-scalable primitive, the quality of a frame depends on the fraction of packets received (under a fixed coder state). 
Thus, it would be ideal to packetize the \newae coder's output in a way that improves the quality when a certain fraction of packets are received.

To this end, \name uses a novel strategy based on the randomization packetization used in \newae training (\S\ref{??}), but optimizes the quality under a given number of packets by leveraging the {\em skew distribution} of high-saliency elements in \newae coded data. 
Here, saliency is defined in the same way as Eq.~\ref{eq:3}, \ie if an element has a high saliency, changing it has a higher impact on the decoded quality than other elements. 
To motive our strategy, we run an analysis across \fillme videos in our dataset and the \newae models of \fillme different quality levels. 
Overall, the sum of saliency of the top \fillme-\fillme\% of elements is higher than the sum of saliency of all remaining elements. \jc{need a few words on why saliency is skewed? will it contradict fig~\ref{fig:per-frame}?}

These skewed distributions of saliency suggest that giving the high-saliency elements more protection can improve decoded quality, even at a cost of slightly more bytes. 
\name employs a simple yet efficient strategy of duplicating the top \fillme\% elements with the highest saliency. 
\jc{more details of the exact strategy}

\end{comment}

\subsection{Choosing when to decode a frame}

As new packets arrive at the receiver queue (the internal jitter buffer), the data-scalable abstraction allows the receiver to flexibly decide whether to decode the frame now using currently arrived packets or waiting for more packets in hope of improving the quality. 
In contrast, with FEC-based loss-resilient schemes and other H.26x-based schemes (\fillme), the receiver simply has to wait for more packets until the data is decodable. 

\name embraces this flexibility by carefully trading frame delay with decoded quality. 
When there is at least one more packet missing, the receiver estimates the distribution of the interval to the next packet arrival using past inter-packet intervals.
With this distribution and the quality-packet profile (Eq.~\ref{eq:3}) of the \newae that encodes the frame, \name's receiver chooses to decode a frame when \jc{an equation here}

\jc{Ziyi and Hanchen: please add a nice description of your logic here}

This strategy is a well-defined, in sense that it will not decode a frame when new packets are expected to arrive, nor will it wait for more packets if the next packet arrives a long time later. 
\jc{can we also use an illustrative example to help people understand it?}


\subsection{Packet scheduling by sender}

\jc{need to discuss it}

In a WebRTC's sender, retransmitted packets (specified in selective/negative acks) are always prioritized over new packets, simply because selectively retransmitted packets are required by the receiver to decode a prior (reference) frame. %\footnote{Exceptions exist, \eg Salsify may skip certain frames.}
\name rethinks this seemingly natural choice, and instead prioritizes new packets in order to leverage data-scalable delivery.
The reason is that a receiver in \name can decode anytime after it receives the first packet, so a retransmitted packet may not be useful if it arrives after the frame is already decoded. 
On the other hand, each packet of a new frame, if delivered, is more likely to arrive before the receiver decodes the new frame and can thus improve its quality. 

To make it work, the sender and the receiver be aware of the other's decision, regarding whether a previous frame's packets are still being resent or 



%\mypara{Extension with multi-path TCP}
%\jc{more text}


\subsection{Reference frame synchronization}

\jc{need to discuss it}

An acute reader may have realized an unresolved issue, arising from encoding and decoding being asynchronous. 
If the $(i+1)^{\textrm{th}}$ frame is a P-frame, by default the sender will encode it with the decoded $i^{\textrm{th}}$ frame as the reference (used to compute motion vectors and residuals) with the assumption that the $i^{\textrm{th}}$ was fully received by the receiver. 
Now, if the receiver decodes the $i^{\textrm{th}}$ frame with only a subset of its packets, the P-frame encoding of the $(i+1)^{\textrm{th}}$ frame have a low quality when being decoded with a different reference frame than the encoder has assumed. 

A natural strawman to prevent such quality degradation is always letting the receiver piggyback ``which frame was recently decoded using which packets (just the packet IDs would be sufficient)''. 
With this knowledge, the sender can reconstruct the identical latest frame decoded by the receiver (autoencoder decoding is deterministic), and use this reconstructed frame, rather than the immediate last frame, as the reference of the next P-frame.
However, this means that there will be a non-trivial gap between the reference frame and the frame being encoded, making the P-frame significantly bigger than if the very last frame is used as the reference. 
Such gap between the two frames is usually 3-5 frames (though the exact value depends on the propagation delay), and the P-frames are about \fillme$\times$ bigger. 


To prevent quality degradation with minimum frame size inflation, \name leverages the loss-resilience of \newae. 
Empirically, \newae can tolerate out-of-sync encoding/decoding states for several consecutive frames. 
Figure~\ref{??} \jc{more text}

Inspired by these empirical observations, \name uses a simple logic, referred to as lazy synchronization, to 


% \begin{comment}


% As we have seen, a data-scalable autoencoder is well-suited for connections with dynamic \rates, since its quality is near-optimal under no missing packets but degrade gracefully under higher \rates. 
% While the proposed autoencoders can be functionally integrated in WebRTC or other real-time video platforms by simply replacing the video codec, \name makes several logically simple yet crucial modifications to the video streaming system, to maximally embrace the advantages of data-scalable autoencoders.



% \subsection{Optimizing delivery of individual frames}

% A direct implication of the autoencoder's graceful quality degradation (Figure~\ref{??}) is the ability for the receiver (decoder) to trade delay for quality or vice versa, in a finer granularity than prior solutions. 
% Waiting for one more packet, which may slightly delay the rendering of a frame, always incrementally improve the quality of the frame, allowing the receiver to move along the quality-delay tradeoff in presence of delay/loss of multiple packets.
% In contrast, systems using FEC-based coding have to wait for a certain number of packets, due to the cliff effect (\S\ref{??}) of FEC.

% This property of data-salable autoencoder naturally lands itself to a transport mechanism in between UDP and reliably delivering every packet (or a fixed fraction of packets).
% The example in Figure~\ref{??} illustrates the workflow of how \name determines 



% \jc{
% \begin{itemize}
%     \item on coding a frame: i or p? which ref frame? which model?
%     \item on sending a frame: target sending rate or bitrate?
%     \item on receiving a frame: when to decode a frame?
%     \item on packet loss
% \end{itemize}
% }

% \jc{
% \begin{itemize}
%     \item explain our single-frame delivery module: 
%     \item (1) saliency-based redundancy
%     \item (2) selective retransmission
%     \item (3) multipath tcp extension
%     \item why? plot the impact of zeroing top k values
%     \item compare the original ae vs. new ae
%     \item takeaway: high-impact elements are rare, and impact of each packet is similar
% \end{itemize}
% }



% \subsection{Delivering a sequence of frames}

% \jc{
% \begin{itemize}
%     \item we have to think about long-term effects (propagation effects of \rate)
%     \item (1) packet prioritization in \name: evenly split among new packets.
%     \item contrast it with prioritizing retransmission in webrtc
%     \item (2) \name's way of selecting ref frame (on-demand synchronization)
%     \item explain the tradeoff: always sync-up (high overhead), always not sync-up (low quality)
%     \item empirical result: quality vs. \# of high-\rate frames
%     \item (3) bitrate adaptation: 
% \end{itemize}
% }

% \end{comment}


\section{Implementation}

\name is implemented with \fillme lines of Python (mostly for autoencoder NNs) and \fillme lines of C++ (for frame delivery and WebRTC integration).\footnote{The code and trained model of \name will be made public upon the publication of this paper.} 
We use the method described in \S\ref{??} to fine-tune \fillme~\cite{??} to get \newae's P-frame codec and \fillme~\cite{??} to get \newae's I-frame codec. 
The per-packet entropy encoding uses \fillme~\cite{??}. 



\subsection{Integration with WebRTC}
The integration with WebRTC is logically straightforward, since \newae (including I-frame and P-frame encodings) exposes very similar interface as the default codec in WebRTC. 
\jc{Ziyi, please fill in the details}

\jc{need to explain the gains are not directly from the entropy encoder or motion vector estimation}




\subsection{Optimizations}

While autoencoders are functionally similar to traditional codec (so is \newae), they face a few technical challenges to function as the codec in a real-time video client.
Note that these challenges are not unique to loss resilience, so we do not consider packet losses in the rest of the section. 


\mypara{Key frame insertion}
For the P-frame autoencoder we have tried, we observe that the decoded quality can be very high right after each I-frame but it gradually degrades after about 10 frames. 
A naive solution would be to encode an I-frame very often (say once every 10 frames).
This is obviously not ideal, because the I-frames are much larger than P-frames and sending a large frame frequently and a handful of small frames in between can cause great difficulties for congestion control and bitrate adaptation (which will be discussed shortly).\footnote{We have observed that many computer-vision papers on autoencoders have conveniently used a small GoP when compared against H.265, but the implication of large I-frame size for congestion control is rarely discussed.}

Instead of adding new I-frame frequently, \name encodes a small patch (about \fillme$\times$\fillme) as a tiny I-frame on {\em every frame} (the pixels outside the patch will be encoded as a P-frame), and the location of the patch on a frame changes, such that every $k$ frames, the patch will scan through the whole frame size. 
This scheme effectively ``amortizes'' the size of I-frames across $k$ P-frames, as illustrated in Figure~\ref{fig:keyframe_smooth}.
As a result, the frame size will have much lower variance than if I-frames are encoded entirely and inserted intermittently.

%\jc{
%\begin{itemize}
%    \item start with the need for more key frames (more than that in h265).
%    \item we "amortize" key frames in different frames. (better also to explain why this isn't possible in h264)
%    \item give a simple back-of-envelope estimate of the new size. figure~\ref{fig:keyframe_smooth}
%\end{itemize}
%}

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.85\linewidth]{figs/keyframe_smooth.pdf}
    \caption{}
    \label{fig:keyframe_smooth}
\end{figure}


%A client must be able to encode each frame at a given target size. 
\mypara{Encoding at multiple bitrates}
In real-time video, throughput estimation can vary even between two consecutive frames.
Thus, it is important that most frames are smaller than the target size set by congestion control, but traditional codecs are not able to do that. 
This has been observed in \cite{salsify}, which proposes to encode each frame at multiple quality levels in order to find an encoding that fits the target bitrate. 


\name provides a similar mechanism. 
First, it trains multiple autoencoders, each using a different weight of frame size $\alpha$ in its training loss function (\S\ref{3.1}).
The resulting autoencoders cover a bitrate range \fillme$\times$ difference between the highest bitrate and lowest bitrate. (A wider bitrate range is possible with more autoencoders.)
As long as the target bitrate is within this range, \name should select the autoencoder whose encoded frame size is lower than the target. 

\jc{need a figure here}

\mypara{Bitrate adaptation} 
To select an autoencoder with frame size lower than the target, we leverage an empirical property of these autoencoders (illustrated in Figure~\ref{??}): 
for each pair of a high-bitrate autoencoder (trained with a high $\alpha$) and a low-bitrate autoencoder (trained with a low $\alpha$), if we denote their encoded frame sizes on the same frame are $S_h$ and $S_l$, then $S_h/S_l$ is roughly constant, despite both $S_h$ and $S_l$ vary between frames. 
Thus, each time when a frame is encoded by one autoencoder, \name can then infer the frame size of other autoencoders on the same frame.
This information can be used to correct the estimated frame size of each autoencoder on current frames. 
This logic is similar to the rate control logic in H.264, which corrects the bitrate estimation based on the latest encoded frame sizes.


\mypara{Reducing memory footprint}
For the client to switch between multiple autoencoders (with different bitrates), their memory footprint in should be minimized, so more of them can be loaded in GPU memory to avoid delay of loading and unloading models. 
\name trains multiple autoencoders by fine-tuning the last 10-25\% layers of the same model (\ie they share the backbone layers), so only the one autoencoder and the last few layers of different autoencoders need to be loaded in GPU memory. 
This reduces the memory footprint of the models by \fillme\% compared to when all models are trained separately without sharing any layers.
A similar idea has also been used in Swift~\cite{swift} to reduce memory usage of multiple SVC layer encoders, though \name uses it to reduce memory footprint of data-scalable autoencoders of different bitrates.\footnote{A note on I-frames}


%\jc{
%\begin{itemize}
%    \item explain the rate adaptation logic. how we estimate frame size from complexity
%    \item show empirical correlation between complexity and frame size
%    \item connect it with rate control in h264.
%    \item talk about shared backbone to save memory footprint.
%\end{itemize}
%}


%\mypara{Reducing system overhead}
%Despite that sharing most NN layers (\S\ref{??}) greatly reduces the memory footprint of the multi-bitrate autoencoders, the compute overhead of autoencoder NNs remains substantial---100ms to encode a frame of \fillme$\times$\fillme on a \fillme GPU (though decoding can be much faster). 
%Note that this is already faster than the autoencoder used in a recent work for video streaming.
%Fortunately, because \name's autoencoder contains shallow NNs, the encoding and decoding of \newae can be greatly accelerated by OpenVino~\cite{??} and achieve \fillme even on CPUs. 
%\jc{kuntai/ziyi, fill in the details here}


\mypara{Reducing compute overhead}
Most research on autoencoder focuses on coding efficiency (using less bits to get higher quality), and the encoding, including \name's implementation, is usually slower than heavily engineered codecs like H.265.
That said, we show that \name's encoding speed can be greatly sped up and achieve an acceptable speed on typical commercial GPUs: from 5~fps on 720p HD (and \fillme~fps on 480p) videos by the off-the-shelf implementation to 18~fps (and \fillme~fps) on a single \$\fillme NVIDIA GeForce 3080 GPU). More results in \S\ref{??}. 

\name achieves such speedup by downsizing the image (by default $4\times$) during motion-vector estimation and motion compensation, and then upsample the motion-compensated image before calculating and encoding the residuals. 
This significantly speeds up encoding because motion-vector estimation and motion compensation are the slowest steps during P-frame encoding but their delay is proportional to the input dimension. 
At the same time, because the residuals are still computed between the full-resolution frame and the motion-compensated image, the compression efficiency is not affected for most frames.







% \jc{
% \begin{itemize}
%     \item how to integrate it in webrtc: same logical interface for video coding, packetization. replacing vp8
    
%     \item autoencoder highlight: entropy encoder, i-frame model, p-frame model
    
%     \item use of intel vino to reduce overhead
% \end{itemize}
% }




==> sections/old/technical_v5.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US

\newcommand{\Coder}{\ensuremath{C_\phi}\xspace}
\newcommand{\Decoder}{\ensuremath{D_\theta}\xspace}
\newcommand{\Quality}{\ensuremath{F}\xspace}
\newcommand{\Packetize}{\ensuremath{A}\xspace}
\newcommand{\X}{\ensuremath{\mathbb{X}}\xspace}
\newcommand{\x}{\ensuremath{\textbf{x}}\xspace}
\newcommand{\y}{\ensuremath{\textbf{y}}\xspace}
\newcommand{\z}{\ensuremath{\textbf{z}}\xspace}
\newcommand{\loss}{\ensuremath{P_{\textrm{loss}}}\xspace}
\newcommand{\DistributionEst}{\ensuremath{N_\phi}\xspace}




\tightsection{\newae: Data-Scalable Autoencoder}
\label{sec:training}

%\name is a concrete instantiation of data-scalable delivery. 
At a high level, \name uses a new data-scalable autoencoder, \newae and a custom delivery framework that leverages the new autoencoder (\S\ref{sec:delivery}) to balance tail delay and quality.
%We will describe the autoencoder design in this section, followed by the delivery framework in the next section. 


\tightsubsection{Basic formulation of \newae training}


%We begin with the preliminary of autoencoders. 
We denote the encoder (a neural network parameterized by weights $\phi$) by $\Coder$ and the decoder (a neural network parameterized by weights $\theta$) by $\Decoder$.
For an input frame $\x$ (a $c\times w\times h$ tensor), the coded data $\z=\Coder(\x)$ will be sent to the receiver, which then runs the decoder to reconstruct the original frame from $\z$: $\hat{\x}=\Decoder(\z)$.
Note that the encoder and decoder performing the lossy reconstruction are {\em separate} from the lossless entropy coding or FEC coding. (We will discuss entropy encoding and packetization in \S\ref{subsec:sim-losses}.)
We retrain the DVC autoencoder~\cite{dvc} to encode P-frames, and discuss how to add I-frames in \S\ref{subsec:delivery:iframe}.
(We do not consider B-frames as they are not commonly used in low-latency videos.)
%We customize two existing autoencoder architectures, \cite{dvc} for P-frames (with motion vectors and residuals as input) and \cite{qmap} for I-frames (with a static image as input).\footnote{We do not consider B-frames are they are not commonly used in low-latency videos.} 
%We borrow their neural network architectures (their architectures in details in \S\ref{app:arch}).
%Since they share the same conceptual framework described above, we do not discuss them separately unless necessary.

\mypara{Conventional autoencoder training}
An autoencoder is trained to minimize the ``loss'' function (not ``packet loss'') $\Quality(\hat{\x},\x)= Distortion(\hat{\x},\x)+\alpha\cdot Size(\hat{\x})$, which is a weighted sum of its pixel distortion $Distortion(\hat{\x},\x)$ (L2-norm of $\hat{\x}-\x$)\footnote{Pixel-wise distortion may not be the best way to capture human perception of reconstructed images, but it is often used in autoencoder training for its differentiability. We will evaluate the trained autoencoders in terms of more standard metrics, such as SSIM and PSNR (in RGB and YUV).} and its entropy-encoded size $Size(\hat{x})$ (\eg estimated by a pre-trained neural net).
A smaller $\alpha$ means that the output of $\Coder(\x)$ will tend to have better visual quality in $\Decoder(\z)$ but also higher bitrate. 
(We present \name's bitrate adaptation in \S\ref{subsec:optimize}.)
%To adapt to the dynamic sending rate, multiple versions of the autoencoders are trained, each with a different weight $\alpha$, and they share most (backbone) layers, which significantly reduces the memory footprint when switching between bitrates. (See \name's bitrate adaptation in \S\ref{subsec:optimize}.) 
% A higher $\Quality$ value is better (higher visual quality and/or lower entropy-coded size).
Since $\Coder$, $\Decoder$, and $\Quality$ are differentiable, the encoder and decoder NNs can be trained as an end-to-end architecture on a training video set $\X$:
\vspace{-0.08cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\z = \Coder(\x)
\label{eq:1}
\vspace{-0.08cm}
\end{align}


%\jc{anton/yihua, can you draw a simplified figure to depict the input/output of the used autoencoders? the figure should also include the tensor dimensions of the input and output. }

%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.95\linewidth]{figs/per-packet-encoding.pdf}
%    \caption{\name's packetization and per-packet entropy (arithmetic) encoding. When a packet is lost, the elements mapped to it will be set to zeros.}
%    \label{fig:per-frame}
%\end{figure*}



\mypara{Training data-scalable autoencoder}
The training process in Eq.~\ref{eq:1} can be seen as having no packet loss, \ie the decoder's input equals the encoder's output. 
To improve coding efficiency (low reconstruction distortion with fewer bits) under various packet loss rates, we use a custom training process that uses a random distribution $\loss$ to simulate packet losses:
\vspace{-0.1cm}
\begin{align}
\textrm{\bf max~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\z), \x)\textrm{, where }\color{purple}
\underbrace{\highlight{red}{$\z\sim \loss(\z | \Coder(\x))$}}_{\text{\sf \footnotesize \textcolor{purple!85}{Simulating packet losses}}}
\label{eq:2}
\vspace{-0.1cm}
\end{align}
%where the change is highlighted in color.
$\loss$ takes the encoder output $\Coder(\x)$ and returns the distribution of the data seen by the decoder after packet erasures under some \rate. 
%As we will see next, with appropriate randomization, $\loss$ can simulate the effect of packet losses on data received by the decoder.
Simulating packet losses in Eq.~\ref{eq:2} raises three unique questions, and we will address them next.
\begin{packedenumerate}
\item How should $\loss$ convert $\Coder(\x)$ to data packets to simulate the effect of dropping a packet? 
%This decides what data seen by the decoder would be if packets are randomly dropped. 
\item Given that the function $\loss$ may not be differentiable, how to train autoencoders with Eq.~\ref{eq:2}? 
\item What packet loss rates should be simulated in training so that the trained model can handle unseen loss rates?
\end{packedenumerate}
%It is important to note that these questions are not involved in canonical autoencoder training, but they become critical here for the need to simulate packet losses in the training process.
% \section{Simulating \rates in autoencoder training}



% \mypara{How to simulate packet losses}

%\mypara{Simulating packet losses in autoencoder training}
%Training a data-scalable autoencoder using Eq.~\ref{eq:2} faces three key questions:
%\begin{packedenumerate}
%\item How to make Eq.~\ref{eq:2} differentiable for a wide range of $\loss$ that simulates various packet loss patterns?
%\item How to convert $\Coder(\x)$ to data packets? This decides how losing a packet would affect the data seen by the decoder.
%\item What \rates should be simulated in training, so that the trained model can deal with a range of unseen \rates?
%\end{packedenumerate}
% The first question concerns packetization of the coder output and the second question concerns what \rates should be used to train the model that can deal with a range of \rates.

% , so that the trained model can handle packet losses of various \rates in real networks. 

\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v2.pdf}
    \tightcaption{\name's packetization and per-packet entropy (arithmetic) encoding. When a packet is lost, the elements mapped to it will be set to zeros.}
    \label{fig:per-frame}
\end{figure}


\subsection{\hspace{-0.2cm}Simulating packet losses during training}
\label{subsec:sim-losses}


\mypara{Packetization and data erasure}
First, to packetize the encoder output $\z=\Coder(\x)$, \name uses a {\em packetization function} $\Packetize$ (illustrated in Figure~\ref{fig:per-frame}) to map each element position in $\z=\Coder(\x)$ (a 3-D or 4-D tensor) to one of $k$ non-overlapping lists\footnote{\name uses 8, 16, 24 depends on the size of the input frame} and then losslessly encodes the elements in each list to a bitstream of a packet.
Conversely, depacketization first losslessly decodes each packet to a list of elements and maps elements back to their original positions in $\z$ by the inverse function $\Packetize^{-1}$.
One can use an off-the-shelf entropy coder to losslessly code the elements in a packet to a bitstream. 
With {\em per-packet} entropy coding (will explain in \S\ref{sec:entropy-coding}), each packet is individually decodable. 
(Similar technique is also commonly used in intra-MB insertion (explained in \S\ref{subsec:abstractions}) and other source-coding loss resilient schemes.)
\st{We use arithmetic coding
%~\cite{torchac} to encode each packet. 
Because the elements in each packet share the same distribution as all elements in Z
%$\z$\ 
(as we will show shortly), different packets share the same arithmetic coder (without needing a separate arithmetic distribution per packet), so each list has the same number of elements, the encoded packet size of the list will be roughly the same.}
%Because the elements in each packet are selected randomly from the entropy encoder's input, 
%This is different from typical autoencoders which entropy encodes the whole $\z$ tensor before packetization and thus any lost packet will make the received data not decodable by the entropy decoder. Moreover, since we use arithmetic coding (\fillme), so the total size of individually encoded packets is similar to the output of coding $\z$, if the elements in each packet share the same distribution as all elements in $\z$ (which is fortuitously ensured by random mapping. 

%(We discuss in \S\ref{app:entropy-encoding} \jc{need an appendix here} how to fit the bitstream in the normal packet size of 1.4KB.)


If a packet is lost, \name will set each element whose position is mapped to the lost packet to zero. 
Thus the packetization function $\Packetize$ decides how missing one packet would affect the coded data seen by the receiver.  
\name's packetization function is a {\em uniformly random} mapping (A pseudo-random function which has a reversible mapping\footnote{A reversible mapping allows the decoder to map elements from packets (including lost packets) back to the vector $\z$. An example can be mapping the $i^{\textrm{th}}$ element to the $j=(i*p\textrm{ mod }n)^{\textrm{th}}$ packet at the $(i*p-j)/n^{\textrm{th}}$ position, where $n$ is the number of packets and $p$ is a prime number.}). 
As a result, with a 30\% packet loss rate, $\loss(\z|\Coder(\x))$ will produce a distribution of $\z$ that randomly zeros 30\% of elements in $\z$.

\begin{figure}[t!]
    \centering
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/loss-distribution.pdf}
         \caption{Impact of different data loss distribution used during training}
         \label{fig:training_loss_distribution}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/loss-pattern.pdf}
         \caption{Impact of different data loss patterns used during training}
         \label{fig:training_loss_pattern}
     \end{subfigure}
     \vspace{.05cm}
     \tightcaption{Empirically comparing different ways of simulating packet losses. \jc{fixed loss => fixed loss rate}}
    \label{fig:training_loss_simulation}
\end{figure}

\mypara{Why random packetization}
The choice of randomized packetization empirically works better than alternatives, for two reasons. 
\begin{packeditemize}
\item In an autoencoder output $\z$, some elements have more impact on the decoded quality (defined in \S\ref{subsec:understanding}).
%, and zeroing each important element has disproportionally higher impact on the decoded quality than zeroing other elements.
A random mapping thus makes sure that losing $x\%$ packets will affect $x\%$ important elements (whereas non-randomized packetization may affect more than $x\%$ important elements).
\item A random mapping ensures that all elements in $\z$ have the same distribution as those mapped to each packet. This makes it easier to maintain roughly the same entropy-encoded size of each packet. 
\end{packeditemize}

Figure~\ref{fig:training_loss_distribution}(a) empirically compares \newae trained with the random packetization and \newae trained with alternative schemes, such as block-based packetization (\ie each packet contains a contiguous block of elements in $\z$) and interleaving-based packetization. 
Both are suboptimal, since important elements can be next to each other and have a fixed distance from each other under $\z$'s specific tensor structure, so in the worst case both block-based packetization and interleaving packetization can drop a higher fraction of important elements than packet loss rate.


\mypara{Choice of packet loss rate in training}
At first glance, we should simulate as many packet loss rates during training as possible, so that the model can deal with various packet losses.
However, our empirical results (Figure~\ref{fig:training_loss_simulation}(b)) suggest that adding too much randomness in \loss might make the training converge to suboptimal autoencoder models. 
Specifically, training \newae with just a few values of packet loss rates generalizes better than with a wide range of packet loss rates, even on unseen test packet loss rates.
Moreover, the packet loss rates in training should include 0\% (otherwise the trained autoencoder will perform significantly worse than the pre-trained autoencoder on low packet loss rates. 


%\name uses a {\em random} mapping $\Packetize_{random}$ 
%
%This choice of  $\Packetize$ is driven by two reasons. 
%An inverse function $\Packetize_{random}^{-1}$ (\eg\fillme) can then be used to map the packet data back to $\z$). 
%Once the packetization method is selected, packet losses can then be simulated by zeroing the elements assigned to certain number of packets (we will discuss the choice of packet loss rates used in training shortly). 
%Each packet is numbered so if a packet has not arrived when decoding, the elements mapped to it will be set to zero (this is a natural choice, though we will discuss alternatives in \S\ref{??}). 
%
%%\jc{start with how WE do packetization, including per-packet entropy coding, and then list the alternatives}
%
%We compare the choice of random assignment with two strawmen:
%\begin{packeditemize}
%\item Block-based assignment splits $\z$ to {\em contiguous} blocks so elements close together will be encoded in the same packet, much the same way video data is packetized today. 
%This serves a reference design point.
%\item Interleaving assignment assigns the $i^{\textrm{th}}$ element to the $(i\textrm{ mod }k)^{\textrm{th}}$ packet, where $k$ is the number of packets.
%Interleaving-based packetization is recommended by some traditional loss-resilient schemes~\cite{??}.
%\end{packeditemize}
%Once the packetization method is selected, packet losses can then be simulated by zeroing the elements assigned to certain number of packets (based on \rates selected in \S\ref{??}). 


%\myparaq{Why randomized assignment}
%\name chooses randomized assignment over the block-based and the interleaving ones. 
%The intuitive reason is that 
%
%\jc{\begin{itemize}
%\item why better than block-based? some elements in autoencoder output are more important than others and the important ones are sometimes put together
%\item why better than interleaving? the elements in autoencoder output have structures that align with tensors, etc. so interleaving may destroy some channels entirely.
%\end{itemize}}
%
%Figure~\ref{??} empirically compares these schemes (while fixing other factors, such as packet loss rate and training and testing data).
%\jc{Some initial results.}

% \begin{figure}[t!]
%     \centering
%          \centering
%         \includegraphics[width=0.85\linewidth]{figs/per_frame_quality_degradation_v2.pdf}
%     \caption{}
%     \label{fig:degradation}
% \end{figure}


%\begin{figure*}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.92\linewidth]{figs/transmission_overview.pdf}
%    \caption{Overview of \name's frame delivery workflow.}
%    \label{fig:overview}
%\end{figure*}




%we need to make Eq.~\ref{eq:2} trainable for the weights ($\theta$ and $\phi$) when $\loss$ is a random function. 
%A challenge imposed by Eq.~\ref{eq:2} is how to train the weights ($\theta$ and $\phi$) of the autoencoder, despite that the random distribution $\loss$ is not a naturally differentiable step. 

% that the expected value of $\Quality$ may not always be written in a closed, differentiable form, so before we discuss how \loss simulate packet losses with a non-zero \rate, we must first be able to run backpropagation for weights $\theta$ and $\phi$ in Eq.~\ref{eq:2}. 


%\jc{Yihua/Anton, please explain how you used REINFORCE trick here.
%\begin{itemize}
%    \item this may look like VAE, so a natural solution is reparameterization. it doesn't work because the expectation of $\Quality$ cannot be writtein in a closed, differentiable form
%    \item we use reinforce trick.. how does it work?
%\end{itemize}}

%With the application of packet loss, the loss function is not differentiable, hence the gradient of the expectation of $\Quality$ cannot be directly calculated. To tackle this, we use the reinforce algorithm for reparameterization (\eg~\cite{Kingma2014}). 
\mypara{Making \newae trainable}
Since $\loss$ is a non-differentiable random function, the gradient of the expectation of $\Quality$ in Eq.~\ref{eq:2} cannot be directly calculated. 
To address this issue, we use the REINFORCE trick~\cite{Kingma2014} for reparameterization. 
We express the gradient of Eq.~\ref{eq:2} as
% According to differentiation property of logarithms, we can 

$$ \nabla_\phi \loss(\z) =  \loss(\z) \nabla_\phi \log{\loss(\z)}$$

where $\loss(\z)$ is our packet loss distribution so our gradient of the expectation of $\Quality$ becomes
\begin{multline}
\nabla_\phi \mathbb{E}_{x\sim \loss(\z)}([\Quality(\Decoder(\z), \x)]) \\ 
= \mathbb{E}_{\z\sim \loss(\z)}([\Quality(\Decoder(\z), \x)\nabla_\phi \log{\loss(\z)}])
\end{multline}
which can be estimated using Monte-Carlo sampling
$\approx \frac{1}{N} \sum_{i=1}^{N} \Quality(\Decoder(\z_i), \x) \nabla_\phi \log{\loss(\z_i)} $
Since in our application the loss is independent and identically distributed random variable, the gradient evaluates to either $0$ or $1$, hence we propagate the gradients for the encoder only for $\Quality(\Decoder(\z_i), \x)$ where $\loss(\z_i) = 1$.


\begin{comment}

\subsection{Choice of packet loss rate in training}
\label{subsec:sim-lossrate}

%As the packet loss rate varies over time, a desirable autoencoder should fare well under unseen packet loss rates.
%We acknowledge that it remains an open question what packet loss rates should be used to train \newae to obtain ideal generalization under unseen packet loss rates. 
%But we try our best to explore different strategies of setting packet loss rates. 

At first glance, we should simulate as many packet loss rates during training as possible, so that the trained model can fare well under various packet losses.
However, we found that adding too much randomness in \loss might make the training converge more slowly and even to suboptimal autoencoder models. 
Specifically, our empirical results show that (1) training \newae with just a few values of packet loss rates generalizes better than with a wide range of packet loss rates, even on unseen test packet loss rates, and (2) the packet loss rates in training should include 0\% (otherwise the trained autoencoder will perform significantly worse than the pre-trained autoencoder on low packet loss rates. 

\jc{yihua/anton, please add a figure here to compare psnr-vs-loss under different training loss distributions}

To illustrate them, Figure~\ref{fig:training_loss_distribution} compares three choices of training packet loss rates.
\begin{packeditemize}
\item {\em Distribution-1:} $\loss = 30\%$ all the time.
\item {\em Distribution-2:} For half of the times, $\loss = 30\%$, and for another half of the times, $\loss = 0$.
\item {\em Distribution-3:} $\loss$ is uniformly chosen from $\{0, 20\%, 40\%, 60\%\}$.
\end{packeditemize}
\name uses Distribution-2. As shown in figure~\ref{fig:training_loss_distribution}, the model trained with Distribution-2 outperforms the other ones when loss ratio is between 0 to 40
\%. When loss ratio is 0, which is the most common cases, \name can have 0.85 and 0.71 higher PSNR comparing with the model trained with Distribution-1 and Distribution-3.
%\jc{yihua/anton, please fill in a short para on the read of the figure}

The intuition that more training packet loss rates might not help is that \fillme

\end{comment}

%\jc{
%\begin{itemize}
%    \item experiment setup
%    \item empirical findings: 
%    (1) must have zero loss rate
%    (2) more \rates doesn't help
%\end{itemize}
%}




\tightsubsection{Why is \newae data-scalable?}
\label{subsec:understanding}

%As illustrated in Figure~\ref{fig:autoencoder-pretrained}, compared to the pre-trained autoencoder (which is already data-scalable), \newae (re-trained on the same video dataset but with packet losses) achieves much higher quality on unseen videos under various test packet loss rates, even those that are {\em not} seen during training. 
%This remarkable improvement begs the question why \newae can be much more resilient to packet losses. 

We believe that the reasons are two-fold. 
First, compared to SVC, FEC, or H.26x-based coding, the elements in \newae's encoding output (before entropy encoding) do not impose any strict structure (\eg hierarchy or dependencies). 
Instead, the relationship between elements in \newae output is ``flat'', and changing any element (to zero) would not render the frame non-decodable. 

\newae's decoder can be seen as a special case of variational autoencoders (VAE)~\cite{pu2016variational}, which are generative neural networks trained to create realistic images from a {\em random point} in the input space. 
In the case of \newae, our random point follows the distribution of $\loss$. 

Second, compared to the pre-trained autoencoder, individual elements in \newae's output have a lower impact on the decoding quality, so quality degrades more gracefully with more lost data.
Though the NNs are too complex to show this directly, we can indirectly illustrate it as follows.
For a frame, we first calculate the ``gradient'' of decoding quality with respect to each element in $\z$.
%Mathematically, the gradient of decoding quality with respect to elements in $\z$ is a vector:
$gradient=\frac{\partial \Quality(\Decoder(\z),\x)}{\partial\z}$.
Then, we sort the elements in descending order of their gradients. 
% If top $k$ elements are zeroed, the incremental impact on decoding quality is marginal. 
As more top $k$ elements are zeroed, we observe that the quality of the pre-trained autoencoder drops sharply, whereas that of \newae drops much more slowly (not shown for space limitation). 



%\jc{
%\begin{itemize}
%    \item \newae's performance is surprising, but can be explained.
%    \item flat relationship among elements, no strict hierarchy/dependencies like in svc or fec
%    \item saliency is more robust to losses: figure~\ref{fig:per-frame}
%\end{itemize}
%}




\tightsection{Per-packet entropy coding}\label{sec:entropy-coding}

Traditional video codecs (such as H.265 and VP9) and state-of-art video autoencoders~\cite{dvc,??} use entropy encoding to compress the encoded video {\em before} doing packetization. However, if any part of the entropy-encoded bytestream is lost or corrupted, the whole bytestream cannot be decoded anymore. Therefore, such entropy encoding method prevents the codec being data-scalable. In \newae, we have a new design that does per-packet entropy encoding {\em after} packetization so that any lost packet will not impact the decodability of other packets.
%(preamble: Why we need per packet entropy coding to make \newae data-scalable? Contrast with state-of-art AEs and traditional video codecs: entropy coding then packetization V.S. packetization then entropy coding )
\yihua{how do traditional codecs do entropy encoding -- a natural starting point for readers to understand per-packet entropy coding. Traditional entropy coding --> slightly different entropy coding in autoencoders --> our new solution}

\mypara{Entropy coding in autoencoders}
Entropy coding is a {\em lossless} compression step that encodes $\z$ into a smaller-sized bytestream at the encoder side and decodes the bytestream back to original $\z$ at the decoder side. 
Most of video autoencoders~\cite{dvc,??} including \newae, use arithmetic coding~\cite{torchac} as the entropy coding algorithm.

When compressing $\z$, the entropy encoder takes $\z$ and the {\em distribution of each element} in $\z$ as the input. To decode the bytestream, the entropy decoder needs the bytestream and the same distribution used during encoding. 
Elements in $\z$ usually have different distributions across different frames. Therefore, autoencoders~\cite{dvc,??} use a small neural network $\DistributionEst$ to estimate the distribution for the current $\z$. The estimated distribution will also be encoded into a small bytestream and sent together with $\z$.

% \begin{itemize}
%     \item Input: tensor Z + per-element distribution. Output: a bytestream
%     \item Since the tensor Z of different frames may have different distributions, autoencoders[] use a small neural network to estimate the distribution
%     \item The estimated distribution will also be encoded into a small bytestream and sent with the frame
% \end{itemize}

\mypara{A strawman solution} A working strawman of per-packet entropy encoding has following steps: {\em (i)} Randomly packetize elements in $\z$ into multiple parts as described in \S\ref{subsec:sim-losses}. {\em (ii)}  For each part, assemble the elements to a smaller-sized $\z$ and feed it to $\DistributionEst$ to get the estimated distribution. {\em (iii)} For each part, use the entropy encoder and the estimated distribution to encode the elements to a bytestream. The estimated distribution will also be compressed put into the same packet.

This strawman solution satisfies the requirements of per-packet entropy coding: every arrived packet will be decodable no matter other packets is arrived or not. However, after implementing the strawman, we find it has a huge size inflation -- , the size of the encoded bytestream is \fillme\% larger when comparing to the default entropy encoding schema (\ie, entropy encode the whole $\z$ before packetization). To put the number into context, the PSNR of the frame encoded using the strawman will decrease from \fillme to \fillme when the size of the bytestream is the same as using the default entropy encoding schema.

The cause of such size inflation is the mismatch between the estimated distribution and real distribution of the elements. For example, the estimated distribution indicates an element is highly likely to be zero, while the actual value of element is a large positive number. We discover that in the original $\z$, there is an important feature that adjacent elements usually have similar distribution. However, after randomized packetization, such feature no longer exists. Therefore, $\DistributionEst$ cannot give an accurate distribution estimation after randomized packetization.

% Describe the strawman solution and why it works
% \begin{itemize}
%     \item step 1: randomized packetization
%     \item step 2: estimate the per-element distribution
%     \item step 3: entropy encode the tensor and the distribution for each packet. 
%     \item it's a working solution, because no packet is depending on other packets to decode.
% \end{itemize}

% The problem in the strawman solution: size inflation
% \begin{itemize}
%     \item The strawman solution will have a size inflation of \fillme comparing with entropy encode the whole tensor. This will cause a decrease of \fillme in the end to end PSNR
%     \item The reason of size inflation: per-element distribution is not correct after randomized packetization (for example: ...)
% \end{itemize}

\mypara{Per-packet entropy coding in \newae}
The solution of per-packet entropy coding in \newae is based on the following key insight: the elements will have similar distribution if they are from the same {\em channel}\footnote{In \newae, $\z$ is a 3-D tensor and each element in $\z$ can be indexed by a triplet $(c, h, w)$. Elements from the same channel refers to the elements having the same $c$ (the first number in the triplet) in their index.} in $\z$. More specifically, in the same channel, either most ($>$ 99\%) of elements are zero, or a large portion of elements are non-zero values. We also find that this feature is irrelevant to video contents. 

Based on the insight, then entropy encoding in \newae has the following steps: {\em (i)} Estimate the distribution for each channel in $\z$. {\em (ii)} For each packet, randomly take a subset of elements from every channel by applying the same packetization function defined in \S\ref{subsec:sim-losses} for each channel. {\em (iii)} For each packet, entropy encode the elements using the distribution. In practice, the channel-wise distribution can be encoded to a bytestream of 30-50 bytes, so every packet can have a copy of such distribution. Therefore, every arrived packet can be decodable no matter other packets is arrived or not.

Since we are sacrificing the granularity of distribution (from per element to per channel), on concern is it may also cause size inflation comparing the default entropy encoding schema (\eg entropy encoding before packetization). We test our per-packet entropy coding method among \fillme different videos covering different contents and the average overhead on the encoded frame size is only \fillme.
\yihua{figure to show the overhead across videos?}

% \begin{itemize}
%     \item key insight: elements in tensor Z will share similar distribution if they are in the same "first dimension". (for example ...). This feature holds for different content types.
%     \item Solution: We assume elements having the same "first dimension" shares the same distribution. during encoding, we estimate the distribution and send it along all the packets
%     \item tradeoff: the compression ratio will be a bit lower comparing to entropy encode the whole tensor, but randomly shuffle within a tensor will never cause size inflation.
%     \item real numbers: what's the size of end to end overhead among different videos.
% \end{itemize}







\tightsection{Real-time video delivery over \newae}
\label{sec:delivery}

\name is built on the data-scalable autoencoder \newae. 
%\name is a concrete real-time video communication system built on a data-scalable autoencoder (\newae).
We focus on unique issues arising from the use of \newae as the codec, including how to deliver each frame to strike a desirable delay-quality tradeoff, and how to deliver a sequence of frames when congestion or packet losses affect multiple frames. 
The choice of the congestion control logic is complementary to \newae. 
In \S\ref{subsec:eval:e2e}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{carlucci2016analysis} or Salsify CC~\cite{salsify}. 
We do not claim that \name's strategies are new (\eg reference frame synchronization has been used in~\cite{salsify}). 
Nonetheless, \name integrates concrete design choices driven by the need, in order to unleash the full potential of \newae and its data-scalable codec primitive.

% Here, we highlight three major modifications (more autoencoder-specific optimizations are discussed in \S\ref{subsec:optimize}).


%We group these issues in two categories. 
%\begin{packeditemize}
%\item First, optimizing the delivery of a single frame to optimize the delay-quality tradeoff. 
%\item Second, optimizing the delivery of a sequence of frames when congestion or packet losses persist.
%% synchronize the coding/decoding states between the sender and receiver?
%\end{packeditemize}


%\mypara{Workflow and modules}
%Figure~\ref{fig:overview} depicts 

\begin{comment}
\name's framework comprises three high-level modules: the codec (\newae), the congestion controller, and the transmission controller.
The congestion controller decides the sending rate, and the choice of the congestion control logic is complementary to \newae. 
In \S\ref{??}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{??} or Salsify CC~\cite{??}. 

The transmission controller determines how to packetize \newae coder's output (coded data), deliver the packets, and depacketize all or a subset of packets to the input of \newae's decoder. 
Other than the codec (\newae), most \name's changes are made in the transmission module. 
We do not claim that any of the modifications are exactly new (\eg a variant of reference frame synchronization has been used in~\cite(salsify)). 
Nonetheless, \name integrates concrete design choices driven by the need, in order to unleash the full potential of \newae and its data-scalable codec primitive.

% \jc{we logically separate the system into two level: delivering each single frame and delivering a sequence of frames. }

Here, we highlight on on three major modifications (more autoencoder-specific optimizations are discussed in \S\ref{??}).

%\jc{we don't specify the protocol as they follow naturally from the design and is not our main contribution}
\end{comment}


\tightsubsection{Encoding a sequence of frames}
\label{subsec:delivery:iframe}

%To stream a sequence of video frames, a key question is how often I-frames should be inserted in P-frames. 
Placement of I-frames poses a particular challenge for \name's autoencoders (both pre-trained and re-trained), for two reasons: (1) I-frames are generally bigger in size than P-frames, and 
(2)  while the first few P-frames after an I-frame enjoy high quality, quality gradually degrades after about 10 frames. 
%(As explained in \S\ref{subsec:ae-background}, \name uses only I-/P-frames, as in most real-time video systems.)
%For the P-frame autoencoder we have tried, we observe that the decoded quality can be very high right after each I-frame but it gradually degrades after about 10 frames. 

A strawman would add I-frames frequently (say every 10 frames)\footnote{Many computer-vision papers on autoencoders have conveniently used a small GoP when compared against H.265, but the implication of large I-frame size for congestion control is rarely discussed.}.
Even though this might achieve a decent tradeoff between quality and {\em average} bitrate (comparable to H.264 and H.265 with large I-frame intervals), sending I-frames (which have bigger sizes than the P-frames in between) frequently will make it difficult for congestion control to send the frames at a fixed interval (inversely proportional to the frame rate).


To add I-frames frequently without the intermittent bitrate spikes caused by the I-frames, \name encodes a small patch (about 128$\times$128 to 512$\times$512) as a tiny I-frame, which we call {\em I-patch}, on {\em every frame} %(the pixels outside the I-patch will be encoded as a P-frame)
(an I-patch will not impact the original P-frame), and the location of the I-patch on a frame changes over time such that the I-patch will scan through the whole frame size every $k$ frames. 
Depending on the original frame size, $k$ varies between 6 and 20. 
This scheme effectively ``amortizes'' the size of I-frames across $k$ frames, thus smoothing the frame size as well as quality across frames (illustrated in Figure~\ref{fig:keyframe_smooth}).
Moreover, since the I-frame autoencoder's encoding delay is proportional to the input size, encoding a small I-patch adds only a small compute overhead for each frame.\footnote{We should clarify that design choice of frequent I-frames works well for autoencoders, but {\em not} for classic codecs for two reasons. First, an I-frame generated by our autoencoder is only 2-5$\times$ bigger than a P-frame, whereas this ratio in H.264 is 4-10$\times$. Second, the P-frame quality in H.264 is relatively stable, whereas the quality of a P-frame is high following an I-frame (or an I-patch).}





\begin{figure}[t!]
    \centering
    
        \includegraphics[width=0.85\linewidth]{figs/split-iframe-size.pdf}
    \tightcaption{Encoding each P-frame with a small I-patch leads to smoother frame sizes than naively inserting I-frames.}
    \label{fig:keyframe_smooth}
\end{figure}



\tightsubsection{Packet losses across multiple frames}

An important benefit of adding an I-patch (a tiny patch encoded as an I-frame without referring to previous frames) at a different place in each frame is: each patch will be encoded as an I-patch every $k$ frames. 
This has a significant implication for loss resilience over multiple consecutive frames. 

%\mypara{Encoding/decoding synchronization}
An acute reader may realize a potential problem arising from encoding and decoding being asynchronous. 
For instance, when the sender encodes the $10^{\textrm{th}}$ frame as a P-frame, it needs the decoded the $9^{\textrm{th}}$ frame as the reference (to compute motion vectors and residuals), and without knowing which of the $9^{\textrm{th}}$ frame's packets will be lost, it will assume that the $9^{\textrm{th}}$ frame is decoded with all packets being received. (This is common to classic codecs and autoencoders.)
However, if the receiver decodes the $9^{\textrm{th}}$ frame with only a subset of its packets, the actual reference frame used to decode the $10^{\textrm{th}}$ will differ from what the encoder has assumed. 
Thus, most codecs require all packets of the $9^{\textrm{th}}$ frame to be received before decoding it (thus longer delay), or let the sender encode the $10^{\textrm{th}}$ based on an earlier reference (say the $5^{\textrm{th}}$) whose lost packets are already known to the sender. 
The latter {\em synchronizes} the encoding and decoding states (like in Salsify~\cite{salsify} during packet losses), but it also inflates the frame size, since the difference between the $10^{\textrm{th}}$ and the $5^{\textrm{th}}$ frames  is much greater than between the $10^{\textrm{th}}$ and the $9^{\textrm{th}}$ frames. 


%the P-frame encoding of the $10^{\textrm{th}}$ frame will have a low quality when being decoded with a different reference frame than the encoder has assumed. 




\name uses a simple yet efficient solution---it does not always synchronize the encoding/decoding state on every single frame; instead, it relies on the frequent I-patches (explained in \S\ref{subsec:delivery:iframe}) to synchronize the encoding/decoding states in each patch-size region. 
This works for two reasons.
First, without synchronizing the encoding and decoding states, \newae's quality degradation increases only marginally when multiple consecutive frames (less than about 10) are affected by packet losses.
For instance, applying a 50\% packet loss rate on one single frame can reduce PSNR by 3-4, and applying the same loss rate on 5 consecutive frames reduces PSNR by 7-9. 
%\jc{this corroborates our empirical improvements in \S\ref{??}}
%quality degrades by \fillme\% when 10 consecutive frames are affected by 50\% packet losses without the clients synchronizing their encoding/decoding states. 
Second, each patch will be encoded as an I-patch every $k$ frames ($k$ is between 6 and 20), so the impact of packet losses will not last for more than $k$ frames if the next I-patch is not lost. 
That said, in the worst case, if the I-patches of the same region are dropped persistently, this could cause bad decoded pixel values (\ie a small patch of white pixels), though we have observed it extremely rarely.




\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.995\linewidth]{figs/decode_time.pdf}
        \includegraphics[width=0.995\linewidth]{figs/decode_time_v2.pdf}
    \tightcaption{
    \name waits for the next frame until a deadline $t^*$, after which the utility is lower even if the next packet arrives.
    % At the arrival of the $i^{\textrm{th}}$ packet, \name decides the maximum wait time for the next packet.
    }
    \label{fig:decode-time}
\end{figure}

\tightsubsection{Choosing when to decode a frame}

The data-scalable abstraction allows the receiver to flexibly decide, as packets arrive at the receiver, whether to decode the frame using currently arrived packets or wait for more packets in hope of improving the quality. 
(In contrast, with FEC, the receiver will always wait until enough data is received.)
%(In other loss-resilient schemes (\S\ref{??}), the receiver must wait for more packets until the data is decodable.) 
%\name embraces this flexibility with the following logic to trade frame delay with decoded quality. 

To make this decision, \name defines the {\em utility} of a frame as a linear combination of decoding quality and frame delay (since the natural decoding time) on each frame: $Q(|\{\textrm{pkts before }t\}|)-\beta\cdot t$, where $t$ is when the frame is decoded, $Q(n)$ is the frame's decoding quality with $n$ packets 
The precise values of $Q(n)$ are frame-dependent, but they are roughly similar across frames, so \name estimates $Q(n)$ using history frames.
%, and $\tau$ is the frame's natural decoding time (\eg 40ms after the last frame was decoded with frame rate 25fps).
%In our experiment, we set parameter $\beta=\fillme$.
This objective works well in practice, though there might be other objectives that better capture users' quality perception. An optimal design of such utility is beyond the scope of this paper. 


With this utility in mind, Figure~\ref{fig:decode-time} illustrates \name's logic: on receiving the $i^{\textrm{th}}$ packets of a frame (not necessarily the $i^{\textrm{th}}$ sent packet) at time $t_i$, the receiver will immediately decode the frame if all packets of the frame have arrived; otherwise, it will wait for the next packet of the frame until a deadline $t^*=t_i+\frac{1}{\beta}\cdot(Q(i+1)-Q(i))$, and if it has not received the $(i+1)^{\textrm{th}}$ packet by then, it will decode the frame with $i$ packets. 
The reason is that if the next packet comes at time $t_{i+1}$ after $t^*$, the utility $Q(i+1)-\beta\cdot (t_{i+1}-\tau)$ will be lower than the utility $Q(i)-\beta\cdot (t_i-\tau)$ if the receiver does not wait at all\footnote{This is because {\scriptsize $Q(i+1)-\beta\cdot (t_{i+1}-\tau)<Q(i+1)-\beta\cdot (t^*-\tau)=Q(i)-\beta\cdot (t_i-\tau)$}}. 
%Here, $\beta$ is a tunable parameter, and $Q(n)$ is the quality of the frame based on $n$ packets.
This strategy makes intuitive sense: the receiver will wait longer if the improvement in quality by getting one more packet (\ie $Q(n+1)-Q(n)$) is higher, but it will not wait for too long.

%If a packet comes, the utility will be $Q(n)-1/\beta\cdot \beta\cdot(Q(n+1)-Q(n))$






%When there is at least one more packet missing, the receiver estimates the distribution of the interval to the next packet arrival using past inter-packet intervals.
%With this distribution and the quality-packet profile (Eq.~\ref{eq:3}) of the \newae that encodes the frame, \name's receiver chooses to decode a frame when \jc{an equation here}

%\jc{Ziyi and Hanchen: please add a nice description of your logic here}
%
%This strategy is a well-defined, in sense that it will not decode a frame when new packets are expected to arrive, nor will it wait for more packets if the next packet arrives a long time later. 
%\jc{can we also use an illustrative example to help people understand it?}



%\jc{
%\begin{itemize}
%    \item start with the need for more key frames (more than that in h265).
%    \item we "amortize" key frames in different frames. (better also to explain why this isn't possible in h264)
%    \item give a simple back-of-envelope estimate of the new size. figure~\ref{fig:keyframe_smooth}
%\end{itemize}
%}



\begin{comment}
\subsection{Saliency-based redundancy}

Recall from \S\ref{??} that with data-scalable primitive, the quality of a frame depends on the fraction of packets received (under a fixed coder state). 
Thus, it would be ideal to packetize the \newae coder's output in a way that improves the quality when a certain fraction of packets are received.

To this end, \name uses a novel strategy based on the randomization packetization used in \newae training (\S\ref{??}), but optimizes the quality under a given number of packets by leveraging the {\em skew distribution} of high-saliency elements in \newae coded data. 
Here, saliency is defined in the same way as Eq.~\ref{eq:3}, \ie if an element has a high saliency, changing it has a higher impact on the decoded quality than other elements. 
To motivate our strategy, we run analysis across \fillme videos in our dataset and the \newae models of \fillme different quality levels. 
Overall, the sum of saliency of the top \fillme-\fillme\% of elements is higher than the sum of saliency of all remaining elements. \jc{need a few words on why saliency is skewed? will it contradict fig~\ref{fig:per-frame}?}

These skewed distributions of saliency suggest that giving the high-saliency elements more protection can improve decoded quality, even at a cost of slightly more bytes. 
\name employs a simple yet efficient strategy of duplicating the top \fillme\% elements with the highest saliency. 
\jc{more details of the exact strategy}



\subsection{Choosing when to decode a frame}

As new packets arrive at the receiver queue (the internal jitter buffer), the data-scalable abstraction allows the receiver to flexibly decide whether to decode the frame now using currently arrived packets or waiting for more packets in hope of improving the quality. 
In contrast, with FEC-based loss-resilient schemes and other H.26x-based schemes (\fillme), the receiver simply has to wait for more packets until the data is decodable. 

\name embraces this flexibility by carefully trading frame delay with decoded quality. 
When there is at least one more packet missing, the receiver estimates the distribution of the interval to the next packet arrival using past inter-packet intervals.
With this distribution and the quality-packet profile (Eq.~\ref{eq:3}) of the \newae that encodes the frame, \name's receiver chooses to decode a frame when \jc{an equation here}

\jc{Ziyi and Hanchen: please add a nice description of your logic here}

This strategy is well-defined, in the sense that it will not decode a frame when new packets are expected to arrive, nor will it wait for more packets if the next packet arrives a long time later. 
\jc{can we also use an illustrative example to help people understand it?}


\subsection{Packet scheduling by the sender}

\jc{need to discuss it}

In a WebRTC's sender, retransmitted packets (specified in selective/negative acks) are always prioritized over new packets, simply because selectively retransmitted packets are required by the receiver to decode a prior (reference) frame. %\footnote{Exceptions exist, \eg Salsify may skip certain frames.}
\name rethinks this seemingly natural choice and instead prioritizes new packets in order to leverage data-scalable delivery.
The reason is that a receiver in \name can decode anytime after it receives the first packet, so a retransmitted packet may not be useful if it arrives after the frame is already decoded. 
On the other hand, each packet of a new frame, if delivered, is more likely to arrive before the receiver decodes the new frame and can thus improve its quality. 

To make it work, the sender and the receiver be aware of the other's decision, regarding whether a previous frame's packets are still being resent or 



%\mypara{Extension with multi-path TCP}
%\jc{more text}


\subsection{Reference frame synchronization}

\jc{need to discuss it}

An acute reader may have realized an unresolved issue, arising from encoding and decoding being asynchronous. 
If the $(i+1)^{\textrm{th}}$ frame is a P-frame, by default the sender will encode it with the decoded $i^{\textrm{th}}$ frame as the reference (used to compute motion vectors and residuals) with the assumption that the $i^{\textrm{th}}$ was fully received by the receiver. 
Now, if the receiver decodes the $i^{\textrm{th}}$ frame with only a subset of its packets, the P-frame encoding of the $(i+1)^{\textrm{th}}$ frame have a low quality when being decoded with a different reference frame than the encoder has assumed. 

A natural strawman to prevent such quality degradation is always letting the receiver piggyback ``which frame was recently decoded using which packets (just the packet IDs would be sufficient)''. 
With this knowledge, the sender can reconstruct the identical latest frame decoded by the receiver (autoencoder decoding is deterministic), and use this reconstructed frame, rather than the immediate last frame, as the reference of the next P-frame.
However, this means that there will be a non-trivial gap between the reference frame and the frame being encoded, making the P-frame significantly bigger than if the very last frame is used as the reference. 
Such gap between the two frames is usually 3-5 frames (though the exact value depends on the propagation delay), and the P-frames are about \fillme$\times$ bigger. 


To prevent quality degradation with minimum frame size inflation, \name leverages the loss-resilience of \newae. 
Empirically, \newae can tolerate out-of-sync encoding/decoding states for several consecutive frames. 
Figure~\ref{??} \jc{more text}

Inspired by these empirical observations, \name uses a simple logic, referred to as lazy synchronization, to 

\end{comment}

% \begin{comment}


% As we have seen, a data-scalable autoencoder is well-suited for connections with dynamic \rates, since its quality is near-optimal under no missing packets but degrade gracefully under higher \rates. 
% While the proposed autoencoders can be functionally integrated in WebRTC or other real-time video platforms by simply replacing the video codec, \name makes several logically simple yet crucial modifications to the video streaming system, to maximally embrace the advantages of data-scalable autoencoders.



% \subsection{Optimizing delivery of individual frames}

% A direct implication of the autoencoder's graceful quality degradation (Figure~\ref{??}) is the ability for the receiver (decoder) to trade delay for quality or vice versa, in a finer granularity than prior solutions. 
% Waiting for one more packet, which may slightly delay the rendering of a frame, always incrementally improve the quality of the frame, allowing the receiver to move along the quality-delay tradeoff in presence of delay/loss of multiple packets.
% In contrast, systems using FEC-based coding have to wait for a certain number of packets, due to the cliff effect (\S\ref{??}) of FEC.

% This property of data-salable autoencoder naturally lands itself to a transport mechanism in between UDP and reliably delivering every packet (or a fixed fraction of packets).
% The example in Figure~\ref{??} illustrates the workflow of how \name determines 



% \jc{
% \begin{itemize}
%     \item on coding a frame: i or p? which ref frame? which model?
%     \item on sending a frame: target sending rate or bitrate?
%     \item on receiving a frame: when to decode a frame?
%     \item on packet loss
% \end{itemize}
% }

% \jc{
% \begin{itemize}
%     \item explain our single-frame delivery module: 
%     \item (1) saliency-based redundancy
%     \item (2) selective retransmission
%     \item (3) multipath tcp extension
%     \item why? plot the impact of zeroing top k values
%     \item compare the original ae vs. new ae
%     \item takeaway: high-impact elements are rare, and impact of each packet is similar
% \end{itemize}
% }



% \subsection{Delivering a sequence of frames}

% \jc{
% \begin{itemize}
%     \item we have to think about long-term effects (propagation effects of \rate)
%     \item (1) packet prioritization in \name: evenly split among new packets.
%     \item contrast it with prioritizing retransmission in webrtc
%     \item (2) \name's way of selecting ref frame (on-demand synchronization)
%     \item explain the tradeoff: always sync-up (high overhead), always not sync-up (low quality)
%     \item empirical result: quality vs. \# of high-\rate frames
%     \item (3) bitrate adaptation: 
% \end{itemize}
% }

% \end{comment}


% \tightsection{Implementation}
% \space{}

%We use the method described in \S\ref{??} to fine-tune \fillme~\cite{??} to get \newae's P-frame codec and \fillme~\cite{??} to get \newae's I-frame codec. 
%The per-packet entropy encoding uses \fillme~\cite{??}. 


\tightsubsection{WebRTC integration}
\name is implemented with 3K lines of code, in both Python (mostly for autoencoder NNs) and C++ (for frame delivery and WebRTC integration). The code and trained model of \name will be made public upon the publication of this paper.
The integration with WebRTC is logically straightforward since \newae (including I-frame and P-frame encodings) exposes similar interface as the default codec in WebRTC. 
%\jc{Ziyi, please fill in the details}

We substitute the libvpx VP8 Encoder/Decoder in WebRTC with our \newae implementation. When the sender encodes a frame, it parses the image data from the \texttt{VideoFrame} data structure (YUV format) into \texttt{torch.Tensor} (RGB format) and feed it into our \newae encoder, which will return the encoded result as a byte array. Then the encoded bytes are stored into an \texttt{EncodedImage} (class in WebRTC) and sent through the network to the receiver as RTP packets. 
% \zy{I could also add several sentences about packetization logic (commented out below)}
% The encoded bytes are then packetized as RTP packets and sent through the network to the receiver. 
We modify the built-in \texttt{RtpVideoStreamReceiver} (class in WebRTC) so that the receiver could flexibly decode the received packets even when not all the packets are received. When the receiver decides to decode the frame, it depacketizes the received packets into encoded data. Then it will use the \newae decoder to decode the image into RGB format and then convert it back to YUV for displaying on the receiver side.



%\jc{need to explain the gains are not directly from the entropy encoder or motion vector estimation}




\tightsubsection{Optimizations}
\label{subsec:optimize}

While \newae is functionally similar to traditional codecs, it faces a few technical challenges to function as the codec in a real-time video client.
Note that these challenges are not specific to loss resilience, so we do not consider packet losses in the rest of the section. 



\mypara{Reducing compute overhead}
Most research on autoencoder focuses on coding efficiency (using fewer bits to get higher quality), but the encoding/decoding speed is much lower than the heavily optimized codecs like H.265.
Fortunately, we show that on a single NVIDIA GeForce 3080 GPU, \name's encoding speed can be greatly improved: from 5~fps on 720p HD (and 11~fps on 480p) videos by the off-the-shelf implementation to 18~fps (and 40~fps). More results in \S\ref{subsec:eval:system}. 
\name achieves such speedup by downsizing the image (by default $4\times$) during motion-vector estimation and motion compensation, and then upsample the motion-compensated image before calculating and encoding the residuals. 
This speeds up encoding because motion-vector estimation and motion compensation are the slowest steps during P-frame encoding and their delays are proportional to the input size.
Thus, the overall encoding delay will be reduced if they are fed with downsized images. 
At the same time, because the residuals are still computed between the full-resolution image and the motion-compensated image, the coding efficiency is not affected by this change for most frames.

\mypara{Bitrate control}
In real-time video, throughput estimation can vary even between two consecutive frames, and the encoded frame size should be barely below the target frame size.
This has been a challenge with traditional codecs.
%Thus, it is important that most frames are smaller than the target size set by congestion control, but traditional codecs are not able to do that. 
%This has been observed in \cite{salsify}, which proposes to encode each frame at multiple quality levels in order to find an encoding that fits the target bitrate. 
\name provides bitrate control logic similar to~\cite{salsify} to encode a frame with a maximum size below a target. 
We train multiple autoencoders, each using a different weight of frame size $\alpha$ in its training loss function (\S\ref{subsec:sim-losses}).
These resulting autoencoders cover a range of bitrate range. 
%\fillme$\times$ difference between the highest bitrate and lowest bitrate. (A wider bitrate range is possible with more autoencoders.)
As long as the target bitrate is within this range, \name should be able to select the autoencoder whose encoded frame size is barely lower than the target. 
A naive solution will run multiple autoencoders (like~\cite{salsify}), but the compute overhead will increase linearly.
Fortunately, we can again re-use the motion-compensated image to get the residuals, and only run different versions of residual encoders to encode the residuals with different bitrates.
Since residual encoder is faster than the motion estimation and compensation, the speed up is significant.


\mypara{Reducing memory footprint}
For the client to switch between multiple autoencoders (with different bitrates), their memory footprint should be minimized, so more of them can be loaded into GPU memory to avoid the delay of loading and unloading models. 
\name trains multiple autoencoders by fine-tuning the last 10-25\% layers of the same model (\ie they share the backbone layers), so only the one autoencoder and the last few layers of different autoencoders need to be loaded in GPU memory. 
This reduces the memory footprint of the models by 60\% compared to when all models are trained separately without sharing any layers.
A similar idea has also been used in Swift~\cite{swift} in multiple SVC layer encoders.
%\footnote{\jc{A note on I-frames}}
%, though \name uses it to reduce memory footprint of data-scalable autoencoders of different bitrates.


%A client must be able to encode each frame at a given target size. 


%\jc{this needs to be rewritten}
%\jc{need a figure here}

%\mypara{Bitrate adaptation} 

\begin{comment}
To select an autoencoder with frame size lower than the target, we leverage an empirical property of these autoencoders (illustrated in Figure~\ref{??}): 
for each pair of a high-bitrate autoencoder (trained with a high $\alpha$) and a low-bitrate autoencoder (trained with a low $\alpha$), if we denote their encoded frame sizes on the same frame are $S_h$ and $S_l$, then $S_h/S_l$ is roughly constant, despite both $S_h$ and $S_l$ vary between frames. 
Thus, each time when a frame is encoded by one autoencoder, \name can then infer the frame size of other autoencoders on the same frame.
This information can be used to correct the estimated frame size of each autoencoder on current frames. 
This logic is similar to the rate control logic in H.264, which corrects the bitrate estimation based on the latest encoded frame sizes.
\end{comment}



%\jc{
%\begin{itemize}
%    \item explain the rate adaptation logic. how we estimate frame size from complexity
%    \item show empirical correlation between complexity and frame size
%    \item connect it with rate control in h264.
%    \item talk about shared backbone to save memory footprint.
%\end{itemize}
%}


%\mypara{Reducing system overhead}
%Despite that sharing most NN layers (\S\ref{??}) greatly reduces the memory footprint of the multi-bitrate autoencoders, the compute overhead of autoencoder NNs remains substantial---100ms to encode a frame of \fillme$\times$\fillme on a \fillme GPU (though decoding can be much faster). 
%Note that this is already faster than the autoencoder used in a recent work for video streaming.
%Fortunately, because \name's autoencoder contains shallow NNs, the encoding and decoding of \newae can be greatly accelerated by OpenVino~\cite{??} and achieve \fillme even on CPUs. 
%\jc{kuntai/ziyi, fill in the details here}








% \jc{
% \begin{itemize}
%     \item how to integrate it in webrtc: same logical interface for video coding, packetization. replacing vp8
    
%     \item autoencoder highlight: entropy encoder, i-frame model, p-frame model
    
%     \item use of intel vino to reduce overhead
% \end{itemize}
% }




==> sections/old/technical_v6.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US






\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/dvc-arch-v2.pdf}
    \tightcaption{}
    \label{fig:dvc-arch}
\end{figure*}

\tightsection{\newae: Data-Scalable Autoencoder}
\label{sec:training}

%\name is a concrete instantiation of data-scalable delivery. 
This paper presents \name, a new autoencoder-based video coding system.
After some background on autoencoders, this section will present \name's basic autoencoder and its custom packetization. 
The next section will describe a concrete video delivery framework based on \name's autoencoder.

%designed to achieve close-to-optimal data-scalable coding. 

%and a custom delivery framework for the new autoencoder (\S\ref{sec:delivery}).
%We will describe the autoencoder design in this section, followed by the delivery framework in the next section. 

\tightsubsection{Autoencoder primer and limitations}

Video autoencoders use neural networks (NNs), instead of handcrafted heuristics, to encode and decode video frames.
We denote the encoder by $\Coder$ (with NN weights $\phi$) and the decoder by $\Decoder$ (with NN weights $\theta$).
The encoder encodes a frame $\x$ (a $c\times w\times h$ tensor) to a \aecode $\y=\Coder(\x)$, and the decoder decodes $\y$ to reconstruct a frame $\hat{\x}=\Decoder(\y)$.
%For an input frame $\x$ (a $c\times w\times h$ tensor), the \aecode is the output of the encoder $\y=\Coder(\x)$  will be sent to the receiver, which then runs the decoder to reconstruct the original frame from $\y$: $\hat{\x}=\Decoder(\y)$.
Standard autoencoders minimizes the following: % over inputs from training frames $\X$:
\vspace{-0.08cm}
\begin{align}
%\textrm{\bf min~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\y), \y, \x)\textrm{, where }\y = \Coder(\x)
%\textrm{\bf min~~} \mathbb{E}_{\x} \Distort(\Decoder(\y), \x)+\alpha\cdot\Size(\y)\textrm{, where }\y = \Coder(\x)\\
%\textrm{\bf min~} 
\mathbb{E}_{\x} {\color{black}\underbrace{\highlight{black}{$\Distort(\Decoder(\y), \x)$}}_{\text{\sf \footnotesize \textcolor{black!85}{Pixel error}}}}+
\alpha{\cdot}{\color{black}\underbrace{\highlight{black}{$\Size(\y)$}}_{\text{\sf \footnotesize \textcolor{black!85}{Encoded size}}}}\textrm{, where }\y = \Coder(\x)
\label{eq:1}
\vspace{-0.08cm}
\end{align}
Here, $\Distort(\hat{\x},\x)$ is the pixel-level reconstruction error (typically, L2-norm\footnote{Pixel-wise distortion may not be the best way to capture human perception of reconstructed images, but it is often used in autoencoder training for its differentiability. We will evaluate the trained autoencoders in terms of more standard metrics, such as SSIM and PSNR (in RGB and YUV).} of $\hat{\x}-\x$), and $Size(\y)$ is the entropy-coded data size of $\y$ in bit-per-pixel (BPP).
The parameter $\alpha$ governs the tradeoff between frame size and pixel error: a higher $\alpha$ leads to smaller frame size ($Size(\hat{x})$) but smaller distortion (\ie poorer quality) of the reconstructed frame $\hat{\x}$.
% will tend to have better visual quality in $\Decoder(\z)$ but also higher bitrate. 
In Eq.~\ref{eq:1}, since all of the functions---$\Coder$, $\Decoder$, $\Distort$ and $\Size$ (which is approximated by a pre-trained NN)---are differentiable, the NN weights $\phi$ and $\theta$ can be trained jointly.




%\jc{refer to fig~\ref{fig:dvc-arch}}


This work focuses primarily on using autoencoders to encode P-frames, which are the most common frame type in real-time videos~\cite{??} (introduced in \S\ref{??}). We will discuss I-frame coding later in \S\ref{??}. (B-frames as they are not commonly used in real-time videos~\cite{??}.)
Figure~\ref{fig:dvc-arch} describes the typical workflow of P-frame autoencoders, including that of \name.
Rather than compressing frames from scratch, the workflow is comprised of steps (\eg motion estimation and residuals) typically found in a traditional video codec but replaces 
%Most recent video autoencoders~\cite{??,??,??} combine useful concepts from traditional codecs (\eg motion vectors and residuals) and replace 
handcrafted heuristics with NNs, and they achieve compression efficiency comparable to recent video codecs.
Moreover, since they are trained on large sets of videos (\eg Vimeo-90K~\cite{vimeo-dataset}), their compression efficiency is quite generalizable in a variety of video content (which we also observe in our evaluation \S\ref{??}).
For these reasons, autoencoders attract increasing attention from the multimedia community~\cite{??,??,??}.
%, and achieve comparable compression efficiency as recent compression algorithms.

That said, currently autoencoders must use traditional schemes (like FEC) to handle packet loss. 
They do not tolerate packet loss due to two reasons.
\begin{packeditemize}
\item Traditional entropy encoding compresses the whole encoder output as a single bitstream, so any data loss will render it undecodeable.
\item The standard autoencoder training (Eq.~\ref{eq:1}) assumes that the decoder's input equals the encoder's output, which does not prepare the autoencoders to handle data loss between the encoder and decoder. 
%current autoencoder training assumes that the encoder's output equals the decoder's input, so the trained models are not prepared to handle data loss between the encoder and decoder. 
\end{packeditemize}


\tightsubsection{Overview of \name}

We address these problems in two steps. 

First, \name uses the NN architectures of DVC~\cite{??}, a commonly used autoencoder, but it changes the training of autoenocoders so that the quality of the trained autoencoder degrades gracefully with higher rate of {\em random data erasure} in the \aecode $\y$, \ie setting a fraction of random elements in $\y$ to zeros. 

Second, we change the packetization and entropy coding logic, so that packet loss with a \rate of $n\%$  has the same effect on \aecode $\y$ as randomly erasing (zeroing) $n\%$ of elements in $\y$.




%assume that the impact of packet loss of \rate $=n\%$ on the encoder's output $\y$ is that a subset of random $n\%$ of elements in $\y$ are set to zeros.
%We call this {\em random data erasure}, and present a practical design to realize this assumption in \S\ref{??}.
%We will also explain why the choice of random data erasure is reasonable in \S\ref{??}.





%\begin{figure}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.99\linewidth]{figs/dvc-arch.pdf}
%    \tightcaption{}
%    \label{fig:dvc-arch}
%\end{figure}


\tightsubsection{Training of data-scalable autoencoders}



\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/ae-arch-v2.pdf}
    \tightcaption{Contrasting the proposed loss-resilient design of autoencoders with traditional autoencoders.}
    \label{fig:grace-training}
\end{figure}



%The training process in Eq.~\ref{eq:1} can be equivalently viewed as having a lossless channel between the encoder to the decoder, \ie the decoder's input equals the encoder's output. 
To handle random data erasure, \name jointly trains the encoder and decoder NNs to minimize the following objective 
%which uses a random distribution $\loss$ to simulate the effect of packet loss on the encoder's output:
\vspace{-0.1cm}
\begin{align}
%\textrm{\bf min~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\y), \x)\textrm{, where }
%\color{blue}\underbrace{\highlight{blue}{$\y\sim \loss(\y | \Coder(\x))$}}_{\text{\sf \footnotesize \textcolor{blue!85}{Simulating packet loss}}}
\mathbb{E}_{\x} \Distort(\Decoder(\y), \x)+\alpha{\cdot}\Size(\y)\textrm{, where }
\color{blue}\underbrace{\highlight{blue}{$\y\sim \loss(\y | \Coder(\x))$}}_{\text{\sf \footnotesize \textcolor{blue!85}{Simulate packet loss}}}
\label{eq:2}
\vspace{-0.1cm}
\end{align}
%where the change is highlighted in color.
Given the encoder output $\Coder(\x)$, $\loss$ represents the data distribution seen by the decoder. 
For instance, if \rate is 30\%, then $\loss(\y | \Coder(\x))$ is the probability of $\y$ being the result of randomly setting 30\% of elements in $\Coder(\x)$ to zeros.
Figure~\ref{fig:grace-training} contrasts how \name trains its autoencoder and the traditional autoencoder training.
%each $\y$ drawn from the distribution $\loss(\y | \Coder(\x))$ is a result of randomly setting 30\% of elements in $\Coder(\x)$ to zeros.

We should notice that the random probability distribution $\loss$ may not be expressed as an  function of $\phi$ and thus not differentiable with respect to $\phi$.
To train the weights in $\phi$, we use the REINFORCE trick~\cite{Kingma2014} to approximate this gradient by Monte-Carlo Sampling (see Appendix~\ref{??} for details).

%Normally, to train a model, we need to calculate the gradient of Eq~\ref{eq:2} with respect to weights $\theta$ and $\phi$. The gradient with respect to $\theta$ is trivial, but since $\loss$ is a non-differentiable random function, the gradient with respect to $\phi$ cannot be analytically derived. 
%%of the expectation of $\Quality$ cannot be analytically derived. 
%Fortunately, we can use the REINFORCE trick~\cite{Kingma2014} which approximates this gradient by Monte-Carlo Sampling (see Appendix~\ref{??} for details).


%\jc{why training encoder and decoder jointly?}


\mypara{Choice of \rates in autoencoder training}
The function \loss decides the rate of packet loss (\rates) seen by the autoencoder during training. 
Intuitively, to prepare the autoencoder to handle different packet loss outcomes, we should let the autoencoder see a variety of \rates.
%, so that it will be prepared to deal with different packet loss outcomes. 
When training autoencoders, \name sets \rate to zero for random 80\% of input, and for the remaining 20\% of input, it randomly selects a \rate from [0,100\%].
In other words, it lets the autoencoder see all possible \rates, with a higher weight on 0\% packet loss.

It is important to note that 0\% packet loss is used on more input because otherwise we have observe that the trained autoencoder would perform much poorly on low packet loss rates.
It can be intuitively understood that \fillme
\jc{mention other distributions}


\myparaq{Why is \name loss tolerant}
\name-trained autoencoders can tolerate data erasures due to three reasons.
%Though it is difficult to analytically interpret the NN-based encoders and decoders, there are three intuitive reasons to explain why Grace-trained autoencoders can tolerate data erasures. 
(1) The coded tensors of autoencoders have little strong dependencies between elements making data erasure less impactful on the decoding result than in H.265 output. 
(2) The \name-trained NN encoder learns to output more non-zero values in the coded tensor to contain redundant information and having more non-zero values allows the decoder to easily distinguish erased (\ie zeroed) elements.
(3) \name's training also prepares the NN decoder to recover the erased (zeroed) elements, in addition to generating high-quality frames from received elements. There are many other examples where the convolutional layers, which are used in the NN decoder, can reconstruct images from noisy input or even complete random input. 

%\jc{
%\begin{itemize}
%\item \aecode inherently has little structure
%\item after training, encoder learns to put more redundant information and make erased values more distinguishable
%\item training also makes the decoder learn to recover lost values (by conv layers)
%\end{itemize}
%}

%\mypara{Why training encoder and decoder jointly}
%\fillme


\tightsubsection{Per-packet entropy encoding}
\label{subsec:packetization}

%\begin{itemize}
%
%\item why not cabac? why not random assignment?
%
%\item initial design
%
%\item preliminary results: psnr vs bpp
%
%\end{itemize}

The autoencoders trained using Eq.~\ref{eq:2} can tolerate random data erasure on \aecode at different rates.
To make it practical, however, \name must entropy encode and packetize the encoder's output in a way such that {\em (1) without increase of data size, (2) packet loss appears to be random data erasure on the \aecode}.
%More formally, the encoded


Standard autoencoders~\cite{dvc} entropy codes
%(\eg Torchac~\cite{torchac}) 
the entire \aecode to a single bitstream before packetization.
%Traditional video codecs (\eg H.265 and VP9) also use entropy coding (CABAC).
As a result, any missing packet will render the bitstream undecodable. 
It is important to note that FEC must add redundancy and thus increase the data size.
%(FEC can prevent )
%(as elaborated in \S\ref{??}, FEC is not ideal). 
%However, if any part of this bitstream is lost or corrupted, the whole bitstream will be undecodable.


%\, so this way of entropy coding is incompatible with DS video delivery.


%The random data erasure used in Eq.~\ref{eq:2} needs to be implemented by a practical packetization and entropy coding scheme.
%The output of an autoencoder consists of several tensors, and like in any video codec, they must be packetized and entropy-coded into a smaller-sized packet of bytestream.
%Here, we first motivate why we need a new entropy coding and packetization scheme, before proposing a potential solution.

%\myparaq{Why not existing entropy encoders}

%\mypara{Naive per-packet entropy encoding} 
\name builds on a simple idea depicted in Figure~\ref{fig:per-packet}.
It first randomly splits the elements in \aecode into smaller sub-tensors and then entropy encodes each sub-tensor {\em separately} as an independently decodable packet. 
%for each part, assemble the elements to a smaller-sized $\z$ and feed it to $\DistributionEst$ to get the estimated distribution. {\em (iii)} For each part, use the entropy encoder and the estimated distribution to encode the elements to a bytestream. The estimated distribution will also be compressed put into the same packet.
%This way, each packet is independently decodable. 
If a packet is missing, we set its elements, which is a random subset of the \aecode, to zeros.
This effectively is random data erasure. 


\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v3.pdf}
    \tightcaption{\name's packetization and per-packet entropy encoding. When a packet is lost, the elements mapped to it will be set to zeros.}
    \label{fig:per-packet}
\end{figure}


%This strawman solution satisfies the requirements of per-packet entropy coding: every arrived packet will be decodable no matter other packets is arrived or not. 
However, this naive method significantly increases the size of packets, by \fillme\% compared to entropy encoding the entire \aecode together as in traditional autoencoders.
%---the size of the coded bistream is up-to \fillme\% larger than entropy encoding the entire \aecode before packetization as in standard autoencoders.
%To put the number into context, the PSNR of the frame encoded using this method will decrease from \fillme to \fillme when the size of the bytestream is the same as using the traditional entropy coding.
The reason for the increase is that entropy coding needs to store the {\em symbol distribution} of values in a sub-tensor in order to compress it efficiently. 
When the whole \aecode is compressed together, the additional overhead of symbol distribution is relatively marginal (\fillme-\fillme\%) to the sized of the compressed data.
With per-packet entropy coding, however, we need to include the symbol distribution in each packet, greatly increases the total data size.


%Unfortunately, each sub-tensor has a slightly different symbol distribution, so a separate symbol distribution needs to be saved for {\em each} packet, which greatly increases the packet size.

\begin{comment}

to be most effective, each sub-tensor should be entropy-encoded and decoded using the accurate {\em symbol distribution} of values in a tensor---if either the distribution is incorrect or too big, the entropy-encoded packet size will inflate. 
%at each position and that both the coded data and the value distribution contribute to the size of a packet; 
Unfortunately, each sub-tensor may have a slightly different symbol distribution, so a separate symbol distribution needs to be saved for each packet, which increases the packet size.
%, \eg the top-left element of the first channel in the original tensor may have a totally different distribution than that of the same position in each sub-tensor, which now becomes the value of another position in the original tensor. 
%Thus, a separate value distribution is needed for each packet, which inflates the packet size.

\end{comment}

%\begin{subtask}
%{\bf Low packetization and entropy-coding overhead.} 
%Propose a packetization and entropy coding scheme for DS autoencoder output such that each packet is independently decodable but {\em without} much size inflation of the coded data.
%%with minimum compression overhead compared to traditional codecs.
%\end{subtask}

%Fortunately, this problem is not intractable. 
%Here we present an initial design and plan a more systematic examination for the proposed task. 

%\mypara{Initial ideas} 
%\mypara{Coarse-grained }
To solve this conundrum, we empirically observe that the distribution of values in each channel of a \aecode (which has \fillme channels) can be simply characterized by one single variance.
That is, the values in the same channel roughly follow a Laplace distribution with a mean of zero. 
\jc{Yihua, any reason for it to be so?}
\jc{need a figure to illustrate this. talk to yihua}

This observation inspires a simple yet effective solution: using a {\em coarser-grained} symbol distribution, which has only the standard deviation per channel, can entropy encode data almost as efficiently as using the real symbol distribution.
Compared to the symbol distribution needed by the original DVC model, a coarse-grained symbol distribution needs \fillme$\times$ fewer bits to store.
Thus, even if there are 20 packets, adding the symbol distribution to each packet only increase the total data size by no more than \fillme\%.
%The reason is that each sub-tensor has multiple channels (\eg 96 channels in our case), and the values of the same channel are either similar (mostly small values) or bimodal (only a few similarly large values), so using a coarse-grained distribution can effectively represent their distributions and lead to an entropy-coded data size that compared to the coded size using the accurate value distribution is slightly larger  but only by a small margin.
%Since these coarse-grained symbol distributions need fewer bits to store, they will add to a negligible fraction of each packet. 

Moreover, the use of coarse-grained symbol distribution allows us to reuse symbol distributions. 
In particular, we pre-define \fillme different standard deviations as candidate distributions of each channel. 
Then for each channel's standard deviation, the sender simply adds the index (an integer) of the standard deviation that is most similar to the real one. 

% and observe that in most \aecodes, the symbol distribution can be very closely approximated by one of these candidate symbol, so the sender can simply add the index of the symbol distribution in each packet.

%We propose to store the value distribution of each channel in a {\em coarser} granularity (\eg only a mean and standard deviation) so they are slightly less accurate but much easier to store, and as a result, these distributions will take an almost negligible fraction of each packet. 
%The insight is that each sub-tensor has multiple channels (\eg 96 channels in our case), and the values of the same channel are either similar (mostly small values) or bimodal (only a few similarly large values), so using a coarse-grained distribution can effectively represent their distributions and lead to an entropy-coded data size that compared to the coded size using the accurate value distribution is slightly larger  but only by a small margin.

\jc{Yihua, is this also similar to how CABAC avoid sending symbol distribution?}

\jc{more evidence and intuition}


\tightsection{Real-time video delivery over \newae}
\label{sec:delivery}

\jc{need an end-to-end figure here}

\jc{
\begin{itemize}
\item coding of i-frames (compression)
\item bitrate control (speed)
\item speedup on cpu (speed)
\item end-to-end protocol (why no synchronization, interaction with tcp and abr) (resilience)
\end{itemize}
}

\jc{a table mapping the techniques to effects
\begin{itemize}
\item compression: i-frames, per-packet entropy
\item speed: bitrate control, cpu speedup
\item resilience: retraining, end-to-end protocol
\end{itemize}
}


\tightsubsection{Encoding a sequence of frames}
\label{subsec:delivery:iframe}

%To stream a sequence of video frames, a key question is how often I-frames should be inserted in P-frames. 
Placement of I-frames poses a particular challenge for \name's autoencoders (both pre-trained and re-trained), for two reasons: (1) I-frames are generally bigger in size than P-frames, and 
(2)  while the first few P-frames after an I-frame enjoy high quality, quality gradually degrades after about 10 frames. 
%(As explained in \S\ref{subsec:ae-background}, \name uses only I-/P-frames, as in most real-time video systems.)
%For the P-frame autoencoder we have tried, we observe that the decoded quality can be very high right after each I-frame but it gradually degrades after about 10 frames. 

A strawman would add I-frames frequently (say every 10 frames)\footnote{Many computer-vision papers on autoencoders have conveniently used a small GoP when compared against H.265, but the implication of large I-frame size for congestion control is rarely discussed.}.
Even though this might achieve a decent tradeoff between quality and {\em average} bitrate (comparable to H.264 and H.265 with large I-frame intervals), sending I-frames (which have bigger sizes than the P-frames in between) frequently will make it difficult for congestion control to send the frames at a fixed interval (inversely proportional to the frame rate).


To add I-frames frequently without the intermittent bitrate spikes caused by the I-frames, \name encodes a small patch (about 128$\times$128 to 512$\times$512) as a tiny I-frame, which we call {\em I-patch}, on {\em every frame} (the pixels outside the I-patch will be encoded as a P-frame), and the location of the I-patch on a frame changes over time such that the I-patch will scan through the whole frame size every $k$ frames. 
Depending on the original frame size, $k$ varies between 6 and 20. 
This scheme effectively ``amortizes'' the size of I-frames across $k$ frames, thus smoothing the frame size as well as quality across frames (illustrated in Figure~\ref{fig:keyframe_smooth}).
Moreover, since the I-frame autoencoder's encoding delay is proportional to the input size, encoding a small I-patch adds only a small compute overhead for each frame.\footnote{We should clarify that design choice of frequent I-frames works well for autoencoders, but {\em not} for classic codecs for two reasons. First, an I-frame generated by our autoencoder is only 2-5$\times$ bigger than a P-frame, whereas this ratio in H.264 is 4-10$\times$. Second, the P-frame quality in H.264 is relatively stable, whereas the quality of a P-frame is high following an I-frame (or an I-patch).}





\begin{figure}[t!]
    \centering
    
        \includegraphics[width=0.85\linewidth]{figs/split-iframe-size.pdf}
    \tightcaption{Encoding each P-frame with a small I-patch leads to smoother frame sizes than naively inserting I-frames.}
    \label{fig:keyframe_smooth}
\end{figure}


\tightsubsection{Bitrate control}


In real-time video, throughput estimation can vary even between two consecutive frames, and the encoded frame size should be barely below the target frame size.
This has been a challenge with traditional codecs.
%Thus, it is important that most frames are smaller than the target size set by congestion control, but traditional codecs are not able to do that. 
%This has been observed in \cite{salsify}, which proposes to encode each frame at multiple quality levels in order to find an encoding that fits the target bitrate. 
\name provides bitrate control logic similar to~\cite{salsify} to encode a frame with a maximum size below a target. 
We train multiple autoencoders, each using a different weight of frame size $\alpha$ in its training loss function (\S\ref{subsec:sim-losses}).
These resulting autoencoders cover a range of bitrate range. 
%\fillme$\times$ difference between the highest bitrate and lowest bitrate. (A wider bitrate range is possible with more autoencoders.)
As long as the target bitrate is within this range, \name should be able to select the autoencoder whose encoded frame size is barely lower than the target. 
A naive solution will run multiple autoencoders (like~\cite{salsify}), but the compute overhead will increase linearly.
Fortunately, we can again re-use the motion-compensated image to get the residuals, and only run different versions of residual encoders to encode the residuals with different bitrates.
Since residual encoder is faster than the motion estimation and compensation, the speed up is significant.




\tightsubsection{Reducing compute overhead}

Most research on autoencoder focuses on coding efficiency (using fewer bits to get higher quality), but the encoding/decoding speed is much lower than the heavily optimized codecs like H.265.
Fortunately, we show that on a single NVIDIA GeForce 3080 GPU, \name's encoding speed can be greatly improved: from 5~fps on 720p HD (and 11~fps on 480p) videos by the off-the-shelf implementation to 18~fps (and 40~fps). More results in \S\ref{subsec:eval:system}. 
\name achieves such speedup by downsizing the image (by default $4\times$) during motion-vector estimation and motion compensation, and then upsample the motion-compensated image before calculating and encoding the residuals. 
This speeds up encoding because motion-vector estimation and motion compensation are the slowest steps during P-frame encoding and their delays are proportional to the input size.
Thus, the overall encoding delay will be reduced if they are fed with downsized images. 
At the same time, because the residuals are still computed between the full-resolution image and the motion-compensated image, the coding efficiency is not affected by this change for most frames.








\begin{figure}[t!]
    \centering
         \centering
        \includegraphics[width=0.99\linewidth]{figs/technique-mapping.pdf}
    \tightcaption{}
    \label{fig:technique-mapping}
\end{figure}

\name is built on the data-scalable autoencoder \newae. 
%\name is a concrete real-time video communication system built on a data-scalable autoencoder (\newae).
We focus on unique issues arising from the use of \newae as the codec, including how to deliver each frame to strike a desirable delay-quality tradeoff, and how to deliver a sequence of frames when congestion or packet losses affect multiple frames. 
The choice of the congestion control logic is complementary to \newae. 
In \S\ref{subsec:eval:e2e}, we will evaluate \name with different congestion control logic, such as GCC in WebRTC~\cite{carlucci2016analysis} or Salsify CC~\cite{salsify}. 
We do not claim that \name's strategies are new (\eg reference frame synchronization has been used in~\cite{salsify}). 
Nonetheless, \name integrates concrete design choices driven by the need, in order to unleash the full potential of \newae and its data-scalable codec primitive.





\tightsubsection{Streaming protocol}

\mypara{Handling loss over multiple frames}
An important benefit of adding an I-patch (a tiny patch encoded as an I-frame without referring to previous frames) at a different place in each frame is: each patch will be encoded as an I-patch every $k$ frames. 
This has a significant implication for loss resilience over multiple consecutive frames. 

%\mypara{Encoding/decoding synchronization}
An acute reader may realize a potential problem arising from encoding and decoding being asynchronous. 
For instance, when the sender encodes the $10^{\textrm{th}}$ frame as a P-frame, it needs the decoded the $9^{\textrm{th}}$ frame as the reference (to compute motion vectors and residuals), and without knowing which of the $9^{\textrm{th}}$ frame's packets will be lost, it will assume that the $9^{\textrm{th}}$ frame is decoded with all packets being received. (This is common to classic codecs and autoencoders.)
However, if the receiver decodes the $9^{\textrm{th}}$ frame with only a subset of its packets, the actual reference frame used to decode the $10^{\textrm{th}}$ will differ from what the encoder has assumed. 
Thus, most codecs require all packets of the $9^{\textrm{th}}$ frame to be received before decoding it (thus longer delay), or let the sender encode the $10^{\textrm{th}}$ based on an earlier reference (say the $5^{\textrm{th}}$) whose lost packets are already known to the sender. 
The latter {\em synchronizes} the encoding and decoding states (like in Salsify~\cite{salsify} during packet losses), but it also inflates the frame size, since the difference between the $10^{\textrm{th}}$ and the $5^{\textrm{th}}$ frames  is much greater than between the $10^{\textrm{th}}$ and the $9^{\textrm{th}}$ frames. 


%the P-frame encoding of the $10^{\textrm{th}}$ frame will have a low quality when being decoded with a different reference frame than the encoder has assumed. 




\name uses a simple yet efficient solution---it does not always synchronize the encoding/decoding state on every single frame; instead, it relies on the frequent I-patches (explained in \S\ref{subsec:delivery:iframe}) to synchronize the encoding/decoding states in each patch-size region. 
This works for two reasons.
First, without synchronizing the encoding and decoding states, \newae's quality degradation increases only marginally when multiple consecutive frames (less than about 10) are affected by packet losses.
For instance, applying a 50\% packet loss rate on one single frame can reduce PSNR by 3-4, and applying the same loss rate on 5 consecutive frames reduces PSNR by 7-9. 
%\jc{this corroborates our empirical improvements in \S\ref{??}}
%quality degrades by \fillme\% when 10 consecutive frames are affected by 50\% packet losses without the clients synchronizing their encoding/decoding states. 
Second, each patch will be encoded as an I-patch every $k$ frames ($k$ is between 6 and 20), so the impact of packet losses will not last for more than $k$ frames if the next I-patch is not lost. 
That said, in the worst case, if the I-patches of the same region are dropped persistently, this could cause bad decoded pixel values (\ie a small patch of white pixels), though we have observed it extremely rarely.




\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.995\linewidth]{figs/decode_time.pdf}
        \includegraphics[width=0.995\linewidth]{figs/decode_time_v2.pdf}
    \tightcaption{
    \name waits for the next frame until a deadline $t^*$, after which the utility is lower even if the next packet arrives.
    % At the arrival of the $i^{\textrm{th}}$ packet, \name decides the maximum wait time for the next packet.
    }
    \label{fig:decode-time}
\end{figure}

\mypara{Choosing when to decode a frame}
The data-scalable abstraction allows the receiver to flexibly decide, as packets arrive at the receiver, whether to decode the frame using currently arrived packets or wait for more packets in hope of improving the quality. 
(In contrast, with FEC, the receiver will always wait until enough data is received.)
%(In other loss-resilient schemes (\S\ref{??}), the receiver must wait for more packets until the data is decodable.) 
%\name embraces this flexibility with the following logic to trade frame delay with decoded quality. 

To make this decision, \name defines the {\em utility} of a frame as a linear combination of decoding quality and frame delay (since the natural decoding time) on each frame: $Q(|\{\textrm{pkts before }t\}|)-\beta\cdot t$, where $t$ is when the frame is decoded, $Q(n)$ is the frame's decoding quality with $n$ packets 
The precise values of $Q(n)$ are frame-dependent, but they are roughly similar across frames, so \name estimates $Q(n)$ using history frames.
%, and $\tau$ is the frame's natural decoding time (\eg 40ms after the last frame was decoded with frame rate 25fps).
%In our experiment, we set parameter $\beta=\fillme$.
This objective works well in practice, though there might be other objectives that better capture users' quality perception. An optimal design of such utility is beyond the scope of this paper. 

With this utility in mind, Figure~\ref{fig:decode-time} illustrates \name's logic: on receiving the $i^{\textrm{th}}$ packets of a frame (not necessarily the $i^{\textrm{th}}$ sent packet) at time $t_i$, the receiver will immediately decode the frame if all packets of the frame have arrived; otherwise, it will wait for the next packet of the frame until a deadline $t^*=t_i+\frac{1}{\beta}\cdot(Q(i+1)-Q(i))$, and if it has not received the $(i+1)^{\textrm{th}}$ packet by then, it will decode the frame with $i$ packets. 
The reason is that if the next packet comes at time $t_{i+1}$ after $t^*$, the utility $Q(i+1)-\beta\cdot (t_{i+1}-\tau)$ will be lower than the utility $Q(i)-\beta\cdot (t_i-\tau)$ if the receiver does not wait at all\footnote{This is because {\scriptsize $Q(i+1)-\beta\cdot (t_{i+1}-\tau)<Q(i+1)-\beta\cdot (t^*-\tau)=Q(i)-\beta\cdot (t_i-\tau)$}}. 
%Here, $\beta$ is a tunable parameter, and $Q(n)$ is the quality of the frame based on $n$ packets.
This strategy makes intuitive sense: the receiver will wait longer if the improvement in quality by getting one more packet (\ie $Q(n+1)-Q(n)$) is higher, but it will not wait for too long.

%If a packet comes, the utility will be $Q(n)-1/\beta\cdot \beta\cdot(Q(n+1)-Q(n))$


\tightsubsection{WebRTC integration}
\name is implemented with 3K lines of code, in both Python (mostly for autoencoder NNs) and C++ (for frame delivery and WebRTC integration). The code and trained model of \name will be made public upon the publication of this paper.
The integration with WebRTC is logically straightforward since \newae (including I-frame and P-frame encodings) exposes similar interface as the default codec in WebRTC. 
%\jc{Ziyi, please fill in the details}

We substitute the libvpx VP8 Encoder/Decoder in WebRTC with our \newae implementation. When the sender encodes a frame, it parses the image data from the \texttt{VideoFrame} data structure (YUV format) into \texttt{torch.Tensor} (RGB format) and feed it into our \newae encoder, which will return the encoded result as a byte array. Then the encoded bytes are stored into an \texttt{EncodedImage} (class in WebRTC) and sent through the network to the receiver as RTP packets. 
% \zy{I could also add several sentences about packetization logic (commented out below)}
% The encoded bytes are then packetized as RTP packets and sent through the network to the receiver. 
We modify the built-in \texttt{RtpVideoStreamReceiver} (class in WebRTC) so that the receiver could flexibly decode the received packets even when not all the packets are received. When the receiver decides to decode the frame, it depacketizes the received packets into encoded data. Then it will use the \newae decoder to decode the image into RGB format and then convert it back to YUV for displaying on the receiver side.



%\jc{need to explain the gains are not directly from the entropy encoder or motion vector estimation}


\begin{comment}

\tightsubsection{Optimizations}
\label{subsec:optimize}

While \newae is functionally similar to traditional codecs, it faces a few technical challenges to function as the codec in a real-time video client.
Note that these challenges are not specific to loss resilience, so we do not consider packet losses in the rest of the section. 






\mypara{Reducing memory footprint}
For the client to switch between multiple autoencoders (with different bitrates), their memory footprint should be minimized, so more of them can be loaded into GPU memory to avoid the delay of loading and unloading models. 
\name trains multiple autoencoders by fine-tuning the last 10-25\% layers of the same model (\ie they share the backbone layers), so only the one autoencoder and the last few layers of different autoencoders need to be loaded in GPU memory. 
This reduces the memory footprint of the models by 60\% compared to when all models are trained separately without sharing any layers.
A similar idea has also been used in Swift~\cite{swift} in multiple SVC layer encoders.

\end{comment}




==> sections/old/technical_v7.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US






\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.97\linewidth]{figs/dvc-arch-v3.pdf}
    \tightcaption{Workflow of the autoencoder in \name.}
    \label{fig:dvc-arch}
\end{figure*}

\tightsection{\name: Data-Scalable Autoencoder}
\label{sec:core}

%\name is a concrete instantiation of data-scalable delivery. 
We present, \name, a new {\em autoencoder}-based video coding system.
This section begins with a primer of traditional autoencoders and their limitations and then presents two basic ideas that make \name data-scalable when packet loss affects only one frame.
%---the new autoencoder training to tolerate random data erasure (\S???\ref{subsec:??}) and a custom scheme of packetization and entropy encoding to equate packet loss and data erasure (\S???\ref{subsec:??}).
The next section will describe the video delivery framework over \name's autoencoder.

%designed to achieve close-to-optimal data-scalable coding. 

%and a custom delivery framework for the new autoencoder (\S???\ref{sec:delivery}).
%We will describe the autoencoder design in this section, followed by the delivery framework in the next section. 

\tightsubsection{Autoencoder primer and limitations}
\label{subsec:ae-background}

Autoencoders use learned neural networks (NNs), instead of handcrafted logics, to encode and decode video frames.
We denote the encoder by $\Coder$ (with its NN weights $\phi$) and the decoder by $\Decoder$ (with its NN weights $\theta$).
The encoder encodes a frame $\x$ to a {\em \aecode} $\y=\Coder(\x)$, and the decoder decodes $\y$ to a reconstructed frame $\hat{\x}=\Decoder(\y)$.
%For an input frame \x\x (a c×w×hc\times w\times h tensor), the \aecode is the output of the encoder \y=\Coder(\x)\y=\Coder(\x)  will be sent to the receiver, which then runs the decoder to reconstruct the original frame from \y\y: ^\x=\Decoder(\y)\hat{\x}=\Decoder(\y).
Traditionally, autoencoder training minimizes the following expectation (\ie training loss function):% over inputs from training frames \X\X:
\vspace{-0.04cm}
\begin{align}
%\textrm{\bf min~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\y), \y, \x)\textrm{, where }\y = \Coder(\x)
%\textrm{\bf min~~} \mathbb{E}_{\x} \Distort(\Decoder(\y), \x)+\alpha\cdot\Size(\y)\textrm{, where }\y = \Coder(\x)\\
%\textrm{\bf min~} 
\mathbb{E}_{\x} {\color{black}\underbrace{\highlight{black}{$\Distort(\Decoder(\y), \x)$}}_{\text{\sf \footnotesize \textcolor{black!85}{Pixel error}}}}+
\alpha{\cdot}{\color{black}\underbrace{\highlight{black}{$\Size(\y)$}}_{\text{\sf \footnotesize \textcolor{black!85}{Encoded size}}}}\textrm{, where }\y = \Coder(\x)
\label{eq:1}
\vspace{-0.08cm}
\end{align}
Here, $\Distort(\hat{\x},\x)$ is the pixel-level reconstruction error of the decoded frame $\hat{\x}$ (by default, L2-norm\footnote{
Note that L2-norm (or mean squared error) of $\hat{\x}$ and $\x$ are closely related to PSNR of $\hat{\x}$. To avoid this bias, 
our evaluation in \S\ref{sec:eval} measures the quality improvement in SSIM and user subjective studies.
% To avoid bias towards PSNR, our evaluation in \S\ref{sec:eval} measures the quality improvement in not only PSNR, but also SSIM and user subjective studies.
Following the common practice of autoencoder training, the training loss function also includes the reconstruction loss of the motion-compensated prediction. 
%Pixel-wise distortion may not be the best way to capture human perception of reconstructed images, but it is often used in autoencoder training for its differentiability. We will evaluate the trained autoencoders in terms of more standard metrics, such as SSIM and PSNR (in RGB and YUV).
} of $\hat{\x}-\x$), and $Size(\y)$ is the entropy-coded data size of $\y$ in bit-per-pixel (BPP).
The parameter $\alpha$ influences the size/quality tradeoff: a higher $\alpha$ leads to smaller frame size ($Size(\hat{x})$) but higher distortion (\ie poorer quality) of the reconstructed frame $\hat{\x}$.
% will tend to have better visual quality in $\Decoder(\z)$ but also higher bitrate. 
%In Eq.~\ref{eq:1}, s
Since all of the functions---$\Coder$, $\Decoder$, $\Distort$ and $\Size$ (which is approximated by a pre-trained NN~\cite{dvc})---are differentiable, the NN weights $\phi$ and $\theta$ can be trained jointly to minimize Eq.~\ref{eq:1}.




%\jc{refer to fig~\ref{fig:dvc-arch}}



This work focuses primarily on encoding P-frames, the most common frame type in real-time videos as mentioned in \S\ref{subsec:background}. 
Specifically, we use the NN architectures of DVC~\cite{dvc}, a popular autoencoder, whose architecture is depicted in Figure~\ref{fig:dvc-arch}.
(We will discuss I-frame in \S\ref{subsec:protocol}, and B-frames are rarely used in real-time videos~\cite{ffmpegstreaming}.)
%Figure~?????????????????????????????????????????????\ref{fig:dvc-arch} describes the typical workflow of a P-frame autoencoder, which \name follows.
%Rather than compressing frames from scratch, the workflow 
It is comprised of steps (\eg motion and residual estimation) typically found in a traditional video codec (\S\ref{subsec:background}) but  uses NNs to replace
%Most recent video autoencoders~\cite{??,??,??} combine useful concepts from traditional codecs (\eg motion vectors and residuals) and replace 
handcrafted heuristics for motion estimation, compensation, and \st{transformation} \edit{compression} of residual and motion vectors.
%, and they achieve compression efficiency comparable to recent video codecs.
Since they are trained on large sets of videos (\eg Vimeo-90K~\cite{vimeo-dataset}), their compression efficiency is comparable to recent video codes and is reasonably generalizable across a variety of video content (which we also observe in our evaluation \S\ref{sec:eval}).
For these reasons, autoencoders attract increasing attention from the multimedia community~\cite{dvc, swift, hu2021fvc}.
%, and achieve comparable compression efficiency as recent compression algorithms.

\mypara{Limitations}
Currently autoencoders still requires traditional schemes (like FEC) to handle packet loss. 
Their lack of packet loss tolerance is due to two reasons.
\begin{packeditemize}

\item The standard autoencoder training (\ie minimizing Eq.~\ref{eq:1}) implicitly assumes that the encoder's output equals the decoder's input,
% \footnote{A recent work~\cite{??,??} adds Gaussian random noise\jc{check!} between the encoder and decoder to simulate wireless signal noise, but this is different from packet loss which masks a fraction of the data.}, 
so it does not prepare the autoencoder to handle data loss between the encoder and decoder. 

\item Entropy encoding used in autoencoders compresses the whole encoder output as a single bitstream, so any data loss will render it undecodeable.

%current autoencoder training assumes that the encoder's output equals the decoder's input, so the trained models are not prepared to handle data loss between the encoder and decoder. 
\end{packeditemize}


%\tightsubsection{Overview of \name}

\mypara{Roadmap}
At a high level, we address these problems in two logical steps:
\begin{packeditemize}
\item 
%{\em Turning packet loss to random data erasure:} 
We use a new packetization and entropy-coding logic to make packet loss (with \rate of $n\%$) have the same effect as randomly setting $n\%$ of elements in the \aecode to zeros, \ie $n\%$ {\em random masking} of \aecode.
\item 
%{\em Training for resilience random data erasure:} 
Then, we re-train the autoencoder such that its quality degrades gracefully with more {\em random masking} on the \aecode (\ie setting more elements in $\y$ to zeros).
\end{packeditemize}
%As a result, the autoencoder will be data-scalable with respect to packet loss. 

\begin{comment}

Specifically, we first leverage that the autoencoder NNs are trainable and use a new training process to optimize the quality when different fractions of randomly selected elements in \y\y are set to zeros. 
In other words, the autoencoder is data-scalable, if the packet loss is in the form of random data erasure.
Next, we use a new packetization and entropy coding logic, such that packet loss with a \rate of n%n\%  has the same effect on \aecode \y\y as randomly erasing (zeroing) n%n\% of elements in \y\y.


% resilient to {\em random data erasure}---the quality is optimized when $n\%$ of randomly selected elements in $\y$ are set to zeros. 
%
%degrades gracefully if more randomly selected elements in $\y$ are set to zeros.
%
%Put together, the quality of the new autoencoder will meet the three 


so that the quality of the trained autoencoder degrades gracefully with higher rate of {\em random data erasure} in the \aecode $\y$, \ie setting a fraction of random elements in $\y$ to zeros. 
(2) Second, we change the packetization and entropy coding logic, so that packet loss with a \rate of $n\%$  has the same effect on \aecode $\y$ as randomly erasing (zeroing) $n\%$ of elements in $\y$.
\end{comment}



%assume that the impact of packet loss of \rate $=n\%$ on the encoder's output $\y$ is that a subset of random $n\%$ of elements in $\y$ are set to zeros.
%We call this {\em random data erasure}, and present a practical design to realize this assumption in \S\ref{??}.
%We will also explain why the choice of random data erasure is reasonable in \S\ref{??}.





%\begin{figure}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.99\linewidth]{figs/dvc-arch.pdf}
%    \tightcaption{}
%    \label{fig:dvc-arch}
%\end{figure}


\tightsubsection{Training \name's data-scalable autoencoders}
\label{subsec:training}





%The training process in Eq.~???????????????????????????\ref{eq:1} can be equivalently viewed as having a lossless channel between the encoder to the decoder, \ie the decoder's input equals the encoder's output. 

We begin with the second step---training autoencoders that are resilient to various rate of random masking, assuming that missing one of $n$ packet has the same effect as random masking of $1/n$ elements (we will explain how to do it in \S\ref{subsec:packetization}).
%In order to let autoencoders perform well under various rates of random data erasure, 
To this end, \name jointly trains the encoder and decoder NNs to minimize: 
%which uses a random distribution \loss\loss to simulate the effect of packet loss on the encoder's output:
\vspace{-0.04cm}
\begin{align}
%\textrm{\bf min~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\y), \x)\textrm{, where }
%\color{blue}\underbrace{\highlight{blue}{\y∼\loss(\y|\Coder(\x))\y\sim \loss(\y | \Coder(\x))}}_{\text{\sf \footnotesize \textcolor{blue!85}{Simulating packet loss}}}
\mathbb{E}_{\x} \Distort(\Decoder(\y), \x)+\alpha{\cdot}\Size(\y)\textrm{, where }
\color{blue}\underbrace{\highlight{newblue}{$\y\sim \loss(\y | \Coder(\x))$}}_{\text{\sf  \footnotesize \textcolor{blue}{Simulate packet loss}}}
\label{eq:2}
\vspace{-0.04cm}
\end{align}
%where the change is highlighted in color.
The key difference to the traditional autoencoder loss function Eq.~\ref{eq:1} (highlighted in blue) is the distribution function $\loss$, which characterizes the distribution of decoder input.
%Given the encoder output \Coder(\x)\Coder(\x), \loss\loss represents the data distribution seen by the decoder. 
%Remember that 
For instance, with a 
\rate of 33\%, $\loss(\y | \Coder(\x))$ is the probability of $\y$ being the result of randomly zeroing 33\% of elements in $\Coder(\x)$.
 An example of such random masking between \name's encoder and decoder can be found in Figure~\ref{fig:grace-training}.
% trains its autoencoder and the traditional autoencoder training.
%each \y\y drawn from the distribution \loss(\y|\Coder(\x))\loss(\y | \Coder(\x)) is a result of randomly setting 30\% of elements in \Coder(\x)\Coder(\x) to zeros.

It should be noticed that the random probability distribution $\loss$ may not be expressed as an  function of $\phi$ and thus not differentiable with respect to $\phi$.
To train the weights in $\phi$, we use the REINFORCE trick~\cite{Kingma2014} to approximate this gradient by Monte-Carlo Sampling.

%Normally, to train a model, we need to calculate the gradient of Eq~??????????????????????????????\ref{eq:2} with respect to weights θ\theta and ϕ\phi. The gradient with respect to θ\theta is trivial, but since \loss\loss is a non-differentiable random function, the gradient with respect to ϕ\phi cannot be analytically derived. 
%%of the expectation of \Quality\Quality cannot be analytically derived. 
%Fortunately, we can use the REINFORCE trick~\cite{Kingma2014} which approximates this gradient by Monte-Carlo Sampling (see Appendix~???????????????????????????\ref{??} for details).


%\jc{why training encoder and decoder jointly?}


%The function \loss decides the rate of packet loss (\rates) seen by the autoencoder during training. 


\begin{figure}[t]
    \centering
%    \includegraphics[width=0.99\linewidth]{figs/ae-arch-v2.pdf}
    \includegraphics[width=0.95\linewidth]{figs/ae-arch-v3.pdf}
    \tightcaption{\name applies {\em random masking} (setting a fraction of randomly selected elements to zeros) to the NN encoder output, whereas the traditional autoencoder training has no data loss between the encoder and the decoder.
    Random masking can be made equivalent to packet loss as shown in \S\ref{subsec:packetization}.}
%    Contrasting the proposed loss-resilient design of autoencoders with traditional autoencoders.}
    \label{fig:grace-training}
\end{figure}


\mypara{Setting random masking rates in training}
%A key design choice in \name is the function \loss that governs what random data erasure rate the autoencoder learns to handle during training. 
Intuitively, in order to prepare the autoencoder to handle different rates of random masking, we should not use a fixed rate of random masking; instead, we should include many different rates of random masking from the range [0, 100\%).
However, picking the masking rate uniformly from [0, 100\%) does not work well in practice, as it will rarely see 0\% masking, which translates to \rate of 0\%, while 0\% \rate is the common case in practice. 
Thus, by default, \name uses the following distribution to pick the random masking rate:
\begin{packeditemize}
\item 80\% probability: set the random masking rate to 0\%; and
\item 20\% probability: uniformly randomly pick a masking rate from the set \{10\%,20\%,\dots,60\%\}.
\end{packeditemize}
%In \S\ref{subsec:??}, we will compare it with other training distributions of random erasure rate

\jc{need to explain why this particular distribution of simulated loss rates}



%We use a pre-trained P-frame autoencoder~\cite{dvc} to encode frames from a video (not from the training set) and test its decoded quality with an increasing rate of random data erasure (we will explain how this simulates packet losses in \S\ref{subsec:sim-losses}). 
%To emulate the effect of different packet loss rates, we randomly zero \fillme-\fillme\% of values in the autoencoder-returned data (before entropy encoding). 
%The red curve shows that as more data is received, the decoded quality gradually improves. 


%(To avoid overfitting, we test it on a different video dataset than the training dataset.)
%It is very encouraging that even a pre-trained autoencoder leads to a (suboptimal) data-scalable delivery.




%
%let the autoencoder see a variety of \rates.
%%, so that it will be prepared to deal with different packet loss outcomes. 
%When training autoencoders, \name sets \rate to zero for random 80\% of input, and for the remaining 20\% of input, it randomly selects a \rate from [0,100\%].
%In other words, it lets the autoencoder see all possible \rates, with a higher weight on 0\% packet loss.
%
%It is important to note that 0\% packet loss is used on more input because otherwise we have observe that the trained autoencoder would perform much poorly on low packet loss rates.
%It can be intuitively understood that \fillme
%\jc{mention other distributions}
%



\begin{comment}

\mypara{Graceful degradation}
Figure~\ref{fig:autoencoder-pretrained} shows an example where \name's quality degrades much more gracefully than under different rates of random data erasure. 
The model is trained on the same training dataset used by DVC, and tested on different videos (details in \S\ref{??}).
Compared to the original DVC autoencoder (which shares the same NN architecture with \name but different NN weights), the video quality of \name drops much more gracefully, as a higher fraction of random values are erased in the \aecode.


\begin{figure}[t!]
    \centering
         \includegraphics[width=0.5\linewidth]{figs/psnr-loss-vs-pretrained.pdf}
    \tightcaption{\jc{UPDATE!}
%    Loss resilience of an example pre-trained autoencoder (red). It is already data-scalable (decodable with any subset of packets), but the quality drops much faster than the graceful degradation observed in our solution. 
    % \jc{YIHUA, make the figure wider. Swap the order of the legend to "Pre-trained autoencoder" and "Our custom autoencoder"} \jc{also add a horizontal line of H.264/265 without loss}
%    Our models has a more graceful quality degradation under packet losses comparing to pretrained models
    }
    \label{fig:autoencoder-pretrained}
\end{figure}

\end{comment}


\myparaq{Why is \name loss tolerant}
As we will show in \S\ref{subsec:eval:resilience}, the quality of \name's autoencoder degrades much more gracefully than both the standard DVC autoencoders as well as other loss-resilient baselines under different rates of random masking. 
Our \name-trained autoencoders can tolerate random masking for three reasons.
%Though it is difficult to analytically interpret the NN-based encoders and decoders, there are three intuitive reasons to explain why Grace-trained autoencoders can tolerate data erasures. 
(1) The coded tensor (NN encoder output) has little stringent dependencies between its elements, making random masking less impactful on the decoding result than in H.265 output. 
(2) Empirically, we found that the \name-trained NN encoder learns to output more non-zero values, which
% in the coded tensor to contain redundant information and having more non-zero values 
\edit{both added some redundancy to the $\y$ and} allows the decoder to easily distinguish  zeroed (masked) elements.
(3) \name's training also prepares the NN decoder to recover the masked (zeroed) elements from unmasked elements. 
%, in addition to generating high-quality frames from received elements. 
\name's autoencoder can be intuitively understood as between a traditional autoencoder and generative NNs.
% In generative deep learning, there are plenty of examples where the convolutional layers, which the NN decoder mostly consists of, can reconstruct images from noisy input or even complete random input. 



%\jc{
%\begin{itemize}
%\item \aecode inherently has little structure
%\item after training, encoder learns to put more redundant information and make erased values more distinguishable
%\item training also makes the decoder learn to recover lost values (by conv layers)
%\end{itemize}
%}

%\mypara{Why training encoder and decoder jointly}
%\fillme


\tightsubsection{Randomized per-packet entropy encoding}
\label{subsec:packetization}

%\begin{itemize}
%
%\item why not cabac? why not random assignment?
%
%\item initial design
%
%\item preliminary results: psnr vs bpp
%
%\end{itemize}

Next, we need to design a packetization and entropy encoding scheme to make {\em packet loss appears to have the same random masking on the \aecode} and do so {\em without increase of data size}.
This is not possible with standard autoencoders such as~\cite{dvc}, which entropy codes the entire \aecode to a single bitstream before packetization.
As a result, any missing packet will render the bitstream undecodable. 
% (FEC does not meet our requirement since it adds substantial redundancy to the data size ().)

\begin{comment}
The autoencoders trained with Eq.~\ref{eq:2} can tolerate random data erasure on \aecode at different rates.
To make it practical, \name must entropy encode and packetize the encoder's output in a way such that {\em (1) without increase of data size, (2) packet loss appears to have the same random data erasure on the \aecode}.
\end{comment}
%More formally, the encoded

%(\eg Torchac~\cite{torchac}) 

%Traditional video codecs (\eg H.265 and VP9) also use entropy coding (CABAC).

%It is important to note that 
%(FEC can prevent )
%(as elaborated in \S\ref{??}, FEC is not ideal). 
%However, if any part of this bitstream is lost or corrupted, the whole bitstream will be undecodable.


%\, so this way of entropy coding is incompatible with DS video delivery.


%The random data erasure used in Eq.~\ref{eq:2} needs to be implemented by a practical packetization and entropy coding scheme.
%The output of an autoencoder consists of several tensors, and like in any video codec, they must be packetized and entropy-coded into a smaller-sized packet of bytestream.
%Here, we first motivate why we need a new entropy coding and packetization scheme, before proposing a potential solution.

%\myparaq{Why not existing entropy encoders}

%\mypara{Naive per-packet entropy encoding} 
\name builds on a simple idea (Figure~\ref{fig:per-packet}).
It first randomly splits the elements in \aecode into smaller sub-tensors and then entropy encodes each sub-tensor {\em separately} as an independently decodable packet. 
%for each part, assemble the elements to a smaller-sized $\z$ and feed it to $\DistributionEst$ to get the estimated distribution. {\em (iii)} For each part, use the entropy encoder and the estimated distribution to encode the elements to a bytestream. The estimated distribution will also be compressed put into the same packet.
%This way, each packet is independently decodable. 
If a packet is missing, we set its elements in the original \aecode to zeros.
Since these elements are randomly selected, zeroing them effectively mimics random masking. 
It is important to note that this scheme ensures that losing any packet appears to be uniform random masking on the \aecode.

%\jc{data erasure is independent to which packets are lost}



%This strawman solution satisfies the requirements of per-packet entropy coding: every arrived packet will be decodable no matter other packets is arrived or not. 
However, this naive method significantly increases the size of packets, \eg by 40\% compared to the entropy encoding used in traditional autoencoders.
% the entire \aecode together as in traditional autoencoders.
%---the size of the coded bistream is up-to \fillme\% larger than entropy encoding the entire \aecode before packetization as in standard autoencoders.
%To put the number into context, the PSNR of the frame encoded using this method will decrease from \fillme to \fillme when the size of the bytestream is the same as using the traditional entropy coding.
The reason for the increase is that entropy coding needs to store the {\em symbol distribution} of elements in the sub-tensors in order to compress it efficiently.
% \footnote{\jc{need a footnote to explain why can't the symbol distribution be a fixed one?}}
When the whole \aecode is compressed together, this additional overhead of symbol distribution will be marginal (5-20\% of the compressed data).
However, with the per-packet entropy coding, the symbol distribution needs to be included in each packet to make any received packet decodable, which greatly increases the total data size.


%Unfortunately, each sub-tensor has a slightly different symbol distribution, so a separate symbol distribution needs to be saved for {\em each} packet, which greatly increases the packet size.

\begin{comment}

to be most effective, each sub-tensor should be entropy-encoded and decoded using the accurate {\em symbol distribution} of values in a tensor---if either the distribution is incorrect or too big, the entropy-encoded packet size will inflate. 
%at each position and that both the coded data and the value distribution contribute to the size of a packet; 
Unfortunately, each sub-tensor may have a slightly different symbol distribution, so a separate symbol distribution needs to be saved for each packet, which increases the packet size.
%, \eg the top-left element of the first channel in the original tensor may have a totally different distribution than that of the same position in each sub-tensor, which now becomes the value of another position in the original tensor. 
%Thus, a separate value distribution is needed for each packet, which inflates the packet size.

\end{comment}

%\begin{subtask}
%{\bf Low packetization and entropy-coding overhead.} 
%Propose a packetization and entropy coding scheme for DS autoencoder output such that each packet is independently decodable but {\em without} much size inflation of the coded data.
%%with minimum compression overhead compared to traditional codecs.
%\end{subtask}

%Fortunately, this problem is not intractable. 
%Here we present an initial design and plan a more systematic examination for the proposed task. 

%\mypara{Initial ideas} 
%\mypara{Coarse-grained }


To solve this conundrum, we leverage the fact that autoencoder training regularizes the distribution of  elements in each channel of a \aecode (A \aecode in DVC has 224 channels, each having 48$\times$80 elements) to follow a Laplace distribution with a mean of zero. 
This means that the variance (a single float) is enough to describe the symbol distribution in each channel of a \aecode, and the entropy encoding will be as efficient.
%This leads to a simple yet effective solution---we can use just the variance (a single float) to describe the symbol distribution in each channel of a \aecode, and the entropy encoding will be as efficient.
Such {\em coarse-grained} symbol distribution needs 10$\times$ fewer bits to store than the naive per-packet entropy encoding: even if there are 20 packets, adding the symbol distribution to each packet only increase the total data size by no more than 5\%.

\edit{The concept under discussion is inapplicable to conventional codecs such as H.264, primarily due to their inability to randomly shuffle the coded byte stream prior to entropy encoding. H.264, for instance, capitalizes on the likelihood of adjacent macroblocks having similar motion vector values, thereby enabling the reuse of the symbol distribution. Random shuffling of the macroblocks in H.264 disrupts this adjacency, preventing code blocks in the byte stream from sharing the same distribution, and inevitably leading to size inflation~\cite{KUMAR2006425}.}


%\jc{Yihua, any reason for it to be so?}
%\jc{need a figure to illustrate this. talk to yihua}


\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v3.pdf}
%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v4.pdf}
        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v5.pdf}
    \tightcaption{Example of \name's packetization and per-packet entropy encoding. When a packet is lost, the elements mapped to it will be set to zeros.}
    \label{fig:per-packet}
\end{figure}

\begin{comment}
This observation inspires a simple yet effective solution: using a {\em coarser-grained} symbol distribution, which has only the standard deviation per channel, can entropy encode data almost as efficiently as using the real symbol distribution.
Compared to the symbol distribution needed by the original DVC model, a coarse-grained symbol distribution needs \fillme$\times$ fewer bits to store.
Thus, even if there are 20 packets, adding the symbol distribution to each packet only increase the total data size by no more than \fillme\%.
\end{comment}

%The reason is that each sub-tensor has multiple channels (\eg 96 channels in our case), and the values of the same channel are either similar (mostly small values) or bimodal (only a few similarly large values), so using a coarse-grained distribution can effectively represent their distributions and lead to an entropy-coded data size that compared to the coded size using the accurate value distribution is slightly larger  but only by a small margin.
%Since these coarse-grained symbol distributions need fewer bits to store, they will add to a negligible fraction of each packet. 

\begin{comment}
    

Moreover, the use of coarse-grained symbol distribution allows us to reuse symbol distributions. 
In particular, we pre-define 64 different standard deviations as candidate distributions of each channel. 
Then for each channel's standard deviation, the sender simply adds the index (an integer) of the standard deviation that is most similar to the real one. 

\end{comment}

% and observe that in most \aecodes, the symbol distribution can be very closely approximated by one of these candidate symbol, so the sender can simply add the index of the symbol distribution in each packet.

%We propose to store the value distribution of each channel in a {\em coarser} granularity (\eg only a mean and standard deviation) so they are slightly less accurate but much easier to store, and as a result, these distributions will take an almost negligible fraction of each packet. 
%The insight is that each sub-tensor has multiple channels (\eg 96 channels in our case), and the values of the same channel are either similar (mostly small values) or bimodal (only a few similarly large values), so using a coarse-grained distribution can effectively represent their distributions and lead to an entropy-coded data size that compared to the coded size using the accurate value distribution is slightly larger  but only by a small margin.

% \jc{Yihua, is this also similar to how CABAC avoid sending symbol distribution?}

%\jc{more evidence and intuition}



==> sections/old/technical_v8.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US






\begin{figure*}[t!]
    \centering
         \centering
        \includegraphics[width=0.97\linewidth]{figs/dvc-arch-v3.pdf}
    \tightcaption{Workflow of the autoencoder in \name.}
    \label{fig:dvc-arch}
\end{figure*}

\tightsection{\name: Data-Scalable Autoencoder}
\label{sec:core}

%\name is a concrete instantiation of data-scalable delivery. 
We present, \name, a new {\em autoencoder}-based video coding system.
This section begins with a primer of traditional autoencoders and their limitations and then presents two basic ideas that make \name data-scalable when packet loss affects only one frame.
%---the new autoencoder training to tolerate random data erasure (\S???\ref{subsec:??}) and a custom scheme of packetization and entropy encoding to equate packet loss and data erasure (\S???\ref{subsec:??}).
The next section will describe the video delivery framework over \name's autoencoder.

%designed to achieve close-to-optimal data-scalable coding. 

%and a custom delivery framework for the new autoencoder (\S???\ref{sec:delivery}).
%We will describe the autoencoder design in this section, followed by the delivery framework in the next section. 

\tightsubsection{Autoencoder primer and limitations}
\label{subsec:ae-background}

Autoencoders use learned neural networks (NNs), instead of handcrafted logics, to encode and decode video frames.
We denote the encoder by $\Coder$ (with its NN weights $\phi$) and the decoder by $\Decoder$ (with its NN weights $\theta$).
The encoder encodes a frame $\x$ to a {\em \aecode} $\y=\Coder(\x)$, and the decoder decodes $\y$ to a reconstructed frame $\hat{\x}=\Decoder(\y)$.
%For an input frame \x\x (a c×w×hc\times w\times h tensor), the \aecode is the output of the encoder \y=\Coder(\x)\y=\Coder(\x)  will be sent to the receiver, which then runs the decoder to reconstruct the original frame from \y\y: ^\x=\Decoder(\y)\hat{\x}=\Decoder(\y).
Traditionally, autoencoder training minimizes the following expectation (\ie training loss function):% over inputs from training frames \X\X:
\vspace{-0.04cm}
\begin{align}
%\textrm{\bf min~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\y), \y, \x)\textrm{, where }\y = \Coder(\x)
%\textrm{\bf min~~} \mathbb{E}_{\x} \Distort(\Decoder(\y), \x)+\alpha\cdot\Size(\y)\textrm{, where }\y = \Coder(\x)\\
%\textrm{\bf min~} 
\mathbb{E}_{\x} {\color{black}\underbrace{\highlight{black}{$\Distort(\Decoder(\y), \x)$}}_{\text{\sf \footnotesize \textcolor{black!85}{Pixel error}}}}+
\alpha{\cdot}{\color{black}\underbrace{\highlight{black}{$\Size(\y)$}}_{\text{\sf \footnotesize \textcolor{black!85}{Encoded size}}}}\textrm{, where }\y = \Coder(\x)
\label{eq:1}
\vspace{-0.08cm}
\end{align}
Here, $\Distort(\hat{\x},\x)$ is the pixel-level reconstruction error of the decoded frame $\hat{\x}$ (by default, L2-norm\footnote{
Note that L2-norm (or mean squared error) of $\hat{\x}$ and $\x$ are closely related to PSNR of $\hat{\x}$. To avoid this bias, 
our evaluation in \S\ref{sec:eval} measures the quality improvement in SSIM and user subjective studies.
% To avoid bias towards PSNR, our evaluation in \S\ref{sec:eval} measures the quality improvement in not only PSNR, but also SSIM and user subjective studies.
Following the common practice of autoencoder training, the training loss function also includes the reconstruction loss of the motion-compensated prediction. 
%Pixel-wise distortion may not be the best way to capture human perception of reconstructed images, but it is often used in autoencoder training for its differentiability. We will evaluate the trained autoencoders in terms of more standard metrics, such as SSIM and PSNR (in RGB and YUV).
} of $\hat{\x}-\x$), and $Size(\y)$ is the entropy-coded data size of $\y$ in bit-per-pixel (BPP).
The parameter $\alpha$ influences the size/quality tradeoff: a higher $\alpha$ leads to smaller frame size ($Size(\hat{x})$) but higher distortion (\ie poorer quality) of the reconstructed frame $\hat{\x}$.
% will tend to have better visual quality in $\Decoder(\z)$ but also higher bitrate. 
%In Eq.~\ref{eq:1}, s
Since all of the functions---$\Coder$, $\Decoder$, $\Distort$ and $\Size$ (which is approximated by a pre-trained NN~\cite{dvc})---are differentiable, the NN weights $\phi$ and $\theta$ can be trained jointly to minimize Eq.~\ref{eq:1}.




%\jc{refer to fig~\ref{fig:dvc-arch}}



This work focuses primarily on encoding P-frames, the most common frame type in real-time videos as mentioned in \S\ref{subsec:background}. 
Specifically, we use the NN architectures of DVC~\cite{dvc}, a popular autoencoder, whose architecture is depicted in Figure~\ref{fig:dvc-arch}.
(We will discuss I-frame in \S\ref{subsec:protocol}, and B-frames are rarely used in real-time videos~\cite{ffmpegstreaming}.)
%Figure~?????????????????????????????????????????????\ref{fig:dvc-arch} describes the typical workflow of a P-frame autoencoder, which \name follows.
%Rather than compressing frames from scratch, the workflow 
It is comprised of steps (\eg motion and residual estimation) typically found in a traditional video codec (\S\ref{subsec:background}) but  uses NNs to replace
%Most recent video autoencoders~\cite{??,??,??} combine useful concepts from traditional codecs (\eg motion vectors and residuals) and replace 
handcrafted heuristics for motion estimation, compensation, and \st{transformation} \edit{compression} of residual and motion vectors.
%, and they achieve compression efficiency comparable to recent video codecs.
Since they are trained on large sets of videos (\eg Vimeo-90K~\cite{vimeo-dataset}), their compression efficiency is comparable to recent video codes and is reasonably generalizable across a variety of video content (which we also observe in our evaluation \S\ref{sec:eval}).
For these reasons, autoencoders attract increasing attention from the multimedia community~\cite{dvc, swift, hu2021fvc}.
%, and achieve comparable compression efficiency as recent compression algorithms.

\mypara{Limitations}
Currently autoencoders still requires traditional schemes (like FEC) to handle packet loss. 
Their lack of packet loss tolerance is due to two reasons.
\begin{packeditemize}

\item The standard autoencoder training (\ie minimizing Eq.~\ref{eq:1}) implicitly assumes that the encoder's output equals the decoder's input,
% \footnote{A recent work~\cite{??,??} adds Gaussian random noise\jc{check!} between the encoder and decoder to simulate wireless signal noise, but this is different from packet loss which masks a fraction of the data.}, 
so it does not prepare the autoencoder to handle data loss between the encoder and decoder. 

\item Entropy encoding used in autoencoders compresses the whole encoder output as a single bitstream, so any data loss will render it undecodeable.

%current autoencoder training assumes that the encoder's output equals the decoder's input, so the trained models are not prepared to handle data loss between the encoder and decoder. 
\end{packeditemize}


%\tightsubsection{Overview of \name}

\mypara{Roadmap}
At a high level, we address these problems in two logical steps:
\begin{packeditemize}
\item 
%{\em Turning packet loss to random data erasure:} 
We use a new packetization and entropy-coding logic to make packet loss (with \rate of $n\%$) have the same effect as randomly setting $n\%$ of elements in the \aecode to zeros, \ie $n\%$ {\em random masking} of \aecode.
\item 
%{\em Training for resilience random data erasure:} 
Then, we re-train the autoencoder such that its quality degrades gracefully with more {\em random masking} on the \aecode (\ie setting more elements in $\y$ to zeros).
\end{packeditemize}
%As a result, the autoencoder will be data-scalable with respect to packet loss. 

\zy{Those two steps are in different orders in the following sections (3.2 and 3.3)}
\begin{comment}

Specifically, we first leverage that the autoencoder NNs are trainable and use a new training process to optimize the quality when different fractions of randomly selected elements in \y\y are set to zeros. 
In other words, the autoencoder is data-scalable, if the packet loss is in the form of random data erasure.
Next, we use a new packetization and entropy coding logic, such that packet loss with a \rate of n%n\%  has the same effect on \aecode \y\y as randomly erasing (zeroing) n%n\% of elements in \y\y.


% resilient to {\em random data erasure}---the quality is optimized when $n\%$ of randomly selected elements in $\y$ are set to zeros. 
%
%degrades gracefully if more randomly selected elements in $\y$ are set to zeros.
%
%Put together, the quality of the new autoencoder will meet the three 


so that the quality of the trained autoencoder degrades gracefully with higher rate of {\em random data erasure} in the \aecode $\y$, \ie setting a fraction of random elements in $\y$ to zeros. 
(2) Second, we change the packetization and entropy coding logic, so that packet loss with a \rate of $n\%$  has the same effect on \aecode $\y$ as randomly erasing (zeroing) $n\%$ of elements in $\y$.
\end{comment}



%assume that the impact of packet loss of \rate $=n\%$ on the encoder's output $\y$ is that a subset of random $n\%$ of elements in $\y$ are set to zeros.
%We call this {\em random data erasure}, and present a practical design to realize this assumption in \S\ref{??}.
%We will also explain why the choice of random data erasure is reasonable in \S\ref{??}.





%\begin{figure}[t!]
%    \centering
%         \centering
%        \includegraphics[width=0.99\linewidth]{figs/dvc-arch.pdf}
%    \tightcaption{}
%    \label{fig:dvc-arch}
%\end{figure}


\tightsubsection{Training \name's data-scalable autoencoders}
\label{subsec:training}





%The training process in Eq.~???????????????????????????\ref{eq:1} can be equivalently viewed as having a lossless channel between the encoder to the decoder, \ie the decoder's input equals the encoder's output. 

We begin with the second step---training autoencoders that are resilient to various rate of random masking, assuming that missing one of $n$ packet has the same effect as random masking of $1/n$ elements (we will explain how to do it in \S\ref{subsec:packetization}).
%In order to let autoencoders perform well under various rates of random data erasure, 
To this end, \name jointly trains the encoder and decoder NNs to minimize: 
%which uses a random distribution \loss\loss to simulate the effect of packet loss on the encoder's output:
\vspace{-0.04cm}
\begin{align}
%\textrm{\bf min~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\y), \x)\textrm{, where }
%\color{blue}\underbrace{\highlight{blue}{\y∼\loss(\y|\Coder(\x))\y\sim \loss(\y | \Coder(\x))}}_{\text{\sf \footnotesize \textcolor{blue!85}{Simulating packet loss}}}
\mathbb{E}_{\x} \Distort(\Decoder(\y), \x)+\alpha{\cdot}\Size(\y)\textrm{, where }
\color{blue}\underbrace{\highlight{newblue}{$\y\sim \loss(\y | \Coder(\x))$}}_{\text{\sf  \footnotesize \textcolor{blue}{Simulate packet loss}}}
\label{eq:2}
\vspace{-0.04cm}
\end{align}
%where the change is highlighted in color.
The key difference to the traditional autoencoder loss function Eq.~\ref{eq:1} (highlighted in blue) is the distribution function $\loss$, which characterizes the distribution of decoder input.
%Given the encoder output \Coder(\x)\Coder(\x), \loss\loss represents the data distribution seen by the decoder. 
%Remember that 
For instance, with a 
\rate of 33\%, $\loss(\y | \Coder(\x))$ is the probability of $\y$ being the result of randomly zeroing 33\% of elements in $\Coder(\x)$.
 An example of such random masking between \name's encoder and decoder can be found in Figure~\ref{fig:grace-training}.
% trains its autoencoder and the traditional autoencoder training.
%each \y\y drawn from the distribution \loss(\y|\Coder(\x))\loss(\y | \Coder(\x)) is a result of randomly setting 30\% of elements in \Coder(\x)\Coder(\x) to zeros.

It should be noticed that the random probability distribution $\loss$ may not be expressed as an  function of $\phi$ and thus not differentiable with respect to $\phi$.
To train the weights in $\phi$, we use the REINFORCE trick~\cite{Kingma2014} to approximate this gradient by Monte-Carlo Sampling.

%Normally, to train a model, we need to calculate the gradient of Eq~??????????????????????????????\ref{eq:2} with respect to weights θ\theta and ϕ\phi. The gradient with respect to θ\theta is trivial, but since \loss\loss is a non-differentiable random function, the gradient with respect to ϕ\phi cannot be analytically derived. 
%%of the expectation of \Quality\Quality cannot be analytically derived. 
%Fortunately, we can use the REINFORCE trick~\cite{Kingma2014} which approximates this gradient by Monte-Carlo Sampling (see Appendix~???????????????????????????\ref{??} for details).


%\jc{why training encoder and decoder jointly?}


%The function \loss decides the rate of packet loss (\rates) seen by the autoencoder during training. 


\begin{figure}[t]
    \centering
%    \includegraphics[width=0.99\linewidth]{figs/ae-arch-v2.pdf}
    \includegraphics[width=0.95\linewidth]{figs/ae-arch-v3.pdf}
    \tightcaption{\name applies {\em random masking} (setting a fraction of randomly selected elements to zeros) to the NN encoder output, whereas the traditional autoencoder training has no data loss between the encoder and the decoder.
    Random masking can be made equivalent to packet loss as shown in \S\ref{subsec:packetization}.}
%    Contrasting the proposed loss-resilient design of autoencoders with traditional autoencoders.}
    \label{fig:grace-training}
\end{figure}


\mypara{Setting random masking rates in training}
%A key design choice in \name is the function \loss that governs what random data erasure rate the autoencoder learns to handle during training. 
Intuitively, in order to prepare the autoencoder to handle different rates of random masking, we should not use a fixed rate of random masking; instead, we should include many different rates of random masking from the range [0, 100\%).
However, picking the masking rate uniformly from [0, 100\%) does not work well in practice, as it will rarely see 0\% masking, which translates to \rate of 0\%, while 0\% \rate is the common case in practice. 
Thus, by default, \name uses the following distribution to pick the random masking rate:
\begin{packeditemize}
\item 80\% probability: set the random masking rate to 0\%; and
\item 20\% probability: uniformly randomly pick a masking rate from the set \{10\%,20\%,\dots,60\%\}.
\end{packeditemize}
%In \S\ref{subsec:??}, we will compare it with other training distributions of random erasure rate

\jc{need to explain why this particular distribution of simulated loss rates}



%We use a pre-trained P-frame autoencoder~\cite{dvc} to encode frames from a video (not from the training set) and test its decoded quality with an increasing rate of random data erasure (we will explain how this simulates packet losses in \S\ref{subsec:sim-losses}). 
%To emulate the effect of different packet loss rates, we randomly zero \fillme-\fillme\% of values in the autoencoder-returned data (before entropy encoding). 
%The red curve shows that as more data is received, the decoded quality gradually improves. 


%(To avoid overfitting, we test it on a different video dataset than the training dataset.)
%It is very encouraging that even a pre-trained autoencoder leads to a (suboptimal) data-scalable delivery.




%
%let the autoencoder see a variety of \rates.
%%, so that it will be prepared to deal with different packet loss outcomes. 
%When training autoencoders, \name sets \rate to zero for random 80\% of input, and for the remaining 20\% of input, it randomly selects a \rate from [0,100\%].
%In other words, it lets the autoencoder see all possible \rates, with a higher weight on 0\% packet loss.
%
%It is important to note that 0\% packet loss is used on more input because otherwise we have observe that the trained autoencoder would perform much poorly on low packet loss rates.
%It can be intuitively understood that \fillme
%\jc{mention other distributions}
%



\begin{comment}

\mypara{Graceful degradation}
Figure~\ref{fig:autoencoder-pretrained} shows an example where \name's quality degrades much more gracefully than under different rates of random data erasure. 
The model is trained on the same training dataset used by DVC, and tested on different videos (details in \S\ref{??}).
Compared to the original DVC autoencoder (which shares the same NN architecture with \name but different NN weights), the video quality of \name drops much more gracefully, as a higher fraction of random values are erased in the \aecode.


\begin{figure}[t!]
    \centering
         \includegraphics[width=0.5\linewidth]{figs/psnr-loss-vs-pretrained.pdf}
    \tightcaption{\jc{UPDATE!}
%    Loss resilience of an example pre-trained autoencoder (red). It is already data-scalable (decodable with any subset of packets), but the quality drops much faster than the graceful degradation observed in our solution. 
    % \jc{YIHUA, make the figure wider. Swap the order of the legend to "Pre-trained autoencoder" and "Our custom autoencoder"} \jc{also add a horizontal line of H.264/265 without loss}
%    Our models has a more graceful quality degradation under packet losses comparing to pretrained models
    }
    \label{fig:autoencoder-pretrained}
\end{figure}

\end{comment}


\myparaq{Why is \name loss tolerant}
As we will show in \S\ref{subsec:eval:resilience}, the quality of \name's autoencoder degrades much more gracefully than both the standard DVC autoencoders as well as other loss-resilient baselines under different rates of random masking. 
Our \name-trained autoencoders can tolerate random masking for three reasons.
%Though it is difficult to analytically interpret the NN-based encoders and decoders, there are three intuitive reasons to explain why Grace-trained autoencoders can tolerate data erasures. 
(1) The coded tensor (NN encoder output) has little stringent dependencies between its elements, making random masking less impactful on the decoding result than in H.265 output. 
(2) Empirically, we found that the \name-trained NN encoder learns to output more non-zero values, which
% in the coded tensor to contain redundant information and having more non-zero values 
\edit{both added some redundancy to the $\y$ and} allows the decoder to easily distinguish  zeroed (masked) elements.
(3) \name's training also prepares the NN decoder to recover the masked (zeroed) elements from unmasked elements. 
%, in addition to generating high-quality frames from received elements. 
\name's autoencoder can be intuitively understood as between a traditional autoencoder and generative NNs.
% In generative deep learning, there are plenty of examples where the convolutional layers, which the NN decoder mostly consists of, can reconstruct images from noisy input or even complete random input. 



%\jc{
%\begin{itemize}
%\item \aecode inherently has little structure
%\item after training, encoder learns to put more redundant information and make erased values more distinguishable
%\item training also makes the decoder learn to recover lost values (by conv layers)
%\end{itemize}
%}

%\mypara{Why training encoder and decoder jointly}
%\fillme


\tightsubsection{Randomized per-packet entropy encoding}
\label{subsec:packetization}

%\begin{itemize}
%
%\item why not cabac? why not random assignment?
%
%\item initial design
%
%\item preliminary results: psnr vs bpp
%
%\end{itemize}

Next, we need to design a packetization and entropy encoding scheme to make {\em packet loss appears to have the same random masking on the \aecode} and do so {\em without increase of data size}.
This is not possible with standard autoencoders such as~\cite{dvc}, which entropy codes the entire \aecode to a single bitstream before packetization.
As a result, any missing packet will render the bitstream undecodable. 
% (FEC does not meet our requirement since it adds substantial redundancy to the data size ().)

Traditional codecs do have techniques to make each packet individually decodable, such as flexible macroblock ordering~\cite{lambert2006flexible} in H.264. These techniques divids the input frame into independent, non-overlapping partitions. Each partition is encoded separately, packed into its own entropy-encoded packet, enabling decodability if the corresponding packet arrives, as there's no dependency on other packets.

However, this method leads to substantial size inflation, up to \editSOCC{50\%}~\cite{???}, due to the loss of compression efficiency inherent in traditional codecs' exploitation of content dependencies. For example, if two adjacent macroblocks share identical motion vectors (which is common in practice), H.264 can transmit the motion values once. But, if these macroblocks are separated into different partitions, each partition must send the value, resulting in size inflation.

\name employs a different method as shown in Figure~\ref{fig:per-packet}. Instead of dividing the input frame, it {\em randomly} splits the elements in the coded tensor into sub-tensors and entropy encodes each sub-tensor separately. 
The entropy coding in \name necessitates storing the symbol distribution of elements in the coded tensors for efficient compression. This means that, unlike methods that only send the symbol distribution once, our method requires storing it in every packet, potentially leading to additional overhead.
However, this overhead is mitigated by the autoencoder training, which regularizes the distribution of elements in each coded tensor's channel to adhere to a zero-mean Laplace distribution. The variance value of each channel can be efficiently encapsulated with just a few bits. As a result, the overhead of including the symbol distribution in each packet remains minimal: even with 20 packets, the symbol distribution's size does not exceed 5\% of the total frame size.

In \name, if a packet goes missing, we zero its elements in the original coded tensor. Given the random selection of these elements during encoding, this process effectively emulates random element masking, which matches the technique implemented during training. 
Importantly, this approach ensures that the loss of any packet simulates a uniform random mask on the encoded tensor.

The key difference between the per-packet entropy coding method used in traditional codecs and our method is that we don't have size inflation. This is because \name is not exploiting the dependency between elements for a better compression ratio, instead, it has fewer elements in the encoded data than traditional codecs. More specifically, in traditional codecs like H.264, each pixel has its motion vector and residual encoded in the bytestream, but \name's autoencoder will map the motion vector (or residual) of multiple pixels into the same element in the coded tensor. Therefore, \name can achieve the same size as traditional codecs without using dependencies between elements. During training, the autoencoder also learns to generate details to ensure that the quality does not drop even if we are sending less information than the traditional codecs.

% \editSOCC{
% New flow: 
% \begin{itemize}
%     \item traditional codecs also have similar techniques (citations...). However, they are directly splitting the content, which will cause size inflation because there will be redundancy among the partitions. 
%     \item In contrast, our technique does not split the content but split the encoded tensor. ... describe how our randomized per-packet entropy coding works
%     \item Our method does not incur much overhead. The output size is determined by 2 parts: distribution and bytestream .... because the NN encoder regularizes the distribution of encoded elements in each channel during training, send the distribution within each packet does not cause much overhead.
%     \item This technique is unique to autoencoder (cannot be applied on traditional codec without a NN transformation), because ...
% \end{itemize}
% }

\begin{comment}
The autoencoders trained with Eq.~\ref{eq:2} can tolerate random data erasure on \aecode at different rates.
To make it practical, \name must entropy encode and packetize the encoder's output in a way such that {\em (1) without increase of data size, (2) packet loss appears to have the same random data erasure on the \aecode}.
\end{comment}
%More formally, the encoded

%(\eg Torchac~\cite{torchac}) 

%Traditional video codecs (\eg H.265 and VP9) also use entropy coding (CABAC).

%It is important to note that 
%(FEC can prevent )
%(as elaborated in \S\ref{??}, FEC is not ideal). 
%However, if any part of this bitstream is lost or corrupted, the whole bitstream will be undecodable.


%\, so this way of entropy coding is incompatible with DS video delivery.


%The random data erasure used in Eq.~\ref{eq:2} needs to be implemented by a practical packetization and entropy coding scheme.
%The output of an autoencoder consists of several tensors, and like in any video codec, they must be packetized and entropy-coded into a smaller-sized packet of bytestream.
%Here, we first motivate why we need a new entropy coding and packetization scheme, before proposing a potential solution.

%\myparaq{Why not existing entropy encoders}

\begin{comment}
%\mypara{Naive per-packet entropy encoding} 
\name builds on a simple idea (Figure~\ref{fig:per-packet}).
It first randomly splits the elements in \aecode into smaller sub-tensors and then entropy encodes each sub-tensor {\em separately} as an independently decodable packet. 
%for each part, assemble the elements to a smaller-sized $\z$ and feed it to $\DistributionEst$ to get the estimated distribution. {\em (iii)} For each part, use the entropy encoder and the estimated distribution to encode the elements to a bytestream. The estimated distribution will also be compressed put into the same packet.
%This way, each packet is independently decodable. 
If a packet is missing, we set its elements in the original \aecode to zeros.
Since these elements are randomly selected, zeroing them effectively mimics random masking. 
It is important to note that this scheme ensures that losing any packet appears to be uniform random masking on the \aecode.

%\jc{data erasure is independent to which packets are lost}



%This strawman solution satisfies the requirements of per-packet entropy coding: every arrived packet will be decodable no matter other packets is arrived or not. 
However, this naive method significantly increases the size of packets, \eg by 40\% compared to the entropy encoding used in traditional autoencoders.
% the entire \aecode together as in traditional autoencoders.
%---the size of the coded bistream is up-to \fillme\% larger than entropy encoding the entire \aecode before packetization as in standard autoencoders.
%To put the number into context, the PSNR of the frame encoded using this method will decrease from \fillme to \fillme when the size of the bytestream is the same as using the traditional entropy coding.
The reason for the increase is that entropy coding needs to store the {\em symbol distribution} of elements in the sub-tensors in order to compress it efficiently.
% \footnote{\jc{need a footnote to explain why can't the symbol distribution be a fixed one?}}
When the whole \aecode is compressed together, this additional overhead of symbol distribution will be marginal (5-20\% of the compressed data).
However, with the per-packet entropy coding, the symbol distribution needs to be included in each packet to make any received packet decodable, which greatly increases the total data size.
\end{comment}


%Unfortunately, each sub-tensor has a slightly different symbol distribution, so a separate symbol distribution needs to be saved for {\em each} packet, which greatly increases the packet size.

\begin{comment}

to be most effective, each sub-tensor should be entropy-encoded and decoded using the accurate {\em symbol distribution} of values in a tensor---if either the distribution is incorrect or too big, the entropy-encoded packet size will inflate. 
%at each position and that both the coded data and the value distribution contribute to the size of a packet; 
Unfortunately, each sub-tensor may have a slightly different symbol distribution, so a separate symbol distribution needs to be saved for each packet, which increases the packet size.
%, \eg the top-left element of the first channel in the original tensor may have a totally different distribution than that of the same position in each sub-tensor, which now becomes the value of another position in the original tensor. 
%Thus, a separate value distribution is needed for each packet, which inflates the packet size.

\end{comment}

%\begin{subtask}
%{\bf Low packetization and entropy-coding overhead.} 
%Propose a packetization and entropy coding scheme for DS autoencoder output such that each packet is independently decodable but {\em without} much size inflation of the coded data.
%%with minimum compression overhead compared to traditional codecs.
%\end{subtask}

%Fortunately, this problem is not intractable. 
%Here we present an initial design and plan a more systematic examination for the proposed task. 

%\mypara{Initial ideas} 
%\mypara{Coarse-grained }

\begin{comment}
To solve this conundrum, we leverage the fact that autoencoder training regularizes the distribution of  elements in each channel of a \aecode (A \aecode in DVC has 224 channels, each having 48$\times$80 elements) to follow a Laplace distribution with a mean of zero. 
This means that the variance (a single float) is enough to describe the symbol distribution in each channel of a \aecode, and the entropy encoding will be as efficient.
%This leads to a simple yet effective solution---we can use just the variance (a single float) to describe the symbol distribution in each channel of a \aecode, and the entropy encoding will be as efficient.
Such {\em coarse-grained} symbol distribution needs 10$\times$ fewer bits to store than the naive per-packet entropy encoding: even if there are 20 packets, adding the symbol distribution to each packet only increase the total data size by no more than 5\%.

The concept under discussion is inapplicable to conventional codecs such as H.264, primarily due to their inability to randomly shuffle the coded byte stream prior to entropy encoding. H.264, for instance, capitalizes on the likelihood of adjacent macroblocks having similar motion vector values, thereby enabling the reuse of the symbol distribution. Random shuffling of the macroblocks in H.264 disrupts this adjacency, preventing code blocks in the byte stream from sharing the same distribution, and inevitably leading to size inflation~\cite{KUMAR2006425}.

\end{comment}


%\jc{Yihua, any reason for it to be so?}
%\jc{need a figure to illustrate this. talk to yihua}


\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v3.pdf}
%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v4.pdf}
        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v5.pdf}
    \tightcaption{Example of \name's packetization and per-packet entropy encoding. When a packet is lost, the elements mapped to it will be set to zeros.}
    \label{fig:per-packet}
\end{figure}

\begin{comment}
This observation inspires a simple yet effective solution: using a {\em coarser-grained} symbol distribution, which has only the standard deviation per channel, can entropy encode data almost as efficiently as using the real symbol distribution.
Compared to the symbol distribution needed by the original DVC model, a coarse-grained symbol distribution needs \fillme$\times$ fewer bits to store.
Thus, even if there are 20 packets, adding the symbol distribution to each packet only increase the total data size by no more than \fillme\%.
\end{comment}

%The reason is that each sub-tensor has multiple channels (\eg 96 channels in our case), and the values of the same channel are either similar (mostly small values) or bimodal (only a few similarly large values), so using a coarse-grained distribution can effectively represent their distributions and lead to an entropy-coded data size that compared to the coded size using the accurate value distribution is slightly larger  but only by a small margin.
%Since these coarse-grained symbol distributions need fewer bits to store, they will add to a negligible fraction of each packet. 

\begin{comment}
    

Moreover, the use of coarse-grained symbol distribution allows us to reuse symbol distributions. 
In particular, we pre-define 64 different standard deviations as candidate distributions of each channel. 
Then for each channel's standard deviation, the sender simply adds the index (an integer) of the standard deviation that is most similar to the real one. 

\end{comment}

% and observe that in most \aecodes, the symbol distribution can be very closely approximated by one of these candidate symbol, so the sender can simply add the index of the symbol distribution in each packet.

%We propose to store the value distribution of each channel in a {\em coarser} granularity (\eg only a mean and standard deviation) so they are slightly less accurate but much easier to store, and as a result, these distributions will take an almost negligible fraction of each packet. 
%The insight is that each sub-tensor has multiple channels (\eg 96 channels in our case), and the values of the same channel are either similar (mostly small values) or bimodal (only a few similarly large values), so using a coarse-grained distribution can effectively represent their distributions and lead to an entropy-coded data size that compared to the coded size using the accurate value distribution is slightly larger  but only by a small margin.

% \jc{Yihua, is this also similar to how CABAC avoid sending symbol distribution?}

%\jc{more evidence and intuition}



==> sections/old/technical_v9.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en_US







\tightsection{Training \name's autoencoder}
\label{sec:core}


The next two sections present \name's training process of its autoencoder and online video delivery framework, respectively.
The key idea is to achieve DS coding by {\em jointly training the NN encoder and NN decoder of an autoencoder under different packet loss rates}.
We begin with how to simulate packet loss, and then
% such that losing one out of $n$ packets has the same effect as randomly zeroing $1/n$ values in the encoder's output. 
describe \name training process to optimize quality under various packet loss rates.

%In this section, we will first describe the training procedure with the assumption that packet loss appears to be setting values at random positions of the encoder output to zeros. 
%Then we will present a concrete packetization scheme realizes this assumption, so that the trained autoencoder effectively learns how to decode data affected by packet loss.

%
%\jc{this section needs more work}
%
%%\name is a concrete instantiation of data-scalable delivery. 
%We present, \name, a new {\em autoencoder}-based video coding system.
%This section presents the training  make \name data-scalable when packet loss affects only one frame.
%%---the new autoencoder training to tolerate random data erasure (\S???\ref{subsec:??}) and a custom scheme of packetization and entropy encoding to equate packet loss and data erasure (\S???\ref{subsec:??}).
%The next section will describe the video delivery framework over \name's autoencoder.

%designed to achieve close-to-optimal data-scalable coding. 

%and a custom delivery framework for the new autoencoder (\S???\ref{sec:delivery}).
%We will describe the autoencoder design in this section, followed by the delivery framework in the next section. 

%\tightsubsection{Training loss}

\mypara{Terminology}
Figure~\ref{fig:dvc-arch} shows the workflow of \name's encoder (sender) and decoder (receiver).
The encoder's output is a coded tensor that entails both encoded motion vector (MV) and encoded residuals. 
(We provide details of these tensors in Appendix~\ref{app:details}.
We denote the encoder by $\Coder$ (with its NN weights $\phi$) and the decoder by $\Decoder$ (with its NN weights $\theta$).
The encoder encodes a frame $\x$ to a {\em \aecode} $\y=\Coder(\x)$, and the decoder decodes $\y$ to a reconstructed frame $\hat{\x}=\Decoder(\y)$.
Traditionally, autoencoder training minimizes the following training loss function:% over inputs from training frames \X\X:
\vspace{-0.04cm}
\begin{align}
%\textrm{\bf min~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\y), \y, \x)\textrm{, where }\y = \Coder(\x)
%\textrm{\bf min~~} \mathbb{E}_{\x} \Distort(\Decoder(\y), \x)+\alpha\cdot\Size(\y)\textrm{, where }\y = \Coder(\x)\\
%\textrm{\bf min~} 
\mathbb{E}_{\x} {\color{black}\underbrace{\highlight{black}{$\Distort(\Decoder(\y), \x)$}}_{\text{\sf \footnotesize \textcolor{black!85}{Pixel error}}}}+
\alpha{\cdot}{\color{black}\underbrace{\highlight{black}{$\Size(\y)$}}_{\text{\sf \footnotesize \textcolor{black!85}{Encoded size}}}}\textrm{, where }\y = \Coder(\x)
\label{eq:1}
\vspace{-0.08cm}
\end{align}
Here, $\Distort(\hat{\x},\x)$ is the pixel-level reconstruction error of the decoded frame $\hat{\x}$ (by default, L2-norm\footnote{
Note that L2-norm (or mean squared error) of $\hat{\x}$ and $\x$ are closely related to PSNR of $\hat{\x}$. To avoid this bias, 
our evaluation in \S\ref{sec:eval} measures the quality improvement in SSIM and user subjective studies.
% To avoid bias towards PSNR, our evaluation in \S\ref{sec:eval} measures the quality improvement in not only PSNR, but also SSIM and user subjective studies.
% Following the common practice of autoencoder training, the training loss function also includes the reconstruction loss of the motion-compensated prediction. 
%Pixel-wise distortion may not be the best way to capture human perception of reconstructed images, but it is often used in autoencoder training for its differentiability. We will evaluate the trained autoencoders in terms of more standard metrics, such as SSIM and PSNR (in RGB and YUV).
} of $\hat{\x}-\x$), and $Size(\y)$ is the entropy-coded data size of $\y$ in bit-per-pixel (BPP).
The parameter $\alpha$ governs the size-quality tradeoff: a higher $\alpha$ leads to smaller frame size ($Size(\hat{x})$) but higher distortion (\ie poorer quality) of the reconstructed frame $\hat{\x}$.
% will tend to have better visual quality in $\Decoder(\z)$ but also higher bitrate. 
%In Eq.~\ref{eq:1}, s
Since all of the functions---$\Coder$, $\Decoder$, $\Distort$ and $\Size$ (which is approximated by a pre-trained NN~\cite{dvc})---are differentiable, the NN weights $\phi$ and $\theta$ can be trained jointly to minimize Eq.~\ref{eq:1}.
%For an input frame \x\x (a c×w×hc\times w\times h tensor), the \aecode is the output of the encoder \y=\Coder(\x)\y=\Coder(\x)  will be sent to the receiver, which then runs the decoder to reconstruct the original frame from \y\y: ^\x=\Decoder(\y)\hat{\x}=\Decoder(\y).



\begin{figure}[t!]
    \centering
         \centering
%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v3.pdf}
%        \includegraphics[width=0.99\linewidth]{figs/per-packet-encoding-v4.pdf}
        %\includegraphics[width=0.95\linewidth]{figs/per-packet-encoding-v5.pdf}
        \includegraphics[width=0.9\linewidth]{figs/per-packet-encoding-v5.pdf}
    \tightcaption{Example of \name's packetization.
    % and per-packet entropy encoding. 
    When a packet is lost, the elements mapped to it will be set to zeros.}
    \label{fig:per-packet}
\end{figure}


\mypara{Simulating packet loss}
Figure~\ref{fig:per-packet} shows how \name splits the encoder's output into individual packets.
\name's sender first splits the encoded tensor to multiple subtensors by a uniform random mapping. We use a reversible pseudo-random function to generate the mapping so that the receiver can correctly recover the original tensor with the same random seed. 
More specifically, we map the $i^{\textrm{th}}$ element to the $j=(i*p\textrm{ mod }n)^{\textrm{th}}$ packet at the $(i*p-j)/n^{\textrm{th}}$ position, where $n$ is the number of packets and $p$ is a prime number.
%\footnote{A reversible mapping allows the decoder to map elements from packets (including lost packets) back to the vector $\z$. An example can be mapping the $i^{\textrm{th}}$ element to the $j=(i*p\textrm{ mod }n)^{\textrm{th}}$ packet at the $(i*p-j)/n^{\textrm{th}}$ position, where $n$ is the number of packets and $p$ is a prime number.} 
%\jc{Yihua, please fill in here. how is the encoded tensor split into subtensors? how is the psuedo random split done?}
If a packet is lost, the decoder will set each element whose position is mapped to the lost packet to zero. 
As a result, a $x$\% packet loss rate will be translated to randomly zeroing $x$\% values in the encoder's output tensor.
\S\ref{subsec:packetization} will explain how each subtensor is losslessly compressed via entropy encoded into the bitstream of a packet, but such lossless compression is bypassed during simulation.
% In practice, each subtensor will then be entropy encoded into an individual packet and sent through the network.
%\jc{Yihua please fill in here}



\mypara{Training loss function}
During training, \name simply simulates packet loss at a rate randomly selected from a distribution of packet loss rates (explained shortly), rather than running a packet-level simulator. \passed{\amz{why not use a simulator? seems like it would introduce the burst-y distribution you explicitly induce later, but perhaps is not differentiable? Might be helpful to explain explicitly, this is one of the big contributions of this section IMO.}}
Given a packet loss rate distribution, \name jointly trains the encoder and decoder NNs to minimize: 
\passed{\yc{maybe we just say we use the simulation for packet losses that is the same as the packetization}}
%which uses a random distribution \loss\loss to simulate the effect of packet loss on the encoder's output:
\vspace{-0.04cm}
\begin{align}
%\textrm{\bf min~~~~} \mathbb{E}_{\x\sim \X} \Quality(\Decoder(\y), \x)\textrm{, where }
%\color{blue}\underbrace{\highlight{blue}{\y∼\loss(\y|\Coder(\x))\y\sim \loss(\y | \Coder(\x))}}_{\text{\sf \footnotesize \textcolor{blue!85}{Simulating packet loss}}}
\mathbb{E}_{\x} \Distort(\Decoder(\y), \x)+\alpha{\cdot}\Size(\y)\textrm{, where }
\color{blue}\underbrace{\highlight{newblue}{$\y\sim \loss(\y | \Coder(\x))$}}_{\text{\sf  \footnotesize \textcolor{blue}{Simulate packet loss}}}
\label{eq:2}
\vspace{-0.04cm}
\end{align}
%where the change is highlighted in color.
The key difference between this and the traditional loss function Eq.~\ref{eq:1} (highlighted in blue) is the distribution function $\loss$, which characterizes the distribution of decoder input under packet loss.
%Given the encoder output \Coder(\x)\Coder(\x), \loss\loss represents the data distribution seen by the decoder. 
%Remember that 
For instance, with a 
loss rate of 33\%, $\loss(\y | \Coder(\x))$ is the probability of $\y$ being the result of randomly zeroing 33\% of elements in $\Coder(\x)$.
 % An example of such random masking between \name's encoder and decoder can be found in Figure~\ref{fig:grace-training}.
% trains its autoencoder and the traditional autoencoder training.
%each \y\y drawn from the distribution \loss(\y|\Coder(\x))\loss(\y | \Coder(\x)) is a result of randomly setting 30\% of elements in \Coder(\x)\Coder(\x) to zeros.

It should be noticed that the random probability distribution $\loss$ may not be expressed as a  function of $\phi$ and is thus not differentiable with respect to $\phi$.
To train the weights in $\phi$, we use the REINFORCE trick~\cite{Kingma2014} to approximate this gradient by Monte Carlo Sampling. This is commonly used in reinforcement learning~\cite{zhang2021sample, peters2008reinforcement}.

\begin{figure}[t]
    \centering
%    \includegraphics[width=0.99\linewidth]{figs/ae-arch-v2.pdf}
    %\includegraphics[width=0.9\linewidth]{figs/ae-arch-v3.pdf}
    \includegraphics[width=0.85\linewidth]{figs/ae-arch-v3.pdf}
    \tightcaption{\name applies {\em random masking} (setting a fraction of randomly selected elements to zeros) to the NN encoder output, whereas the traditional autoencoder training has no data loss between the encoder and the decoder.
    Random masking can be made equivalent to packet loss as shown in \S\ref{subsec:packetization}.}
%    Contrasting the proposed loss-resilient design of autoencoders with traditional autoencoders.}
    \label{fig:grace-training}
\end{figure}



\mypara{Distribution of simulated packet loss rates}
%A key design choice in \name is the function \loss that governs what random data erasure rate the autoencoder learns to handle during training. 
Intuitively, in order to prepare the autoencoder to handle different loss rates, we should simulate a wide range of packet loss rates in training.
% not use a fixed rate of random masking; instead, we should include many different rates of random masking from the range [0, 100\%).
% as it will rarely see 0\% masking, which translates to \rate of 0\%, while 0\% \rate is the common case in practice. 
\name uses the following distribution to pick the simulated loss rate:
with 80\% probability, the loss rate is set to 0\%; with 20\% probability, the loss rate randomly chosen from \{10\%,20\%,30\%,40\%,50\%,60\%\}.
%In \S\ref{subsec:??}, we will compare it with other training distributions of random erasure rate

It is worth some words to explain why we do not choose packet loss rate uniformly from [0, 100\%).
Empirically, we found that if a high loss rate (\eg 90\%) is selected for a great fraction of time, the quality during 90\% packet loss will slightly improve, but it will also hurt the quality at low loss rates. 
This is because the encoder will learn to add more redundant information to prepare for high loss rates and it becomes difficult to learn a decent NN encoder when the loss rate is low.

\myparaq{Why is \name loss tolerant}
% As we will show in \S\ref{subsec:eval:resilience}, the quality of \name's autoencoder degrades much more gracefully than both the standard DVC autoencoders as well as other loss-resilient baselines under different rates of random masking. 
There are two intuitive reasons.
% The jointly trained NN encoder and decoder can tolerate packet loss for three reasons.
(1) The NN encoder output has little stringent dependencies between its elements, so setting elements at random positions is less impactful on the decoding result than in H.265 output. 
(2) We empirically found that the \name-trained NN encoder learns to output more non-zero values than the original DVC, which makes it easier for the decoder to tell which values are affected by packet loss. 
The increased number of non-zero values also means the encoder might learn to add redundancy in the encoded data to allow more accurate decoder reconstruction. 
This is a unique benefit of jointly training NN encoder and decoder. 
This corroborates our empirical result in \S\ref{subsec:eval:micro} that if only the decoder is trained with packet loss (with the encoder weights fixed), the quality will be worse than \name.
% \edit{both added some redundancy to the $\y$ and} allows the decoder to easily distinguish  zeroed (masked) elements.
% (3) \name's training also prepares the NN decoder to recover the zeroed elements from unmasked elements. 
% \name's autoencoder can be intuitively understood as between a traditional autoencoder and generative NNs.
% \S\ref{subsec:eval:resilience} shows empirical evidence that \name exhibits better loss resilience than baselines. 


% However, picking the masking rate uniformly from [0, 100\%) does not work well.

% \jc{need to explain why this particular distribution of simulated loss rates}










==> sections/old/temp_figure.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% TEMPORARY RESULTS %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-queue15delay50.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, queue=15, delay=50}
         \label{fig:queue15-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-delay50.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, queue=25, delay=50}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-queue35delay50.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, queue=35, delay=50}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \vspace{-0.2cm}
     \tightcaption{Delay = 50}
     \label{fig:simulation-queue15}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-queue15.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, queue=15, delay=100}
         \label{fig:queue15-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-normal.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, queue=25, delay=100}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-queue35.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, queue=35, delay=100}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \vspace{-0.2cm}
     \tightcaption{Delay = 100}
     \label{fig:simulation-queue15}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-queue15delay150.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, queue=15, delay=150}
         \label{fig:queue15-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-delay150.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, queue=25, delay=150}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/delay-results-queue35delay150.pdf}
         \caption{SSIM V.S. 95\% tail frame delay, queue=35, delay=150}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \vspace{-0.2cm}
     \tightcaption{Delay = 150}
     \label{fig:simulation-queue15}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-queue15delay50.pdf}
         \caption{SSIM V.S. stall, queue=15, delay=50}
         \label{fig:queue15-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-delay50.pdf}
         \caption{SSIM V.S. stall, queue=25, delay=50}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-queue35delay50.pdf}
         \caption{SSIM V.S. stall, queue=35, delay=50}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \vspace{-0.2cm}
     \tightcaption{Delay = 50}
     \label{fig:simulation-queue15}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-queue15.pdf}
         \caption{SSIM V.S. stall, queue=15, delay=100}
         \label{fig:queue15-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-normal.pdf}
         \caption{SSIM V.S. stall, queue=25, delay=100}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-queue35.pdf}
         \caption{SSIM V.S. stall, queue=35, delay=100}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \vspace{-0.2cm}
     \tightcaption{Delay = 100}
     \label{fig:simulation-queue15}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-queue15delay150.pdf}
         \caption{SSIM V.S. stall, queue=15, delay=150}
         \label{fig:queue15-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-delay150.pdf}
         \caption{SSIM V.S. stall, queue=25, delay=150}
         \label{fig:queue15-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/stall-results-queue35delay150.pdf}
         \caption{SSIM V.S. stall, queue=35, delay=150}
         \label{fig:queue15-psnr-stall}
     \end{subfigure}
     \hfill
     \vspace{-0.2cm}
     \tightcaption{Delay = 150}
     \label{fig:simulation-queue15}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% TEMPORARY RESULTS END %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
         \centering
         %\includegraphics[width=\linewidth]{figs/placeholders/gcc-default-delay.pdf}
         \includegraphics[width=\linewidth]{figs/placeholders/gcc-delay-results-queue25delay50.pdf}
         \caption{SSIM V.S. delayed frame ratio, using GCC}
         \label{fig:normal-psnr-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/gcc-stall-results-queue25delay50.pdf}
         \caption{SSIM V.S. average stall ratio, using GCC}
         \label{fig:normal-ssim-delay}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/sal-delay-results-queue25delay50.pdf}
         \caption{SSIM V.S. delayed frame ratio, using Salsify-CC}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.245\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/placeholders/sal-stall-results-queue25delay50.pdf}
         \caption{SSIM V.S. average stall ratio, using Salsify-CC}
         \label{fig:normal-psnr-stall}
     \end{subfigure}
     \hfill
     \vspace{-0.2cm}
     \tightcaption{Delay = 50, queue = 25 \textcolor{red}{this is on 1 trace, quality of smart baselines is around 9-11)}}
     \label{fig:normal-simulation}
\end{figure*}

